Beyond ELBOs: A Large-Scale Evaluation of Variational Methods for Sampling

Monte Carlo methods, Variational Inference, and their combinations play a pivotal role in sampling from intractable probability distributions. However, current studies lack a unified evaluation framework, relying on disparate performance measures and limited method comparisons across diverse tasks, complicating the assessment of progress and hindering the decision-making of practitioners. In response to these challenges, our work introduces a benchmark that evaluates sampling methods using a standardized task suite and a broad range of performance criteria. Moreover, we study existing metrics for quantifying mode collapse and introduce novel metrics for this purpose. Our findings provide insights into strengths and weaknesses of existing sampling methods, serving as a valuable reference for future developments. The code is publicly available here.

==> figures/visualizations/fashion/fashion_fig.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[]
\begin{tabular}{cccc}
\includegraphics[width=0.32\textwidth]{figures/visualizations/fashion/fashion_gt.pdf} &   
\includegraphics[width=0.32\textwidth]{figures/visualizations/fashion/fashion_mfvi.pdf} &   
% \includegraphics[width=0.32\textwidth]{figures/visualizations/fashion/fashion_gt.pdf} &   
\includegraphics[width=0.32\textwidth]{figures/visualizations/fashion/fashion_fab.pdf} 
\\
$\x_i \sim \target$ &   
MFVI &   
% SMC &
FAB &
\\
\end{tabular}
    \centering
    \caption{The left-most figure shows samples from the NICE model trained on images of the Fashion MNIST dataset. The middle and right-most figure shows samples from different methods trained on the NICE model.}
    \label{tab:my_label}
\end{table}



\begin{minipage}[b]{\textwidth}
\centering
% \resizebox{\textwidth}{!}{%
\begin{tabular}{l|cc}
\toprule
\textbf{Method}   & \textbf{ELBO} $\uparrow$ & \textbf{EMC} $\uparrow$ \\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $-59.86 \scriptstyle \pm 0.055$ % ELBO digits
& $0.000 \scriptstyle \pm 0.000$ % EMC digits
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $-18.66 \scriptstyle \pm 0.156$ % ELBO digits
& $0.231 \scriptstyle \pm 0.118$ % EMC digits
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
% }
\captionof{table}{Preliminary results for the Fashion MNIST ($28 \times 28$) dataset.}
\label{tab:ess}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{minipage}[b]{\textwidth}
% \centering
% % \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cc|cc}
% \toprule
%    & \multicolumn{2}{c|}{\textbf{Digits} $\mathbf{28 \times 28}$} & \multicolumn{2}{c}{\textbf{Fashion} $\mathbf{28 \times 28}$}   \\ 
% \toprule
% \textbf{Method}   & \textbf{ELBO} $\uparrow$ & \textbf{EMC} $\uparrow$ & \textbf{ELBO} $\uparrow$ & \textbf{EMC} $\uparrow$  \\ 
% \midrule
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MFVI
% & $0.000 \scriptstyle \pm 0.000$ % ELBO digits
% & $0.000 \scriptstyle \pm 0.000$ % EMC digits
% & $0.000 \scriptstyle \pm 0.000$ % ELBO digits
% & $0.000 \scriptstyle \pm 0.000$ % EMC digits
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FAB
% & $0.000 \scriptstyle \pm 0.000$ % ELBO digits
% & $0.000 \scriptstyle \pm 0.000$ % EMC digits
% & $0.000 \scriptstyle \pm 0.000$ % ELBO digits
% & $0.000 \scriptstyle \pm 0.000$ % EMC digits
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \bottomrule
% \end{tabular}
% % }
% \captionof{table}{Preliminary results for the Fashion MNIST ($28 \times 28$) dataset.}
% \label{tab:ess}
% \end{minipage}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> figures/visualizations/funnel/aft_samples.tex <==
\addplot [semithick, aft, opacity=0.7, mark=x, mark size=3, mark options={solid}, only marks]
table {%
-2.03298783302307 0.686470031738281
-0.435279428958893 0.68471497297287
-1.21127569675446 -0.268089532852173
-0.519156217575073 0.117427229881287
0.300720572471619 -0.164398342370987
1.87469136714935 -0.919577360153198
1.81062471866608 4.53825998306274
0.46001660823822 -0.255330801010132
-1.2617015838623 0.20254123210907
1.87740671634674 0.22822117805481
-0.997523725032806 0.712787091732025
-0.140437424182892 -0.972960352897644
1.03816187381744 3.80512380599976
0.205196112394333 -0.97324538230896
1.20231521129608 -0.274754494428635
-1.47569966316223 -1.39467442035675
1.80542600154877 -1.08177733421326
3.25579428672791 -1.88024926185608
1.83402693271637 -2.71062612533569
-0.558145344257355 -0.419806301593781
1.11594676971436 -1.64357757568359
4.14303922653198 5.52567005157471
0.822078585624695 2.01965093612671
-0.297097980976105 0.0527881905436516
1.80429220199585 2.93958425521851
1.65467476844788 0.438585788011551
1.12406146526337 0.384450554847717
1.3275101184845 2.16079640388489
-1.73179745674133 0.349447250366211
-1.303879737854 -0.487027078866959
0.825674057006836 0.544466435909271
1.21527433395386 -0.623234391212463
-4.58788394927979 -0.0410120040178299
-2.65600109100342 -0.106653206050396
0.771008908748627 -0.144075304269791
-2.65922164916992 -0.0553749203681946
-0.472820222377777 1.24587547779083
-3.16798138618469 -0.325414806604385
1.84919321537018 1.62555062770844
2.61376309394836 0.57316780090332
-1.42226624488831 -0.806423485279083
2.36390781402588 0.750589311122894
-0.572179019451141 0.190210491418839
-0.0214238651096821 -0.270399689674377
1.56673920154572 2.14307689666748
2.00348711013794 -0.859955251216888
-0.0567137002944946 1.45336437225342
1.24837338924408 -1.42937994003296
-3.06730604171753 0.208860278129578
-0.896633327007294 0.997471332550049
-2.97815203666687 0.150588095188141
-1.9472416639328 0.352723091840744
2.65513968467712 1.4790586233139
0.417967200279236 -0.14349353313446
1.35254526138306 0.952612698078156
0.066877581179142 0.211405545473099
-2.11796832084656 -0.812283635139465
0.512697517871857 0.291849911212921
-0.445902645587921 0.0126395002007484
-1.14027976989746 0.469090402126312
0.867624342441559 -5.05445861816406
1.35451209545135 0.334775269031525
0.642303586006165 1.54186272621155
-2.8380708694458 -0.267165213823318
-1.92457807064056 0.663145840167999
-0.911755979061127 0.69501006603241
0.0804260969161987 1.16459894180298
1.72359561920166 -3.17539048194885
0.300908446311951 0.584139764308929
-4.52628755569458 -0.123398959636688
-1.57160699367523 -0.422845005989075
2.07754898071289 -1.42287623882294
0.735682249069214 0.019399106502533
2.74509954452515 -6.29564666748047
1.63553607463837 1.06207633018494
1.32378625869751 -1.70323538780212
-1.92477881908417 -0.293253600597382
1.77688419818878 0.107629388570786
0.20069245994091 0.633831799030304
1.66746747493744 0.119271650910378
0.566105723381042 -0.0341865979135036
1.10128903388977 -0.231907993555069
-0.57605767250061 0.428739964962006
1.50592696666718 -2.3173668384552
-0.969506561756134 0.0566605217754841
-3.27458953857422 -0.0518908947706223
1.81094765663147 -0.306424885988235
1.36901903152466 1.73182141780853
1.26354074478149 -1.97945189476013
2.00461411476135 -1.28857409954071
-3.73766565322876 0.175119057297707
0.953901648521423 -0.799215972423553
1.85279190540314 3.77260780334473
0.86572653055191 2.71445751190186
2.64616727828979 1.20710957050323
-0.18713441491127 0.895259439945221
-0.706678628921509 -0.257688283920288
1.29798746109009 -1.37143266201019
1.60644376277924 4.63637638092041
-0.49578595161438 0.158297553658485
0.282050848007202 1.17870616912842
0.397119700908661 0.901522815227509
-0.992416858673096 -0.0178595259785652
-2.08649682998657 -0.197672814130783
-0.747068703174591 0.694810569286346
-3.74950528144836 0.129817143082619
-4.11768817901611 0.120348572731018
0.236106231808662 -0.78939026594162
-2.89601111412048 -0.0460522696375847
1.30694580078125 -1.68405592441559
-0.943923711776733 -0.0685983002185822
-1.2656581401825 -0.36760276556015
1.36031055450439 -0.858959913253784
1.07848680019379 1.77916884422302
-0.380833566188812 -0.0319610685110092
-3.94382047653198 0.141263052821159
1.46663057804108 -1.42834007740021
1.78961825370789 -7.97542476654053
-1.56588339805603 0.187308996915817
-1.84932744503021 1.01157808303833
2.40121936798096 2.78076863288879
1.23356926441193 3.16059684753418
1.70298826694489 0.555757284164429
0.98569130897522 0.0080098919570446
2.00268244743347 0.893218159675598
0.412613570690155 0.0908186733722687
0.501614332199097 0.482591301202774
-1.82295739650726 0.295967698097229
-0.199622735381126 -0.42241570353508
-1.3116307258606 0.863381028175354
1.82978439331055 0.636498272418976
-3.08405709266663 -0.199110090732574
2.43847131729126 2.47027468681335
0.803285717964172 -1.84212386608124
-2.87568473815918 0.233507573604584
-0.0843639820814133 -1.46059226989746
0.648902297019958 2.18360733985901
0.488010287284851 -1.81407225131989
2.05238699913025 2.83628845214844
0.647940754890442 -0.775200843811035
-0.0119656026363373 -1.83968269824982
-3.01652121543884 0.253907918930054
-2.9607412815094 0.0659834668040276
2.17584824562073 -5.72240877151489
2.0751268863678 2.07007813453674
1.28674232959747 -2.80280709266663
1.84897494316101 0.0721411406993866
1.25936460494995 1.03978192806244
0.0328795909881592 -1.11932551860809
1.98232734203339 1.57062447071075
-0.0484526231884956 -0.179692938923836
0.84177178144455 0.788819789886475
-3.13475012779236 -0.299157232046127
1.62543213367462 -0.849499225616455
-1.09392130374908 0.412663161754608
1.16446912288666 0.572999536991119
-2.15540480613708 0.354296654462814
0.506140291690826 -0.45281845331192
-0.772105157375336 -1.0128515958786
-4.0730128288269 0.114563621580601
-2.68077802658081 0.378218740224838
-0.218006730079651 0.878707408905029
-1.56876397132874 0.290938496589661
-1.77640056610107 0.487184137105942
0.964741826057434 2.79922962188721
0.0362950637936592 0.104914858937263
-5.53306818008423 0.012929399497807
-1.27412903308868 -0.0622849725186825
-4.69491672515869 0.153645381331444
-0.112315803766251 -1.27470445632935
-0.390931248664856 -0.287016570568085
-4.46477508544922 -0.00508048199117184
-1.25937902927399 0.721587598323822
0.634556770324707 -0.298951327800751
-1.22179961204529 0.0715571120381355
0.014591314829886 1.82647848129272
-1.98181164264679 -0.15224577486515
-1.07537579536438 -0.301157593727112
-4.85726594924927 0.118629492819309
0.656292617321014 1.41027534008026
-3.72369289398193 0.0569576621055603
2.07894992828369 -1.37451899051666
-3.47737383842468 0.0538915991783142
-1.76568496227264 -0.349060773849487
-0.544130861759186 -0.210092753171921
-0.137929081916809 1.24639558792114
1.83343613147736 -5.09319734573364
-4.19501829147339 0.126392781734467
-1.06950032711029 -0.0274386070668697
3.19451475143433 -1.0190315246582
0.768249750137329 -2.20170426368713
-2.08408284187317 0.107950612902641
-2.41240525245667 -0.0925993621349335
0.64961177110672 -1.59373092651367
1.34189796447754 3.23008179664612
-0.759699642658234 0.0132882297039032
-2.92574501037598 0.0503377243876457
-1.66422927379608 -1.20121741294861
-0.518030345439911 0.551796138286591
-0.42846804857254 0.259623885154724
1.20495998859406 2.12739896774292
1.7539986371994 -5.7607364654541
-1.35414552688599 -0.123491674661636
-1.1520893573761 -0.432517498731613
-0.713808178901672 0.0433180183172226
2.69062042236328 -2.11965799331665
2.18012380599976 -2.92630124092102
-2.08576917648315 0.262779831886292
-3.59295225143433 -0.0432403460144997
-1.97499251365662 -0.282813906669617
0.643979907035828 -1.20610213279724
-1.55257868766785 -0.0751828625798225
2.05626678466797 -1.22133409976959
-0.677221477031708 0.47032505273819
-0.70258092880249 -0.252223670482635
-1.19169402122498 0.0982940122485161
-0.37036606669426 1.3385044336319
1.71177613735199 -1.17219185829163
2.23565340042114 -4.07296180725098
0.185536801815033 0.632715702056885
2.18130207061768 3.27589702606201
-2.00316858291626 0.223181307315826
-1.54916322231293 0.295078247785568
-0.40386226773262 0.403891146183014
0.355408489704132 -2.53009819984436
-0.80647349357605 -0.0247625857591629
-0.681961417198181 0.366960912942886
0.920208275318146 -1.65720653533936
1.75620257854462 -0.0291614532470703
0.749932765960693 2.90423059463501
0.528626263141632 2.16391015052795
-0.348471581935883 0.0495931319892406
-3.01384687423706 -0.357323348522186
-1.44821393489838 -0.139692187309265
1.14881932735443 0.621534287929535
-1.24229371547699 -0.680651247501373
-0.183162957429886 -1.05686664581299
-0.406274974346161 0.788754105567932
0.393742978572845 -0.411727726459503
2.91274428367615 4.64205598831177
3.99170088768005 -4.66754817962646
-0.396000266075134 0.496970415115356
-0.971666693687439 0.91436094045639
1.18419647216797 -2.04463124275208
1.19475162029266 0.131432294845581
2.21905422210693 1.20901393890381
0.632475435733795 0.690344393253326
-0.0581145063042641 -0.910699784755707
0.303514540195465 -0.308106303215027
-5.15284585952759 -0.0032978430390358
0.282502800226212 0.194804191589355
2.03577423095703 2.72319626808167
-2.09779977798462 0.245334878563881
2.75397872924805 3.7392909526825
-2.03963375091553 -0.000598505139350891
0.00642192363739014 0.249340653419495
1.10440576076508 0.362885624170303
2.07317304611206 -6.29687881469727
0.571830928325653 -0.644810914993286
0.713555037975311 0.0701855272054672
-0.202751636505127 0.962386131286621
-1.06723439693451 -0.779431700706482
-0.352131545543671 -0.789147794246674
1.35001873970032 -1.36830520629883
0.0715756565332413 -1.31910622119904
0.248699799180031 -0.218546897172928
-0.626743853092194 0.0882571786642075
0.783443927764893 -1.22372257709503
2.30158352851868 -0.543070375919342
1.78751659393311 2.01704025268555
-1.53014147281647 0.871641218662262
0.479611605405807 -1.20371842384338
-4.93984174728394 -0.0166672170162201
-1.39072930812836 0.441493570804596
-0.982428133487701 0.775603294372559
-1.1278977394104 -0.709079384803772
-1.8592187166214 0.102405667304993
0.0886052250862122 -0.0660723447799683
-1.0260763168335 -0.359025359153748
0.670198023319244 2.12087416648865
-0.685874462127686 -0.402363210916519
-3.31826210021973 -0.244278699159622
0.0176325514912605 -0.721243143081665
1.21298027038574 1.84161484241486
0.533465147018433 0.678414106369019
-0.217262804508209 -0.118746116757393
-0.553094089031219 0.337149202823639
1.38867390155792 0.679836750030518
-1.08163452148438 -1.69879102706909
0.671391069889069 0.151821985840797
0.452410817146301 3.13036727905273
-0.107465088367462 0.394596934318542
3.65908670425415 0.36240342259407
2.12145638465881 1.24709987640381
0.35928750038147 -0.111807465553284
-0.174302592873573 -0.422283679246902
-3.87732005119324 0.146183416247368
-0.530093669891357 -1.24242281913757
-2.28839302062988 -0.00528165325522423
1.47943925857544 -0.125805258750916
-3.0177013874054 0.158175423741341
-1.77431726455688 0.0203706584870815
0.59197610616684 -0.919354677200317
2.24000692367554 2.34605860710144
-1.15896475315094 -0.00404581427574158
0.0292124301195145 0.485938131809235
2.07433533668518 2.32916831970215
0.075639396905899 0.0147264152765274
0.306119412183762 -0.367307245731354
1.22533440589905 -2.09277749061584
-3.11037349700928 0.187472522258759
1.60878133773804 -1.95078670978546
1.84897804260254 2.897216796875
1.94942021369934 -0.519030928611755
-0.610515773296356 -1.31868243217468
0.340901404619217 -2.0496199131012
1.58256328105927 -2.56470274925232
-1.32111537456512 0.184418261051178
0.309558212757111 -0.368055284023285
-3.36023950576782 0.0569508969783783
-1.08300530910492 0.152801513671875
0.749649286270142 0.0839948728680611
-1.24042356014252 1.28879523277283
-0.0419853068888187 1.07479071617126
3.84424066543579 4.27927207946777
-3.01225113868713 -0.0947789251804352
-2.198410987854 0.230497345328331
0.320974856615067 -0.236075609922409
-0.544552683830261 1.36644744873047
1.27184438705444 -1.89131343364716
-0.371795773506165 2.16432166099548
-0.967534780502319 -0.0405576601624489
1.38844811916351 -0.876057803630829
1.58861541748047 -1.7621386051178
-0.920542299747467 -0.322986125946045
-3.28141188621521 -0.25719341635704
-2.26441836357117 0.339796721935272
-0.201469004154205 -0.644771099090576
-2.79369163513184 -0.129069119691849
-2.24254560470581 -0.437921822071075
-1.31437540054321 0.185738235712051
-2.5612165927887 -0.14703257381916
2.50618982315063 0.056268785148859
-1.42123210430145 0.0660721138119698
-2.38859176635742 0.448881059885025
0.654566168785095 1.63985466957092
2.2793390750885 2.06578254699707
-1.98009407520294 0.490015923976898
0.332129210233688 -0.0210258550941944
0.801274299621582 1.66993749141693
1.00996911525726 1.95666563510895
-0.89685469865799 0.423036217689514
-3.61160373687744 0.00132023543119431
-1.01132810115814 0.0283334255218506
1.14718961715698 -0.00644923746585846
0.283594250679016 0.811715841293335
1.1253889799118 1.3420307636261
-0.837970018386841 -0.158460482954979
-0.142960771918297 -0.791610598564148
1.15208256244659 3.95768737792969
-1.70777547359467 0.252941012382507
-3.33714008331299 -0.0581747815012932
2.0846312046051 1.12018227577209
-1.05037271976471 -0.361418604850769
-1.8486602306366 0.319117426872253
0.700610339641571 -1.08291804790497
-0.0343261696398258 -0.253738641738892
1.58365845680237 -1.38239431381226
0.434897422790527 -1.58086228370667
-0.250542223453522 -0.0119780898094177
-3.64018869400024 0.0708652287721634
-1.26339554786682 -0.817788064479828
-1.08320009708405 0.210936576128006
-0.0704165250062943 -0.520594418048859
0.802305161952972 -1.41589629650116
1.62908816337585 2.58291101455688
-0.336853444576263 0.641464114189148
0.660493135452271 -0.684667408466339
1.14914667606354 0.000550834462046623
1.81503617763519 0.197099566459656
-0.461204767227173 -2.06263065338135
0.106957621872425 0.158712401986122
-0.426753312349319 0.876953065395355
-0.415515810251236 0.232054352760315
-3.28015160560608 -0.0247429683804512
-2.97868609428406 -0.0241900198161602
0.00312176719307899 0.889961898326874
1.09281504154205 0.805076539516449
-1.08373093605042 0.248296067118645
1.42710196971893 -1.09813094139099
-1.99449801445007 -0.420395076274872
-4.9279899597168 -0.0914739966392517
-0.662848591804504 -0.411210030317307
0.797565400600433 0.308940470218658
1.97194051742554 4.84156322479248
-2.59616756439209 0.0998974740505219
0.559869825839996 2.40745377540588
-0.231575608253479 0.646053612232208
0.0294812768697739 -0.988251090049744
1.67929792404175 -2.32802391052246
-0.693686842918396 -0.85962575674057
0.689947724342346 0.645590543746948
1.1042388677597 2.17538738250732
-1.27786111831665 0.0502055883407593
1.13640296459198 -2.223881483078
2.90196800231934 1.6166387796402
-3.07881951332092 0.074583612382412
1.23885989189148 2.4237585067749
-2.72835326194763 -0.322530150413513
0.834155440330505 0.724092662334442
-1.96566426753998 0.65458470582962
-0.632764935493469 -0.229343071579933
-3.02472257614136 -0.0224444046616554
-0.217167437076569 -1.20167112350464
1.65082657337189 -0.3462755382061
0.698423743247986 -1.09664678573608
0.106813877820969 -0.124259933829308
-1.95919620990753 -0.911093831062317
-3.19312238693237 0.0996391549706459
0.781224250793457 0.868420958518982
0.234425455331802 -1.30764138698578
-3.89005279541016 0.0891107469797134
2.14179921150208 3.13341307640076
-0.884158611297607 0.911394238471985
1.4200165271759 1.53384506702423
-1.94687843322754 -0.526542186737061
-1.46754884719849 0.449548721313477
2.1848578453064 0.231932744383812
-4.78022336959839 -0.142468631267548
-3.35074305534363 -0.0131443710997701
1.13116705417633 -1.78117311000824
1.39816951751709 -0.505598127841949
0.500723838806152 0.878232002258301
1.06781280040741 -0.980857491493225
-3.10665082931519 0.0905238538980484
2.2768816947937 0.162120342254639
-0.131540194153786 0.89749151468277
1.17820191383362 -0.803312838077545
0.564138770103455 -0.194594264030457
0.0382078848779202 1.06688582897186
-0.882679998874664 0.275457143783569
-0.981991231441498 -0.591397345066071
2.36661624908447 0.581729829311371
0.660921454429626 -1.69689500331879
0.765816807746887 -1.15457439422607
-4.24720096588135 0.0876615419983864
2.65933656692505 -3.41367316246033
-0.374097585678101 0.458462446928024
-1.95007538795471 0.310185462236404
-0.995749473571777 0.900206089019775
-0.889722049236298 0.48961552977562
-3.96089959144592 -0.0511511713266373
-1.77905929088593 -0.0602535381913185
1.77893626689911 0.000418465584516525
1.47795057296753 1.12306880950928
0.525995671749115 -1.26596260070801
-2.56207728385925 -0.361336141824722
-2.9221453666687 0.282830327749252
0.800566971302032 -2.24235916137695
1.92917108535767 -3.81985187530518
0.198486611247063 -2.02642726898193
-2.76636385917664 -0.285955965518951
0.34216383099556 1.41229617595673
1.93855905532837 -1.9470808506012
-3.12843656539917 -0.395428597927094
-1.14981412887573 -0.145045474171638
1.18865931034088 1.56829285621643
-2.4539783000946 -0.627882540225983
0.577424764633179 0.0782343596220016
-1.77802073955536 -0.022686704993248
-2.35155844688416 -0.173670172691345
-1.57474684715271 0.44236621260643
1.30607855319977 1.65136694908142
2.17823600769043 -2.9607253074646
-0.182675987482071 -0.0424433499574661
0.525424420833588 -0.166121542453766
-0.0157887972891331 0.19531437754631
-0.989834606647491 -0.0156726315617561
-1.30806088447571 -0.0176352709531784
1.28127670288086 -0.0237580724060535
0.204859673976898 0.66051572561264
1.11952030658722 -0.925688982009888
0.789690315723419 -1.11281728744507
2.46771955490112 2.92954230308533
-0.663469135761261 1.59920430183411
0.498049706220627 0.642983555793762
-0.913664221763611 -0.770523309707642
0.399409383535385 0.477778226137161
-0.525286614894867 0.732994258403778
3.07832264900208 4.49440050125122
-3.73179507255554 0.110135048627853
1.8194432258606 1.52099668979645
0.846412360668182 -1.00802266597748
1.06364452838898 2.23577427864075
-2.49178385734558 0.127206280827522
-0.426089942455292 -0.683465242385864
0.686952412128448 0.670580089092255
3.75223779678345 4.3490514755249
-3.54568076133728 -0.121796555817127
-0.554075539112091 0.402155131101608
0.586708188056946 -1.28569066524506
0.992896854877472 2.84332466125488
-2.58763861656189 0.229229614138603
0.537521183490753 2.06845426559448
-0.519501924514771 0.426105082035065
0.001908078789711 0.925215303897858
1.0324718952179 -2.76222515106201
2.0232048034668 3.4167377948761
0.558763742446899 0.836768627166748
1.67329668998718 0.950364470481873
1.50297236442566 -0.393110305070877
-0.452128529548645 1.84435343742371
-0.939094126224518 1.35140693187714
2.79113531112671 -0.964847505092621
3.04627776145935 -2.74645495414734
-0.0758346617221832 0.0875835940241814
0.871778428554535 0.695481956005096
-1.40383565425873 -0.626780569553375
-0.138938903808594 -1.67291581630707
-0.300057083368301 -0.925665974617004
1.86851131916046 -4.06750869750977
-0.838127553462982 -0.198579102754593
-1.94203531742096 0.00011887401342392
1.61576557159424 1.31217789649963
0.962666690349579 2.67477107048035
0.526921629905701 1.45044553279877
-1.03370034694672 -0.00950078666210175
0.239460781216621 -0.437597006559372
-2.32632160186768 -0.112140737473965
1.37256693840027 1.13092863559723
0.53179806470871 -0.0549570582807064
1.98915636539459 -1.06246185302734
-0.102241471409798 0.540264189243317
-1.89820575714111 0.293851912021637
0.717870473861694 1.83754861354828
-2.46627926826477 -0.120819300413132
-2.84932470321655 -0.158237412571907
2.12172293663025 0.918386995792389
0.990005433559418 -1.79360258579254
0.660928845405579 -0.898604035377502
-1.95649862289429 -0.35053563117981
-0.197526812553406 -0.907407879829407
-1.27902138233185 0.303578466176987
-1.68488585948944 0.246193051338196
0.014588750898838 -0.30924379825592
-1.49647879600525 -0.00915220379829407
-2.27075362205505 -0.107779130339622
0.695089399814606 -0.172050729393959
-0.386660039424896 -2.33902955055237
2.49865746498108 -0.813628137111664
-2.55112552642822 -0.0809883698821068
2.74451017379761 3.79695844650269
2.40373039245605 -6.87796688079834
1.69539403915405 0.852632284164429
-0.220753148198128 -1.12655675411224
-2.24608778953552 -0.386081218719482
1.59173774719238 -1.49567532539368
1.00125551223755 1.02641558647156
0.021298736333847 -1.5628787279129
1.38307881355286 -0.107545077800751
0.831311821937561 1.4576518535614
-0.963747382164001 -0.389725685119629
-1.21395230293274 -0.431817680597305
-0.35098397731781 0.276236236095428
1.56549954414368 0.339048057794571
0.228372201323509 0.957555890083313
0.890958845615387 0.0773682147264481
-0.740247786045074 0.378686398267746
-0.00294847786426544 0.112866699695587
-0.597583770751953 0.176971703767776
-0.611279845237732 -0.474451661109924
0.682294249534607 0.336629062891006
1.00301933288574 3.09554696083069
-2.42514610290527 0.513156712055206
-2.18217492103577 0.155459895730019
-1.29695010185242 0.168551728129387
-3.7203106880188 -0.19019603729248
-2.26456451416016 -0.730732321739197
-0.831050395965576 -0.889686226844788
0.0230189487338066 1.2347571849823
-2.49030756950378 -0.2353835105896
1.3559947013855 -1.16038334369659
0.525758802890778 -0.544151842594147
0.759259700775146 1.1130359172821
-0.0991861969232559 -1.97121787071228
0.548822283744812 -0.389372706413269
1.52480459213257 -2.74797916412354
-2.1875467300415 0.455540478229523
0.414641708135605 -1.53441762924194
-0.620097100734711 -0.121537208557129
3.26408362388611 -3.87412858009338
2.14012145996094 2.27889633178711
-2.07980346679688 0.282877087593079
1.5337347984314 -0.504536926746368
-0.926601946353912 -0.763518214225769
-1.34829235076904 -0.639959752559662
-1.75753617286682 -0.760519206523895
-1.08278656005859 -0.83158016204834
0.327953457832336 1.30685341358185
-0.756921231746674 -0.201337605714798
-0.0308166220784187 0.797771394252777
0.04097580909729 1.16715562343597
1.79902362823486 4.12593746185303
-0.474476277828217 0.146984174847603
-0.762914717197418 -0.00746816582977772
0.584930598735809 -1.37677490711212
-4.20176267623901 0.0879241600632668
-0.791538536548615 1.47717893123627
-2.88477349281311 0.484947144985199
-0.581406116485596 1.01905882358551
-1.98901784420013 -0.295591324567795
-0.0981766879558563 -1.66089713573456
-0.205413058400154 -1.62635183334351
-0.172024458646774 -0.67581981420517
-2.18166780471802 0.235652387142181
-4.63925886154175 0.101174421608448
-1.86389696598053 -0.0731738805770874
-1.59871053695679 -0.38906466960907
2.41137623786926 0.651634335517883
-2.16201186180115 0.258110582828522
-0.540665745735168 1.04067182540894
-0.0672559440135956 -2.3138792514801
0.622767627239227 -2.69270801544189
-0.353084892034531 0.300110399723053
1.95683896541595 1.46386623382568
-2.78750371932983 -0.243684962391853
-2.7558901309967 -0.420962184667587
1.37362229824066 -0.844798922538757
1.37294268608093 -0.542648732662201
1.14425814151764 -2.67331862449646
1.15906298160553 0.10812309384346
1.7317967414856 -1.92310976982117
-1.26986980438232 0.64641922712326
0.582020282745361 0.19869838654995
0.785076439380646 -1.7496463060379
2.76225447654724 3.03663659095764
-1.04909038543701 0.507035911083221
1.19783711433411 0.21223658323288
1.70020031929016 0.95311576128006
-0.233189165592194 1.08686292171478
-3.99827480316162 -0.269663423299789
-0.49535921216011 0.182839184999466
-3.30310916900635 -0.271179676055908
0.0685591548681259 0.602656126022339
0.409658312797546 -1.2894504070282
1.40096485614777 1.12098634243011
-2.70526576042175 -0.0305287539958954
2.55415177345276 -1.39833641052246
0.0376952812075615 1.11543166637421
2.07653141021729 -1.80510199069977
-1.2205513715744 0.376597315073013
-2.2464075088501 -0.787127435207367
-4.28769969940186 0.0680645778775215
-0.102760910987854 -0.0268841926008463
1.39487183094025 -2.99566698074341
1.61899924278259 -5.32563781738281
-0.787902176380157 0.384572386741638
-1.13778448104858 0.660094857215881
0.410180568695068 2.21406817436218
-0.0953554883599281 0.300856739282608
-0.796886265277863 -0.0445363223552704
-3.85715222358704 -0.159348964691162
0.793661177158356 -0.00386496633291245
-0.341927826404572 -0.541620135307312
-0.391768574714661 1.20131194591522
1.00352764129639 -2.381192445755
-0.418148159980774 -0.933635592460632
-0.751779198646545 -0.236468508839607
-2.83910059928894 -0.198290407657623
-3.2269344329834 0.0423682183027267
-3.01200246810913 -0.0376525670289993
-2.20756077766418 -0.189409255981445
-0.517558872699738 -0.176922231912613
-0.587324023246765 -0.81128716468811
-1.33307123184204 0.635259211063385
-3.08002090454102 -0.115796864032745
-1.82498848438263 0.438599914312363
-0.628606557846069 0.705406248569489
0.30217444896698 -0.123797751963139
1.4666246175766 -0.445239961147308
2.27416110038757 -1.89752590656281
-2.80213928222656 -0.199745401740074
0.223426938056946 -2.53301525115967
0.114357106387615 -0.728490352630615
-4.69799423217773 -0.163530275225639
2.05891227722168 4.80164766311646
-4.70757818222046 -0.102066680788994
-1.71594953536987 -0.382708728313446
-3.78594040870667 0.0199622008949518
2.94385433197021 -4.59052181243896
-1.61837184429169 -0.786651134490967
-1.98299121856689 0.451419413089752
-0.160590127110481 0.530206680297852
1.44581663608551 -0.983363330364227
-1.76038289070129 -0.930071830749512
-1.42221617698669 0.128945395350456
-0.296064287424088 0.235490068793297
0.741439878940582 -2.49166584014893
0.704624831676483 0.57419615983963
0.810933768749237 -0.246678948402405
-1.54259777069092 -0.206677347421646
-1.18412411212921 -1.26689922809601
-1.83653390407562 -0.366786658763885
-1.10347080230713 -0.936697363853455
-0.388514280319214 0.265247941017151
0.910960555076599 0.59555447101593
-0.37692528963089 -1.47921359539032
0.494440674781799 3.71826601028442
1.48852872848511 -4.48904991149902
2.17256569862366 -3.27080297470093
-3.58460664749146 -0.299575299024582
0.713812410831451 -2.20266842842102
-1.95932006835938 0.51358836889267
-2.44299387931824 0.247600391507149
-0.739235460758209 -0.409562110900879
1.56610691547394 1.25396656990051
2.10799288749695 0.956523001194
1.09740996360779 0.667502999305725
-0.787633061408997 0.408295631408691
-1.72385370731354 0.506847262382507
-3.90298318862915 0.0761218890547752
-2.31931734085083 0.809383809566498
-1.40510702133179 1.15035438537598
-1.57909548282623 0.57662558555603
0.276429682970047 -0.0469275712966919
0.740289807319641 -1.70587706565857
-3.69289469718933 -0.0297042801976204
-0.498404979705811 -0.423919856548309
-2.77435255050659 -0.119602724909782
-2.24474406242371 0.268431216478348
-1.70193469524384 0.0338407009840012
0.581982254981995 0.695060789585114
2.30599355697632 -4.30084180831909
1.01351821422577 0.148857489228249
1.34272658824921 -1.12129771709442
-2.2373743057251 -0.314731925725937
-0.490264028310776 -0.526657283306122
-1.86224353313446 -0.769911646842957
1.65193271636963 0.621174335479736
0.653849124908447 -2.5134961605072
-2.25532341003418 0.272199213504791
0.185524195432663 0.257840842008591
1.71288979053497 2.31498122215271
-2.82448697090149 -0.0907910466194153
1.8278876543045 -2.16893982887268
-2.21524739265442 -0.385013937950134
1.08323073387146 0.112099997699261
1.33082020282745 1.11268651485443
3.21255230903625 -1.33041226863861
-1.64155757427216 0.747849225997925
1.95078802108765 -0.491637051105499
-0.409089297056198 1.34246420860291
0.861090898513794 2.58749914169312
2.31308722496033 -2.0642728805542
2.44497346878052 4.0740761756897
-2.15171313285828 0.251960933208466
0.999123930931091 -1.35841178894043
-0.847473680973053 -0.548781275749207
1.2041472196579 -1.55847251415253
-0.865198135375977 -0.869639098644257
-0.205792337656021 0.546000957489014
-0.319698452949524 -1.23563182353973
-1.29913377761841 -0.720832347869873
-4.00265073776245 0.0399786382913589
0.722352206707001 0.95256906747818
-1.47651410102844 -0.060723677277565
1.30715692043304 0.484693467617035
0.161169499158859 -0.715548694133759
-1.89292061328888 0.0380844473838806
2.71207499504089 -0.975314915180206
-1.1205381155014 -0.098766528069973
-0.798231244087219 0.6751988530159
-0.333497583866119 0.692816138267517
-2.32658767700195 -0.215104773640633
0.704920172691345 -3.17408752441406
0.540068686008453 -0.792201340198517
-1.06859624385834 1.19525563716888
0.0679350346326828 0.582082867622375
-1.90473663806915 -0.367158889770508
0.54481703042984 0.200882226228714
-3.27206206321716 -0.346331894397736
-0.745509088039398 0.188444212079048
0.100524552166462 -0.463029772043228
0.468449592590332 0.333355277776718
-2.01172232627869 -0.262055963277817
-1.07824158668518 1.01006066799164
0.282938063144684 -1.47253942489624
-1.04162085056305 -0.0801902040839195
1.67881286144257 -0.0757122933864594
-0.636036336421967 -0.620643496513367
-0.48181676864624 -0.994950771331787
0.120366871356964 0.943968713283539
1.5421849489212 -1.51914381980896
-3.53300833702087 0.138543635606766
1.19773030281067 0.642167687416077
1.72350990772247 -4.93294525146484
-0.12359020113945 -1.8658539056778
1.23488509654999 0.00953507609665394
-0.330624103546143 -0.910333514213562
0.210798367857933 1.97278106212616
0.876188814640045 -0.703766465187073
0.458254218101501 1.22337019443512
-1.15790748596191 0.178753778338432
1.14278399944305 -1.38762962818146
1.72459530830383 -2.32965302467346
-3.03987336158752 -0.237772703170776
-3.28400468826294 -0.093180276453495
1.13355481624603 1.84652209281921
-3.07346487045288 0.289165437221527
-2.52452421188354 -0.185904070734978
-1.20817399024963 -0.827668368816376
-1.780597448349 0.344764977693558
1.97086453437805 1.51879584789276
0.52071076631546 -1.07896494865417
2.33488774299622 -1.2757955789566
-0.479578912258148 -0.247650593519211
0.152711495757103 1.04901385307312
1.08683216571808 1.9212771654129
-3.81730031967163 0.0440503060817719
1.59859800338745 -1.66673386096954
0.263553977012634 -2.49974489212036
1.68733751773834 -2.30202412605286
1.22354423999786 -2.18170213699341
1.39170444011688 -1.80507493019104
-3.65337920188904 0.0726229101419449
2.42839932441711 -3.02497506141663
0.845269799232483 0.19948123395443
2.12543845176697 1.46913385391235
-0.635239362716675 1.58081650733948
-2.82155466079712 -0.335255742073059
-0.0147288795560598 0.665197551250458
0.708337783813477 2.62864804267883
-3.03645372390747 0.0433853641152382
-0.558677732944489 2.13579797744751
2.49166798591614 -2.69955658912659
-0.354636967182159 -1.26564788818359
-0.546148478984833 0.614576041698456
2.76680064201355 -0.890073835849762
2.17194437980652 1.87516188621521
-0.876095116138458 -0.528961777687073
-0.751751661300659 0.250985354185104
1.4977490901947 -0.88953161239624
1.81865012645721 0.278482556343079
0.084494024515152 0.921744346618652
-0.0578283369541168 -0.417020499706268
0.654816389083862 0.00478854402899742
-1.51749467849731 0.110802948474884
-0.551079869270325 1.69443821907043
-0.114838629961014 1.63068234920502
0.0626030117273331 -1.29851639270782
0.0325503498315811 0.779116034507751
1.59270942211151 -0.0527590066194534
-0.992349565029144 -0.13299497961998
2.39328408241272 -2.54524254798889
-1.37834906578064 0.59513795375824
-1.66337704658508 -0.0769519880414009
-4.14059686660767 0.213924795389175
-0.439531296491623 -0.332387089729309
-1.00972390174866 0.570545971393585
-0.807081699371338 -1.58121573925018
1.96302819252014 0.590217232704163
-0.116525381803513 0.865822911262512
-0.644427895545959 -0.990451157093048
-1.29478251934052 -0.931888461112976
0.874166011810303 3.99314188957214
1.75863122940063 2.96478652954102
3.10375118255615 3.99173188209534
-2.25247359275818 -0.578699469566345
-1.39325380325317 0.598463714122772
-0.40964287519455 0.971222102642059
-2.57532382011414 0.362794816493988
0.0600443631410599 2.21417927742004
0.773275911808014 -0.397699266672134
-0.312264233827591 -1.01352655887604
-1.07484567165375 -0.199417471885681
1.47940683364868 -0.201330780982971
-2.93326354026794 -0.0183471105992794
4.18130207061768 -2.83718681335449
-1.92843973636627 0.510392963886261
1.10681700706482 -3.87791299819946
1.18841695785522 2.3619339466095
-3.17636728286743 -0.118961155414581
0.0248008072376251 -0.260640263557434
1.88267016410828 -1.95960450172424
-0.0834940299391747 -0.424275755882263
-3.09607481956482 -0.245405524969101
-1.85882139205933 0.571037948131561
-0.921606481075287 0.186083436012268
-0.93582820892334 0.565002977848053
-2.18731045722961 0.0572262853384018
-4.41109561920166 -0.230356529355049
-0.798054695129395 0.823294639587402
0.0020008273422718 -0.173065155744553
-1.39669513702393 0.780658781528473
1.92075061798096 -1.6000542640686
1.07679426670074 -4.71273279190063
1.55352222919464 -1.52936136722565
0.848251760005951 1.15451455116272
0.448837786912918 0.258596122264862
0.617718160152435 -1.61609888076782
-0.0863673910498619 0.371905297040939
1.34819328784943 0.304119825363159
-1.69873213768005 0.14739952981472
-0.940003871917725 -0.92402857542038
-0.514562904834747 -1.13297367095947
-0.493730396032333 -0.403151333332062
-2.07792353630066 0.00411792099475861
-0.236314862966537 0.469508945941925
-0.00202196836471558 -0.0824164301156998
-1.15484750270844 0.479863524436951
-1.15790724754333 -1.34552240371704
-0.980734169483185 -0.330681681632996
-1.51623952388763 0.543267011642456
2.29259061813354 0.652794599533081
0.897207617759705 2.03391146659851
1.98767161369324 2.9468719959259
0.348010212182999 -0.536634802818298
1.86084640026093 -2.92176556587219
-0.341224640607834 -0.550646841526031
0.342411518096924 0.304123997688293
0.257098823785782 -0.0220825895667076
-0.0972273647785187 0.16329899430275
-0.8437539935112 1.07035660743713
-0.795350849628448 -0.160605311393738
-1.8961375951767 0.0234487950801849
0.610217988491058 0.629979491233826
0.637008965015411 -0.945124685764313
2.16974401473999 1.12173402309418
-1.55452561378479 0.064277209341526
1.66562259197235 -0.187123984098434
0.175159052014351 -1.30837821960449
-1.27625465393066 0.439978241920471
-0.20987731218338 0.85023421049118
-3.3169858455658 -0.114886470139027
-2.81149959564209 0.130827978253365
-1.95355546474457 0.0340890809893608
0.799586057662964 1.77067792415619
1.16246676445007 -4.14842939376831
-1.34535157680511 0.177646219730377
1.06899952888489 1.15555310249329
-0.193171322345734 -1.14220631122589
-0.545770823955536 -0.121583119034767
1.65328192710876 -1.66966307163239
2.79088997840881 -0.544733822345734
1.31110394001007 0.501893639564514
-0.691840469837189 0.595552861690521
0.969695389270782 2.83246183395386
-2.60715198516846 -0.0555224791169167
1.46750199794769 -2.21074509620667
1.27244508266449 -0.474055290222168
1.06306052207947 2.19304037094116
-0.14330281317234 0.103200972080231
-2.38433742523193 -0.140922740101814
-0.105704545974731 -0.435642242431641
-0.579357445240021 0.766327738761902
0.419285416603088 1.25346803665161
0.947131156921387 -1.2680196762085
0.286241263151169 -1.8505312204361
-0.447686046361923 0.781904876232147
2.32381343841553 -3.51081967353821
-0.691607773303986 -0.652823090553284
1.22608947753906 0.293029397726059
0.504865705966949 -1.03660535812378
0.16607928276062 0.716176927089691
1.01623737812042 -0.801962912082672
2.22058582305908 2.339195728302
1.26704001426697 0.804008483886719
0.791810512542725 0.177745118737221
0.510203838348389 0.236420422792435
1.0785174369812 0.0291209369897842
1.64318287372589 0.102449432015419
0.478135734796524 -0.789534389972687
0.621667981147766 0.946422278881073
1.46449100971222 -1.20245170593262
0.0622652992606163 0.770709991455078
0.368864744901657 -1.62880873680115
1.42832684516907 -0.098728783428669
0.272950738668442 -1.09697532653809
1.06415808200836 2.28968715667725
-0.811480522155762 -0.398832350969315
3.88238954544067 -2.37901020050049
1.78297448158264 1.30610346794128
1.43706905841827 -4.7077260017395
0.375859051942825 0.46730637550354
-2.97079753875732 0.575503528118134
2.24800682067871 2.63369083404541
0.794705629348755 -0.179511725902557
-1.44341206550598 0.582354485988617
1.31846714019775 1.38345015048981
-0.916280031204224 -0.33380925655365
0.829657077789307 -3.456378698349
-0.615772902965546 -0.565231382846832
1.40872800350189 -1.2151221036911
-0.423632144927979 -0.684704780578613
0.236384749412537 -1.77713763713837
-0.0336755625903606 -0.777222812175751
0.0671974569559097 0.788780450820923
-0.988248586654663 0.759425461292267
1.26595544815063 -0.593997716903687
1.14533269405365 -3.4424877166748
};

==> figures/visualizations/funnel/cmcd_samples.tex <==
\addplot [semithick, cmcd, opacity=0.7, mark=x, mark size=3, mark options={solid}, only marks]
table {%
-2.30208230018616 0.362786889076233
2.7171003818512 -1.65186321735382
-3.14564394950867 -0.119930237531662
1.47875010967255 -1.70825338363647
-1.73326086997986 -0.432312577962875
-0.655137419700623 -0.652547597885132
0.687709450721741 -0.892738103866577
-2.92404794692993 -0.0449565276503563
-5.67604970932007 0.0548960752785206
-4.14117479324341 -0.0868239551782608
-1.18148422241211 0.338684111833572
0.261565536260605 -0.426490396261215
2.43929195404053 0.298619121313095
-4.40932750701904 0.0119086802005768
-3.13482213020325 -0.0672796592116356
1.74538731575012 -3.41481685638428
1.63197457790375 -3.87472105026245
3.34630346298218 2.61588907241821
-2.05412578582764 -0.156171977519989
0.479670882225037 -1.0824898481369
-4.51081705093384 -0.119341433048248
-4.37457084655762 -0.154290288686752
-1.34151458740234 -0.305000960826874
-0.709448575973511 -0.0645730420947075
-2.44557976722717 -0.332595616579056
1.10438120365143 -0.582320988178253
0.194427564740181 -1.70407176017761
-5.29938840866089 -0.0959467589855194
2.54329013824463 -1.38253390789032
0.934271037578583 -0.117978423833847
0.102634117007256 -0.60459303855896
0.126162350177765 0.358488410711288
-2.41111135482788 0.237556591629982
-2.62286806106567 -0.634850382804871
-1.75728893280029 0.18694843351841
-1.63239693641663 -0.151073440909386
3.74513411521912 -14.563214302063
0.334777265787125 -2.60297393798828
-2.08902096748352 0.615383267402649
2.10188412666321 2.92349815368652
-4.35520648956299 0.118375971913338
3.18628621101379 1.82514786720276
1.42134070396423 1.68188285827637
0.389383107423782 -1.56170606613159
-1.70286095142365 -0.356187760829926
0.745360255241394 -1.60229051113129
2.46880221366882 2.81368446350098
-2.51940560340881 0.493895769119263
0.780130863189697 0.957087934017181
1.35142266750336 0.253028094768524
-2.37483978271484 -0.331306040287018
-2.53758835792542 0.221447169780731
-4.00477123260498 0.270595490932465
3.07800340652466 5.08150625228882
1.88637185096741 0.681332051753998
-2.49924564361572 0.22571262717247
-3.37186861038208 -0.218872427940369
2.46878433227539 2.41400814056396
-0.216463252902031 1.26306581497192
-2.88521409034729 0.287937462329865
-1.10066473484039 -0.348720043897629
1.7230372428894 -6.31761693954468
-0.877839267253876 -1.09952414035797
-3.20428586006165 0.0284880772233009
-2.79749250411987 0.00308118760585785
-3.01828050613403 0.0536929406225681
0.728119075298309 0.87138295173645
-4.17105913162231 -0.147174686193466
-3.73850917816162 -0.0632457807660103
-1.533562541008 -0.260816246271133
2.57455658912659 -5.09431028366089
0.286241829395294 -0.534470677375793
1.47265243530273 1.09735465049744
-3.85304355621338 0.0278423503041267
-0.362686395645142 0.267061710357666
0.611332535743713 0.61564713716507
-1.94827663898468 -0.196267575025558
2.49382090568542 -3.08833813667297
1.18264758586884 -0.0395106300711632
-1.22510552406311 -0.0188040733337402
-2.03360462188721 -0.0418381094932556
1.32620882987976 0.0318944081664085
-2.34767246246338 0.00894230045378208
-3.77154922485352 -0.0657923147082329
-5.1399998664856 -0.11900170147419
-3.38804650306702 -0.260301917791367
1.99720108509064 0.371448189020157
-0.827505111694336 0.557141184806824
-0.291697770357132 0.353471457958221
-0.450476169586182 0.294170737266541
0.556157648563385 -0.323330283164978
-1.50665366649628 0.0296870023012161
-0.351439535617828 -0.203158557415009
3.28635549545288 1.13929319381714
-0.396553933620453 1.08379828929901
-3.36624240875244 0.133124619722366
0.569333910942078 -1.85746133327484
0.401472270488739 1.13127911090851
-3.05183982849121 0.0547827258706093
-0.47257798910141 -1.2005181312561
-0.351429909467697 1.03138971328735
-1.36775517463684 0.52592670917511
-2.67317867279053 0.00917946547269821
1.86317420005798 0.654433071613312
-3.00956320762634 0.0833903700113297
0.56285685300827 0.691882371902466
2.86231184005737 3.38829207420349
-1.18566370010376 0.770609855651855
1.98075032234192 1.49773144721985
-1.37035667896271 -0.748934268951416
-2.50723195075989 0.0740931108593941
-2.55357885360718 -0.142339318990707
-1.4274491071701 -0.25725120306015
0.978760480880737 1.50561380386353
0.249609008431435 -2.45698690414429
-0.192046895623207 0.121488213539124
-1.79480385780334 -0.492500156164169
-4.3081636428833 0.18324813246727
-3.40154528617859 0.229927495121956
2.47679352760315 -1.16241478919983
-0.376980006694794 0.517403721809387
0.669437170028687 0.422679603099823
-1.9537558555603 -0.453294277191162
-2.00602841377258 0.280425548553467
1.14094531536102 -0.280426740646362
0.796629130840302 -0.507753014564514
-1.05643546581268 -1.00607907772064
-1.8794572353363 0.212180629372597
1.57623660564423 3.60369658470154
-0.24577260017395 -0.0453710407018661
-0.637722969055176 0.179309725761414
1.11420154571533 -1.78423273563385
3.09062337875366 3.42069244384766
-2.50913071632385 0.103024505078793
-1.98097491264343 -0.495594263076782
1.18274509906769 0.941350698471069
3.04225325584412 3.73650789260864
-1.7293666601181 0.699838995933533
-1.49757242202759 0.512784540653229
2.80108737945557 -3.5123085975647
-1.80459630489349 -0.0420553758740425
-0.530957698822021 -1.00483453273773
-1.64709520339966 -0.0395486429333687
0.824929535388947 1.09728741645813
-1.14047825336456 -1.20660054683685
-3.81651091575623 0.209468185901642
0.359627783298492 0.66913366317749
-0.544584929943085 1.3301078081131
-0.789445579051971 -0.476477384567261
0.414855480194092 0.615433931350708
-1.4376106262207 0.419523239135742
-0.689470529556274 -1.12411761283875
2.65849804878235 -1.41596662998199
-2.36788654327393 0.450698554515839
-0.178494498133659 -0.871802866458893
-2.86436581611633 -0.263439774513245
-3.38040781021118 -0.0478535294532776
-1.79826724529266 0.56205016374588
3.95255756378174 2.06366753578186
-3.2652747631073 0.0328786745667458
0.985350906848907 0.403819799423218
3.51566648483276 3.55701613426208
-0.544667840003967 -0.152097523212433
-0.420660674571991 0.0289724450558424
0.37913054227829 1.36237907409668
-0.498568058013916 -0.804461598396301
-0.219818651676178 0.373979091644287
2.4400486946106 1.75431942939758
-0.407999604940414 1.82887721061707
-2.67430377006531 0.0719060748815536
-3.5762140750885 0.026050578802824
1.65539562702179 -1.94826459884644
1.8859258890152 -1.32261407375336
1.56378638744354 2.33208060264587
-2.79864454269409 0.161026731133461
-0.545779407024384 0.0307101458311081
-2.56002497673035 -0.135431706905365
-0.925067245960236 1.27540767192841
-1.18574607372284 -1.48981356620789
-1.48631072044373 0.129202708601952
-0.195961847901344 -0.472383439540863
1.5730801820755 -1.30089056491852
2.02178883552551 -2.32845115661621
2.6140296459198 -0.22905233502388
-2.16020512580872 0.74322772026062
1.16006624698639 -2.05025935173035
-0.166780516505241 1.00552463531494
1.80971360206604 0.470361202955246
0.89510703086853 0.662114262580872
3.12928509712219 -4.58078479766846
0.407101392745972 0.353823453187943
2.83808469772339 0.487019032239914
1.12669658660889 0.316863596439362
0.117959260940552 -0.769904136657715
2.03095865249634 -0.894437849521637
1.96081960201263 2.7940661907196
-1.44419026374817 -0.586205363273621
-1.06438779830933 -0.71156632900238
-0.0976469069719315 0.63213711977005
1.43019556999207 -2.84971594810486
0.0571096166968346 1.49556195735931
-2.46654009819031 0.42408674955368
2.26380228996277 -1.70848453044891
-4.28937816619873 0.0632260665297508
0.830391049385071 -0.043201245367527
-3.77880167961121 0.114401832222939
0.0275368336588144 -0.101536057889462
2.80512189865112 3.22798562049866
-2.44158577919006 -0.0202529467642307
-2.69072079658508 -0.0542356930673122
2.95171689987183 7.15444755554199
-0.801789522171021 -0.94489985704422
-1.36654686927795 0.545961618423462
-0.441480368375778 0.864718616008759
-0.0622625723481178 -0.432999789714813
1.81221461296082 2.15034246444702
-2.71568012237549 -0.18689589202404
1.62453937530518 -5.73915815353394
-1.71781754493713 0.0627190992236137
-2.57448625564575 0.542004525661469
2.59657740592957 -6.86068677902222
0.609205484390259 -0.723338305950165
1.89208209514618 -1.34260809421539
-0.100334137678146 0.0356565713882446
1.45100688934326 -0.962580144405365
-2.23346972465515 0.299578189849854
-4.08244514465332 -0.197323232889175
0.990418970584869 0.912942469120026
-3.84825897216797 0.170094788074493
3.47205638885498 5.82311868667603
-4.25164413452148 -0.130094677209854
1.65261483192444 2.70830106735229
0.887675821781158 0.923561871051788
0.536516964435577 -0.334793329238892
-2.80558085441589 0.136392503976822
2.88104701042175 -0.995132923126221
-2.61217141151428 0.127317935228348
0.707710146903992 2.24015617370605
-0.578520715236664 -1.1073614358902
-1.61617171764374 0.816118001937866
3.01820588111877 -6.93044710159302
-2.30034971237183 -0.361677289009094
-0.893504321575165 -0.243973135948181
-1.65202188491821 -0.751781761646271
-2.05429434776306 0.0843074172735214
0.737037718296051 -0.0801028311252594
2.40439200401306 3.73613882064819
-4.06510972976685 -0.284668743610382
0.774557113647461 3.40075349807739
0.85279244184494 1.23981404304504
-1.25508689880371 -1.09622621536255
1.36607825756073 1.25596392154694
-0.286471724510193 1.58217895030975
0.226858407258987 -0.702772557735443
0.874981760978699 0.479863852262497
0.736682951450348 2.38274812698364
3.37625813484192 1.57103073596954
-2.8657763004303 0.202816247940063
-1.47554731369019 -0.0513875409960747
-3.53297519683838 0.112373068928719
-4.98286819458008 0.0702867805957794
1.28840637207031 -1.37267541885376
-2.94943237304688 -0.0296349693089724
-0.781444072723389 -0.320687890052795
0.16594024002552 1.61781430244446
-0.923273921012878 -0.0284068007022142
-0.0075273048132658 0.90231591463089
2.92359209060669 -3.0477249622345
-3.5117609500885 -0.0732870250940323
-3.48800539970398 0.150953710079193
-3.16359996795654 -0.0722439214587212
-0.693071305751801 -1.19655573368073
-0.39429771900177 0.612525224685669
0.261335968971252 -0.0139225423336029
-1.81866228580475 -0.0677271038293839
2.67588686943054 1.81082832813263
-3.79115629196167 0.0510430224239826
1.74121165275574 0.127547383308411
-0.757433831691742 1.33648884296417
1.64857828617096 2.31671571731567
1.34255862236023 -0.824857771396637
-4.42196035385132 0.0670761168003082
0.690129399299622 -1.60860073566437
1.39913976192474 -1.8473048210144
-4.56214904785156 0.166682451963425
-1.39532864093781 0.330370634794235
0.0861040279269218 1.83739483356476
-4.16238355636597 -0.100973650813103
-0.826078176498413 1.10019159317017
-1.21893906593323 -0.488842815160751
-1.65195739269257 0.460340678691864
0.925214409828186 0.790398478507996
-1.27864825725555 0.655551433563232
-5.09289455413818 -0.00900017842650414
-1.18346285820007 -0.203020572662354
2.96587467193604 -6.22861909866333
-2.78154850006104 -0.151209354400635
-0.50571882724762 0.736527144908905
-1.16954123973846 0.278275668621063
0.682295143604279 -0.72213351726532
2.5342264175415 1.64290475845337
-1.01637470722198 -0.430694222450256
3.35691165924072 -1.50487649440765
-3.11584997177124 0.339296847581863
-0.798559188842773 0.761052072048187
-1.59655380249023 0.801748216152191
4.8570671081543 -1.83841717243195
0.987015187740326 1.78458273410797
-1.29985463619232 0.299048334360123
1.2233110666275 0.882010519504547
-0.119635112583637 -0.0663030371069908
-2.9011435508728 -0.219653487205505
-3.11263012886047 -0.0403545051813126
-0.264707803726196 0.1824641674757
0.59709644317627 1.76474511623383
-4.90238428115845 -0.0467400327324867
-2.8348662853241 -0.042135588824749
-3.49815225601196 -0.0544164031744003
2.03420543670654 0.349259912967682
-1.87784814834595 0.149083137512207
3.44561672210693 5.16639089584351
-3.612553358078 0.206716656684875
-3.10220623016357 -0.132712870836258
-4.02302598953247 -0.124311849474907
-3.51406025886536 0.0452307835221291
1.77804362773895 2.38022184371948
-5.0241527557373 0.0549766533076763
0.14217783510685 -0.617537677288055
2.89847588539124 -8.49435424804688
1.85171091556549 -0.507254064083099
0.546282410621643 0.116581290960312
1.52605926990509 4.20659923553467
-1.32107973098755 -0.46805876493454
2.5929901599884 -0.173280954360962
-0.0589744858443737 -0.073182001709938
-3.94377112388611 0.0643153563141823
-3.59183049201965 -0.0915213227272034
0.195572674274445 0.157785505056381
-3.24327111244202 0.245842128992081
2.12115383148193 -4.41902017593384
1.7695198059082 -0.989477694034576
-0.344148069620132 -1.80856704711914
-1.35372722148895 0.84822005033493
-1.1185690164566 0.223315894603729
-1.07125198841095 1.03717648983002
-0.474471151828766 0.941662907600403
-2.89269161224365 -0.284313797950745
-4.49756383895874 0.193252921104431
-1.72702133655548 -0.288746118545532
1.28680837154388 -1.87812185287476
-4.872962474823 -0.15587230026722
2.1258909702301 -2.9945821762085
-2.96474432945251 -0.223529189825058
1.47809457778931 0.659901022911072
-0.0863701552152634 -0.695176005363464
1.56522536277771 -1.53751122951508
2.5647566318512 -0.114001676440239
-0.809803605079651 0.234254240989685
2.17990207672119 7.75526332855225
-3.02723693847656 -0.468369841575623
-1.48462414741516 -1.18080508708954
-1.99065256118774 0.0659720301628113
0.480706751346588 1.17605662345886
1.75003707408905 4.9382438659668
-2.00510478019714 -0.249830305576324
-3.6706018447876 0.100103236734867
-0.283848792314529 -0.664498805999756
-0.769624710083008 0.827411651611328
3.28059792518616 0.132847860455513
-5.76660919189453 -0.105024687945843
-2.4539897441864 0.13241508603096
2.73796391487122 -2.68213534355164
0.765443027019501 0.2416150867939
1.04783391952515 3.86014723777771
-0.441294968128204 -1.10984599590302
-1.90254366397858 0.0705086588859558
0.529346227645874 -1.55487453937531
-1.69893980026245 0.589592695236206
2.23954391479492 -1.91657984256744
-1.68936812877655 -0.302253246307373
-2.35564422607422 0.126272171735764
-0.47098383307457 0.458116292953491
-2.98863625526428 0.0856582447886467
-2.5823814868927 -0.0233441740274429
0.836834013462067 1.43259954452515
-2.43321418762207 0.101322650909424
-0.908910572528839 -0.606834173202515
-0.250907421112061 -0.381898641586304
2.35286712646484 4.48986625671387
-0.572398722171783 -0.307494252920151
0.957313776016235 -0.671710848808289
2.20559549331665 2.18390679359436
0.499347031116486 0.476000070571899
-5.44216632843018 0.021197184920311
1.14892673492432 -0.0695659294724464
0.224615082144737 -0.856479048728943
-0.617664456367493 -1.33929085731506
1.68356287479401 0.625133275985718
0.759997487068176 -0.665313065052032
-1.95272898674011 0.32958909869194
-2.79791879653931 0.392808526754379
-4.54120063781738 0.0876566544175148
0.473898410797119 -1.36842691898346
-0.0212510786950588 -0.409141451120377
1.80367803573608 -2.98533010482788
-0.459336847066879 -0.608856379985809
-4.04125022888184 -0.0939730107784271
-2.71941876411438 0.0476906411349773
1.30111610889435 -0.993039011955261
-1.29469442367554 -0.399461299180984
1.9147584438324 1.72094464302063
1.69372177124023 2.26769685745239
-1.06558358669281 -1.11235022544861
0.0817957147955894 0.260275661945343
0.0116390790790319 -2.51369905471802
1.30812835693359 2.12811732292175
0.420611143112183 -0.284651935100555
-1.04773831367493 0.132026940584183
1.50834393501282 -0.239928126335144
-0.247863098978996 -0.499522656202316
0.533463001251221 0.450864344835281
-2.79115772247314 -0.0566530078649521
0.717430353164673 1.30711257457733
-4.63746690750122 0.056474294513464
-4.40272998809814 -0.0271355509757996
1.78283166885376 -1.98297917842865
-0.0490867123007774 -0.77021062374115
0.901458442211151 2.28624057769775
2.24546122550964 -2.34614253044128
2.46879911422729 -3.70331978797913
-2.43215894699097 0.0225836783647537
-2.70969653129578 -0.0713595524430275
3.0592052936554 -0.0651790723204613
-3.4477424621582 -0.0709922313690186
2.44825959205627 -0.928495049476624
0.406482517719269 -1.12120735645294
0.764986932277679 -1.53926479816437
2.08948588371277 -2.93431305885315
-3.22449994087219 0.0670458897948265
-1.77355206012726 0.296485126018524
-2.48492479324341 -0.675649225711823
-0.0278173238039017 1.07648134231567
-0.509989321231842 -1.07772088050842
-1.03073084354401 0.119814790785313
-0.764114260673523 0.800506770610809
-0.485774517059326 -0.400130480527878
-4.64206695556641 -0.0689306333661079
0.865048706531525 0.00924161076545715
2.5479531288147 3.28223752975464
1.95163512229919 5.26158285140991
-4.53976392745972 0.116949737071991
1.5562607049942 -1.73981535434723
-3.81839394569397 -0.121868878602982
-0.736979067325592 -0.078726626932621
1.19165992736816 0.915927708148956
-0.667041778564453 -0.306623905897141
-3.0672070980072 -0.00394248589873314
-2.17386746406555 -0.37434047460556
-2.24428105354309 0.439842253923416
-0.404360085725784 -0.301631569862366
-2.88290596008301 0.155837938189507
0.0632791146636009 -3.12935972213745
-3.26118659973145 -0.339702546596527
-2.24665284156799 0.0661615952849388
-1.36183404922485 0.111703410744667
-3.12135195732117 0.182295009493828
-2.74488282203674 0.489793628454208
-3.57368206977844 -0.028278261423111
-1.14494395256042 0.557770252227783
-1.2936784029007 -0.201003983616829
-3.27806615829468 -0.259244710206985
0.6402508020401 -2.31924939155579
0.36837163567543 1.68782198429108
-0.330765783786774 -0.0542052239179611
2.75222778320312 -1.60071730613708
-3.43357563018799 -0.127645790576935
0.203010335564613 0.724565327167511
-2.71325063705444 0.0478768348693848
2.08287715911865 0.778626978397369
0.264988780021667 -1.09172403812408
-0.252411097288132 0.462847471237183
1.25379908084869 0.574257731437683
1.29037797451019 -0.0024762749671936
1.08283710479736 2.34058499336243
0.824772238731384 -1.18117606639862
2.38531041145325 1.53977370262146
3.66129732131958 8.95305824279785
0.179835245013237 0.494024455547333
-2.38812565803528 0.188704892992973
1.82021987438202 -0.385249316692352
-1.81683075428009 -0.258655369281769
-0.335434317588806 -0.367032706737518
-2.75825595855713 0.0808726400136948
1.76474726200104 -3.68990004062653e-05
0.358520656824112 -1.052321434021
-2.89318418502808 0.185671165585518
-2.46579766273499 0.342991650104523
-2.41471171379089 -0.0987686961889267
0.420952022075653 -0.515073895454407
-3.43390846252441 0.232507899403572
-0.524203419685364 0.622418403625488
-4.00625896453857 -0.245864003896713
1.1920360326767 -0.882647514343262
2.77573609352112 3.01216793060303
-4.3151330947876 0.0912788510322571
-4.88968658447266 -0.00396052189171314
2.7368323802948 -0.642444491386414
3.50457119941711 2.71880626678467
-2.67702436447144 0.263212084770203
1.84451389312744 1.39757776260376
-1.41951990127563 -0.128973320126534
-2.00478410720825 -0.0140212327241898
-1.01409876346588 0.242940276861191
0.582031428813934 -0.259143471717834
2.25995111465454 -1.51726853847504
3.2991509437561 -1.42447829246521
-0.80503910779953 -0.73255443572998
-1.81200432777405 1.06856513023376
-2.69887638092041 -0.373937368392944
0.891327977180481 -1.68042099475861
-1.82642686367035 -0.109845012426376
-1.85527992248535 0.232040047645569
2.23714780807495 3.02656888961792
-1.18456888198853 -0.724180161952972
0.446583986282349 -0.509427607059479
2.36581134796143 -3.33284878730774
-1.57928073406219 0.0889676213264465
0.234058782458305 -1.19763350486755
2.09529113769531 -1.68612694740295
0.160494774580002 -0.838825285434723
-0.145181864500046 -0.289985150098801
-0.601208090782166 0.583211183547974
-0.98172789812088 0.407713294029236
0.538583755493164 -0.592114984989166
-3.67766308784485 0.0162239000201225
2.28724551200867 -2.51845860481262
-2.94481945037842 -0.189375057816505
4.32026195526123 -3.4715838432312
0.682162523269653 1.14354717731476
-3.98836302757263 -0.0325181260704994
2.90360498428345 2.90693163871765
-3.16948270797729 -0.473074555397034
-2.88454461097717 0.0627515017986298
1.43230521678925 -0.343464225530624
-1.73612356185913 -0.337055385112762
-0.0177527219057083 0.647844195365906
-0.382912307977676 -0.115573838353157
1.93020510673523 -0.318282097578049
-2.75976181030273 -0.309788048267365
2.44294929504395 1.79119372367859
1.88472926616669 4.21410799026489
0.283589750528336 0.415066778659821
0.684654951095581 -0.600085198879242
0.796032905578613 0.0247116573154926
-2.69837236404419 0.0601491332054138
-1.2939327955246 -1.27021551132202
-2.08837127685547 -0.497909307479858
3.00602459907532 -1.58838951587677
-1.32669484615326 0.386551141738892
-1.31084263324738 -0.0311946980655193
-1.29874813556671 0.156776458024979
2.22240614891052 2.02823162078857
-3.08617687225342 0.20905889570713
3.04262280464172 0.0336129367351532
-0.854834973812103 1.59940755367279
2.26993107795715 5.29361772537231
-1.43026041984558 0.621486783027649
-0.308151811361313 -0.676142275333405
1.34490430355072 -0.590077459812164
-3.48015069961548 0.0114852264523506
-0.124113857746124 0.248080939054489
-2.51259279251099 -0.164539217948914
1.52411842346191 -0.881658434867859
-2.22854447364807 -0.166476786136627
-0.152923882007599 1.14753699302673
3.06551003456116 -7.22037029266357
-0.0950737297534943 -0.423427045345306
0.105441674590111 1.58545649051666
1.90543019771576 1.85610234737396
-2.16553163528442 0.190557718276978
-1.96101415157318 0.0563642531633377
0.594898760318756 0.118544146418571
0.479553669691086 1.37535154819489
0.493056386709213 0.491905301809311
-3.08847045898438 0.321054011583328
2.59726119041443 1.66989433765411
2.0705246925354 -2.63745999336243
0.99374657869339 0.900365948677063
2.62200951576233 0.90730494260788
-1.31361401081085 -0.344259798526764
0.920861899852753 -0.731464147567749
1.49938678741455 -0.46942549943924
-3.46809720993042 0.0588676631450653
0.55962073802948 1.19613552093506
1.90727531909943 -1.11333298683167
-2.04040145874023 0.174297824501991
-4.21056270599365 0.262108147144318
-2.91663503646851 -0.0588577464222908
1.69169044494629 -2.9130871295929
0.319084107875824 -0.121100343763828
-3.03871297836304 0.171753481030464
0.946214258670807 1.03059148788452
-2.74442005157471 -0.0786163285374641
1.47985208034515 1.54109048843384
2.9256854057312 -1.09208691120148
-0.0374418944120407 -0.469968676567078
3.09969520568848 4.98941326141357
-0.901846885681152 1.2270632982254
-1.8718329668045 0.477956831455231
-0.752480685710907 0.653258144855499
0.925705015659332 0.674989938735962
-1.75443637371063 0.114292472600937
1.52148258686066 -1.65115082263947
0.887070119380951 1.33245074748993
-0.339293211698532 0.630004584789276
-3.3284592628479 -0.0841153264045715
-2.97152876853943 0.364216089248657
-4.57932424545288 0.0552827045321465
-1.43564713001251 0.741263449192047
1.77590799331665 2.35607647895813
-2.01139402389526 -0.125698238611221
-3.08495044708252 0.307777941226959
-0.99890261888504 -0.276525616645813
0.299282670021057 0.55711030960083
2.13226008415222 3.15523457527161
-0.88004744052887 0.0781773328781128
0.328909605741501 -1.52182686328888
-1.87493801116943 0.231176510453224
0.947214424610138 -1.87665188312531
-5.66822052001953 0.0842369198799133
-3.09024667739868 0.0367505997419357
0.581417262554169 0.314980745315552
-0.10035202652216 0.684579908847809
0.964889824390411 2.89822006225586
-5.6561598777771 0.070491187274456
-2.9203143119812 -0.054181694984436
4.11799049377441 -0.265176594257355
1.66551911830902 2.22968578338623
-2.40212273597717 0.131675213575363
-0.97672963142395 -0.0711934044957161
-0.412145882844925 -0.235219955444336
1.37817716598511 2.08927583694458
-1.83469069004059 -0.188941970467567
2.64148831367493 0.623509585857391
1.7960319519043 -0.305446058511734
3.89846539497375 0.209194794297218
1.07839584350586 0.723275482654572
2.6347336769104 4.71444511413574
1.11371636390686 1.81846034526825
-2.27403903007507 0.680481493473053
-0.662387430667877 0.385394185781479
-2.35162210464478 0.297390758991241
-3.12855362892151 -0.0269780121743679
0.149440854787827 0.318672657012939
-3.56290411949158 0.0605707988142967
-2.3298807144165 -0.116119161248207
0.551699757575989 -1.29741954803467
0.78470367193222 -3.33151125907898
0.475525200366974 -1.13560938835144
0.171769186854362 0.171548187732697
0.72588986158371 2.15797209739685
2.27626872062683 -7.5868763923645
-2.72184276580811 0.0801096484065056
-1.71035873889923 0.0199632216244936
-0.343000203371048 0.543796300888062
0.548973202705383 -0.993918836116791
-0.716006278991699 -1.16856694221497
0.384878396987915 -0.819054901599884
1.10969841480255 2.52899432182312
1.70511591434479 0.213087916374207
2.18616461753845 -0.960623145103455
1.89691460132599 2.71245646476746
0.0586024336516857 0.301463752985001
-2.52726769447327 -0.342686474323273
1.08188557624817 -0.0661337599158287
0.59411233663559 1.49758887290955
-1.56958186626434 -0.354020774364471
-3.23653793334961 0.127724170684814
-2.29474306106567 0.369739651679993
3.52721309661865 -12.8576679229736
0.349404782056808 1.2028284072876
0.793523073196411 4.44968223571777
-3.70329880714417 0.0647354498505592
-0.128304123878479 0.372785270214081
1.16828978061676 -1.72980642318726
-1.74072170257568 0.129710853099823
-2.44798564910889 0.11974485963583
5.00405931472778 5.14560461044312
-0.838922381401062 -1.19591331481934
2.55861210823059 4.43782472610474
-0.485708594322205 0.325979858636856
4.26673173904419 -8.3962516784668
-0.80145251750946 0.300472378730774
-1.68231093883514 -0.159596413373947
-3.0252251625061 -0.25081929564476
-4.41457939147949 0.00990009866654873
0.745792627334595 0.573913395404816
-4.25961208343506 0.104804612696171
1.87555503845215 0.572713971138
-3.77645206451416 0.0712590664625168
-1.9755551815033 0.141249090433121
-4.1962251663208 0.0751764476299286
2.02997994422913 -2.76992845535278
-1.26159071922302 0.407806545495987
-3.50945448875427 0.27208536863327
1.56595802307129 -1.83015418052673
-2.55816602706909 0.0466928593814373
-0.280522435903549 -0.707475781440735
-2.02188587188721 -0.464499682188034
1.61209666728973 -4.64798974990845
2.91826629638672 -3.7639262676239
-2.25629878044128 -0.287000864744186
-0.465569913387299 -1.23771464824677
1.060671210289 -3.16750597953796
-0.739365041255951 0.597453594207764
1.19223380088806 0.286566883325577
1.11190903186798 -1.81835305690765
0.973237216472626 1.33212840557098
-1.38287091255188 0.930080354213715
-3.17320322990417 -0.0747046172618866
-1.29514873027802 -0.432478874921799
0.421845257282257 0.539729952812195
0.485871404409409 -0.991905689239502
1.37017631530762 -4.05656957626343
-4.26833009719849 -0.229175537824631
1.07931196689606 1.83561265468597
0.923323571681976 -0.122310698032379
3.28580236434937 0.0738621577620506
-3.12149620056152 -0.225478410720825
-1.41845309734344 -0.788547515869141
2.58569097518921 -3.85611057281494
2.88805413246155 0.248792588710785
-0.920380473136902 0.279596537351608
-3.76298236846924 -0.114637494087219
1.36245858669281 -2.27119445800781
-0.416745632886887 1.16432428359985
-0.244131684303284 -0.724121332168579
-2.38861846923828 -0.0251835472881794
-1.67105746269226 -0.0941397100687027
2.64896726608276 4.70099687576294
-3.16540193557739 -0.063693530857563
-2.03097009658813 -0.324192106723785
-1.17228555679321 -0.237165287137032
1.12333369255066 -1.42185008525848
-4.55741596221924 0.0494871474802494
-4.14573574066162 0.0197938643395901
-1.18471777439117 0.544628262519836
-2.45546793937683 0.341768234968185
3.26270985603333 3.73557901382446
-2.0400447845459 0.18572898209095
-1.42212045192719 0.530097782611847
-1.1572322845459 0.46623820066452
0.261306941509247 0.395331025123596
-1.25919806957245 0.130489438772202
-2.91969871520996 0.345440655946732
-0.702312409877777 -0.51446121931076
-2.74755096435547 -0.183678448200226
-3.24529480934143 1.06208026409149e-05
0.298828810453415 -1.71345853805542
-0.712678015232086 -0.171918794512749
1.52907335758209 -5.22555208206177
1.11921632289886 1.91008734703064
-0.436768144369125 -0.867516338825226
-0.305682986974716 0.106649570167065
1.06492757797241 0.545832812786102
-2.23040270805359 -0.510605812072754
0.490620672702789 -1.95316600799561
1.42800116539001 -0.562555015087128
1.26581263542175 1.30582141876221
2.49201655387878 5.10423898696899
-2.54898118972778 0.234422147274017
-0.483404546976089 1.36004960536957
3.13239884376526 1.26201438903809
-1.38154411315918 0.135726496577263
-0.412076115608215 0.154836118221283
1.66577768325806 4.83018159866333
-3.82329678535461 -0.0137085542082787
-3.03328800201416 0.201407581567764
-0.729000926017761 0.287188768386841
-3.54878306388855 -0.156520053744316
-0.949964225292206 -0.780733585357666
-1.05504989624023 -0.330441772937775
0.872285962104797 3.44915103912354
1.48721122741699 0.838246941566467
0.332593739032745 0.840720236301422
-2.20260238647461 -0.53994619846344
2.8627655506134 -4.07384347915649
-1.63822305202484 -0.138301059603691
-3.00141167640686 -0.0564258694648743
-0.42671999335289 -0.46166068315506
-0.965391516685486 -0.690343260765076
-2.37169289588928 -0.678893029689789
1.94422578811646 -0.387053638696671
2.17110157012939 -1.90260243415833
1.79980003833771 3.9613983631134
-1.90869116783142 -0.0888776034116745
-0.292499631643295 0.579079449176788
-3.09170746803284 -0.210752755403519
-1.78324747085571 0.00850053410977125
2.93765497207642 2.61043524742126
0.0281550586223602 -0.220344573259354
0.430868566036224 0.66599714756012
-0.205866515636444 0.414734959602356
-0.461273998022079 0.00992595124989748
3.17447209358215 2.40350341796875
1.74320101737976 -1.12402641773224
-2.96442627906799 -0.0395150855183601
-0.120989799499512 -1.16922581195831
0.342549175024033 1.54644501209259
1.38997495174408 -1.60400366783142
-3.04812431335449 -0.0301020592451096
-1.80586075782776 0.51164585351944
-1.61245334148407 -0.180832639336586
2.09267330169678 -2.79349112510681
-0.0868182852864265 -1.03709173202515
2.78893446922302 1.40026330947876
-0.667653977870941 0.477499783039093
1.96190357208252 5.05496072769165
-0.399097770452499 0.749789178371429
-1.6087486743927 0.646359384059906
1.95346963405609 -3.91883134841919
-3.57363939285278 -0.150068581104279
-3.21623802185059 -0.104781821370125
-4.56254816055298 0.0401255190372467
2.1393711566925 -1.51889634132385
0.558095633983612 -0.34686017036438
0.348548829555511 -0.65940922498703
-0.483225852251053 -0.141041427850723
3.81026363372803 -16.5469188690186
-0.386463135480881 0.63820606470108
3.31096696853638 -15.5821762084961
-1.11506712436676 -0.772433280944824
0.486555397510529 -0.902139604091644
-3.93620562553406 0.181055292487144
-3.05685830116272 -0.141920447349548
3.08562994003296 -2.30211472511292
-1.07229197025299 -0.0979652628302574
-4.40255069732666 -0.0325464308261871
3.43607807159424 2.87592577934265
-3.77820253372192 0.203157067298889
-0.42164021730423 -0.588117122650146
-5.42066526412964 -0.0181583687663078
1.45814025402069 -0.738970518112183
1.65345799922943 -1.38251769542694
-1.28320956230164 0.750353276729584
-3.61960864067078 -0.0625186115503311
-1.19034957885742 -0.649728298187256
1.33063495159149 0.142922386527061
-3.09478068351746 0.14896297454834
-4.65705823898315 0.233201831579208
-1.91335356235504 -0.212797462940216
-1.93104803562164 0.0549244061112404
-3.54456114768982 -0.165458142757416
0.75561398267746 -2.22627210617065
-3.01392078399658 -0.0238115526735783
-2.79797029495239 -0.0148774720728397
0.58929830789566 2.88199758529663
-2.16120767593384 -0.13717582821846
-2.39264369010925 -0.015559010207653
-1.89882922172546 0.33819842338562
0.5180943608284 2.09244608879089
2.88425636291504 2.28277111053467
-4.18526363372803 -0.130960673093796
0.667211711406708 -1.59710586071014
-0.289350181818008 -1.13798856735229
-1.92036557197571 0.315309464931488
-1.91903853416443 -0.0584585443139076
-0.0568813867866993 -0.163920134305954
-0.998595774173737 0.163744300603867
1.73277795314789 1.61528646945953
-3.05258727073669 0.135787934064865
-1.39071345329285 -0.176966026425362
-1.71491158008575 0.262603461742401
-0.0550556629896164 0.188554093241692
-0.454734623432159 1.47963011264801
1.99033319950104 0.363799899816513
-0.899916410446167 0.420083582401276
-1.7995697259903 -1.06612813472748
1.14569199085236 -0.452534884214401
-3.8415904045105 -0.0637833550572395
1.46553111076355 -3.61625504493713
3.22716403007507 -3.00811886787415
1.0430862903595 -0.229095250368118
-1.57330358028412 0.479143559932709
-0.521791338920593 -0.549563348293304
2.10920023918152 -1.54137444496155
-1.99001550674438 0.361792832612991
-0.622338175773621 -0.149000778794289
-0.985875844955444 -0.862089276313782
-1.71878743171692 -0.431792110204697
3.3643639087677 1.91404163837433
3.21537065505981 -0.736657321453094
0.548851788043976 1.2770721912384
2.23642826080322 -0.830296635627747
-1.89124238491058 0.168490782380104
3.82390880584717 -4.4859561920166
2.85283803939819 1.20346891880035
-0.97395533323288 0.441461056470871
-3.17365193367004 0.203599572181702
0.676170825958252 -0.157763630151749
0.110015362501144 0.0557580702006817
2.26113700866699 -0.0155092775821686
3.57277035713196 -6.34268522262573
1.82099163532257 0.430171430110931
-0.0105090588331223 0.411687940359116
0.412619411945343 0.0345486775040627
-0.500151216983795 -0.226421296596527
-0.888684988021851 0.00620373524725437
0.200189888477325 -0.31515246629715
-1.93664765357971 0.246870487928391
-1.25392293930054 -0.0522946789860725
-0.333204925060272 0.167621865868568
1.99002957344055 3.65206956863403
0.675696730613708 -0.881980121135712
-0.0349946580827236 -1.2817599773407
-2.64826464653015 -0.275894165039062
1.15348601341248 -1.4049586057663
-1.83597791194916 0.231230407953262
0.616984307765961 0.023855784907937
0.0422417595982552 -2.41928839683533
-4.83651828765869 -0.0870563983917236
-2.78895497322083 -0.244197100400925
-3.44915175437927 -0.0638816207647324
1.23172497749329 -0.784863710403442
-1.31646680831909 -0.591280400753021
2.06249785423279 -0.538774788379669
-3.04299306869507 -0.226466193795204
-1.352210521698 0.972522377967834
-3.62032341957092 0.269873946905136
-1.11529433727264 -0.441705495119095
-2.04973292350769 0.532503962516785
0.797682881355286 -1.67392313480377
-2.15898060798645 -0.310077339410782
1.13372159004211 1.03213560581207
-1.04056251049042 1.29782831668854
-2.26891446113586 0.390050619840622
-0.429043143987656 -0.695970773696899
0.0959770232439041 -0.55976003408432
-1.73969483375549 0.109934210777283
-3.08328700065613 0.362690806388855
0.536123096942902 -0.115064196288586
1.3173942565918 -1.35263502597809
0.600278258323669 -1.00111269950867
-2.45712113380432 0.0511401556432247
2.52313828468323 -2.4295756816864
-0.52817964553833 0.80996698141098
-1.05465245246887 1.48877561092377
-3.61239719390869 0.397925734519958
-0.082734152674675 -0.385774940252304
2.75041794776917 0.396359235048294
-1.80399298667908 -0.224921762943268
-1.36806297302246 -0.671281337738037
0.536606788635254 0.142962411046028
0.892207026481628 2.51916193962097
-0.0254232957959175 1.94608724117279
-0.245789170265198 -1.27598834037781
2.06795263290405 2.92218995094299
-1.14744579792023 0.0694152265787125
-3.66562628746033 0.00416113901883364
0.134268760681152 -1.71751856803894
1.11297178268433 2.66963815689087
-0.456498444080353 -0.21143901348114
0.0814232155680656 0.243585214018822
-1.4436662197113 -0.147269397974014
-1.65627884864807 -0.360403746366501
0.75504744052887 0.0205450654029846
2.14319205284119 -1.07837569713593
1.52293217182159 -0.814693570137024
3.71135187149048 -4.63974380493164
3.77188110351562 -7.38850879669189
-1.55896592140198 0.131288319826126
-0.730309903621674 -0.0282757226377726
1.72129416465759 1.04686331748962
-1.19846022129059 -0.141079917550087
1.34126055240631 -1.58603525161743
3.41647863388062 0.665999293327332
-1.51580560207367 -0.325151681900024
-1.3656085729599 0.11598028242588
-0.666090905666351 -0.273932337760925
-1.54703390598297 0.232625290751457
2.47042012214661 -4.76293611526489
-2.63967227935791 0.0565592832863331
3.34690642356873 3.86113333702087
0.57414573431015 0.646076619625092
2.04032945632935 -1.15847849845886
-2.58111190795898 0.0239095278084278
0.107312403619289 -1.03263545036316
-2.87457609176636 -0.105194680392742
-1.69555115699768 0.0699272304773331
0.416549414396286 -1.79441475868225
1.97800505161285 1.77634596824646
1.98315393924713 -2.07525610923767
-1.10722041130066 -0.180222272872925
-2.54790592193604 -0.188520848751068
1.9675589799881 -0.100728698074818
1.21144342422485 3.16471219062805
-2.52055931091309 -0.0959104001522064
1.64115333557129 2.30013847351074
-0.187492519617081 0.719014346599579
-1.06172788143158 -0.619142293930054
};


==> figures/visualizations/funnel/craft_samples.tex <==
\addplot [semithick, craft, opacity=0.7, mark=x, mark size=3, mark options={solid}, only marks]
table {%
-5.22692728042603 -0.0655412003397942
-3.12017679214478 0.364177733659744
1.67344403266907 3.3939528465271
-0.680065095424652 -0.931869685649872
1.70548021793365 2.16067242622375
0.855702638626099 1.67858695983887
1.05882096290588 -0.923746764659882
2.40793657302856 3.70080590248108
0.995828032493591 0.53462290763855
0.0421813726425171 -0.30791187286377
-1.1944317817688 0.550591945648193
-1.28303873538971 -0.861440241336823
-0.712029635906219 -0.787580847740173
2.85604619979858 2.70764470100403
1.99347114562988 1.85427534580231
3.76490044593811 6.05027198791504
-2.84646439552307 -0.000369399785995483
-4.94594573974609 -0.0244247615337372
0.133275628089905 -2.64712977409363
1.32018983364105 -1.76829707622528
0.64449542760849 -0.774529933929443
0.899121701717377 -1.89930391311646
-5.28659105300903 0.0747693479061127
1.6586582660675 -2.7636194229126
-5.28659105300903 0.0747693479061127
-2.74513268470764 -0.197977900505066
0.350169211626053 -3.67725014686584
1.69543123245239 -2.37410616874695
1.11406421661377 3.48851680755615
2.33696556091309 1.00542759895325
0.836676597595215 0.610965967178345
1.46061968803406 -2.93138933181763
1.35035836696625 -4.74601030349731
0.233090206980705 1.13112342357635
-1.67291963100433 0.765132367610931
1.40026187896729 2.93890166282654
-1.56764423847198 -0.126831203699112
1.09880232810974 -2.40640115737915
-2.63829660415649 -0.0831981301307678
-0.450164198875427 -0.295978724956512
-3.11622738838196 -0.00450398959219456
1.87544333934784 -0.780687868595123
0.699340045452118 0.211203962564468
-0.809925317764282 -0.211800932884216
-0.150271743535995 1.60803663730621
-3.20859742164612 0.249088943004608
-5.25138902664185 -0.0634013935923576
-1.67824256420135 -0.34718731045723
-2.47180390357971 -0.0565357096493244
-1.79642808437347 0.284950315952301
0.7043297290802 -1.52033042907715
2.48859882354736 5.74382543563843
1.63481938838959 -0.930744826793671
-0.605241179466248 1.1061863899231
1.8417489528656 0.398310661315918
-2.69465613365173 -0.311465114355087
2.32319331169128 0.678681790828705
1.65983915328979 -1.19414663314819
-5.25138902664185 -0.0634013935923576
-4.24957180023193 0.0760090202093124
1.62408590316772 -1.52724599838257
-0.752336025238037 0.0604381188750267
-0.446356862783432 -0.822398126125336
-3.96247410774231 0.0985831990838051
-0.352498888969421 0.187766656279564
-3.39955449104309 -0.0483191981911659
2.16322994232178 -1.94730734825134
1.65612077713013 4.69045782089233
-2.42742395401001 0.0173695534467697
1.2273850440979 -1.80831015110016
-3.26855754852295 0.056491918861866
-2.44161367416382 0.169218838214874
-0.706776916980743 -0.465749233961105
-0.386464595794678 -0.0872354432940483
-3.70944905281067 -0.3063585460186
1.63654911518097 -2.77361464500427
-5.28659105300903 0.0747693479061127
0.774903297424316 -0.049001581966877
0.698482751846313 0.384635329246521
1.31553733348846 -2.23654460906982
2.52206468582153 0.46624693274498
-2.11944437026978 -0.0630160272121429
-5.28659105300903 0.0747693479061127
1.42577612400055 0.0579154938459396
0.223587095737457 -2.67088270187378
-2.61214733123779 1.00446665287018
-0.178512156009674 0.765325784683228
0.208908826112747 0.415902495384216
0.693174660205841 -2.24443078041077
2.01837873458862 -1.0474579334259
-1.12462663650513 -0.15610483288765
-3.24701952934265 0.184669271111488
1.13728272914886 0.0428507924079895
-2.19015097618103 -0.134539127349854
-5.109375 0.0289114825427532
-1.08372914791107 0.980396866798401
-3.07929944992065 0.300694227218628
-5.25138902664185 -0.0634013935923576
-1.88709962368011 -0.36388111114502
2.32045817375183 3.10029768943787
1.45182609558105 0.899222075939178
1.83992648124695 -0.941677749156952
2.14151811599731 -6.98836088180542
1.40929961204529 -3.33938598632812
1.0814061164856 -1.41032457351685
1.60045695304871 -1.79787087440491
-5.34721231460571 -0.0303570479154587
-3.72582340240479 0.00733831338584423
-0.474511802196503 -0.761731028556824
-5.28659105300903 0.0747693479061127
1.84974420070648 -2.87648153305054
-1.88528609275818 -0.812979996204376
-0.879276156425476 -0.0857767015695572
-0.671717345714569 -0.148732379078865
-4.06365489959717 0.131237328052521
-0.113053970038891 -0.972866177558899
3.38440489768982 5.9084358215332
2.17200350761414 -3.37746119499207
-5.21707916259766 0.00441128760576248
3.16632866859436 2.74324584007263
1.925626039505 -0.910256028175354
-3.48768091201782 -0.0434561185538769
-2.57200217247009 -0.421768546104431
-0.805040895938873 -0.351808965206146
-0.989582598209381 0.107467301189899
2.02151703834534 -2.69121479988098
-3.09863710403442 -0.200853079557419
-2.31719350814819 0.345764309167862
-4.16610479354858 0.149631395936012
1.54221332073212 3.24304842948914
-2.69046902656555 -0.118181176483631
-2.22977113723755 -0.00607274100184441
-5.28659105300903 0.0747693479061127
-0.979719817638397 0.0199724137783051
-1.93480288982391 0.134434476494789
-1.55086517333984 -0.618676066398621
1.63661444187164 -0.994835078716278
-2.62555980682373 -0.32497176527977
1.32204508781433 -2.29752469062805
0.8265620470047 2.03278660774231
-3.5669367313385 0.160386234521866
2.91333723068237 0.729791700839996
-2.44465470314026 -0.18158070743084
1.68902003765106 1.73951363563538
2.83044743537903 3.12864446640015
-1.0166392326355 0.172880902886391
0.674135982990265 -0.997824847698212
3.48266363143921 3.92730665206909
-3.5012674331665 0.0131555199623108
-5.25138902664185 -0.0634013935923576
3.02474689483643 -0.0647323429584503
-1.76647281646729 0.326398193836212
-1.26807188987732 0.999409079551697
-1.45009696483612 -0.395069092512131
-3.51486682891846 0.0159806907176971
3.37695074081421 4.31617641448975
0.909467995166779 -1.47005522251129
3.37890148162842 0.713399887084961
-2.98862099647522 -0.12990514934063
-2.51586294174194 -0.0307299047708511
1.89107358455658 -2.61272430419922
0.640853464603424 -1.05231475830078
0.42916351556778 -0.978138506412506
0.118367083370686 -2.03368020057678
-4.72324657440186 -0.197437793016434
1.16738510131836 -1.47790050506592
-1.11797571182251 0.222623199224472
0.860048651695251 -0.543204188346863
-5.11092472076416 0.161855950951576
0.593088626861572 0.0547161102294922
1.16097247600555 0.897686243057251
-0.517283916473389 -0.577468812465668
0.732181251049042 1.27799272537231
2.42652750015259 -1.53173220157623
1.0316960811615 -2.36038708686829
3.85751676559448 6.46333265304565
-2.27173209190369 0.0827447026968002
0.36083510518074 2.41281008720398
-2.96727204322815 -0.24631679058075
0.435127437114716 -2.39130067825317
-3.73178339004517 0.195466428995132
-0.172463536262512 0.168037325143814
-2.79084491729736 -0.140083983540535
-0.963679075241089 0.415666401386261
-0.121426716446877 -0.915931403636932
-2.73793292045593 -0.209012985229492
-2.29016137123108 -0.736587941646576
-5.28659105300903 0.0747693479061127
-3.21002960205078 0.21515366435051
-0.524387240409851 1.2067859172821
0.0545101165771484 0.794249296188354
-2.19566345214844 0.0893202424049377
-1.92270302772522 0.327785044908524
0.202718392014503 1.96950435638428
0.786624491214752 -0.892428159713745
-2.1657280921936 -0.487266898155212
-4.69246339797974 0.176840662956238
-5.28659105300903 0.0747693479061127
0.271729677915573 0.39826762676239
-1.36758852005005 0.169353649020195
-2.91727089881897 -0.128494873642921
-5.28659105300903 0.0747693479061127
-2.18426704406738 0.27059668302536
-3.6219425201416 0.0248079597949982
3.19575715065002 -3.35639452934265
-2.15240669250488 0.534764528274536
0.604182183742523 0.0199820511043072
0.818001866340637 1.87941253185272
-1.12089204788208 0.386809468269348
0.261841237545013 -0.988502502441406
-2.69046902656555 -0.118181176483631
-4.97585010528564 -0.0817979872226715
-2.66375708580017 -0.203066915273666
-3.92649960517883 -0.000203728675842285
-5.28659105300903 0.0747693479061127
0.189092889428139 -0.787330627441406
-2.69655084609985 0.019159622490406
1.98376166820526 -1.76030921936035
0.939421236515045 1.72618234157562
-4.14759206771851 0.349413603544235
-4.94594573974609 -0.0244247615337372
-3.39592623710632 -0.0472953319549561
1.67335879802704 0.706211388111115
0.745787799358368 1.50464880466461
-0.811968445777893 -0.131204411387444
0.734140992164612 0.758103609085083
-4.94594573974609 -0.0244247615337372
0.366382837295532 0.135693147778511
1.19775462150574 2.65101361274719
-4.5775933265686 0.0485123172402382
2.63164496421814 -3.01764559745789
-3.23210740089417 0.0146920122206211
2.14136457443237 -0.520588636398315
-1.89743876457214 -0.110417380928993
3.10338878631592 -3.71235752105713
1.22876882553101 0.452626585960388
-0.69747120141983 0.470105856657028
-5.28659105300903 0.0747693479061127
1.63435304164886 0.444687634706497
2.22348976135254 -6.7978458404541
1.19696724414825 0.372622102499008
-0.53198254108429 -1.30270063877106
0.920300483703613 0.934049963951111
0.0443475693464279 1.95366704463959
-1.26184678077698 -0.0872722268104553
-3.86911678314209 0.0507324151694775
-0.928438484668732 -0.0701755881309509
-4.27342796325684 -0.120681867003441
-3.27196264266968 0.237020552158356
-1.59244859218597 0.678800642490387
-1.62147748470306 0.178695529699326
-2.21799683570862 0.139908626675606
1.72748553752899 3.85544061660767
1.01067614555359 3.06579947471619
-2.17752647399902 -0.444228500127792
-4.8539514541626 0.060029149055481
-5.28659105300903 0.0747693479061127
1.92208981513977 -2.06477737426758
-0.661139369010925 1.02481484413147
-3.85950660705566 -0.270362824201584
-1.11064875125885 0.49871701002121
-1.47989058494568 -0.359804451465607
-2.03179574012756 0.368600636720657
-2.3937783241272 -0.484450399875641
-1.61426115036011 -0.242574453353882
1.33773481845856 -1.93718194961548
-0.569294333457947 0.00761784613132477
-5.25138902664185 -0.0634013935923576
-2.62333822250366 -0.00790614634752274
1.14626824855804 0.327629745006561
-5.25138902664185 -0.0634013935923576
1.26521301269531 0.640651524066925
-0.575461626052856 0.357213348150253
2.34036445617676 1.56882476806641
-3.50556874275208 -0.104991689324379
2.49934458732605 -0.802924752235413
-5.28659105300903 0.0747693479061127
-2.63267397880554 0.585945308208466
1.90254664421082 1.1632764339447
3.07847261428833 3.77571582794189
-2.43516135215759 0.284411430358887
3.21046805381775 1.98155641555786
2.358562707901 2.51148796081543
3.05271649360657 -3.29872894287109
-2.32306385040283 -0.299732595682144
0.798292636871338 0.801899552345276
-2.45255255699158 0.0217950716614723
-5.17622232437134 0.0767383500933647
-0.726464509963989 -0.426331132650375
-2.46228098869324 0.301272124052048
-4.36717319488525 0.0783631503582001
-2.41511249542236 -0.00629860907793045
-0.166334196925163 1.7912335395813
-0.604606509208679 0.373209565877914
-1.39884519577026 -1.32585692405701
-1.50767195224762 0.392098635435104
2.71121025085449 2.0953676700592
0.368882566690445 0.920737981796265
4.25283336639404 0.387242138385773
-5.25138902664185 -0.0634013935923576
-1.4843647480011 -0.0794502347707748
-0.438467770814896 1.03951358795166
2.61731719970703 -0.771659076213837
-4.75255441665649 -0.096436470746994
-4.14795589447021 -0.0555177144706249
-2.68085598945618 0.320960193872452
3.23219132423401 5.73718738555908
-0.310704350471497 -0.502583384513855
-3.86160063743591 -0.0241695195436478
-2.98096394538879 0.340688288211823
0.933151721954346 1.78375971317291
-0.0504913777112961 0.957870602607727
-2.96360850334167 0.216345399618149
2.17943787574768 -3.29567742347717
1.38005065917969 -1.65982234477997
1.16170883178711 -0.00488226301968098
-1.01388669013977 0.431031465530396
1.2338535785675 0.768055200576782
-1.96300601959229 0.335720926523209
-2.98399305343628 -0.0453365445137024
-2.03372144699097 0.0792832523584366
-0.633225083351135 0.322351515293121
0.954198181629181 -0.457496643066406
1.96287131309509 0.276444852352142
-1.21798193454742 0.528056085109711
-5.28659105300903 0.0747693479061127
0.540932238101959 -1.77357614040375
1.43911910057068 0.155272826552391
0.814110994338989 0.57826042175293
1.85100650787354 0.151199162006378
1.0393899679184 -0.168396025896072
0.0340022444725037 0.690424382686615
-4.68303394317627 0.167499378323555
0.788175225257874 0.616452813148499
-1.66379761695862 1.5139467716217
2.20729446411133 0.332225978374481
-5.25138902664185 -0.0634013935923576
-2.23410058021545 -0.249593913555145
3.90982246398926 -0.768489480018616
-3.17437124252319 -0.0725657418370247
-2.57480263710022 0.315677523612976
1.2238495349884 0.204665467143059
-1.54070663452148 0.388569295406342
-5.28659105300903 0.0747693479061127
1.05008935928345 1.64782965183258
-0.902503252029419 0.427741378545761
0.975820422172546 1.46839094161987
-2.55735015869141 -0.444125384092331
-5.28659105300903 0.0747693479061127
-3.94699883460999 -0.15822234749794
-0.270418077707291 -0.263256072998047
-3.78682065010071 -0.0933535471558571
1.939661860466 -1.74687480926514
0.182963162660599 -0.593385577201843
0.33044558763504 1.46684896945953
-5.11128234863281 0.0359737575054169
-3.53003740310669 0.340247452259064
-2.70157146453857 0.215725362300873
-0.672628462314606 0.876092493534088
-0.910512864589691 -0.131889522075653
-3.38152575492859 -0.16225677728653
-0.199971973896027 0.551126003265381
-1.55284643173218 0.719524681568146
1.55607402324677 -1.1140878200531
2.74368405342102 -0.101737946271896
2.36770105361938 -0.475697100162506
0.206600457429886 -1.08781802654266
-1.34996902942657 0.857894837856293
-0.55316698551178 0.163382261991501
0.494753003120422 -1.74856626987457
-3.06087970733643 -0.108881860971451
-1.74117088317871 -0.213173612952232
-4.91496992111206 -0.00582285970449448
3.921138048172 5.28466510772705
1.24458158016205 0.567506790161133
2.8731791973114 -3.3367486000061
-3.55607938766479 -0.0844303891062737
0.779899716377258 -2.65219306945801
-2.17553567886353 0.231587395071983
4.07887649536133 6.38676261901855
0.0251049026846886 -1.85354244709015
1.86822164058685 -1.64552044868469
-2.75894498825073 -0.0916931182146072
1.58404219150543 1.20430588722229
-2.16561079025269 0.190446600317955
-1.65826880931854 0.168819189071655
-3.24586200714111 0.000324726104736328
-2.20755338668823 0.23833379149437
-2.06818795204163 0.161274328827858
0.3224977850914 -0.608542799949646
1.21860671043396 -0.1349266320467
-1.17256832122803 0.382398813962936
-0.897792756557465 -0.958274662494659
-1.43277966976166 0.584275484085083
-0.277889162302017 -0.651160955429077
-3.30374312400818 0.288568258285522
-1.40788125991821 -0.517564833164215
2.5749626159668 1.36015605926514
0.782880187034607 0.548317670822144
0.205263167619705 0.50866836309433
0.946112632751465 1.96107685565948
1.28469920158386 2.17636346817017
-2.98987555503845 -0.152474761009216
-2.63190340995789 0.116962805390358
-5.25138902664185 -0.0634013935923576
-2.04812979698181 -0.195828288793564
-1.229825258255 0.50403767824173
-0.361567795276642 -0.821471810340881
-3.53662419319153 -0.230423226952553
-2.84346055984497 0.157331064343452
-4.94594573974609 -0.0244247615337372
-5.11092472076416 0.161855950951576
2.31438207626343 2.43644762039185
1.55571067333221 0.617212235927582
3.0285336971283 7.02329206466675
-0.607776463031769 0.496482133865356
-4.38911247253418 0.182191371917725
-2.93664526939392 0.0237289220094681
-5.25138902664185 -0.0634013935923576
-1.49064564704895 0.22226619720459
0.363370329141617 2.06459355354309
-2.79463958740234 -0.242012873291969
-1.8317574262619 -0.677954137325287
-2.7746913433075 0.345455706119537
-2.17597675323486 -0.373659700155258
-1.44200778007507 -0.0440402925014496
-0.716230511665344 -0.893951237201691
2.23308730125427 1.38882040977478
0.869725108146667 -3.28364706039429
-1.76873183250427 0.686025679111481
-4.74283266067505 -0.0636922866106033
-0.847696602344513 0.047733336687088
0.37298971414566 -0.669951498508453
-5.25138902664185 -0.0634013935923576
-5.11822271347046 0.0504489317536354
-0.393972307443619 -0.876935839653015
2.68201518058777 2.91051173210144
2.97157120704651 0.5372633934021
2.47552895545959 3.86455368995667
2.09400963783264 -1.60757064819336
2.91060948371887 -0.287160366773605
2.3796854019165 5.97517251968384
1.20686912536621 0.34814265370369
1.0062483549118 -0.582545936107635
-2.4711742401123 0.0516860783100128
-4.90894269943237 -0.266314744949341
-0.489486336708069 -1.41124868392944
-0.203790307044983 1.00004947185516
1.72648763656616 -0.768564164638519
0.346458435058594 0.114796251058578
-1.69209718704224 0.030450738966465
-1.15603470802307 -0.550235509872437
0.999120831489563 -0.339047968387604
-0.11738409101963 0.0433649867773056
-3.48607850074768 0.187437579035759
-0.60055810213089 0.0653186216950417
1.22610414028168 -1.96875321865082
1.47281062602997 -1.59328591823578
0.94429087638855 0.351325362920761
-4.26477336883545 -0.0181467402726412
-0.272453844547272 0.645252525806427
0.610243439674377 0.840481877326965
0.466961234807968 -0.537087261676788
1.40164184570312 0.838348746299744
0.262726277112961 0.957162380218506
2.70192885398865 -4.61913442611694
-2.34482431411743 -0.00912486761808395
-1.49590253829956 0.448449611663818
1.36148500442505 1.68959665298462
1.4038348197937 0.0430045425891876
0.104868896305561 -0.330452352762222
-0.839052379131317 -0.999063551425934
-1.41044342517853 0.227161183953285
1.89462959766388 -2.60584950447083
-1.44834566116333 -0.00102846324443817
1.4633800983429 0.0574106425046921
-3.1767201423645 -0.188139975070953
-2.37587809562683 0.149186760187149
-3.55571293830872 0.187982857227325
-0.102849647402763 0.044287234544754
-1.28305792808533 0.368916302919388
1.59658718109131 -2.49036860466003
-1.57953882217407 -0.124262407422066
-1.412677526474 -0.387567490339279
-1.74195146560669 -1.18876910209656
-5.28659105300903 0.0747693479061127
-1.09488952159882 0.769073724746704
1.63763236999512 0.0624575391411781
0.427304178476334 1.49888801574707
0.125508457422256 0.88370555639267
-4.79158306121826 0.0696697682142258
-1.08785140514374 -0.216607317328453
-0.586701452732086 0.140643179416656
-1.39813053607941 0.167965576052666
2.55611824989319 1.29062294960022
0.360647708177567 0.316938728094101
0.777469217777252 -4.22124481201172
-2.07418274879456 -0.300622582435608
-1.44766747951508 -0.223481491208076
1.26222097873688 0.821924865245819
1.09995055198669 -1.20844435691833
-3.01809740066528 -0.208657175302505
-3.36834144592285 -0.156947001814842
-3.85898065567017 -0.00338486954569817
2.31038665771484 3.03153586387634
0.135754331946373 -0.988071501255035
-1.9830493927002 -0.0155313834547997
1.13309025764465 0.916875064373016
-3.05132341384888 -0.0369063541293144
0.466129958629608 0.883035957813263
-5.28659105300903 0.0747693479061127
-1.66165935993195 -0.615032970905304
2.94172835350037 -7.26822566986084
-2.51910948753357 -0.0228407103568316
1.54028213024139 1.89247262477875
1.55582821369171 0.328860342502594
2.9443953037262 0.0975835174322128
-4.20263147354126 -0.0220255553722382
2.55128931999207 -1.61340188980103
-2.59034967422485 0.122735396027565
-5.25138902664185 -0.0634013935923576
-1.36852097511292 -0.0822475403547287
0.768580138683319 2.44716119766235
-0.980410993099213 0.104560032486916
-2.56823134422302 0.144256725907326
-1.49575972557068 0.408261358737946
2.07033467292786 0.176299020648003
1.86630153656006 -0.364609360694885
1.15868532657623 0.919603407382965
-0.0986488237977028 0.00639070570468903
-0.938688814640045 -0.339463949203491
-2.98479461669922 -0.185257166624069
-4.94594573974609 -0.0244247615337372
-0.89823055267334 0.189540654420853
1.3074654340744 -0.979707717895508
2.0519688129425 -1.92111384868622
-3.83769226074219 0.0357452742755413
-0.641769170761108 -1.22185075283051
1.51795446872711 -0.0430585108697414
1.64491283893585 -0.031015619635582
-0.609644412994385 1.21920323371887
-5.28659105300903 0.0747693479061127
-2.40229940414429 -0.260651707649231
-2.27255129814148 0.449576109647751
-1.70686602592468 0.0635044202208519
1.82691752910614 3.14042687416077
1.44243943691254 0.479892939329147
1.20833444595337 1.99939811229706
-4.98127269744873 0.00890202820301056
-2.6298942565918 0.157678842544556
3.836993932724 4.90348863601685
-0.7563436627388 -0.516600847244263
-1.50425601005554 0.283474802970886
1.02188038825989 -0.661672115325928
1.90134572982788 -1.89925372600555
2.98080253601074 -5.55205631256104
-3.32595658302307 -0.253439486026764
0.0782782956957817 1.03706848621368
-5.25138902664185 -0.0634013935923576
-3.22589039802551 0.226556867361069
3.07394814491272 5.5330171585083
-5.25138902664185 -0.0634013935923576
-2.21648263931274 0.113245211541653
-1.68004369735718 -0.0354145094752312
0.606436550617218 -1.82602035999298
2.18532299995422 -0.472372144460678
2.88630294799805 0.602417171001434
-1.47724461555481 0.102784231305122
-2.56139183044434 -0.180159851908684
-2.90058016777039 -0.301928997039795
-0.11828774958849 -1.33123767375946
-0.282840371131897 0.939014554023743
-1.95311105251312 0.0548268482089043
-4.37054777145386 -0.0117685571312904
0.299510568380356 -1.02250683307648
-2.78252768516541 0.202323898673058
-2.13561749458313 0.0639098584651947
1.11602389812469 1.1140958070755
-0.177163749933243 0.590549886226654
-3.26409077644348 0.1330736130476
0.335011780261993 -2.53318357467651
-1.06687688827515 0.360999137163162
1.67573606967926 0.239554777741432
1.74644470214844 2.45108413696289
-3.61527729034424 -0.00408505648374557
-2.05364894866943 0.329519331455231
3.43717265129089 5.44650173187256
-0.0188254881650209 0.0613121278584003
-0.736743807792664 0.2702916264534
0.421863734722137 -0.552434504032135
-0.923491299152374 -0.785340487957001
4.01068115234375 5.28674030303955
-3.14130806922913 0.21954034268856
1.9554750919342 1.19993436336517
2.21192693710327 1.07529580593109
1.49407601356506 0.631312310695648
-2.07942724227905 0.253071993589401
-0.831361949443817 -0.181059449911118
-4.02022743225098 -0.00320161879062653
-5.28659105300903 0.0747693479061127
0.911505699157715 0.652782678604126
0.193870648741722 -0.549483835697174
1.06185817718506 -0.385756433010101
2.37841606140137 1.40867388248444
-1.11913216114044 0.237539127469063
0.757456541061401 -0.903014302253723
-0.999580383300781 -0.0374462157487869
-5.28659105300903 0.0747693479061127
-0.080756738781929 -0.730625152587891
0.0948490053415298 0.749842882156372
-3.40281414985657 0.185708194971085
1.71214282512665 2.70407199859619
2.94080352783203 -0.55654388666153
-0.122629970312119 2.16676759719849
-5.28659105300903 0.0747693479061127
-1.71612763404846 0.155968010425568
0.170553654432297 1.23009157180786
-3.02415037155151 0.366937041282654
0.573585093021393 1.38066625595093
-0.149857223033905 -0.905726075172424
-0.789375007152557 0.021532416343689
-0.377112150192261 0.157211050391197
-2.03101849555969 0.257958024740219
-4.52153062820435 -0.161325395107269
2.51307940483093 -0.477063775062561
-0.764435648918152 0.294028043746948
1.38175559043884 4.20944023132324
1.8878425359726 -0.200026035308838
3.95918893814087 -2.1281270980835
1.48754441738129 -1.75827193260193
3.82373428344727 5.41528129577637
1.014120221138 2.8386607170105
3.03790807723999 8.4296236038208
-1.46724700927734 1.26823461055756
2.35655522346497 2.69783902168274
1.9888459444046 2.73213148117065
1.26587498188019 -0.668736636638641
-0.284122347831726 1.05486118793488
-5.25138902664185 -0.0634013935923576
1.3143059015274 0.0655162632465363
-2.93874859809875 0.268497467041016
3.37408304214478 5.38370704650879
-1.36249136924744 -0.349343657493591
-3.28522324562073 -0.235074013471603
-0.355140388011932 -0.378058791160583
1.02703070640564 0.901399612426758
3.26626992225647 3.93915414810181
-4.3255410194397 -0.0381341129541397
-4.91257905960083 0.04262475669384
-1.6059604883194 -0.0328114964067936
-2.74538087844849 0.211154937744141
-0.6933913230896 0.969901323318481
-0.0200609639286995 -0.0178323909640312
-5.08631992340088 0.0619744583964348
0.324192494153976 0.164085268974304
-1.46771919727325 -0.195368573069572
-3.26805877685547 0.613226592540741
-1.82041442394257 -0.307908266782761
-1.20947659015656 0.89463859796524
-1.50238180160522 -0.157779678702354
-2.01034927368164 0.0746361166238785
0.191801428794861 0.191866531968117
-0.109747149050236 -0.49403390288353
1.0632472038269 -0.42907389998436
-2.9295597076416 0.222368627786636
3.30100250244141 -4.35732698440552
2.39207053184509 -3.29570651054382
-4.14795589447021 -0.0555177144706249
1.73011088371277 2.43786239624023
1.89592278003693 -1.42112720012665
-4.08363199234009 -0.111570924520493
-1.49583065509796 0.866544783115387
-3.27859854698181 -0.185465946793556
-5.28659105300903 0.0747693479061127
4.0085072517395 -7.37924528121948
-2.78260111808777 -0.398578733205795
-2.56947422027588 0.282708466053009
4.13722705841064 -2.94397211074829
-1.91640532016754 0.41277489066124
-2.29562544822693 0.0496722012758255
2.16546869277954 -0.7153559923172
-0.776084780693054 0.396961390972137
0.0976145640015602 0.728349268436432
-4.08441877365112 -0.00787962973117828
2.1397488117218 0.302377223968506
3.56492328643799 5.2366681098938
1.42915046215057 -0.157531931996346
1.42022931575775 1.08852100372314
2.86912226676941 4.50804662704468
-3.13869524002075 0.183391526341438
-1.40668714046478 -0.085901215672493
-3.97384238243103 -0.0793392732739449
-0.10838358104229 -1.74194443225861
0.696764409542084 -0.813763022422791
-1.73817789554596 -0.534552395343781
1.66363120079041 -4.02793550491333
-1.30439758300781 -0.942829668521881
-0.0492317080497742 -0.560375571250916
0.0992298498749733 -0.345787048339844
2.13388633728027 4.06450700759888
0.0372134149074554 -0.875882744789124
-0.547924876213074 1.41542649269104
0.071831114590168 -0.614452600479126
-0.53219074010849 0.0345738418400288
0.210518062114716 0.751394867897034
-4.9385232925415 -0.109001837670803
-5.13650608062744 0.0522455610334873
-2.39310789108276 0.342227905988693
0.776417851448059 2.07560539245605
-5.28659105300903 0.0747693479061127
0.483450174331665 -2.18411707878113
0.362660020589828 -1.67728495597839
-2.91646432876587 0.0610982067883015
2.74444675445557 3.84957146644592
-4.8497486114502 -0.102037101984024
2.3189263343811 2.19200897216797
-1.24190330505371 -0.741761684417725
-0.663963735103607 -1.4086127281189
2.14135146141052 3.85301923751831
-5.28659105300903 0.0747693479061127
-0.609962344169617 0.170575141906738
-1.09913969039917 -0.0489207580685616
2.3017213344574 3.99801349639893
2.21284174919128 -1.22282612323761
0.229585140943527 0.59122759103775
2.44468998908997 -0.662278294563293
2.0599308013916 0.999079942703247
2.29784750938416 2.2300763130188
1.59294390678406 -0.53473973274231
1.94260108470917 2.18604135513306
-1.74227869510651 -0.225826695561409
-1.54437375068665 0.0798650234937668
0.705746591091156 0.813600599765778
2.9423234462738 1.49481165409088
-0.040375605225563 -1.01195347309113
-0.948171734809875 -0.941897749900818
-0.853287816047668 -0.227282419800758
-4.51024103164673 -0.031259223818779
-0.721885025501251 -0.383087903261185
2.20542287826538 -4.48063516616821
2.11166143417358 1.54197227954865
2.42973518371582 4.74966859817505
0.467683583498001 0.692959904670715
-1.60292935371399 0.0425649248063564
1.92216444015503 2.04517030715942
-1.48468625545502 -0.291207849979401
-5.28659105300903 0.0747693479061127
3.08242797851562 0.520977079868317
-0.102752774953842 -0.419494867324829
1.06773388385773 -0.375157535076141
-1.47012615203857 0.0790545716881752
0.616166830062866 -0.507212221622467
-1.95829916000366 0.547617256641388
-2.07570695877075 0.0142565052956343
-0.626905381679535 -0.394540816545486
0.505535662174225 -1.89459919929504
1.3741215467453 2.21180105209351
0.873108565807343 -1.12959611415863
2.35632658004761 1.67741453647614
-1.24115693569183 0.114673033356667
-5.28659105300903 0.0747693479061127
-5.28659105300903 0.0747693479061127
0.700808107852936 -0.533034265041351
-1.72424912452698 0.29304376244545
-0.177377715706825 -0.597979128360748
-4.55945444107056 0.0664704442024231
0.673022150993347 0.389978647232056
-2.90093374252319 -0.278927087783813
0.176785752177238 1.17261552810669
2.34514784812927 -1.71908938884735
-4.00940752029419 0.223800480365753
-3.57087874412537 -0.107704348862171
-1.87558889389038 -0.129827111959457
-3.37193512916565 -0.149062067270279
-3.07377600669861 0.3526271879673
1.02437794208527 -3.38535523414612
-5.28659105300903 0.0747693479061127
2.46104884147644 -1.32467901706696
0.738330185413361 1.65823066234589
0.160761207342148 0.0188323594629765
-1.40604662895203 0.627036392688751
0.322384715080261 -0.378442227840424
-1.55981683731079 0.00802678242325783
0.323905229568481 -0.306610405445099
-0.265119880437851 2.02157402038574
0.572814881801605 0.527345359325409
0.338916331529617 -1.48855543136597
0.163945987820625 -0.67553585767746
-1.36248481273651 -0.130599647760391
-3.57005167007446 -0.178271099925041
0.614189743995667 3.17674016952515
2.20922160148621 -1.10241627693176
1.76164615154266 2.29371976852417
2.72870278358459 0.739211678504944
2.17019319534302 1.62687408924103
2.12416291236877 -1.75069785118103
-3.18725037574768 -0.312442302703857
-2.33153200149536 0.222703337669373
-0.726743280887604 0.26013046503067
-4.07262468338013 -0.0923676118254662
-3.57661390304565 -0.0421800911426544
0.0657737478613853 1.5057954788208
-4.57190465927124 0.0827232152223587
3.60503721237183 3.70191025733948
0.0211897678673267 0.561990439891815
-1.8418824672699 0.103824995458126
-4.94811487197876 -0.151801481842995
0.868519484996796 -1.24648606777191
0.835112452507019 0.639345347881317
2.10464310646057 -2.39797687530518
-3.73764395713806 -0.198205947875977
-4.3470983505249 -0.26384037733078
2.89551877975464 1.29550385475159
0.124002180993557 -0.252877801656723
3.08411645889282 3.60510182380676
-1.33500564098358 -0.630428552627563
-2.62169337272644 -0.320089936256409
-2.60843420028687 -0.799101114273071
-3.66411328315735 -0.0482608526945114
-5.28659105300903 0.0747693479061127
-3.05273866653442 0.106482230126858
0.289338797330856 0.845300674438477
-0.279150068759918 0.700823724269867
-1.65507590770721 -0.0164186656475067
-2.67085003852844 -0.365905553102493
2.41369533538818 -2.14936470985413
-2.08393454551697 -0.162497043609619
0.0246452689170837 -0.296306192874908
0.457032889127731 0.254954725503922
1.10186040401459 -3.22723317146301
-3.14033126831055 0.159325495362282
1.10971701145172 0.0510395020246506
-0.404103219509125 0.770764648914337
0.428040534257889 -0.391592592000961
-2.71585440635681 -0.0775390714406967
1.75315308570862 1.64322280883789
-0.892570376396179 -0.265084743499756
-2.55729842185974 4.34964895248413e-05
-0.283613234758377 0.404623806476593
-2.06336355209351 0.241255834698677
-0.142676800489426 0.312639862298965
1.89355456829071 2.67008233070374
3.10006713867188 3.02819204330444
1.93381881713867 -1.51758313179016
0.70176362991333 -0.667910575866699
3.23712635040283 0.0517450198531151
-1.24652576446533 -0.183631479740143
-2.53499460220337 -0.0858130231499672
2.28932976722717 -1.13251769542694
-3.0649688243866 -0.345628708600998
1.83543884754181 -0.101033054292202
-0.755997657775879 0.558345198631287
0.530239284038544 -0.925487577915192
0.977478921413422 0.305440813302994
2.87261462211609 8.93292140960693
-1.07534575462341 -0.866236686706543
-0.581736624240875 -1.26478826999664
-5.28659105300903 0.0747693479061127
-0.158210426568985 2.14863300323486
-2.88955235481262 -0.0819382220506668
2.38415670394897 0.00227505713701248
0.421584337949753 -0.504429161548615
-4.61020612716675 0.0736362114548683
0.115514561533928 3.02954030036926
-4.58276653289795 -0.0278175175189972
1.74834704399109 0.798033773899078
-2.25326633453369 0.295207351446152
-0.946639716625214 -0.320464253425598
2.13433980941772 -0.595540642738342
-0.49218487739563 -0.0751071125268936
2.53715181350708 2.87024641036987
0.799052953720093 0.849985420703888
0.842178285121918 0.7658371925354
1.70154571533203 -1.50318729877472
-5.28659105300903 0.0747693479061127
0.406889230012894 2.48504638671875
-0.239900186657906 0.429885685443878
2.51770853996277 -3.02557826042175
-5.25138902664185 -0.0634013935923576
-0.251727283000946 0.324528247117996
-2.79862284660339 0.113186612725258
-5.25138902664185 -0.0634013935923576
1.69110119342804 1.67126202583313
-5.28659105300903 0.0747693479061127
-1.64563143253326 0.178987398743629
-5.28659105300903 0.0747693479061127
-1.42970848083496 -0.220678329467773
-3.28484678268433 -0.21906989812851
0.465394079685211 -0.0212261006236076
0.778101444244385 -0.504362285137177
-4.70472574234009 0.0392222702503204
-3.26961994171143 0.561105906963348
1.00899195671082 -2.2348964214325
-1.81877422332764 0.577469646930695
-1.07507085800171 -1.01446497440338
0.210544139146805 -1.78735983371735
1.74434447288513 -3.19631862640381
0.244802325963974 0.157381191849709
-2.84962630271912 0.0858372375369072
0.063172347843647 -1.81853580474854
1.3735020160675 -1.25732243061066
-5.28659105300903 0.0747693479061127
-0.869702100753784 -0.548589825630188
-0.804757297039032 0.26482167840004
2.12721633911133 -1.47008788585663
-0.283775717020035 -1.42103672027588
-3.2447350025177 0.138981759548187
0.847298979759216 1.989861369133
0.171084344387054 0.282331645488739
-5.28659105300903 0.0747693479061127
-2.50743579864502 0.740926146507263
1.1267774105072 -0.889835000038147
2.52179932594299 -2.16958785057068
-2.56318187713623 -0.424582093954086
2.80375456809998 4.92934131622314
-1.82382023334503 0.122006595134735
-3.01523542404175 0.0218198448419571
-4.5717921257019 0.172848775982857
3.46310329437256 2.97903370857239
-2.99825811386108 -0.201012760400772
-0.187142595648766 -0.597564518451691
-3.01336526870728 0.169981300830841
-2.47094440460205 -0.160802975296974
-4.61280107498169 0.104933045804501
-1.10259187221527 -0.197701171040535
-5.25138902664185 -0.0634013935923576
0.61030101776123 0.579790115356445
1.48369467258453 1.87931191921234
-0.00646661594510078 -0.982807755470276
1.28254401683807 0.429385364055634
-1.0501856803894 -0.576681435108185
-1.50763738155365 0.250573843717575
1.4880256652832 -0.0500584281980991
-5.28659105300903 0.0747693479061127
1.87225186824799 0.281615406274796
0.345717042684555 2.59411907196045
-2.67458724975586 0.345144838094711
1.88252508640289 1.30065155029297
0.476956605911255 1.47558867931366
1.26107478141785 2.03625535964966
-0.656276822090149 -0.418479710817337
-2.32256937026978 0.475029110908508
0.8485267162323 -1.5581841468811
-0.0857878625392914 0.216819792985916
-5.25138902664185 -0.0634013935923576
0.54511433839798 -0.0140588656067848
-0.476208984851837 -0.691220939159393
1.14858210086823 -0.703821659088135
-0.669962465763092 -0.329134166240692
-4.40686988830566 0.004999078810215
-1.65469574928284 0.102384924888611
-5.15017175674438 0.0431982204318047
-1.42704224586487 0.651723921298981
2.85840106010437 0.396544367074966
0.201504126191139 -1.66401767730713
-2.33629179000854 0.0949158221483231
3.19461154937744 6.31242990493774
0.201123759150505 -0.391538858413696
-0.331759035587311 1.17678606510162
-1.8732705116272 -1.05845308303833
-3.21830582618713 -0.0418754257261753
-4.26255083084106 -0.134864673018456
3.07616662979126 -7.23438787460327
-2.48950529098511 -0.281636744737625
-3.0383574962616 0.173182994127274
-0.961869478225708 0.215153604745865
0.903566122055054 0.948023080825806
0.496730327606201 0.453819513320923
-0.432817012071609 -0.0707906559109688
-3.19844079017639 0.193450883030891
0.0647315680980682 -1.77412569522858
-1.50686264038086 0.773222804069519
0.494939863681793 -0.413321435451508
-1.63429057598114 -0.359764814376831
-0.227275878190994 0.00389896333217621
-4.4768009185791 0.0885276719927788
-2.84126377105713 -0.26517391204834
3.64755058288574 -0.629638314247131
-4.27342796325684 -0.120681867003441
-0.626866936683655 -0.0771962627768517
-0.861945986747742 -0.0408412180840969
2.19625544548035 -1.31002378463745
4.15501642227173 3.99246430397034
0.546137392520905 -0.333187103271484
-3.50198483467102 0.0524974688887596
-1.8635014295578 -0.401333421468735
-2.88340902328491 0.207535549998283
3.04568767547607 3.70360326766968
-1.39694929122925 -0.370830416679382
-1.90721690654755 0.795103549957275
-2.1712658405304 0.163769066333771
-1.93421685695648 0.438837379217148
-1.94022142887115 0.41565278172493
3.19136238098145 5.07839012145996
1.83239841461182 1.35188162326813
-4.84659385681152 -0.0156503543257713
2.24385118484497 -1.00620651245117
-5.25138902664185 -0.0634013935923576
1.6566675901413 1.80720818042755
-5.03697967529297 0.0971906930208206
};


==> figures/visualizations/funnel/dds_samples.tex <==
\addplot [semithick, dds, opacity=0.7, mark=x, mark size=3, mark options={solid}, only marks]
table {%
-0.921514928340912 0.594062089920044
-1.0408456325531 -0.0469527542591095
-0.403298676013947 0.417708992958069
-1.86252665519714 0.0598455183207989
-0.325799494981766 0.828166961669922
0.980258941650391 0.280052483081818
-2.78342986106873 0.0222004484385252
0.724721014499664 0.899542808532715
2.52636981010437 -1.35874092578888
0.776564419269562 -1.5110239982605
-0.618643760681152 1.2728499174118
-2.9869430065155 -0.00579096470028162
-1.06686055660248 -0.876945614814758
-0.509259343147278 1.42623341083527
0.299991577863693 1.45830035209656
-1.4195704460144 -0.271007478237152
-0.66979318857193 0.407076358795166
-0.00822763051837683 0.968589305877686
0.0362334027886391 -0.966760218143463
-2.0359034538269 0.136888906359673
-3.16836428642273 -0.110834024846554
0.402885496616364 -2.80471014976501
-2.58571267127991 0.169843211770058
0.603599369525909 -0.46825510263443
0.988546550273895 -2.83900880813599
-0.496743649244308 0.478558272123337
0.688651144504547 -0.218827664852142
-0.737736523151398 1.233238697052
1.06459295749664 0.928434431552887
-0.481838345527649 -0.986110746860504
1.66364514827728 2.14804887771606
-0.686748564243317 -0.257582753896713
1.39011776447296 -0.626693785190582
-0.75702953338623 1.51672649383545
1.56779778003693 0.189011290669441
-1.83561205863953 0.0808421224355698
-1.13771295547485 0.571516215801239
0.460271179676056 2.22528886795044
1.38772666454315 2.73824501037598
-0.736450254917145 0.0444070585072041
-0.595483422279358 -0.0778501778841019
-2.41054081916809 0.00282569508999586
-3.52849888801575 0.0825281515717506
-1.7935893535614 0.138622254133224
0.62890499830246 1.2077260017395
1.0911545753479 3.96547389030457
-0.329901248216629 -2.10178542137146
0.643274307250977 -0.826205790042877
-3.01301145553589 -0.341649353504181
-2.84512877464294 -0.361689180135727
-0.468248695135117 -0.744709968566895
-2.75716328620911 0.0439929701387882
-3.02554035186768 0.0446886084973812
0.031296119093895 1.24737727642059
0.413143783807755 0.546773791313171
0.424715220928192 2.47992372512817
-1.42054772377014 -0.195829749107361
2.14440655708313 -1.43567526340485
-3.01520490646362 0.0500456839799881
-1.04509508609772 -1.01265358924866
-0.378986418247223 0.263127207756042
-0.733149647712708 -0.00248250621370971
-0.73217785358429 -0.723117768764496
0.576662182807922 -0.720098495483398
0.0212354809045792 0.966144800186157
-1.26359415054321 -0.0496163927018642
-1.23940193653107 0.507522761821747
0.907080769538879 0.0909892469644547
-0.72646701335907 0.645088016986847
-1.43978083133698 -0.519311487674713
-1.35706377029419 0.328902631998062
-3.21985816955566 0.484629839658737
0.336975008249283 0.844619691371918
-0.365550965070724 0.518713057041168
-2.35137486457825 0.770405948162079
-1.47010517120361 -0.104052148759365
1.34387731552124 0.0309782791882753
-2.47625994682312 -0.101123973727226
1.48994863033295 1.1068354845047
-1.72069990634918 -0.115198902785778
0.822281718254089 -2.42002606391907
1.02142822742462 0.172206848859787
1.01335418224335 -2.12852478027344
1.68111562728882 4.85426902770996
0.424209773540497 0.0513713993132114
-1.94708645343781 -0.1081378236413
0.501090705394745 -0.537474274635315
-3.33987188339233 -0.00231080548837781
-1.4348087310791 -0.337766945362091
-3.21317481994629 0.365809321403503
0.404077619314194 -0.227212071418762
-1.43668627738953 -0.669118463993073
0.20965288579464 -0.526121616363525
-0.757301092147827 1.63549840450287
-0.503385663032532 -0.241204887628555
-1.6094776391983 0.311434626579285
-3.36317253112793 -0.148761928081512
1.65480506420135 0.785708010196686
-3.15729475021362 -0.383081942796707
1.72382271289825 1.86420869827271
1.38514077663422 -0.47161802649498
0.994292318820953 -2.79473543167114
0.488420367240906 1.52878046035767
1.42347061634064 2.51529240608215
-0.16366058588028 -0.477582365274429
-0.871601045131683 1.05269587039948
0.00947537738829851 0.365561813116074
-1.28869831562042 0.708625137805939
-2.45968627929688 0.516891539096832
-1.51006877422333 -0.375990062952042
-1.18031477928162 -0.265795886516571
0.37612909078598 0.363419979810715
1.42617726325989 -0.213974967598915
1.17854964733124 0.585037410259247
-1.42954933643341 0.941501796245575
0.702565371990204 1.56834995746613
-1.4582587480545 -0.272242695093155
-1.76705837249756 0.561552464962006
-1.14811134338379 -0.159358620643616
2.27204966545105 2.75939130783081
0.158388137817383 -3.33548998832703
1.86126363277435 1.28333699703217
-2.00946736335754 -0.554425001144409
-0.411982417106628 0.666445076465607
0.714050650596619 -2.60962510108948
1.11706149578094 -0.0841452851891518
1.45374059677124 0.897735774517059
2.31459021568298 -2.08451890945435
-0.706868052482605 -0.11716902256012
1.33286380767822 -3.47532272338867
0.691499292850494 1.15558850765228
-2.58861994743347 0.658887028694153
0.841383099555969 -2.77691221237183
-0.109033107757568 -1.61380970478058
1.4572662115097 1.92686212062836
-2.19159340858459 -0.46237775683403
0.913262248039246 0.960172295570374
-1.3689112663269 0.879914581775665
0.508045792579651 0.937371909618378
0.406731009483337 -1.21644449234009
0.512734293937683 1.23675680160522
-0.111122339963913 -1.0667370557785
-1.37171268463135 0.422449707984924
-2.13819193840027 0.0990833416581154
-0.402571141719818 -0.0990999713540077
0.344901710748672 -0.578256249427795
-3.00969743728638 -0.0731966495513916
-4.91554546356201 0.00857896450906992
-1.44869160652161 0.15805496275425
1.17863512039185 1.10001182556152
-2.30365800857544 -0.289734601974487
0.78667813539505 -0.395659506320953
0.916543483734131 1.67793774604797
0.952294170856476 -2.05735731124878
-1.35933649539948 0.438086658716202
1.0531964302063 -0.0488663762807846
-0.306697130203247 0.365193247795105
0.0215509291738272 -1.24086475372314
-1.56344294548035 0.470257937908173
0.910698413848877 0.891294538974762
-1.25032043457031 -0.189614936709404
-0.591800510883331 -0.172030493617058
-1.36620461940765 -0.242307931184769
-0.407868415117264 1.14501249790192
0.321618378162384 -0.546629130840302
-2.28555941581726 0.456463426351547
1.19193696975708 -1.77923774719238
2.08668565750122 -2.26433038711548
0.6166011095047 1.35256230831146
0.933075904846191 1.05672264099121
-1.26882970333099 -0.173463225364685
1.51880764961243 1.9677631855011
1.32636535167694 -0.801212668418884
1.07584404945374 1.32159554958344
1.28551232814789 -0.640998482704163
1.03167748451233 0.0296609587967396
-1.5621896982193 -0.0430805794894695
-1.79349708557129 0.0098993144929409
2.4640793800354 2.42560076713562
1.69427597522736 -1.60714030265808
-0.19528403878212 -1.15142846107483
-0.584648728370667 1.05667555332184
-0.64982807636261 0.200542032718658
-0.381396114826202 -0.820915818214417
0.357820332050323 -0.654190421104431
1.16640257835388 -4.72538805007935
0.0540948212146759 -0.191226437687874
-0.842465698719025 1.32132995128632
0.699360132217407 0.0142981261014938
2.34360408782959 1.31774270534515
2.62122201919556 -4.8503212928772
0.969786286354065 1.2625093460083
-1.86079359054565 0.213442802429199
-0.758123397827148 -0.409913867712021
2.21290516853333 1.45479309558868
-1.57186377048492 0.475984483957291
2.75401496887207 3.76558470726013
-3.20441365242004 -0.288249313831329
-0.603297531604767 0.908406257629395
1.04610693454742 2.01218390464783
-1.43949329853058 -0.455673784017563
-1.20303797721863 -0.174403369426727
-1.05238509178162 0.798758208751678
-1.97938346862793 -0.962891578674316
1.44863295555115 1.09684479236603
-1.23833787441254 0.341226816177368
0.389756739139557 0.668559968471527
-2.67847800254822 0.519697368144989
0.730277419090271 0.630944013595581
1.08726668357849 -1.5761786699295
-0.573158264160156 -0.315093487501144
-0.719898879528046 -0.239074215292931
0.634666442871094 -3.48061919212341
1.99729216098785 -1.58269381523132
1.67632031440735 -3.05553245544434
-0.157839149236679 -0.135258808732033
1.33485972881317 -0.588094174861908
1.94618499279022 0.523250341415405
0.354072153568268 1.11257147789001
0.736200630664825 -0.971276819705963
-0.843776166439056 -0.611438572406769
-0.261053174734116 -0.0942483395338058
0.628643274307251 -0.432750046253204
0.0175020713359118 0.328298360109329
-5.36803579330444 -0.022009426727891
-5.429274559021 -0.0679889023303986
1.10776174068451 0.169283553957939
-1.88617765903473 0.0045964177697897
-2.9019570350647 -0.158092364668846
-4.1190299987793 -0.10868176817894
1.12971818447113 2.12765550613403
-2.84593272209167 -0.078856848180294
1.96892917156219 -2.19904851913452
-0.923842966556549 1.06716549396515
3.11549854278564 -8.30645084381104
-0.694634974002838 -0.396660357713699
0.101776905357838 0.774084627628326
-1.27110981941223 0.575208902359009
-2.41296219825745 -0.172880262136459
-0.756208956241608 -0.213369086384773
-0.500189900398254 -0.383381754159927
0.832003116607666 0.705798089504242
-1.34017133712769 -0.162816777825356
0.532435059547424 -1.70796954631805
-2.29455399513245 0.222968310117722
2.09555673599243 3.69459438323975
1.20077669620514 2.69988656044006
-2.43739247322083 -0.191491305828094
-0.138332441449165 0.981971323490143
0.629258334636688 2.34664416313171
-0.580563962459564 0.977376103401184
-2.58741140365601 -0.238922029733658
-0.0798007994890213 0.47150045633316
-4.33847427368164 -0.0622708573937416
-0.761737763881683 0.126678347587585
-2.62091135978699 0.276108086109161
1.90095674991608 1.47479009628296
0.0825029313564301 0.771467924118042
-0.27900093793869 -1.7181624174118
-1.93969428539276 -0.356223821640015
1.61884105205536 0.199686542153358
2.69097208976746 2.23035645484924
-0.553414762020111 0.308588415384293
-0.642735421657562 -0.440109044313431
-2.65173530578613 -0.731578409671783
-0.699485778808594 -0.619810044765472
-0.0389091074466705 1.33442401885986
-2.62791347503662 -0.0856879875063896
0.4386106133461 -0.363607048988342
0.86569607257843 0.446425080299377
0.0103262048214674 0.405901461839676
1.10841631889343 1.33945631980896
1.57481229305267 -3.0290150642395
0.0680895820260048 0.793704271316528
-1.62824642658234 -1.06021344661713
-2.60089468955994 -0.0901461616158485
-2.2786602973938 0.339358985424042
2.00133275985718 -1.38180196285248
0.753821432590485 1.33911824226379
0.355981528759003 1.56267046928406
1.95837616920471 0.357557326555252
-0.200077593326569 0.950294375419617
-0.151893585920334 -0.572892487049103
-0.558484077453613 1.28404819965363
-0.457643121480942 -0.326695889234543
-3.3148500919342 -0.178467288613319
3.12229990959167 -4.78222322463989
-1.68543803691864 0.686543822288513
-0.147146388888359 1.23832070827484
0.324599266052246 1.4767906665802
-1.22829067707062 0.724780261516571
1.22695004940033 2.45472741127014
-0.266847282648087 -0.159268319606781
1.54823684692383 -1.36143684387207
-0.609855473041534 -0.580667853355408
-2.05628228187561 0.191028475761414
-0.0654278546571732 -1.67116475105286
1.2572910785675 -2.65528321266174
-2.3501763343811 -0.00867137126624584
-0.888954281806946 0.679247140884399
-2.10054302215576 0.269866913557053
1.05485451221466 -2.25776839256287
-0.532231688499451 0.0671077743172646
-0.37647870182991 -1.14258444309235
-2.84052920341492 -0.0966911986470222
-0.484214574098587 0.176938965916634
-0.246893003582954 -0.462254405021667
-0.0150313852354884 -0.021975539624691
-0.450908720493317 -0.79668664932251
1.44616365432739 3.64547085762024
-1.39228904247284 1.21675038337708
0.666035115718842 -2.3494348526001
0.969023644924164 -1.25773513317108
-0.364223659038544 2.08637738227844
1.74114942550659 1.36584424972534
-1.2351301908493 0.733632624149323
0.953739881515503 0.292645573616028
-1.31377995014191 0.691860914230347
-0.228861108422279 0.686046957969666
0.0606450699269772 0.378558725118637
-0.49353888630867 -0.157686918973923
1.24419903755188 1.09977996349335
-2.92184162139893 -0.10987763851881
0.275864988565445 -1.24842894077301
0.323127180337906 1.44936728477478
-1.10888969898224 0.0921794772148132
1.09638607501984 -0.0251891482621431
-1.22258770465851 -0.161496222019196
0.545646727085114 -0.0539846979081631
-4.77278423309326 -0.0382999293506145
-2.65343022346497 0.552055239677429
1.06708717346191 -0.220971778035164
2.0551643371582 0.0073135057464242
-0.83293229341507 0.966099858283997
-1.06904685497284 -1.57502329349518
-2.57244849205017 0.0483031831681728
0.20912267267704 -0.430617600679398
-4.51094818115234 -0.242171183228493
-1.37031638622284 0.0245004817843437
0.49731382727623 -1.94984030723572
0.150544673204422 -0.0896296426653862
-0.484108150005341 -0.358145177364349
-0.609343230724335 0.295900970697403
0.167371436953545 -0.585505664348602
0.957076132297516 -0.638912558555603
0.270380556583405 1.30913555622101
1.84773635864258 -3.41434216499329
-1.82635486125946 -0.0822633728384972
1.03643035888672 1.60888886451721
-1.13157737255096 -0.103798769414425
-1.79022753238678 0.174412369728088
-0.954403817653656 -0.0777687504887581
0.529025137424469 -0.497626066207886
-1.72530603408813 -0.0949542745947838
1.46649122238159 0.830231308937073
-2.49199104309082 -0.0379850678145885
-0.730908930301666 0.712191164493561
0.205697938799858 0.263175368309021
-0.0477460846304893 -0.412156760692596
-3.25286078453064 -0.0421052947640419
-1.01941967010498 -0.135523214936256
-1.50403738021851 0.156209319829941
2.59832406044006 -1.48897480964661
0.0602256767451763 -0.209235489368439
-2.33390045166016 0.535172164440155
-0.750222086906433 0.656017899513245
1.4707692861557 1.49560463428497
0.67714387178421 0.739260375499725
0.0650132521986961 -0.197208091616631
-1.95011270046234 -0.0930250808596611
-0.18375064432621 -1.14023649692535
-0.758267045021057 0.735333979129791
-0.727023184299469 -0.170494452118874
1.72395980358124 -0.713494300842285
1.73447823524475 4.34507656097412
-0.345160365104675 2.12874341011047
0.418469101190567 1.09240007400513
-2.00032353401184 -0.440735071897507
-1.21934449672699 -1.0833352804184
2.46535849571228 4.20490550994873
0.24064114689827 0.321470946073532
-2.67143273353577 0.221404552459717
0.938436388969421 0.331805288791656
-0.451192289590836 -0.701695322990417
1.4247100353241 -1.79775774478912
-4.04809284210205 -0.222826927900314
-1.63009321689606 -0.474570542573929
-1.3598667383194 0.352885037660599
-2.70294713973999 -0.410922259092331
0.641592264175415 -1.91494369506836
-1.29263412952423 0.298834353685379
2.82258057594299 7.71265840530396
-3.96208095550537 0.20400695502758
0.0672686174511909 -0.88586413860321
1.24217402935028 -0.789637684822083
2.70708060264587 -0.99083811044693
-1.92887949943542 -0.204316601157188
2.1268105506897 -2.91000509262085
1.56712830066681 -2.0799458026886
0.726367115974426 1.77432668209076
-2.28625226020813 0.710385024547577
-4.74652576446533 0.114431485533714
-1.96977984905243 0.322585433721542
1.24730014801025 3.00900197029114
1.95552933216095 0.341133534908295
-1.36827993392944 0.349052906036377
-0.431986570358276 -0.0640227869153023
-0.0401140674948692 0.0076641789637506
-2.1733877658844 0.818334519863129
2.48221731185913 -1.83196067810059
-1.73852503299713 0.625665545463562
-0.334589630365372 -1.2691478729248
3.17617511749268 1.16270363330841
0.993674397468567 2.40798401832581
-2.46421551704407 -0.0289232823997736
0.0670879706740379 1.17220604419708
0.692641198635101 0.476469963788986
0.967220425605774 0.333780318498611
-0.75429767370224 0.415642201900482
0.838551938533783 -2.44061589241028
-1.157151222229 -0.0278986692428589
-3.46539616584778 0.117041304707527
-1.90920305252075 0.348896086215973
-2.21332716941833 -0.205112248659134
-0.0987298712134361 -1.21940791606903
-1.84283077716827 -0.0403237603604794
1.51171267032623 0.422439306974411
-3.051997423172 -0.434951156377792
0.856245398521423 1.64848291873932
-1.6949816942215 0.0616666674613953
1.2584456205368 3.38307619094849
2.15600490570068 2.82130146026611
3.64741253852844 1.21750688552856
-0.607696115970612 -0.0480738878250122
-0.962533116340637 -1.3504878282547
-2.12436413764954 0.175596669316292
-0.77080774307251 0.714791059494019
-1.24542641639709 0.041168674826622
0.741668164730072 -1.03167724609375
-0.963433742523193 -1.08761405944824
-2.0350649356842 -0.128644317388535
-0.860984265804291 -0.574734449386597
2.22519302368164 1.32996809482574
-1.47525036334991 0.357216894626617
1.63234412670135 0.763799667358398
1.93325805664062 2.40175628662109
1.9539520740509 1.59870231151581
-0.756351172924042 -1.21833491325378
0.411191582679749 1.42737281322479
2.1231746673584 2.69494771957397
1.53705132007599 -2.93080377578735
0.103159576654434 -0.586139917373657
1.92826724052429 1.08412611484528
-3.41905117034912 0.127854570746422
-2.94193029403687 -0.423860102891922
-2.93707132339478 -0.512837469577789
-2.29819488525391 0.39236256480217
-0.873736202716827 0.112618736922741
-1.77673828601837 0.302079975605011
2.35477614402771 2.81303882598877
0.431576579809189 0.0842849463224411
-1.35105454921722 0.57514625787735
-3.79784941673279 -0.139604613184929
1.09833991527557 -3.88521289825439
0.0161739848554134 2.01045155525208
-1.08621990680695 0.781574487686157
1.07111144065857 2.91171622276306
2.63223195075989 2.63144969940186
0.731552124023438 -0.685310184955597
0.300888657569885 -1.81287682056427
-1.86209762096405 -0.790555655956268
-1.38228952884674 -0.581836044788361
-0.02149130217731 -0.287725478410721
0.0925840064883232 -0.020250279456377
0.348517209291458 2.10239863395691
0.267779946327209 1.34843635559082
-2.34328532218933 -0.165371045470238
-1.05224347114563 0.169869497418404
-2.22423052787781 -0.742097914218903
-1.75402557849884 -0.0880921259522438
-1.59794104099274 -0.101192735135555
-3.12379956245422 0.0769669711589813
1.5101900100708 -0.00900726485997438
-2.09030675888062 0.57515561580658
1.2662034034729 -0.788585066795349
-0.956403255462646 0.0412746034562588
0.558376252651215 -0.170081824064255
-2.88778424263 0.22070524096489
2.5347888469696 3.34118914604187
1.26380968093872 -1.24677526950836
0.0758960694074631 0.932676792144775
-1.04893612861633 1.36406791210175
0.833452522754669 -0.59266859292984
-1.18100941181183 0.066478043794632
-2.07764935493469 0.787413537502289
-3.18903732299805 0.204043015837669
0.493782937526703 0.0088996235281229
1.65716278553009 0.102308019995689
1.83047199249268 3.98301577568054
-1.13065981864929 0.613607347011566
0.967332482337952 -0.828654229640961
-0.141573816537857 -1.62537562847137
1.64312827587128 -1.07237350940704
-3.11528015136719 -0.0894413441419601
0.391000360250473 0.986849427223206
1.27047061920166 2.11330795288086
-2.03352546691895 -0.468087047338486
-0.712964415550232 0.84480082988739
0.633591413497925 -0.410030275583267
1.71665775775909 -1.33619046211243
-2.0945897102356 0.462226390838623
-1.38153028488159 0.250589430332184
0.877230048179626 -0.730282425880432
0.0860142856836319 -0.472309172153473
-2.20925378799438 -0.959935784339905
1.57520890235901 -1.96470165252686
-1.56707727909088 -0.137491226196289
-1.11023819446564 0.324294120073318
-0.286376267671585 -1.01434063911438
-1.57060623168945 -0.339331567287445
1.5159866809845 -0.890271008014679
1.49171257019043 2.06273221969604
-2.23050928115845 -0.652032613754272
-0.143110126256943 0.546428978443146
2.38694882392883 2.77451014518738
0.951828062534332 0.513774156570435
1.85073173046112 -0.407544016838074
-2.74324607849121 0.0026175593957305
1.10086345672607 -1.11747419834137
1.62014031410217 -2.57960724830627
-2.47778677940369 -0.173007801175117
-2.04901242256165 0.307477623224258
-2.40017747879028 -1.13357532024384
2.11560153961182 -3.29308724403381
-0.989751696586609 0.775291204452515
-1.10356378555298 -0.874340534210205
-0.850356221199036 -1.41372132301331
-0.961095809936523 0.797103047370911
-0.00725484732538462 0.490081161260605
1.1638650894165 1.22487509250641
-1.60674929618835 0.459730625152588
-1.54821944236755 0.444861054420471
1.75692367553711 0.731384038925171
0.763405203819275 -2.23406958580017
-1.53814661502838 0.0355849750339985
-0.267573565244675 0.818154156208038
-1.66680192947388 0.530674695968628
-2.06472277641296 -0.393587380647659
-2.96287608146667 0.288661897182465
2.62283253669739 4.27540159225464
0.651795029640198 -0.852588951587677
0.538017094135284 -0.727426111698151
-0.249685525894165 -0.382567822933197
0.0828188583254814 -0.40328311920166
1.15733706951141 -1.09095573425293
1.35217642784119 -2.20295333862305
-3.98467826843262 0.0574625842273235
-0.93819272518158 -0.00326948054134846
2.54118347167969 2.19162940979004
-0.112826846539974 -0.11545617133379
1.84814167022705 -0.115479350090027
2.01787662506104 3.38502931594849
1.45427572727203 -4.58457803726196
1.86445808410645 2.99580669403076
0.100014828145504 -1.59164273738861
-1.84728705883026 0.197006553411484
1.3055567741394 -1.14161622524261
1.69920670986176 0.330600202083588
-2.64990592002869 0.226432576775551
-1.35533487796783 0.167914465069771
-0.827963948249817 0.42703115940094
1.00198090076447 0.405512303113937
1.28618741035461 -0.673677384853363
-0.702511131763458 -0.682405352592468
-0.202635020017624 0.138769447803497
2.05894804000854 -2.07332491874695
0.113354898989201 0.0680854395031929
0.376608341932297 -1.01056754589081
0.704810619354248 -1.21420526504517
1.107266664505 -0.0547967776656151
-3.62764739990234 0.00125554215628654
1.43028771877289 0.922592222690582
-0.0274591967463493 0.896889448165894
-1.6169114112854 0.283134400844574
-0.644581496715546 -0.171367079019547
-2.69859290122986 -0.113327212631702
-1.17203497886658 -0.385682612657547
-0.373582035303116 -0.232620060443878
-0.686964511871338 0.736684620380402
2.41092300415039 -0.655050694942474
-0.341345757246017 -0.373006343841553
-1.3632425069809 0.16768091917038
1.20555543899536 2.77677178382874
-1.40797579288483 -0.123555794358253
-2.14960789680481 -0.00864672474563122
-1.22026479244232 0.517244040966034
-1.61519348621368 -0.638560354709625
0.0114309880882502 -0.76580798625946
-0.435223072767258 -0.315293192863464
-2.27937602996826 0.57208639383316
-0.97539210319519 0.717092573642731
-0.662483394145966 0.653012096881866
0.243346855044365 0.423276960849762
-3.2849109172821 0.16691766679287
1.1594979763031 -2.32928490638733
-2.52271032333374 0.246143206954002
-1.84867358207703 -0.156482502818108
0.783359289169312 -0.833208978176117
-1.79768538475037 0.452161520719528
-1.09211397171021 0.61297482252121
0.504900693893433 2.03868818283081
-1.16614103317261 -0.252573579549789
-2.10097455978394 -0.287094473838806
-0.249411001801491 -0.267438113689423
-0.458780288696289 -0.0784573256969452
-0.836892366409302 -0.0985681042075157
0.867588877677917 -1.55786406993866
1.30301189422607 -2.01418280601501
-0.830636382102966 -0.162331312894821
1.16013514995575 -4.66386461257935
-3.10694050788879 -0.1635622382164
-0.270782142877579 -0.658571362495422
-0.170982018113136 0.502663910388947
-0.606055498123169 0.839271664619446
-0.0091306921094656 -0.518302381038666
0.996713578701019 1.0675767660141
-1.81681060791016 -0.371015191078186
1.92777001857758 1.10798645019531
0.617640137672424 -0.233138784766197
-0.871054887771606 -0.697515726089478
1.03424775600433 1.27715361118317
-1.14785528182983 -0.47679078578949
1.27110719680786 0.918153941631317
-1.93492197990417 -0.019946625456214
2.3241491317749 0.128098145127296
-0.698940694332123 -0.58306086063385
-0.591481566429138 -0.8787602186203
-0.616435348987579 -0.262232035398483
-0.406636834144592 -0.274686455726624
-1.66608655452728 -0.152571141719818
-1.32976865768433 -0.330397367477417
-3.82242870330811 -0.0858625695109367
-1.77010440826416 0.365788817405701
0.265697479248047 -1.016446352005
0.879268765449524 1.13176476955414
-1.33804225921631 0.557589769363403
0.0374090038239956 -1.85209679603577
-0.632274568080902 0.515652596950531
-0.79820591211319 -0.741419434547424
1.28439450263977 3.21371412277222
-0.611638188362122 -0.624990880489349
-0.0525035485625267 1.58685326576233
-0.276547312736511 1.15417790412903
-0.495357811450958 -1.04430115222931
-3.23061347007751 0.0315337032079697
-0.129900977015495 -0.669504165649414
-2.42399311065674 0.472247153520584
-1.87699723243713 0.465322196483612
-1.54187762737274 -0.425610065460205
-1.58587491512299 0.288008362054825
1.01644670963287 -0.141971558332443
1.27664685249329 0.366577327251434
1.50898039340973 -1.54874062538147
0.346280694007874 -0.512885272502899
0.0946420431137085 2.30932450294495
1.6443065404892 1.20360052585602
-0.308630764484406 -0.603989720344543
1.94329583644867 0.423610359430313
-0.624355971813202 -0.702191889286041
-1.13988411426544 -1.22917103767395
0.295829623937607 1.62548613548279
-1.75996017456055 -0.623549997806549
-1.39507973194122 0.445709049701691
-0.672493398189545 -0.0594805106520653
-2.40015053749084 -0.267874002456665
0.3154656291008 -1.70660996437073
-0.809077322483063 -0.31641897559166
-0.902901411056519 -0.435903489589691
0.684183180332184 1.0283637046814
1.14526116847992 -1.53718483448029
0.304184347391129 -2.4551842212677
-2.16534280776978 0.248260334134102
1.58924472332001 -0.942744851112366
1.05069446563721 4.12542867660522
1.69971895217896 -0.012173518538475
1.28231656551361 -0.993884325027466
-2.19311857223511 -0.534189462661743
0.151335075497627 1.43762254714966
3.18393087387085 -0.409015595912933
-1.95553362369537 0.573859572410583
0.346088200807571 0.776023626327515
0.745231509208679 0.854136168956757
1.38348495960236 1.33306956291199
-0.441041320562363 -0.728088438510895
-2.55171418190002 -0.19256916642189
-2.3065037727356 0.0501048043370247
-1.15588748455048 0.405048847198486
-2.90708112716675 -0.299698084592819
1.0109783411026 4.86870574951172
-0.259963005781174 -1.01377403736115
-3.0317440032959 0.308843612670898
0.895214200019836 0.329638838768005
-0.0234517436474562 -0.772306382656097
0.502502918243408 0.992344379425049
0.389151066541672 -1.79580450057983
1.40408325195312 -3.22733521461487
-2.95524621009827 -0.118906177580357
-0.101634681224823 1.85346019268036
-0.369143724441528 0.792480051517487
0.146703511476517 -0.548306524753571
-2.01158857345581 -0.465223997831345
-1.74135231971741 0.874913573265076
1.38409531116486 -1.89586091041565
0.399465471506119 -0.28882560133934
-1.90285158157349 -0.139032453298569
2.2685272693634 -4.19602537155151
-0.701636731624603 0.770285546779633
-0.425576359033585 -1.41658902168274
1.09664309024811 0.877072334289551
-0.259721159934998 -0.0457106344401836
0.697096765041351 -1.00142800807953
1.109659075737 -0.169125616550446
-1.27846813201904 0.0458888150751591
1.06823515892029 0.326410055160522
1.63431036472321 0.156439244747162
-2.30640363693237 0.333317190408707
-4.24016284942627 -0.143554747104645
0.1539007127285 0.8051877617836
0.223453134298325 -1.67471981048584
-1.54058110713959 0.0753195956349373
-3.25995516777039 0.121617399156094
-0.902971148490906 -0.768206119537354
0.62053120136261 3.15528964996338
-2.33493256568909 -0.164561092853546
-0.0385298877954483 0.126262471079826
-0.306325376033783 0.978718280792236
-0.536562323570251 0.263992697000504
1.86550915241241 -0.48840594291687
-1.41830277442932 -0.100305631756783
-0.823662757873535 -1.30721282958984
-0.300119310617447 2.00481963157654
-0.475634723901749 -1.19084930419922
1.06392991542816 -2.85028624534607
-0.616848707199097 0.391552954912186
0.840309262275696 0.563365519046783
0.245223358273506 1.78700184822083
-3.49836206436157 0.0267716776579618
-0.744298219680786 0.606577336788177
-3.26514720916748 -0.17761692404747
-0.181165099143982 0.772041916847229
-3.93180203437805 -0.127883747220039
-1.26023542881012 0.545743227005005
-1.17373144626617 -0.263195961713791
-0.414004683494568 0.733106672763824
1.29149079322815 2.80256056785583
-1.02529239654541 -0.12060422450304
-0.0841854736208916 1.39727210998535
-1.97080826759338 -0.138136655092239
0.291413813829422 0.94140088558197
-0.0501994155347347 -0.611194789409637
-3.20114302635193 -0.385465949773788
-0.577780604362488 0.394348591566086
-1.63863158226013 -0.120730035007
-1.10074079036713 -0.767891764640808
1.75057351589203 2.27100992202759
2.74797487258911 -5.42039394378662
-1.23968470096588 0.767474591732025
-0.840143799781799 -0.792236089706421
-1.050253033638 -0.211267456412315
-2.79515528678894 -0.00760283507406712
-0.123375937342644 1.09487342834473
1.12170553207397 -0.931044816970825
1.21736931800842 1.01133191585541
1.62588250637054 -1.60324025154114
-1.79041492938995 0.0188604462891817
-0.921765148639679 0.0905827283859253
1.07313466072083 0.230429500341415
0.88852733373642 2.15220236778259
0.958698034286499 1.3637580871582
-0.877077758312225 -0.159610033035278
-2.26792311668396 0.225206136703491
-2.38751935958862 -0.309065014123917
-0.678142845630646 -0.654096245765686
2.04360389709473 2.54447460174561
-1.17551076412201 0.455030500888824
0.459735661745071 -1.1556042432785
0.0717680528759956 -0.921042799949646
1.6252589225769 -0.7092205286026
0.86447662115097 1.19869744777679
-0.443122297525406 -0.0773014575242996
0.425173193216324 -0.99845290184021
0.128071591258049 -0.593157351016998
1.40942859649658 0.393355578184128
-1.28000020980835 0.324707359075546
-1.02849340438843 -1.04026973247528
-0.77392452955246 0.311462163925171
-1.62059819698334 1.86144030094147
-1.47749578952789 -0.49395215511322
0.974689841270447 0.116102069616318
0.26862832903862 -1.54133260250092
2.28454113006592 -1.18667256832123
-0.463199883699417 0.29956528544426
2.0541844367981 3.84589600563049
-0.983305037021637 -0.95714396238327
-1.92894518375397 0.195326000452042
-1.90586495399475 -0.256644695997238
-2.2933177947998 -0.583959698677063
-0.89272928237915 1.23658585548401
-1.27236974239349 -0.0776144787669182
1.58763706684113 -0.79707008600235
-0.192684754729271 -0.66046154499054
-2.0325026512146 -0.338083773851395
-0.466867387294769 -0.960616111755371
-1.55823040008545 0.437396496534348
-1.21494483947754 -0.56368088722229
-0.24421738088131 0.58491176366806
2.44630599021912 3.61048340797424
1.00836050510406 3.21933460235596
0.312118500471115 1.00177431106567
1.76070964336395 -1.49556767940521
2.24079966545105 -0.591904997825623
0.806923389434814 -4.08121681213379
-0.393996804952621 0.0352250635623932
-2.20549941062927 -0.00660669477656484
-1.74276471138 -0.165262252092361
-0.175598099827766 -0.668766498565674
1.09213542938232 0.659774124622345
1.20969796180725 -1.55020940303802
0.629078149795532 1.30189657211304
-0.466279596090317 -0.0610841512680054
-3.56605553627014 -0.0174131616950035
0.326251089572906 2.43598508834839
-0.87688934803009 0.199384734034538
-2.52533984184265 -0.0200922954827547
1.36342811584473 1.37089240550995
0.887801289558411 -0.496730178594589
1.35726451873779 -0.577898442745209
-1.30707573890686 -0.204716801643372
1.09812414646149 1.2950975894928
2.35027098655701 0.873418271541595
-0.46175879240036 -0.3115573823452
1.07331514358521 2.90289378166199
-3.83598780632019 0.0774388834834099
-1.23366379737854 -0.297667741775513
-0.971965968608856 0.979781806468964
-0.191023170948029 0.0697818472981453
0.272800713777542 1.30839717388153
-1.13983988761902 0.346913039684296
1.206387758255 -0.62775456905365
-0.0961204990744591 -0.905883550643921
1.51375079154968 -1.94609653949738
-1.91602730751038 0.148117825388908
1.67163527011871 1.71948432922363
-0.755081117153168 0.36649876832962
-0.443037390708923 1.1092004776001
-2.2475471496582 -0.158914893865585
-1.20572006702423 0.0355006381869316
-1.00185310840607 -1.51827096939087
1.49476480484009 -0.348417729139328
-0.144616171717644 -0.00528193265199661
0.1860681027174 -0.273510038852692
0.212244883179665 0.174622103571892
-2.07575559616089 -0.75827294588089
1.60617184638977 1.26968419551849
1.76436579227448 1.42712771892548
1.61205077171326 -1.69668579101562
1.28142893314362 -3.93591976165771
-1.70890378952026 0.277583688497543
-3.04964566230774 -0.178133085370064
0.995556473731995 0.273952454328537
-0.32608437538147 0.03095967695117
0.0878220945596695 0.0295732915401459
-3.35599303245544 0.132637858390808
-0.812331557273865 0.376530677080154
2.12930417060852 6.60662174224854
1.14473819732666 1.52928960323334
0.842131912708282 0.55585640668869
2.05605912208557 -1.36493468284607
-1.18100607395172 -1.02142417430878
0.231837883591652 2.1993203163147
3.08966088294983 3.03783893585205
-2.06987166404724 -0.254132777452469
1.79311954975128 -5.06175994873047
0.958962798118591 1.44813132286072
-3.75134372711182 0.0909194722771645
-1.37996971607208 0.451598167419434
-6.33894491195679 0.0115804057568312
0.266758471727371 0.156529083848
0.981405854225159 1.06475961208344
-2.0735490322113 0.115006290376186
-1.19930291175842 -1.12300753593445
-1.08704602718353 0.418919593095779
-3.56713438034058 -0.0477338321506977
-1.1975109577179 -0.079935185611248
0.856070935726166 1.01216650009155
0.398314356803894 1.10028219223022
0.475506365299225 -0.761412560939789
-0.44190976023674 0.211359739303589
-3.57118344306946 -0.192349970340729
0.579850792884827 1.66026329994202
-1.36563920974731 0.435484290122986
-0.133954420685768 0.230525255203247
-2.7618134021759 -0.199332907795906
0.056539636105299 -1.70988595485687
-1.92694330215454 0.0133646996691823
0.778965294361115 -2.50080919265747
-1.75360918045044 0.447698205709457
-1.12971997261047 -0.360252320766449
-0.896030128002167 0.166638270020485
-0.521145343780518 -1.98446249961853
0.234788820147514 -1.42250537872314
-0.513116300106049 -0.242443710565567
-4.15914344787598 -0.000939064892008901
-0.842995762825012 0.252411425113678
3.91976237297058 3.56691312789917
-1.85194432735443 0.556557357311249
2.32931566238403 2.662358045578
-1.25039124488831 0.303995907306671
-1.09662067890167 0.910599887371063
-2.42761921882629 -0.294551849365234
-2.52071213722229 0.276297062635422
0.623974502086639 1.55475151538849
-1.79645109176636 -0.556128799915314
0.455554485321045 1.1290020942688
-0.561995625495911 0.951219379901886
0.51961475610733 -0.198864355683327
1.5950939655304 -1.72933280467987
-0.692334949970245 0.149705439805984
-1.35905265808105 -0.0503926873207092
0.0790968909859657 0.371683597564697
0.243867799639702 -0.31184396147728
-2.57148814201355 0.629628956317902
0.420105844736099 0.0161049533635378
1.10067903995514 2.06511878967285
-0.670543372631073 0.358290404081345
-0.00183024676516652 -0.406516641378403
1.46947753429413 -3.39799642562866
1.02054309844971 1.17561793327332
-0.2542864382267 0.0729552134871483
1.11184930801392 0.0569766461849213
-0.248258203268051 -1.0047060251236
0.308682501316071 0.678565561771393
-1.30180025100708 -0.103923492133617
-2.19358420372009 0.233621448278427
0.215505450963974 -0.521282494068146
-1.14727282524109 0.0410933941602707
2.22171115875244 -0.717395544052124
-0.724153816699982 1.73811531066895
2.17543745040894 -0.250419914722443
-3.65478205680847 -0.139680609107018
-0.609323143959045 0.473572820425034
-2.08211970329285 -0.166028961539268
0.71495658159256 -1.64958202838898
-1.71797370910645 -0.186228066682816
-0.176418334245682 -0.80097758769989
2.35222148895264 1.13022494316101
-2.23534941673279 -0.141479313373566
0.597505629062653 -1.39842796325684
1.59601354598999 1.23773062229156
-2.08657956123352 0.0941574349999428
1.15148794651031 -0.993390142917633
-1.65153288841248 -0.351430654525757
0.487807869911194 1.2811017036438
-1.44846630096436 -0.876435279846191
0.561648726463318 0.0629388466477394
1.22210454940796 -2.00633764266968
-0.0966615453362465 -0.513931214809418
-1.05604672431946 -1.32464063167572
-0.772771000862122 -0.374188244342804
-0.970228493213654 -0.497632265090942
-0.978344082832336 0.691480278968811
-1.94753873348236 -0.164756819605827
0.910293400287628 -0.481577455997467
-1.89000236988068 -0.104380115866661
-1.98265433311462 -0.0219070166349411
-0.169602528214455 0.861490547657013
-3.19233679771423 0.156660065054893
1.06341242790222 -2.57477474212646
-0.866057217121124 -0.179784804582596
1.48046004772186 -3.82259821891785
0.200668811798096 0.353643625974655
-1.14499819278717 -0.361356168985367
-2.25275111198425 -0.117577888071537
-0.340257614850998 -0.674819529056549
-1.64791166782379 0.119147181510925
0.870265781879425 0.279930412769318
-2.17309808731079 0.356825292110443
-2.69203543663025 -0.165511414408684
-2.33626651763916 0.335864245891571
2.30645823478699 2.5710072517395
1.48968386650085 -1.10455763339996
-1.73772752285004 -0.0486271679401398
3.37900590896606 -0.528839409351349
-0.412238717079163 0.0689874216914177
1.09920227527618 1.67005455493927
-2.25460934638977 -0.26678204536438
1.21694993972778 -1.57933688163757
1.50684118270874 0.302781611680984
1.54704129695892 -0.518617987632751
2.01551032066345 -1.06787478923798
};


==> figures/visualizations/funnel/fab_samples.tex <==
\addplot [semithick, fab, opacity=0.7, mark=x, mark size=3, mark options={solid}, only marks]
table {%
5.49282360076904 -0.395412892103195
7.01633024215698 -2.82544541358948
-1.74362134933472 -0.0398303270339966
7.23224258422852 58.8375625610352
0.53056001663208 -0.338882595300674
-0.925468862056732 -1.2955048084259
-3.97216320037842 0.0797662436962128
6.74238967895508 27.3786487579346
-2.41576743125916 0.127588301897049
0.709000825881958 0.504565000534058
0.768537223339081 1.39127421379089
-2.82067394256592 -0.519128203392029
6.34722375869751 -42.7049598693848
1.68880617618561 1.67033076286316
-0.0338089466094971 -1.319016456604
4.61792278289795 4.9367094039917
-2.76512908935547 -0.123842895030975
-4.72620582580566 0.0445170551538467
3.74672603607178 -3.37978935241699
2.51670455932617 -5.70106649398804
1.3798291683197 -1.02888870239258
-2.95852518081665 -0.0571879483759403
3.03285670280457 4.42056894302368
-3.82602977752686 0.0621888525784016
1.98451614379883 0.539434671401978
5.47300148010254 -18.8008823394775
-0.11537429690361 0.394042819738388
0.970568716526031 -1.82267761230469
-0.777083158493042 0.000292956829071045
-0.764558792114258 -0.117209821939468
-3.44750642776489 -0.21343606710434
-3.21667408943176 -0.151229411363602
1.73388707637787 3.63706231117249
0.763565123081207 0.670469284057617
-2.7754180431366 -0.180852934718132
4.07874393463135 5.44452428817749
0.412190407514572 0.351492881774902
-1.4974604845047 -0.228873759508133
2.25552368164062 -2.55449628829956
2.66358399391174 -5.39511728286743
-0.0293811708688736 1.28429889678955
3.43318653106689 0.662524938583374
-0.366617202758789 -1.10464715957642
-5.35221862792969 0.0163467265665531
-2.52950882911682 0.33804726600647
-6.86901950836182 -0.0553113706409931
-4.56521511077881 0.013713926076889
0.845640063285828 1.62719905376434
0.100996419787407 0.335462898015976
2.29015922546387 2.43591213226318
1.26317191123962 -2.94426465034485
-1.7606475353241 0.15993458032608
3.20804595947266 4.07511281967163
0.349024295806885 2.29633522033691
-0.234533682465553 0.533800005912781
1.98535013198853 -2.6166775226593
-2.1933274269104 -0.329315006732941
1.11946177482605 0.459435641765594
-1.20776462554932 0.859530925750732
1.19778788089752 -1.74122738838196
-1.26209378242493 1.36197113990784
5.98954677581787 -1.15760934352875
-4.65317821502686 0.0936854183673859
3.5994553565979 -3.84842920303345
-1.74742889404297 -0.071595698595047
3.31604218482971 -6.30576801300049
1.07516694068909 -0.0548727288842201
2.63220453262329 3.77404260635376
1.44989669322968 1.57441139221191
-0.0377079844474792 1.37504196166992
-1.70335221290588 0.0984730273485184
-0.897975087165833 -0.00725382566452026
-5.44436931610107 0.00135010667145252
1.91199946403503 1.90242505073547
-0.00312658399343491 0.254663020372391
-0.732809901237488 -0.204617142677307
-0.0105128288269043 1.62755358219147
-2.92677307128906 -0.122977696359158
-1.8094654083252 -0.946727573871613
6.35730600357056 -10.1979341506958
-1.7916511297226 -0.302486300468445
-4.47594118118286 -0.0369057841598988
2.77948522567749 -4.91527652740479
1.53684687614441 0.785865902900696
-2.53281760215759 -0.056806419044733
-3.58080530166626 0.171137005090714
-4.92363929748535 -0.053742665797472
2.70314574241638 -1.19740653038025
1.56565737724304 -2.07438778877258
6.65635204315186 42.280704498291
2.26287460327148 -4.38765382766724
-1.17673790454865 -0.0871988832950592
-0.080889418721199 0.715737164020538
0.147034347057343 0.466209679841995
-1.49424600601196 -0.0353525094687939
-1.97042608261108 -0.33358246088028
1.20588195323944 1.8401997089386
-1.7936452627182 -0.264479219913483
-1.17097949981689 -0.127757132053375
1.56964468955994 1.22801387310028
0.934260487556458 -0.730682373046875
3.94738435745239 0.345302134752274
0.848731637001038 1.68984341621399
0.750671327114105 1.00306081771851
1.49437010288239 -1.72545945644379
-2.87396907806396 0.0676418095827103
3.21783351898193 -7.50211238861084
-3.58253717422485 -0.00042431615293026
-2.65670323371887 -0.42503297328949
-0.993885397911072 0.225618258118629
1.4723128080368 1.06814169883728
1.99864721298218 2.9930739402771
-4.66652870178223 0.00409219413995743
-3.69772958755493 0.00672551058232784
3.75457715988159 -3.1979124546051
-1.0090526342392 0.163124889135361
3.06268858909607 -6.09437036514282
3.69169092178345 -1.14236354827881
2.8347806930542 -3.03955292701721
-1.19014716148376 -0.0696157515048981
-3.56315183639526 -0.270183086395264
-0.786484658718109 -0.611868500709534
3.00899982452393 3.51319074630737
-3.77630162239075 0.170634180307388
0.916317701339722 2.43691730499268
2.73605370521545 -2.00870394706726
-0.00290843844413757 2.60819268226624
2.3512077331543 5.52861881256104
-1.54049730300903 0.233651280403137
2.06937742233276 -4.35683298110962
-0.217559725046158 1.23681211471558
-0.641783654689789 0.367324233055115
-3.69854927062988 -0.00731971301138401
5.31542015075684 -24.7224540710449
-1.28283834457397 -0.130908861756325
0.206309974193573 0.690478324890137
0.054151639342308 2.82290816307068
-0.87371551990509 0.20366433262825
1.55599224567413 -0.86952805519104
-7.8419075012207 0.0017143078148365
1.5674821138382 2.41515350341797
-3.10622644424438 -0.291747480630875
-1.99146628379822 0.61330258846283
6.15433311462402 12.9852352142334
-1.68830573558807 -0.984883427619934
2.32424306869507 -6.26720523834229
-0.0908254235982895 0.600194692611694
4.67675256729126 -12.292308807373
3.34499526023865 -0.00440901517868042
1.98425269126892 1.34356904029846
-6.83063364028931 -0.0478574633598328
2.6540379524231 3.04949712753296
-1.90023994445801 -0.287690997123718
1.17980682849884 1.03407835960388
-2.33924865722656 0.294080883264542
2.18008089065552 -1.01132869720459
-2.75348281860352 -0.244929626584053
-1.79885613918304 0.856202065944672
2.80497646331787 -0.0990689098834991
4.00767469406128 13.8690013885498
4.62765884399414 -0.748231172561646
5.01214790344238 6.36319303512573
5.43554067611694 14.996994972229
-3.98294901847839 0.243355453014374
-0.0566213726997375 -1.54382407665253
-1.50817036628723 -0.0462826490402222
-1.70229256153107 0.043104462325573
0.640404880046844 0.865815818309784
0.761145830154419 1.3826949596405
3.72661709785461 4.92997932434082
-1.49608170986176 -0.175146102905273
-0.19098736345768 0.212025493383408
4.38488864898682 7.2085976600647
1.63691306114197 1.30815625190735
-3.03220272064209 0.109133303165436
5.86764478683472 6.02486896514893
0.707623898983002 -0.331479400396347
-3.07659125328064 0.0871414840221405
4.70666170120239 -38.0302848815918
-1.03492736816406 -0.00676801800727844
4.84086513519287 -0.448215067386627
-0.0963961482048035 -0.714999735355377
-3.19756007194519 -0.444895803928375
4.09067726135254 -0.81507134437561
-2.7471764087677 -0.08713598549366
-0.887716948986053 -0.385984808206558
-2.11373353004456 0.777428567409515
-2.50170850753784 -0.423005998134613
6.25508499145508 -17.9091987609863
-6.25203371047974 0.0296136140823364
3.60061645507812 7.79420375823975
-1.86211693286896 0.184005811810493
1.28618192672729 0.523634433746338
-1.28648328781128 -0.376259982585907
1.06480395793915 -0.469001948833466
2.04639959335327 0.483711272478104
-2.45126605033875 0.0677811056375504
0.857307195663452 -0.125090077519417
-0.054444432258606 -0.334015429019928
0.400758862495422 0.678106427192688
-0.104908652603626 -0.916035652160645
2.09874248504639 5.28269624710083
4.91826295852661 -5.10220098495483
1.59951460361481 0.648710250854492
4.55291509628296 -3.38468742370605
6.38765335083008 -6.9709300994873
0.256480544805527 -2.04010558128357
4.24089241027832 -7.76855516433716
-6.96037626266479 0.0140974223613739
1.27873349189758 0.524015784263611
-0.485653400421143 0.253691822290421
-0.949008226394653 0.698893308639526
7.84411096572876 74.7695770263672
1.74880015850067 0.736274123191833
-2.98138880729675 0.00383708067238331
3.34045791625977 -7.36100482940674
1.3917121887207 -0.230420500040054
-4.50068807601929 -0.0671425461769104
4.7693452835083 0.401923894882202
2.40646839141846 -2.59537386894226
1.24661421775818 1.35034680366516
-1.3997118473053 0.144249439239502
1.01410174369812 0.806165814399719
0.910176455974579 5.02860736846924
-0.935071051120758 -0.132365167140961
0.361854195594788 -2.35860395431519
-1.80239737033844 0.472629606723785
1.52039098739624 -3.75874972343445
-1.43074369430542 -0.468495666980743
-4.69357013702393 0.0779172629117966
-1.5307868719101 -0.190641403198242
-0.649400949478149 0.059113472700119
0.773373484611511 0.137838959693909
4.19603872299194 4.12914800643921
-1.60922014713287 0.556242406368256
-5.49815368652344 -0.0874867886304855
-0.89275074005127 0.482208609580994
1.7267279624939 -2.84192967414856
3.64596199989319 -8.05777549743652
-7.50907182693481 0.0501283407211304
4.03875494003296 -11.3679857254028
-5.56161022186279 -0.043312169611454
2.68881988525391 -1.11193954944611
4.88188409805298 -3.99567294120789
3.81233286857605 -6.38429164886475
-1.30953931808472 0.31658136844635
3.335369348526 -7.95229053497314
0.778460144996643 -3.0244140625
-1.33076190948486 -0.345096617937088
-5.46308279037476 -0.0735915675759315
1.12268459796906 0.652343034744263
1.15713620185852 1.37532079219818
5.1795859336853 20.9839630126953
1.75526809692383 1.47484314441681
0.822675406932831 -0.257048517465591
-1.50910210609436 -0.112804114818573
0.0394324362277985 -0.703225016593933
4.30016136169434 -16.9144401550293
1.57613146305084 -0.680037379264832
0.680038452148438 -0.736656069755554
-0.459227591753006 -0.196756333112717
3.29677176475525 5.87937784194946
-3.85255742073059 -0.207115471363068
-2.42651104927063 -0.243400245904922
-2.19572353363037 -0.346329092979431
2.1103298664093 -5.51876735687256
-2.60008406639099 -0.135089322924614
1.91748356819153 0.0526915788650513
-1.79676413536072 -0.608148694038391
0.930074453353882 0.113477349281311
0.655337631702423 1.35905456542969
2.85228633880615 -4.143479347229
5.51288366317749 5.58826398849487
2.8886456489563 -2.03586888313293
-0.884076178073883 -1.21080756187439
-5.05106592178345 -0.0717673748731613
3.10982465744019 5.0426869392395
6.24998807907104 -28.1664600372314
-4.07977199554443 0.137447327375412
-8.60527515411377 0.0543511062860489
1.20546758174896 1.5822981595993
3.13546442985535 1.0001460313797
-8.29426574707031 -0.00765810254961252
0.22837795317173 0.425031453371048
6.18443059921265 20.0449275970459
2.06173992156982 -0.32913339138031
-1.36442065238953 -0.550074994564056
-1.38622629642487 -0.881682574748993
-2.51570582389832 -0.171470940113068
3.1636323928833 4.35786056518555
4.0726957321167 12.490364074707
2.79404616355896 -2.14610910415649
1.15373241901398 0.340831935405731
-0.929825246334076 0.535167217254639
-0.625851929187775 1.05561208724976
1.26819467544556 1.42218673229218
2.1148841381073 4.16812229156494
4.00349235534668 3.23296689987183
-5.05019664764404 -0.05378657579422
-0.670976400375366 0.662719130516052
-5.85211515426636 0.0492776855826378
4.1247878074646 -3.61326766014099
3.01667666435242 -4.14245080947876
0.125454843044281 0.478419184684753
0.98038375377655 -0.416980862617493
-1.77465045452118 0.302129209041595
-3.42858147621155 0.0814290046691895
0.558199048042297 0.438070952892303
-1.7631801366806 1.05947422981262
5.32578611373901 -3.49794936180115
1.89499592781067 -0.242921531200409
7.59466123580933 92.7291946411133
1.11069774627686 -1.92380213737488
1.72555065155029 -4.25481939315796
1.88089871406555 2.61583852767944
-0.821102619171143 -0.272652208805084
-2.07266235351562 0.508217751979828
0.144469410181046 1.03878104686737
2.58133983612061 -7.32545614242554
-2.51263117790222 0.549003720283508
-1.80251741409302 -0.453851819038391
0.688349306583405 -0.00469255447387695
-5.76154899597168 0.0629287213087082
4.05876493453979 -13.1129884719849
-2.33452415466309 -0.123176217079163
-0.706125199794769 0.306462228298187
1.68799817562103 -1.72603869438171
-0.387369155883789 -0.156453967094421
-3.19762849807739 0.0256378445774317
-2.86958861351013 -0.121070578694344
-3.25876188278198 -0.0353536903858185
0.562810838222504 1.72108912467957
0.179863065481186 -0.260593593120575
-4.01562595367432 -0.0738083571195602
-4.68107652664185 -0.0609114915132523
-2.13488793373108 0.423856496810913
-5.31142711639404 -0.0141084585338831
4.15079116821289 2.95031666755676
3.40028858184814 7.80841541290283
-1.02141952514648 -0.839212775230408
3.63350009918213 2.03521394729614
2.77368903160095 -2.94724297523499
-4.15605545043945 -0.124613292515278
-3.25606822967529 -0.0239776205271482
-2.50404453277588 0.315589219331741
-5.7191686630249 -0.0150206116959453
-0.263731360435486 0.0803208947181702
1.00202608108521 1.96116971969604
5.46075057983398 25.4893608093262
2.09168934822083 -0.265496671199799
-0.0416342616081238 1.29752290248871
0.343299984931946 0.433412939310074
-0.672491550445557 0.621547937393188
-0.0585330724716187 -0.655032455921173
-1.56195604801178 -0.0561361536383629
-5.48314905166626 -0.0802596211433411
2.69144439697266 -0.627749443054199
-2.24181985855103 -0.261132478713989
-0.523441314697266 -0.0657178312540054
0.478458970785141 -1.34475123882294
-0.65854549407959 -0.760510683059692
0.306224375963211 0.549724102020264
4.03017282485962 -3.8515613079071
-1.50720226764679 -0.618492662906647
-1.87126898765564 -0.375903725624084
-0.752188920974731 -0.120048254728317
-3.66228151321411 -0.214428350329399
6.42065620422363 -12.683892250061
-1.3683226108551 -0.489307403564453
-0.970357358455658 0.803202748298645
-2.28884553909302 0.094924233853817
1.78927958011627 3.01056838035583
-6.07996463775635 0.00118225254118443
-1.2962738275528 0.106939971446991
-1.17781472206116 1.2829737663269
-3.9687807559967 0.309500932693481
-3.22407293319702 -0.574158668518066
1.82954227924347 0.376165866851807
-0.986539661884308 -0.202152460813522
-0.877808928489685 0.193441808223724
-4.10550546646118 0.19859953224659
-0.708574771881104 0.248023867607117
-4.51755714416504 0.0184051692485809
-5.84692430496216 0.111510246992111
-7.85203075408936 0.00966297276318073
1.57484555244446 -0.739578068256378
-0.53822922706604 -0.318993866443634
0.837472081184387 0.0740202069282532
-1.23044514656067 -0.10091358423233
2.64692211151123 4.67941570281982
2.15163207054138 0.708701729774475
-4.36244869232178 0.0880722478032112
3.88093137741089 -2.06984710693359
1.26073598861694 2.10814523696899
-0.94583648443222 0.173644572496414
-1.56611931324005 -0.58736389875412
-2.10349750518799 -0.430525928735733
4.17597150802612 0.449171662330627
-1.08049094676971 1.38566434383392
-1.29323887825012 -0.184082001447678
4.67348623275757 -7.77282810211182
1.48982572555542 0.163262620568275
-4.66153907775879 0.0499960705637932
1.77082300186157 5.0356650352478
0.457509607076645 -0.526225030422211
-2.3220579624176 -0.452094554901123
5.3147144317627 10.0772285461426
1.29684746265411 2.13592123985291
-0.657716035842896 0.469535619020462
-2.58933115005493 0.0292837079614401
0.836704432964325 3.11037635803223
-0.755412101745605 0.00286123156547546
3.86700630187988 -11.6908292770386
-1.84293615818024 -0.146057978272438
7.02141904830933 0.993640005588531
1.26856601238251 2.58918952941895
0.59648209810257 0.360757440328598
0.477538853883743 1.18078422546387
-2.68459296226501 0.237163722515106
2.90347266197205 -3.99509620666504
-1.81887412071228 0.0977597087621689
2.70842814445496 -3.13624382019043
-3.36094188690186 -0.166627421975136
-2.58325362205505 0.149999260902405
4.19431114196777 4.59889459609985
-1.1435033082962 -0.268499255180359
2.84411478042603 2.27380132675171
-1.29953896999359 -0.0755719989538193
-0.664043724536896 0.0150131732225418
-0.379660308361053 -1.03596973419189
-0.597335696220398 0.395856827497482
-4.33660793304443 0.0816114768385887
-1.47492289543152 -0.851513266563416
1.21081304550171 -0.818834483623505
0.761010885238647 -0.956718742847443
-3.66691184043884 -0.0763068944215775
3.72911953926086 -6.7867603302002
1.22202813625336 -1.82423031330109
-3.88594794273376 -0.0442588850855827
4.10037040710449 -2.78706884384155
6.02069187164307 37.244010925293
0.17721688747406 1.88256537914276
1.10134625434875 -0.596489548683167
-0.646888673305511 -0.0116427093744278
5.81213855743408 -15.1529712677002
-1.16112959384918 -0.786396861076355
2.4534707069397 -3.79413199424744
2.57379269599915 -5.75329303741455
-4.06166982650757 0.0274697784334421
4.14507865905762 0.711806893348694
-1.41945540904999 -0.0454424619674683
0.115677177906036 0.183800876140594
-5.28995418548584 -0.0473638847470284
-1.18311154842377 -0.497616231441498
-1.27744626998901 -0.276281446218491
-0.499974995851517 0.757154941558838
0.155129909515381 -0.844957947731018
1.61934280395508 -1.31002688407898
-2.40502238273621 0.145779356360435
3.67920351028442 3.50223684310913
-3.55186820030212 0.271699756383896
-0.0534588992595673 -0.0563207566738129
-2.85398960113525 -0.00161796808242798
2.2401487827301 -0.152596801519394
-0.627119541168213 0.476156294345856
-0.646290421485901 0.652056455612183
3.39591383934021 -1.68947017192841
0.0102291703224182 1.38734567165375
-0.180568814277649 -1.91564297676086
4.37930727005005 -21.1595668792725
2.33844017982483 -4.70127725601196
2.55575084686279 -3.25601744651794
0.680244922637939 -1.21772372722626
-3.97447657585144 -0.235902190208435
1.1482264995575 1.38871622085571
4.45242261886597 2.0276050567627
0.864205598831177 0.555288076400757
1.49439930915833 -2.34989333152771
1.3203456401825 1.35490238666534
5.58388900756836 -11.8420381546021
2.57147860527039 0.102861806750298
1.22377860546112 2.31300401687622
-0.164111167192459 -0.904129326343536
1.46424150466919 -3.93511271476746
2.30158758163452 -4.39584159851074
2.30860686302185 -3.00113773345947
3.90964961051941 3.0777804851532
-4.78970003128052 -0.113779582083225
-5.23025321960449 -0.00760201085358858
-7.13273668289185 0.0299223959445953
-1.66929113864899 -0.159457087516785
0.247856289148331 0.364705175161362
-2.12817907333374 -0.216782808303833
-1.33523201942444 -0.207673817873001
-0.131369471549988 -1.15020525455475
-1.64784109592438 1.23914957046509
5.76474618911743 14.3996105194092
-1.32239842414856 -0.137227445840836
1.78655767440796 2.05436301231384
-0.847120881080627 1.13756895065308
-2.92203164100647 -0.181096196174622
-1.56997609138489 -0.995689153671265
-0.363325089216232 1.36172270774841
-1.87910652160645 -0.45324382185936
-1.94437623023987 0.082720622420311
2.5582971572876 0.438983082771301
-1.16857969760895 0.279610455036163
0.281499743461609 1.38209581375122
-0.56353759765625 0.338749825954437
0.887006402015686 -2.35660362243652
1.07171559333801 0.320378124713898
-3.67026019096375 -0.38623720407486
-6.02345323562622 -0.0620190352201462
-3.29982209205627 0.187774077057838
8.66569328308105 -148.393783569336
-2.17420649528503 -0.354079633951187
-1.3758008480072 0.310073971748352
-0.384238481521606 -0.563482761383057
1.50560235977173 -2.96092629432678
1.67102384567261 0.218172878026962
2.07851099967957 -0.497783929109573
4.38710880279541 -10.4536399841309
-0.728813767433167 0.146634131669998
-4.34147882461548 0.0764307230710983
-2.76193928718567 0.139665842056274
1.51370751857758 -1.60063314437866
-4.97136735916138 -0.0250943321734667
-1.9917573928833 -0.147473067045212
-3.90954685211182 -0.0560344681143761
-0.242348074913025 0.567391991615295
-3.79749631881714 0.0463004559278488
4.1068639755249 4.02788543701172
0.817180633544922 0.386499285697937
0.280945748090744 1.58136820793152
-2.68378257751465 0.57327139377594
-1.40308475494385 -0.10137015581131
-3.89120221138 -0.0974361822009087
7.07443571090698 -34.0834655761719
4.20760202407837 5.76001071929932
2.29003596305847 0.358840137720108
1.6451176404953 0.696184635162354
-4.71545696258545 0.102964237332344
-1.75465905666351 0.487765610218048
1.30458474159241 2.97428178787231
-1.6425404548645 -0.225385457277298
-3.72124910354614 -0.0714180916547775
6.1341028213501 32.0250434875488
1.51351177692413 1.18265628814697
1.20366168022156 0.171463191509247
0.344135046005249 -0.558263003826141
-4.73755073547363 0.104365631937981
3.1726987361908 -4.9302544593811
-3.41927790641785 -0.125728160142899
-1.61288511753082 -0.188634693622589
-2.46025657653809 0.255666792392731
-0.566102027893066 -0.82053017616272
1.33919680118561 -0.61418092250824
-1.12418830394745 -0.743866920471191
-1.65865385532379 0.548026621341705
-2.24591660499573 0.39638152718544
-0.272619903087616 0.662481844425201
1.53088748455048 2.84619069099426
-3.61527109146118 -0.0757884308695793
3.75450658798218 22.5409259796143
6.42221736907959 28.2677936553955
4.0109224319458 4.43858289718628
3.74194097518921 10.2013654708862
-1.8917248249054 0.0253447294235229
2.72957873344421 0.8813236951828
1.43468379974365 0.931700944900513
7.13652324676514 -18.6464443206787
1.66463470458984 -3.21821808815002
-1.3487503528595 -0.358387351036072
0.38965630531311 0.282946765422821
-5.03465223312378 0.123506635427475
-2.67319655418396 -0.449075162410736
0.129927650094032 1.59330558776855
-0.810245037078857 -0.372804194688797
-0.778263807296753 -1.10151839256287
-1.06027126312256 -0.388946354389191
1.60299205780029 -1.7441371679306
4.88460206985474 -13.1177930831909
-3.25058507919312 0.0912554264068604
1.20581984519958 1.34664344787598
0.0313291996717453 0.986190617084503
2.56588292121887 -5.78740072250366
-1.40390241146088 -0.18902163207531
-3.3000864982605 0.00317093171179295
1.7179924249649 -3.92424869537354
0.954042613506317 0.349482774734497
3.98339319229126 3.61378049850464
4.20620012283325 -1.71698141098022
6.0852255821228 28.6896572113037
-0.775270164012909 0.838911175727844
1.6552323102951 -1.58100116252899
-7.89333534240723 -0.0165453981608152
-1.954141497612 0.0831374526023865
1.91413950920105 0.177861422300339
1.07596528530121 -0.419169008731842
-2.06168508529663 -0.241377845406532
-0.826288044452667 -1.04608380794525
-2.1115345954895 0.286042779684067
3.91781330108643 11.9466190338135
1.02333796024323 -1.93472790718079
2.89249682426453 -3.82993912696838
1.05459690093994 0.0166023820638657
-5.80468225479126 -0.0102275600656867
1.0413920879364 3.40833854675293
1.21416091918945 -0.567890763282776
0.54252690076828 0.250822335481644
0.317222595214844 1.47408974170685
2.1203248500824 2.48437881469727
0.0732288509607315 -0.563228130340576
-2.85600423812866 -0.319511443376541
3.7142927646637 4.79117965698242
-0.285936653614044 0.736298382282257
1.11539721488953 1.51502585411072
-0.776523649692535 -0.556774318218231
-1.16593778133392 0.177754670381546
4.75829553604126 12.2802181243896
-1.25987040996552 0.223485320806503
4.84539651870728 -1.20662879943848
-0.557311713695526 0.574214041233063
6.50289249420166 32.7827301025391
1.25485014915466 2.99745678901672
-0.968294143676758 0.963742852210999
-0.97124969959259 -0.0228397343307734
1.3307718038559 1.28071510791779
0.868597269058228 -0.789819717407227
0.380486309528351 -2.4004979133606
0.773810148239136 -0.830172181129456
-2.69729471206665 0.0839300751686096
-4.61142492294312 -0.109569579362869
2.06625509262085 -0.299513339996338
-0.194306582212448 -1.4767849445343
3.7692813873291 4.99284553527832
-3.782555103302 0.420179098844528
1.94159758090973 0.362160056829453
-4.52007722854614 0.138327896595001
-1.82687997817993 0.0771938860416412
-2.04666447639465 0.373796433210373
3.85479521751404 -7.0499382019043
0.361251413822174 1.16282856464386
1.90682315826416 3.04740238189697
-5.35911846160889 -0.0084940018132329
-3.08455610275269 0.0230587273836136
-1.19889199733734 0.635937809944153
-5.52960538864136 -0.0485507175326347
-1.56089687347412 -0.104760482907295
3.34277963638306 4.65030002593994
1.47303986549377 0.869939208030701
-2.13030362129211 0.327091336250305
-1.22192597389221 0.467447191476822
2.45536327362061 -0.70820939540863
-1.35684323310852 -0.209121495485306
-2.95192909240723 -0.0931701958179474
0.256360560655594 -0.204091221094131
5.67047357559204 -11.4125986099243
2.38298797607422 -4.97417736053467
7.67350101470947 49.1213912963867
1.2803590297699 2.76716685295105
-1.21978318691254 0.00344455242156982
1.94118189811707 -0.710233926773071
-1.5852085351944 0.896122634410858
4.51461362838745 3.15988397598267
3.95308589935303 10.0066766738892
6.34542751312256 -18.1935043334961
-4.79889822006226 0.0499519594013691
-2.45123982429504 -0.330067932605743
3.04847741127014 -4.54486656188965
5.26430702209473 -2.50805020332336
-1.5049866437912 0.647387206554413
0.668054759502411 0.443701893091202
5.61486768722534 -6.98116636276245
-0.920501828193665 -0.888919115066528
-0.081904761493206 0.500800728797913
0.149306282401085 0.508561253547668
0.677643060684204 1.30325269699097
-3.44928550720215 -0.136648952960968
1.5060783624649 1.10681259632111
-5.45976161956787 0.109236687421799
-1.276740193367 0.157802939414978
-0.0238015577197075 -1.25347793102264
-0.119544290006161 -0.802628993988037
-0.207078993320465 0.099316343665123
-2.56281113624573 0.254185736179352
-3.09942269325256 -0.107841409742832
-1.85077393054962 -0.455720692873001
1.82485210895538 1.55300748348236
5.04950618743896 5.70691061019897
-2.39307188987732 -0.367956459522247
-0.387970685958862 0.823127269744873
5.08826303482056 -4.47435188293457
0.0528384745121002 -1.26193857192993
2.53510355949402 -3.90799760818481
0.427913784980774 0.0025198757648468
2.78795409202576 -2.52287673950195
-0.720475196838379 -1.42828440666199
6.28935766220093 12.0113439559937
-0.164440870285034 -0.585360884666443
0.856199681758881 1.37598073482513
3.74603962898254 6.89486646652222
3.06192898750305 4.69120645523071
1.25377690792084 2.38187551498413
-2.54604935646057 -0.759844183921814
4.91556739807129 13.1930980682373
-4.65686893463135 0.0205708779394627
2.92354273796082 -6.97593116760254
-2.17898440361023 -0.175882458686829
6.82816362380981 -11.1421279907227
-4.4188666343689 0.0234761219471693
-1.87035655975342 0.0958513617515564
6.6976170539856 21.3088188171387
-3.34519696235657 -0.242653623223305
2.19563674926758 -1.23201823234558
2.11456751823425 -0.916797399520874
-2.18728947639465 -0.0760791301727295
6.76204633712769 50.2884063720703
-3.35819792747498 -0.000944823026657104
3.59226989746094 -3.34842824935913
3.64400386810303 1.16932058334351
-2.61947798728943 -0.481013983488083
3.72009253501892 6.02695941925049
4.48891019821167 -14.5794563293457
6.14322519302368 -14.2541208267212
-8.96589374542236 0.00303423218429089
1.83928167819977 2.44366931915283
2.72437596321106 -3.79252457618713
-3.01513314247131 -0.176573991775513
0.0719301849603653 1.99780666828156
-1.74999213218689 -0.383120179176331
1.41114604473114 -1.00805389881134
1.04419076442719 2.73400902748108
-0.866915822029114 -0.0834663510322571
-8.49511528015137 0.0136738810688257
-3.12373089790344 -0.0927261263132095
1.39429020881653 0.90277099609375
-3.83807277679443 0.160406112670898
0.935750901699066 -1.05175602436066
-1.23143899440765 0.207370519638062
-1.24829912185669 0.478738397359848
-5.63183355331421 0.000369371846318245
-3.17276620864868 -0.180386886000633
1.01732850074768 1.43988060951233
-4.68553066253662 0.0656806603074074
-0.459192156791687 1.06678354740143
1.33995258808136 -0.471804171800613
1.09790599346161 1.11022889614105
-0.787777900695801 -0.239514827728271
0.938162207603455 -2.14643383026123
-1.99047386646271 0.148137509822845
-6.8689980506897 -0.0285170469433069
-1.11573708057404 0.0900352820754051
0.699217796325684 1.05660593509674
0.195448875427246 -0.385548532009125
2.95237135887146 -7.14495849609375
3.23323702812195 1.34464728832245
-2.97899580001831 0.0513955429196358
11.1723518371582 -55.3289337158203
2.00565028190613 2.84143829345703
-2.36105728149414 -0.203753978013992
-7.02516078948975 -0.00756512116640806
-1.86801600456238 -0.144280448555946
-1.85602474212646 -0.64565122127533
1.85372030735016 -7.00666046142578
-0.361918658018112 -0.925934314727783
-0.543074727058411 0.969716846942902
1.95116114616394 -0.389778137207031
-1.88914704322815 0.416591554880142
-0.632079601287842 0.364958077669144
1.10800719261169 -0.510567128658295
3.61464762687683 -1.77176833152771
1.19284176826477 0.450213253498077
-1.83582496643066 0.133169680833817
-1.51617050170898 -0.533495783805847
-0.199982926249504 -0.798802495002747
-6.3133978843689 0.0487263165414333
-1.52533149719238 -0.218913495540619
-2.72560715675354 -0.282632350921631
-0.76512885093689 0.581202805042267
1.62879812717438 -4.69835472106934
1.6385782957077 -5.58752250671387
-1.07392060756683 -0.815760791301727
-1.81056046485901 -0.0760418474674225
4.60800886154175 1.96100628376007
-0.724368035793304 0.305822014808655
0.754372358322144 0.70535135269165
-1.01859200000763 1.21551430225372
-3.8047616481781 -0.0483126901090145
-2.92630887031555 0.24064302444458
0.0617127120494843 -0.128640666604042
1.12133347988129 -1.04903602600098
2.09858989715576 -4.34826803207397
-0.0842775106430054 -1.3017555475235
-1.67943811416626 0.856176018714905
1.409339427948 -0.122321262955666
-0.590724050998688 0.115655928850174
-1.25944232940674 0.249335527420044
0.101046830415726 -1.95165038108826
1.49297332763672 -0.92704313993454
0.239845335483551 0.896477103233337
-2.16231775283813 -0.178358852863312
-0.282292008399963 -0.241650521755219
-1.59061098098755 0.354753166437149
-1.48144817352295 -0.0428554266691208
0.568862020969391 1.30891418457031
-4.69812488555908 -0.0119468187913299
-3.70995140075684 -0.0736883580684662
-0.0775336623191833 -0.287151843309402
7.45192050933838 -13.2323923110962
-3.84750413894653 0.16046978533268
-1.52418577671051 0.127574473619461
-1.04623174667358 -0.465532660484314
0.567896008491516 -1.82537698745728
7.2922158241272 -54.9461708068848
0.263103604316711 1.06282353401184
-2.82873058319092 -0.56090635061264
-0.389402985572815 1.02930653095245
4.30703639984131 -0.27557110786438
-0.553106009960175 0.259385526180267
-3.13941860198975 -0.0090154018253088
2.8195276260376 3.01094889640808
0.0997476950287819 -0.2477126121521
-0.457376748323441 0.0629674643278122
2.2330858707428 -1.56703126430511
1.50242221355438 0.623510479927063
-0.07888463139534 0.442732304334641
2.05965566635132 1.37489748001099
2.26951956748962 0.402306944131851
-4.22506999969482 0.228226706385612
4.8592095375061 2.06062626838684
-9.53913879394531 0.00379767641425133
-6.46811008453369 -0.00445140153169632
3.34097504615784 -4.77575254440308
3.77950763702393 -1.66527473926544
0.122024238109589 2.45693206787109
-0.0286577343940735 -0.682439923286438
-6.28483963012695 0.0374618321657181
1.57312488555908 1.26212728023529
-0.209330871701241 1.35868442058563
-0.09665447473526 0.366648972034454
-5.84339475631714 -0.138657346367836
2.01682662963867 1.88933479785919
1.25525951385498 -1.27236831188202
-3.77708339691162 -0.0755008831620216
0.396007359027863 -0.691428780555725
-5.18074655532837 0.0619037039577961
-3.98827242851257 -0.0590909942984581
-0.330198884010315 0.0908680260181427
1.15238583087921 -0.393112301826477
0.155407726764679 0.482775032520294
6.33952188491821 -4.07618379592896
8.09600734710693 -72.8164672851562
1.66843461990356 0.659348726272583
2.56863784790039 -3.58399868011475
-4.0900993347168 0.0808513611555099
3.79522824287415 6.38650560379028
-0.204663470387459 -0.210260719060898
-5.09345054626465 -0.100034900009632
1.71951305866241 -5.56644773483276
1.03326225280762 -1.54869771003723
-1.91926443576813 0.125414043664932
-0.721290409564972 -0.266084849834442
-1.48342514038086 -0.796600937843323
-6.70482778549194 0.0574403330683708
0.277204096317291 -0.981281101703644
2.09837102890015 -0.857783794403076
2.88625550270081 -2.83232021331787
0.851323843002319 2.19802665710449
0.842123925685883 1.3722460269928
0.383714824914932 1.17704498767853
1.88217997550964 1.97346615791321
1.33429479598999 2.33985662460327
-4.57780408859253 -0.0900203883647919
-2.99136328697205 0.247943982481956
-0.888171076774597 -0.778252065181732
-2.78207421302795 0.0684676319360733
3.78076314926147 -7.43588399887085
2.62637400627136 -1.91050136089325
-1.95828056335449 -0.308564513921738
2.03424978256226 -1.77796947956085
-1.45523262023926 -0.636654257774353
0.044807780534029 -0.0458691418170929
-0.914083361625671 0.481970071792603
1.93849849700928 -0.365589201450348
2.11848306655884 1.235924243927
-1.84791970252991 -0.521665930747986
-0.742361724376678 -0.0593822225928307
2.08507204055786 -2.24485802650452
-0.937173843383789 1.22553682327271
-5.97713088989258 0.0794272571802139
-4.57745695114136 0.0428774058818817
4.31259393692017 0.844461679458618
4.41861200332642 -6.70863437652588
-4.26203536987305 0.11163929104805
1.84831249713898 0.857008218765259
3.66925048828125 4.11559963226318
-0.855177998542786 -0.416542291641235
-2.27692484855652 -0.546920478343964
2.54643368721008 1.09262704849243
-1.92885375022888 0.384276419878006
-2.80559325218201 -0.149053677916527
1.83379280567169 -1.72079730033875
-0.121978968381882 -0.960277259349823
1.49700677394867 -0.371013104915619
1.15757036209106 1.13533437252045
0.439254462718964 -0.211012482643127
0.446985602378845 0.1916114538908
2.42155647277832 6.47888374328613
-3.73761415481567 -0.0108813513070345
-2.59159803390503 0.021532878279686
-1.27919578552246 0.157984465360641
-4.39801406860352 0.0270383246243
-0.2010617852211 0.714489459991455
0.269284963607788 -0.479871928691864
1.75616085529327 -1.89680826663971
-1.65976786613464 -0.419167548418045
6.43253374099731 -34.9535713195801
1.94743418693542 -0.360063314437866
0.772517085075378 3.13201856613159
2.58821272850037 -4.91420555114746
-0.0832604244351387 1.94204068183899
3.73821043968201 -2.73755192756653
-0.328407227993011 -0.985713303089142
-2.7294294834137 -0.295556932687759
-2.72566342353821 -0.0804121196269989
-1.43415498733521 0.197041541337967
-1.61699783802032 0.161968573927879
4.91861629486084 -14.4272594451904
-4.49575519561768 0.114372603595257
0.779828786849976 1.25169801712036
2.00645971298218 0.592297375202179
2.53579449653625 0.317132264375687
-1.86667776107788 -0.288650512695312
-2.33283495903015 -0.457542955875397
8.16844654083252 19.0157089233398
-4.50618696212769 -0.0635700523853302
3.53225469589233 10.1112403869629
6.89050388336182 20.0268650054932
-2.60409712791443 0.18132583796978
1.12432181835175 -2.57750248908997
0.745662868022919 -1.34542870521545
-3.91603708267212 -0.017172971740365
2.85349321365356 -7.8320369720459
1.69193279743195 0.654974818229675
0.735280632972717 -0.240539595484734
-2.73576593399048 0.312603145837784
-2.50867509841919 -0.0137427449226379
-2.92119741439819 0.00999832339584827
-1.65917026996613 -0.343367457389832
-1.42240273952484 0.161613345146179
0.776811182498932 0.906889498233795
-0.869579672813416 0.420008569955826
4.93539571762085 -13.2277946472168
0.151987016201019 -0.741881132125854
0.856607794761658 1.62471175193787
2.35758948326111 7.92490005493164
-1.16435134410858 0.652074038982391
-1.9802131652832 0.267434418201447
-2.80744600296021 -0.0609798617660999
-1.25921416282654 -0.00444820523262024
0.38288402557373 -0.177353903651237
0.346176594495773 0.47935751080513
3.23330330848694 -3.58729982376099
-1.1989209651947 0.716081440448761
3.02361249923706 -9.45854091644287
1.18987333774567 1.1167004108429
5.48208093643188 32.5261840820312
-0.0325773656368256 -1.66576790809631
-0.389675498008728 0.954747080802917
-7.09751558303833 -0.0094656040892005
1.10337162017822 1.32545018196106
-1.80618250370026 -0.464533448219299
-0.393299788236618 -0.36216151714325
-0.150382906198502 0.887300729751587
-4.29552459716797 -0.0799637138843536
-0.364132821559906 0.578807950019836
2.08948707580566 -1.96307861804962
-4.88986206054688 0.015542060136795
-3.18994164466858 0.152381956577301
4.82494163513184 -16.1566047668457
1.30002343654633 -1.34037435054779
4.4066276550293 -4.05606698989868
0.0778549462556839 0.790891289710999
4.44164228439331 -2.34481477737427
-0.787781655788422 -0.100497782230377
-1.86074376106262 0.30158269405365
-4.57396411895752 0.00374558381736279
1.59744834899902 -1.98785328865051
6.99892282485962 44.9204521179199
-1.86604857444763 0.0889573246240616
2.35452079772949 4.04717779159546
0.888045907020569 -2.26314926147461
-3.15199303627014 -0.0461488403379917
0.501814007759094 0.35501417517662
-6.86187982559204 0.0551558323204517
3.03403043746948 -5.44467353820801
-1.78508412837982 0.58407062292099
-1.42565941810608 -0.192730009555817
0.534265160560608 -0.690388441085815
};


==> figures/visualizations/funnel/gmmvi_samples.tex <==
\addplot [semithick, gmmvi, opacity=0.7, mark=x, mark size=3, mark options={solid}, only marks]
table {%
-1.93930041790009 0.0274647977203131
-1.14557862281799 0.78064501285553
-1.11602401733398 0.275223702192307
4.24004173278809 -5.76905298233032
-2.2781229019165 -0.0191496759653091
-4.45291233062744 -0.0286688264459372
-3.14529228210449 0.123492233455181
-2.42486691474915 0.209317371249199
-7.44819593429565 0.00244465377181768
-1.26867055892944 -0.43818187713623
-1.33419585227966 0.763352453708649
1.90985560417175 7.06694936752319
0.853903412818909 1.15878069400787
2.40208315849304 -4.33283805847168
5.23194694519043 -14.6050500869751
0.471729248762131 0.268007040023804
0.772069334983826 0.0613982900977135
5.26675033569336 14.8788356781006
-1.50244927406311 0.0902679413557053
0.820206522941589 0.658798158168793
-4.96707201004028 -0.15015321969986
1.96566140651703 0.395188629627228
1.24774563312531 1.50236475467682
1.22060441970825 -1.25749921798706
-0.706941187381744 -0.339953243732452
3.13798761367798 -4.71289110183716
3.68470025062561 1.29690992832184
-1.79566383361816 -0.494715213775635
0.588742971420288 0.97293883562088
0.732616662979126 -0.960012674331665
4.21275043487549 6.17623233795166
4.05741453170776 9.27587413787842
4.6139702796936 -0.404728770256042
-3.48749613761902 0.0785267204046249
-1.12180590629578 0.0487161427736282
3.0858998298645 4.56491327285767
7.23988485336304 9.87482738494873
-5.41901254653931 0.0913484245538712
-4.72631406784058 0.0238033644855022
0.106026202440262 0.880626559257507
-8.3533935546875 0.00941532105207443
1.7693704366684 1.01142847537994
-2.55940508842468 -0.000684699625708163
1.65101325511932 -2.55084824562073
0.672470271587372 1.44179368019104
0.561142086982727 1.68097877502441
1.79551446437836 -1.87735235691071
0.111352540552616 -0.461651355028152
-4.59275531768799 0.0338422358036041
-4.5656852722168 -0.0853374972939491
-6.27280569076538 0.00127250060904771
4.62562608718872 -2.38731384277344
-2.60033512115479 -0.268850475549698
1.94384336471558 -0.61408519744873
-0.296288669109344 -0.412924826145172
-1.722123503685 -0.807641208171844
-7.02323579788208 -0.0120532680302858
-1.13677000999451 -0.831259191036224
-1.5679167509079 0.00271552661433816
4.03974771499634 2.73887038230896
-6.42422914505005 0.0202530175447464
1.44160354137421 -1.17005097866058
5.56291437149048 13.516206741333
-1.59926080703735 -0.0991566181182861
1.3009318113327 -2.08103227615356
-0.464770346879959 0.421406418085098
-1.28306722640991 0.226361498236656
1.76208996772766 4.41235065460205
-4.13904333114624 0.193298429250717
0.409625351428986 0.100130170583725
1.42864573001862 -1.64178144931793
5.48830413818359 -11.550760269165
-1.12317204475403 0.213656172156334
4.12228202819824 5.93943881988525
0.361956685781479 0.420519173145294
-3.00604462623596 0.143767729401588
-5.7924919128418 0.0188155602663755
2.85805892944336 -3.96847820281982
4.10010671615601 -5.36764335632324
-0.624105393886566 0.103771291673183
-0.69997251033783 0.88171648979187
-4.99208116531372 -0.0924966782331467
2.17081642150879 4.17023134231567
1.35510230064392 -0.305323570966721
1.78227293491364 0.786781013011932
0.0884747803211212 0.8914994597435
-4.83662843704224 0.097786121070385
-0.434827893972397 -0.0146344266831875
-1.86103928089142 0.158760130405426
-2.66951394081116 -0.242848828434944
3.94089770317078 2.21199512481689
3.22010445594788 0.842576742172241
2.87658143043518 -3.287034034729
2.01695346832275 -2.15970778465271
-2.6858286857605 0.031674113124609
-0.162870094180107 0.774881958961487
-1.04914617538452 -0.368753254413605
2.71428680419922 0.65307742357254
1.37376356124878 -0.00507627427577972
-0.25897940993309 -0.387324780225754
3.73752331733704 -3.28928303718567
-1.36987960338593 -0.27653494477272
1.42998480796814 4.48881673812866
-2.13094353675842 0.235151216387749
-1.63889133930206 0.136366873979568
5.19799327850342 -25.9628810882568
0.938787817955017 -1.35460448265076
-3.17230010032654 -0.129656329751015
-5.14321184158325 0.0370886661112309
1.15393090248108 -3.65801358222961
-4.45126485824585 -0.0224450770765543
-0.23661145567894 0.706751108169556
-1.45829772949219 0.53524923324585
-3.68460750579834 0.0653457343578339
-4.89697360992432 -0.0920714735984802
3.75947546958923 1.96939373016357
0.154288649559021 -0.0829390734434128
-4.08403968811035 0.0919691100716591
4.99316740036011 -11.307544708252
1.14431416988373 0.336387753486633
-0.00361253321170807 -1.51697325706482
-0.431964904069901 0.623425602912903
4.57770490646362 2.34115529060364
2.38327574729919 -0.810411691665649
0.982236683368683 1.37911176681519
1.16192603111267 -1.19859302043915
-0.215016424655914 0.139308005571365
-2.39213991165161 -0.170199036598206
-4.09841823577881 0.273238003253937
-0.283060997724533 -2.17337250709534
-1.16187012195587 -0.848130106925964
-1.05116260051727 -0.297808557748795
0.911264657974243 0.0249741673469543
4.53915977478027 7.43084478378296
-0.88445782661438 -1.48428928852081
-3.53515362739563 -0.13631734251976
1.53606200218201 0.60411524772644
0.569231271743774 -2.6266655921936
3.09260249137878 5.14090585708618
-0.0435614958405495 -0.46897080540657
-1.69437503814697 0.50460547208786
0.166641056537628 0.194470897316933
-3.64796161651611 0.0151448715478182
4.69076299667358 10.4603624343872
-2.68352174758911 0.00169987324625254
0.59111487865448 0.202386304736137
1.42435050010681 -3.29497003555298
-1.66440546512604 -0.0205198880285025
-3.2812488079071 0.113964200019836
2.89766240119934 1.98727369308472
-7.21558952331543 0.00746014341711998
3.53322505950928 -4.14619588851929
3.36871957778931 -6.39310932159424
-1.97694218158722 0.151831954717636
1.21663403511047 0.425948202610016
0.242268308997154 -1.15926706790924
1.650355219841 5.0030574798584
2.17981910705566 -1.62780606746674
0.666886508464813 0.152013808488846
0.147004753351212 0.656181991100311
-0.369986444711685 0.856681406497955
-0.617450416088104 0.465354382991791
1.59484267234802 -4.02326345443726
-4.19202899932861 0.10118917375803
-3.29349255561829 0.0485427714884281
3.61817812919617 -6.46539354324341
-2.00860738754272 0.207512781023979
-1.46260023117065 -0.246907323598862
4.3390851020813 -1.10995674133301
-0.093149870634079 1.0418815612793
3.02413702011108 8.3634729385376
-0.875021457672119 0.217993810772896
2.36234736442566 1.88679981231689
-2.34439086914062 0.421822905540466
3.72407245635986 1.03105342388153
3.23391509056091 -0.600621223449707
-1.93738222122192 0.132905870676041
-0.327073454856873 1.09463357925415
0.154202610254288 -0.9908287525177
-3.80878710746765 -0.119187265634537
0.188686609268188 0.443434000015259
0.68517279624939 -0.709523558616638
0.759737491607666 -1.59606981277466
-1.17570459842682 -1.41470324993134
-0.434803009033203 -0.932079911231995
-0.333169996738434 0.684507310390472
0.178293585777283 1.24956035614014
4.08841562271118 -4.83789825439453
2.47275924682617 4.90851354598999
1.67768621444702 -4.52010440826416
-2.03117489814758 -0.112236343324184
-1.30263519287109 -0.290573179721832
-0.901196181774139 0.124757006764412
-6.58225917816162 -0.0295694246888161
-3.76536297798157 0.05319719389081
5.0787525177002 3.01329350471497
-0.0200724080204964 0.242504671216011
1.49661874771118 1.36616504192352
0.739288628101349 -1.37727832794189
0.639900624752045 -2.46078038215637
-2.11227464675903 -0.590846180915833
-2.7739589214325 0.121350184082985
-1.65162789821625 -0.113515734672546
-0.57893979549408 -0.66988867521286
1.71594250202179 -0.600749015808105
-0.177720963954926 -0.101729214191437
-1.3611079454422 0.0712250545620918
-1.53687250614166 0.644349336624146
-0.166178792715073 1.45611345767975
3.20303916931152 -1.82815825939178
-0.97086089849472 0.559958636760712
6.1920485496521 29.0776481628418
3.09410405158997 0.454615920782089
-2.06224608421326 -0.127807527780533
0.712613344192505 0.368972331285477
0.573860883712769 -1.83914887905121
1.52427613735199 -1.58504915237427
-2.22362923622131 0.253080189228058
-9.63378620147705 0.00061298260698095
0.409083306789398 0.480267703533173
2.39784789085388 -2.29871535301208
-1.16241502761841 -0.128002628684044
3.17085456848145 6.42184734344482
3.83158707618713 7.75698280334473
-5.76374959945679 -0.0502995625138283
1.84154284000397 2.14967036247253
1.2439239025116 -0.850223302841187
-0.448568850755692 -0.42320990562439
-7.24798250198364 -0.00793742202222347
2.62202334403992 1.35693168640137
-1.49472427368164 0.421567052602768
-1.3280725479126 0.0674902647733688
-0.998344123363495 1.02656805515289
-1.27469074726105 -0.0360036455094814
-1.63957345485687 0.279568761587143
-0.447198569774628 -0.841930091381073
-2.84895014762878 0.640199303627014
3.15987873077393 0.105845972895622
1.0527275800705 -0.335551053285599
-3.18315434455872 -0.0306236930191517
-0.343200743198395 -0.235929802060127
-4.74012804031372 -0.0581857226788998
-1.4027658700943 -0.0166298281401396
-1.9955587387085 -0.151142597198486
0.71444046497345 1.07589721679688
-7.23538637161255 -0.0154703492298722
-0.917443752288818 0.117275893688202
-0.663258969783783 -0.18660469353199
1.3372950553894 -1.66883850097656
0.595594108104706 -1.47057116031647
-2.4661123752594 0.215740919113159
1.28832340240479 2.95329713821411
-3.5136604309082 0.124394975602627
-0.716197729110718 1.8533091545105
-1.55860638618469 0.184734240174294
2.64749765396118 -6.80359983444214
5.35240316390991 0.376597762107849
1.41859090328217 -1.74557852745056
-4.20634651184082 0.174697279930115
1.43991732597351 -0.583554625511169
-1.68378102779388 0.204333424568176
0.134081244468689 -1.35276794433594
4.65218496322632 2.60468816757202
-0.349402368068695 0.5966437458992
-3.8741672039032 0.24351179599762
-1.30491244792938 0.104207716882229
0.257108449935913 0.133631870150566
-0.9799644947052 -0.484484493732452
-2.44092559814453 0.363038808107376
7.40336990356445 -6.90195846557617
3.47604727745056 -9.89761352539062
0.766160130500793 0.976361334323883
-1.48391509056091 0.243753269314766
4.75415134429932 -14.6692743301392
4.27689552307129 12.1096467971802
2.32504653930664 6.50096130371094
-1.16850209236145 0.0806023925542831
-1.25092089176178 -0.203463360667229
-0.229103326797485 1.07194685935974
-1.72977089881897 -0.322473794221878
4.91804218292236 -3.88408660888672
-0.311206549406052 0.293108761310577
-0.0619715601205826 0.78655469417572
-2.83424687385559 0.13446170091629
0.835479497909546 -0.847424685955048
0.10932631790638 1.57561349868774
-0.43421071767807 -0.535358548164368
-8.19956207275391 0.0157364457845688
1.66177988052368 0.132330000400543
-1.09487557411194 -0.673859059810638
1.05803275108337 1.23139846324921
4.58310842514038 12.40784740448
3.07536506652832 3.37997794151306
2.16446685791016 0.972262740135193
2.0338306427002 -2.04366016387939
-0.313112407922745 0.651351571083069
0.0404664129018784 0.420849710702896
2.54064798355103 -0.929996252059937
-5.83633136749268 0.0025705611333251
5.64678621292114 3.03891324996948
-3.6128842830658 0.222855404019356
4.17971897125244 3.47963070869446
-3.72834730148315 -0.19453452527523
-1.00126838684082 -0.183791995048523
-0.536385476589203 0.161689087748528
-0.173477783799171 -0.0810959339141846
2.21688032150269 -0.211226552724838
3.7590320110321 3.58342409133911
-6.48232841491699 -0.0225214790552855
0.628252625465393 3.61518311500549
-1.70569705963135 -0.0189041271805763
-0.256692111492157 0.126023650169373
-5.19806241989136 -0.0285861250013113
-3.48182082176208 -0.374884098768234
0.588881254196167 -0.375682681798935
1.48981046676636 -1.52475237846375
-3.26272630691528 0.295359313488007
0.750138819217682 1.82801079750061
0.866816103458405 1.06019043922424
2.76510071754456 -5.43098115921021
1.24482786655426 5.24187755584717
-1.0346462726593 -1.23462700843811
3.03024697303772 -3.4808611869812
-2.05901336669922 0.0960874482989311
-1.47839462757111 0.156922161579132
-1.62473154067993 0.220673426985741
0.699720740318298 -2.14249968528748
0.529301524162292 1.66885697841644
3.65427613258362 0.464569389820099
-0.895691275596619 -0.642491102218628
4.1955509185791 -7.00260639190674
-6.89134550094604 0.0126879075542092
-0.520577073097229 -0.590356945991516
1.59159600734711 1.57881379127502
-1.4504816532135 0.364588886499405
1.28311324119568 3.58098244667053
-0.609396934509277 0.154911756515503
2.4900004863739 2.59711933135986
1.93355119228363 1.39018630981445
-1.70146870613098 -0.355025231838226
-1.2246572971344 -0.209213212132454
0.757757782936096 -1.13072955608368
2.26249361038208 -1.84932422637939
-2.22260475158691 -0.521257877349854
-4.17513275146484 0.282893389463425
4.20420455932617 1.18440365791321
-2.71133661270142 -0.304993838071823
0.558294296264648 -1.43821108341217
0.105801820755005 -0.598007798194885
-3.43009114265442 0.12745076417923
6.19541072845459 12.4565210342407
-2.97625088691711 0.305642694234848
-1.10520219802856 -0.997704029083252
1.18471169471741 -0.970366299152374
4.68254661560059 -8.85898113250732
-3.66226315498352 0.161244973540306
-3.70158958435059 0.124036066234112
-3.73502564430237 -0.162998422980309
3.94614553451538 3.22668719291687
-3.53846073150635 -0.287078082561493
2.87584400177002 3.42955803871155
1.82457506656647 -2.4113130569458
-2.66542553901672 0.0949259176850319
3.71442794799805 -9.66289806365967
-0.929315149784088 -0.314301759004593
-3.2220311164856 0.195108726620674
0.0584570281207561 0.538438379764557
1.17125523090363 1.57903623580933
0.503228485584259 1.08025050163269
4.15100049972534 3.93043947219849
-2.62007451057434 0.0975047573447227
-2.937575340271 -0.119210436940193
-0.681863725185394 -0.507391154766083
-1.18441438674927 0.379745781421661
-5.20269680023193 0.137813106179237
3.72775673866272 5.66149520874023
-5.54703855514526 -0.0147131700068712
1.86841213703156 -1.57113587856293
-0.762093305587769 1.71770083904266
-1.93860769271851 0.548312246799469
-7.55120706558228 0.00492901680991054
5.86795234680176 -13.8136539459229
-3.45580196380615 0.101039506494999
-2.26800179481506 -0.0802089795470238
2.56777119636536 4.42616081237793
-2.92117357254028 0.467381745576859
-4.66716623306274 0.0607220716774464
-1.13363862037659 -0.340079754590988
1.46373987197876 1.98090326786041
0.205817043781281 -0.206861972808838
8.00563430786133 5.8718433380127
2.23987078666687 5.64183378219604
3.40729665756226 0.14278969168663
7.28086090087891 23.1468276977539
6.30325555801392 30
-1.76196694374084 -0.274892300367355
-4.43158102035522 0.0324046723544598
1.02690601348877 1.70523965358734
1.37182259559631 -0.156029105186462
-5.99945306777954 0.0191883333027363
0.454809784889221 -0.0827043354511261
3.12982416152954 -6.79627084732056
-0.964109539985657 0.203823298215866
0.000382069498300552 -1.34525811672211
-0.846948504447937 0.227381676435471
2.19998979568481 -2.19543671607971
2.33026266098022 -0.778693437576294
-3.47702670097351 -0.0227076672017574
-0.473167687654495 -0.985222578048706
-1.26060855388641 -1.08435618877411
-0.960061550140381 0.264022707939148
0.052546177059412 -1.10374212265015
-4.37753391265869 0.0364889577031136
2.82584857940674 -5.35376453399658
4.32297945022583 -6.18930101394653
-2.16603207588196 -0.126872405409813
7.33457660675049 26.2801456451416
3.27099275588989 1.74829936027527
-0.605497539043427 0.961127698421478
2.34345984458923 1.68259119987488
-3.79512763023376 0.168650031089783
-5.10431432723999 0.0288251060992479
-0.846327185630798 0.798858106136322
-1.68540382385254 0.674489438533783
-0.569032549858093 0.833495676517487
-0.472615301609039 -1.2173490524292
1.37746000289917 0.702277660369873
1.85975742340088 3.09491276741028
0.924154341220856 -1.92320430278778
1.04320597648621 -0.239334151148796
2.78412771224976 3.86162829399109
2.80634927749634 -1.569131731987
-0.106752589344978 1.33071577548981
-2.16370415687561 -0.176585778594017
-3.68760371208191 -0.175812989473343
-2.10504364967346 0.700836837291718
2.61628580093384 -2.55366063117981
2.06917023658752 2.57769727706909
2.84569358825684 -7.05466508865356
5.92504978179932 4.46491861343384
1.96584105491638 0.0916570425033569
-0.632517218589783 0.698556661605835
-5.10137128829956 0.105649702250957
-0.963439524173737 -0.0987366586923599
-3.76220536231995 -0.0512903816998005
-2.67167854309082 -0.151109173893929
-5.89451885223389 0.00614453898742795
-1.23892140388489 -1.60868883132935
-0.83139580488205 -0.553782999515533
3.58418154716492 8.99545764923096
-2.72664093971252 0.147595316171646
-1.40632128715515 -0.882287859916687
-1.37596082687378 -0.539780676364899
2.88207006454468 1.29228043556213
2.48032760620117 -3.00147080421448
2.34416103363037 -5.85726833343506
4.91014671325684 -7.29175281524658
0.761104822158813 0.698127806186676
1.60345125198364 5.31527614593506
-4.61281394958496 -0.0241277571767569
-7.04446649551392 -0.0381298214197159
0.273462772369385 0.927231788635254
-0.288576751947403 0.521625697612762
0.927588701248169 2.65436720848083
0.323050796985626 1.02562344074249
1.48789954185486 -1.68798494338989
2.56683778762817 1.76861429214478
-0.441070914268494 -0.215857610106468
2.22750449180603 -1.07793939113617
1.85887539386749 3.99638772010803
-2.87754273414612 0.195076510310173
3.48378801345825 -5.06655693054199
-1.82742726802826 -0.29323348402977
-1.49378073215485 0.18390941619873
-2.31367111206055 -0.389083683490753
3.20706820487976 6.85973024368286
-2.07108688354492 0.4899722635746
1.58482646942139 1.42096042633057
-2.80340147018433 0.251320421695709
0.798078954219818 1.30206084251404
-2.64988541603088 -0.049373310059309
-0.261876493692398 -0.414099395275116
-3.53538250923157 -0.00261596590280533
-4.29223108291626 0.0766838192939758
-3.09833335876465 0.0124842245131731
-7.38742160797119 0.0184327010065317
-3.12056756019592 -0.04735142365098
0.282007992267609 -0.260910719633102
-0.420069396495819 0.590577781200409
-4.29602146148682 0.0618542842566967
-1.04764556884766 0.302796453237534
-3.34023118019104 -0.0860784873366356
3.21570944786072 -4.58020114898682
0.42540255188942 -0.660945236682892
0.509003520011902 0.106580853462219
-0.0641819536685944 0.759543478488922
-0.706203937530518 -0.22907580435276
-0.466375410556793 0.362217456102371
6.15128087997437 18.568489074707
4.16820335388184 -18.7753372192383
-0.254391759634018 -0.315270662307739
-3.49989986419678 -0.168798804283142
1.30387234687805 1.33187758922577
3.58186674118042 -0.833344340324402
0.236799255013466 -0.927751243114471
2.27929329872131 0.605737805366516
0.810942947864532 0.826354205608368
-5.12117671966553 0.080810084939003
0.928915739059448 -1.07352483272552
-1.52963352203369 -0.426583141088486
-1.69146585464478 -0.852123916149139
-3.10414671897888 -0.0861116945743561
1.08206152915955 -0.458639115095139
3.59779381752014 0.167895317077637
1.12138485908508 -0.419133484363556
-4.33547782897949 -0.0549972578883171
1.30968153476715 0.738115906715393
1.3736674785614 1.41947519779205
-2.69825148582458 -0.303424865007401
-0.245158523321152 0.117289088666439
0.654769718647003 -2.0117552280426
-4.04100656509399 0.104729436337948
1.0352303981781 0.522552192211151
0.632367610931396 1.1732097864151
-2.66893696784973 -1.07610332965851
-4.75873184204102 0.0521651171147823
1.21120619773865 0.936569571495056
0.453155994415283 -0.335983574390411
-2.36883664131165 0.308019816875458
-7.20669317245483 0.0328575819730759
-1.77477443218231 -0.716805756092072
-2.40163779258728 -0.0711436793208122
-0.282375633716583 0.182144269347191
2.29734301567078 -6.51056146621704
4.04146146774292 -13.9499530792236
-6.20854902267456 0.0291504692286253
-2.12395834922791 -0.452014356851578
1.07292354106903 -1.38702881336212
-2.66749310493469 -0.653440475463867
2.21702694892883 -1.05727231502533
-1.47012388706207 0.183125883340836
-0.118423417210579 -1.18808805942535
-5.60705852508545 -0.0334598459303379
1.52177977561951 -0.922030031681061
0.558216273784637 0.260572880506516
0.679024696350098 -1.41204249858856
-0.0207537189126015 0.789415955543518
0.690667510032654 -0.759174942970276
-0.394129991531372 -0.938805937767029
-1.80823564529419 -0.0689553245902061
0.617922067642212 0.28143447637558
3.13125586509705 2.29660606384277
-6.47797393798828 -0.0150749962776899
-0.647608697414398 1.33387565612793
1.90007376670837 0.287485241889954
0.118754409253597 0.362665951251984
0.0647262781858444 1.92794990539551
-0.541902422904968 1.1616952419281
-2.70737385749817 -0.0558942444622517
3.41523003578186 0.824827790260315
-2.58460569381714 0.0248369015753269
-3.40982580184937 -0.028143897652626
-0.84962010383606 -0.248405918478966
-0.969020545482635 -0.311845928430557
7.32012987136841 5.47367095947266
3.6192090511322 -6.32574510574341
-6.69748973846436 -0.0371258892118931
0.166332870721817 -1.55050468444824
1.6980916261673 -5.31683206558228
-1.55749440193176 0.257326394319534
2.90111041069031 10.6243801116943
3.20398116111755 2.65080332756042
0.556078374385834 0.963762938976288
-6.62046432495117 -0.0182790644466877
1.58082389831543 -0.709016263484955
-3.89456963539124 0.00851991679519415
0.115101039409637 0.80355304479599
-4.45645141601562 0.0278175678104162
3.45201325416565 10.9349975585938
-5.74215650558472 0.0323062352836132
-2.74808073043823 0.0759685933589935
-2.07513356208801 0.0116476295515895
0.439269840717316 0.987448751926422
1.33607196807861 0.890210390090942
-5.46754503250122 -0.0355644188821316
-0.738524615764618 1.4833881855011
-1.05155408382416 -0.58671772480011
6.10853290557861 5.26238298416138
1.3969738483429 -0.621835708618164
-3.0215585231781 -0.133514150977135
-4.8609733581543 0.0456716902554035
-4.04589509963989 0.193185403943062
1.85498058795929 -0.63064306974411
-3.11777329444885 0.245325461030006
-3.75902128219604 -0.135623335838318
-1.07738709449768 1.64160478115082
3.03698134422302 1.64831721782684
-1.74906766414642 -0.822413802146912
1.86823642253876 0.067743331193924
-1.95728647708893 -0.22742472589016
2.79783892631531 -8.54624366760254
7.57649040222168 -30
1.03483009338379 -0.454501658678055
-3.48233032226562 0.0104400655254722
-4.07611465454102 0.338689267635345
-0.343110680580139 0.0154365375638008
5.43713808059692 -7.76063251495361
-3.10656094551086 -0.0874033197760582
0.857492446899414 0.0437355786561966
-0.434487551450729 0.202000662684441
1.23628330230713 0.477549344301224
2.61256551742554 -0.200453400611877
4.11005020141602 8.48286819458008
-1.31892788410187 -0.0808979570865631
2.75186920166016 -7.33031177520752
-3.49979567527771 0.115940921008587
-2.92236161231995 -0.0266774855554104
4.93983364105225 8.52674579620361
4.58765602111816 -0.923252761363983
-2.00086283683777 -0.468737721443176
3.84407162666321 8.61777019500732
2.13578748703003 0.618409752845764
-0.232538253068924 -0.824600994586945
-0.64827024936676 0.237736687064171
1.34911513328552 0.136057123541832
-1.03021252155304 0.0436289422214031
0.856685996055603 -0.435394167900085
0.640265703201294 0.384950041770935
4.08109617233276 11.9973173141479
4.33373975753784 10.9296064376831
2.44296598434448 5.79949617385864
-1.98487997055054 -0.0153605006635189
-4.04103660583496 0.0420830622315407
-4.70110321044922 -0.0125927682965994
0.331387907266617 0.487623393535614
1.33552551269531 -0.982899129390717
-3.16853523254395 0.0199629738926888
0.911782085895538 0.430142641067505
-2.50395917892456 0.238899454474449
-1.02930724620819 0.338045924901962
-1.04426550865173 -0.769892036914825
2.04146099090576 -2.08105444908142
3.98120522499084 -4.31491184234619
-3.00141024589539 0.202684178948402
-1.84225022792816 -0.567356705665588
-1.45691013336182 -0.699195921421051
-0.857837796211243 -1.28261911869049
4.05354738235474 16.1732139587402
-1.35926353931427 -0.12043322622776
-4.45892190933228 -0.0181580055505037
0.676172494888306 -1.82059240341187
4.57099866867065 13.1833629608154
1.57072854042053 2.33036971092224
0.749817669391632 -1.18893921375275
2.14692497253418 3.32590961456299
0.667920708656311 -0.642934560775757
3.70626401901245 -3.0640549659729
-0.855124831199646 0.476159274578094
-1.80393981933594 0.172922819852829
-1.72646403312683 -0.498361885547638
0.949658870697021 0.871704876422882
0.504108071327209 0.692443311214447
-0.774237275123596 0.0563164502382278
-0.940471589565277 0.672436118125916
4.38108825683594 -2.80559158325195
1.52223920822144 3.24346709251404
3.0254373550415 -4.38131046295166
0.59664261341095 0.0809661597013474
-0.428695529699326 0.0257420595735312
-6.88428068161011 -0.00496208667755127
2.34647750854492 2.73838686943054
2.1382167339325 -2.4239547252655
2.5143358707428 -0.166602209210396
-0.420500934123993 0.653741717338562
-1.125852227211 0.0233025476336479
-5.97585868835449 0.0288804080337286
-1.3985356092453 -0.662966072559357
0.455968260765076 -1.60053944587708
-2.93037486076355 0.0552595891058445
-4.80531644821167 0.0690665021538734
-2.99983906745911 -0.173155561089516
-1.59494984149933 -0.160646870732307
-3.78383016586304 -0.0949815288186073
-0.486029595136642 -0.994500637054443
1.34712409973145 -1.10235369205475
0.384499490261078 -1.06843435764313
0.310397386550903 -0.772896707057953
6.56543302536011 23.3868598937988
1.36098396778107 -1.48391997814178
1.65532112121582 -0.513977289199829
-1.40740084648132 -0.535435140132904
-0.763251960277557 0.0200430266559124
-3.76142168045044 0.101205237209797
2.21832942962646 1.15437829494476
-3.03722810745239 0.070029690861702
-3.56864595413208 -0.174734249711037
-2.42139577865601 0.0186670944094658
-7.08783912658691 0.0141437156125903
1.34097361564636 -0.258480668067932
2.18817639350891 1.18789851665497
1.2732812166214 -2.96393847465515
-3.44734025001526 0.368911117315292
-3.02979755401611 -0.303529649972916
1.53596496582031 -5.35977506637573
5.31823015213013 -16.9181995391846
1.80817520618439 -4.1994800567627
3.57142853736877 2.55174112319946
0.349264532327652 0.0589840710163116
2.51635980606079 -0.420219361782074
3.33270597457886 -4.68357038497925
-0.211146235466003 0.684332311153412
3.06031894683838 -0.740160286426544
-0.823588252067566 -1.10812330245972
0.290582567453384 1.11035513877869
-4.13925790786743 -0.0142000671476126
-1.61664485931396 -0.366101890802383
1.64509010314941 2.73782515525818
1.89874291419983 -2.2029013633728
-3.23731446266174 0.346422016620636
3.16324782371521 11.1351871490479
0.520990073680878 0.76206362247467
0.278344959020615 0.00913052260875702
-4.58978891372681 0.172838747501373
-1.49703085422516 0.193568214774132
-5.30709981918335 0.0838376730680466
-5.60365533828735 -0.0186615902930498
3.23011207580566 2.5687780380249
0.0469395667314529 1.13242852687836
-3.55294299125671 -0.28222918510437
-0.639120578765869 -0.0449654422700405
2.33438062667847 -3.76188182830811
-5.70727396011353 -0.0151658793911338
-1.61471176147461 -0.557929039001465
-2.4767005443573 -0.227892741560936
-1.36194062232971 0.276969730854034
-0.655210793018341 -0.0918126404285431
-0.940937340259552 -0.221133098006248
-2.59353995323181 0.460838586091995
2.10362434387207 -1.66107594966888
1.50627493858337 -3.69214272499084
4.89868640899658 5.67541933059692
0.324831396341324 -0.800974071025848
1.2960079908371 0.817989468574524
3.94859552383423 2.79436087608337
2.31290125846863 1.34667491912842
-5.13841485977173 0.0456472225487232
0.141500234603882 -0.789914667606354
-3.41800832748413 0.0166544038802385
0.314038991928101 2.52437114715576
0.815611004829407 -0.229172959923744
-0.10241587460041 -1.01537215709686
-3.37198305130005 0.0700614005327225
-4.97867441177368 -0.195054396986961
1.3418425321579 2.87921786308289
-2.7219614982605 -0.220352560281754
-5.76532077789307 0.042171623557806
0.0643312931060791 2.42417931556702
1.36753249168396 0.388583213090897
0.0880874246358871 -1.37476372718811
1.27838218212128 -0.781495213508606
1.24690222740173 -0.154319390654564
6.06710290908813 17.3160533905029
0.538668036460876 -1.00331497192383
3.11280870437622 0.534431219100952
2.31465005874634 -5.44945907592773
0.997417688369751 -0.0135854305699468
4.28412342071533 3.80218148231506
4.85693740844727 -4.32743453979492
-0.213636577129364 -0.372367352247238
0.151421964168549 -0.0864638909697533
0.817857444286346 1.32440626621246
-6.30169343948364 0.0377604514360428
3.29373908042908 4.62940645217896
-1.70292353630066 -0.342793226242065
-3.39130473136902 -0.0442018434405327
-2.42234897613525 -0.0878285616636276
-5.7802300453186 -0.00796086154878139
-1.24081873893738 -0.0927948504686356
-6.55908393859863 -0.0759586021304131
2.69703269004822 -0.116662964224815
3.88812613487244 -0.3890340924263
-3.55060815811157 0.0465157106518745
-0.368831515312195 0.0869945585727692
-2.12912273406982 -0.333566844463348
-1.43891167640686 0.447137951850891
-5.25380516052246 0.140312612056732
1.34180021286011 -1.63670456409454
-2.10210871696472 0.559768319129944
1.1829799413681 -0.452328592538834
-4.94224882125854 -0.156136363744736
1.88561534881592 -0.681133091449738
-4.50629234313965 -0.0541733205318451
-1.10135674476624 0.901069641113281
0.000827543437480927 0.989834010601044
-0.455583333969116 -1.53737020492554
-0.773130238056183 0.252787709236145
-5.82220840454102 -0.0284330081194639
-1.7630467414856 -0.650190711021423
-1.21817255020142 0.469946712255478
0.412658154964447 1.30936861038208
-0.430056184530258 0.307799786329269
3.75378203392029 4.60313749313354
2.03226900100708 -4.5380482673645
-3.96859908103943 -0.0279017891734838
3.56419491767883 -2.29783272743225
1.64289879798889 4.85056972503662
-0.262674152851105 -0.46425861120224
1.19292652606964 -0.816493690013885
-2.04109978675842 0.505603849887848
0.191779285669327 -0.0143718114122748
6.31282901763916 -14.7626447677612
2.14256000518799 -0.397376000881195
-1.27194213867188 -0.473351806402206
-0.134026944637299 0.574472308158875
6.05227327346802 -30
-8.95897102355957 0.0210139881819487
4.95361089706421 -3.98415565490723
-5.53910875320435 -0.0570904389023781
-2.8050742149353 -0.0193790830671787
0.221418336033821 0.884595513343811
-3.24544644355774 0.144852742552757
3.74755907058716 -13.3923120498657
-3.01114773750305 0.0731789022684097
-3.2470281124115 0.100620359182358
0.117585428059101 -0.774772644042969
2.4119918346405 -2.13997912406921
-3.36351656913757 0.142209589481354
0.853452324867249 1.96387887001038
0.183182030916214 0.116201736032963
1.69028091430664 1.29050171375275
-1.22296452522278 -0.418344408273697
2.8766872882843 2.60781407356262
1.72813260555267 1.78164494037628
-3.09660172462463 0.306435704231262
1.84868133068085 -3.22281265258789
2.68071317672729 5.4233078956604
-2.36527371406555 -0.0444280728697777
3.97119188308716 -0.493819892406464
0.207367867231369 0.451250910758972
0.772345423698425 -0.746531307697296
-1.46959292888641 -0.588874995708466
-3.20793509483337 0.0334882661700249
0.130637586116791 0.104698978364468
1.6322728395462 0.0131221413612366
1.60591161251068 2.30047559738159
-1.2367696762085 -0.457647234201431
1.11713767051697 0.626836836338043
0.138124197721481 0.366012245416641
0.883131384849548 -0.423353642225266
-2.48797011375427 -0.0184543803334236
1.42569637298584 -1.92223262786865
7.58073806762695 30
0.0920305922627449 -0.806097090244293
5.43386840820312 -8.52005195617676
0.722478032112122 2.16779923439026
-1.64114391803741 0.356054544448853
-2.02597856521606 -0.309340268373489
5.50952196121216 -0.457498967647552
4.88989686965942 -0.807373821735382
3.72946643829346 12.9987020492554
-5.69767713546753 -0.0252824239432812
-3.88309621810913 -0.183571398258209
2.34930038452148 5.64369535446167
3.97297477722168 -20.1577739715576
-2.742516040802 -0.249209329485893
-3.93438720703125 -0.0424760691821575
2.04768800735474 -2.49331116676331
-2.1166136264801 -0.664622724056244
3.55091094970703 -1.17350327968597
-0.302955985069275 0.97504985332489
-0.944472312927246 -0.488434791564941
0.592522919178009 -1.12642920017242
-2.75856518745422 0.39847669005394
-0.196695595979691 -0.618594229221344
-0.804440259933472 0.547764420509338
-3.15783405303955 0.056433729827404
-2.93327236175537 -0.0252505131065845
-0.650495409965515 -0.0453273765742779
-4.88195419311523 0.0950212702155113
-1.22501242160797 0.292514026165009
-4.85722637176514 -0.129705429077148
3.42401218414307 1.63664150238037
1.55307459831238 0.448217898607254
2.11467528343201 -0.934765934944153
1.30569851398468 1.05333805084229
-0.187527045607567 -0.770199835300446
6.32880973815918 14.8503799438477
-3.48516702651978 -0.0478283390402794
-2.53891158103943 -0.335502177476883
-1.53897345066071 -0.898194313049316
4.73049879074097 10.432788848877
-0.742289900779724 1.22672069072723
-1.548464179039 0.630785703659058
4.54393482208252 -4.79404878616333
-6.55286979675293 0.035371758043766
-1.78641879558563 0.644361078739166
-2.28156971931458 0.453263580799103
0.544746518135071 -0.17591780424118
-0.84694892168045 0.13494086265564
-0.703053653240204 0.656549453735352
2.53897666931152 -2.97326731681824
-2.53497982025146 -0.167450025677681
1.05221617221832 -1.16993653774261
-0.646256625652313 -0.504010736942291
8.59377670288086 30
-2.81453323364258 0.0728324949741364
-1.36242437362671 0.0869163647294044
0.645513355731964 -0.660999655723572
7.54595375061035 30
-3.02627325057983 -0.234249323606491
-1.67153036594391 -0.0421899408102036
-1.74120378494263 -0.439787805080414
4.71692991256714 16.1353893280029
-1.87126266956329 0.492497891187668
0.373385339975357 2.11642742156982
2.53757905960083 7.53413963317871
0.811671733856201 -0.329620093107224
-1.17810046672821 0.364351600408554
3.41585755348206 -4.459716796875
0.403428494930267 0.267512708902359
4.37710857391357 18.6763973236084
0.954115271568298 0.250078737735748
-2.09387302398682 0.405294597148895
-0.95952445268631 0.668095231056213
-0.228962242603302 -0.0615430288016796
-0.0374790281057358 0.408667683601379
-3.2207670211792 0.136471480131149
-0.12610799074173 -0.152071446180344
-2.78447103500366 -0.0274120941758156
-8.34328460693359 -0.0362169481813908
-1.55888509750366 0.548216938972473
2.4539258480072 0.256974458694458
0.123416006565094 -0.490282416343689
-2.87837100028992 0.112685106694698
3.74012804031372 3.07286190986633
-0.535512030124664 -0.240354225039482
-3.64481425285339 0.141758024692535
-3.37894153594971 0.0293458607047796
-1.55884337425232 0.572253465652466
-4.53907299041748 0.0443407818675041
-1.27562963962555 0.169914066791534
-2.18346285820007 -0.258859634399414
0.641831874847412 -0.0015878239646554
-0.0149539858102798 -0.0992274731397629
1.53799819946289 0.924479186534882
3.20725250244141 8.98987102508545
-3.90082621574402 0.00519606471061707
-8.80334186553955 0.00171159172896296
3.1607940196991 2.49805021286011
2.73353981971741 -2.30922865867615
-4.83172607421875 -0.0336603112518787
4.38857316970825 -5.70453023910522
0.241091340780258 -0.612433433532715
-4.21121501922607 -0.0946479365229607
-3.06908702850342 -0.0829691886901855
1.76140427589417 1.88356602191925
0.0155938304960728 1.33705055713654
2.28850841522217 1.88139796257019
-0.09077188372612 -0.160099282860756
-0.653301119804382 0.63429468870163
0.56942081451416 1.97137999534607
-7.76467800140381 0.0205230452120304
-2.34535551071167 0.103584855794907
-0.447050631046295 -0.921488463878632
-3.64617323875427 -0.180086851119995
-5.08980703353882 -0.0384405218064785
0.117362141609192 0.481977730989456
-2.58465456962585 -0.257415384054184
1.62317001819611 0.935620963573456
0.798446893692017 1.56642544269562
1.5737179517746 -3.44689631462097
4.49232625961304 4.91377210617065
-4.79545068740845 -0.0756892114877701
8.40532112121582 30
1.73467588424683 0.858779966831207
2.61206984519958 -1.27854335308075
-4.4094672203064 -0.0852546095848083
0.801881670951843 -1.84192681312561
-4.55878114700317 -0.0320693999528885
-2.64769077301025 -0.477385550737381
-7.3302903175354 -0.038185078650713
-2.96339845657349 0.218295693397522
-2.09537744522095 0.166598722338676
-0.04802405834198 -0.406557530164719
3.79820513725281 -4.2620210647583
6.55645561218262 -28.9842681884766
1.33289313316345 -1.52519917488098
-2.37492895126343 -0.442336410284042
-1.39573335647583 0.270442068576813
-1.69294440746307 -0.252587825059891
5.89755868911743 6.01188993453979
0.439708262681961 0.344151169061661
-0.6836918592453 0.948498249053955
-3.56795644760132 -0.0476695373654366
-2.65962243080139 -0.042848140001297
6.23934602737427 -4.15438985824585
-2.68960475921631 -0.280612677335739
-2.43360495567322 -0.109532877802849
1.01214778423309 0.777535796165466
2.06100225448608 1.76199114322662
};


==> figures/visualizations/funnel/gt_samples.tex <==
\addplot [draw=red, fill=red, mark=x, mark size=3, opacity=0.5]
table{%
x  y
4.21579647064209 13.0401983261108
-0.724560737609863 -1.04279375076294
4.46266651153564 0.887613832950592
4.25742483139038 -1.68010854721069
-1.36634075641632 -0.505505263805389
-0.243616670370102 -1.0844202041626
4.68987512588501 -11.6507616043091
-2.29664206504822 0.170774966478348
3.99973964691162 -0.316058486700058
2.30520629882812 -4.80420637130737
1.52782952785492 0.888938724994659
1.68535280227661 -2.1472692489624
-1.49677515029907 0.232198521494865
4.13348388671875 -0.715278446674347
-0.32040748000145 0.453363418579102
2.25086855888367 5.24600219726562
3.70039224624634 4.66236639022827
3.39515686035156 -13.0227718353271
-0.532911598682404 -0.328217655420303
-2.90227746963501 0.139089837670326
1.28063058853149 -1.14943242073059
6.64327335357666 -16.9680805206299
-2.7258734703064 -0.228360190987587
2.51805114746094 -2.25203895568848
-0.108969002962112 -0.0423554331064224
-2.07682991027832 0.315516978502274
-4.28767538070679 -0.168200075626373
4.21579647064209 13.0401983261108
-1.73505842685699 -0.0254475772380829
2.71044397354126 -5.17835569381714
6.47292518615723 -3.27375149726868
3.94655442237854 5.99253988265991
-3.58450078964233 0.139293849468231
0.103410713374615 -1.14075326919556
5.47602462768555 6.32907342910767
-4.81892585754395 -0.0773270577192307
3.99973964691162 -0.316058486700058
-2.90227746963501 0.139089837670326
-4.97099637985229 0.105389520525932
1.98809218406677 3.27123808860779
-1.75995802879333 0.503219604492188
4.638503074646 -2.12086844444275
2.71044397354126 -5.17835569381714
4.13348388671875 -0.715278446674347
-4.80634498596191 -0.0354718901216984
0.978306651115417 0.963323414325714
1.16129493713379 -1.89839720726013
-4.78192377090454 0.178990989923477
-1.27255713939667 -0.178541854023933
-1.12557709217072 -0.301618576049805
-1.06835198402405 0.0864693224430084
-3.76725816726685 -0.174817100167274
-2.44335460662842 0.0508918315172195
3.20833873748779 2.2506206035614
-0.454359591007233 1.05217564105988
0.974479556083679 2.64197397232056
3.73489856719971 0.607548415660858
0.792280316352844 2.21278119087219
-0.532911598682404 -0.328217655420303
-5.49270677566528 -0.055444560945034
3.09704828262329 -4.04108190536499
-0.983257591724396 -0.52081435918808
-0.764086246490479 -0.111030839383602
1.25469374656677 0.9087273478508
-1.28227996826172 -0.429578691720963
-0.171741187572479 -0.11963976919651
3.22834873199463 -0.0324504263699055
0.703173756599426 -1.1216516494751
2.48760890960693 -1.53341782093048
2.5228533744812 4.11706447601318
-5.955726146698 0.0978508368134499
1.3130909204483 0.506673514842987
-1.43456602096558 -0.335603594779968
0.88945609331131 0.0269786324352026
3.72817945480347 -4.82991456985474
-2.06450009346008 -0.196017310023308
2.5228533744812 4.11706447601318
0.299231618642807 -2.44684171676636
-5.955726146698 0.0978508368134499
3.5971040725708 0.120423018932343
-3.28436088562012 0.201638519763947
-4.52827644348145 -0.0766643956303596
1.9205664396286 0.271769732236862
4.4903450012207 4.80953645706177
-2.10626244544983 -0.369075983762741
0.974479556083679 2.64197397232056
0.563997805118561 0.523704349994659
-6.01852655410767 0.0277892779558897
-2.5789999961853 -0.178958147764206
7.83485794067383 -30
-1.45209407806396 -0.110316269099712
0.563997805118561 0.523704349994659
-0.108969002962112 -0.0423554331064224
-0.0448628924787045 -0.489235728979111
1.16129493713379 -1.89839720726013
-1.37762296199799 -0.413537919521332
-2.75337982177734 -0.306492537260056
3.94655442237854 5.99253988265991
4.61474561691284 12.1431865692139
3.76681756973267 -13.6286382675171
1.43284809589386 -3.62494850158691
0.671877324581146 -0.326901644468307
0.297548770904541 -0.105311773717403
-1.06960535049438 0.562589704990387
-0.548940300941467 0.506373941898346
1.9205664396286 0.271769732236862
1.96635639667511 2.51011896133423
-2.94433283805847 -0.0773886069655418
1.98809218406677 3.27123808860779
0.671877324581146 -0.326901644468307
0.658028304576874 -0.873378157615662
4.61474561691284 12.1431865692139
0.829277515411377 -0.535600423812866
-3.48004245758057 -0.126925125718117
-2.5789999961853 -0.178958147764206
4.25742483139038 -1.68010854721069
-4.58389568328857 -0.0410890020430088
-4.81892585754395 -0.0773270577192307
-0.493629693984985 -1.57511079311371
-0.372926890850067 -0.0957531854510307
-1.27255713939667 -0.178541854023933
2.60556697845459 2.37644791603088
0.829277515411377 -0.535600423812866
5.30822801589966 11.7469844818115
3.72817945480347 -4.82991456985474
0.341557800769806 0.382521122694016
0.792280316352844 2.21278119087219
-1.37386775016785 -0.504270315170288
2.55198907852173 4.13015556335449
-5.5916576385498 -0.0496327020227909
4.638503074646 -2.12086844444275
4.60954666137695 8.23816871643066
-3.09032440185547 0.0772528350353241
5.47602462768555 6.32907342910767
-0.773026406764984 -0.305904448032379
-2.23509001731873 0.0044785444624722
-3.14692115783691 -0.0626349300146103
-1.06978690624237 -0.238626182079315
-3.58450078964233 0.139293849468231
-0.454359591007233 1.05217564105988
-1.06960535049438 0.562589704990387
3.39484405517578 -1.47180247306824
2.21308398246765 -2.353839635849
-7.50819253921509 -0.0451909117400646
3.39484405517578 -1.47180247306824
-1.37762296199799 -0.413537919521332
-0.930631577968597 0.137795865535736
3.09704828262329 -4.04108190536499
2.33587884902954 0.19071501493454
-2.0035297870636 0.283347517251968
0.176985710859299 -0.789522647857666
-4.44076776504517 0.0978821218013763
5.15700721740723 -5.92321825027466
4.59893083572388 3.6631875038147
-1.05076825618744 0.579788744449615
-3.19336032867432 0.253227829933167
5.47602462768555 6.32907342910767
2.51805114746094 -2.25203895568848
-1.28227996826172 -0.429578691720963
-4.78192377090454 0.178990989923477
4.24092102050781 2.2727267742157
-2.57115602493286 0.132166892290115
-1.2894092798233 -0.658928215503693
-0.90313446521759 -0.0909571573138237
0.88945609331131 0.0269786324352026
1.17212080955505 -1.49177539348602
0.73319947719574 0.213009595870972
-3.43296074867249 -0.0480761379003525
3.48357009887695 6.44677591323853
-4.81892585754395 -0.0773270577192307
5.49995470046997 -9.74271678924561
0.962197959423065 0.264603972434998
-5.0534086227417 -0.0226232577115297
1.68535280227661 -2.1472692489624
-0.454359591007233 1.05217564105988
3.77108001708984 -4.26216697692871
-1.50185441970825 -0.580154955387115
4.638503074646 -2.12086844444275
4.70445108413696 -10.0938558578491
-1.06960535049438 0.562589704990387
4.29431343078613 10.7376356124878
3.95892119407654 -0.212842911481857
-1.49677515029907 0.232198521494865
4.70445108413696 -10.0938558578491
-2.76444387435913 0.182089596986771
-1.06960535049438 0.562589704990387
-0.210569724440575 -1.21234977245331
0.103410713374615 -1.14075326919556
-5.44822406768799 -0.00317747122608125
7.83485794067383 -30
-1.86249911785126 0.11442656069994
-1.75995802879333 0.503219604492188
-2.44335460662842 0.0508918315172195
-1.06960535049438 0.562589704990387
0.671877324581146 -0.326901644468307
3.88584184646606 -6.37120532989502
-1.00395011901855 -0.259714007377625
1.7487291097641 -3.05248093605042
4.25742483139038 -1.68010854721069
-0.724560737609863 -1.04279375076294
0.829277515411377 -0.535600423812866
-4.80634498596191 -0.0354718901216984
-1.52947962284088 0.30043625831604
4.49595022201538 10.7048892974854
-0.956662058830261 0.848761320114136
-0.967084586620331 -0.201608419418335
-2.27890467643738 0.0636680424213409
-1.98979890346527 0.464213997125626
-1.36634075641632 -0.505505263805389
-1.52947962284088 0.30043625831604
2.25086855888367 5.24600219726562
2.30520629882812 -4.80420637130737
-5.74251222610474 0.06560018658638
3.48357009887695 6.44677591323853
-0.650388062000275 -0.331962496042252
7.37156105041504 -30
-4.29217290878296 -0.0597222335636616
0.108930870890617 -0.662217915058136
3.48357009887695 6.44677591323853
0.108930870890617 -0.662217915058136
-4.41720104217529 0.123535439372063
0.974479556083679 2.64197397232056
-0.956662058830261 0.848761320114136
-1.41702973842621 -0.65802401304245
-5.64675903320312 -0.0481567159295082
-0.372926890850067 -0.0957531854510307
-1.37386775016785 -0.504270315170288
-2.33635425567627 0.324826329946518
0.767479181289673 -0.89514696598053
0.671877324581146 -0.326901644468307
-0.372926890850067 -0.0957531854510307
2.93721866607666 1.04370927810669
0.563997805118561 0.523704349994659
-0.984438121318817 -0.680793523788452
-0.773026406764984 -0.305904448032379
-1.45209407806396 -0.110316269099712
3.88584184646606 -6.37120532989502
-3.84437894821167 0.116523258388042
-2.843829870224 0.0396817326545715
1.96635639667511 2.51011896133423
-4.29217290878296 -0.0597222335636616
3.94655442237854 5.99253988265991
-3.82392978668213 -0.0094161182641983
-2.90227746963501 0.139089837670326
-4.28767538070679 -0.168200075626373
-1.32005500793457 0.0975430607795715
-2.20027565956116 0.258385181427002
3.4191906452179 6.25448560714722
-1.97855043411255 -0.205120861530304
0.011351871304214 0.966729164123535
1.77357065677643 1.01545882225037
-0.586202204227448 -0.189690172672272
-2.07165551185608 0.0988775491714478
-2.83039236068726 0.222098171710968
-1.98979890346527 0.464213997125626
-2.12707376480103 -0.0889774933457375
-3.65466451644897 0.075229287147522
4.638503074646 -2.12086844444275
-0.994120180606842 -0.710514008998871
-2.06450009346008 -0.196017310023308
4.25742483139038 -1.68010854721069
3.5971040725708 0.120423018932343
-1.49677515029907 0.232198521494865
-0.909914612770081 1.35930418968201
-5.74251222610474 0.06560018658638
2.41515469551086 -1.33797895908356
-5.74251222610474 0.06560018658638
-2.94433283805847 -0.0773886069655418
-1.00395011901855 -0.259714007377625
-1.80504441261292 0.399160474538803
4.59893083572388 3.6631875038147
3.76681756973267 -13.6286382675171
-0.493629693984985 -1.57511079311371
-0.372926890850067 -0.0957531854510307
-1.98979890346527 0.464213997125626
0.28079280257225 -1.20521640777588
-0.548940300941467 0.506373941898346
-2.57115602493286 0.132166892290115
0.103410713374615 -1.14075326919556
-5.53476333618164 -0.0871203765273094
-1.06960535049438 0.562589704990387
-4.01467943191528 0.385116845369339
1.21353316307068 3.61678242683411
0.563997805118561 0.523704349994659
4.46266651153564 0.887613832950592
-1.23906207084656 0.410196781158447
2.71044397354126 -5.17835569381714
2.51805114746094 -2.25203895568848
-5.955726146698 0.0978508368134499
-2.7258734703064 -0.228360190987587
-0.984438121318817 -0.680793523788452
1.57143139839172 -4.19039583206177
1.29115319252014 -0.168404370546341
-8.64988231658936 -0.0152275199070573
-2.6009783744812 -0.401807844638824
-1.06960535049438 0.562589704990387
-4.80634498596191 -0.0354718901216984
2.48760890960693 -1.53341782093048
-3.9682924747467 0.0183633826673031
-3.09032440185547 0.0772528350353241
};


==> figures/visualizations/funnel/ldvi_samples.tex <==
\addplot [semithick, ldvi, opacity=0.7, mark=x, mark size=3, mark options={solid}, only marks]
table {%
0.321329385042191 0.611365079879761
-1.81011962890625 0.360499024391174
-1.53907263278961 -0.558936476707458
0.971223950386047 -1.51674258708954
-1.29309403896332 -0.684349358081818
-1.04815328121185 0.414765119552612
0.860160529613495 -1.23768079280853
1.8844290971756 1.08321499824524
-2.94911241531372 0.156106293201447
-0.544813334941864 0.535808622837067
-0.46791684627533 -0.773904323577881
-0.30395320057869 -0.134456962347031
-0.0881735682487488 -0.536425471305847
0.678066372871399 0.0742383599281311
-0.311731785535812 -0.671447455883026
-2.74343609809875 -0.476400256156921
2.48063397407532 0.89707088470459
-0.448835223913193 -1.00888526439667
1.67660510540009 2.9798002243042
-2.48203206062317 -0.119628965854645
0.583009004592896 -1.32009410858154
-3.77917432785034 -0.0123506411910057
1.26745939254761 3.53935861587524
1.80262851715088 5.57366704940796
-0.314846873283386 0.00809149816632271
-0.211139261722565 -0.286245971918106
0.257908403873444 -0.528846979141235
-0.523153841495514 -0.142805069684982
-1.58565151691437 0.154307290911674
-1.07359099388123 -0.0175309740006924
0.882790803909302 0.145724415779114
-0.768044531345367 -0.262728869915009
-2.64858174324036 0.0529146939516068
-0.523221433162689 -0.431544780731201
-3.76724123954773 -0.154173046350479
0.411293864250183 -0.581931471824646
-1.1689430475235 0.0468940436840057
-0.323780298233032 0.909525573253632
-0.0889491066336632 -0.0159513652324677
-0.608763098716736 0.0933418273925781
1.0313628911972 -1.89290392398834
0.144927859306335 -0.864467263221741
-0.134139031171799 0.852203786373138
-2.36849117279053 -0.692454814910889
1.1748274564743 0.103702582418919
0.236981108784676 0.487915396690369
0.428855150938034 -0.315053254365921
-0.526895999908447 0.341055452823639
-2.09551978111267 0.3446264564991
0.759153544902802 -0.216019421815872
-0.142756059765816 1.06068301200867
-0.252207040786743 1.23755872249603
-3.45830416679382 0.14192821085453
1.36288273334503 0.97750848531723
-2.0609655380249 -0.371762782335281
-0.27994692325592 -1.039999127388
-0.682444989681244 -0.711219906806946
0.521636128425598 0.192997246980667
-0.390274465084076 1.10695457458496
-0.200448900461197 1.57061588764191
-1.65471935272217 0.166511923074722
-0.290752083063126 0.645009398460388
-0.326182216405869 0.703636229038239
1.29067599773407 3.16869640350342
1.48525810241699 1.53842902183533
2.92406797409058 1.26432693004608
-0.314739555120468 -1.46666443347931
-0.30438905954361 1.05638754367828
1.74991500377655 0.305372059345245
-0.493539601564407 -1.09431791305542
-1.06104183197021 -0.692835569381714
-0.861508965492249 -0.35379883646965
-0.589261114597321 -0.121495589613914
0.973948240280151 1.12652969360352
0.441317468881607 0.130038693547249
0.584676682949066 -1.52269113063812
-0.695361137390137 -0.889516770839691
0.773618400096893 0.408223062753677
0.0344851613044739 0.538415133953094
1.06025838851929 -0.622292816638947
-3.46476173400879 0.0314285010099411
0.441920667886734 -0.405063599348068
0.0263151526451111 2.05957078933716
0.540136516094208 2.23102521896362
-2.61024856567383 -0.204421684145927
-0.199791327118874 1.47310090065002
1.31779193878174 -2.00720572471619
1.94482982158661 -1.22173976898193
0.0355841889977455 -1.0126177072525
-0.093090683221817 1.51222479343414
-2.82613015174866 0.0628286302089691
-3.48851442337036 -0.413841366767883
-0.0497610792517662 -0.331627577543259
-1.96872437000275 0.0528416484594345
-2.33259725570679 0.0875786393880844
0.808707714080811 -0.309949398040771
-2.27970433235168 -0.776796996593475
1.69856441020966 -3.4235246181488
-0.787957370281219 -0.603285133838654
-2.58627843856812 -0.167415499687195
-1.59130930900574 0.221267983317375
2.44988489151001 1.07497203350067
1.05820989608765 0.825078427791595
0.558331668376923 -0.0969212129712105
-1.9589809179306 -0.225620463490486
-2.34603142738342 0.644117414951324
-0.534026861190796 -1.23184549808502
0.347807973623276 -1.08885502815247
0.151754558086395 -2.68873500823975
-0.427210241556168 -0.714037120342255
1.50127935409546 -1.66796493530273
0.319664299488068 -1.25515413284302
-0.33804714679718 -0.167497709393501
-1.15490984916687 1.13562977313995
-4.2958869934082 -0.0194290839135647
-1.43794214725494 -0.0660677999258041
-1.13355183601379 0.0637028515338898
0.0412361770868301 0.704323828220367
-1.57800006866455 -0.632837295532227
-0.279734939336777 1.19974565505981
0.260572224855423 0.309114664793015
1.35397887229919 0.820704758167267
-3.7366681098938 -0.107249066233635
-2.66731834411621 0.0327747911214828
-2.54549479484558 -0.233841896057129
-1.43415749073029 0.161859512329102
-0.464984893798828 0.115962505340576
-0.550057649612427 0.499455392360687
1.2035197019577 1.3204118013382
1.83697402477264 -2.012362241745
-0.471338123083115 -1.11773312091827
1.60294222831726 1.35953795909882
-2.51820492744446 -0.13067464530468
-1.42561757564545 0.755834817886353
0.51764190196991 -0.659246265888214
1.26628541946411 0.892105221748352
1.56026554107666 -0.16815410554409
-0.874260485172272 -1.06982898712158
0.667750835418701 -0.645402431488037
0.59541928768158 1.24879109859467
-3.60950946807861 0.0439039617776871
-0.00407908111810684 0.389793545007706
1.52798175811768 0.855061888694763
2.33367109298706 -2.29445219039917
-0.51472932100296 -1.00448131561279
0.924923837184906 -1.24144876003265
-3.76321887969971 -0.123094283044338
0.334212332963943 -1.34940958023071
-0.647159159183502 0.850848197937012
0.719322741031647 2.46919250488281
-4.65076780319214 0.0645803436636925
-0.77874082326889 0.621615707874298
-1.53780651092529 0.423384726047516
0.7285236120224 1.17731642723083
1.19844806194305 1.24918138980865
2.44181060791016 -1.50384938716888
0.724009394645691 -1.95124006271362
-1.18854486942291 1.03360033035278
1.57290482521057 -2.37603640556335
-0.279312372207642 1.81518137454987
-2.99487805366516 -0.0586100779473782
0.340343296527863 -1.01164436340332
2.01368808746338 -0.686196208000183
0.554668605327606 1.42841875553131
-0.142261236906052 -0.176617532968521
-2.01744651794434 0.236640334129333
2.83266878128052 -4.66642045974731
-2.28788590431213 -0.378906935453415
2.46396207809448 -0.0100871026515961
2.10097241401672 2.34742951393127
1.10428237915039 -0.420473039150238
-0.634787976741791 -0.301951110363007
1.9645881652832 0.866249620914459
1.93386352062225 1.68531823158264
0.132335677742958 -0.968345284461975
2.23986983299255 1.27209150791168
0.757982432842255 -0.669080495834351
2.22689509391785 -1.74917232990265
-0.138065755367279 -0.489884674549103
-0.307305634021759 0.100894212722778
-1.03586518764496 -0.190673142671585
-1.18488156795502 -0.661497473716736
-0.0517131090164185 -0.45833495259285
0.533483624458313 1.37429332733154
-0.540456116199493 -0.502192616462708
-2.8870325088501 0.294463932514191
-2.76101756095886 0.147731140255928
-3.63632726669312 -0.123634085059166
-0.365721732378006 -0.698818683624268
-1.38003575801849 -1.27888607978821
-1.44047248363495 -0.597290515899658
1.13752138614655 -1.83306038379669
-0.786045491695404 0.802154362201691
-0.690941393375397 -0.800840973854065
-2.60729575157166 -0.114467456936836
-0.508605420589447 -0.445003658533096
-0.361098617315292 -0.157206326723099
-0.567409873008728 0.71649968624115
0.363504707813263 -0.411914139986038
0.748992443084717 -0.21326918900013
-1.44866633415222 0.0707587003707886
1.00918865203857 -1.61680114269257
-2.69151949882507 0.126886516809464
1.58972036838531 -1.72931706905365
2.0212197303772 -1.12421536445618
-4.25831270217896 0.0513097941875458
-1.08698129653931 -0.41869068145752
-0.0376346409320831 0.970840752124786
-0.331180840730667 0.370699614286423
0.0367582812905312 0.0990801155567169
0.320970892906189 -0.81849193572998
1.16246962547302 0.597005903720856
-0.827640652656555 -0.354658514261246
0.756220042705536 -0.358768969774246
-2.90857696533203 -0.0434361882507801
0.440493166446686 -0.0369918681681156
-0.611440122127533 1.03180336952209
0.0889323949813843 -1.74681341648102
0.0167241245508194 0.711065411567688
-0.837619006633759 -0.309296667575836
0.0210492499172688 0.372701168060303
0.797592282295227 0.813433289527893
-0.409545242786407 0.169764131307602
0.751481354236603 -0.170943275094032
-0.358502119779587 0.79914253950119
-0.624706864356995 0.4663345515728
2.12825584411621 -1.4346410036087
-0.18687492609024 1.13260185718536
-1.41381931304932 -0.123376801609993
2.00424098968506 4.74634742736816
0.853798151016235 1.06876492500305
-0.52900904417038 0.539319574832916
0.327269613742828 0.685331225395203
-1.32343280315399 0.904826998710632
-2.62280511856079 0.211462140083313
-0.674910843372345 0.0794546157121658
1.53806066513062 4.59170198440552
-0.426216125488281 -0.122158005833626
0.155151560902596 0.356261521577835
1.85400307178497 1.79980754852295
-1.19813096523285 -0.0712162628769875
1.00287342071533 -0.885727405548096
2.17132139205933 3.78958606719971
-0.865191102027893 0.709974229335785
-2.14197421073914 -0.170808643102646
-2.82119131088257 -0.174685299396515
1.35993564128876 0.922150313854218
1.17238664627075 2.08339953422546
-1.0236599445343 0.368869364261627
-3.30254745483398 -0.0463042259216309
-0.958001315593719 0.661075949668884
0.538853645324707 -0.543656349182129
1.64751100540161 -0.0555712394416332
2.63573718070984 -4.81128454208374
2.13601350784302 1.47754287719727
2.4287633895874 0.538547575473785
0.48150047659874 0.177958384156227
1.40693068504333 5.03162574768066
-1.36769223213196 0.231714904308319
2.16513013839722 -3.75455117225647
1.29631388187408 0.615853905677795
-0.621047973632812 -0.0377858951687813
-0.866141736507416 0.552304804325104
0.819720149040222 1.72226738929749
-1.03588569164276 -0.554677605628967
1.24340295791626 0.192613020539284
-0.352907598018646 -0.0904656052589417
2.69469499588013 -3.75429177284241
2.07518434524536 -1.20348751544952
-0.204737812280655 -0.517264366149902
-2.27005791664124 -0.026175357401371
-0.284919202327728 1.31137955188751
-1.36592602729797 -1.02598226070404
-2.56094145774841 -0.354722559452057
-3.62489533424377 -0.0351241677999496
0.00153054110705853 0.610208451747894
-0.0938538461923599 -0.664687991142273
-0.827232360839844 0.283084988594055
1.18712508678436 -2.4883291721344
-0.0312862992286682 0.734065473079681
-0.377186596393585 0.644103825092316
-1.1789288520813 -1.48202669620514
3.00511407852173 -4.53833484649658
-0.745244741439819 0.182448267936707
-0.56243771314621 -0.352699130773544
0.504316568374634 -1.71717429161072
-0.827932238578796 -0.764110922813416
4.05084753036499 5.36076354980469
1.42871129512787 -0.29526150226593
-2.09065103530884 -0.105408765375614
-0.0174528788775206 0.178157597780228
-0.79827755689621 0.2409927546978
0.256830632686615 -0.110886618494987
0.278230905532837 -1.16494810581207
-1.31399655342102 -0.666843235492706
-1.13546919822693 0.53800243139267
1.97356307506561 0.915322184562683
1.38651621341705 0.876163244247437
0.307475715875626 1.79968476295471
1.33240735530853 -1.70939648151398
-0.522838950157166 -1.23343312740326
-2.31051754951477 0.474951028823853
-0.048002801835537 0.113584950566292
-2.62009072303772 -0.0171199664473534
-0.785170018672943 1.69866466522217
0.80603152513504 -0.372621059417725
-1.1915922164917 -0.591634154319763
1.57203340530396 -2.47282838821411
-1.2893728017807 0.164617016911507
1.56987333297729 -1.08516108989716
0.391898572444916 -1.83692908287048
0.995490670204163 0.523055195808411
-2.30669784545898 -0.0822903215885162
0.452274084091187 1.1735600233078
-0.695537209510803 0.101545691490173
0.926792919635773 -3.27388048171997
-0.87591689825058 0.455839335918427
-2.60424780845642 -0.338632076978683
0.148100510239601 -0.894514203071594
2.81060433387756 2.37613344192505
-0.444973468780518 -0.0834339410066605
-1.14055263996124 -0.327309817075729
-2.56894826889038 -0.12001359462738
0.89983594417572 0.277857601642609
-2.09373831748962 -0.0186484009027481
1.60502922534943 -0.383082985877991
-0.166166409850121 0.0583024471998215
-2.8077175617218 -0.102781988680363
-1.10642206668854 -0.693308174610138
-1.45114624500275 -0.0917266756296158
0.820019721984863 -1.34879910945892
-3.00377821922302 -0.440622806549072
0.925716996192932 3.46245336532593
-0.967673659324646 0.173871472477913
1.4327232837677 -1.36590886116028
1.25461232662201 0.744205236434937
-0.459572404623032 0.931089758872986
0.413166463375092 0.373973250389099
2.06576466560364 2.02279448509216
0.282492458820343 -1.09811460971832
-2.26124954223633 -0.086535781621933
-3.48277950286865 0.131511002779007
1.34199380874634 2.19253325462341
1.35208666324615 1.2516028881073
-0.863651037216187 0.788628101348877
-2.22748136520386 0.282862603664398
-0.114951938390732 -0.155688047409058
1.41158652305603 1.70531439781189
-0.130559027194977 -0.478148460388184
-0.790834307670593 -0.297134876251221
0.694810450077057 -0.501648604869843
0.543154716491699 0.262554258108139
0.586136877536774 0.44125160574913
0.32029002904892 0.605709314346313
-1.15936398506165 0.330574929714203
-0.578670144081116 1.02900671958923
-3.04868483543396 -0.0892633199691772
-1.3578577041626 -0.243843346834183
-1.1679652929306 0.392144739627838
0.386224031448364 -0.34479558467865
-0.638374924659729 -0.303953170776367
0.989910125732422 -1.80844414234161
-0.751130342483521 -0.843005836009979
-0.586099922657013 -0.149459481239319
-0.704854786396027 -0.951241850852966
-0.638020038604736 -0.658127844333649
-0.735692203044891 0.631658852100372
-0.828315615653992 1.84552478790283
-1.16863059997559 -0.283080220222473
1.65487909317017 0.614303648471832
1.26653480529785 -0.0612813606858253
-0.550784051418304 0.134255230426788
-0.694712400436401 -1.15114867687225
0.24819777905941 0.828950822353363
0.781911015510559 -0.0496668592095375
-0.100553601980209 0.918960869312286
0.612804710865021 0.962452292442322
-0.550317764282227 0.500823497772217
1.67936050891876 1.16739249229431
-0.472634792327881 -0.801094591617584
-0.283859580755234 -0.252710610628128
-2.13832449913025 -0.21847315132618
-1.10399377346039 0.81399929523468
-0.846939563751221 -0.515554368495941
0.900338232517242 -1.82027077674866
-1.51214051246643 1.07701694965363
-1.25373220443726 -1.03435564041138
-0.0141347516328096 1.82708942890167
-1.16473615169525 -0.031798217445612
-1.2956759929657 0.561836421489716
0.696809947490692 0.902197480201721
-3.38881802558899 -0.0467898547649384
-1.59564328193665 0.0219094660133123
-1.33322322368622 -0.456491827964783
1.20822179317474 -1.70670425891876
0.231971755623817 1.53037524223328
2.22483253479004 2.9040584564209
0.979458212852478 0.0861792117357254
3.83025336265564 -4.5177435874939
1.69734585285187 -0.988618016242981
1.05605638027191 0.111568562686443
1.13105952739716 0.428029179573059
1.21068012714386 -1.22105014324188
-2.13387489318848 -0.590330719947815
-0.012987494468689 2.21908450126648
-1.39729177951813 0.399415105581284
-2.12506341934204 -0.310359060764313
-2.37962508201599 -0.366832196712494
-0.0302739255130291 1.8740611076355
0.932418167591095 -3.60789847373962
0.201060593128204 -0.302770525217056
1.03274440765381 -0.431445270776749
1.59822857379913 -1.51823925971985
0.83368194103241 0.355824947357178
-0.207412749528885 0.295117348432541
-2.1337673664093 -0.00368114560842514
1.85401856899261 -1.52512884140015
-1.6181606054306 0.00604713708162308
-1.14610540866852 0.299914658069611
0.348715841770172 -0.665143013000488
1.46974492073059 -3.56187295913696
-2.71501779556274 -0.0108163058757782
-0.864534795284271 0.334096610546112
-0.109457701444626 -0.562489032745361
-2.6121187210083 0.0849516838788986
0.698435366153717 0.96240621805191
-0.556186735630035 0.473408639431
-1.1197338104248 0.570739090442657
0.0281907897442579 -1.64505755901337
1.43361139297485 -0.289246499538422
1.85183024406433 -1.46996641159058
1.2200825214386 1.42837989330292
0.781071662902832 0.0278605446219444
0.987187445163727 0.510991632938385
-0.698153734207153 0.481561452150345
1.71344673633575 -5.66708755493164
-2.18669080734253 -0.115733437240124
-0.12932001054287 -0.420477211475372
1.46470952033997 2.73206305503845
1.32201075553894 -2.48807764053345
2.71310091018677 -1.72999083995819
-1.99833488464355 -0.273379147052765
-0.0515454560518265 0.372367829084396
-1.66318297386169 -0.312243789434433
-3.98330545425415 -0.117365978658199
-0.00445627421140671 -0.4963458776474
0.0381411835551262 -0.129120752215385
-2.17983746528625 -0.537764489650726
-1.98938548564911 -0.0686525478959084
-1.2243744134903 -0.218493685126305
2.59033536911011 6.69255208969116
0.854400634765625 3.3487286567688
1.58453798294067 0.815291345119476
0.592873454093933 -2.25981378555298
1.47962260246277 -0.390015870332718
-0.0457517206668854 0.393314838409424
0.803121984004974 2.0363495349884
-4.18457174301147 0.240687236189842
1.20138335227966 -0.265494287014008
1.38581728935242 -1.16679096221924
0.492187231779099 2.02607345581055
3.30360078811646 6.1806001663208
0.145409449934959 1.51983547210693
-0.59573757648468 -0.644016623497009
-1.78188860416412 0.229351103305817
0.758247137069702 -1.63285553455353
2.2821033000946 0.429113298654556
1.72788608074188 1.99331367015839
-1.81364226341248 -0.371156066656113
-1.20591449737549 -0.244503304362297
-1.42272102832794 0.644725620746613
-1.92725253105164 -0.305681049823761
0.776856482028961 -1.94841825962067
-0.438900649547577 -0.660738468170166
1.2435017824173 -1.46931898593903
-0.844914436340332 -0.148614704608917
0.758126080036163 -0.516296863555908
-1.74378991127014 0.195512890815735
0.245641142129898 1.26127147674561
2.15239834785461 3.52165198326111
0.533387899398804 0.658448934555054
0.214402332901955 1.70660030841827
1.36883163452148 -5.21032905578613
-2.74932909011841 0.262910813093185
0.0130980182439089 0.549018561840057
0.33089891076088 1.0374870300293
0.618065059185028 1.30212116241455
-1.45024251937866 -0.0544102862477303
2.68778014183044 -2.34420466423035
0.72723650932312 -2.4019250869751
-0.564699411392212 0.521996021270752
0.0367221236228943 0.234141975641251
-1.31368410587311 0.132488399744034
0.385188043117523 0.97922956943512
2.22661828994751 -0.263215065002441
-0.340374708175659 -0.511038184165955
2.37312150001526 -0.902541875839233
1.11417365074158 -2.32879829406738
0.965054988861084 1.0566908121109
0.740287005901337 -0.355302214622498
0.78932774066925 0.846194267272949
-2.89085745811462 -0.212246298789978
-2.16947078704834 0.700017154216766
1.12209713459015 1.77536725997925
-0.62188196182251 -0.152330383658409
-0.195811063051224 -0.54643702507019
-3.89151549339294 -0.353436470031738
0.760745286941528 -1.50900399684906
2.25811910629272 -2.96760320663452
1.20848143100739 2.67244124412537
-1.11116695404053 -0.161122217774391
0.0068242996931076 0.235449373722076
-0.675544381141663 0.76881617307663
0.655154585838318 0.156972765922546
1.72498035430908 -0.31187430024147
0.638273596763611 -1.20428836345673
0.352606296539307 -0.702281475067139
0.260979235172272 -0.0141674764454365
2.38313436508179 4.93104076385498
1.83655762672424 -2.05307245254517
0.258113384246826 1.28008425235748
-0.895944058895111 0.351737320423126
1.39300513267517 -0.054063655436039
1.48112308979034 2.29400205612183
1.19808220863342 0.0393449366092682
2.41461968421936 2.22423076629639
-2.18826937675476 0.318271577358246
2.30897903442383 -4.35197877883911
-0.57718563079834 0.963903725147247
0.821414053440094 1.26551640033722
-2.51547408103943 -0.195226758718491
0.710979819297791 -0.726864278316498
-0.736305117607117 0.500316441059113
2.07627511024475 1.34242975711823
0.426001995801926 2.80691456794739
-0.857703328132629 -0.291210055351257
-0.507269263267517 -0.582750976085663
-0.338733792304993 -0.432380348443985
-2.65377259254456 -0.173684924840927
-2.06919026374817 0.230461418628693
0.972739279270172 -1.32848298549652
-2.78719568252563 -0.187401697039604
1.17532861232758 -1.13643872737885
-0.713675856590271 -0.516520082950592
2.04991960525513 3.17999958992004
0.333329647779465 -0.935069561004639
1.04045796394348 -1.10444569587708
-0.0284772422164679 -0.793485343456268
-0.383926510810852 0.622460722923279
1.59223771095276 5.30385446548462
-1.31009840965271 -0.565064668655396
-0.520788729190826 -1.8058465719223
0.198275610804558 -2.14353322982788
1.38714110851288 0.256279587745667
-0.213270306587219 1.43846797943115
-1.2136322259903 -0.373813629150391
1.04679393768311 3.44115710258484
-1.19179654121399 0.434485137462616
-0.34247487783432 -0.548679351806641
1.01598823070526 -0.234337761998177
-0.759831726551056 -0.680343151092529
-2.85280299186707 -0.410216361284256
-0.358984231948853 -1.5400105714798
-0.871206641197205 -0.523172855377197
0.493828237056732 2.53982615470886
-0.91963517665863 -0.058850958943367
-1.87364757061005 0.655903577804565
0.403602808713913 -0.843655526638031
-0.212239816784859 -0.639302968978882
0.0944933444261551 -0.174639299511909
-0.304450839757919 1.34627068042755
-1.76678240299225 -0.30386546254158
-0.28691890835762 0.310951441526413
-3.21294713020325 0.113853260874748
-0.199699848890305 -0.184156522154808
1.64988100528717 0.953512489795685
-1.05413603782654 -0.447740316390991
-1.18007874488831 0.339826464653015
-1.21460449695587 0.791512310504913
-3.30451965332031 0.148425042629242
-1.53511202335358 0.24948026239872
1.14422428607941 -0.463417291641235
-1.33665215969086 1.31335306167603
0.785045444965363 0.342568278312683
1.3972635269165 -0.552978694438934
1.66340839862823 -2.51266932487488
-0.311227738857269 0.0707369670271873
0.905381321907043 3.84060168266296
-2.48265385627747 0.052198201417923
-3.85538840293884 0.00287077948451042
-2.45559883117676 -0.29331848025322
-0.0677784159779549 0.0470677651464939
-0.15648677945137 -0.180693343281746
-1.75847232341766 -0.921815812587738
2.23753261566162 1.0133763551712
1.54147553443909 -5.32326364517212
0.997798264026642 2.38457059860229
-1.43301784992218 -0.345653176307678
1.76006925106049 0.0624939426779747
0.50868147611618 -0.27685284614563
0.935219764709473 -0.811733722686768
-2.19086146354675 -0.180610880255699
1.31140530109406 -0.880552887916565
2.06224536895752 -0.483659863471985
3.36898469924927 0.98991459608078
-0.565159201622009 -0.396172761917114
-2.94884872436523 -0.197364524006844
-0.309381276369095 0.245699778199196
-2.25301718711853 -0.235456347465515
1.47474205493927 -0.290848344564438
2.00320148468018 -3.29780960083008
-0.150647401809692 -0.558021426200867
0.404885619878769 -0.676008701324463
2.52734756469727 -3.25231456756592
-0.0832711905241013 0.0102456845343113
-1.75820767879486 0.409726798534393
-0.641987860202789 -1.36072278022766
-1.5163322687149 0.412340879440308
1.77880692481995 2.35018730163574
0.414330273866653 1.43571722507477
-1.83105874061584 -0.699509024620056
-1.67302906513214 -0.27943542599678
0.812111735343933 -0.0254225879907608
-2.19862008094788 0.46720278263092
0.341681301593781 -0.825274705886841
-1.31522011756897 -0.0814772471785545
0.137971669435501 -1.80604147911072
1.3668646812439 -2.97406148910522
-2.08724594116211 0.508108139038086
1.33822202682495 3.06055068969727
0.408786058425903 -1.07495927810669
0.079234391450882 -0.894978582859039
1.12955784797668 -0.217941910028458
-1.9063549041748 0.349514901638031
1.70175492763519 1.18007946014404
-2.73750615119934 -0.234095975756645
1.53532230854034 -3.40082597732544
-5.17664813995361 0.0246787592768669
-3.34574556350708 0.0291738398373127
-0.106627076864243 0.756011307239532
1.05395221710205 -3.92745137214661
-3.51420855522156 -0.0315236523747444
-1.21560335159302 -0.204133659601212
0.197653338313103 0.796616971492767
-1.00772190093994 -0.624563992023468
-1.63335990905762 -0.0095228161662817
-0.471112251281738 0.178931713104248
-0.828397035598755 0.7972332239151
0.4131720662117 -0.30845445394516
0.857090830802917 -0.557535886764526
0.184432864189148 -2.0098283290863
1.90438687801361 1.36952924728394
0.101051673293114 -1.59268879890442
-1.66495633125305 -0.267396301031113
-2.05773687362671 -0.355204313993454
0.916480958461761 2.02180457115173
0.537650644779205 1.11684572696686
-0.695514619350433 0.288697361946106
-2.4918999671936 0.0328818038105965
1.58898258209229 -1.46101236343384
1.91824209690094 -3.71075916290283
-0.802192807197571 -0.920627951622009
-0.327401697635651 0.00750236585736275
-2.01797699928284 0.4923976957798
0.519288420677185 -0.117132514715195
0.125835373997688 1.45812094211578
1.03429806232452 -2.20200514793396
0.634159505367279 0.674201905727386
0.5108562707901 -1.21094846725464
0.76161926984787 -0.864502310752869
0.362959116697311 0.486591339111328
0.890395104885101 0.442024797201157
-1.97972702980042 -0.50578761100769
-0.459250092506409 1.17326951026917
1.32119333744049 0.221047580242157
-1.48641490936279 -0.45881399512291
0.406691253185272 -1.45906448364258
-1.68732631206512 0.808596670627594
1.86042821407318 -1.41747164726257
0.477623522281647 -3.13808035850525
1.22760140895844 -2.65894341468811
-0.629530847072601 0.044621467590332
0.111731290817261 0.636071741580963
-2.07816815376282 -0.311726540327072
-1.15700352191925 0.0390941090881824
1.31476998329163 -0.182886809110641
2.45576357841492 1.43105399608612
0.116276256740093 -0.704976260662079
1.48341453075409 -1.43882203102112
-1.70620000362396 0.361035466194153
-1.82814431190491 0.200804248452187
1.91367506980896 -0.248502880334854
1.4130185842514 0.635719656944275
-3.19230985641479 0.270867884159088
-0.995628952980042 0.973133683204651
-1.23165011405945 -0.546970427036285
-0.866926789283752 0.669587969779968
-1.36371982097626 -0.859736561775208
-1.49909579753876 -0.157872468233109
-0.177437961101532 -0.508686661720276
0.465090423822403 0.460039436817169
2.62864780426025 -0.200316429138184
-0.90690279006958 -0.0247811805456877
-2.89541935920715 0.531655609607697
1.27383673191071 -0.594109237194061
-1.52049827575684 0.183507651090622
-3.89552783966064 0.231195703148842
1.40907311439514 3.81180095672607
1.90354585647583 -2.62017703056335
-0.38750821352005 1.21545827388763
1.91131973266602 0.0558464229106903
0.280722558498383 -1.66705715656281
-0.195541128516197 -0.837051212787628
-2.40021085739136 0.105501569807529
1.40554010868073 0.879514932632446
-0.768317341804504 1.17190444469452
1.75681579113007 -0.615362107753754
1.30794036388397 0.207555323839188
-0.114746704697609 -0.162341445684433
-1.84848892688751 0.812777161598206
1.20522916316986 -2.84251022338867
0.375161290168762 -2.08141922950745
1.47028923034668 -0.773874044418335
2.348060131073 -2.40800666809082
1.89848911762238 -1.32999014854431
0.631522536277771 -1.01220500469208
0.455758541822433 1.33094906806946
-0.257105737924576 -0.384648084640503
1.13628327846527 0.0519869662821293
2.1288890838623 -3.77628946304321
-0.399214535951614 0.783695876598358
0.0723536014556885 0.0717577338218689
0.462612807750702 -0.160796239972115
-0.402471035718918 0.605645895004272
0.164871647953987 -0.76187402009964
1.75712633132935 0.0874494016170502
-0.566578388214111 -0.132600069046021
-0.906081438064575 0.723024010658264
-0.502955317497253 -0.695943176746368
0.366249978542328 1.19391703605652
-3.49118113517761 -0.227850645780563
-3.61600136756897 0.115568958222866
-3.58986186981201 -0.116170719265938
-0.583640515804291 -0.717617988586426
0.547279715538025 -1.0793319940567
1.29336869716644 0.406767994165421
2.15972256660461 2.25011110305786
3.38033938407898 1.03895878791809
1.06006550788879 -3.72381067276001
1.63776516914368 2.3108184337616
-1.58040332794189 -0.361055314540863
3.29800987243652 0.926536917686462
-0.081859327852726 1.07880580425262
-3.51667857170105 -0.104575484991074
0.395568132400513 -0.11860079318285
1.40878796577454 -0.770626306533813
-1.17503559589386 0.0882391929626465
0.23913311958313 -0.394595563411713
-3.94170331954956 0.240868985652924
2.05404591560364 -5.97695779800415
0.40262433886528 0.461670398712158
-1.01973795890808 0.419780164957047
-0.429747879505157 0.369616746902466
-0.717855453491211 0.167730525135994
-1.39115583896637 -0.365607917308807
1.05963921546936 -0.147379025816917
-2.72818231582642 0.215024396777153
1.41053104400635 -1.93020617961884
3.22762537002563 -3.88961434364319
-0.644370913505554 0.0805037766695023
-2.94251275062561 0.398991018533707
-0.704334080219269 0.540798187255859
1.66703701019287 1.77482652664185
2.21181440353394 1.87729966640472
-0.274323374032974 -0.229682505130768
1.3562468290329 -0.0933191031217575
-0.0423771142959595 -0.00664099492132664
-2.99143767356873 -0.242372468113899
-1.08430886268616 -0.243642359972
-2.73499608039856 0.174286469817162
2.87558460235596 2.97392010688782
-0.565413177013397 -0.0485703125596046
-0.550560534000397 -0.551186442375183
-2.0683958530426 -0.0774121880531311
0.994828879833221 -1.5235071182251
0.735274195671082 2.07931661605835
-0.422367930412292 1.34467935562134
0.0318026468157768 -1.23779904842377
0.757847428321838 1.72089791297913
2.42493343353271 3.54456615447998
-1.52736067771912 0.230317607522011
-1.18918871879578 -0.025943785905838
0.546314895153046 -2.33930945396423
-1.59807980060577 -0.350198656320572
-2.53702259063721 0.144228711724281
-2.40605497360229 -0.400679469108582
-0.43515819311142 -0.172610133886337
0.72772216796875 0.820416331291199
0.285795629024506 1.0090616941452
-0.419480115175247 -0.82037740945816
-0.645145237445831 -0.726025998592377
1.23214018344879 0.947432637214661
-0.958345353603363 0.136090993881226
-3.97554492950439 0.0126070901751518
-0.734071493148804 0.235224097967148
0.952024400234222 3.57825827598572
-0.559226155281067 0.0996217727661133
0.057451955974102 -0.669777393341064
0.0876786410808563 -1.11906588077545
-0.0460344552993774 -0.898714482784271
-1.19451653957367 0.620212972164154
1.37252986431122 -0.160514041781425
0.47009202837944 -2.59479713439941
-0.309824109077454 0.1852066218853
-0.183271378278732 -0.322768330574036
-0.746459245681763 0.372098952531815
0.233453214168549 -2.88290882110596
-1.15032684803009 -0.235912248492241
-0.534503221511841 1.05244374275208
-2.96192073822021 0.104734137654305
0.199587732553482 0.650837779045105
-0.697813034057617 -0.427198886871338
0.00496210204437375 1.2410079240799
2.43957471847534 -4.00950717926025
1.14437234401703 0.685889184474945
-0.216659039258957 0.417370736598969
-0.501776099205017 -0.394339084625244
-0.0310285314917564 -0.2308679074049
2.37570786476135 -9.23235511779785
-3.70903968811035 0.170254781842232
-0.416502296924591 -0.248249173164368
2.13156342506409 1.15055668354034
-1.39900493621826 -0.0452367067337036
-0.497704088687897 0.760708153247833
0.302480429410934 1.63874673843384
2.17482352256775 -0.430681169033051
-0.330684065818787 0.770957589149475
0.993407964706421 0.868905365467072
-3.15827322006226 -0.0401137545704842
0.272381216287613 1.23555445671082
1.56858050823212 -1.43664562702179
0.128228545188904 1.55813729763031
0.368173271417618 -0.700171291828156
0.137754797935486 -0.574195206165314
1.72784173488617 1.16188025474548
0.0886952728033066 -0.276258707046509
-0.314351171255112 0.174975797533989
0.973830580711365 -0.931291580200195
1.38062822818756 -0.0506672970950603
-1.16757190227509 -0.755372583866119
-0.550633311271667 0.0706856101751328
-2.34337210655212 -0.216408625245094
2.3121190071106 -2.36656308174133
1.78336179256439 1.85966992378235
1.18359041213989 -1.25224232673645
-1.58729910850525 0.248742774128914
2.52054953575134 -0.294768095016479
1.53408563137054 -4.13839244842529
0.490961968898773 2.27188611030579
2.4457950592041 -3.16185665130615
-0.435114026069641 -1.19411897659302
-0.0993941575288773 -0.366291582584381
0.420646280050278 -0.288679271936417
0.849302411079407 -1.54007959365845
-0.00752099417150021 -0.245036363601685
1.34358036518097 -3.0621075630188
-0.932999610900879 0.510292828083038
0.746567487716675 1.66228878498077
0.887935519218445 1.55092024803162
-2.15407276153564 0.300749897956848
-1.05113685131073 -0.12545719742775
1.1976215839386 -2.08763909339905
2.25679993629456 -2.16762161254883
-1.21719360351562 0.234386831521988
2.21652150154114 -2.84037065505981
-0.832868158817291 -0.0874138474464417
1.28519999980927 0.312370985746384
-2.69574046134949 0.350590318441391
1.43657302856445 -1.2787252664566
-1.6359623670578 -0.346777081489563
1.29197728633881 -1.59697306156158
1.71493291854858 -2.7006242275238
-1.46734845638275 0.0377732589840889
-2.54742980003357 0.115579545497894
-3.7385721206665 -0.0192509070038795
0.139052271842957 -0.868195116519928
0.907013177871704 -0.425463318824768
-0.366976499557495 -1.56843507289886
1.20031344890594 0.416461735963821
-1.93039131164551 0.406470984220505
0.480820268392563 0.945944845676422
-2.8648202419281 -0.493320226669312
0.285684376955032 2.6266622543335
-2.35654950141907 0.287841469049454
-0.27779483795166 -1.29072833061218
0.231190651655197 0.448350101709366
0.0713241472840309 0.679852604866028
-0.865547478199005 -1.4377875328064
1.22425973415375 -0.191019997000694
1.44466722011566 1.44703376293182
0.785528421401978 -1.9817727804184
1.21514570713043 -0.959935307502747
0.687625288963318 0.615269899368286
0.628228425979614 -1.49274671077728
0.141924262046814 -0.975611448287964
-0.634113073348999 0.328450232744217
1.19930768013 -1.855388879776
0.820254385471344 2.02939605712891
1.02468800544739 -1.82502496242523
0.282354384660721 1.6490398645401
1.834303855896 -0.544424295425415
-2.17076516151428 -0.683026432991028
0.770301282405853 0.50826758146286
2.23112225532532 -2.26262211799622
1.0346223115921 -1.87736821174622
-2.09133768081665 -0.377539664506912
-0.0139983501285315 0.079938530921936
-1.6424605846405 -0.418683171272278
-0.302322894334793 0.296192556619644
-0.345320463180542 -1.01308190822601
0.617641508579254 -0.674430906772614
3.21524214744568 2.41435647010803
1.12736558914185 -2.64996743202209
-0.937438488006592 -0.895052552223206
-0.864311516284943 -0.461309015750885
-1.63565695285797 -0.414237320423126
-0.967866957187653 -0.0685601681470871
1.34135115146637 -1.64011025428772
0.4817034304142 0.295207321643829
-2.68262100219727 -0.161874666810036
-0.389873087406158 0.908670961856842
-1.00684905052185 -0.150208935141563
-1.61155438423157 0.249996453523636
1.58919155597687 -0.354469060897827
-1.45156991481781 -0.353198438882828
-0.329935729503632 -0.31231951713562
0.540514469146729 -0.359977424144745
0.688541293144226 0.899308204650879
0.445223718881607 0.505105972290039
-0.874935150146484 0.442409932613373
0.426115453243256 -0.148150533437729
0.0635016262531281 -0.438631862401962
-0.133380740880966 -0.64352023601532
-1.14918291568756 0.653596580028534
0.455192863941193 1.72684419155121
0.187102526426315 1.80017650127411
0.841336011886597 0.805750012397766
1.95923745632172 2.5151481628418
0.38693231344223 -1.83883094787598
-2.79329919815063 0.0128608345985413
-2.24289965629578 0.122536867856979
-1.01189863681793 -1.66799581050873
0.668033599853516 -1.29815709590912
1.17396628856659 -0.21295228600502
0.448720335960388 0.000761345028877258
0.329893589019775 -1.24937224388123
-3.06049132347107 0.208348989486694
-1.88605952262878 0.961002826690674
-3.70820903778076 0.135993748903275
0.903910636901855 -0.792711198329926
-2.71781039237976 -0.125938892364502
-0.624902069568634 0.430535018444061
-0.211154878139496 -1.02501404285431
3.32774114608765 0.0713501200079918
0.0555969774723053 1.19765472412109
1.0139377117157 -0.704135656356812
1.07781994342804 -1.74745500087738
-0.522024989128113 -0.248090445995331
0.843191087245941 1.25739204883575
-1.91551208496094 -0.00824767351150513
0.427246630191803 0.127241134643555
1.1463668346405 1.24649691581726
-0.729088664054871 0.385790377855301
1.1268424987793 0.301819920539856
-0.657708764076233 0.561636090278625
-0.39660906791687 -0.966774761676788
0.174728244543076 0.167517781257629
-0.149029642343521 -2.03250479698181
-0.196622669696808 -0.185078904032707
2.74425530433655 -2.35192108154297
-0.435911446809769 0.242548063397408
0.071095883846283 1.93224859237671
-1.49768853187561 0.454432964324951
0.020514577627182 -0.271434813737869
-0.249828651547432 2.1098039150238
-1.47712254524231 0.323204457759857
0.866928696632385 -1.97663104534149
1.15164685249329 1.5582709312439
1.82557117938995 -0.728158950805664
-1.14492666721344 -0.327639698982239
-0.30517303943634 -0.501590132713318
1.71519708633423 -1.83659470081329
2.92153859138489 -1.97646570205688
-3.20272183418274 0.319926500320435
1.72909653186798 -1.16468703746796
1.849973320961 3.28006792068481
-0.0981066524982452 1.32136416435242
2.71466398239136 -2.38567590713501
1.83895492553711 2.77412748336792
-0.923563599586487 -0.757038116455078
};


==> figures/visualizations/funnel/mcd_samples.tex <==
\addplot [semithick, mcd, opacity=0.7, mark=x, mark size=3, mark options={solid}, only marks]
table {%
-0.149131670594215 0.0741682946681976
-0.601897180080414 1.3249454498291
-1.32761681079865 -0.302078455686569
-3.72349953651428 -0.111978448927402
-0.926945865154266 -0.151094764471054
-1.33433830738068 -0.181874752044678
-0.704169154167175 0.344500809907913
-2.48105549812317 -0.451597809791565
-1.95506227016449 0.189674228429794
-2.21495985984802 0.347923070192337
-0.928682923316956 0.109102040529251
-0.393611490726471 0.260342538356781
-1.69085800647736 -0.344312131404877
-2.5631148815155 0.29244601726532
-1.28779113292694 0.0573483183979988
0.659326612949371 0.654230117797852
0.967541098594666 1.399249792099
-0.0242568701505661 -0.539434254169464
-2.51743245124817 0.289904356002808
0.1500383913517 0.0286209918558598
0.225394308567047 -0.0860893279314041
-1.34371340274811 -0.521046876907349
-0.886989593505859 -0.417908132076263
-1.23256349563599 -0.346414476633072
-4.1053318977356 0.0390175729990005
0.0873461738228798 0.699570953845978
-1.87436008453369 -0.652469515800476
-0.8523108959198 -0.253511816263199
0.131258130073547 -0.180513128638268
-0.747066676616669 0.0141431167721748
-1.84544801712036 -0.277682721614838
0.358841478824615 0.683450698852539
-1.94655442237854 0.188922867178917
0.0817368403077126 -0.439564168453217
-1.71102750301361 0.264576494693756
-0.0308702681213617 -0.309064567089081
-1.22713041305542 -0.247173801064491
0.257852822542191 -0.19082273542881
-0.00151700899004936 -0.604917287826538
-2.10937404632568 -0.351854890584946
-0.493497788906097 -0.940997540950775
-0.0761529058218002 1.2845870256424
-0.300440192222595 0.726126670837402
-0.713493704795837 -0.641713440418243
0.495124101638794 -2.92192602157593
0.557328402996063 -1.54840362071991
-1.66589093208313 0.0367519706487656
-1.45058810710907 -0.329143226146698
-0.567424714565277 0.0458001494407654
-1.0368504524231 0.390763998031616
0.613039672374725 2.15397071838379
-2.633633852005 0.202338010072708
-0.968321144580841 -0.730060517787933
-0.226386472582817 -1.7096471786499
0.119727045297623 -0.950714409351349
-1.70617866516113 -0.242286413908005
0.0336426869034767 -0.167051434516907
0.284378260374069 -1.23422503471375
-1.29382026195526 -0.154921397566795
-0.252149552106857 0.804134130477905
-1.13433301448822 0.734100759029388
-2.05165386199951 -0.396203011274338
-1.26057958602905 0.708008587360382
-0.37318617105484 1.39523005485535
-1.78579139709473 0.77854722738266
0.150154680013657 0.866400361061096
0.20681419968605 0.654560923576355
-0.898809790611267 0.389852434396744
-1.48981380462646 -0.711721003055573
-0.51504647731781 -0.21573780477047
0.771235048770905 -0.350792765617371
-2.8351674079895 -0.0549733899533749
-3.07135438919067 -0.270987868309021
-2.0819776058197 0.0125442370772362
-0.0654394254088402 -2.00674080848694
-0.16166764497757 1.07390916347504
-0.506134331226349 -0.127388000488281
0.167269602417946 -0.289674788713455
-1.01861381530762 0.19770485162735
0.0938012227416039 -1.11128008365631
-0.0109815709292889 1.48359107971191
0.382403463125229 0.00660054385662079
-1.80000782012939 -0.115946441888809
-1.7375636100769 -0.623830616474152
-1.93747234344482 -0.976470708847046
-1.63329255580902 -0.0576233416795731
-3.46458005905151 -0.0640121251344681
-0.622383177280426 0.837196946144104
-0.87854278087616 0.409379184246063
-2.38538432121277 -0.170234203338623
-0.555678963661194 -1.49195826053619
-1.91934609413147 0.0843757465481758
-0.083084300160408 -1.70388984680176
1.07153010368347 -1.20599937438965
-1.19147884845734 0.0188106149435043
-3.03575778007507 0.310755431652069
1.23704719543457 1.4669497013092
-0.475956469774246 -0.832886159420013
-1.01482534408569 0.120881281793118
-0.198611795902252 0.15935093164444
0.256598472595215 -0.489754289388657
0.216131493449211 0.912941932678223
1.12599110603333 0.82397586107254
0.454800426959991 1.5309944152832
-4.26695871353149 -0.0201800614595413
-2.10605978965759 -0.000582113862037659
-1.52903532981873 0.0815985798835754
0.0940298065543175 -1.64730799198151
0.467255383729935 -0.516376733779907
0.0138661563396454 1.39966380596161
-1.51044344902039 0.644394516944885
-0.396557629108429 -0.901288092136383
-0.115140974521637 -2.72488808631897
-1.55733895301819 0.303389877080917
-1.74838578701019 -0.793970763683319
0.331245541572571 -0.151545912027359
-0.539666712284088 0.0297128856182098
-1.34993457794189 0.0857816189527512
-1.66198623180389 0.294135242700577
1.32757091522217 1.79229092597961
-1.17011415958405 -0.0356982126832008
1.00080215930939 0.752650797367096
0.213185057044029 -0.0794806182384491
0.381556212902069 0.70518171787262
-2.60361647605896 0.0402549877762794
-0.70699155330658 0.378836035728455
-1.93631851673126 -0.60490471124649
0.309534877538681 0.405356466770172
-0.958410382270813 1.39634954929352
-1.301682472229 0.403564810752869
-0.467445433139801 0.504240274429321
0.413062781095505 -2.16020750999451
-3.23486685752869 -0.0110705494880676
-0.192110255360603 1.64698612689972
-0.876241564750671 -0.128454506397247
-0.359586983919144 0.672753751277924
-3.85104417800903 -0.186247155070305
-0.48294597864151 0.627815842628479
-0.299562811851501 -0.872732758522034
0.782431364059448 2.9157772064209
-1.14544022083282 0.192031651735306
0.457898050546646 -1.22575616836548
0.452278017997742 -0.316825389862061
-0.704677045345306 1.09589099884033
-0.980589926242828 0.738727271556854
-0.906033575534821 -0.342351794242859
-1.90106165409088 0.112745381891727
-0.639041423797607 0.887088716030121
0.00135432183742523 -0.0542320013046265
0.667857050895691 -0.0272065103054047
-0.787304937839508 0.141645789146423
1.86053657531738 0.355876266956329
-1.55757355690002 -0.518132328987122
-1.74977934360504 0.0122308954596519
0.0156988799571991 -1.24323451519012
-2.02288103103638 0.041802916675806
-1.91258764266968 0.238002315163612
-1.41540932655334 -0.113170273602009
0.38509926199913 -1.07558846473694
-1.99686443805695 -0.200313359498978
-1.03901076316833 0.0764566734433174
-1.40090489387512 -0.907350182533264
-1.90908193588257 -0.987502217292786
0.44272643327713 1.15139150619507
0.204531908035278 -0.360189199447632
-1.02368330955505 0.117165818810463
-1.21743881702423 0.354191601276398
-0.546172738075256 -0.78976571559906
-0.945052564144135 -0.777103185653687
-3.78117179870605 -0.303211092948914
-2.27118849754333 -0.418950200080872
0.593508541584015 -0.328831315040588
-0.913317441940308 -0.113188527524471
-1.05108153820038 0.31808790564537
-2.78207516670227 -0.113331519067287
-0.210969567298889 1.36789512634277
-1.17444264888763 0.313653647899628
0.282797157764435 0.566922068595886
0.132362097501755 1.3839373588562
-1.57274222373962 -0.479990452528
-1.75254130363464 -0.0985146686434746
-0.812286198139191 0.0608649104833603
-0.660158514976501 -0.401190161705017
1.21131014823914 -0.771267831325531
-3.37825155258179 0.269298821687698
-3.1874794960022 0.209613010287285
-1.04463374614716 -0.941017627716064
0.710335314273834 -0.284763604402542
0.442936897277832 -0.40931499004364
0.382499039173126 0.332641422748566
-2.52387404441833 0.389914602041245
0.982146084308624 0.331531047821045
-0.49109148979187 0.890504896640778
-2.00426077842712 -0.56520801782608
-0.292096942663193 0.338640570640564
-2.36723041534424 0.132437407970428
-0.617517411708832 1.47789180278778
-1.80061209201813 0.505120575428009
-1.19764816761017 0.0952475368976593
-2.17881536483765 -0.326850712299347
-1.71599733829498 0.729978799819946
0.150512173771858 -0.081032320857048
0.42083016037941 1.2638258934021
0.298512011766434 0.230231776833534
-1.6612206697464 0.303426265716553
0.916549921035767 -3.21900725364685
-1.40201318264008 0.452474683523178
-2.42143154144287 -0.171014353632927
-0.424779951572418 0.0504086837172508
0.64128965139389 -0.902051031589508
-1.55986356735229 -0.137715846300125
0.0858886241912842 -1.01282954216003
-3.94861102104187 0.0620175898075104
-1.92996609210968 0.232318848371506
0.713913261890411 0.509039700031281
0.208361223340034 0.293923258781433
-4.37868499755859 0.0788115262985229
1.17973923683167 -0.666130483150482
0.720296859741211 -1.39867854118347
-1.24094998836517 0.412971585988998
-0.428678900003433 0.047647338360548
-0.75513482093811 -0.0522235371172428
-3.40962481498718 0.115605108439922
-2.39922976493835 -0.374499261379242
-0.701701760292053 0.978777289390564
-2.2595636844635 -0.202631145715714
-1.09901106357574 0.0820655301213264
-0.586488008499146 -0.629807770252228
-2.86784887313843 0.0580817833542824
1.10098528862 1.9079053401947
-2.40704274177551 -0.257768034934998
0.357588738203049 -0.865947961807251
0.320710122585297 0.016139842569828
-0.558475255966187 0.189754381775856
0.73061591386795 -1.5357973575592
-0.819448173046112 0.00123000144958496
-0.256927847862244 0.588830351829529
-1.80250144004822 -0.781916320323944
-0.351396918296814 -1.75665271282196
-0.32799619436264 -0.122152462601662
-1.16566669940948 -0.039931382983923
-1.62626659870148 0.592197358608246
0.0399852991104126 -1.44740188121796
-2.0748074054718 -0.100027784705162
-0.596542239189148 0.981779634952545
0.424842298030853 -0.753544330596924
-0.395213901996613 0.0728233754634857
0.592870056629181 -1.41832041740417
-3.65167570114136 0.16146445274353
-1.53440427780151 -0.434972822666168
-1.32332861423492 -1.08448219299316
-3.0911078453064 0.22985415160656
0.345821410417557 0.0782240852713585
-3.53483748435974 -0.0145671814680099
-2.02869129180908 -0.160039111971855
0.633709073066711 2.06887102127075
-0.175772562623024 0.199461549520493
1.92588901519775 0.743798732757568
-2.84536242485046 -0.171971410512924
-2.68935704231262 0.30972620844841
-3.86167597770691 0.0160476043820381
-0.277746617794037 0.399549454450607
2.04905557632446 -2.7967963218689
-3.1752073764801 0.211122170090675
1.11139631271362 0.115248702466488
0.0463127344846725 -0.0790185257792473
-3.01846694946289 -0.387643456459045
-1.2302143573761 -0.24119034409523
-1.01718103885651 0.653178334236145
-2.71462750434875 0.177043080329895
-0.447469532489777 -0.791622698307037
-2.68415451049805 0.100712180137634
-0.53725391626358 0.0410061813890934
-1.01372182369232 0.103116646409035
0.567802786827087 -1.79895663261414
-1.46918165683746 0.461325258016586
-0.996959030628204 -0.11302638053894
-1.7422022819519 0.154261365532875
-0.0158700793981552 0.194446623325348
0.452401131391525 -1.04802942276001
-0.983502626419067 0.0163749232888222
-0.723151743412018 -0.289833188056946
-1.93923044204712 -0.23437337577343
-0.130491226911545 0.417619824409485
1.20429134368896 -0.399105608463287
0.203647956252098 -1.23563063144684
-0.555552661418915 0.0297294855117798
-0.719334363937378 0.437734127044678
-1.37781202793121 -0.0487747192382812
0.42362767457962 -0.246213093400002
-2.78364229202271 0.152227491140366
-0.462994307279587 1.88610422611237
-2.68718981742859 -0.216859608888626
-1.74733936786652 0.139382511377335
0.112806901335716 0.837403953075409
-0.637768745422363 -0.520755290985107
0.0680704638361931 0.589183807373047
-0.810266137123108 0.846893429756165
-3.57638001441956 0.142668724060059
0.23860402405262 1.04957163333893
-1.42020213603973 0.260182619094849
0.479472100734711 1.29452979564667
-0.539337515830994 -1.46126544475555
0.376914441585541 2.01980113983154
-2.65609240531921 -0.279872238636017
-4.78925561904907 0.0455376692116261
0.858011364936829 -1.45748722553253
-1.19915699958801 -0.514322876930237
-0.0777719467878342 -0.105345338582993
-3.27153444290161 0.0610169060528278
0.407392799854279 1.30682384967804
-0.444944024085999 -0.336034446954727
0.0232300087809563 1.33304524421692
-2.35333824157715 0.0719567462801933
-0.698442280292511 -1.16976284980774
-0.52192747592926 1.49222016334534
-1.8824759721756 -0.0994376018643379
-0.408536732196808 -0.437024146318436
-0.0155439004302025 -0.903253674507141
-3.59729599952698 -0.183079019188881
-0.253904610872269 0.491799175739288
-1.38631534576416 0.642634630203247
-2.560795545578 -0.0139741003513336
-0.53686249256134 -0.576789915561676
-0.814245581626892 0.479573756456375
-2.62683892250061 -0.0680499374866486
0.0914105698466301 -0.0340801477432251
0.592506408691406 -2.19490504264832
0.0415694490075111 1.14374482631683
-0.00711836479604244 -1.36495006084442
-0.494006514549255 1.14576196670532
-0.718722522258759 -0.697497606277466
-0.0687885582447052 0.796590745449066
-0.557546257972717 0.049527034163475
0.236354634165764 -1.73955845832825
0.0717295408248901 -0.282320648431778
-1.01984846591949 1.04764604568481
-1.48567020893097 0.223679468035698
-1.23086071014404 -0.240718930959702
-1.22384524345398 0.327749967575073
-1.00801348686218 -1.43376290798187
-0.901009261608124 -0.0983438566327095
0.0230546407401562 -0.831293225288391
-0.0409510843455791 -0.42550927400589
-0.998103678226471 0.276295781135559
-2.00329852104187 -0.170880720019341
1.32801651954651 -1.18363857269287
-2.22790932655334 0.34438556432724
-0.487820863723755 -1.66638517379761
0.695672988891602 -1.09439826011658
-0.681663870811462 -0.142272457480431
-0.679299235343933 0.240751296281815
0.300009727478027 0.276732087135315
-0.499717324972153 -0.568589091300964
-2.03425979614258 -0.482751548290253
-0.356385469436646 -0.183378994464874
0.197705760598183 -0.224971920251846
0.937147915363312 -0.752972602844238
0.905827820301056 1.19446969032288
-1.25466310977936 0.342169642448425
-1.39335417747498 -0.737641572952271
1.08162140846252 -2.40305399894714
0.495174556970596 0.802401185035706
-3.96165752410889 0.0378594100475311
-1.54942572116852 -0.0389605648815632
-0.0333265960216522 1.0665442943573
-0.374665230512619 0.781462609767914
0.579575419425964 1.06914520263672
0.146003589034081 1.14037013053894
-0.875644743442535 -0.1250069886446
-0.119359865784645 0.268050253391266
-0.0525741279125214 0.570229470729828
0.827677249908447 0.492263853549957
-0.895352780818939 -0.879491686820984
-0.0675875693559647 -0.16582515835762
-1.60921967029572 -0.51768296957016
-0.563764810562134 0.749640882015228
-3.21943759918213 -0.185331642627716
-0.911248445510864 -0.753533780574799
-0.165861308574677 -0.432574927806854
-2.63956260681152 -0.00312972068786621
0.620537400245667 -1.8530547618866
0.369138389825821 0.699597418308258
-1.17390787601471 -0.604120671749115
0.43021622300148 -0.194888472557068
-1.08534550666809 -0.126482084393501
-3.5894832611084 0.0815743952989578
-0.981430649757385 -1.65976524353027
0.485661864280701 1.20758962631226
-4.1360502243042 0.0203682594001293
0.682070374488831 0.057042557746172
0.405853539705276 0.628213703632355
-0.805046379566193 0.577534317970276
-3.51851630210876 0.0147150084376335
0.619337201118469 0.335736662149429
-0.919942140579224 -0.971232831478119
-3.31742334365845 0.197549134492874
0.583354592323303 -1.18372941017151
-1.94585490226746 -0.640652358531952
-1.69718217849731 0.0899421349167824
0.486995249986649 0.177039787173271
-0.374480128288269 1.12291586399078
-2.44775819778442 -0.0894428566098213
-0.723435342311859 1.19004213809967
-0.583936989307404 -0.0447915643453598
-4.2435564994812 -0.256616055965424
-0.9207563996315 1.20041918754578
0.149515420198441 0.37815323472023
-2.21189308166504 -0.0313567668199539
-0.593465805053711 -1.19337809085846
-0.103999733924866 0.821646511554718
-0.152448311448097 0.207816228270531
-1.4371030330658 -0.544570326805115
-1.83722984790802 0.0679426342248917
-0.551134943962097 0.479544758796692
-1.37216377258301 -0.320125758647919
-3.13236045837402 0.0824632719159126
0.325503647327423 2.25770235061646
-1.11267125606537 -0.473738551139832
-1.56537592411041 0.327538847923279
0.253283083438873 -0.384074509143829
0.788997411727905 0.222582951188087
-1.15416777133942 -0.733468413352966
-2.06138205528259 -0.130490884184837
-0.304378926753998 1.21797609329224
-0.17266184091568 -0.123960062861443
-0.254618048667908 -1.65474045276642
-1.55155491828918 -0.769518613815308
0.188684463500977 -0.388371735811234
-2.73529648780823 0.245680645108223
-2.10309982299805 0.544197618961334
0.154558062553406 -1.48319232463837
-3.62194466590881 -0.255811095237732
-0.530003130435944 0.72383451461792
-0.951713979244232 0.445471584796906
0.194997504353523 -1.63607037067413
-0.224656641483307 0.625384569168091
-0.127925142645836 -0.441047996282578
0.511444449424744 -1.8535304069519
0.409425973892212 0.39158222079277
1.35709118843079 1.87494385242462
-1.92549562454224 0.238946959376335
0.535987615585327 1.02622485160828
-1.29397058486938 0.349256455898285
0.575598955154419 -1.39817595481873
1.5826004743576 -1.4299111366272
-0.201250582933426 0.900989830493927
-1.46496474742889 -0.839845418930054
-1.04658532142639 -0.044131688773632
-2.16405463218689 -0.118475735187531
-1.6126720905304 -0.121608801186085
-0.513273656368256 -0.332277685403824
0.0826238542795181 -0.937854528427124
-0.101322703063488 1.12291014194489
-0.428546398878098 -1.08894717693329
-1.57657492160797 0.550926327705383
-0.981925368309021 -0.313470900058746
-0.00635612569749355 -1.65107297897339
0.192553132772446 -0.311645954847336
0.620689392089844 1.86633861064911
0.0958876758813858 -1.05248785018921
-0.671312034130096 -1.06517362594604
1.13334345817566 -0.43650221824646
-2.74814677238464 0.159850433468819
-0.353155434131622 0.339684784412384
-1.97247576713562 0.529051780700684
1.01868081092834 -2.85094499588013
0.210101425647736 0.596008062362671
1.19775700569153 -0.539440751075745
0.193527743220329 -0.62395167350769
-2.67280197143555 -0.244634032249451
-1.95476722717285 -0.220425024628639
0.344765901565552 1.82500720024109
-2.13178968429565 0.348999857902527
0.0252539329230785 -1.28720307350159
-2.84154462814331 0.203702166676521
-0.852229475975037 -0.181032091379166
0.487896978855133 -0.0772130638360977
-0.383306801319122 0.319390475749969
-0.40896925330162 0.753000617027283
-0.131722450256348 0.121246337890625
-0.0588657632470131 -1.29461824893951
-2.60573244094849 0.0740092471241951
-1.91970324516296 0.116166837513447
0.600134193897247 -1.50384616851807
-2.70706486701965 0.38012284040451
-0.458778142929077 0.430751919746399
0.0981880724430084 0.668501138687134
-0.58331310749054 -1.32662153244019
-0.948053419589996 -0.56951779127121
-1.21561050415039 -0.627974927425385
-0.847476005554199 -0.77044939994812
0.489107012748718 -1.01936936378479
-0.856630146503448 0.560491025447845
-2.80778956413269 -0.0535034872591496
-2.20637488365173 -0.0525640249252319
-1.83598029613495 -0.251488268375397
-1.36205422878265 -0.269586563110352
0.207536906003952 0.896137475967407
-0.653822124004364 0.424709349870682
1.18069660663605 0.144206970930099
0.135085642337799 -0.40647965669632
1.11125648021698 2.21077299118042
0.0887403190135956 -0.917491137981415
-1.08895087242126 0.517501294612885
0.0821626037359238 1.02566385269165
-0.270754605531693 -0.620479345321655
-2.93260502815247 -0.202258810400963
-2.27962279319763 0.0105602592229843
-0.433544665575027 0.0981106162071228
-2.49939823150635 0.0348905585706234
-0.0155827254056931 0.0400798618793488
-4.57962608337402 -0.0862328037619591
-0.367543816566467 -1.54915106296539
-0.214782893657684 1.32604336738586
-0.810040831565857 0.125956475734711
-0.852152347564697 -1.40294659137726
-2.16602563858032 0.273049175739288
-1.07578527927399 -1.12898814678192
-2.90762090682983 0.289924085140228
0.996986627578735 -0.265684932470322
-0.109040543437004 -0.835898101329803
-0.0716045200824738 1.28010988235474
-1.17039632797241 0.371201574802399
-1.70036649703979 -0.557252764701843
0.0117844268679619 -0.170143961906433
0.698561131954193 1.91335690021515
-0.447753429412842 -1.50076639652252
-2.20927715301514 0.201575860381126
0.859856307506561 -0.280937254428864
0.284946203231812 -0.680743455886841
0.0651057511568069 0.222066000103951
-0.569822430610657 -0.107220396399498
-0.0467571541666985 0.826596140861511
1.39977645874023 -2.62756252288818
-0.491604834794998 1.23631811141968
-0.38385272026062 1.03028106689453
-1.95974886417389 0.119536362588406
-0.39459952712059 0.70651113986969
-2.35799717903137 -0.447589665651321
-0.107999861240387 -0.685143232345581
-1.07049870491028 0.0168396048247814
-1.37397682666779 0.577854156494141
0.604681730270386 1.94538378715515
-3.21457958221436 -0.0420006439089775
0.146068230271339 0.0823501348495483
0.146246805787086 1.19428968429565
-1.78963613510132 -0.615944743156433
-1.3388307094574 0.00429139286279678
1.28783738613129 1.89787721633911
-2.64067268371582 0.130241110920906
0.362459123134613 1.58045327663422
1.35599601268768 0.694952487945557
-0.364944159984589 -1.54309976100922
-0.997899413108826 0.196184679865837
0.912168562412262 -1.15722692012787
-0.136085331439972 1.03964233398438
-2.29034495353699 0.0962300673127174
-0.501626431941986 -0.565211117267609
-1.4205539226532 -0.369992524385452
-2.42717552185059 0.626936554908752
-1.65788817405701 0.345755457878113
1.16609215736389 0.759021639823914
-0.656156897544861 -0.279722034931183
-1.08198165893555 0.497267097234726
0.848021507263184 0.00578403472900391
-1.58753836154938 0.800392508506775
-1.05117428302765 0.520046949386597
-3.45993232727051 0.0872486084699631
-1.05079114437103 0.384760856628418
0.811385452747345 0.430174022912979
-1.59344100952148 -0.456600785255432
0.00670146942138672 -0.0626457333564758
-0.738102912902832 0.0726566165685654
-2.24493861198425 -0.148055493831635
-2.14360165596008 -0.643816113471985
-1.4544757604599 -0.380240678787231
-2.11158537864685 -0.569358348846436
0.775031924247742 0.653306245803833
-1.18268632888794 0.448576748371124
-0.929370760917664 0.937634885311127
0.796084523200989 -0.564786374568939
-1.11199879646301 0.659611761569977
-0.459470301866531 -0.377058357000351
-1.27880144119263 -0.575173377990723
-2.10632920265198 -0.136890023946762
-0.311293244361877 -0.295592129230499
-3.80096578598022 -0.00890526920557022
-2.0949923992157 0.498222172260284
-0.525561332702637 -1.68966734409332
-0.248927608132362 1.50903165340424
-1.36342978477478 0.394336521625519
-1.88583111763 -0.32569819688797
0.858301639556885 1.52036619186401
-0.922060906887054 -0.261069297790527
0.047742947936058 -0.681296467781067
-0.855963587760925 0.220547884702682
-2.6293728351593 0.368139922618866
-2.86653685569763 0.0431143194437027
-0.96545934677124 0.731771230697632
0.194054469466209 1.74302124977112
-1.71674752235413 0.274773508310318
-1.0168297290802 0.60989910364151
-0.746571898460388 -0.682490229606628
1.29722416400909 -1.48096144199371
-0.234844610095024 -0.207822009921074
0.372012376785278 -0.418069452047348
-2.09861135482788 -0.660956919193268
-1.29720985889435 -0.679128766059875
-0.177431032061577 -0.384023189544678
0.621793270111084 -0.0182879343628883
-2.5397686958313 -0.183882758021355
-2.42280435562134 -0.146928206086159
-0.00196569040417671 -1.65035307407379
1.29378914833069 -1.73168981075287
-1.45676481723785 0.0713830441236496
-0.785154461860657 1.03793585300446
-0.124692246317863 0.373647689819336
-0.125437393784523 -0.169271469116211
0.120234087109566 -0.187540665268898
0.124352350831032 -0.775577187538147
1.44108498096466 3.52420520782471
1.51462697982788 -1.63539338111877
-1.50915133953094 -0.0672032386064529
-0.695457994937897 -0.840200960636139
0.459636569023132 -1.25751066207886
-1.74186658859253 0.457776933908463
-0.708173632621765 -0.1224225461483
0.521093368530273 -1.59614753723145
-0.97814530134201 -0.953408479690552
-0.247150748968124 1.28393626213074
-0.98134446144104 -0.152183279395103
0.325738787651062 -0.294138371944427
-1.77155876159668 -0.302489697933197
0.641945779323578 -0.810172557830811
-1.7348370552063 -0.392746269702911
-2.92511463165283 -0.00978638231754303
0.352024078369141 0.443801790475845
-0.560684204101562 -1.74926435947418
-3.82006788253784 0.0561429187655449
-2.65649056434631 -0.11337023973465
-1.55778205394745 -0.465590566396713
2.16350674629211 1.26739716529846
0.955461621284485 2.09704875946045
-2.34577178955078 -0.281973123550415
-2.05907869338989 0.0953167080879211
-1.83376049995422 0.531984508037567
0.126245617866516 0.202074453234673
-2.36903285980225 -0.10815916955471
1.354651927948 1.28859829902649
-0.760178923606873 -1.56047260761261
-2.03406810760498 0.60765129327774
-1.99802684783936 0.404405027627945
-0.768324673175812 -0.482288271188736
0.410429954528809 -0.0444359481334686
-1.68200612068176 -0.995046973228455
-0.843193233013153 0.669413387775421
-2.77161407470703 -0.0488297715783119
0.300305485725403 1.2891571521759
-2.95290660858154 0.00647889077663422
0.556705594062805 -1.73172986507416
1.38954722881317 2.35613560676575
-2.13909697532654 0.201952397823334
-0.659017860889435 1.14161431789398
-0.644411325454712 0.268071174621582
-0.87084686756134 0.95564740896225
-1.6759546995163 0.113092973828316
0.733649790287018 0.232805788516998
-2.20747089385986 0.40274366736412
0.392703652381897 0.216182261705399
-0.641646683216095 -0.959008276462555
-2.14069318771362 0.239332631230354
0.856236696243286 1.18452250957489
-1.24575543403625 0.298767626285553
0.0412489473819733 0.0157169252634048
-1.44720637798309 -0.000218577682971954
1.90508306026459 -2.73598790168762
0.676008582115173 -0.203371420502663
0.988079965114594 2.74334955215454
-2.59507584571838 -0.643302023410797
-3.09949541091919 0.118426866829395
-1.5380687713623 0.935589969158173
0.903509318828583 -0.974047064781189
-2.00831890106201 0.0052390992641449
0.723792314529419 -0.235336393117905
-0.322240024805069 0.062930166721344
-1.13217008113861 0.0123294740915298
-0.816896259784698 -0.266778469085693
-0.359707176685333 0.763981997966766
-1.60489284992218 -0.0362699329853058
-1.22519540786743 0.2668377161026
1.67748522758484 0.172313332557678
-1.65130805969238 -0.20894493162632
-0.709812343120575 -0.512122392654419
-0.252023756504059 0.380297660827637
0.958488941192627 -0.0523566007614136
-2.11262774467468 0.745882153511047
-2.45933389663696 -0.470704197883606
1.45204269886017 -2.79873538017273
-0.775950372219086 -1.44770395755768
-2.80200457572937 0.420192778110504
-0.277645528316498 -0.397560775279999
-1.05652117729187 -0.487182259559631
-0.532085716724396 -1.28910410404205
-1.42333436012268 0.315788507461548
-0.718506455421448 0.558730781078339
1.14192819595337 2.18411755561829
-1.42104434967041 0.426628082990646
-4.05943059921265 0.0795829445123672
-0.511190116405487 0.555009245872498
-2.59440183639526 0.39536315202713
-0.216346114873886 -0.64649909734726
-0.638978958129883 0.397971749305725
-1.4119199514389 -0.188555598258972
-2.74776816368103 -0.242579311132431
0.237662792205811 -0.947199046611786
-2.84503269195557 0.0436369925737381
-1.78801774978638 -0.160764008760452
0.183441877365112 1.84790325164795
0.884895503520966 -1.46886134147644
0.118646413087845 -1.77714991569519
0.783103942871094 0.0425575152039528
-1.34782087802887 -0.0801224261522293
-0.815853714942932 0.0285088717937469
-1.39734292030334 -0.4109967648983
-1.56118905544281 -0.213871359825134
-0.282848685979843 0.00546848401427269
-0.0930043160915375 0.422678649425507
1.91033339500427 -0.507898449897766
0.276355236768723 0.110454127192497
-1.41233313083649 0.0731955915689468
-0.776146292686462 0.186743527650833
-0.888856291770935 -0.0492480173707008
-2.35887861251831 0.170504420995712
-1.78020989894867 -0.576354563236237
-0.232842832803726 -0.223404601216316
-1.9995197057724 -0.346399396657944
0.318438589572906 0.83153885602951
-2.2505669593811 -0.332877069711685
-2.70654773712158 -0.365159690380096
0.31635046005249 1.81038689613342
-2.83121180534363 -0.300458699464798
-1.36895787715912 0.0867136269807816
-1.8528094291687 -0.197472631931305
-1.33233880996704 -0.677464246749878
-0.569413483142853 -0.575482666492462
-2.90802550315857 -0.369357287883759
-2.47906756401062 -0.461826622486115
0.719916522502899 0.985542237758636
-1.07541251182556 0.545083165168762
-1.11408758163452 0.910630583763123
-0.61580628156662 0.933994650840759
-1.1035680770874 -0.461269527673721
0.505827307701111 0.320663511753082
-0.353441387414932 -0.838256239891052
0.0753753930330276 -1.16218113899231
-0.0516490265727043 -0.253146111965179
-0.304722428321838 -0.0774557963013649
0.213058695197105 0.738468408584595
0.19382181763649 -0.211413979530334
-3.26393818855286 -0.267813503742218
-0.981905341148376 -1.13789927959442
1.45329320430756 1.79062974452972
0.0401412397623062 0.923618495464325
-1.92365801334381 0.859583854675293
-0.457439124584198 -1.15019607543945
-1.66681027412415 0.451639831066132
-1.9964302778244 -0.371746331453323
-0.00875911116600037 -0.345015168190002
-0.203601568937302 -1.17337894439697
0.911807894706726 2.2640974521637
-0.559627950191498 -0.865578651428223
0.682305991649628 1.8765412569046
-1.44582951068878 0.249287620186806
-0.62111496925354 0.464456588029861
-1.31493079662323 -0.119505986571312
-2.22444128990173 -0.420638501644135
0.934272348880768 -1.46580135822296
0.996778070926666 0.825873970985413
0.0817679315805435 1.02841830253601
-0.968729436397552 -0.291188389062881
-1.18608093261719 -0.398227155208588
-1.358722448349 1.03416001796722
-0.168463140726089 -0.423612087965012
-0.394397139549255 -1.22159397602081
1.22625589370728 -0.705029845237732
0.473608672618866 -1.4402836561203
-3.01912426948547 0.259389281272888
-1.2924896478653 0.454346418380737
-0.541963517665863 -0.493402689695358
-2.50323224067688 -0.0959002524614334
0.131369262933731 1.37159705162048
-1.69390022754669 -0.0422861948609352
-0.0229140408337116 -0.519734025001526
-0.287096381187439 -0.743217706680298
-1.10436117649078 0.916265964508057
-1.18350231647491 -0.168073266744614
-0.036597978323698 -0.0328970775008202
0.211094528436661 1.69686949253082
-0.79878443479538 0.787521839141846
-2.32542967796326 -0.69378662109375
0.143195241689682 -1.92182719707489
-0.852733373641968 -0.131275713443756
-0.206471145153046 1.68223142623901
0.251665234565735 0.959205508232117
-0.053620234131813 0.178842186927795
0.3740114569664 -1.04437601566315
-1.62905085086823 0.732431948184967
-1.84352922439575 0.201455637812614
-3.44842314720154 0.0641193315386772
0.00318963825702667 0.947547256946564
-1.00846266746521 -1.11648797988892
-0.0144575387239456 -1.03853535652161
-1.34656596183777 0.456688851118088
0.856421649456024 0.36854562163353
0.635994434356689 0.510774731636047
0.387088894844055 -0.305637776851654
-1.57505106925964 0.8016237616539
-3.75378489494324 -0.200669676065445
-0.910804331302643 -1.10128939151764
-1.95367419719696 0.600957036018372
-1.18274915218353 0.446454524993896
-0.778038442134857 0.134751185774803
-1.20958566665649 0.602745473384857
-0.286957532167435 1.55604696273804
-3.29128861427307 -0.392672061920166
-2.21719336509705 0.191975191235542
-2.87528657913208 -0.250376880168915
0.727975428104401 1.51516091823578
0.721516788005829 -0.088983416557312
-1.54945719242096 0.108787447214127
-0.317881286144257 -0.177365154027939
-4.12589740753174 -0.0934228673577309
-0.186609208583832 1.22450125217438
-0.741945266723633 -0.149137184023857
-1.29970073699951 -0.213738560676575
0.89201420545578 1.80485773086548
-0.510980546474457 -1.5684597492218
0.588916838169098 1.10763657093048
0.277426183223724 -1.40736198425293
1.12434411048889 -1.65764832496643
-0.538976311683655 -0.0598908476531506
-0.418791383504868 0.512355089187622
-3.98766899108887 -0.0147518385201693
1.39342069625854 -1.47162759304047
0.654952764511108 1.67998766899109
-0.0517581701278687 0.68513149023056
-1.3693140745163 0.0994936153292656
0.23430335521698 -0.577759385108948
-2.25787591934204 -0.100806757807732
-1.02165222167969 0.485633879899979
-0.666167020797729 0.383138507604599
-1.741379737854 -0.823872208595276
-1.39887702465057 0.166299358010292
-1.03324449062347 1.4524142742157
-1.63994228839874 -0.860469818115234
0.0239353645592928 -0.883781611919403
0.0571592599153519 -2.08200240135193
-3.41200089454651 -0.245198711752892
1.08460402488708 -2.92882585525513
-1.68742978572845 0.0984073132276535
-0.360090225934982 -0.509252369403839
-0.891249299049377 -0.817464709281921
0.376876711845398 1.44576382637024
-2.02871918678284 0.204763859510422
0.753199934959412 0.644238770008087
-2.3761682510376 0.0981791093945503
1.03667438030243 0.0377811715006828
-2.86234712600708 0.19338670372963
-0.75305700302124 -1.23684561252594
-3.91127514839172 -0.167337983846664
-0.0258629620075226 -1.09255969524384
-0.303683400154114 0.113709695637226
0.620408296585083 -0.862141072750092
-0.999660074710846 -0.977601170539856
0.947639465332031 0.858833849430084
-0.482801586389542 -0.403199076652527
-2.41153717041016 -0.156131595373154
0.30169665813446 -0.2074284106493
2.03087949752808 -0.777107298374176
-1.06285154819489 -0.652666509151459
-0.487247824668884 0.173503831028938
2.00193357467651 -1.08005487918854
1.85702061653137 -1.41678440570831
-1.99139702320099 0.110674791038036
-3.69187951087952 -0.0326125659048557
-1.74046075344086 0.410347908735275
-2.21481680870056 0.0829655826091766
1.14040076732635 0.979559421539307
0.966010451316833 -1.7062520980835
-0.150321274995804 1.29252898693085
-0.631521880626678 0.343658477067947
-1.90892672538757 0.224126160144806
-1.3565137386322 -0.0392461642622948
0.54944908618927 -1.0250049829483
-2.80248951911926 -0.227559119462967
-2.92242407798767 0.048346683382988
0.601417064666748 -0.626132249832153
1.46742033958435 -0.149547472596169
-0.402796447277069 -0.818192362785339
-2.37701082229614 0.259051442146301
-1.09423911571503 -1.12707567214966
0.359445571899414 0.40197017788887
-0.348503232002258 -0.211426109075546
-0.658337235450745 0.704865574836731
1.04531908035278 -2.40612840652466
-3.44259881973267 -0.186172306537628
0.497460663318634 -0.503974139690399
-1.1561861038208 0.751911044120789
-0.246801137924194 -0.180063456296921
-0.629777073860168 0.335701823234558
-0.0890293642878532 0.988578379154205
-0.701259672641754 0.438908815383911
-0.894384860992432 0.317609339952469
-3.06971788406372 -0.110037066042423
-1.34128761291504 -0.25254288315773
-0.38173907995224 0.195728480815887
-0.061494342982769 0.380502641201019
-2.26812672615051 -0.195136353373528
-2.42015671730042 0.087124727666378
-2.88380551338196 0.358328491449356
-0.327381253242493 -1.21640992164612
-3.5286271572113 -0.0882532149553299
-1.21313166618347 0.524343609809875
-0.496318757534027 -1.18823599815369
-1.32802987098694 -0.0227926876395941
1.01027393341064 0.02558583766222
-0.0674142688512802 -0.278306007385254
-1.32084023952484 -0.786162614822388
-3.26368641853333 0.142467319965363
-1.61739981174469 -0.312500059604645
-1.37519383430481 -0.266158998012543
-1.79169011116028 0.011733241379261
-0.00082678347826004 -0.278345793485641
0.214316755533218 -0.80352395772934
-2.85412383079529 0.571625351905823
-1.22641158103943 -0.545635223388672
-0.986239910125732 0.248069167137146
-0.88826709985733 0.590741753578186
-1.6108295917511 0.570249795913696
-2.99980068206787 -0.536120533943176
0.671658635139465 -0.347340404987335
-0.863825678825378 -0.769449532032013
-0.690320611000061 0.89564049243927
-2.40523672103882 -0.0318161100149155
-2.14226770401001 0.119415655732155
-2.084388256073 0.221012160181999
-2.04818177223206 -0.764091014862061
0.0854942798614502 -0.342876225709915
0.214844927191734 -1.54281580448151
0.280929446220398 -0.00561104714870453
-0.882370352745056 -1.00993120670319
-1.43346667289734 -0.511259913444519
-0.703563690185547 0.395369112491608
0.740067481994629 0.919722676277161
0.738823354244232 0.217171877622604
0.0850330889225006 1.26390266418457
-1.61124634742737 -0.37738224864006
0.478385865688324 0.584407866001129
-1.04983258247375 0.248495355248451
-0.122709929943085 -0.824891686439514
-1.06527674198151 0.447604179382324
-1.48081588745117 -0.40675351023674
0.626978397369385 1.26280379295349
-1.22424173355103 0.520374655723572
0.508676111698151 0.408428102731705
-0.107993178069592 -0.776524722576141
-0.700144827365875 -0.320312649011612
-2.10004925727844 0.492027312517166
-1.76185739040375 0.333377420902252
-0.926565051078796 -0.343207031488419
-1.55492389202118 0.205059617757797
-1.04194033145905 0.822965145111084
1.45033049583435 0.746213853359222
0.0533023178577423 0.677817940711975
-0.813012361526489 0.250731527805328
-2.20137429237366 -0.258826196193695
0.0417779870331287 -0.846660017967224
-1.00314128398895 -0.941672027111053
-0.255207091569901 -1.4932165145874
-0.495244413614273 0.265752553939819
0.93089359998703 -2.4247088432312
0.159853100776672 1.85157537460327
-3.60824537277222 -0.0628386437892914
-1.21104383468628 -0.635552704334259
1.03383612632751 2.32514262199402
0.401467144489288 1.7733850479126
-0.550247251987457 -1.35946893692017
-2.19831681251526 -0.0646114647388458
-3.38334202766418 0.133626654744148
-1.8323085308075 0.469145655632019
-0.275068581104279 0.0900243148207664
-0.124863922595978 -2.48219871520996
-2.20623874664307 0.154647842049599
0.452686876058578 -3.27412295341492
0.686464667320251 0.0414210557937622
-0.668955624103546 0.0997190251946449
-0.577956914901733 -0.656257212162018
-2.6076512336731 -0.310275018215179
0.638330221176147 -0.958970367908478
};


==> figures/visualizations/funnel/mfvi_samples.tex <==
\addplot [semithick, mfvi, opacity=0.7, mark=x, mark size=3, mark options={solid}, only marks]
table {%
-0.546237468719482 0.388371795415878
0.789855599403381 -0.420998871326447
0.145024850964546 1.08318138122559
-0.227278470993042 -0.204801470041275
0.565920472145081 -2.73963499069214
0.105116568505764 0.366099685430527
0.0744241327047348 1.32426834106445
0.189736798405647 0.230549708008766
0.293201595544815 0.0561640337109566
-0.665766477584839 0.402381509542465
-0.458097010850906 -1.66937613487244
-0.559180378913879 -0.227737307548523
0.265169203281403 0.548230648040771
0.628548681735992 -0.543849945068359
-0.620427310466766 -0.905415952205658
0.388495117425919 -0.235191136598587
-0.0533669218420982 0.824183881282806
0.140349343419075 -0.20863763988018
-0.490508615970612 0.960894227027893
0.322637319564819 -1.77208387851715
0.579177558422089 -0.997272133827209
0.598994970321655 0.228134721517563
0.445602655410767 -1.61008942127228
-0.664437353610992 0.685165882110596
-0.194522589445114 1.80597376823425
-0.417145550251007 -0.489796549081802
0.607404828071594 0.245521530508995
-0.0313266739249229 1.007772564888
-0.200652346014977 -0.810070216655731
-0.46341609954834 2.18780994415283
-0.0688460096716881 -1.17515575885773
-0.254934966564178 -0.160043492913246
-0.198537021875381 -0.25177475810051
0.0300840567797422 -0.00466000149026513
-0.117315076291561 -0.79014664888382
-0.0107752848416567 -0.112322710454464
0.270179659128189 1.59154665470123
-0.0656348690390587 0.948709845542908
-0.750123202800751 -1.86464655399323
-0.321469187736511 -0.144964173436165
-0.149021282792091 -1.22490084171295
-0.464770078659058 0.664166271686554
-0.043606348335743 1.31284248828888
0.477061986923218 -0.481929987668991
-0.520027458667755 -0.564255774021149
-0.165838032960892 -0.188724264502525
0.142026737332344 0.43686243891716
0.305380910634995 0.0707968398928642
-0.310688853263855 -0.599016845226288
-0.304935961961746 -1.05998718738556
-0.216474011540413 -0.746759712696075
0.319752365350723 1.20749008655548
-0.126186728477478 0.134612381458282
0.0321056023240089 -0.0456383936107159
0.365595608949661 -1.38336873054504
0.552751779556274 -0.556181371212006
-0.222267270088196 -0.0483634918928146
-0.17789688706398 -0.828167259693146
0.633339822292328 1.12197661399841
-0.00123602338135242 -1.93758618831635
-0.149128779768944 1.06873166561127
-0.178187504410744 -0.640073418617249
-0.765041828155518 0.855774462223053
0.181041166186333 0.373566806316376
-0.0430825352668762 -1.14266550540924
-0.764918863773346 1.50287282466888
-0.525587439537048 0.497341305017471
0.107354678213596 1.09762096405029
0.161727175116539 -0.951015830039978
-0.0291045587509871 -1.14315402507782
0.187850460410118 -0.379786312580109
0.0572319850325584 -0.278871595859528
-0.0145097188651562 -0.937493622303009
0.387794703245163 -0.122214749455452
-0.348924309015274 -0.755212962627411
-0.830282926559448 0.389872193336487
0.252569377422333 0.146319299936295
-0.0473304986953735 -1.26296925544739
0.0968262702226639 -0.988721191883087
-0.181817293167114 1.52689242362976
0.657363474369049 -0.446206271648407
0.149394318461418 -1.33342838287354
-0.165720894932747 0.179120257496834
-0.109654679894447 -0.557982563972473
-0.947507441043854 1.03047096729279
-0.213150694966316 1.23254477977753
0.463053703308105 0.650000989437103
-0.49873298406601 0.809677720069885
-0.537780225276947 -0.563367247581482
-0.381333351135254 -0.0687950104475021
0.134825631976128 -0.725694477558136
0.510213494300842 -1.56123566627502
-0.0111208334565163 -0.920145571231842
0.125936985015869 -0.12149752676487
0.262820571660995 -0.653891324996948
-0.208706736564636 1.05074167251587
0.188456952571869 0.443314671516418
-0.151521474123001 0.507578551769257
-0.465449929237366 0.45551785826683
0.0110253347083926 3.02451729774475
-0.443420439958572 1.33855438232422
1.28259897232056 -0.693454325199127
-0.194788724184036 0.361233562231064
-0.043303944170475 -1.41444933414459
-0.312649071216583 1.93283236026764
-0.543497681617737 1.00634598731995
-0.14857292175293 -1.1335973739624
-0.967192947864532 -0.832833707332611
-0.413799285888672 -0.24616414308548
-0.289119631052017 -2.01402759552002
0.164790362119675 -0.595492124557495
-0.306328177452087 -1.55260252952576
0.0452966168522835 -0.0737687349319458
0.390279680490494 -0.833379209041595
0.545976996421814 -0.708683848381042
0.39725723862648 0.0529858842492104
-0.433451235294342 1.1635559797287
0.0446460992097855 -0.0650336071848869
0.567204833030701 1.72257697582245
0.0620358064770699 -1.05628263950348
0.209808886051178 -2.55623316764832
0.151835501194 -1.05264925956726
-0.752086400985718 1.40302264690399
0.487639576196671 1.28631472587585
-0.359450489282608 1.37128031253815
0.206715628504753 -0.463792860507965
0.362941771745682 -1.39450109004974
0.107342906296253 -1.01427507400513
0.31656014919281 -0.401460409164429
0.521509170532227 -0.288130730390549
0.402921110391617 -1.84690189361572
0.421563148498535 -0.970847964286804
-0.00629798322916031 -2.20379567146301
-0.0515032261610031 0.75970047712326
1.24028027057648 -1.16565501689911
0.0781662315130234 -1.3149516582489
-0.566855669021606 0.234063267707825
0.541739702224731 0.594786465167999
0.7810178399086 -1.54691863059998
-0.60646790266037 0.572898626327515
-0.044269010424614 -0.233107551932335
0.352619528770447 -1.01690411567688
0.139104545116425 -0.81469315290451
-0.261229068040848 0.443668514490128
1.07351112365723 -1.59757506847382
-0.336596012115479 0.409539848566055
0.0823111683130264 0.0645940825343132
0.292409479618073 -1.95504415035248
0.559239208698273 0.762413740158081
0.690782308578491 0.184515804052353
0.0400298796594143 -0.886771321296692
0.629350662231445 0.953115344047546
-0.203885972499847 -0.191427513957024
0.0551581755280495 1.06623351573944
-0.0815551653504372 0.58542662858963
-0.0923677608370781 1.48093342781067
-0.651199162006378 0.303613275289536
0.457312643527985 -0.445408016443253
-0.247479498386383 -0.734933733940125
0.187498956918716 -1.93848598003387
-0.113243483006954 0.0428402721881866
1.04137408733368 0.124509334564209
0.363293260335922 0.371399700641632
0.391574800014496 0.540561258792877
-0.925993144512177 1.03585302829742
-0.191909521818161 1.95121133327484
0.133954092860222 -2.11581254005432
-0.434686928987503 0.153952673077583
-0.113378576934338 -1.12438476085663
0.10946749150753 0.117325857281685
-0.49969494342804 2.50585222244263
-0.714490711688995 0.429582417011261
-0.180438712239265 -0.592725813388824
-0.0203009862452745 0.965499341487885
0.0760512351989746 -0.631884455680847
0.204029381275177 0.813026607036591
0.0502932444214821 -1.1828715801239
0.0160544589161873 -0.171852886676788
-0.0422602370381355 1.01473128795624
0.289984792470932 -0.674940407276154
0.348953187465668 0.858487248420715
-0.720215678215027 -0.176577851176262
1.04330241680145 0.11658450961113
0.487033009529114 -0.202619552612305
0.836479008197784 0.446840673685074
-0.24579593539238 -1.71309947967529
0.249661594629288 -0.00583483092486858
-0.089566595852375 -1.17942261695862
0.201472833752632 0.149567827582359
0.348141074180603 -0.10067792981863
0.773238182067871 0.552600622177124
-0.185022205114365 -0.0660239830613136
0.635913372039795 -0.889231622219086
-0.368695944547653 -0.311459928750992
-0.787577629089355 -0.419039636850357
-1.07192194461823 2.95810604095459
-0.00332973245531321 1.26408815383911
-0.155291154980659 -0.193221643567085
0.104706212878227 1.47746157646179
0.272961169481277 0.554894685745239
0.673654794692993 -1.80270230770111
-0.299650609493256 -0.037321999669075
-0.926647067070007 -1.10367226600647
-0.134814485907555 0.606658458709717
0.308466374874115 0.641995131969452
-0.0237661134451628 0.826620817184448
0.223254665732384 -0.0846977382898331
0.32337149977684 -1.27509224414825
-0.141280978918076 -0.18092580139637
-0.135931208729744 -0.703581213951111
0.612196624279022 0.679070889949799
-0.399087458848953 -1.67002940177917
-0.860731840133667 -0.337358057498932
-0.581467509269714 0.174162432551384
0.104820847511292 -0.846252381801605
0.00973285362124443 0.769135653972626
-0.193931847810745 -1.92123663425446
0.10838557779789 0.084954522550106
0.542446255683899 -0.14509953558445
-0.0788828507065773 -0.325692504644394
-0.17703552544117 1.22130334377289
-0.390008568763733 1.15951418876648
0.733452081680298 0.744774103164673
-0.539294004440308 -0.856283366680145
-0.272043704986572 1.17554903030396
0.956761360168457 -1.0829199552536
0.552006840705872 -0.116828434169292
0.370248705148697 0.450932502746582
-0.657696604728699 1.13835895061493
-0.0360951796174049 -1.5721447467804
0.0331449508666992 0.661972999572754
-0.373962163925171 0.486270695924759
0.921902656555176 1.37984585762024
-0.430545836687088 0.371683865785599
0.950672030448914 -1.6345032453537
-0.808357656002045 -1.12133526802063
-0.0657883808016777 2.59757971763611
0.0669987052679062 -0.658251881599426
-0.389432460069656 -0.743515312671661
-0.564223289489746 0.23062501847744
0.0255924519151449 -1.0962165594101
-0.203022450208664 -1.02325928211212
-0.580013453960419 0.327438205480576
0.131723329424858 -2.01490569114685
-0.432812333106995 -0.893928647041321
-0.585264444351196 -0.0411629304289818
-0.224764287471771 1.17456531524658
-0.237176194787025 -1.93774223327637
-0.179913237690926 -1.82701051235199
-1.14971613883972 0.685913026332855
-0.0844391509890556 -2.34510445594788
0.128105252981186 0.328397214412689
0.0767588391900063 -0.269071847200394
-0.76862508058548 0.251230150461197
-0.501949667930603 0.119111508131027
0.0187129285186529 0.206372082233429
-0.02830277569592 -1.21976947784424
-0.135800316929817 -1.62603914737701
-0.00156879238784313 -0.0355489365756512
0.0113315787166357 2.07056140899658
0.864397943019867 -0.335565656423569
-0.749313473701477 -0.879608690738678
-0.334340363740921 -0.854422748088837
-0.0431986227631569 0.0845560729503632
-0.76914381980896 0.797272205352783
0.258609056472778 -0.34390851855278
0.689456820487976 -1.40231013298035
0.912967205047607 -0.629284381866455
0.240859895944595 -0.392373621463776
-0.337356239557266 0.0417115055024624
-0.0210182871669531 2.291743516922
0.769903838634491 0.824026346206665
0.324605375528336 -0.50333172082901
-0.314438432455063 -0.104974709451199
0.590453326702118 2.44754815101624
0.206044390797615 -0.537290155887604
0.383319050073624 1.5002875328064
-0.0367640480399132 0.900819718837738
-0.544361591339111 0.419061124324799
0.234148755669594 -0.924870729446411
-1.06534016132355 0.44371622800827
0.242192417383194 1.55779051780701
0.257804661989212 -0.418823748826981
-0.846291065216064 0.49197706580162
-0.248304843902588 -0.452347248792648
0.0470606908202171 -0.810669898986816
-0.548972904682159 0.38869521021843
-0.518520951271057 0.275016039609909
0.194635555148125 0.931132018566132
0.659636735916138 -1.00314939022064
0.41351056098938 0.560725033283234
-0.203169271349907 0.210328161716461
-0.486739784479141 1.81575667858124
0.315896183252335 0.556770741939545
0.0845398679375648 0.455431789159775
-0.25738251209259 -1.14054548740387
-0.278605908155441 -0.857754528522491
0.164204761385918 -0.970892429351807
0.250323683023453 0.30444273352623
-0.393820524215698 -1.0892596244812
-1.86344385147095 -1.73940277099609
0.326966375112534 -2.79712533950806
0.0336917787790298 0.320285648107529
0.241004139184952 0.0632487088441849
-0.0130241569131613 -0.620326519012451
-0.152117013931274 0.776327073574066
-0.0738453045487404 0.551084995269775
0.922681093215942 -1.1004638671875
0.222377464175224 1.24358105659485
0.183969438076019 0.215665459632874
-0.0825410410761833 -1.66015350818634
-0.500930368900299 -1.5608948469162
0.205239966511726 -0.624996364116669
0.524007439613342 -1.01229822635651
0.942348957061768 -0.73807692527771
-0.111796505749226 0.272261142730713
-0.576508283615112 0.482985824346542
0.365256756544113 1.44995045661926
-0.246916741132736 1.60299777984619
-0.35143318772316 -1.31776988506317
0.172236159443855 -1.18769872188568
-0.112830370664597 0.211262792348862
0.141424238681793 1.45761811733246
-0.38774973154068 0.432448476552963
0.615804314613342 -0.18297915160656
0.0677337720990181 0.535289287567139
0.490825891494751 -0.00517603009939194
0.545646548271179 -0.641163647174835
0.196201890707016 2.47415018081665
-1.1629501581192 0.701639652252197
0.115902833640575 1.0622570514679
0.392631709575653 -0.721198678016663
1.36170542240143 -1.58741569519043
-0.379747837781906 -0.546859979629517
-0.549839675426483 -0.00264440989121795
-0.311935424804688 0.900524616241455
0.17793233692646 -1.18364214897156
-0.991497814655304 0.759400904178619
0.319667994976044 0.107202708721161
-0.225504204630852 1.06210649013519
-0.370332270860672 -0.0177529193460941
-0.167037561535835 -0.00487260054796934
-0.338520437479019 -0.920302927494049
0.554408431053162 -0.344660758972168
-0.323408931493759 0.526600301265717
-0.318720161914825 -2.4107711315155
0.796469211578369 -0.81351900100708
-0.777911365032196 -0.528848946094513
-0.647741675376892 0.862208068370819
0.173064216971397 2.68498396873474
0.356255829334259 -0.476093351840973
-0.331199437379837 0.755890488624573
-0.126805916428566 -0.228740096092224
-0.737526595592499 -0.00058706384152174
0.337666571140289 -1.20446300506592
0.832997679710388 0.420895904302597
-0.0261318143457174 -0.896784901618958
0.141153261065483 -0.177349403500557
-0.475508391857147 0.138279110193253
-0.528851747512817 -0.792049467563629
0.291703283786774 1.83049368858337
-0.0626633539795876 -0.143696472048759
-0.194138243794441 -0.889528274536133
0.0646276995539665 0.505117058753967
0.384246587753296 0.443417072296143
0.610888481140137 -0.177974566817284
-0.0944513380527496 -1.33665490150452
-1.00253558158875 0.283030062913895
0.288234412670135 0.659215033054352
-0.086002454161644 -0.716362655162811
-0.178976744413376 0.292145997285843
0.0228495933115482 0.485827624797821
-0.918388903141022 0.0608370080590248
-0.611814320087433 1.5516631603241
0.187862679362297 0.299003720283508
0.0433957725763321 -0.189862087368965
0.349009871482849 1.95910882949829
-0.0327087640762329 -1.29375219345093
-0.179312393069267 0.868825197219849
0.217511370778084 -0.0448819696903229
-0.717572689056396 -0.664167582988739
-0.0899128168821335 0.126405522227287
-0.317596942186356 -0.635529816150665
-0.231596991419792 1.02744519710541
0.346948057413101 -0.213813289999962
0.253092378377914 -0.0642170011997223
0.346529334783554 1.20910131931305
0.45790833234787 0.671266257762909
-0.731253027915955 -0.320221573114395
-0.796639382839203 -0.405642449855804
-0.0394267067313194 -0.851539373397827
-0.0579331293702126 0.166161492466927
0.478413313627243 -1.27863752841949
-0.0774922892451286 1.57070124149323
-0.331331312656403 -0.324339777231216
-0.280580192804337 0.468789935112
-0.0474852249026299 -0.0599703043699265
0.279906064271927 -0.728544056415558
-0.17529159784317 -0.992771446704865
0.107218079268932 -0.403947740793228
-0.468881607055664 0.31935927271843
-0.360992223024368 0.680330693721771
-0.545513868331909 1.09773468971252
-0.519944608211517 -0.283743739128113
-0.107474699616432 -1.12609875202179
0.522213041782379 0.995412051677704
0.42380553483963 -0.31935578584671
0.514736831188202 -1.0879944562912
-0.20535010099411 -0.453191936016083
0.0963741019368172 1.41482126712799
0.377999395132065 0.703396081924438
0.510557174682617 0.248379692435265
-0.848325312137604 0.307098746299744
0.197545453906059 -0.0331146866083145
0.723145484924316 0.020089216530323
0.609937489032745 -0.227667048573494
-0.0852171927690506 0.573706567287445
1.3817572593689 1.26680541038513
0.567012906074524 -0.228372767567635
0.828565001487732 0.651209533214569
0.413948476314545 -0.963941633701324
-0.492245376110077 -1.79073011875153
-0.437706798315048 0.261840373277664
0.427898406982422 1.36141085624695
-0.577021420001984 -1.14595234394073
-0.359787315130234 -0.313939183950424
-0.619718194007874 2.2032458782196
-0.253726154565811 0.0589129328727722
-0.209342077374458 -1.13335061073303
0.044148363173008 0.170343548059464
0.454893887042999 0.133881762623787
0.196097478270531 0.556289553642273
-0.288587480783463 0.947446823120117
0.388554126024246 -0.927668690681458
-1.06072604656219 -0.338059961795807
-0.0014605550095439 -0.738372385501862
-0.41527995467186 0.817822933197021
0.707813441753387 0.307877898216248
0.597089469432831 1.03803110122681
0.00171220861375332 -0.383237779140472
-0.285350024700165 0.270918071269989
-0.0673484802246094 -1.22133910655975
-1.47221124172211 -0.975053012371063
0.39266961812973 0.135355994105339
0.602826595306396 -0.675093948841095
0.244429290294647 1.22973072528839
0.08637335896492 1.47953975200653
-0.301092594861984 -0.916300237178802
0.415182739496231 0.615006923675537
-0.0569914653897285 -0.10750538110733
-0.195723921060562 -1.10425984859467
0.0992309302091599 0.831640303134918
-0.243107676506042 -0.453263789415359
0.286531180143356 -0.722126007080078
-0.237364247441292 -2.49707388877869
-0.034628763794899 -0.994943976402283
-0.667718946933746 -0.913292109966278
-0.0866489335894585 -0.0860045179724693
-0.0763157531619072 -0.711486995220184
0.426804274320602 1.15781307220459
-0.0265645179897547 0.974841117858887
-0.392141669988632 -0.949140250682831
0.685922265052795 -1.40667474269867
0.796790421009064 0.499518066644669
-0.294208705425262 0.336355179548264
0.0713291838765144 0.857121765613556
0.501143217086792 -1.668661236763
-0.156805396080017 -0.326026231050491
0.688895404338837 -0.459348648786545
-0.122162587940693 -1.3624175786972
0.118925966322422 -0.85086864233017
-0.116164661943913 2.30975437164307
-1.05651569366455 -1.87478041648865
1.12737429141998 0.838573932647705
0.111979305744171 1.80391621589661
1.31276166439056 -0.969223916530609
-0.035164512693882 0.149212375283241
0.643602609634399 -0.745944678783417
-0.624044835567474 -0.000921726226806641
-0.149389833211899 -0.829353332519531
0.304393380880356 -2.0663857460022
0.228026539087296 -1.29202449321747
-0.376023828983307 -1.09126329421997
-0.140423998236656 -0.0896841809153557
0.0369035750627518 0.48939111828804
-0.303946733474731 1.17565906047821
0.0798075199127197 0.40371710062027
0.990211308002472 -1.16427206993103
0.276417076587677 1.46690738201141
-0.13224895298481 -0.646239817142487
0.0157722309231758 -1.57981252670288
0.22925691306591 0.470864325761795
-0.433249533176422 -0.29358583688736
0.0354359038174152 1.33443903923035
0.845153152942657 -2.21514630317688
-0.347602188587189 1.2863175868988
0.0430100448429585 -0.121026463806629
0.313474416732788 -0.287472248077393
0.767073571681976 0.882673680782318
0.0141097269952297 0.934375643730164
-0.114058636128902 -1.10824990272522
-0.771165192127228 1.64045548439026
0.350151151418686 0.720324456691742
-0.562462687492371 -0.117729812860489
0.424747258424759 -0.240353584289551
0.362834274768829 -0.104408405721188
0.0244932845234871 -1.58475017547607
-0.35971462726593 0.766089916229248
0.268243581056595 1.91170394420624
-0.352204918861389 0.850449562072754
-0.157822549343109 -0.432816863059998
-0.476137757301331 1.364302277565
0.487096965312958 -0.545592844486237
-0.845265209674835 -1.67988550662994
-0.580528497695923 -0.0700700730085373
0.608994781970978 1.86070835590363
-0.046747513115406 0.585685551166534
-0.169741198420525 0.476899534463882
0.0366071835160255 -1.0182501077652
-0.120511017739773 0.542208075523376
-0.163397610187531 -0.441469073295593
0.388993293046951 -0.490860015153885
0.431232690811157 0.959277331829071
-0.232547774910927 0.503579318523407
-0.439695239067078 0.849425673484802
-0.0945504233241081 0.625522911548615
-0.173608303070068 0.454024940729141
-0.00126714631915092 1.95324611663818
-0.0724173337221146 0.0277336575090885
0.199212253093719 -0.155794009566307
-0.605550825595856 0.389542698860168
-0.802932381629944 -0.294895082712173
-0.0537139400839806 0.303327143192291
-0.45411342382431 1.16019535064697
-0.161843702197075 -0.183337673544884
-0.193402722477913 -0.984451174736023
0.0828443691134453 0.90637594461441
-0.201909497380257 0.794974505901337
-0.404128164052963 -0.757219016551971
0.0138911176472902 0.187594309449196
0.210427224636078 -0.221200734376907
-0.586313962936401 -1.0747686624527
0.323500156402588 -1.26285195350647
0.428309202194214 -1.81979501247406
0.747716188430786 -1.40541207790375
0.42506343126297 -1.57730734348297
-0.142070829868317 0.364210605621338
0.167429596185684 -0.577896535396576
-0.0837360024452209 0.528510928153992
0.437937647104263 1.61180555820465
0.131282299757004 -0.954927802085876
0.435597389936447 1.30095756053925
-0.519498527050018 -1.46180295944214
0.598455309867859 0.395831048488617
0.644530713558197 0.276147365570068
0.252421408891678 -1.44324851036072
0.092794768512249 -0.656690061092377
0.254938900470734 -0.211875319480896
-0.285441875457764 -0.00541956815868616
-0.157615438103676 -1.74036455154419
1.03394830226898 0.400252550840378
0.0700649544596672 -0.131948783993721
-0.129703655838966 0.921983897686005
-1.21148252487183 -1.03063356876373
-0.102853894233704 -0.332851648330688
0.0412745997309685 0.64475953578949
0.670407295227051 -1.40270400047302
-0.236151322722435 -0.952521920204163
-1.27066159248352 0.111017309129238
-0.384857088327408 -0.466173857450485
-0.439693808555603 -0.177247032523155
-0.285995781421661 -0.420738130807877
-0.375573635101318 1.45781826972961
0.282957494258881 -0.947407782077789
0.38278466463089 0.607802450656891
-0.626194357872009 0.185398831963539
-0.0442238226532936 0.409554570913315
-0.00320883840322495 1.58007884025574
-0.0267183762043715 0.422381460666656
0.229995638132095 2.06284594535828
0.110018737614155 1.08762645721436
0.322855532169342 0.952305018901825
1.01562833786011 -0.793533802032471
-0.720367431640625 0.304464638233185
-0.0271745380014181 2.76215410232544
-0.1709905564785 0.154836729168892
-0.144925355911255 0.266252785921097
-0.528935372829437 -0.44194084405899
0.33173131942749 0.455230593681335
0.0641221329569817 0.946252405643463
-0.0466797575354576 -0.481921970844269
0.437022835016251 -0.812339842319489
0.677776157855988 -0.163982465863228
0.573193848133087 0.909170031547546
-0.0224277731031179 -0.484893977642059
-0.0656358599662781 -0.0233160834759474
-0.298742920160294 0.848898649215698
0.160579785704613 -0.340528458356857
0.762186706066132 0.59116393327713
-0.644855737686157 -0.870492577552795
-0.254019230604172 -0.989501953125
0.203137069940567 -1.15709018707275
0.324753224849701 -0.265374779701233
1.27979457378387 -0.0651518926024437
-0.56543356180191 0.11485331505537
0.605926990509033 0.657912909984589
0.083978533744812 -0.535389363765717
-0.0989612936973572 0.251723796129227
-0.132263794541359 0.904126822948456
-0.234232246875763 0.15665340423584
-0.424999713897705 -0.115583814680576
0.0686769112944603 -0.201047882437706
0.181576550006866 -0.142385736107826
0.636486828327179 -0.160317465662956
-1.23120844364166 0.511485040187836
0.134423106908798 -0.516790211200714
0.6872438788414 1.69422876834869
0.245384603738785 -0.685644388198853
0.557510316371918 0.416386544704437
-0.404971331357956 0.197772920131683
-0.632099032402039 0.106409460306168
-0.0533213317394257 -0.159166514873505
0.530197858810425 0.232151329517365
-0.0381322577595711 0.943319797515869
-0.068201020359993 -0.0269983448088169
0.984430551528931 0.289618313312531
-0.363280653953552 -0.934313774108887
0.150734007358551 0.28840634226799
0.350942254066467 0.408984214067459
-0.283449560403824 2.14044404029846
0.0111742205917835 -1.43353796005249
0.305545181035995 -0.397177368402481
-0.115858860313892 0.784409940242767
-0.192159697413445 -2.13367366790771
-0.427392870187759 0.0977010875940323
-0.0977699384093285 0.474836140871048
0.135136917233467 -0.330864369869232
0.786367058753967 -0.520375430583954
0.00559025118127465 1.69653928279877
-0.266069531440735 0.461225271224976
-0.0787711590528488 -0.278845578432083
-1.00460052490234 -0.241034060716629
-0.453863978385925 1.18837106227875
-0.856699407100677 0.753308475017548
-0.584450364112854 -0.42626816034317
-0.215457394719124 -0.444781243801117
0.250689893960953 -0.0575352646410465
-0.584800660610199 0.000558003783226013
-0.435954719781876 1.17560577392578
0.240618750452995 0.596209168434143
0.447469800710678 1.41972255706787
-0.0213959012180567 1.36599493026733
-0.0148346871137619 1.16044545173645
-0.261139124631882 0.776496946811676
0.547770798206329 -1.34436869621277
1.11430764198303 -0.631532967090607
0.127185508608818 -2.1904821395874
0.686796307563782 2.00100421905518
-0.778736293315887 0.895239949226379
-0.345302700996399 0.206191539764404
0.745427846908569 0.00876813102513552
-0.471587598323822 -1.35355615615845
0.713308870792389 0.306678205728531
0.203826695680618 0.939300179481506
0.0367462635040283 -0.0175422988831997
0.180128708481789 -0.338037669658661
-0.0907652601599693 0.858162939548492
0.56504499912262 0.960191011428833
0.281558007001877 0.466685593128204
-0.335161864757538 0.824001729488373
0.612388908863068 -0.838022232055664
-0.0167209059000015 1.33082294464111
-0.0312530174851418 0.0189874172210693
0.129471078515053 -0.461117029190063
-0.546547472476959 1.35189473628998
0.708627045154572 -1.58391332626343
0.353179395198822 1.26545631885529
0.0188657213002443 -0.107742831110954
-0.286817967891693 0.250427842140198
0.175803482532501 0.837817788124084
-0.165412113070488 0.61686635017395
-0.646346211433411 1.52568972110748
-0.190892159938812 0.658865034580231
0.541194021701813 -1.24316906929016
0.490746051073074 0.0759223103523254
0.0948193967342377 -0.811315715312958
-0.464979290962219 0.211878046393394
-0.064383864402771 -0.783117651939392
0.338353753089905 -0.0548658221960068
0.0755851939320564 -0.273050516843796
-0.330310046672821 0.357647299766541
0.659933626651764 -0.0149527303874493
0.650523126125336 0.545330822467804
0.411374092102051 0.834567904472351
0.346448093652725 -1.49330949783325
-0.160444959998131 -0.552176773548126
0.241463467478752 0.906867206096649
-0.719294726848602 -1.10560381412506
-0.660004436969757 -0.815756142139435
0.180837005376816 0.591035783290863
0.117503561079502 1.76439428329468
-0.303358316421509 -0.333091735839844
1.07561552524567 -0.669631958007812
-0.175522640347481 0.401332825422287
-0.485080391168594 0.553204417228699
-0.122553832828999 0.663258910179138
0.0400053933262825 -1.52985656261444
-0.0284175109118223 0.0408494137227535
-0.187122315168381 0.313567757606506
-0.0679563209414482 -0.484676092863083
-0.16929604113102 1.00295078754425
-0.246121823787689 0.922323822975159
0.248540058732033 -0.910690784454346
0.245903924107552 0.678545653820038
-0.318965077400208 0.0302516333758831
0.619074583053589 1.45573687553406
-0.525003552436829 0.662692129611969
-0.497837483882904 -0.0226847492158413
0.394200801849365 0.775008261203766
-0.415706634521484 -0.189017847180367
0.277465671300888 0.0964198261499405
0.0106014534831047 0.634235560894012
0.331816136837006 -1.00730967521667
0.62148255109787 1.37979209423065
0.684632956981659 -1.81608724594116
-0.228024914860725 -0.583227217197418
0.906340837478638 0.41221022605896
0.646985530853271 0.944858253002167
-0.403419852256775 -0.056922797113657
0.240345865488052 0.891734719276428
0.702055811882019 0.626114666461945
0.111974887549877 0.196421667933464
0.46400973200798 -0.773669183254242
-1.00884258747101 -0.58895605802536
-0.0817721486091614 -0.0744014903903008
-0.285251051187515 0.311247557401657
0.174660474061966 -2.82923555374146
-0.514356970787048 1.36832165718079
0.70225203037262 0.354150235652924
-0.112049758434296 0.543903052806854
-0.330611556768417 1.30943691730499
-0.21798612177372 -2.75417494773865
-0.303915083408356 1.14930689334869
-0.438586741685867 -0.362019270658493
0.940338492393494 -0.0236987471580505
0.528337717056274 -0.569113671779633
-0.323922395706177 0.559941828250885
0.599522709846497 -0.488104611635208
0.5250164270401 0.59022068977356
-0.276383012533188 -1.60848760604858
0.338006138801575 0.358707636594772
0.0741324946284294 -0.0938104838132858
-0.0556068122386932 0.815526187419891
1.02324712276459 0.592266917228699
-0.504326105117798 0.951576471328735
0.969461858272552 -0.0131994131952524
0.0252781584858894 -0.279931873083115
0.11735861748457 0.334852606058121
-0.134609550237656 -0.341107428073883
0.374288469552994 -1.5988929271698
-1.01112031936646 -1.53414690494537
-0.150164589285851 -0.355843812227249
0.0202107392251492 -2.07725620269775
-0.274894237518311 -0.606367588043213
0.569229304790497 1.09560537338257
-0.471546322107315 -1.49701678752899
-0.302925795316696 0.459733754396439
0.977423369884491 -0.494511425495148
-0.101704619824886 0.794635474681854
0.0342124924063683 2.74159955978394
0.222345739603043 -0.432972729206085
-0.209930658340454 0.725732088088989
0.973041176795959 -1.07917475700378
0.165763437747955 0.258943259716034
0.000394237227737904 0.0331375226378441
-0.17795230448246 -0.262397468090057
-0.498890399932861 0.74134224653244
0.708937704563141 -0.95233553647995
-0.0978059247136116 0.200228601694107
-0.207511633634567 -0.147842556238174
0.688190102577209 -0.29337266087532
0.426340281963348 0.713450849056244
0.392722457647324 0.36246982216835
0.410511493682861 -0.587896168231964
-0.926966190338135 -0.743907749652863
-0.456991195678711 -1.70249056816101
0.417839229106903 0.252985149621964
-0.0543734505772591 -1.0406801700592
0.666806817054749 0.288608729839325
0.073506273329258 2.41607069969177
0.534820020198822 -0.0902773067355156
0.00195351056754589 1.19615018367767
0.288134008646011 0.527588486671448
0.582319557666779 -0.507989943027496
-0.438488125801086 0.565995991230011
0.483670622110367 -0.619857311248779
-0.230698436498642 2.25652360916138
-0.000104799866676331 0.404202163219452
0.752601861953735 1.07402908802032
0.315763056278229 -1.3131730556488
0.136320978403091 0.848151683807373
0.24839161336422 -0.169604226946831
0.888885676860809 -1.28467202186584
-0.00796017423272133 -0.0973682031035423
0.667397260665894 -0.760050714015961
0.484763920307159 -0.100987911224365
0.26430332660675 0.284867167472839
0.472805291414261 -0.957807540893555
-0.648347079753876 -0.318642646074295
-0.0867813304066658 -1.66502547264099
-0.165929049253464 0.561630308628082
-0.294535905122757 0.211343258619308
-0.532905757427216 -0.611888885498047
1.21044111251831 0.571992576122284
0.19922748208046 -1.09678530693054
-0.331315785646439 1.8103346824646
-1.11788666248322 0.571492731571198
-0.863346219062805 -0.0440778471529484
0.305197507143021 0.33001896739006
-0.0559971705079079 -0.85843813419342
1.26003849506378 -0.638274490833282
-0.31436026096344 1.29343724250793
-0.511637032032013 0.962831020355225
-0.321393370628357 1.99623811244965
0.0126065537333488 -0.929158926010132
-0.563624918460846 0.500435709953308
0.394958823919296 -0.608692705631256
0.734332144260406 -0.772867977619171
-0.514796733856201 0.603150367736816
0.46857613325119 -0.98883581161499
-0.145577982068062 -0.919516563415527
0.345702797174454 0.449237495660782
0.173899590969086 0.299736738204956
-0.548692882061005 0.703557431697845
0.0276991687715054 1.47815132141113
-0.195481479167938 0.359091311693192
-0.28009757399559 1.84886038303375
0.0501821711659431 -1.36642754077911
-0.213413536548615 -0.404309540987015
-0.452710539102554 0.19119781255722
0.192890882492065 -1.13059198856354
0.288933843374252 -2.23685359954834
-0.53496903181076 0.0502685606479645
0.772973120212555 0.265456944704056
-0.457438170909882 0.226134434342384
0.618785560131073 -0.0508877597749233
0.388500720262527 -1.38263952732086
-0.270381778478622 -1.19480311870575
0.641117334365845 -0.234734162688255
0.203426569700241 -1.07493388652802
-0.511757016181946 -0.243839383125305
-0.103391617536545 -1.14762258529663
-0.549040794372559 -0.548892557621002
0.105740450322628 -0.427921950817108
0.0354222767055035 -0.692660331726074
0.667822241783142 1.95714485645294
0.20597043633461 -0.551610231399536
-0.436337292194366 -0.575709104537964
0.135209128260612 -0.373841494321823
-0.87722784280777 -0.135785654187202
-0.653342485427856 0.0371229611337185
-0.341550707817078 1.45037972927094
0.158195808529854 0.0676418021321297
0.541062831878662 0.951831042766571
0.829890966415405 -1.07902693748474
0.506873667240143 0.601711928844452
-0.37165156006813 0.07340457290411
-0.317253857851028 -0.690307378768921
-0.583475530147552 -1.56511056423187
-0.114826180040836 1.31132209300995
0.799896717071533 -0.503212153911591
-0.0618152916431427 1.72411406040192
-1.05779099464417 -0.755873739719391
0.102944195270538 -0.0339034646749496
0.756955087184906 -1.48400294780731
-0.381146043539047 0.427247554063797
-0.0230921003967524 -0.690683007240295
-0.19327487051487 -0.999532222747803
0.327413946390152 2.28828310966492
-0.521215856075287 -1.49949610233307
0.270898252725601 -0.92582243680954
-0.158293381333351 -0.453453809022903
0.55867999792099 0.204662397503853
-0.890434384346008 1.08774209022522
-0.392706304788589 1.12640035152435
0.712165892124176 2.04796004295349
-0.182613030076027 0.0637801811099052
-0.867900490760803 -0.121422916650772
0.0905497446656227 0.62978720664978
0.188130214810371 -0.592325031757355
0.891830742359161 1.58674216270447
-0.473509013652802 -0.874300420284271
0.178724572062492 -0.40550309419632
0.390478789806366 1.60252726078033
-0.670278251171112 1.18921184539795
0.146810472011566 0.373293489217758
0.170862764120102 -0.620822131633759
-0.365393847227097 -1.6045835018158
-0.263803392648697 0.426916122436523
0.138422101736069 -0.0369732864201069
0.16288922727108 0.515168726444244
-0.434155285358429 1.42664384841919
0.489872664213181 -0.280445426702499
0.873642385005951 1.70112586021423
-0.300760388374329 -0.0445263460278511
-0.195557728409767 1.46627688407898
-0.151058539748192 0.631919503211975
-0.630524039268494 -0.352428525686264
0.630866050720215 0.518120169639587
0.316063046455383 2.15081715583801
0.381195425987244 -1.14036667346954
-0.591614723205566 -0.559087991714478
-0.0415633842349052 0.605741024017334
-0.233691692352295 -0.020534735172987
-0.300468236207962 -0.285210907459259
0.27214440703392 0.33832049369812
0.388300150632858 0.0298510789871216
0.799264907836914 -0.586758613586426
0.511246681213379 -0.592223227024078
0.544405877590179 -0.564621806144714
0.175681993365288 0.70888888835907
0.770298480987549 0.798755347728729
0.42071059346199 0.502763688564301
-0.424761295318604 -0.262871354818344
0.273988097906113 1.12100338935852
-0.180258095264435 -0.524747371673584
-0.064282514154911 0.0539254248142242
-0.276162892580032 -0.197374016046524
0.40672567486763 1.54814076423645
0.259269207715988 0.359300881624222
-0.226143389940262 -1.54609882831573
-0.615901052951813 -0.561764359474182
0.392098516225815 -1.4404205083847
-0.439288109540939 0.224611476063728
0.240605741739273 -1.77873182296753
-0.199409246444702 1.05074846744537
0.833505392074585 -0.563669919967651
-0.655226171016693 -0.415269941091537
-0.998900592327118 -0.350998282432556
-0.0831665322184563 -1.9256626367569
-0.177219748497009 0.524234056472778
0.281198024749756 0.957647085189819
-0.481058448553085 -1.76581752300262
-0.346678346395493 -0.499386489391327
-0.329728662967682 1.31578922271729
-0.303556025028229 -0.658225655555725
0.0175664592534304 -0.995684325695038
0.0137377865612507 1.20799469947815
0.139926046133041 1.78518414497375
0.172031566500664 -0.795713484287262
0.610204994678497 -0.937279343605042
0.771518230438232 0.964964866638184
0.241975098848343 -0.0525078736245632
0.404970228672028 0.50460159778595
0.78107625246048 -0.0544944070279598
0.692494571208954 0.563907146453857
-0.379067540168762 0.914810180664062
0.226900935173035 -0.14068116247654
0.560209810733795 -0.627881169319153
0.42904669046402 -2.18110680580139
0.572510778903961 0.934749901294708
-0.261261910200119 -0.763875305652618
-0.413362592458725 1.6015373468399
0.432914435863495 0.37812140583992
-0.111619964241982 -0.959616720676422
0.171873152256012 -1.58015036582947
-0.669601619243622 -0.128357380628586
0.66908860206604 -0.473271876573563
-0.0482932478189468 0.134291991591454
-0.483276158571243 -1.00462830066681
0.332062095403671 -0.982654869556427
0.672559082508087 -0.295356065034866
-0.420113116502762 -0.420797079801559
0.0269302912056446 0.0862053260207176
0.198677778244019 0.220279559493065
0.228806138038635 1.05576014518738
0.320568859577179 -0.549534976482391
-0.216686680912971 -0.398627549409866
0.132285237312317 -0.113975815474987
0.644296824932098 0.557871758937836
-0.15070104598999 -1.75529766082764
-0.167040273547173 -0.459921091794968
-0.439788937568665 0.2893907725811
-0.353584438562393 1.06081128120422
0.0480611100792885 0.881737649440765
-0.0156612154096365 -0.384575068950653
0.234330952167511 -0.406988590955734
-0.366195321083069 -1.72698402404785
-0.571181893348694 -0.896619617938995
0.256369471549988 -1.72752368450165
0.471145451068878 -1.12570095062256
0.52869439125061 -0.565436184406281
-0.158062756061554 -0.445673316717148
0.249948799610138 1.07049489021301
-0.24338361620903 -0.0824973955750465
0.646476209163666 -0.0145925283432007
0.121464475989342 1.86231768131256
0.146307706832886 0.837250053882599
-0.163886234164238 0.72828084230423
-0.0276799444109201 0.454842388629913
};


==> figures/visualizations/funnel/pis_samples.tex <==
\addplot [semithick, pis, opacity=0.7, mark=x, mark size=3, mark options={solid}, only marks]
table {%
3.29951763153076 -0.0561203956604004
0.754003167152405 -0.452847570180893
1.65965211391449 1.78506624698639
-0.394728302955627 0.802358865737915
0.290246278047562 -1.49904823303223
1.50004529953003 1.65964019298553
3.39098215103149 -2.98015713691711
2.44423317909241 -0.505376279354095
-0.289761990308762 -0.877671122550964
0.639561176300049 4.63085508346558
2.88305497169495 -0.928755939006805
0.899044036865234 0.626598477363586
3.28491306304932 -13.7130432128906
2.32293653488159 3.92975568771362
3.36500382423401 -0.816571354866028
3.43295407295227 0.863197565078735
0.554185628890991 0.0340208187699318
-1.55885100364685 -0.606861472129822
0.861290216445923 -0.242462038993835
-0.297426998615265 0.815077602863312
2.50920557975769 -0.104326389729977
0.592899560928345 -0.578023076057434
1.29195618629456 -0.207999706268311
-0.000853220000863075 -0.149580895900726
-0.584116399288177 0.353621125221252
-1.1796760559082 -0.0529404431581497
3.36508703231812 -0.0630086809396744
0.869214236736298 -0.262412071228027
0.634679675102234 2.91266894340515
2.15513849258423 0.379931151866913
1.64215648174286 1.50098347663879
-0.777588546276093 0.264527916908264
-1.69786238670349 -0.693560123443604
1.41890776157379 2.7274055480957
0.467322289943695 0.92508339881897
1.71973955631256 -0.58357310295105
-1.23569297790527 -0.190688952803612
-2.62545704841614 -0.124798566102982
-0.813055276870728 -1.76814687252045
1.5470118522644 -1.27470886707306
0.93868762254715 0.320212870836258
0.642551958560944 0.266536295413971
0.757329523563385 0.994146883487701
0.638802289962769 1.88571631908417
0.426775634288788 -0.948242843151093
0.879703760147095 -1.68409252166748
-1.71801340579987 0.237589001655579
-0.854092836380005 -0.361733973026276
2.01880383491516 -5.98267316818237
-0.19280418753624 0.10968990623951
2.6542854309082 -2.69515824317932
-0.355660170316696 0.510751187801361
0.165744796395302 1.3293673992157
1.57267439365387 -2.23537349700928
0.425531983375549 0.542692184448242
2.8817617893219 3.16490006446838
2.47020101547241 -3.29998111724854
-2.00203061103821 0.164705365896225
-0.736216604709625 1.11719501018524
3.27524924278259 -0.883557558059692
-0.113080039620399 -1.44261574745178
-0.332456827163696 -1.40672993659973
1.92726910114288 0.562055110931396
-0.911401510238647 0.30148583650589
-2.09435606002808 -0.105987265706062
-0.543519198894501 -1.76606011390686
3.81273508071899 -4.12666940689087
-0.546624481678009 -0.23498123884201
0.392913222312927 -0.204735338687897
-0.804236233234406 -0.244632035493851
0.623587429523468 -0.904788374900818
-0.360309630632401 0.425266414880753
1.5606861114502 -0.743305087089539
0.445435494184494 2.12440371513367
-0.408464223146439 -1.48233330249786
0.0862243920564651 0.638237416744232
-0.866319417953491 0.261731743812561
0.671790897846222 0.431165426969528
1.35204684734344 -2.22662019729614
-0.0399519503116608 0.188872486352921
3.59945392608643 6.46924257278442
-1.64400792121887 -0.702652096748352
0.924720942974091 -2.295569896698
1.96419358253479 -0.966148138046265
-2.26304197311401 0.0247820615768433
1.20694291591644 1.47015810012817
2.2472198009491 1.25044906139374
1.48773002624512 -2.6356201171875
0.161491826176643 0.10062375664711
-0.246016621589661 0.685296416282654
2.06259250640869 -4.42295455932617
3.00518822669983 1.34914445877075
-1.14765286445618 0.566728591918945
2.3860399723053 -1.82792258262634
1.43034267425537 1.53132176399231
-0.0643611252307892 0.507315039634705
2.35661792755127 2.5604419708252
2.98256635665894 -1.31491911411285
-1.73075246810913 0.0573831796646118
-1.608402967453 0.199191614985466
2.6157238483429 4.32910680770874
0.94081437587738 -0.60003936290741
-0.743478894233704 0.225849613547325
0.0430088713765144 -0.00428169965744019
1.43513762950897 3.59549999237061
3.49224185943604 12.6542310714722
-0.923831284046173 0.382038116455078
-0.447585254907608 0.17633056640625
-0.361385822296143 -1.04660046100616
0.103575959801674 -0.011157363653183
-0.588313639163971 0.668550252914429
-0.214449554681778 0.201161965727806
2.44123458862305 4.99840688705444
-2.30691075325012 0.784502387046814
1.47286105155945 -4.91423654556274
1.47159039974213 -1.76556277275085
-3.48318529129028 0.601611316204071
-0.505493402481079 -0.101095527410507
0.705801725387573 -0.0988351330161095
1.47319221496582 5.49526977539062
0.792574524879456 -1.20552492141724
3.24207067489624 4.4497218132019
-1.45918035507202 0.132986381649971
-0.0829196572303772 -0.651500880718231
-0.564175486564636 -0.670670330524445
1.13762092590332 -0.000507503747940063
-0.49388587474823 0.397217720746994
2.1410596370697 -0.860161781311035
0.104982390999794 2.88789367675781
0.523309588432312 0.464373171329498
2.49025416374207 -4.50543642044067
-1.58080041408539 -0.0311333723366261
4.49493217468262 11.7440805435181
2.73759317398071 -2.05471730232239
1.31011509895325 0.900326669216156
0.134745538234711 0.337554663419724
0.386867165565491 -0.179171711206436
3.99571466445923 -11.1876859664917
0.932453989982605 2.89005565643311
-2.82786464691162 -0.164656162261963
-0.722531795501709 0.316741466522217
2.12943077087402 0.566268980503082
3.44351649284363 -8.73969650268555
1.83806538581848 1.47925543785095
0.422970592975616 -0.318457096815109
0.899982571601868 1.03800868988037
-0.30236092209816 0.152273565530777
-1.15765798091888 -0.175319373607635
0.704881072044373 1.18520629405975
-0.292207628488541 0.740947961807251
2.4316930770874 1.78998076915741
2.41058802604675 -0.465162515640259
0.324228584766388 0.64666748046875
-0.732922554016113 -0.0533311814069748
1.10430419445038 2.31094789505005
0.529760777950287 1.10544168949127
-0.528437435626984 -0.539441704750061
-0.94166362285614 -0.269164621829987
4.21629333496094 -6.87922525405884
0.0233477652072906 1.63258421421051
1.18373644351959 1.95148098468781
0.618828415870667 -0.155303090810776
-0.0642449259757996 0.379794090986252
2.67207860946655 -0.980277597904205
0.422615855932236 2.19136762619019
2.3273561000824 -1.23996686935425
2.07408952713013 -0.61826890707016
-0.26959627866745 0.663777351379395
-0.977705955505371 -0.11451356112957
2.04220366477966 0.953714430332184
-0.443982690572739 0.155294597148895
1.9535539150238 2.82871651649475
3.0996310710907 -0.270046681165695
-1.43664360046387 0.0646147429943085
-0.983056843280792 0.219942465424538
-0.303772449493408 -0.0461904257535934
1.42783606052399 -4.18005657196045
-1.77008152008057 0.528010368347168
2.55511665344238 -2.03146123886108
2.1904239654541 -3.19281363487244
2.32663345336914 1.32559895515442
2.85409927368164 -1.12601935863495
1.50349712371826 0.1272973716259
2.7641806602478 -6.08615064620972
-1.24728572368622 0.720549643039703
3.61004018783569 1.76042330265045
2.25947427749634 3.5115659236908
2.52245807647705 -0.490907967090607
-1.92104613780975 -0.397128969430923
2.04036736488342 1.91323804855347
-0.751812994480133 -0.330485194921494
-0.209099978208542 -0.689216017723083
3.2877082824707 -1.03815603256226
1.04701292514801 3.77651119232178
-0.0582004487514496 1.12485837936401
0.0102411061525345 -2.13406229019165
1.17232882976532 1.57393395900726
0.743403911590576 0.0458642840385437
1.20684480667114 -0.931937694549561
2.61649298667908 -7.70182657241821
1.03356862068176 3.53019618988037
1.50582766532898 -2.42194318771362
3.4439799785614 9.41680908203125
2.15481877326965 2.08393931388855
-0.361589670181274 0.623858451843262
4.59778118133545 3.47822642326355
0.450035899877548 -1.2966456413269
3.52134776115417 0.656624853610992
-0.482675790786743 0.301144480705261
0.67613160610199 -0.157566487789154
0.700501382350922 0.186315834522247
0.808417081832886 1.25203251838684
-0.694107532501221 -0.869590520858765
-0.422554939985275 -1.2621853351593
-0.330759614706039 0.927814960479736
-2.0655312538147 -0.103319734334946
3.00682139396667 -7.31004905700684
-2.20577526092529 -0.383368760347366
2.46782183647156 1.4190080165863
0.908037722110748 -1.0027402639389
-0.432545691728592 0.156539604067802
3.06868076324463 5.83095741271973
-0.725655198097229 0.499135941267014
3.27721548080444 -4.29721117019653
-0.36617523431778 -0.305500864982605
0.953565061092377 0.874832928180695
2.80896329879761 10.0326433181763
3.85041236877441 -3.28030800819397
-1.83823907375336 -0.0485454499721527
2.1823251247406 -3.6405656337738
0.563549399375916 2.0346782207489
1.70899975299835 3.21223616600037
2.65451622009277 -2.94449663162231
2.21900987625122 3.88758230209351
-1.71249055862427 0.114330887794495
2.08566689491272 1.61904847621918
1.30339348316193 -0.373808771371841
0.820446968078613 -0.0792306736111641
-0.716576218605042 -0.708295047283173
2.27146649360657 1.00725328922272
1.06894516944885 -0.281281471252441
-0.29898139834404 1.30818426609039
2.86063456535339 -4.18691873550415
0.438617169857025 0.365087926387787
-1.86307287216187 -0.201890453696251
1.03425741195679 -1.09252405166626
2.74691653251648 3.54883480072021
1.90668129920959 -1.56639897823334
1.04865682125092 -1.38025033473969
-1.60138726234436 -0.513387739658356
0.251066207885742 0.597276329994202
-2.04986667633057 -0.0114398598670959
-1.13499999046326 -0.595048487186432
2.51394104957581 1.69020986557007
3.16272497177124 -0.160727947950363
-1.56232368946075 0.648964583873749
0.740070343017578 0.573606491088867
-0.576177537441254 1.09688436985016
0.803332090377808 1.20576524734497
2.10607671737671 -0.174496650695801
-0.139218479394913 -0.0943543612957001
-0.514136254787445 0.0515540316700935
-0.364772975444794 0.882773518562317
2.81034278869629 -3.32766151428223
1.13816726207733 -2.35827088356018
2.29116177558899 -1.00276017189026
2.49185562133789 0.267797857522964
-0.89271605014801 0.110638588666916
-0.259972333908081 -0.468460440635681
3.93505430221558 13.5849533081055
-0.333700180053711 -0.829335570335388
-0.607339143753052 1.36981177330017
-0.133273541927338 0.0957121998071671
-0.934531688690186 0.627560496330261
-0.325403451919556 -0.757298529148102
0.0536734312772751 0.598144233226776
0.00317806005477905 0.222709327936172
1.7508385181427 -6.13436126708984
-1.33686351776123 0.974984109401703
-1.53426420688629 -0.0756918340921402
1.55373537540436 0.749814331531525
-0.159708216786385 -0.93023669719696
2.81081104278564 -4.43255615234375
3.3561487197876 -7.376868724823
2.04178977012634 -0.811742782592773
0.0470906719565392 -2.05330610275269
-2.02828812599182 0.190370157361031
3.81661987304688 5.16035127639771
-1.26148009300232 0.248568892478943
0.449671685695648 0.0292305946350098
-0.400384366512299 -0.721924841403961
1.51273083686829 1.13357484340668
0.150735527276993 -0.550846695899963
-1.99525141716003 -0.370933204889297
2.74099230766296 1.42150497436523
2.22569155693054 1.08522582054138
-1.3506361246109 -1.56645703315735
0.906137824058533 2.49315404891968
0.709546446800232 1.13313341140747
1.48275065422058 -4.47703647613525
-0.176196113228798 -0.132160425186157
1.86386442184448 1.58604550361633
-0.555272281169891 -0.464567840099335
3.44905042648315 3.76475596427917
2.52596688270569 2.77732276916504
-0.0435010492801666 0.759529769420624
-2.2627694606781 -0.246105521917343
0.0712057948112488 1.24119997024536
0.688955843448639 -1.83808660507202
-0.359678208827972 -1.64226698875427
0.384939968585968 1.33681857585907
3.38826513290405 8.30726051330566
-0.778957724571228 -0.880209624767303
3.39801239967346 0.337734133005142
1.50397562980652 -0.72409200668335
-0.86000257730484 -0.332307666540146
2.83139634132385 -1.95180118083954
1.25300765037537 -1.01904094219208
-1.16301035881042 0.149280205368996
2.56039333343506 1.88023567199707
3.10489749908447 -3.04339861869812
-0.454715013504028 1.62680542469025
2.03038048744202 1.18138575553894
0.391072571277618 -0.119108363986015
-2.29937362670898 -0.291613787412643
1.73667359352112 -2.4310462474823
2.7675929069519 2.044837474823
-0.611310243606567 0.604979276657104
2.71296715736389 -1.17370617389679
1.7114200592041 -1.81570529937744
-0.819008827209473 0.232019156217575
-1.42430186271667 0.296034246683121
2.15062594413757 -0.308258295059204
1.51403617858887 1.54846394062042
1.55261361598969 -1.536700963974
-1.48959422111511 -0.869836807250977
-0.649868726730347 1.08051717281342
2.1897599697113 -2.14665484428406
1.85220348834991 -3.50897312164307
-1.68454217910767 -0.304955184459686
2.86169266700745 3.66455721855164
-1.99727833271027 -0.0476966798305511
0.406019300222397 -0.422125607728958
-1.3930584192276 -0.0254706144332886
0.0735370740294456 -0.867993295192719
1.1349995136261 -1.1294013261795
2.52776908874512 2.11442375183105
-0.576804220676422 -0.4486443400383
-1.49889969825745 -0.184406265616417
-0.0958475694060326 -1.45780622959137
-1.69847226142883 -0.394009292125702
-0.104422852396965 0.573459923267365
1.16729390621185 -0.975571632385254
2.85339140892029 0.860328197479248
1.37124717235565 1.55325543880463
3.1994366645813 -0.486496239900589
3.40710616111755 -0.705365002155304
2.62126088142395 2.3878870010376
1.09948003292084 -3.87342953681946
1.61295342445374 -0.737968802452087
0.288576990365982 1.72791159152985
0.619090974330902 0.0777541100978851
3.23896431922913 -2.893963098526
-0.271264255046844 -0.0840663611888885
1.1476263999939 1.45105278491974
-1.34501647949219 0.402855187654495
-1.71004152297974 0.140477433800697
3.55036664009094 4.23112964630127
2.93686032295227 7.09004926681519
1.72600030899048 -4.45451307296753
-0.328923165798187 1.00424337387085
2.8262038230896 -2.59931659698486
-0.965021848678589 -1.1106915473938
0.922006785869598 2.11476135253906
-2.29133152961731 0.839161574840546
-0.603603482246399 -0.284672647714615
1.89099907875061 0.326653301715851
-0.581195116043091 -1.40437388420105
1.81706357002258 -0.095561295747757
0.0780918896198273 -2.19910740852356
0.425808668136597 1.03335332870483
1.99266219139099 -0.931731224060059
-0.896804332733154 0.499084115028381
1.73822152614594 1.62901771068573
1.32468581199646 -0.0937966257333755
1.07314872741699 1.27468872070312
-1.15846955776215 0.257331401109695
2.57439136505127 -4.75888252258301
1.38460314273834 2.92256689071655
-1.45009517669678 -0.487201392650604
-1.22442758083344 0.382410138845444
0.245210081338882 -0.856859385967255
-2.03519892692566 -0.536972224712372
0.317813575267792 1.02601182460785
2.31335830688477 -0.862656354904175
-1.03394198417664 -0.468335270881653
1.28159308433533 -1.19004964828491
1.89583444595337 4.24591016769409
-0.938331842422485 1.23810875415802
1.25045728683472 -0.420341908931732
-1.34665071964264 -0.400862634181976
-0.399331033229828 0.452202618122101
1.18094849586487 2.45926213264465
1.13824617862701 -1.38465535640717
-1.33534741401672 -1.07331562042236
1.81731951236725 3.49002647399902
-1.01440441608429 0.447156578302383
0.621100902557373 2.62148404121399
1.11133456230164 -0.910189747810364
1.50027549266815 -0.00653535127639771
2.66635036468506 0.982753932476044
0.552979648113251 -0.60538113117218
1.3844712972641 1.62043654918671
2.38183045387268 1.37686145305634
-1.49535322189331 0.698406100273132
-0.0492715463042259 0.0175617784261703
1.37911736965179 -2.16943979263306
-1.71940183639526 -0.31152606010437
1.62273800373077 2.63056516647339
-1.48406863212585 -1.15093100070953
-0.250148564577103 1.06399655342102
2.92045068740845 0.922955393791199
0.775392770767212 0.650948345661163
-0.911133646965027 -1.01173639297485
2.72007870674133 2.60312914848328
0.214599743485451 -1.09736740589142
-1.35322630405426 -0.0444053113460541
3.34378623962402 7.70350646972656
1.20454299449921 4.6040678024292
-0.607112765312195 0.0036437064409256
1.16082763671875 1.42771983146667
1.44462370872498 0.293048501014709
-0.536240220069885 0.147655114531517
2.7652530670166 -3.79013013839722
1.43435966968536 3.02715396881104
0.692123651504517 0.283497780561447
3.79593992233276 6.10494899749756
1.52571201324463 1.54472160339355
2.96664333343506 -11.6615943908691
-0.428939312696457 1.18563139438629
1.67389678955078 1.94993197917938
2.10521602630615 -1.52360129356384
-0.784253776073456 0.173037499189377
-1.70458364486694 0.576970219612122
1.26261448860168 0.093109205365181
0.176232025027275 -0.172623574733734
3.08220410346985 2.32830452919006
-1.1350005865097 0.381052076816559
-0.876198530197144 -0.704956114292145
-1.06153464317322 -0.412951558828354
-1.33129715919495 1.02923691272736
1.24191665649414 -0.320623874664307
-0.490018397569656 1.41687703132629
-2.15125226974487 0.190742030739784
1.65656208992004 1.28947174549103
1.89305663108826 -0.513694643974304
-1.03810119628906 -0.183709233999252
-0.837185561656952 -0.154422640800476
-1.86713552474976 0.360305190086365
-0.643846213817596 -0.039003998041153
-1.91192245483398 -0.00674573332071304
2.18010377883911 -7.98481893539429
0.370287388563156 2.03767967224121
1.80196726322174 -3.19347143173218
0.264894247055054 1.10573291778564
2.89200735092163 4.27243041992188
-0.944255709648132 -0.325895190238953
-1.7644157409668 0.421983659267426
2.36371684074402 -6.45074701309204
2.1598904132843 6.0761981010437
0.983471155166626 -0.228497833013535
2.87155270576477 -0.298248618841171
2.38611221313477 0.0505869537591934
0.448443055152893 1.87650966644287
3.54021072387695 1.74408352375031
1.01506471633911 1.00349700450897
0.777597010135651 1.74358236789703
2.6316134929657 1.21877825260162
-1.05352520942688 -0.484708040952682
4.12153434753418 5.41094732284546
1.57042169570923 2.74155521392822
3.81605839729309 0.550523221492767
-1.52994418144226 0.3476602435112
2.11946535110474 -0.0488666035234928
1.48119056224823 -0.130133673548698
-0.333860605955124 0.845950305461884
2.47656989097595 -5.16302967071533
-1.62050259113312 -0.729322373867035
-1.30165231227875 0.459360003471375
0.83597457408905 0.0557405613362789
-0.934874832630157 -0.0855810344219208
1.88267767429352 -1.52191734313965
1.06568849086761 -1.10948169231415
2.79355096817017 -1.12820041179657
-0.32089164853096 1.22133469581604
2.43955421447754 2.5608823299408
-1.59306597709656 0.889907777309418
-1.30388855934143 0.0967599153518677
1.95808744430542 1.86413395404816
-1.72930181026459 -0.0498058199882507
-0.168951109051704 0.947260081768036
-1.09011971950531 -0.423157215118408
3.40865278244019 -1.11413431167603
3.12836241722107 1.7157621383667
3.23039627075195 -1.73231148719788
1.50883674621582 -1.65774989128113
0.385334551334381 0.924786925315857
-1.10038673877716 -1.00185477733612
0.758206784725189 1.50690543651581
1.95282292366028 2.6149845123291
0.290803879499435 2.59037303924561
-2.07442569732666 0.909876227378845
0.745892405509949 -2.18129539489746
-1.32862913608551 0.504541218280792
2.3562216758728 3.24710512161255
-0.0865519642829895 1.74485671520233
1.72642052173615 0.844459772109985
1.64215648174286 3.32033944129944
2.56671047210693 4.9987850189209
1.95098543167114 -0.767255961894989
2.32014274597168 4.21187782287598
2.08591747283936 6.20841884613037
2.24847340583801 1.40078449249268
1.21816182136536 0.346155345439911
0.543601155281067 1.40489542484283
0.533479690551758 0.28544420003891
0.2669937312603 -2.3892867565155
3.30569458007812 -0.52369898557663
1.51918041706085 1.93350183963776
0.138419479131699 -0.0173935927450657
0.46368333697319 0.445019572973251
-2.03891921043396 0.99354350566864
0.602810502052307 0.708864450454712
-0.523203372955322 1.68885457515717
0.48924708366394 1.89515280723572
0.758729338645935 -2.43385744094849
-0.255394577980042 -0.468212753534317
2.22824358940125 0.85002326965332
-1.99281787872314 -0.0925043523311615
-1.5032240152359 -0.582220315933228
-1.17207944393158 0.472810834646225
-0.387798696756363 -1.38408946990967
-0.985207319259644 0.907530546188354
2.38204669952393 -0.967753410339355
2.62313342094421 -0.911769509315491
1.01357650756836 -1.66371488571167
-2.48300671577454 -0.229589700698853
1.54865705966949 4.52303743362427
3.61118030548096 -9.64505481719971
-1.59452819824219 0.442669540643692
2.40315270423889 -0.377885729074478
0.615664005279541 -0.485926240682602
-1.39071822166443 -0.421962052583694
0.517403542995453 -1.13786923885345
3.4994330406189 2.24853014945984
3.04395246505737 -2.0993127822876
1.65287029743195 0.663455128669739
-2.99102354049683 -0.338265627622604
4.05639410018921 -9.28316116333008
3.55269527435303 -0.683168649673462
1.37041318416595 -0.233250200748444
0.623657464981079 -0.856278717517853
2.50887370109558 -2.30418729782104
-0.85780394077301 0.728995561599731
1.9666200876236 -0.0203702747821808
-1.08472347259521 0.041711837053299
1.12859559059143 -1.1902529001236
-1.56302523612976 0.0618959218263626
2.03994011878967 -4.91368532180786
-1.47523248195648 0.441136240959167
0.346545696258545 3.08856058120728
2.88785672187805 2.77570414543152
-0.515304207801819 -0.266032874584198
-1.43900942802429 -0.415101796388626
0.456177115440369 -2.04181790351868
0.170445337891579 -0.0998854041099548
1.67552554607391 -3.35241723060608
1.05638253688812 -1.2096962928772
-1.3970844745636 0.559439182281494
1.88232147693634 -0.990044593811035
-2.51724576950073 -0.103316158056259
-0.800463676452637 0.252841591835022
-1.44449937343597 -0.263128995895386
-2.28726243972778 0.812711179256439
1.80569171905518 -3.9092869758606
3.48033380508423 -2.78089570999146
-0.324048429727554 -0.282173871994019
3.63376975059509 3.54110980033875
2.91676092147827 4.10901689529419
0.36222705245018 1.70121574401855
1.49163722991943 -1.11659729480743
-0.78827965259552 0.967373073101044
-1.59896337985992 -0.55450576543808
-0.846850156784058 0.111551344394684
2.51759266853333 1.57181704044342
1.20407438278198 3.41747808456421
1.00789034366608 -2.81398582458496
2.04012084007263 -1.20326280593872
0.0456146895885468 -0.208792209625244
0.764528870582581 -1.55684816837311
-0.428169459104538 2.47356247901917
1.46926391124725 -1.21210432052612
3.65020155906677 -0.902617931365967
-1.82737290859222 -0.0353368297219276
2.46942448616028 -1.55675148963928
0.261221498250961 -1.56509292125702
0.367667496204376 1.14688968658447
2.86159896850586 -6.57579565048218
0.679048240184784 1.21340680122375
-0.303996413946152 0.378430247306824
1.66349506378174 0.06810063123703
3.38497543334961 1.35191452503204
2.44995212554932 -5.16542816162109
1.53537142276764 1.62222611904144
0.633814752101898 0.567505598068237
-0.0870423093438148 -0.292219460010529
-0.180767714977264 0.163617968559265
2.44234228134155 -3.60957145690918
-0.40273717045784 0.309725910425186
0.936436474323273 1.28401947021484
3.09361720085144 2.34886527061462
0.595118761062622 -1.38922023773193
0.785893857479095 0.0711496397852898
2.69227290153503 -3.95256972312927
1.60438644886017 1.31955969333649
0.907622814178467 -0.0978101268410683
0.868062317371368 0.11532174050808
-0.497285604476929 1.40365326404572
-1.07397270202637 0.338410079479218
2.24011993408203 1.80247473716736
-0.124255329370499 0.693459928035736
0.59686404466629 -0.832493722438812
-1.46419286727905 -0.311914175748825
3.20013546943665 0.801642775535583
-1.87424802780151 -0.338685125112534
1.14580118656158 -1.31768810749054
-0.776005029678345 -0.186925813555717
-0.860670566558838 -1.01294589042664
-1.9457403421402 -0.308222889900208
-0.0938969552516937 0.0247100442647934
0.457182645797729 -1.12797260284424
-0.259095579385757 -0.236899584531784
0.0524242669343948 -0.28540912270546
0.580835521221161 -1.62082695960999
0.792717754840851 1.29107570648193
-0.881212472915649 0.229161262512207
4.25941562652588 9.17699718475342
0.056058257818222 0.181064754724503
2.2871105670929 -0.819738805294037
0.347107619047165 0.112247429788113
-0.473987758159637 -1.71704173088074
2.25781655311584 -2.47128677368164
1.64782917499542 -2.39038395881653
-0.357985258102417 -1.43993449211121
1.42184221744537 0.893291592597961
0.261931926012039 -0.176943644881248
-0.803406357765198 0.0947988927364349
0.209696963429451 -0.718959867954254
2.49888324737549 3.66419816017151
-1.72362053394318 -0.0277507603168488
1.41992163658142 2.31409215927124
0.363116860389709 -1.20988643169403
0.97879683971405 -2.61541223526001
2.34905791282654 4.93488264083862
3.31499600410461 2.98776841163635
2.66446805000305 -3.1382942199707
2.22826194763184 -4.9483699798584
2.58518052101135 -3.35629773139954
0.473384618759155 0.676630198955536
3.08120608329773 -7.96520900726318
2.9448926448822 0.757124006748199
0.496238589286804 -2.191561460495
-2.02988815307617 0.153846263885498
-2.86003684997559 0.00534842908382416
0.0538237988948822 -1.15384101867676
0.769365668296814 1.1319831609726
0.112293004989624 0.165987953543663
-0.767328798770905 -0.526389598846436
2.85633778572083 4.61950492858887
-0.540574371814728 0.28743839263916
-0.884373605251312 -0.177107602357864
0.505193829536438 -0.169130176305771
3.58551406860352 -6.53304290771484
1.57906055450439 0.664269208908081
3.19978165626526 2.78733706474304
0.675550818443298 -0.926091849803925
1.30636525154114 -0.700192213058472
1.78047811985016 2.32496905326843
1.32477176189423 -0.368738114833832
2.34055924415588 5.40494775772095
1.78499269485474 2.79708433151245
1.05074155330658 -2.53217506408691
-2.3537073135376 -0.0162435621023178
-1.43840205669403 0.0472227185964584
1.91509020328522 -2.5669162273407
0.796711981296539 -1.67723548412323
-0.534615159034729 -0.543100297451019
1.06291627883911 0.207960531115532
0.356110751628876 -1.74907982349396
3.34090256690979 1.09961771965027
1.02943420410156 -0.56129515171051
0.277138531208038 -0.194465667009354
2.1038658618927 5.79835939407349
-1.94423878192902 -0.331139147281647
1.43766057491302 -1.23407733440399
-0.8430495262146 0.19976419210434
2.53243350982666 -2.27806568145752
-0.350705027580261 0.781268775463104
2.27277135848999 -5.11450910568237
0.954115629196167 1.2395156621933
2.72039079666138 -2.13660645484924
-1.20483613014221 -0.136634796857834
0.625204980373383 -1.11317443847656
-0.306131482124329 0.121282666921616
1.56266474723816 -1.33534586429596
1.68099653720856 2.84124422073364
3.08353304862976 -5.04751920700073
0.910956025123596 3.32510900497437
2.28766512870789 1.98794794082642
0.455797672271729 -1.07471072673798
2.5468635559082 -3.98138356208801
2.86930561065674 2.67662477493286
1.31489872932434 -1.62875580787659
0.848257839679718 1.59638130664825
-0.334153473377228 0.780697107315063
0.0900640189647675 1.50864279270172
0.116203285753727 0.261468827724457
1.49842464923859 1.31106340885162
0.620739042758942 1.86795115470886
-0.193640649318695 1.32719933986664
-0.378031224012375 -0.616541087627411
2.15460228919983 -3.11247873306274
3.39845681190491 -2.84314846992493
2.69265532493591 -11.1881456375122
-1.55733907222748 -0.18326473236084
-0.811657786369324 -1.10178172588348
-1.51697587966919 -0.509573459625244
-0.861413478851318 0.0124573707580566
-1.07901251316071 0.898024022579193
2.75881886482239 -3.66253542900085
0.0620925650000572 0.259069889783859
-0.304876208305359 0.290748745203018
-0.262968927621841 -0.524779081344604
1.43160915374756 -1.01158475875854
1.59649884700775 -1.20142781734467
-1.84073007106781 0.123308211565018
2.79587435722351 3.65926456451416
2.11663794517517 -0.80043089389801
3.44701194763184 -3.64452004432678
0.60577118396759 0.829164028167725
-0.38239997625351 -1.09361302852631
2.87482666969299 3.54224133491516
-0.757981181144714 -0.371989637613297
3.25880861282349 3.07351326942444
4.06760215759277 -2.98552823066711
3.11411929130554 6.21019601821899
0.187492534518242 -0.213941395282745
1.40298104286194 -0.0915823876857758
0.746461629867554 3.10187411308289
-1.94918239116669 0.555873692035675
1.29375874996185 0.00371956825256348
1.57330322265625 -2.65025973320007
2.2835681438446 3.36843919754028
0.714483201503754 -0.458634793758392
2.98521375656128 2.54814481735229
-1.13777506351471 0.565429925918579
-1.95026934146881 -0.624831736087799
2.04863452911377 3.46587681770325
-1.20028293132782 -0.229736462235451
-0.967204928398132 -0.0921246111392975
-0.561706304550171 0.923978328704834
2.12176418304443 1.47227716445923
-1.86309123039246 0.0786624401807785
1.85567593574524 1.12936818599701
1.22234308719635 2.49109768867493
-2.21761870384216 -0.506524264812469
-1.52009510993958 -0.190481200814247
0.476102143526077 0.408968061208725
2.7537260055542 -1.55945765972137
-2.04211783409119 -0.0560384877026081
0.00570207834243774 -0.666250705718994
3.18097829818726 5.65797805786133
2.19851160049438 -4.50754642486572
0.121910214424133 -2.41306018829346
1.31546378135681 -0.51877099275589
-0.31311959028244 1.02625644207001
0.386455446481705 -0.348734617233276
-1.4988055229187 -0.670387983322144
-0.98477840423584 0.593392312526703
0.0668376386165619 -0.80317348241806
1.04821813106537 -0.447651028633118
1.07973003387451 -0.413759261369705
0.803856015205383 -1.19374692440033
-0.662046253681183 0.447712808847427
-0.575091898441315 1.05381071567535
-1.22376668453217 1.04268407821655
0.579449117183685 -0.319450467824936
2.60453629493713 -9.7077693939209
0.861757040023804 0.203850328922272
-1.53946340084076 -0.582070291042328
0.351102232933044 -1.00946152210236
-2.72925043106079 0.140978708863258
0.998441934585571 0.0873604267835617
2.87689399719238 1.57168233394623
0.838964581489563 -0.939594686031342
1.85351765155792 -0.453177571296692
1.70636260509491 1.25061988830566
-0.419483780860901 -1.21625196933746
-2.57346796989441 0.444099962711334
0.487978458404541 -1.42416369915009
1.57110238075256 0.600413024425507
-2.13170838356018 0.439402848482132
-1.80141806602478 0.191194579005241
0.253181964159012 1.23027312755585
0.161297962069511 -0.562557756900787
-0.202652961015701 -0.84777045249939
-0.0274640023708344 -0.255179941654205
0.965416252613068 1.07772016525269
-1.58593857288361 -0.211312964558601
2.12076377868652 0.33776730298996
-1.03154540061951 -0.315671622753143
-0.059787429869175 0.681059241294861
-0.384516775608063 0.084837794303894
0.0637830570340157 0.224368914961815
-1.9513201713562 -0.596261382102966
0.706733047962189 -1.54475116729736
2.49046730995178 4.78124713897705
2.09102630615234 0.668353140354156
0.639715254306793 -0.277984440326691
-2.8706738948822 0.387522280216217
-0.703694581985474 -0.892783045768738
1.09797215461731 -2.13853192329407
1.49116706848145 1.94858300685883
1.24869418144226 1.83289766311646
-0.111607670783997 0.531991839408875
-0.551503777503967 -0.101674571633339
-0.018068939447403 1.49893975257874
0.559225499629974 0.791394114494324
-1.94529509544373 -0.0326091945171356
0.747952818870544 0.801204144954681
0.897249400615692 0.728591680526733
1.16018617153168 -0.0254896692931652
1.6402575969696 -1.35600531101227
-0.30938583612442 0.64628803730011
-1.68635582923889 0.629733085632324
3.93016386032104 -6.81061840057373
-0.00476247072219849 -0.338962614536285
-0.921051144599915 -0.575268745422363
3.40896558761597 7.06446027755737
0.749387860298157 0.862311840057373
3.3802170753479 5.06525421142578
-0.0468255653977394 0.970792531967163
-0.130770474672318 0.52617621421814
1.63219082355499 0.0247137136757374
1.49746668338776 1.57944405078888
1.56079304218292 -2.16509032249451
2.59660053253174 -0.819608449935913
0.0502149909734726 0.855323970317841
1.65809571743011 -2.81724810600281
-0.0639683306217194 1.12366318702698
3.20418167114258 3.19526982307434
0.856243550777435 2.43167161941528
1.93195533752441 -3.01566600799561
1.91673827171326 0.161119222640991
-1.12534213066101 0.393557101488113
1.63376152515411 1.31423711776733
1.71917176246643 3.79677844047546
0.721383333206177 -1.12658488750458
1.63722920417786 -0.0846397876739502
-0.363363236188889 -1.06525111198425
-2.65771746635437 0.536335468292236
1.17093968391418 0.765462636947632
-0.594628751277924 0.964816629886627
-1.75740921497345 0.47723376750946
-0.254464000463486 -0.762119472026825
1.30155563354492 -0.0185577068477869
-3.44034051895142 -0.0319965183734894
-2.9914128780365 0.141254454851151
-1.03570127487183 0.846395790576935
3.98314952850342 -0.862989187240601
0.555456399917603 -0.295950412750244
-0.0429048836231232 -1.3128297328949
2.38717126846313 -3.17924165725708
3.05899524688721 -5.62088966369629
2.80749702453613 6.55206680297852
-1.5628490447998 -0.22450315952301
-1.95859718322754 -0.26002448797226
1.01233720779419 -1.94518625736237
-1.96600520610809 -0.168881773948669
-0.865475058555603 -0.314840614795685
-1.15338754653931 -0.178675442934036
3.57203340530396 5.05096817016602
3.38920140266418 5.05248260498047
-0.261533111333847 -0.251850426197052
2.5615234375 2.5807044506073
-3.17844581604004 -0.333239734172821
1.3600264787674 0.219048976898193
2.42553853988647 -1.11979591846466
-0.439453601837158 0.666900992393494
0.426516443490982 1.57307183742523
2.34858155250549 -1.15663480758667
1.40657925605774 1.76678156852722
0.509778618812561 0.0556086674332619
-0.102602943778038 -0.617056310176849
-0.199664726853371 1.42566788196564
0.682084202766418 0.165770709514618
4.36341381072998 -3.09565401077271
-1.17093110084534 -0.670553147792816
-0.374783903360367 0.570004642009735
-0.390395253896713 1.40743625164032
1.0284583568573 1.79999756813049
1.84043002128601 -0.341918289661407
1.24259173870087 2.15283012390137
-1.83024501800537 -0.221044272184372
-0.773585915565491 -0.273186981678009
3.19702744483948 6.5911602973938
0.127882182598114 -0.340827286243439
0.937714517116547 -1.38053929805756
2.87604475021362 -1.85039114952087
-1.35565757751465 0.113000348210335
-0.8870929479599 0.333935678005219
-1.22404170036316 0.243381634354591
0.739710927009583 -0.662924766540527
1.32206106185913 0.256350368261337
3.05648994445801 1.08089518547058
-1.14268827438354 -0.277604281902313
-1.57534503936768 -0.0802768468856812
1.91750729084015 0.491491466760635
-0.266463398933411 -0.0440140515565872
0.411032944917679 0.381497144699097
0.842869162559509 1.54288446903229
1.36387193202972 -2.39770293235779
3.81814789772034 9.37960338592529
0.263417541980743 -1.57739877700806
-0.19200199842453 -0.0890971571207047
-0.769473433494568 0.726000070571899
0.230198621749878 1.09224033355713
2.46685266494751 -1.12673854827881
3.63506603240967 0.726149797439575
-0.362788140773773 0.681029677391052
1.38569319248199 -3.10861039161682
0.673896372318268 0.86654531955719
1.43970811367035 1.72962617874146
0.161015406250954 -0.873399257659912
0.878690958023071 0.0702217593789101
0.0902083814144135 0.095268577337265
3.63847780227661 -5.11003303527832
1.05766773223877 -0.79608291387558
0.879909992218018 0.148472592234612
0.134598523378372 0.498987168073654
1.30900239944458 -4.39701747894287
-1.46172606945038 0.835859775543213
3.0153021812439 -0.979702234268188
-0.0303928926587105 -0.361285269260406
2.20985007286072 0.430838942527771
2.03062725067139 -2.00823783874512
-2.38359951972961 0.144903391599655
2.07262134552002 -4.74713897705078
0.417600870132446 -0.0865439921617508
-2.06252765655518 -0.0825467705726624
-1.03622722625732 0.481243193149567
2.5801465511322 -1.5612154006958
0.231310173869133 -1.37679958343506
2.4866623878479 -2.69625520706177
-0.25767120718956 -0.571780204772949
-1.5472457408905 0.390707671642303
0.430434435606003 0.454591989517212
-0.3222835958004 -0.92579185962677
2.72547602653503 1.8779628276825
2.74485516548157 -2.50960564613342
2.68762063980103 -5.10076570510864
2.21028590202332 -0.086386501789093
4.00939607620239 6.78739452362061
1.18918585777283 1.39475154876709
-0.738742768764496 0.0886147022247314
0.693489074707031 -1.49732553958893
2.06375932693481 -3.10366177558899
0.662247955799103 -1.90490198135376
1.07403492927551 -1.76356637477875
2.14994525909424 -0.704306244850159
3.04553008079529 2.49137759208679
1.18476867675781 -2.48635149002075
2.42102074623108 6.24667835235596
0.194493353366852 -0.720472872257233
1.25095796585083 2.28949236869812
2.49159002304077 7.74189567565918
-2.71228837966919 0.386485457420349
-1.49863147735596 0.544586539268494
-0.446310639381409 1.31590974330902
3.19571161270142 -5.20552110671997
-0.788667440414429 0.687594592571259
-0.0486068427562714 -0.224785059690475
2.04091048240662 -2.44182467460632
1.57877779006958 1.2492071390152
2.23561215400696 -2.78078508377075
0.1421237885952 -0.379204750061035
-0.809584438800812 0.0259663946926594
2.27020001411438 -0.302293986082077
0.648818492889404 -0.791931509971619
-0.312136143445969 0.272197961807251
};


==> figures/visualizations/funnel/smc_samples.tex <==
\addplot [semithick, smc, opacity=0.7, mark=x, mark size=3, mark options={solid}, only marks]
table {%
2.51525950431824 -2.09167742729187
-2.73498058319092 0.207288190722466
0.192354738712311 0.835411489009857
-2.69611120223999 0.144458651542664
-1.11802589893341 -0.622180342674255
0.0920396000146866 0.29291096329689
-3.17417168617249 -0.143703907728195
-0.202439919114113 -0.361902743577957
-4.68594360351562 0.128749817609787
1.0555100440979 2.34137439727783
0.0695298090577126 0.117904759943485
-0.466674447059631 0.0753540545701981
-0.605318665504456 -0.67486560344696
-4.26659393310547 -0.0359963774681091
0.116707846522331 -0.696248710155487
-2.0558078289032 -0.710240960121155
0.025789886713028 0.140510737895966
-2.99752736091614 -0.139280617237091
-0.625979244709015 -0.675326228141785
0.472374469041824 0.390032857656479
-2.56769394874573 -0.335721224546432
-1.31649804115295 0.33545845746994
0.634650766849518 1.95256781578064
-2.20698213577271 -0.312110751867294
0.808586776256561 0.730993568897247
1.20198714733124 0.33375284075737
1.47213089466095 1.81254363059998
0.839925527572632 -1.85454499721527
-3.30391597747803 0.225728958845139
-5.20873117446899 0.0751101523637772
-0.991944670677185 -0.224424242973328
-1.71991360187531 0.368466824293137
2.02503228187561 -0.208828076720238
-0.123968377709389 1.27522075176239
-0.925159335136414 -0.638130307197571
-1.21331858634949 -0.36256206035614
1.65066361427307 1.94337844848633
-1.15133333206177 -0.413222759962082
0.0243050791323185 1.84086811542511
-3.53166341781616 -0.101556934416294
0.251208752393723 -1.31006300449371
0.762608170509338 2.85481834411621
0.280658006668091 -0.454026699066162
-2.94683241844177 0.253457546234131
1.92175042629242 2.27451109886169
-3.53617763519287 0.1072161719203
-0.905906975269318 0.494805306196213
-0.756980180740356 0.287576377391815
-1.33612537384033 -0.341165393590927
0.327627450227737 0.0343878641724586
-2.61453795433044 -0.248620361089706
-1.82646536827087 -0.584470272064209
-4.40644884109497 0.247603133320808
0.329973220825195 -2.08010339736938
-2.45817017555237 -0.344637453556061
0.360316663980484 -1.13870453834534
-0.199282675981522 0.475647151470184
-2.36869072914124 0.264327257871628
-3.18112277984619 0.13863143324852
1.58005726337433 0.689415097236633
-1.76670229434967 0.49738222360611
-0.965429544448853 0.0765037015080452
-0.333558678627014 -0.0334260836243629
0.738885283470154 -1.09684693813324
-2.92253565788269 -0.0400151386857033
-3.59100985527039 -0.0215772390365601
-0.0629309639334679 1.69059991836548
-0.424485325813293 0.393938839435577
0.461558014154434 0.724504172801971
-3.59191823005676 -0.0249049328267574
-1.0013290643692 0.0305022895336151
-0.336818158626556 0.388582944869995
1.41057026386261 -1.38702416419983
2.7514922618866 -0.630885183811188
2.12989258766174 -0.705390989780426
-2.75509214401245 -0.0150466412305832
0.750512182712555 2.48307156562805
-3.3822774887085 -0.273260146379471
-5.05691528320312 -0.0100662857294083
-0.248876690864563 0.303103446960449
-2.15728712081909 0.16220235824585
0.434871524572372 0.837191104888916
-0.69359028339386 2.36188364028931
1.04795002937317 -0.555326700210571
1.17844343185425 -2.12453031539917
0.518348515033722 1.72890412807465
-2.70410656929016 -0.196183189749718
-1.63616299629211 -0.182878106832504
0.2552330493927 0.655059635639191
0.109310634434223 -0.330999851226807
2.10222268104553 -2.6034984588623
-0.480576276779175 -1.19265997409821
-1.3445235490799 0.640174448490143
2.0214319229126 -1.49963545799255
-1.38557922840118 0.0700018778443336
-0.383561491966248 0.0983739048242569
-3.2201681137085 0.29815611243248
-1.64339554309845 -0.263973474502563
1.08189451694489 0.63678514957428
-2.24984359741211 0.077333465218544
-0.626910448074341 -0.5250363945961
1.65201270580292 2.12772560119629
-4.32030200958252 0.0265438891947269
-1.59508275985718 0.71550327539444
-3.64113259315491 1.44839286804199e-05
-0.166073977947235 0.375665426254272
-2.80117535591125 -0.273294866085052
-5.51302433013916 -0.0197094269096851
3.08212423324585 3.71724200248718
-3.98638987541199 -0.130036175251007
1.25086998939514 -0.679739713668823
-0.623836755752563 -0.524080574512482
2.42013883590698 -0.552630007266998
0.504063308238983 0.197129234671593
1.11423981189728 0.0423001684248447
2.41352653503418 -0.136290803551674
-0.533358514308929 -0.796715557575226
-2.46549820899963 -0.242754116654396
-1.02789258956909 0.2547248005867
-3.10198569297791 -0.128342285752296
1.9255530834198 2.75653481483459
-2.72360062599182 -0.182004988193512
-2.76114344596863 0.266852378845215
-1.33169591426849 -0.205600723624229
-1.39115238189697 -1.08659553527832
1.72118616104126 -2.36540961265564
-3.69196224212646 0.122092992067337
-2.97091555595398 -0.283438056707382
2.02639651298523 1.37066996097565
2.13550448417664 -1.2020229101181
-1.78646504878998 0.188823565840721
-1.41329944133759 -1.04738056659698
1.03615593910217 -1.44298577308655
-1.70664131641388 0.281939923763275
-1.5795693397522 -0.241582840681076
-3.90234279632568 0.0963166207075119
-1.14429092407227 -0.964563310146332
-3.75495171546936 0.272363096475601
1.37628555297852 -0.837613642215729
3.27652478218079 -1.06731951236725
-2.8906238079071 -0.31219157576561
-1.97729563713074 0.165716037154198
-4.54385995864868 -0.116726748645306
-3.9534695148468 0.0581218637526035
-2.15262794494629 0.0968996807932854
-0.0829844027757645 -0.223766505718231
0.052303459495306 -1.17407953739166
-0.24569608271122 -0.161346882581711
-3.80834794044495 -0.265542149543762
0.553512513637543 1.53552341461182
-4.51719379425049 -0.0732795521616936
-0.107322841882706 0.0617577731609344
-3.6699640750885 0.142392680048943
-2.25148510932922 -0.0973494052886963
-0.790050685405731 -0.282215774059296
1.09865975379944 -1.07139539718628
1.19044637680054 -2.56564593315125
-0.884258091449738 0.415050059556961
-0.161899343132973 0.189583167433739
1.25360083580017 0.871396720409393
0.126807868480682 0.31925493478775
-1.18763554096222 -0.229769736528397
0.538085460662842 2.24065160751343
-2.00728225708008 -0.0639279261231422
-0.603766083717346 0.0606001242995262
-0.534217834472656 -1.39837908744812
-3.09655117988586 -0.252106010913849
-0.985857486724854 0.602204442024231
-2.13935470581055 -0.791632652282715
0.585489988327026 1.77847766876221
0.949277341365814 0.539587318897247
-0.56769061088562 -0.512769937515259
-4.85415267944336 0.0401722900569439
-0.109636627137661 1.62985730171204
0.0753048062324524 0.425144225358963
1.20423126220703 -0.11770187318325
-5.00138998031616 0.0650168731808662
0.554135978221893 0.322104126214981
-2.37129044532776 -0.101642861962318
0.468700915575027 -0.94651734828949
-3.83563208580017 -0.0791897103190422
-0.813685774803162 0.935832262039185
-1.21107876300812 0.862585663795471
-2.66635203361511 -0.292669206857681
0.890955150127411 1.61231541633606
-0.674033522605896 -0.285726130008698
1.9263482093811 -1.75686383247375
1.13218891620636 1.08473241329193
-1.01064610481262 -0.128637790679932
-2.56473278999329 0.133966684341431
-0.780061602592468 -0.263647019863129
-1.13774657249451 -0.692975461483002
-0.11871051043272 -0.85857492685318
-0.0950600281357765 0.604440689086914
-0.280782133340836 0.0233233422040939
-0.835446834564209 0.468078583478928
-0.14716050028801 0.90012913942337
0.981663048267365 -4.41062879562378
1.51610243320465 -1.78722524642944
0.555180132389069 0.283936053514481
2.15608930587769 -1.55296289920807
-1.73224997520447 0.369497239589691
0.473680168390274 -1.18883371353149
1.48378932476044 -2.25739908218384
0.552784204483032 0.571715950965881
-0.40984907746315 -0.369100034236908
-0.555443346500397 -1.12649261951447
-1.15665376186371 -0.0872111022472382
0.310303777456284 -0.605011463165283
1.73491752147675 -2.6534640789032
-1.78220367431641 -0.0599097386002541
-1.92132496833801 -0.204191088676453
1.39629912376404 2.75101757049561
-1.30955445766449 0.159221649169922
0.546463012695312 -0.585460305213928
-2.36508870124817 0.0510558485984802
-4.17445230484009 -0.0130732357501984
0.703431665897369 1.08029103279114
2.70494055747986 -1.78899431228638
0.659126937389374 0.657875597476959
1.36095297336578 -0.121846526861191
-0.354458868503571 -1.16614162921906
0.0730666667222977 -0.170897081494331
0.285114258527756 -2.35629439353943
1.98267543315887 3.73685646057129
-1.6835378408432 0.687024176120758
-2.24505424499512 -0.0611633583903313
-2.68626070022583 0.0185896381735802
1.18546426296234 1.31175553798676
1.25647246837616 0.469715058803558
-0.557981073856354 1.38257157802582
-0.76960688829422 0.175932705402374
-0.0325430482625961 -0.169876366853714
-2.63390827178955 -0.18792836368084
0.954656422138214 1.05579710006714
1.15234708786011 0.469185054302216
-3.15139698982239 -0.0616881549358368
0.548165559768677 -0.948587536811829
0.481956899166107 -0.826856434345245
-0.65714704990387 0.0507675558328629
-3.72659111022949 -0.232844993472099
-0.783642888069153 0.456483423709869
-2.10731291770935 -0.0615954175591469
-4.66587495803833 0.0896736979484558
0.492338001728058 -0.886865794658661
-2.19213461875916 0.211600452661514
-0.854584038257599 0.865734338760376
-1.33165001869202 -0.138558059930801
-3.58523988723755 0.051489632576704
0.156828388571739 0.469695806503296
-0.0676474198698997 -0.0867238566279411
2.34823322296143 1.16987800598145
-1.01354324817657 1.27783727645874
-0.0418511293828487 1.90009903907776
1.2739999294281 -1.09060716629028
-1.10263955593109 -0.953285574913025
1.19383537769318 -1.54172813892365
-0.632491648197174 -0.137916564941406
-0.606058418750763 0.851404190063477
1.45385527610779 2.83978915214539
0.950437068939209 0.22054535150528
-3.59919357299805 -0.339287400245667
-3.10744690895081 0.0208224542438984
-0.671713590621948 -0.323047131299973
-1.78819680213928 -0.649674534797668
-5.13092088699341 -0.0535833388566971
1.3860194683075 -0.248759120702744
-2.08898448944092 -0.165339380502701
-1.89240753650665 0.359283924102783
-0.300034433603287 0.0125883352011442
2.29503178596497 -1.4426873922348
1.79118204116821 -4.83607006072998
-0.133925050497055 0.0992630198597908
-0.0614657700061798 -0.6201052069664
-2.56362557411194 0.454210042953491
0.689801752567291 -1.55258882045746
-0.0553467087447643 1.34023642539978
0.529617249965668 1.69516587257385
-1.77192056179047 -0.277714043855667
1.10153865814209 -1.02509129047394
-0.0148932188749313 -0.0513046756386757
-2.57732844352722 0.600854933261871
-1.58099520206451 -0.247617080807686
-3.60898494720459 -0.369665920734406
1.08307218551636 0.784358978271484
-1.47371923923492 0.200968563556671
1.39814412593842 -0.201282650232315
-2.66186690330505 -0.0393522158265114
1.87605047225952 0.791668593883514
-1.66689383983612 -0.156945586204529
-0.851579964160919 1.5979677438736
1.92932534217834 2.18224024772644
-2.21588087081909 -0.260769844055176
0.88785856962204 2.61230492591858
-1.49215686321259 0.436265528202057
1.05849862098694 2.5437331199646
-3.05198073387146 -0.277492702007294
-5.5707859992981 -0.0768306627869606
-1.61355125904083 -0.338131546974182
-0.510493636131287 0.0488426350057125
1.07047593593597 -2.49565815925598
-1.8803426027298 0.0628387555480003
0.409841775894165 1.39480137825012
0.147178441286087 -1.34958004951477
0.842270493507385 -3.85717868804932
-1.42456233501434 -0.498672634363174
-2.11997556686401 -0.0282366126775742
-2.77237939834595 0.0729238465428352
-1.76616072654724 -0.451115608215332
2.51348423957825 -0.116824746131897
-0.0601692348718643 0.599808096885681
-0.738939046859741 -0.303953170776367
-0.315758585929871 -0.0362434312701225
-3.06916952133179 -0.101848095655441
-1.90482413768768 -0.281470984220505
0.045489601790905 -0.834474742412567
-2.49567532539368 -0.0668590664863586
-0.863052129745483 0.289029628038406
1.46046340465546 -3.09316873550415
0.653811156749725 -0.13807013630867
-0.638342142105103 -0.388380408287048
0.828443050384521 1.48186230659485
0.688261210918427 -0.956619322299957
-0.769096076488495 -1.24048149585724
-1.81157279014587 -0.138681471347809
-0.914286851882935 0.0209131762385368
1.7288830280304 -2.95546674728394
0.457285791635513 -2.46278548240662
-2.13592290878296 -0.447705984115601
-0.528111636638641 -0.055303230881691
-0.397620797157288 0.122780650854111
-0.0682055428624153 -1.34403491020203
0.702329993247986 2.9920380115509
1.7145015001297 1.18852388858795
0.509511590003967 1.36644768714905
-1.64266729354858 -0.097767174243927
-0.336884647607803 0.0370149612426758
0.690719366073608 2.7241222858429
0.364871323108673 -1.84842371940613
-3.55729365348816 -0.0724228769540787
-0.506651401519775 -0.221703290939331
0.0545613132417202 0.802080571651459
-3.80713438987732 0.0788183510303497
0.000308126211166382 -0.374522656202316
-1.9074592590332 -0.0153778046369553
-0.368950128555298 -0.742857575416565
-0.212966457009315 -1.42744946479797
-3.12151169776917 -0.150559097528458
-3.99631977081299 0.0350935645401478
-1.01469564437866 -0.333163917064667
-0.977521479129791 0.604334235191345
-0.487029999494553 1.28843903541565
-3.42610883712769 -0.422764748334885
-1.34611403942108 -0.474519163370132
-2.10328912734985 -0.309880197048187
-3.66488838195801 0.167028158903122
-2.63127636909485 0.0858921483159065
-3.95091938972473 -0.0782817825675011
-0.788955986499786 0.141969457268715
1.77058529853821 3.86994314193726
-3.10047841072083 0.274955540895462
-0.327730894088745 -0.487034976482391
-0.307141155004501 -0.302377194166183
1.17172491550446 1.25204610824585
0.560393929481506 -0.254228740930557
-1.5457010269165 0.669182658195496
-1.60792922973633 0.0391502007842064
0.525381326675415 -0.22883266210556
2.22931480407715 1.43758654594421
1.19832587242126 0.362291991710663
-0.866401255130768 0.739571809768677
-0.543630063533783 -1.08893346786499
-0.658693253993988 0.352235227823257
-0.683646261692047 -0.251781344413757
-0.684806704521179 0.64466917514801
0.816651403903961 -2.0550365447998
-2.77734589576721 0.119829058647156
-2.86877202987671 0.200276389718056
-0.669506669044495 -0.82392430305481
0.323898106813431 0.522752344608307
1.47525858879089 5.90340614318848
-1.68174493312836 -0.194632902741432
-0.956489086151123 -0.762450277805328
-0.119260750710964 0.0659372732043266
-1.73548758029938 -0.0567731931805611
-1.09836256504059 0.442119628190994
-0.596744775772095 -0.29879155755043
-3.15814805030823 -0.0548942387104034
1.56373226642609 -4.13983726501465
1.32612824440002 -1.57419502735138
-2.20441722869873 0.431778192520142
-0.0947648882865906 0.478988111019135
2.17513060569763 4.43234872817993
-1.38440608978271 -0.0276718065142632
0.310232818126678 -1.79041957855225
-1.51232826709747 0.420474946498871
-0.814723789691925 -0.681641459465027
0.845859408378601 -1.70005416870117
2.40841722488403 -1.52587187290192
-1.51560890674591 0.140797913074493
-3.6015248298645 -0.0900684297084808
2.20363402366638 -3.11061143875122
-0.268609166145325 -1.38158583641052
-2.45088386535645 -0.119744554162025
-3.41521573066711 -0.234123632311821
-1.95367288589478 -0.43043252825737
0.458381921052933 2.84449076652527
0.476895928382874 -0.479806631803513
-0.860521078109741 -1.07166838645935
-1.92661440372467 0.0709172934293747
0.566405594348907 1.34803438186646
-2.00890588760376 0.429334580898285
-0.0504701621830463 -0.0959373041987419
1.45559751987457 -0.426583170890808
0.651556611061096 -0.645341575145721
2.29309391975403 6.12044715881348
-3.7952253818512 0.065970204770565
-2.15043354034424 -0.159234717488289
-1.63725340366364 0.493336141109467
0.17989219725132 -0.117499232292175
1.71782290935516 -2.41817259788513
-0.72796893119812 -1.23889517784119
-1.90683531761169 -0.459668725728989
-2.70031142234802 0.348414212465286
-1.65228128433228 -0.203236728906631
0.731504321098328 -0.6293785572052
0.589214086532593 -0.902770221233368
-1.43645346164703 -0.68828010559082
1.10537242889404 -3.3915798664093
-1.320063829422 -0.267396748065948
-0.829903423786163 -0.0863147974014282
-3.19341945648193 -0.43832740187645
-0.535908818244934 -0.286822110414505
1.43794083595276 -1.12812578678131
-0.446733504533768 0.818246185779572
4.07010698318481 -1.51454699039459
-0.687310993671417 -0.439813494682312
-2.24031829833984 -0.0140617340803146
0.835606873035431 -1.06334209442139
2.24040031433105 1.55261838436127
0.737975716590881 0.188568815588951
-0.455689340829849 0.30488321185112
-3.02749991416931 -0.0347928181290627
0.692480206489563 0.397990256547928
1.57441234588623 0.876146197319031
-0.138549715280533 -0.160785362124443
-2.28747248649597 -0.0285964012145996
-1.83392477035522 0.128484725952148
1.22307503223419 -1.50238811969757
-3.19139814376831 0.238627359271049
-3.92508316040039 0.0441192537546158
-3.01646089553833 0.09909837692976
-0.701667666435242 0.931545734405518
-0.77236944437027 -0.136876195669174
-0.259297847747803 2.21093130111694
1.20950746536255 -0.623055458068848
-1.33175122737885 0.488828182220459
-2.11122989654541 -0.125168487429619
1.19676101207733 0.983583033084869
1.37474632263184 1.07044446468353
-0.793864250183105 0.0055670477449894
0.409543365240097 0.136793851852417
-1.30447697639465 0.27800726890564
0.145692005753517 -1.12867403030396
0.000126436352729797 -0.413306534290314
-2.18088531494141 0.100489974021912
-5.50276517868042 -0.0913230031728745
-0.956428349018097 -0.875683069229126
-3.67757725715637 -0.109188713133335
1.49037063121796 0.11132451146841
0.188668042421341 0.126492828130722
-2.7741436958313 0.0310076922178268
0.0958028137683868 0.534830868244171
-1.89459669589996 0.119206368923187
0.526821672916412 0.400614053010941
-3.54870438575745 -0.432314991950989
1.19348931312561 -1.06120228767395
-3.46343874931335 0.0729955434799194
-2.4973509311676 -0.237019538879395
0.316311061382294 3.59430432319641
0.0717830210924149 1.28328585624695
0.291790902614594 0.718468308448792
-3.48268222808838 -0.0831007808446884
-2.77795720100403 -0.226150587201118
-1.56263947486877 -0.187081381678581
1.61383724212646 1.87478244304657
0.359465509653091 0.382430553436279
-1.81841742992401 -0.0547704547643661
-0.00898939371109009 0.774623572826385
-2.64539456367493 0.118290305137634
-2.74759984016418 0.246098682284355
-1.96072745323181 -0.0450702644884586
-1.5898209810257 1.31888127326965
1.58034229278564 0.714225888252258
-3.23407649993896 0.0832187905907631
1.03358471393585 -0.0117866732180119
-1.1821254491806 0.348867863416672
-0.738057196140289 -0.334735214710236
-0.327370345592499 0.820658385753632
2.47413182258606 4.15428495407104
-2.32873368263245 -0.118981868028641
-2.16292762756348 -0.382480204105377
0.16986620426178 -0.942789196968079
-3.96003746986389 -0.118367597460747
0.639278531074524 -0.887379288673401
2.71164989471436 3.94262504577637
0.0392498075962067 -1.08813333511353
2.63855695724487 0.508595585823059
-1.10252439975739 -0.113907247781754
-2.19402289390564 0.164635807275772
-0.604980170726776 0.856705963611603
0.698242127895355 -0.436875402927399
-0.552090108394623 -0.408080875873566
-1.32474839687347 0.10610606521368
-0.50432550907135 -2.16483497619629
-1.06907737255096 -0.827461719512939
2.20543766021729 2.3632869720459
-4.60234975814819 0.0234071351587772
0.14923769235611 0.390628427267075
1.47602546215057 -0.210275337100029
0.296403408050537 -2.01947259902954
-0.227149024605751 -1.34853410720825
-0.151771634817123 -0.816313862800598
-1.57197570800781 -0.789638578891754
1.04574334621429 2.0657684803009
-2.26336526870728 -0.0899633541703224
-0.20346836745739 1.3653290271759
0.159438401460648 0.65165776014328
-0.855141401290894 -1.3231635093689
-0.622132539749146 0.909217119216919
-1.57121980190277 0.306634426116943
1.08788764476776 -1.07915902137756
-2.59053158760071 0.019459180533886
0.535784602165222 1.8189914226532
0.510223507881165 -0.00546367466449738
-1.27560842037201 -0.158137083053589
1.86102211475372 -1.11761045455933
-3.13403487205505 0.662869572639465
-0.708850979804993 -0.086658388376236
-2.82301616668701 0.0975996628403664
-2.81288051605225 -0.00705957040190697
-0.118981085717678 1.1712965965271
-1.22186183929443 -0.39864656329155
1.81034696102142 -1.96648442745209
-0.302062332630157 -0.30571261048317
-2.50331497192383 0.0884240418672562
0.0626808702945709 1.12586224079132
-4.30677032470703 -0.360022097826004
-1.27133309841156 0.149246051907539
-0.0493725724518299 1.70287525653839
-0.760031819343567 0.414505481719971
-3.46045637130737 0.184876099228859
-1.88264286518097 -0.694491624832153
-0.078665554523468 0.582638800144196
4.14153718948364 -0.0836262330412865
-4.5301308631897 0.0644986853003502
-0.030247176066041 -0.993244111537933
-0.375912636518478 0.190640285611153
0.521768391132355 -1.06410992145538
-2.279541015625 0.157658725976944
0.533543288707733 0.434096455574036
-0.0183180198073387 -0.546747863292694
-0.531046986579895 -0.344180941581726
1.58211851119995 0.915334165096283
2.33287978172302 -3.6161150932312
-0.682372689247131 0.902381837368011
-0.166651219129562 0.00167809426784515
1.38182687759399 1.09235024452209
-2.75442981719971 -0.237410485744476
1.0461505651474 -0.13707435131073
1.19168651103973 -0.909782409667969
-2.22218489646912 0.438574194908142
1.08062827587128 -0.73597925901413
-0.598230957984924 0.97559517621994
-0.524174571037292 -1.24591326713562
0.640877664089203 1.71304249763489
0.869955122470856 2.88299131393433
-0.218865841627121 0.0309273153543472
0.810002088546753 1.4713397026062
1.35087895393372 0.335113853216171
-0.985631108283997 1.20029580593109
-0.68294632434845 -1.74503648281097
-0.552590072154999 -0.96477198600769
-3.55309247970581 0.08151875436306
-0.0103011727333069 -0.111366465687752
1.20736086368561 -0.640752673149109
-2.90340542793274 -0.169119134545326
2.17542791366577 1.57808089256287
-0.00452958233654499 -0.968709886074066
-0.984536826610565 -0.185890212655067
-0.297935485839844 -0.632437229156494
-1.49410343170166 -0.198544040322304
-0.137681096792221 0.658410966396332
0.506808161735535 -0.489827692508698
-1.14105701446533 0.470949023962021
-1.05767548084259 1.3210107088089
-0.0590659081935883 0.907689809799194
-2.66340351104736 0.0232160240411758
1.65321457386017 -1.34441113471985
1.22708332538605 -2.14935398101807
-3.48331165313721 0.0649022310972214
-0.492575436830521 -0.683780133724213
1.11146676540375 0.216654896736145
-1.05029165744781 0.670340001583099
-0.599692940711975 -0.148411199450493
-1.67234289646149 -0.688367068767548
-0.132807731628418 1.14613997936249
-4.62566661834717 -0.000399040058255196
2.12904453277588 2.3983907699585
-1.6246771812439 -0.68794047832489
1.34863889217377 -2.31217241287231
-1.06056690216064 0.40923684835434
-1.68781518936157 0.602092444896698
1.24461901187897 1.43353855609894
0.435338824987411 1.25109648704529
1.87077260017395 1.13154220581055
-1.49826276302338 -0.318090111017227
-1.53064179420471 -0.6065314412117
-2.00996541976929 0.110687956213951
-0.283134907484055 0.603901207447052
0.909203052520752 0.929791510105133
0.535559833049774 0.259746462106705
-1.33367002010345 0.103530913591385
-1.33722567558289 0.617613971233368
-1.97091865539551 -0.405599623918533
-1.05543887615204 1.02567219734192
1.27667319774628 3.57324194908142
0.756736874580383 1.04451036453247
0.121790364384651 -1.53753733634949
-2.58880925178528 -0.159062087535858
-1.57847774028778 -0.926177680492401
0.078571654856205 -0.615893065929413
0.687963664531708 -0.430245667695999
-3.33181881904602 0.0216836612671614
-4.63861799240112 0.000915192067623138
-3.17888712882996 0.0569511391222477
-1.26274132728577 -0.667940139770508
1.90743982791901 2.69862937927246
-1.26810824871063 0.316047966480255
1.06673991680145 1.07707357406616
-1.03672826290131 0.213790267705917
-5.13129997253418 -0.0608674511313438
0.0162473991513252 0.72823292016983
-0.216510474681854 -0.997216761112213
-1.18794655799866 -0.647019743919373
1.1940358877182 1.46811079978943
-0.984930992126465 0.4337517619133
-2.45195579528809 0.238129258155823
-4.54990196228027 -0.224184826016426
0.044887226074934 1.41392707824707
-1.14017987251282 0.856048345565796
-2.14869475364685 0.786678373813629
-0.130905777215958 0.107544511556625
1.16863453388214 -0.297149121761322
1.56540858745575 0.705430507659912
-2.84412312507629 -0.12917098402977
1.01621580123901 0.958202004432678
-3.70651745796204 0.0981191843748093
-1.61235928535461 0.315964102745056
0.648815095424652 0.604749441146851
-0.980197846889496 0.249043762683868
1.70964109897614 -0.968077659606934
-1.99458193778992 0.0274750534445047
1.78657722473145 -0.508122801780701
-1.50977575778961 0.407236248254776
1.20172905921936 0.519402265548706
0.656572699546814 2.10828495025635
2.39343595504761 -2.11735677719116
0.667008638381958 -0.581724643707275
0.867989599704742 -0.0395411401987076
-3.49759984016418 -0.0450425297021866
1.90606486797333 -1.40787553787231
-3.7242910861969 0.104389764368534
0.0968826785683632 1.13413822650909
0.863309562206268 2.10753965377808
0.896115720272064 -2.03037428855896
1.23623549938202 1.59423589706421
1.46902716159821 0.340003669261932
-2.68252182006836 0.226345285773277
-1.08734059333801 0.166370064020157
0.805535495281219 0.501862645149231
-1.56074726581573 0.248482406139374
0.0802134871482849 -1.85272789001465
-2.1156017780304 0.153280824422836
-4.58405256271362 0.0135593861341476
0.210690289735794 -1.23443293571472
1.55355656147003 -0.978561043739319
1.32894861698151 0.252597033977509
-2.65539622306824 -0.110591351985931
-2.51891469955444 0.246693328022957
0.158655077219009 0.407742083072662
-0.757184743881226 -0.938589632511139
-1.34917676448822 -0.474200367927551
1.78196549415588 -2.53724598884583
-1.40023958683014 -0.0762397721409798
-0.199765354394913 -2.02868103981018
-2.06656551361084 -0.145537704229355
1.02575552463531 -1.32363057136536
0.87706196308136 0.623019218444824
0.476248651742935 -0.103153243660927
0.881374061107635 -1.52682292461395
0.077710822224617 0.356584966182709
-0.0701414346694946 -0.265899896621704
0.316786557435989 -1.79554712772369
-3.30366444587708 0.1574487388134
-0.692722082138062 -0.251694768667221
-0.805211544036865 -0.258530020713806
-4.04781484603882 -0.143029808998108
0.693244814872742 1.65454912185669
-0.61709201335907 0.00196551601402462
-2.34487891197205 0.178291797637939
0.61273467540741 1.13888227939606
-2.33613157272339 -0.188589751720428
1.22145259380341 2.10158681869507
1.41671407222748 1.01784372329712
-0.485030472278595 0.386445492506027
-0.573270797729492 -0.408959805965424
-4.17945671081543 0.00941085070371628
-1.82168614864349 -0.0080118365585804
0.624910414218903 -2.39109110832214
-2.12563037872314 0.303224474191666
-0.276364922523499 -0.56874817609787
-2.17818808555603 0.280853629112244
-2.06071972846985 -0.0536256656050682
-2.53740501403809 -0.302027344703674
-5.23654794692993 -0.115143768489361
-2.16599583625793 0.351412296295166
-0.0215217508375645 1.06103014945984
0.0924693048000336 0.85513436794281
-1.36605882644653 0.397045612335205
-3.59717917442322 -0.108667179942131
0.349242746829987 0.203844398260117
-0.973094999790192 0.525651097297668
-4.04708766937256 -0.0328885838389397
0.484890937805176 0.382088661193848
1.92391097545624 1.23576092720032
-0.651486873626709 -0.838849008083344
-0.370163023471832 0.55094850063324
0.392114639282227 -1.14022886753082
-0.270149707794189 0.53706157207489
-3.31793975830078 0.0502515956759453
-1.65001904964447 -0.10581511259079
0.970909833908081 1.85798358917236
-0.0460871234536171 -0.623632788658142
-0.716703414916992 0.378416329622269
1.20662689208984 2.36589288711548
-1.93986248970032 -0.0646658837795258
-1.13635885715485 0.79776257276535
3.01333999633789 5.62685394287109
-5.25381517410278 -0.00452091544866562
-2.18848323822021 -0.115649029612541
0.497563153505325 -0.686388254165649
-2.2799026966095 -0.352711260318756
-0.225359708070755 0.929592728614807
-0.149256438016891 1.94962525367737
0.541214883327484 0.0106556713581085
0.500763177871704 1.78047716617584
0.717132747173309 0.472207099199295
-2.53065586090088 -0.423164069652557
1.30441045761108 2.16621208190918
0.085166409611702 1.00214159488678
2.70561623573303 -0.920208930969238
-0.483226895332336 -0.25686502456665
0.0314515307545662 0.67685067653656
-1.78476428985596 -0.32491797208786
-0.642872631549835 1.5076071023941
1.54829812049866 2.55069160461426
-2.3735818862915 -0.293091535568237
-0.963594198226929 0.368537604808807
-2.03339219093323 -0.276683419942856
0.507260680198669 -0.370464444160461
1.08159077167511 -2.26067662239075
2.42904186248779 -0.075106680393219
-3.15319895744324 0.240124940872192
-1.40426516532898 -0.322805553674698
0.730402052402496 -1.27121579647064
2.01017141342163 -0.898200273513794
-1.95984613895416 -0.462241798639297
-1.16097068786621 0.236514523625374
-1.26750373840332 0.246663898229599
1.07473826408386 0.83727490901947
-0.128287822008133 1.79501140117645
2.35795998573303 3.05357623100281
-1.76867687702179 -0.662335574626923
2.61699318885803 -3.90694665908813
-1.91356730461121 0.0223289281129837
2.18628311157227 2.37737631797791
0.152142941951752 -0.232785910367966
0.418505430221558 1.05945134162903
-2.70770025253296 0.00412620604038239
-2.01389694213867 -0.526686429977417
1.02547240257263 2.01246070861816
-2.13491034507751 0.195836901664734
0.157579123973846 -0.430558204650879
-1.48840045928955 -0.47213739156723
-1.33818233013153 0.972555339336395
2.10278916358948 -3.49864196777344
-3.95962858200073 -0.188082963228226
-2.83204436302185 0.2340377420187
1.23903918266296 -0.879575788974762
1.02926659584045 1.34858703613281
-3.30585122108459 0.121902301907539
1.36316764354706 0.692803084850311
-0.0399010628461838 0.882216930389404
2.81254291534424 3.79088926315308
-5.19590663909912 -0.00446793437004089
0.358001112937927 -0.429618239402771
1.63315320014954 -1.60720503330231
0.323190331459045 -0.398605525493622
-2.76810503005981 0.0563749447464943
1.36634457111359 0.0651968419551849
-3.15778136253357 0.00508618354797363
1.16372108459473 -4.52790832519531
-1.13523077964783 -1.0097633600235
-0.616117656230927 0.711144685745239
3.27175807952881 3.50605297088623
-4.14115285873413 -0.188522934913635
-1.0447986125946 0.206076443195343
1.15920376777649 5.17194747924805
-0.35851389169693 -0.434535205364227
-3.84796810150146 -0.212495088577271
-3.04184150695801 0.174106240272522
-0.183925732970238 -0.477876603603363
-0.700510263442993 0.440593123435974
1.6457804441452 -2.02098846435547
0.827541708946228 -0.126897618174553
0.44210958480835 0.963877558708191
-0.535708427429199 -0.872978806495667
-2.31177377700806 -0.0705819427967072
-1.41482865810394 -0.81970226764679
-0.237432241439819 0.126643419265747
-0.417764574289322 0.454031884670258
-1.60693264007568 -0.12020654976368
0.307822585105896 2.24896621704102
1.20332717895508 -2.23917436599731
1.1859917640686 -1.95893573760986
0.820652544498444 0.99286299943924
-2.87673139572144 -0.00080021470785141
-2.79453659057617 0.240857481956482
-1.93004894256592 0.20114478468895
0.570612907409668 -0.246320754289627
-3.93824815750122 0.202612325549126
-4.43510150909424 -0.0165797118097544
-1.41150414943695 0.176985666155815
-1.10703063011169 0.348049283027649
-0.173869341611862 -0.234132245182991
-2.43212461471558 0.0113815851509571
1.31003618240356 -0.398896217346191
0.559586524963379 1.15032279491425
-3.47094750404358 -0.202790603041649
-0.932125687599182 -0.342307239770889
1.86343717575073 -1.83500063419342
-3.6484694480896 -0.112311989068985
-1.67891848087311 0.380989521741867
0.414666146039963 0.367317318916321
-3.3048894405365 -0.0235984586179256
-2.35992813110352 0.647373259067535
-2.96241688728333 -0.0236475393176079
-4.58454942703247 0.0630572587251663
1.93855154514313 1.33977293968201
1.22072219848633 -0.755785882472992
1.39734029769897 -1.18323922157288
0.41170471906662 0.881781816482544
1.46294820308685 1.09119606018066
-2.24501323699951 0.283594191074371
-0.970418453216553 -0.333278775215149
-0.30265673995018 1.01467740535736
-4.11641979217529 -0.00995749793946743
-0.761577963829041 -0.439956337213516
-1.69581496715546 0.376709789037704
-3.10297584533691 0.332622110843658
1.9573118686676 1.48029446601868
2.81412935256958 7.0710186958313
-1.84052920341492 0.0753187090158463
-3.285325050354 0.0419116094708443
0.520609319210052 0.323089122772217
-0.0246596746146679 0.908864736557007
-1.61205887794495 0.188085436820984
-1.48752963542938 -0.535472273826599
-0.428596973419189 -0.474750757217407
0.795858144760132 -0.712208271026611
-1.00793886184692 0.234603181481361
0.930856704711914 0.54729837179184
1.723353266716 -0.248993471264839
-2.27874135971069 0.203209072351456
-1.89935255050659 -0.77480673789978
1.5449800491333 -1.88089621067047
-2.72387003898621 0.0748473927378654
0.16100312769413 -0.234877422451973
-2.49521493911743 -0.438482582569122
-0.988862276077271 -0.322359830141068
1.72439622879028 2.92774057388306
-3.07767796516418 -0.207206636667252
0.100950844585896 -0.637427628040314
-0.512170433998108 0.580296456813812
1.35514354705811 -1.02072489261627
1.11099910736084 0.715460062026978
-1.54336023330688 0.363684952259064
-0.154889553785324 0.267839282751083
-5.59397840499878 0.00156310945749283
0.60614287853241 0.0457616150379181
-1.46310496330261 0.293733388185501
0.944440484046936 0.468784600496292
-3.10833501815796 0.00724167376756668
-2.48870754241943 -0.308393895626068
-1.31577920913696 0.304998576641083
-0.781160712242126 -0.738351583480835
1.08946740627289 1.14278495311737
-0.18799889087677 1.70337545871735
2.23773670196533 1.21157670021057
-0.70874559879303 -1.01986515522003
-1.52493739128113 0.20852917432785
-2.12956118583679 -0.229739308357239
-1.46747553348541 0.334592252969742
-1.15193009376526 0.553865015506744
2.26766538619995 -5.03235101699829
-0.249821722507477 0.64057981967926
-4.84160661697388 0.0842009782791138
-0.526414155960083 -1.03127729892731
-0.669137179851532 0.0914144217967987
-0.564926743507385 -0.173162594437599
0.541744470596313 -0.277314305305481
-1.04937028884888 0.517159402370453
1.24139213562012 2.81696748733521
2.2457799911499 0.27226448059082
3.01698684692383 6.46112823486328
2.111656665802 2.62923550605774
1.72986197471619 -3.86055397987366
1.65126299858093 0.914274215698242
-1.97601532936096 -0.277552783489227
-1.16020619869232 -0.712480187416077
-2.71697425842285 -0.373425722122192
-3.20513486862183 -0.0890562608838081
0.735071957111359 1.41952240467072
-2.45521640777588 -0.109426811337471
-0.367419868707657 -0.424759864807129
-2.28758955001831 0.0728573501110077
-1.36698079109192 -0.358486473560333
0.397394001483917 -0.637798726558685
-1.07227063179016 0.113608598709106
2.04155302047729 -3.7489755153656
-0.061146080493927 0.319353044033051
-0.0994570627808571 0.26963472366333
1.80444514751434 0.541776120662689
-1.70904672145844 -0.357043504714966
-2.34367418289185 0.431398510932922
1.4876344203949 1.19191515445709
1.83886361122131 2.83031511306763
1.4185094833374 -2.01858711242676
-0.965271770954132 -0.264544010162354
0.701210737228394 -0.0168182179331779
-0.762296199798584 -0.928937673568726
0.224663525819778 0.949767827987671
-2.17141151428223 -0.0090881772339344
-2.52881526947021 0.182941734790802
1.07563674449921 -1.19400358200073
0.953138768672943 0.707589447498322
0.373957872390747 -1.98436880111694
0.948830604553223 0.451556444168091
-1.35127115249634 -0.240816175937653
-2.82665824890137 -0.275961339473724
1.19863057136536 -2.33323454856873
1.39304876327515 -0.546856760978699
1.88389360904694 -0.36340057849884
0.180966109037399 -1.40935230255127
-3.80766654014587 -0.48312970995903
-0.274620831012726 0.435422122478485
0.54248982667923 -0.561477780342102
-3.42559361457825 -0.113729178905487
-5.35481739044189 0.0374784916639328
0.61920177936554 0.315201222896576
-1.51285123825073 0.266309559345245
-2.83676600456238 -0.143157541751862
0.24719475209713 1.26449346542358
-2.38599562644958 0.0117130363360047
0.564177989959717 1.56808888912201
-2.76662445068359 0.251633256673813
0.490609705448151 0.416583836078644
1.57543849945068 2.79083108901978
-4.12885713577271 -0.00200626999139786
1.10017740726471 0.843154966831207
1.55790746212006 -0.066156417131424
0.261978954076767 0.800783455371857
-1.67676389217377 -0.402629226446152
-1.09356164932251 0.448379397392273
-1.12825405597687 0.663697242736816
-0.782061576843262 -0.269397348165512
-0.66595447063446 0.32949823141098
-3.16750168800354 -0.305078566074371
-3.31036710739136 -0.147149816155434
-0.569927394390106 -0.056604877114296
-3.31937074661255 -0.296877056360245
-0.38116466999054 0.697961211204529
-0.733758926391602 0.209398418664932
-2.42658066749573 -0.203604131937027
-4.50017499923706 0.130751550197601
0.792226314544678 0.664919793605804
-0.842954039573669 0.0448162779211998
-2.98343539237976 -0.0903756767511368
-5.17192792892456 0.106129340827465
};


==> figures/visualizations/gmm40/aft_samples.tex <==
\addplot [semithick, aft, opacity=0.7, mark=*, mark size=3, mark options={solid}, only marks]
table {%
10.5478382110596 36.2195777893066
-9.8241024017334 29.670654296875
-2.00713419914246 10.5764665603638
26.1127376556396 18.7661781311035
23.6409816741943 -14.6724653244019
1.19608664512634 -27.2930774688721
12.9120931625366 38.4612846374512
25.016092300415 -17.9033985137939
12.723484992981 39.0898628234863
6.21838712692261 38.647518157959
-0.172427281737328 -21.4903030395508
-40.8911590576172 -20.6168594360352
1.1078907251358 -13.3343191146851
-6.60122728347778 11.6206560134888
-39.1637191772461 -31.2618179321289
-38.3207893371582 20.2509136199951
21.8317279815674 -9.49880981445312
-14.2679166793823 18.3782157897949
11.5219764709473 -30.0707397460938
24.9054222106934 -28.3387870788574
-15.2278003692627 18.4156970977783
9.50606155395508 29.1275730133057
-4.39291763305664 38.4111785888672
-1.81561994552612 -15.2066240310669
21.6563892364502 -1.76280951499939
23.4155387878418 17.2023029327393
-7.01262092590332 20.7668895721436
-38.7744979858398 -29.4690341949463
0.592457592487335 -11.4366960525513
18.9486770629883 22.4313659667969
0.586577296257019 -27.232738494873
-3.64802575111389 32.2168502807617
-8.4950532913208 19.0171947479248
37.0792350769043 4.60339450836182
1.58549129962921 -28.5868854522705
11.6146278381348 31.1961498260498
-16.4429874420166 23.4483909606934
-33.6597328186035 22.1250858306885
29.6486892700195 -10.3524799346924
18.6681308746338 -0.697240114212036
25.3916873931885 -38.8960456848145
-31.975456237793 40.2140007019043
18.5964107513428 23.642541885376
-3.53623414039612 30.6972637176514
18.00390625 3.27993392944336
13.3124589920044 28.3154106140137
1.05754327774048 -15.5112361907959
-5.69142293930054 0.746351182460785
5.79662275314331 4.8645167350769
-38.993236541748 21.3414363861084
-16.1501445770264 17.9624996185303
-19.7774105072021 16.5394535064697
-38.9370727539062 19.1234531402588
-7.77849245071411 29.3563594818115
2.17218255996704 -21.7263698577881
-5.46027898788452 30.2548866271973
6.52302217483521 0.90077418088913
-33.378173828125 37.2326965332031
1.85648953914642 -21.2436084747314
27.3599243164062 -27.3025341033936
25.700927734375 -36.011157989502
-23.7804718017578 26.9507255554199
-32.260124206543 38.8593635559082
10.3124380111694 27.8073692321777
6.47170925140381 39.3456153869629
-1.86102533340454 39.5283126831055
19.605785369873 0.910371899604797
21.944953918457 25.8183631896973
21.1519088745117 0.707971334457397
-5.3336296081543 12.5119771957397
6.43544864654541 2.82313704490662
21.9658679962158 -36.6645278930664
12.0170125961304 -26.4756870269775
-32.509708404541 36.056510925293
10.3001441955566 27.3901653289795
9.60605430603027 35.6841239929199
22.7345809936523 28.5031185150146
34.6708183288574 -11.7766828536987
-0.904690682888031 37.3755989074707
4.72732973098755 2.38511800765991
-30.564474105835 37.3425254821777
17.0591144561768 20.4654388427734
-23.9094123840332 21.2185459136963
5.32112884521484 41.8741798400879
29.549259185791 -15.4060583114624
-4.54323101043701 32.3291473388672
-9.47119235992432 29.1382236480713
27.1735210418701 -11.9135684967041
20.5780048370361 24.6259860992432
31.4498767852783 -8.12665939331055
19.0752601623535 -25.811351776123
-3.74970626831055 11.2631549835205
33.3291053771973 5.19474649429321
34.0029335021973 -15.4287261962891
14.5825672149658 -30.6423511505127
26.4923763275146 18.2637691497803
-3.93359613418579 1.72897064685822
-6.79227209091187 13.0758075714111
11.9288139343262 26.3090209960938
15.1544055938721 -28.5908374786377
12.3907699584961 39.2111282348633
-35.8617210388184 -34.7493705749512
-1.1341587305069 -11.7311353683472
22.007152557373 -14.4831457138062
-40.795654296875 20.8723278045654
17.6883926391602 -4.74472332000732
0.696078479290009 -30.2028141021729
24.0690250396729 -15.7172908782959
16.6071147918701 -6.06198978424072
1.01474595069885 -0.741632699966431
-37.1961708068848 -19.3737716674805
21.0517120361328 -12.7869234085083
32.8108291625977 -11.177529335022
18.2632293701172 -10.7324495315552
26.9510955810547 15.4670476913452
5.6272668838501 4.2599983215332
19.599889755249 1.24660158157349
9.90941333770752 -26.4785022735596
1.46426093578339 -19.5692749023438
29.0350112915039 -11.4083127975464
-16.7671737670898 19.5998077392578
26.4348430633545 23.1111755371094
19.5368003845215 -1.81523561477661
10.7637300491333 37.93115234375
-40.028205871582 -22.2665481567383
-23.3035202026367 18.4150829315186
9.88187503814697 -26.3813571929932
10.7246751785278 34.5622673034668
-4.86856985092163 17.8397026062012
22.2510452270508 0.31619530916214
24.252384185791 18.0680751800537
-19.1828231811523 22.9036731719971
33.6177825927734 36.412784576416
23.6594409942627 -15.8249454498291
-33.1760864257812 36.4980049133301
22.8159198760986 -0.0766769424080849
30.2093486785889 38.0340919494629
20.0398349761963 -6.60518884658813
-1.09300780296326 -23.0605049133301
-23.2336864471436 21.0161762237549
-8.0283203125 17.2289447784424
0.996866941452026 -20.9243354797363
28.4868183135986 -28.7286834716797
5.60786771774292 3.52898454666138
17.9552974700928 -6.09907674789429
11.7221565246582 -27.3282794952393
12.0148105621338 -26.8796634674072
-14.148720741272 36.2709007263184
-6.03655576705933 30.6111392974854
1.4536452293396 -12.5223627090454
23.2775020599365 -29.2687358856201
20.1775150299072 -6.28872537612915
21.9397792816162 -15.2156438827515
-7.72633171081543 9.81013298034668
25.0087699890137 -37.7899169921875
16.9354724884033 -13.6280517578125
-7.70899343490601 28.2554016113281
0.499477088451385 -26.0548801422119
13.2801532745361 -27.5208530426025
11.523175239563 29.9617977142334
1.73176968097687 -29.9047431945801
25.8998756408691 -28.0743637084961
22.7516899108887 -26.0493640899658
15.3741397857666 -11.5768089294434
-38.7007789611816 -31.3426208496094
-16.9025630950928 20.5150165557861
24.7998161315918 -35.201473236084
-33.1834106445312 35.7783851623535
28.5423812866211 -13.4960842132568
34.5124092102051 7.96461153030396
19.9405784606934 23.473295211792
-21.1215953826904 20.1560516357422
36.8184928894043 7.79853057861328
-8.7727108001709 17.9706344604492
7.0038857460022 4.0086669921875
-34.8066215515137 38.2599182128906
10.2621688842773 -26.4033985137939
-0.21197871863842 38.4516983032227
1.55448853969574 -27.5528526306152
36.2554054260254 -12.3665924072266
24.4985733032227 -27.4237632751465
19.6127624511719 22.1788997650146
34.808837890625 -11.0927734375
19.4554443359375 1.28688395023346
-15.9221439361572 23.9134063720703
-39.4980964660645 -24.7906017303467
26.7716083526611 -27.5862007141113
-3.01067042350769 -8.61681842803955
-14.3482341766357 18.8058090209961
17.5836601257324 -6.47437238693237
5.06437540054321 38.5416297912598
-12.8642444610596 35.0075187683105
16.6447086334229 22.5070304870605
16.5398921966553 -11.9816913604736
34.1420631408691 -15.7593946456909
33.1267433166504 36.5392723083496
35.0202293395996 4.11492490768433
18.9816608428955 23.0197200775146
0.380135357379913 0.678176939487457
34.1557159423828 -16.05788230896
17.4772644042969 -6.17795324325562
-2.09310412406921 2.7818751335144
-35.5251770019531 23.7862358093262
23.4600772857666 -35.6202850341797
-1.81314849853516 -1.25907623767853
-22.7704162597656 18.2647285461426
-34.5143165588379 19.3612899780273
19.5744800567627 -8.48196983337402
15.8511934280396 -3.73272252082825
34.0117988586426 -12.1905660629272
36.0672378540039 6.45910453796387
-0.518045961856842 -22.8787078857422
21.7674293518066 23.3263816833496
21.8626613616943 1.24237763881683
-3.63516044616699 28.1273612976074
30.6678695678711 -14.2973318099976
-29.1249103546143 40.1969261169434
-38.6835250854492 -22.8015575408936
26.1407356262207 -24.1154136657715
23.172082901001 0.495928525924683
6.33981513977051 37.2704696655273
20.6399955749512 -7.62259721755981
21.9127292633057 17.8376407623291
17.3925533294678 -5.09355163574219
-32.6978797912598 39.7124710083008
14.4414539337158 36.1134605407715
19.1802806854248 23.4790859222412
4.98332929611206 -12.4283485412598
33.8657264709473 33.8970108032227
-37.8027992248535 22.3102741241455
4.36554670333862 3.56304979324341
26.7353267669678 -38.818531036377
-6.57919502258301 15.6906127929688
15.064003944397 -26.0360279083252
32.787036895752 -15.1673746109009
-23.6620540618896 19.3861217498779
-5.60926532745361 13.9883279800415
-1.11939215660095 1.68909215927124
35.8976440429688 -13.0492362976074
-0.0843762531876564 -12.3448057174683
10.9290142059326 40.4286994934082
6.21102142333984 34.7452049255371
31.8304386138916 -12.2745656967163
33.3375625610352 36.8224067687988
-1.50104796886444 27.1606063842773
12.7855348587036 40.5731201171875
36.8165397644043 2.2898850440979
38.1755905151367 4.22488307952881
1.27976632118225 -21.4770259857178
26.3024921417236 -26.0277729034424
8.36483287811279 28.8482761383057
-5.36365985870361 30.5259609222412
-20.3795795440674 20.8846397399902
11.5221014022827 26.9719390869141
29.4938850402832 -13.9106559753418
4.94479513168335 39.7629814147949
12.8392190933228 37.9595985412598
17.7285003662109 26.0499515533447
-23.1612873077393 21.3302268981934
23.7056121826172 -24.6151294708252
32.6124229431152 7.54075241088867
0.783310413360596 -13.0669956207275
1.86208713054657 -13.679235458374
4.94580125808716 3.02414393424988
26.7867774963379 -29.9698181152344
-11.0153350830078 26.8216724395752
25.5707626342773 -14.3793745040894
-2.53791403770447 12.2294301986694
-4.19474983215332 31.1413707733154
11.5812616348267 29.4446620941162
9.83290386199951 -28.9571208953857
-16.1867904663086 21.6051807403564
-2.33034157752991 28.9503879547119
-16.1568717956543 38.943733215332
10.1992950439453 -28.2159652709961
0.269099682569504 -13.090277671814
10.8187093734741 39.5035743713379
12.1128149032593 27.7798156738281
14.0105323791504 -25.5000839233398
22.0167961120605 -27.7378749847412
-5.9623966217041 20.0009212493896
5.67765855789185 2.80336046218872
21.3332138061523 18.024471282959
-7.80950927734375 17.0804977416992
23.1139850616455 -26.9576950073242
-14.8200998306274 23.3897895812988
-21.848575592041 18.8293972015381
-1.47144854068756 29.0958595275879
16.8463096618652 25.9495105743408
24.0157814025879 -24.9516201019287
-1.14598762989044 37.7910232543945
12.6892423629761 35.0112037658691
-10.9195747375488 19.7496433258057
12.2032680511475 -24.8376655578613
-5.54507637023926 9.24912738800049
13.0463371276855 -26.1989269256592
5.75999689102173 2.96612548828125
1.66518723964691 -27.3600063323975
3.11046886444092 -11.7141456604004
2.68979477882385 38.4561882019043
-40.2894058227539 -30.3160743713379
34.6968116760254 -11.9072332382202
10.952579498291 -27.9091148376465
6.07148694992065 8.09250640869141
-22.3785648345947 23.1732196807861
5.98156452178955 39.5076637268066
19.2091083526611 20.1632308959961
25.2682781219482 -37.7365264892578
21.1403636932373 22.4545192718506
33.3248710632324 -15.7319402694702
-0.754950642585754 -27.9800930023193
22.9531536102295 0.138760834932327
-9.32429790496826 27.6530570983887
-20.0701465606689 21.8755226135254
-4.54653072357178 17.1282901763916
-0.739277541637421 40.4302139282227
-0.534511387348175 37.1852378845215
8.09977626800537 28.8031387329102
-2.27975082397461 32.1248245239258
-4.55020427703857 12.6332445144653
20.849702835083 -6.11483287811279
12.0099267959595 36.8926620483398
19.1416358947754 21.5251522064209
7.36799478530884 41.2016220092773
-32.6070556640625 -31.7856979370117
-14.9445877075195 36.0256958007812
-35.3992919921875 -21.8689422607422
14.0822792053223 -26.1757411956787
34.4946365356445 -13.2800912857056
-3.86264395713806 4.4053053855896
28.2253189086914 -13.310754776001
34.4666862487793 5.02042961120605
14.260443687439 29.6303787231445
-31.3181838989258 38.5812454223633
24.6561450958252 -27.1827392578125
10.6533422470093 -24.6450672149658
-15.710150718689 18.3610305786133
-15.5798835754395 33.7497291564941
-29.9827823638916 40.9186859130859
24.1580486297607 0.455730080604553
26.4759006500244 -9.76284599304199
29.4019107818604 -15.8231086730957
34.9860954284668 5.58293914794922
21.0562534332275 -8.00215339660645
23.132640838623 -38.8866806030273
28.980785369873 -10.9084720611572
4.05867147445679 -13.7904272079468
25.0876636505127 -37.3290481567383
15.7448644638062 -1.00360369682312
22.6111316680908 -26.019868850708
0.502345442771912 -14.9010696411133
-36.9819869995117 19.544017791748
35.6199417114258 -13.6890096664429
-37.8297882080078 -23.4844646453857
32.7519874572754 -10.6717147827148
-39.6783218383789 -35.3573837280273
-22.9005718231201 20.7864971160889
40.7607231140137 -12.3372106552124
-36.0724906921387 -33.5928840637207
19.3903007507324 -0.084474690258503
20.0193767547607 19.1377868652344
34.212532043457 -14.5443925857544
24.7108459472656 -36.746452331543
24.7118587493896 -36.7884521484375
6.4505443572998 4.79025030136108
12.750207901001 34.6949348449707
-1.03738808631897 -19.6850509643555
-10.6961431503296 25.3006725311279
-0.266010493040085 39.6659736633301
29.8752136230469 -14.4940118789673
-1.86420214176178 1.9526139497757
22.1085338592529 -28.5690021514893
-33.9416580200195 35.7819061279297
24.4730892181396 -17.0243854522705
24.6818428039551 -25.2005500793457
-3.77423071861267 2.22927474975586
10.9033603668213 27.3167285919189
-7.81220865249634 20.7554492950439
-0.875725984573364 37.3412322998047
-8.31447124481201 26.993932723999
-3.5419807434082 11.4335250854492
-33.4927291870117 41.2231369018555
20.3407135009766 -0.138100534677505
29.267162322998 -27.6852130889893
4.10090303421021 38.9866752624512
1.79706573486328 -22.0212745666504
18.4785499572754 26.9218349456787
1.45692384243011 -20.7297992706299
-2.79889893531799 2.14766812324524
-3.37664198875427 18.3448238372803
6.40077686309814 3.69023299217224
3.57725715637207 3.87379097938538
25.1143646240234 -37.9221000671387
14.6724729537964 -25.9072933197021
0.743309915065765 -27.2359428405762
11.7158994674683 -28.0684413909912
-35.436824798584 23.2994709014893
-16.1596603393555 20.3189373016357
-37.0052337646484 -20.8849124908447
-6.94463586807251 21.1624946594238
19.8309860229492 -27.4346446990967
20.1538944244385 -3.16980862617493
18.840763092041 -8.692702293396
-39.6924095153809 -31.3099708557129
24.1629314422607 16.0273418426514
29.1127872467041 -10.212438583374
12.4884595870972 -23.3954887390137
-6.44729614257812 12.4130821228027
20.3216304779053 -14.5879678726196
-7.05447864532471 17.0618095397949
18.2812061309814 22.6480464935303
0.248308837413788 40.2517585754395
20.7144031524658 -9.32168769836426
10.7579927444458 37.1160354614258
21.4122295379639 -0.140846267342567
-0.275908410549164 -24.3622207641602
-40.2452011108398 -35.2741584777832
-22.3424472808838 18.4462261199951
-37.835880279541 -30.8392276763916
26.26637840271 -11.1632537841797
27.0751857757568 -38.0904426574707
-36.6861190795898 17.4445877075195
25.9214572906494 -26.2622604370117
-39.2894058227539 15.9299650192261
12.8211479187012 28.5412654876709
8.28980255126953 38.8971252441406
10.0821027755737 -25.3444499969482
-1.16022801399231 -28.6075592041016
-14.5359392166138 38.366138458252
6.24159002304077 38.9841003417969
27.5351886749268 -27.7061862945557
30.9139461517334 37.2792282104492
11.4508180618286 28.9696578979492
0.162411004304886 -21.4927310943604
6.57355976104736 38.6743927001953
33.3427848815918 -15.8880558013916
17.1617393493652 -12.7078151702881
-31.872974395752 36.5475006103516
20.3146419525146 -1.6303334236145
23.0056190490723 0.0290952268987894
12.6471548080444 -26.8875713348389
-38.8173484802246 -22.9027919769287
1.87803947925568 -12.5340385437012
-17.1086578369141 20.9697093963623
-14.930456161499 36.5985221862793
9.646071434021 -24.8050422668457
36.6198883056641 7.22370672225952
2.34539341926575 -11.1942749023438
17.5427646636963 23.55006980896
13.8302974700928 35.0501937866211
27.5491523742676 -9.0910062789917
0.919487059116364 -10.8463039398193
-12.0482778549194 39.2704925537109
26.4073009490967 -37.479305267334
-38.0879058837891 20.9364967346191
-7.23129558563232 14.1541566848755
17.7128162384033 22.5035495758057
-32.7955360412598 36.5021362304688
6.94140577316284 3.6697690486908
13.0587711334229 -25.7858371734619
-33.9476699829102 21.3962650299072
25.171459197998 -14.1072549819946
5.30249500274658 3.33118724822998
-38.5267868041992 -30.9602069854736
1.99261915683746 -28.3855590820312
4.22289943695068 4.87531757354736
11.4971504211426 26.2349071502686
-3.85297250747681 -20.2675628662109
-8.85564041137695 27.8752536773682
26.4409427642822 -11.5904350280762
21.7368450164795 -6.91792488098145
5.78760957717896 6.3301854133606
24.5859394073486 -11.5755472183228
36.0548973083496 -13.0641717910767
-8.09890365600586 21.2888774871826
6.37641477584839 5.72727012634277
-0.967454373836517 41.0166473388672
7.377610206604 3.85850620269775
20.8893165588379 1.80618572235107
6.60915565490723 5.12996816635132
1.80192518234253 -27.885950088501
-9.36701011657715 16.0878715515137
6.83616256713867 5.68993186950684
21.9150924682617 -25.5873394012451
32.7803764343262 -14.6052112579346
-5.40666580200195 11.7148771286011
-1.86231553554535 36.7126808166504
-2.4775013923645 2.0030574798584
0.132338345050812 -12.4163236618042
-14.6576175689697 38.0554542541504
25.4752445220947 -38.346019744873
7.69363737106323 4.76233768463135
-34.5393905639648 38.7400703430176
19.3396339416504 -4.33144950866699
25.5209007263184 20.4668426513672
-0.516794621944427 36.5846939086914
27.4564609527588 -35.060920715332
-35.91259765625 -32.9021644592285
-39.251838684082 20.3210868835449
16.7264709472656 -6.69316911697388
19.9193363189697 25.7534503936768
16.6144485473633 -5.9365382194519
26.1146907806396 -28.7790775299072
30.1265487670898 34.6025466918945
14.352686882019 31.080099105835
4.8864893913269 38.8627586364746
-1.40157794952393 -18.1568412780762
13.7002010345459 -27.6681480407715
1.58905744552612 -12.0417461395264
-3.48525762557983 30.4711380004883
16.6476745605469 -5.26664924621582
31.3711452484131 -11.9579448699951
5.39886569976807 5.74484252929688
-16.2864952087402 21.8194255828857
36.1511306762695 7.61259365081787
-14.6233139038086 35.0331840515137
20.2434635162354 24.253454208374
-15.4028844833374 14.7916669845581
22.2696952819824 -1.52316105365753
-6.36374759674072 26.5885219573975
0.660403370857239 -11.2461490631104
2.98520565032959 -22.1680450439453
34.1396827697754 -13.5239095687866
24.1996459960938 -26.2670574188232
8.99826908111572 -26.5852375030518
-32.0759048461914 40.1174201965332
-18.3646621704102 23.5605773925781
-16.6215057373047 23.5733509063721
11.7671899795532 37.8364868164062
28.9535484313965 -29.1648368835449
19.0857276916504 22.458345413208
5.51794338226318 1.54818820953369
9.37135410308838 33.0934181213379
-30.2949848175049 40.1320991516113
22.6656608581543 -37.2038307189941
-15.389741897583 17.0678462982178
-0.640390694141388 40.5580062866211
-1.11794352531433 -30.2891502380371
32.681095123291 35.140064239502
25.189302444458 -23.2938098907471
-15.8401775360107 37.6753921508789
18.4042549133301 1.47150731086731
22.7711887359619 -24.4998912811279
17.5676784515381 -13.0727596282959
20.468807220459 -17.9937992095947
-34.4789161682129 37.1205024719238
12.0124464035034 39.1255073547363
28.5076675415039 -27.5142822265625
-31.5487003326416 40.6456756591797
-1.32268691062927 -14.1137208938599
-13.4560871124268 35.7300033569336
13.3475503921509 -25.2546520233154
-0.111917294561863 32.5580062866211
26.4942779541016 -13.7012491226196
34.4821014404297 3.61004066467285
25.4393463134766 -39.3845558166504
-35.7332649230957 -29.9604511260986
-2.97007298469543 0.767985343933105
6.81753206253052 3.50026750564575
30.3279056549072 -12.5496473312378
21.7116050720215 17.1426677703857
-0.963526844978333 2.47699546813965
-36.2435150146484 19.7238655090332
26.7191066741943 -12.4690265655518
25.0289211273193 18.3457260131836
-0.531297266483307 -1.25134146213531
-34.1358337402344 19.8382816314697
15.1244955062866 -12.7766246795654
20.4464530944824 23.7993068695068
-4.1369161605835 10.5240697860718
-1.16670608520508 -29.8678894042969
-7.15508699417114 28.2507858276367
21.2179374694824 20.1496849060059
-39.2238426208496 -22.3718147277832
-0.453392893075943 36.0221176147461
23.2310485839844 -0.62522429227829
-2.51433944702148 29.6099262237549
18.2153568267822 -5.35412120819092
2.27388477325439 -13.7057447433472
-19.040189743042 21.4615268707275
6.03465032577515 39.9987640380859
-0.308164268732071 37.4732780456543
13.5950794219971 -25.4512252807617
27.1645526885986 -37.4979629516602
-0.4971042573452 38.8369674682617
18.180700302124 -0.319164425134659
-0.1475580483675 -15.0241756439209
11.118462562561 29.956823348999
-34.189323425293 20.9392147064209
-32.6411170959473 18.909875869751
-0.233126536011696 37.488395690918
-2.3788161277771 1.0707266330719
-15.8231210708618 37.3593902587891
-15.1852369308472 31.9336948394775
-38.0647850036621 -32.4738349914551
25.1121158599854 -25.5536880493164
22.505558013916 -25.8502502441406
2.02193641662598 -12.7683572769165
7.62236976623535 39.8279075622559
32.3889617919922 34.9041862487793
33.6805381774902 4.03091096878052
16.4692401885986 -13.6906776428223
26.8233165740967 21.4731960296631
-8.25037670135498 15.7990570068359
-2.2096426486969 10.6536626815796
9.55289840698242 -27.8547458648682
22.5408687591553 -23.5047073364258
23.3869953155518 16.3669471740723
6.86939430236816 1.50882732868195
19.9272308349609 -8.0453634262085
11.4052429199219 -25.0437107086182
24.7109718322754 -26.7513179779053
-9.34860897064209 28.7782039642334
-30.4930076599121 39.7675704956055
8.28209781646729 4.6102237701416
-2.5200617313385 31.5481605529785
-4.87689018249512 9.91209602355957
-13.2060785293579 33.2525901794434
18.0691680908203 -8.44684028625488
-32.4949417114258 41.5899620056152
-4.67103004455566 20.9543151855469
6.32381820678711 28.480504989624
33.6303787231445 36.6916809082031
-14.1437854766846 17.2830638885498
0.512520492076874 -30.6762180328369
23.9843597412109 -39.3287506103516
24.2599849700928 -0.8666832447052
26.029899597168 20.3543548583984
-28.9859161376953 40.1518516540527
18.7520027160645 25.1514701843262
-2.09385800361633 -30.8294296264648
23.8329772949219 -26.9547691345215
-0.914221048355103 30.8988952636719
17.6142578125 -5.78948211669922
-38.5188064575195 -21.5789985656738
-33.4250030517578 21.3966007232666
-0.651019096374512 -12.2076711654663
26.9491004943848 -25.3313388824463
15.1576280593872 -14.5966968536377
21.4630832672119 -1.04975664615631
21.3998584747314 -23.4147796630859
-36.0762557983398 22.7777233123779
-32.7780456542969 40.6599197387695
29.292537689209 -27.5239334106445
-29.9102401733398 40.491569519043
9.95646858215332 -26.8113822937012
-4.38018608093262 29.5912342071533
25.5762214660645 19.1210250854492
17.1935520172119 -10.2100601196289
2.07464385032654 -12.3601303100586
20.8770713806152 22.8100166320801
1.88410937786102 38.6642799377441
17.7099075317383 -6.90839862823486
-34.7407875061035 40.3843421936035
37.3160591125488 -10.6152372360229
17.7824039459229 -4.28870344161987
18.2607917785645 -8.04838275909424
-5.6887001991272 10.9154853820801
18.7730731964111 25.471715927124
0.510615766048431 39.0546073913574
12.3604078292847 -28.3753395080566
14.6349592208862 -27.814884185791
-3.04846143722534 28.9650363922119
35.4683952331543 6.04859495162964
19.2021503448486 25.9034957885742
20.2909736633301 -7.4886622428894
-32.517017364502 36.9069519042969
24.6762733459473 -39.2765808105469
6.88137435913086 4.64238691329956
13.6976518630981 -24.6321582794189
-32.6962814331055 17.5448169708252
-3.14619517326355 -30.5684986114502
23.7353591918945 -36.0923690795898
20.4779586791992 24.2699222564697
10.9062824249268 26.8830966949463
1.00306284427643 -23.0844497680664
-4.84619379043579 33.7632713317871
-3.34965753555298 30.7743549346924
20.1503219604492 24.4625263214111
20.8701553344727 -26.8217639923096
8.83328342437744 4.71055459976196
35.0474891662598 4.44422578811646
-32.0834121704102 39.7962875366211
-21.3148288726807 19.0163974761963
9.78739547729492 40.1016883850098
0.899272680282593 -12.010760307312
35.109790802002 8.17283344268799
-5.82995128631592 31.3190937042236
18.1225318908691 25.3433589935303
18.7235260009766 25.381519317627
33.1710014343262 -16.7011966705322
4.64397001266479 41.0697822570801
-32.5579795837402 38.4890174865723
-0.512382507324219 40.6165733337402
-4.47724962234497 10.859169960022
19.3276290893555 4.47302913665771
-1.55893301963806 11.3961725234985
-14.3492479324341 17.1166458129883
12.3055248260498 37.6237831115723
14.2309722900391 -11.4576835632324
-18.0236358642578 16.9259738922119
-39.7708396911621 19.9818115234375
11.91441822052 -29.1921787261963
14.9635820388794 -10.7798719406128
34.6945533752441 6.08535528182983
15.7652978897095 -16.2480068206787
-4.15198659896851 19.1085109710693
8.49692726135254 30.1552772521973
16.9750881195068 22.8731803894043
4.4708685874939 4.32419013977051
12.2300844192505 29.6223068237305
-0.594538807868958 -26.7759552001953
-14.1073751449585 36.4819984436035
8.10426235198975 4.38411569595337
-14.8867788314819 13.9204111099243
5.94106674194336 38.9191856384277
20.3884334564209 25.3154964447021
-7.22354459762573 26.1917266845703
33.5790176391602 7.969078540802
39.6217269897461 7.16988468170166
-34.5582962036133 19.9530296325684
-0.784007251262665 -19.2331523895264
-1.56848239898682 40.9165267944336
32.4038543701172 6.01737117767334
-39.4935874938965 -23.961950302124
-29.7659378051758 36.7545204162598
-5.15783452987671 18.8256187438965
-39.5755653381348 19.5374984741211
-32.0827140808105 23.5668048858643
-30.9232883453369 39.2167816162109
4.71153974533081 4.26325845718384
26.5584316253662 -12.9524002075195
12.5537014007568 -10.8819665908813
-37.523567199707 -29.6928539276123
-13.0294313430786 36.8681030273438
26.0445976257324 -38.3516159057617
12.0289039611816 29.172534942627
0.246587723493576 -29.4772891998291
-12.7822637557983 20.8837242126465
-11.5298805236816 39.0202865600586
-9.22913265228271 16.0061149597168
34.756519317627 7.85954189300537
-2.62609171867371 39.5363655090332
21.7614421844482 -15.4582834243774
-32.8553199768066 37.3442459106445
-1.66515862941742 -27.8567810058594
23.9215850830078 -37.2377586364746
-14.2555360794067 37.0419692993164
1.06957542896271 -13.428747177124
9.76583576202393 -23.6393451690674
1.15386545658112 -10.8709888458252
-1.78952443599701 -22.5823059082031
21.1689414978027 0.757507503032684
16.4238471984863 20.7698135375977
12.1913118362427 30.3564014434814
-20.8633823394775 20.6125564575195
-15.7822885513306 38.2408981323242
11.601583480835 -26.5697116851807
-38.4699821472168 -21.4786987304688
14.69020652771 36.2778167724609
0.591508030891418 -14.1509428024292
-6.97927141189575 29.6725845336914
11.8678131103516 26.0503482818604
15.4369773864746 38.758602142334
14.844407081604 -27.3560657501221
-3.72641515731812 31.9668617248535
26.057788848877 -24.6764888763428
-0.469110310077667 39.5478858947754
-14.9554996490479 37.7634887695312
35.6166648864746 -14.7679471969604
5.84131050109863 3.27827739715576
24.3230323791504 15.6457471847534
28.7220668792725 -26.6345272064209
22.7686614990234 -0.214228421449661
-6.09351634979248 11.7593803405762
18.8215885162354 -14.3303442001343
12.0522727966309 28.1747131347656
12.9013404846191 27.2389621734619
12.9175729751587 41.5048675537109
34.4329833984375 -12.7006225585938
15.6052904129028 -13.9282169342041
-1.57715952396393 37.8020858764648
-4.61548805236816 0.550932168960571
39.637622833252 -12.4033870697021
0.770723819732666 40.2138404846191
35.8703994750977 3.62368631362915
2.57971811294556 -22.1806221008301
35.4525833129883 7.08622026443481
-7.4776782989502 19.6750831604004
21.9291648864746 -8.0388298034668
18.2833099365234 25.8896369934082
22.1397552490234 24.1618347167969
8.23537921905518 0.90480238199234
-6.71303081512451 8.20698642730713
-14.4290933609009 33.6317329406738
-41.0584335327148 20.7678451538086
25.5203952789307 22.7447986602783
-36.7114295959473 16.5793209075928
1.5215756893158 -28.2111778259277
34.9380798339844 37.0878448486328
-3.11778831481934 27.6682090759277
17.3415794372559 21.3615550994873
-13.7257423400879 37.5380668640137
-6.40229225158691 9.51871967315674
-28.9381847381592 36.8997383117676
1.14374005794525 -23.0036106109619
34.4938201904297 6.18573665618896
23.918872833252 -25.165994644165
19.2947731018066 25.5251522064209
-7.77715015411377 18.4017105102539
26.727912902832 -24.316463470459
0.500161170959473 38.0007247924805
3.34756016731262 -22.3939361572266
21.2680644989014 -29.0676345825195
17.7251491546631 -1.41461336612701
1.96125245094299 -12.8418407440186
-6.16136884689331 14.2413110733032
31.39035987854 4.58418369293213
32.7746620178223 36.9105606079102
-1.57760620117188 33.0202522277832
-4.28947401046753 11.7477426528931
19.0251369476318 -7.47339200973511
-36.8117599487305 -35.3433456420898
2.77159714698792 -20.6982326507568
-16.4624862670898 19.1189918518066
28.1752109527588 -37.9024505615234
20.8835010528564 1.52975761890411
13.5341758728027 26.6073246002197
23.7831554412842 -27.0956020355225
31.684534072876 -15.1351375579834
38.0032577514648 -13.2447786331177
-16.4973964691162 35.8096733093262
17.9987945556641 20.5726699829102
37.0692863464355 -9.80259609222412
12.3137073516846 -27.7224903106689
21.5217189788818 -13.2801427841187
6.86438703536987 5.01440858840942
-33.5800514221191 19.9084224700928
1.23841905593872 -12.6832323074341
-14.7219753265381 37.1649703979492
-39.1094169616699 -31.2504272460938
21.0182361602783 -2.40126752853394
-17.1762542724609 22.7499904632568
-6.01694917678833 18.2665386199951
-0.508317947387695 36.808780670166
-6.28856372833252 29.2240257263184
11.2429466247559 -26.0237293243408
11.4751462936401 29.328104019165
0.119299031794071 41.7927322387695
24.1285705566406 0.670651137828827
2.38443565368652 -11.6817007064819
31.4263439178467 34.4635772705078
-37.2596817016602 -23.927526473999
-15.2619657516479 19.6079654693604
18.1826496124268 23.4277114868164
6.03705787658691 4.78468132019043
35.9085273742676 -14.6645345687866
-37.4884338378906 -32.4897003173828
24.4021663665771 19.8488006591797
21.3502655029297 -8.45398426055908
34.4543304443359 -12.753454208374
10.8459215164185 26.3387775421143
12.3863954544067 38.795524597168
0.646432995796204 -13.6313009262085
12.858567237854 -27.6436748504639
-35.9687690734863 20.9677505493164
16.589298248291 -6.9594874382019
6.8612585067749 4.71901750564575
0.227722644805908 -22.2707748413086
11.6044855117798 28.8604373931885
21.733865737915 1.46014058589935
13.6619701385498 -26.4485511779785
5.10139560699463 39.4014434814453
10.6809244155884 -29.8501987457275
5.34591865539551 3.39046716690063
-22.0595893859863 21.1245555877686
-6.15213298797607 16.1665840148926
-0.0382911451160908 -21.1214199066162
-10.9956350326538 29.6811618804932
2.79874658584595 -22.816650390625
2.47065591812134 -29.8989524841309
2.10162949562073 -16.8845920562744
-8.17567157745361 28.0888290405273
2.8884449005127 -19.7148151397705
26.9716033935547 -29.240140914917
-38.3197059631348 -22.5023345947266
-32.1177787780762 22.1709842681885
31.5325393676758 -9.71828365325928
21.9507751464844 -23.1471881866455
21.700159072876 -22.63743019104
33.4241065979004 37.8631057739258
-38.3843307495117 -34.8404998779297
-31.4503612518311 37.8894844055176
20.6066474914551 -13.0765008926392
-38.1368637084961 -30.769495010376
7.00033092498779 4.06333494186401
22.1835823059082 -0.882887661457062
25.1234378814697 -9.0699987411499
12.1483793258667 -30.1521911621094
27.1466255187988 17.9654808044434
33.888744354248 34.892936706543
-13.3637075424194 36.2679252624512
-16.388069152832 38.0101051330566
-1.86463809013367 12.4341831207275
-5.81463813781738 13.8680543899536
2.25395965576172 -11.1449575424194
-13.8075132369995 37.5398025512695
5.25936794281006 -22.9718189239502
24.8935718536377 22.898775100708
37.6672706604004 -14.3804168701172
37.4690971374512 -13.3464031219482
34.6391181945801 36.5340461730957
1.73209369182587 -27.459867477417
17.8450717926025 -15.6434869766235
24.1678066253662 -25.693000793457
32.416675567627 -15.1082677841187
26.4961853027344 -24.7621154785156
-0.346073806285858 -23.3327121734619
2.4289014339447 -9.768630027771
-7.68114757537842 28.2137851715088
-35.5461578369141 18.1187801361084
-38.4140243530273 20.9912719726562
28.2483806610107 -37.6706123352051
-1.07646691799164 -27.9716053009033
17.7774066925049 -6.28686857223511
0.738413274288177 -18.9180507659912
9.89537143707275 -26.0283031463623
-5.05923128128052 -1.62778985500336
-8.961106300354 18.8289203643799
27.775821685791 -37.1496734619141
24.673900604248 -38.5318031311035
-9.22539138793945 29.6971530914307
0.681032478809357 -20.1972751617432
22.1880435943604 -7.69937038421631
35.8661270141602 -11.4471235275269
26.8050785064697 -26.5176124572754
28.5115222930908 -12.584451675415
-35.1766777038574 39.9957237243652
17.6292018890381 -14.8772611618042
23.4634761810303 16.7194442749023
39.3329887390137 -12.2956705093384
34.3951683044434 4.86936140060425
-18.7135620117188 19.1992511749268
8.05090713500977 39.9343452453613
19.421724319458 -9.39884471893311
-8.44279479980469 25.9368057250977
-1.68847453594208 -13.3068361282349
-3.00507783889771 37.033519744873
20.9425659179688 -2.41699385643005
5.89601469039917 41.2778053283691
-2.72415208816528 1.0705314874649
31.1343803405762 -13.8787126541138
23.3090705871582 19.0836029052734
10.8208103179932 29.6052513122559
-13.8957433700562 37.567195892334
19.0442008972168 -6.73776054382324
-31.6368427276611 19.3856678009033
24.9186935424805 -36.0971488952637
-40.9345855712891 -24.7733058929443
17.3370552062988 -3.06796622276306
11.1581516265869 37.4909820556641
-37.7290458679199 18.2977600097656
9.84551334381104 28.0358486175537
23.4864482879639 -36.3836975097656
10.6868343353271 25.4585056304932
12.9314088821411 34.094799041748
1.01434409618378 -13.4591846466064
-1.49585390090942 38.4743766784668
19.4012794494629 0.404709279537201
-3.91387605667114 14.8847713470459
25.6388893127441 -27.0323677062988
-20.5188617706299 23.0087547302246
3.24629426002502 -9.78822422027588
-5.7830605506897 16.5936012268066
5.85440158843994 40.4463005065918
19.8489284515381 -12.0250759124756
10.9049224853516 -25.885555267334
-0.664575457572937 -29.5837230682373
22.1501979827881 -2.62386226654053
25.7661094665527 -37.4416770935059
25.4711284637451 -23.4596691131592
4.18764305114746 38.0401344299316
-37.4980392456055 -21.3392696380615
-35.4301605224609 38.760326385498
-38.5987091064453 20.3406467437744
22.4450054168701 1.28966617584229
-7.18837070465088 20.1188907623291
21.9020290374756 -12.6118230819702
20.0882701873779 -6.37966680526733
7.55275583267212 -0.00381412520073354
18.7957782745361 -2.23984146118164
-5.13191175460815 13.0034999847412
-39.0922431945801 -21.3934555053711
9.97587776184082 28.9759788513184
0.110094733536243 -0.543362021446228
18.0967922210693 -0.0455393120646477
-34.7874145507812 37.3528785705566
-5.84749984741211 15.3135099411011
29.1161403656006 -12.6457576751709
6.21513414382935 4.42948913574219
};


==> figures/visualizations/gmm40/cmcd_samples.tex <==
\addplot [semithick, cmcd, opacity=0.7, mark=*, mark size=3, mark options={solid}, only marks]
table {%
22.443998336792 -1.25115549564362
-7.03655624389648 11.1320533752441
-5.93368577957153 17.7610759735107
-7.10702276229858 11.3678331375122
-3.65924263000488 -0.859875023365021
-9.67302322387695 18.6583385467529
7.05827808380127 3.76871752738953
-2.1907958984375 1.01666378974915
-0.0557042211294174 -14.2695722579956
-3.27757000923157 0.360478609800339
-7.01077747344971 19.6798477172852
-18.3436603546143 20.9354515075684
-3.93895411491394 11.8921298980713
-6.43587398529053 11.2045555114746
-7.33057880401611 18.3885269165039
-8.411865234375 18.3274631500244
5.09626626968384 4.16442203521729
-5.90057325363159 1.78653454780579
21.8944931030273 -0.0480992533266544
7.04599666595459 3.06548810005188
7.09522676467896 4.03412771224976
-2.32915711402893 -1.14523208141327
-5.03274822235107 11.0574350357056
35.0774803161621 5.1697998046875
-4.10898780822754 1.88541781902313
-2.99065732955933 0.856290996074677
7.9880542755127 3.44946265220642
-3.28824400901794 11.581015586853
-2.29128789901733 0.37858834862709
-5.38211250305176 11.8220233917236
4.81133937835693 4.89788770675659
7.1483850479126 2.68732070922852
-3.11127591133118 -0.0030985726043582
-4.90220546722412 10.3896293640137
-4.22402572631836 10.8846406936646
-1.70477342605591 3.60124540328979
-20.1729068756104 20.351505279541
-2.82753539085388 0.914869666099548
-16.6696109771729 35.2561378479004
-3.00173664093018 2.38878273963928
-7.87251615524292 20.4842395782471
21.6001625061035 0.658274173736572
-5.28187131881714 18.3893566131592
-17.8989448547363 20.7171840667725
20.5208911895752 -9.10946464538574
20.885570526123 -7.30546522140503
-2.48635816574097 1.0425271987915
-4.19870662689209 1.35569334030151
5.61797857284546 3.99237108230591
17.7956237792969 -7.24878740310669
-2.79299283027649 1.27036273479462
-6.40181684494019 10.661602973938
-4.32306957244873 -2.28783845901489
-7.01959991455078 19.4671077728271
9.16537380218506 5.55893230438232
-3.79323816299438 1.01518070697784
5.80449867248535 3.46172857284546
20.0547828674316 -0.538999676704407
-4.86306858062744 12.113000869751
7.99955320358276 3.97999262809753
-5.09648132324219 13.0544843673706
23.9792919158936 17.874195098877
-3.5099766254425 1.12129104137421
24.6379776000977 18.1222305297852
6.1028881072998 3.49703907966614
-3.00974202156067 12.2983560562134
7.19921398162842 6.03970575332642
-4.63300609588623 2.22757577896118
-6.58275032043457 11.4445219039917
-5.01807689666748 10.6754417419434
-0.890162885189056 3.64548063278198
-4.39341259002686 12.5708503723145
22.1159973144531 -0.919837117195129
0.572050034999847 -22.1387462615967
1.31234753131866 -14.7823991775513
6.11447143554688 4.17787218093872
7.60288524627686 2.09444665908813
-8.01417827606201 26.4603748321533
6.4801344871521 3.87273716926575
5.8486008644104 3.16939806938171
-5.00024366378784 11.6330089569092
21.9063606262207 -2.00189900398254
-2.94193530082703 0.447276890277863
7.49345302581787 4.07772350311279
-5.22185468673706 11.8684148788452
6.65948534011841 5.29200887680054
-18.8643817901611 21.5976696014404
-2.97613644599915 -0.336638957262039
-4.85847425460815 13.3024444580078
-4.76489448547363 12.474684715271
7.44745588302612 2.850172996521
-6.19984149932861 11.9241371154785
19.9681529998779 -7.03786563873291
-4.10346269607544 0.97460001707077
-15.7499217987061 34.4269752502441
17.5446434020996 -4.57619476318359
34.137809753418 6.68883228302002
-18.5237655639648 17.1357402801514
-4.91573715209961 11.3475685119629
-3.5256187915802 0.334079533815384
6.88231992721558 4.02580547332764
-2.22155237197876 2.6067636013031
6.62338209152222 4.28606271743774
-10.9073619842529 25.9209938049316
9.13080406188965 4.61474609375
8.81618785858154 3.14586877822876
-3.59271693229675 2.44768309593201
-9.48594951629639 19.455659866333
-0.893783688545227 -1.87858664989471
-2.2256965637207 3.08222436904907
8.5256929397583 4.62371253967285
6.80197191238403 2.48959922790527
-2.60132479667664 -0.297944009304047
-2.91529679298401 1.04001331329346
36.5842323303223 4.8992166519165
-2.3530261516571 0.627819716930389
-7.17594003677368 17.7744140625
6.53585433959961 4.7490234375
6.49008131027222 6.11713838577271
-3.67470383644104 11.1933031082153
5.24302196502686 4.79131078720093
-5.97761869430542 11.9927263259888
20.6833190917969 -0.858810245990753
-3.5556948184967 -0.00897033605724573
9.0042200088501 2.93056058883667
6.53936195373535 4.48262929916382
5.9725399017334 3.66530752182007
34.3729362487793 3.72488951683044
-4.44120597839355 10.4205932617188
34.5694313049316 6.68771314620972
5.21107912063599 4.06323957443237
6.39071321487427 5.43344879150391
-6.89279508590698 10.599781036377
-4.54611873626709 1.64499843120575
7.4826512336731 3.07319307327271
-16.5874099731445 21.8901348114014
7.1931266784668 5.28743076324463
-11.6634664535522 28.1558170318604
-21.6025390625 19.9771137237549
20.5642566680908 0.11578119546175
-2.68919944763184 1.76748907566071
-3.31555223464966 0.0906438156962395
6.81920576095581 2.83052492141724
-5.45163679122925 13.1222724914551
21.1396446228027 -1.43476831912994
-2.52485775947571 30.2644538879395
-9.15249252319336 28.2009201049805
-6.57871866226196 12.6322040557861
-3.89582467079163 1.90312230587006
22.2169437408447 0.192313894629478
-3.54325437545776 -0.604587256908417
-6.07260513305664 10.541130065918
8.48045253753662 5.54834604263306
-6.13767528533936 13.273193359375
-5.87645244598389 9.43759727478027
36.2766418457031 7.26260757446289
34.0439605712891 4.91468477249146
35.5803298950195 4.51204586029053
-4.48313570022583 10.7894792556763
-5.8739218711853 10.54088306427
-1.87500202655792 30.7813262939453
22.5333271026611 0.193853259086609
7.50480079650879 2.58690309524536
-9.67323780059814 17.7158184051514
7.76475715637207 4.43652772903442
-2.59803771972656 0.730599045753479
-2.82233262062073 2.31550717353821
6.57613801956177 4.90062713623047
18.1152477264404 -3.07954716682434
-10.219051361084 18.6566562652588
7.13048505783081 5.09085750579834
-7.55077409744263 17.0757579803467
-7.55667877197266 18.2917232513428
-3.18523216247559 9.22189140319824
-4.42194652557373 11.5355415344238
21.138277053833 -0.79262763261795
-5.95996856689453 11.5254411697388
-3.01803135871887 1.29582321643829
-3.22413110733032 0.269994765520096
-11.527437210083 34.0165710449219
-5.78962850570679 9.62276935577393
19.7193641662598 -7.62531328201294
-2.94715118408203 2.5219783782959
6.08704900741577 4.98079347610474
22.5021018981934 -0.0816799700260162
-0.717855095863342 2.03493213653564
-3.21141934394836 1.4904932975769
7.35466718673706 4.54334163665771
-4.35938501358032 29.8632850646973
-4.00951528549194 11.3140439987183
-6.51542139053345 12.5922060012817
-3.64957761764526 1.0811151266098
-18.9541339874268 20.2553329467773
20.5236206054688 1.93311035633087
0.871029913425446 -11.09010887146
7.49969577789307 5.52763843536377
5.70723152160645 4.87387752532959
-4.62638139724731 1.39080190658569
5.93991708755493 5.41322469711304
6.64293193817139 4.58125734329224
17.7602958679199 -7.40737104415894
-3.14849495887756 13.6563634872437
-2.02952837944031 2.0419065952301
-2.41514277458191 1.36400663852692
-4.67203664779663 9.94688606262207
16.0684967041016 -5.80086421966553
-2.08153319358826 1.13162910938263
20.3582744598389 0.332170426845551
6.41167545318604 2.68460488319397
8.89760684967041 4.87742137908936
7.53285646438599 2.9120180606842
-6.34651708602905 16.4465560913086
6.46936988830566 4.70388317108154
-5.95755767822266 9.46528720855713
21.1434173583984 -1.0604772567749
6.77847528457642 4.72589111328125
8.46706771850586 3.32888531684875
-5.58203792572021 18.9414501190186
7.69678592681885 2.98753094673157
-4.4207239151001 1.06756675243378
20.5024795532227 0.342071920633316
-3.05280613899231 -0.349603027105331
-17.707706451416 21.5080299377441
-1.28330099582672 0.846693694591522
-6.59990692138672 18.511100769043
-5.01675415039062 11.9023866653442
-2.80171918869019 2.36485862731934
-14.3134117126465 38.3381156921387
-5.51603221893311 11.6806840896606
6.97838401794434 5.27480697631836
6.85168218612671 5.00842237472534
-0.983750998973846 1.91407608985901
21.5201454162598 -1.74216496944427
-2.36713743209839 -0.0599645264446735
19.8077850341797 0.325508207082748
6.61599159240723 2.53787708282471
-7.39420461654663 19.1296367645264
-3.9438579082489 0.193911269307137
-4.85970830917358 11.6576461791992
6.90737009048462 4.34269332885742
-3.35416769981384 12.9182691574097
-6.35022878646851 13.6630735397339
-6.02172565460205 17.0058422088623
-4.06040573120117 11.4943113327026
-4.56653594970703 8.94617748260498
7.30844020843506 5.01919317245483
-3.03645586967468 2.68168687820435
-1.78191602230072 0.770151793956757
-0.478426873683929 1.61000037193298
-3.73028373718262 1.19857513904572
6.99413681030273 6.06127452850342
7.39143085479736 4.43370819091797
7.99762487411499 3.70130062103271
-3.1438262462616 0.206541061401367
33.2541580200195 3.86821818351746
7.8021559715271 3.41001152992249
5.35868883132935 2.51950836181641
-6.64609527587891 16.5698776245117
-9.10405826568604 16.7412338256836
-2.85572981834412 1.46016252040863
-3.26038861274719 0.236343100667
19.5814380645752 -9.03941345214844
-1.16058230400085 1.58021306991577
-3.82176399230957 31.7007579803467
-7.08496713638306 17.397029876709
7.36699151992798 6.00390815734863
-6.49601173400879 11.2109880447388
-6.78143215179443 12.8657722473145
35.8126564025879 5.31789207458496
-14.7091493606567 33.9987716674805
-2.26742339134216 -0.00293072313070297
6.91055536270142 4.68370962142944
-2.64552736282349 0.281760275363922
6.76997470855713 6.32483339309692
-5.85060787200928 10.0853691101074
-2.21095108985901 0.650344252586365
-2.07849669456482 0.173469573259354
9.49404907226562 4.31979942321777
6.71040105819702 4.13996171951294
19.914041519165 0.355178356170654
-16.3340187072754 18.4747524261475
21.342342376709 0.238882407546043
-1.96540379524231 1.32647609710693
-6.27977514266968 9.85240745544434
-15.1822195053101 19.227596282959
-5.03311729431152 12.9007110595703
20.5450267791748 0.245608374476433
34.344554901123 6.53294992446899
-8.82870578765869 27.4563732147217
-4.96302223205566 9.30124568939209
6.74343109130859 2.82115960121155
21.4833393096924 0.0522060506045818
-1.95744204521179 11.545768737793
19.3695774078369 0.873786151409149
-6.23268365859985 9.7886381149292
-2.78736209869385 1.21207058429718
5.11973094940186 4.82220363616943
-4.92520713806152 12.0210952758789
-2.96000361442566 2.94762086868286
-3.02551627159119 1.5875096321106
21.2503318786621 -1.17835867404938
-17.6227893829346 23.1926746368408
7.50187730789185 2.63088512420654
-6.4373893737793 19.4890594482422
-4.46334409713745 12.8943891525269
14.9142084121704 -12.7983283996582
-5.63470315933228 12.1548728942871
-12.4578399658203 35.7241058349609
20.0034408569336 -2.38277316093445
18.7297840118408 1.09158527851105
-2.16081428527832 0.686881840229034
7.37844657897949 4.3388032913208
21.2132091522217 0.741750419139862
-5.91989660263062 11.6320953369141
-9.56395149230957 27.1599349975586
6.72665071487427 5.44067430496216
18.9559555053711 -3.51026153564453
-4.28963327407837 12.7636384963989
22.4416656494141 -0.176896318793297
33.5618515014648 5.9211277961731
23.3854656219482 -0.0611073784530163
6.84059858322144 4.03271389007568
-2.69241809844971 -1.87865078449249
-5.85988664627075 11.3535251617432
-0.367047756910324 0.941367030143738
1.31695699691772 -11.1955394744873
-16.6015396118164 18.6977882385254
-14.9379568099976 21.0501823425293
5.99883985519409 4.62726783752441
-4.97760438919067 9.88675308227539
-9.06868648529053 16.9106884002686
6.73167133331299 4.68920230865479
-6.6854681968689 17.917142868042
-4.57082843780518 11.5379953384399
-1.28753197193146 1.04521346092224
-2.1348237991333 1.35298454761505
4.66613340377808 3.37225413322449
21.8365726470947 -8.15930461883545
-3.30772137641907 0.535465836524963
6.06881618499756 3.59544038772583
-5.72319841384888 12.4121170043945
-5.49065351486206 11.5293064117432
-3.65422296524048 -0.505088686943054
-4.74132108688354 11.3681058883667
-2.27631545066833 0.660382091999054
-4.90958023071289 13.099404335022
6.28510904312134 4.20745325088501
-5.54604864120483 11.9771165847778
-3.55357527732849 11.8381700515747
-4.27544260025024 12.5389566421509
-17.1624126434326 20.9286632537842
5.67794609069824 3.8380389213562
7.74266338348389 4.95077180862427
17.325475692749 -5.87453365325928
24.2537498474121 0.19083234667778
-5.45684862136841 16.4864635467529
21.6773128509521 0.995867371559143
-15.5272006988525 18.2981719970703
6.01911544799805 3.46611332893372
-6.04210662841797 12.627571105957
20.523962020874 -0.770928382873535
-6.41370296478271 16.0313014984131
22.35569190979 -0.639854669570923
-5.01139450073242 10.0678691864014
-6.90468597412109 13.2222557067871
-4.89404010772705 12.0914449691772
-7.47101259231567 18.4122161865234
23.2603454589844 1.58337831497192
-3.04598522186279 1.8531391620636
34.4829597473145 6.01653957366943
-7.68624687194824 17.2762451171875
11.8869895935059 29.0140819549561
19.8193054199219 -1.8303816318512
-5.38385057449341 10.5262031555176
-3.33638691902161 1.88217651844025
7.02724123001099 6.05363273620605
-7.87238454818726 12.2392358779907
-16.2015476226807 22.6067485809326
-32.0155143737793 37.9749488830566
-3.6807873249054 10.2255420684814
-3.41075015068054 1.49825143814087
20.3956165313721 0.746993124485016
-6.89885091781616 19.45188331604
-3.1985330581665 -0.515858888626099
-2.34762120246887 2.01264929771423
-2.882732629776 1.85326504707336
-3.66731929779053 12.0717210769653
-1.28289699554443 1.09624695777893
-4.95845127105713 11.3580627441406
-2.84629368782043 0.564750969409943
21.1008434295654 -0.468393385410309
-1.22267997264862 2.46273016929626
18.3575248718262 -4.18814516067505
7.02565002441406 4.65229892730713
-15.6500673294067 19.12619972229
-9.02077198028564 25.7599315643311
21.2182559967041 0.0229305196553469
-14.7000942230225 20.9827709197998
-7.10439014434814 12.5925998687744
-6.00997686386108 19.223970413208
-3.97283363342285 0.0209685694426298
-4.98046350479126 10.8616609573364
-7.81162452697754 9.29666423797607
-3.26911163330078 10.9222850799561
-17.3063278198242 20.3635749816895
-3.36962175369263 0.253406137228012
22.7872200012207 1.29971396923065
16.8369655609131 -3.93489265441895
-0.614891052246094 1.32373833656311
-2.89406871795654 -0.410748094320297
20.6950378417969 0.110683411359787
8.31329345703125 3.63047790527344
-6.40967655181885 11.3175373077393
-0.991257309913635 -0.367498159408569
21.8695259094238 0.932901799678802
-6.67705774307251 17.5581226348877
-1.36984717845917 0.651893615722656
-4.13725757598877 10.6837816238403
-6.45087957382202 17.07834815979
-6.19056081771851 12.6691646575928
6.47217464447021 3.42450213432312
6.2786693572998 3.90062880516052
-7.92902898788452 17.4612236022949
-9.91847705841064 16.4699363708496
35.5320510864258 5.37651014328003
-15.6054439544678 22.3864707946777
6.27033948898315 4.27096128463745
35.9274139404297 8.059157371521
-2.87422132492065 12.0623893737793
6.80407857894897 3.65002417564392
6.9817590713501 4.15080499649048
4.95378017425537 4.2544527053833
-2.40485024452209 2.00276732444763
-2.93758153915405 1.58555507659912
5.96213912963867 2.22114658355713
5.00735759735107 2.69399976730347
-1.31492042541504 1.06627261638641
20.9499263763428 -1.29919421672821
-2.80410575866699 1.05618751049042
-6.83068370819092 17.464879989624
17.4020366668701 -4.57252311706543
-1.13214755058289 2.69990825653076
7.94755697250366 4.12093019485474
35.8302345275879 9.12350082397461
-1.99215042591095 0.0164315719157457
6.33341884613037 2.61337208747864
-2.78151607513428 1.88159358501434
-4.55171203613281 16.4103813171387
-8.58344745635986 18.1300735473633
-16.5419425964355 18.416540145874
5.83541059494019 4.4479832649231
-3.35136747360229 1.09837114810944
-2.45763754844666 1.97036015987396
9.11853790283203 4.97193717956543
1.07311999797821 -9.74350643157959
-5.48523759841919 12.736234664917
-16.830846786499 22.2743587493896
21.5053653717041 -0.273495256900787
-6.94485378265381 11.4526643753052
-2.53354692459106 1.40556025505066
-6.41600704193115 15.977481842041
1.62792873382568 -12.8789615631104
-8.56411170959473 18.3698291778564
-14.2385988235474 35.3863525390625
22.2066135406494 -1.97332036495209
-4.31943082809448 11.2808809280396
-2.44951844215393 0.900258481502533
-6.57484245300293 16.141508102417
-2.78650879859924 1.35483932495117
-4.11328077316284 1.54241228103638
18.1772537231445 -4.67222261428833
-16.1231422424316 17.196195602417
5.07568788528442 3.65796494483948
-0.0500562079250813 -13.3109703063965
7.01330804824829 5.52509689331055
-6.02525234222412 12.248348236084
-9.61046695709229 28.5958919525146
-14.3048133850098 33.1994514465332
4.46611976623535 4.7877049446106
-13.8404445648193 37.1466865539551
-4.53969955444336 9.66933917999268
17.5653476715088 -3.17597031593323
23.1092739105225 -2.62215638160706
-2.97306442260742 -1.59410881996155
-3.35940551757812 1.80364394187927
21.1810455322266 -6.4940972328186
-2.49941873550415 10.1902799606323
-3.4487452507019 12.1783332824707
20.8138942718506 -1.24154710769653
-3.41777777671814 -0.637258648872375
-5.39790964126587 11.472767829895
-4.34194087982178 30.1318740844727
-3.57974982261658 -0.299303740262985
9.26322841644287 4.55748510360718
-5.61629581451416 17.8455238342285
-2.33601117134094 30.3393058776855
-7.38631010055542 10.4043045043945
-4.202561378479 10.7445096969604
34.0891075134277 7.97054004669189
20.0206394195557 -0.597900450229645
-3.21607780456543 0.620630979537964
-4.47077226638794 11.5836210250854
-9.30335998535156 27.9298648834229
5.3276219367981 4.74209928512573
-2.28284811973572 2.81913375854492
15.6394720077515 -6.30901002883911
6.6936182975769 3.3463282585144
-17.2147827148438 17.7241878509521
-3.24636268615723 1.46082615852356
-18.0247459411621 21.4773902893066
-22.040111541748 19.8538722991943
-4.23326301574707 12.0699415206909
6.69285440444946 3.89246916770935
5.83802795410156 5.61675882339478
-17.4007835388184 20.3571453094482
6.42304468154907 5.49269533157349
-2.5442910194397 1.2626610994339
-1.79985189437866 -0.335298597812653
-7.27965497970581 20.5426425933838
-2.47639775276184 0.578943908214569
-8.36414527893066 27.7774982452393
-18.1081428527832 22.4224529266357
-4.20289278030396 2.2343590259552
0.587034702301025 -11.7743701934814
-2.52854466438293 12.5686349868774
5.89900493621826 5.10541534423828
-7.80244731903076 27.0607395172119
-3.34127116203308 1.79171395301819
-9.55314636230469 25.8351421356201
5.80947208404541 4.85504579544067
16.4405345916748 -6.59837532043457
8.42608451843262 4.77679443359375
36.48681640625 5.68898630142212
-1.9953590631485 1.72231328487396
35.970775604248 5.58628749847412
-2.59431886672974 1.09323263168335
-15.6401414871216 17.8948001861572
-2.49738955497742 2.07227754592896
-5.0429539680481 8.67757225036621
6.4392352104187 3.87780666351318
-2.69284272193909 -0.749462366104126
-3.13508582115173 3.08258318901062
5.26206064224243 4.85574436187744
24.8379058837891 1.89733397960663
-3.52421832084656 0.542589247226715
-2.96616101264954 1.39976489543915
-21.6359386444092 20.1802711486816
6.55694913864136 3.59375858306885
6.83830738067627 3.66406631469727
-2.26861047744751 1.64236438274384
20.3328609466553 -0.069157175719738
-3.0936131477356 0.543787717819214
0.986905872821808 -12.5723657608032
-2.4490692615509 1.46084094047546
-19.1432418823242 21.2792949676514
-7.0654091835022 11.6113128662109
-8.22228622436523 28.0347423553467
-5.6353554725647 18.7739887237549
6.9432110786438 4.97891426086426
18.9424152374268 -5.57103538513184
19.2206974029541 -7.98114347457886
-5.82770156860352 10.7384166717529
-5.69156694412231 13.0367527008057
6.73227691650391 4.34279632568359
-13.1379766464233 34.8337249755859
-2.24415373802185 31.9210414886475
-6.65794229507446 18.4261608123779
-2.88647294044495 1.63436532020569
6.88073301315308 4.56796932220459
-18.8227214813232 21.2918968200684
6.55413389205933 4.69016981124878
-3.46887278556824 14.2274160385132
-6.42692184448242 18.1261730194092
-10.1894025802612 27.7473468780518
-14.4828290939331 34.7817268371582
-3.99006533622742 1.36647653579712
7.71123504638672 5.19524621963501
-3.51364612579346 9.58122062683105
-17.1204376220703 17.7736911773682
-5.62369728088379 11.8052339553833
7.40133142471313 4.63041400909424
-4.12469434738159 12.9894218444824
-5.79033422470093 12.3716831207275
-6.62399291992188 18.8704147338867
-10.1702671051025 19.1419830322266
23.1444454193115 18.0236663818359
7.8883228302002 4.92307138442993
-2.82607579231262 0.654597580432892
-4.57863664627075 14.5276670455933
-21.6577091217041 21.1421432495117
20.4623031616211 -1.73048603534698
36.0626831054688 5.580726146698
6.18399477005005 3.62028074264526
6.32582902908325 4.46851634979248
-10.4427356719971 25.0566482543945
5.11791563034058 3.5067982673645
7.27398204803467 3.15830659866333
-8.37973403930664 17.8852863311768
22.1147880554199 0.875205993652344
-3.92402958869934 11.8056974411011
-1.56088483333588 2.155522108078
-15.2185621261597 35.255615234375
6.58735466003418 3.38772416114807
-5.96435403823853 11.0985012054443
-15.9125862121582 36.6061172485352
6.07457160949707 4.827965259552
-4.96941995620728 10.771674156189
22.342435836792 1.33644986152649
21.5488929748535 -0.973219156265259
0.79929506778717 -11.5214281082153
17.3358688354492 -4.83698129653931
6.91311168670654 3.63813948631287
22.1481513977051 0.528828561306
7.26248502731323 5.52340126037598
-16.2998008728027 17.9167327880859
-1.01313447952271 3.13748383522034
6.22816801071167 6.90335369110107
-3.91450142860413 1.32446146011353
-2.60662627220154 1.72834372520447
35.2465972900391 4.70431137084961
7.26959705352783 3.63521480560303
7.16004705429077 2.92209029197693
-5.63992118835449 13.3938369750977
21.0351276397705 0.0123304203152657
-0.40113365650177 2.7846417427063
-5.04834079742432 11.742693901062
-5.00437927246094 10.9580364227295
-4.5082745552063 10.8634605407715
-8.68838214874268 25.8814125061035
-12.1657075881958 34.8351631164551
22.2589015960693 -1.09454226493835
6.55776691436768 5.22793006896973
19.6349334716797 0.0508566834032536
-0.512727797031403 1.27003967761993
7.72508668899536 2.91374087333679
6.70548534393311 2.57486653327942
-3.08750438690186 1.0158566236496
-7.53418827056885 11.9797801971436
-7.05287647247314 18.4478511810303
7.50059223175049 3.12501740455627
18.8846855163574 0.846306324005127
-6.71130180358887 15.5856323242188
-2.93113446235657 12.1841897964478
-13.8352527618408 18.9507217407227
-4.56567764282227 1.56905496120453
-3.3034451007843 0.837157428264618
-6.05321216583252 11.5554962158203
-2.33327698707581 1.05426800251007
5.21177339553833 3.8069121837616
-17.2714710235596 21.5113201141357
-5.04666042327881 2.40204000473022
-4.97039318084717 10.9824142456055
8.03486156463623 2.57587265968323
-3.71258139610291 10.9477319717407
-4.28336095809937 11.1813468933105
-2.97319149971008 0.270558446645737
20.33957862854 -0.544817686080933
-2.07636713981628 0.127094238996506
7.28825283050537 3.62205362319946
-3.36175584793091 11.1041412353516
-2.62951946258545 1.99152839183807
-16.3198661804199 20.2146797180176
6.91743612289429 2.55929136276245
-6.69620752334595 16.8609790802002
-6.12914752960205 0.30968314409256
0.300616919994354 -12.838550567627
-4.97149658203125 11.4914445877075
-3.62734413146973 11.2105751037598
-7.31091690063477 10.6942911148071
-1.84677922725677 -0.0814801901578903
-4.72939586639404 10.3296213150024
0.358684301376343 1.61631953716278
-0.494952291250229 2.82188153266907
-2.17635297775269 2.91340303421021
16.6833438873291 -6.21961116790771
6.32974433898926 4.59805679321289
-3.26078271865845 10.3329086303711
6.16606521606445 4.65760612487793
-3.67373538017273 1.89699947834015
-3.90794324874878 11.530143737793
-7.82348012924194 19.818058013916
-6.74935150146484 18.1481094360352
16.9653339385986 -12.6658506393433
7.60175609588623 4.0401668548584
7.91997146606445 3.77116799354553
-8.37951278686523 19.2837524414062
-8.51991558074951 27.8934707641602
36.5319137573242 5.2849292755127
6.59270000457764 3.04759645462036
-14.1486616134644 16.7728939056396
-14.1523561477661 16.7850589752197
6.36087131500244 4.26184701919556
8.52068424224854 5.23540687561035
-5.3889479637146 12.2719984054565
-1.82314789295197 1.41880893707275
-1.67473864555359 3.09479713439941
-1.50994205474854 1.43520593643188
7.86929273605347 3.76299238204956
-3.13734221458435 12.6922750473022
-8.04219627380371 26.1389064788818
6.68019485473633 4.22898387908936
-6.34452056884766 10.3617382049561
-2.87214374542236 0.897016525268555
20.3723239898682 -0.280936896800995
-7.353835105896 17.5013236999512
-14.9979219436646 21.1784744262695
-14.5158557891846 34.8503799438477
-1.14431893825531 0.826353549957275
6.022705078125 3.62440299987793
7.7962327003479 2.01926064491272
17.5329875946045 -4.90675497055054
21.3413734436035 -1.4679913520813
-14.9035453796387 19.6801586151123
21.3266010284424 0.431958317756653
16.2586898803711 -4.38715553283691
-3.62105870246887 12.6367053985596
-4.19258880615234 10.8541870117188
6.92915725708008 6.0048713684082
-2.98882842063904 0.195399299263954
-6.45807552337646 17.8232650756836
4.97929811477661 4.39336824417114
7.96043300628662 4.16400527954102
-3.45865678787231 2.68186712265015
-3.56464815139771 1.54953920841217
6.85503911972046 3.97055172920227
18.0106449127197 -4.94787836074829
-2.21101355552673 -0.682928860187531
20.5525665283203 1.30560052394867
20.6803112030029 -1.6893572807312
8.12771511077881 3.59433794021606
6.23888492584229 2.25991296768188
0.442772448062897 -11.2682104110718
20.2880992889404 1.32163894176483
-2.14574265480042 1.80384051799774
-17.5959606170654 21.8497543334961
19.9373435974121 -0.779664635658264
7.34570407867432 2.7399787902832
-10.7884569168091 28.0011692047119
7.40480852127075 4.41489267349243
-5.95811414718628 18.7423210144043
7.05803442001343 2.51341271400452
7.35375595092773 2.75697493553162
-14.8016691207886 34.906566619873
8.96686267852783 3.66155052185059
-4.86827039718628 12.4263496398926
6.55636644363403 3.65598273277283
-2.84237098693848 0.927559733390808
8.04659938812256 3.4738392829895
-8.14025020599365 17.9926490783691
19.3570995330811 -10.1557779312134
-8.1519021987915 18.4872894287109
21.6193923950195 -0.308586269617081
-14.7111415863037 19.6490211486816
-5.91388940811157 10.2837715148926
-14.1817016601562 18.4341907501221
-4.76939010620117 11.6884317398071
21.0812835693359 -0.803124248981476
-8.03639030456543 19.9545078277588
19.7213745117188 -2.15100121498108
6.80295133590698 4.8016996383667
-4.2531566619873 12.7832803726196
7.25768566131592 2.78590488433838
6.00622367858887 3.40457129478455
-4.89918661117554 12.5346097946167
-3.59584426879883 1.63381385803223
-4.67150402069092 11.0718126296997
-3.74493861198425 2.02250695228577
-4.19662141799927 10.1439304351807
5.56082773208618 2.69721794128418
-2.41950798034668 0.641469478607178
-2.31332778930664 11.2795257568359
-17.7456951141357 22.7197189331055
-3.6466269493103 -0.294323980808258
15.5876483917236 -5.10460042953491
-3.63770365715027 1.80120003223419
-5.31719207763672 11.5755615234375
6.92513275146484 5.26651668548584
-4.48603248596191 0.734860956668854
-2.96115303039551 0.543201923370361
-6.97520685195923 18.3481864929199
-4.1881947517395 11.0634384155273
-5.76059103012085 10.8347215652466
-4.22976541519165 12.2692937850952
37.5181884765625 5.30706071853638
36.2763442993164 5.61342191696167
-3.68596529960632 -0.158740073442459
-0.370848178863525 0.138654291629791
22.0981578826904 -1.14455235004425
-6.15859651565552 18.4201850891113
-6.23421239852905 12.9035797119141
21.7422466278076 -2.29469704627991
36.8284873962402 5.37007331848145
21.6996040344238 -1.78215670585632
5.45523643493652 5.17806243896484
5.99773168563843 2.93784213066101
6.24822950363159 2.87784314155579
-4.08089065551758 1.82971704006195
6.60538578033447 5.27225875854492
18.3283042907715 -4.98852300643921
20.4066104888916 -0.50105494260788
-3.70884895324707 0.647497236728668
-9.06930541992188 27.4762020111084
-8.80309963226318 27.0578365325928
7.48641729354858 2.76504302024841
5.35209894180298 6.94973945617676
-5.06043338775635 10.8779640197754
-14.3416652679443 17.2958068847656
5.29699182510376 4.53167581558228
18.7449722290039 -6.58034181594849
-17.7534103393555 23.1331825256348
7.4501485824585 2.836758852005
17.6876983642578 -4.78427696228027
18.0316772460938 -5.21342468261719
-1.3305549621582 3.48048734664917
-3.10104250907898 4.25333499908447
-6.01469564437866 11.1481695175171
0.412606000900269 -13.1211395263672
-3.87640500068665 12.7709264755249
21.9937686920166 -0.787182927131653
-2.34640216827393 2.18904781341553
-3.01926493644714 13.9213809967041
-3.80285143852234 10.5346145629883
-15.199857711792 18.8119239807129
-4.02597856521606 0.974023818969727
21.0843467712402 -2.09038949012756
-2.51882696151733 0.781402051448822
20.9815063476562 -1.17629396915436
35.8526420593262 7.16719913482666
-7.55177354812622 17.3448905944824
-0.403578996658325 1.22897064685822
-15.3684120178223 18.4235820770264
36.6884918212891 4.69279050827026
-8.54885959625244 19.1798553466797
1.55776929855347 -13.0735998153687
-8.6368522644043 27.3891582489014
6.99296808242798 5.48754835128784
6.67703676223755 3.05341982841492
-13.9296770095825 18.1731014251709
-14.5704755783081 35.8241767883301
-2.11857867240906 0.0985562354326248
21.9073143005371 -1.37909638881683
-6.73360729217529 12.2401056289673
-7.29425764083862 18.2106151580811
-4.20443248748779 12.4095077514648
0.0715166553854942 -10.6762561798096
20.7607154846191 -0.79150801897049
-8.59327507019043 26.9815921783447
-8.73749160766602 18.1773109436035
21.8328895568848 -0.516447246074677
-7.61014366149902 11.7479600906372
-3.15533876419067 1.29582595825195
6.57505655288696 5.57974481582642
-3.00127005577087 11.5026569366455
8.39294528961182 3.58514666557312
8.61754703521729 3.75164675712585
7.62159824371338 4.23465442657471
19.8032550811768 -0.703038513660431
-5.52802991867065 18.6242961883545
22.1812000274658 0.0229166969656944
6.81870985031128 3.50478434562683
21.1533641815186 -1.2538458108902
-6.03729629516602 12.5466499328613
22.0966682434082 -6.22828102111816
5.82293939590454 3.52269434928894
-6.84929704666138 18.9470024108887
-2.64628458023071 1.46233308315277
-1.73815870285034 1.0480192899704
-4.5668740272522 8.98551845550537
-7.35578632354736 18.4308052062988
22.2330169677734 0.921712756156921
-15.7903890609741 18.6144599914551
-2.47212839126587 -1.23379623889923
21.955696105957 0.199991017580032
-1.28030681610107 -1.4228481054306
-8.24503326416016 17.9552536010742
-15.1084480285645 34.5422058105469
-17.4161720275879 19.3133068084717
-18.512975692749 21.0059947967529
35.1782264709473 5.96405696868896
5.96968650817871 3.48014807701111
6.95386028289795 5.29394292831421
8.0457820892334 1.9788373708725
21.1341228485107 0.773461580276489
6.9278244972229 4.447838306427
-7.38904762268066 17.7036819458008
-4.39944553375244 11.3702535629272
35.6996574401855 7.07253122329712
-0.854375958442688 1.87290513515472
22.5513954162598 0.586992740631104
20.6393203735352 -8.41427516937256
23.3586616516113 -0.0940644294023514
7.11887359619141 4.0995979309082
-2.4397246837616 0.727319598197937
22.0765933990479 0.597132086753845
-8.32931613922119 17.9223728179932
5.91246128082275 4.02846240997314
-0.867500305175781 1.00270617008209
-1.83563792705536 0.492348283529282
8.16398143768311 5.24180746078491
7.18832969665527 2.73406767845154
-2.4534215927124 -0.697266459465027
-4.60102367401123 -0.473175883293152
-3.7909529209137 1.18425238132477
-0.275488883256912 0.92038232088089
-8.58012008666992 18.7311725616455
-3.82797980308533 0.119390070438385
6.69963073730469 3.50185370445251
7.62438821792603 6.19576358795166
-7.50419425964355 16.9110507965088
-6.39687299728394 10.8719339370728
-2.02265954017639 0.222661539912224
-5.32568216323853 11.2420921325684
5.91243743896484 3.9104208946228
-17.8948612213135 16.5345916748047
36.6421852111816 5.90395212173462
-3.55830478668213 1.59861767292023
-7.07839345932007 17.8164310455322
-5.05266380310059 0.945998132228851
-3.36725306510925 0.403870224952698
-2.20033049583435 1.26848924160004
-17.4708385467529 21.8602504730225
-3.03368163108826 2.01781702041626
19.9218330383301 -7.46544075012207
-6.29957962036133 16.4823589324951
5.29852485656738 2.0942645072937
-7.62729072570801 15.8900775909424
-7.29184579849243 16.9236831665039
20.0527286529541 -0.415576696395874
-8.40869903564453 17.2929553985596
-3.43393087387085 1.0901597738266
-18.0198211669922 22.3763484954834
-4.26292371749878 11.4845733642578
33.4814682006836 8.04935550689697
21.0791778564453 -12.6574792861938
36.2015724182129 6.46902561187744
7.24977684020996 3.72876071929932
8.73211574554443 3.38316082954407
5.66554641723633 3.75304794311523
-8.20249271392822 10.8583459854126
22.284574508667 -3.16366791725159
19.8290634155273 0.218775078654289
-1.74595427513123 0.275413572788239
6.26157903671265 3.17567539215088
-3.20676755905151 1.56419944763184
19.7889366149902 1.26645815372467
20.4530506134033 -1.47178173065186
-4.76558446884155 11.4286937713623
-2.16312575340271 0.721470832824707
-4.09360504150391 9.73142528533936
-9.09158706665039 18.1524906158447
-4.01417112350464 1.20884931087494
36.3963241577148 5.44832801818848
-4.21655082702637 -0.525453269481659
-4.93945980072021 11.736777305603
21.6342029571533 0.862001776695251
-4.448073387146 0.663707613945007
-5.05007171630859 14.1456775665283
21.4024085998535 -1.35058689117432
-4.03889846801758 11.2650213241577
-4.29176378250122 10.2630043029785
-17.2142868041992 24.6075630187988
7.43495225906372 2.05180239677429
-5.96824026107788 20.7201766967773
6.03309965133667 4.71340179443359
17.2279205322266 -6.63791275024414
7.53890752792358 4.37161493301392
8.20713424682617 3.85418295860291
7.66302585601807 5.12527179718018
-3.44414901733398 4.04995584487915
-12.9999866485596 34.6257171630859
-7.64404106140137 10.5976333618164
7.43774890899658 5.87173748016357
6.53209114074707 3.1359543800354
-8.59102725982666 19.0452175140381
23.2244396209717 -0.507645189762115
-6.27614545822144 12.6287231445312
-5.11339473724365 12.0009689331055
-2.50035047531128 2.46116423606873
-6.70525503158569 17.0336112976074
36.0117683410645 6.27158737182617
-5.49114942550659 11.3750438690186
-4.66486406326294 10.3184785842896
-6.19964456558228 18.2673244476318
7.43866968154907 4.44421720504761
-4.66503667831421 1.25542175769806
19.1542263031006 -6.10455846786499
6.7168402671814 2.84123182296753
7.64046764373779 3.15217304229736
-2.71273589134216 1.27862215042114
5.7858247756958 5.31952476501465
-1.92516219615936 0.538343191146851
-14.0825862884521 35.8116493225098
-1.84706592559814 -1.37271213531494
21.4073867797852 -7.76371622085571
8.15602779388428 5.91122817993164
-5.09656381607056 12.3247404098511
-4.80443716049194 12.8868913650513
-3.6215763092041 10.2870140075684
-15.9274415969849 18.7346153259277
8.63183689117432 3.4000391960144
};


==> figures/visualizations/gmm40/craft_samples.tex <==
\addplot [semithick, craft, opacity=0.7, mark=*, mark size=3, mark options={solid}, only marks]
table {%
22.9000282287598 -25.4080905914307
17.0780544281006 22.098518371582
-0.794897317886353 36.399112701416
-17.0116863250732 23.8022117614746
15.6439409255981 -11.1614933013916
12.1541709899902 -25.9706916809082
-5.05709791183472 12.4917612075806
15.5808305740356 -11.5195684432983
15.5083532333374 -11.5466566085815
24.1558895111084 -36.4825286865234
-3.67558693885803 2.39410424232483
13.4299230575562 -25.2854633331299
11.0742206573486 26.2161502838135
25.7480602264404 -39.1082534790039
-6.77748727798462 17.9303741455078
0.943400859832764 -21.6371669769287
-1.39884078502655 36.9548988342285
-35.3249664306641 18.8319759368896
11.4908113479614 28.4028072357178
23.0010757446289 -26.2944488525391
0.645761847496033 -13.6835041046143
12.2424507141113 -26.2241020202637
-14.8306789398193 19.2000293731689
18.7306499481201 -8.91916275024414
22.3004264831543 -14.9828262329102
21.4493770599365 -27.3090972900391
1.42492496967316 -22.3519840240479
-39.3208351135254 -32.7553558349609
-37.9875717163086 -30.2724552154541
4.85159969329834 39.5619850158691
3.86468625068665 38.5363464355469
-39.4701309204102 -32.9127998352051
-7.48526382446289 26.565544128418
-6.79734659194946 17.993278503418
23.1913070678711 -15.3841485977173
35.1384048461914 4.4311728477478
35.2772979736328 3.9681191444397
22.0430965423584 -27.1503086090088
26.363597869873 -29.9072036743164
21.512996673584 -0.69966059923172
20.2117538452148 -0.145447343587875
34.5998916625977 5.88860368728638
19.7090263366699 22.9819831848145
10.7053508758545 -27.4778575897217
22.7021522521973 -26.1796646118164
28.6470909118652 -11.7205648422241
-34.3002319335938 21.5037689208984
-6.28228425979614 29.6260852813721
-8.15475559234619 29.3179054260254
0.573332726955414 -20.8287258148193
35.3005104064941 -12.4492692947388
25.5066947937012 -38.9181823730469
19.1704063415527 -8.35454273223877
-2.71024966239929 38.6127166748047
-0.210740879178047 -22.8964595794678
13.1293144226074 28.6976356506348
-2.81265258789062 2.16586422920227
-0.0415548384189606 -20.2538280487061
22.9380168914795 -27.5804195404053
20.1572780609131 23.7995719909668
-32.9206581115723 20.0742473602295
-8.42340660095215 18.5434551239014
34.3197212219238 7.39473676681519
-3.53930807113647 29.9363880157471
13.1240606307983 28.7033309936523
22.1638469696045 -14.4864912033081
-1.33390295505524 36.8127517700195
-1.93058168888092 35.3276557922363
17.9712505340576 -8.78833770751953
-15.708062171936 18.686487197876
-10.1051626205444 27.0304489135742
14.4830770492554 -12.270546913147
-1.81387090682983 -26.9985790252686
27.167667388916 -25.3186836242676
21.5306339263916 -1.57511878013611
-39.282642364502 -32.7779197692871
-37.7656593322754 -30.2661113739014
-21.9740886688232 21.5956726074219
2.9391143321991 -12.8949041366577
-1.39358985424042 36.8461685180664
1.76756775379181 -27.2223014831543
19.6042747497559 -1.70591843128204
22.0405139923096 -24.5240478515625
-13.8936185836792 18.5278701782227
-7.33271789550781 19.5446662902832
15.6367053985596 -11.6265983581543
-16.4004974365234 19.9327754974365
11.7256498336792 -26.7081241607666
-17.6161136627197 17.9231300354004
-19.1601409912109 22.3928108215332
-13.2824954986572 17.8431720733643
22.937557220459 -12.6678771972656
17.9924373626709 23.2724418640137
-17.6606349945068 17.963903427124
8.25626659393311 3.8628990650177
-20.217134475708 19.8509216308594
20.4239902496338 21.1981315612793
25.5043468475342 17.881498336792
9.26119709014893 29.3366146087646
26.3428745269775 -35.9345436096191
25.8671550750732 -39.4254875183105
34.0871734619141 7.18029117584229
16.9996795654297 -9.03371334075928
25.4608917236328 17.9138355255127
15.6626901626587 -11.5407867431641
26.8547496795654 -25.7689609527588
33.2074127197266 38.0802116394043
-37.7991600036621 -30.2218761444092
26.8898468017578 -25.7583103179932
-38.0488471984863 -30.2874011993408
0.376461088657379 -21.5510673522949
21.4752464294434 -26.3439102172852
28.6424541473389 -11.756628036499
19.6726703643799 23.1485633850098
1.36992359161377 -20.7267417907715
-1.60945653915405 35.559455871582
0.046874213963747 37.3306884765625
11.4888973236084 28.3689880371094
27.2656860351562 -25.2865657806396
11.9124002456665 37.5314445495605
15.5022773742676 -11.6131734848022
1.30260121822357 -21.8013706207275
6.39889526367188 40.193489074707
1.57742953300476 -23.060546875
33.5736656188965 -9.84624195098877
-39.4592933654785 -32.8297424316406
25.004186630249 18.8664836883545
-36.9767112731934 20.8443374633789
10.6051578521729 27.9376564025879
-21.0175743103027 19.6509037017822
12.8836040496826 -25.8247356414795
31.6148891448975 36.8549499511719
-4.12508726119995 13.6465797424316
-33.4637145996094 23.068244934082
-20.1936168670654 19.6171779632568
3.37148451805115 -12.1574850082397
18.1681690216064 -7.38917922973633
-6.51190137863159 14.171012878418
-3.55900192260742 29.9093208312988
7.9757924079895 2.67289924621582
-5.72144508361816 12.3208322525024
19.464916229248 21.3008899688721
-39.1721496582031 -33.0822792053223
18.5850734710693 0.749727606773376
6.25116586685181 4.1845326423645
-2.23559951782227 1.90581774711609
23.1559276580811 -25.9559555053711
-35.5174865722656 20.7043228149414
-4.06839895248413 11.1022796630859
-17.245626449585 22.8191719055176
34.7719764709473 5.40364694595337
24.4582118988037 18.5265483856201
22.6072807312012 -25.4556560516357
17.0766086578369 -4.16245603561401
19.9858207702637 -6.55367755889893
23.6879234313965 18.5668525695801
6.08174848556519 3.81786847114563
22.5196094512939 -25.95631980896
-7.48797845840454 18.133939743042
20.1364784240723 20.7537879943848
33.744197845459 -13.1645288467407
26.5520801544189 -36.0639419555664
35.0777473449707 5.60681247711182
18.9898853302002 23.1202545166016
34.7275314331055 5.47953224182129
-9.30203056335449 28.3876647949219
-13.9072294235229 35.8884620666504
12.6051788330078 -25.8772506713867
-39.5197639465332 -32.928108215332
27.2995166778564 -10.9243144989014
0.879637718200684 -20.8924102783203
-39.2298202514648 -33.0522003173828
18.8459091186523 -9.2640438079834
-17.3731956481934 18.3577404022217
-15.8496713638306 17.0690898895264
-1.79150319099426 2.33542418479919
-14.3557901382446 36.4978370666504
-9.29305934906006 29.6633205413818
4.85631704330444 39.5386695861816
34.0100326538086 36.7500038146973
12.791841506958 -25.8897647857666
-8.97365474700928 18.4382362365723
19.235294342041 -8.93080615997314
20.5172843933105 0.110938809812069
32.8920631408691 36.3595504760742
-18.0246391296387 22.4807224273682
26.6248550415039 -27.7410621643066
17.3143692016602 -7.9737811088562
-20.5390949249268 19.5971870422363
35.3685607910156 3.91914510726929
-3.20591139793396 0.200176581740379
24.5581283569336 17.9192810058594
29.5720119476318 -12.2626752853394
33.2084617614746 36.7221755981445
14.493782043457 -11.7509164810181
18.6475257873535 -13.5023231506348
-36.1195640563965 20.5952949523926
0.897756814956665 -21.1083126068115
-8.7808198928833 18.227912902832
25.0335998535156 18.9065284729004
21.87961769104 0.678215146064758
25.1033363342285 20.3181495666504
20.6821899414062 23.8188018798828
1.29421925544739 -20.314525604248
-17.5482692718506 22.7928066253662
-20.4943943023682 19.9027328491211
20.1228733062744 23.8665866851807
33.2307510375977 36.6662139892578
-1.87350273132324 36.8033027648926
-16.3027191162109 18.4597606658936
18.0916881561279 -7.72054433822632
25.651912689209 -39.1037063598633
19.285026550293 21.3847522735596
-1.39881432056427 36.9105072021484
-32.3076171875 20.2370643615723
-1.26967561244965 1.91313755512238
-4.6919994354248 11.4295082092285
11.9022550582886 -27.2670097351074
-3.76542353630066 11.3238735198975
11.853645324707 -27.0881652832031
19.8482971191406 -13.5474376678467
-39.2120018005371 -33.1322402954102
2.65222191810608 -23.8026542663574
4.98286104202271 40.4069290161133
19.6729278564453 -13.2792358398438
5.75434875488281 5.67853164672852
23.5192756652832 -26.3396396636963
33.0832252502441 36.4690856933594
0.653093874454498 -13.5944423675537
29.5481815338135 -12.2419328689575
18.5136795043945 23.0757904052734
21.7351703643799 -0.837713301181793
20.0944557189941 -0.253280639648438
11.4299058914185 28.7421550750732
20.3344554901123 21.2239799499512
18.7917251586914 0.328552782535553
26.2464656829834 -39.6146965026855
26.1381034851074 -36.2586898803711
0.875781953334808 -28.6092662811279
26.3212375640869 -35.665771484375
19.121431350708 -14.0623216629028
13.4963111877441 -25.9445152282715
25.2708683013916 19.387056350708
28.4807929992676 -27.4474124908447
-39.1748046875 -33.0731010437012
11.2252721786499 29.53444480896
26.7923126220703 -28.2196578979492
-0.73118782043457 -22.1485443115234
13.4815607070923 -25.2161083221436
27.0717601776123 18.85227394104
-8.86861515045166 29.2741260528564
22.4141807556152 -25.3587779998779
12.2037582397461 -26.1616706848145
26.0398826599121 -39.614990234375
17.0695648193359 -12.7205991744995
-31.8020305633545 19.9404106140137
6.91894626617432 3.33863854408264
19.4885559082031 24.7036170959473
-2.68210744857788 39.6381988525391
36.5318984985352 4.62808036804199
-39.0970916748047 -33.0808219909668
-17.5357284545898 18.4109725952148
28.5248165130615 -27.1902828216553
33.048828125 36.365592956543
-0.133352607488632 -12.7783050537109
21.0401802062988 -1.02694010734558
17.1984767913818 -4.01761054992676
-38.0929794311523 -30.3586292266846
11.6522912979126 -27.2153263092041
27.180778503418 -25.3056316375732
-0.567319810390472 -22.5927467346191
35.8763465881348 3.70283961296082
-9.47335243225098 27.6866664886475
1.09789979457855 -21.9140663146973
-4.65340900421143 11.3915386199951
-18.2996883392334 22.6706829071045
22.0538654327393 1.49339973926544
-2.30841755867004 2.41895842552185
28.4155292510986 -37.6150207519531
-2.16083478927612 2.57551956176758
33.258171081543 38.0463562011719
-5.92054033279419 19.0432415008545
33.4189262390137 -11.7630939483643
-36.8708648681641 19.9397754669189
14.995231628418 -12.5378293991089
29.5351905822754 -12.3264646530151
23.2954483032227 -25.877311706543
1.25263583660126 -10.6391687393188
-16.2024936676025 18.8991756439209
36.0090484619141 -12.8192481994629
-14.1563348770142 16.319995880127
-36.8292579650879 19.9688510894775
28.407341003418 -12.3604602813721
12.4303522109985 -25.8168106079102
-34.2436485290527 21.3734073638916
24.529016494751 -24.4446296691895
1.02629601955414 -21.0801258087158
19.6696834564209 24.6309509277344
-14.6144113540649 36.473876953125
-36.9485549926758 -25.1242866516113
19.2112865447998 22.6553268432617
17.7354145050049 -7.61727285385132
-39.2492294311523 -32.6624336242676
-19.1643905639648 22.4038047790527
10.0028467178345 28.9567375183105
-38.0962677001953 -30.2753887176514
11.1347179412842 29.4497566223145
19.2573051452637 21.3781547546387
-14.2531070709229 19.2403392791748
-19.0093879699707 22.2993659973145
17.1796188354492 -4.12030792236328
34.9710159301758 4.12137460708618
-39.281379699707 -32.7673683166504
21.7255554199219 -24.966775894165
26.1701965332031 -36.2736396789551
23.2475032806396 -13.8737659454346
17.9225749969482 -8.13309669494629
28.2987861633301 -26.8663425445557
-8.0465841293335 17.8492374420166
12.8999528884888 -25.8956756591797
-4.22802495956421 1.75295007228851
-2.19951057434082 2.59796261787415
10.5839147567749 37.6420860290527
20.475679397583 -8.22873592376709
-39.2742576599121 -32.7110137939453
-1.54071450233459 37.1903877258301
19.9669456481934 -1.33729207515717
20.3907432556152 -1.3561532497406
26.4625205993652 -10.1550283432007
14.5862350463867 -11.6943407058716
-2.17661952972412 30.8984889984131
23.1427345275879 -26.2642726898193
26.2212982177734 -29.481315612793
12.9622802734375 -26.4096431732178
1.36556041240692 -21.785228729248
26.1669826507568 -24.9747695922852
22.2719955444336 -15.9714365005493
-1.98285067081451 39.4979019165039
12.527943611145 -25.8937091827393
5.71980714797974 5.26240062713623
19.1459903717041 23.1313667297363
-39.185115814209 -33.0175018310547
20.3887405395508 21.1373863220215
6.18933820724487 4.17984962463379
-21.4327068328857 21.5485019683838
35.3406982421875 -12.4799728393555
-35.4923858642578 21.2538528442383
-35.5293655395508 21.28076171875
33.244873046875 36.6373252868652
34.844654083252 7.09947443008423
1.29480540752411 -22.0339031219482
-20.2365341186523 19.7882442474365
11.1040105819702 -26.6563129425049
34.9818153381348 4.1140341758728
26.7494087219238 -28.1920433044434
18.0460681915283 23.2873630523682
22.0871715545654 -24.7815532684326
-5.12195777893066 12.5732440948486
-17.7097930908203 22.0450077056885
33.9696388244629 5.79035186767578
-1.49059069156647 37.115608215332
32.9947662353516 36.3537864685059
20.7090511322021 -8.34842586517334
23.2520751953125 -13.7491207122803
19.9769191741943 -1.74520933628082
-1.92389190196991 35.400951385498
-33.2201995849609 23.2340602874756
19.6541843414307 -6.99974393844604
31.1008377075195 35.6001205444336
35.1804161071777 3.59350991249084
10.8003606796265 -26.5986270904541
36.0034599304199 -12.7843647003174
-39.2831573486328 -32.6514549255371
-0.0913503021001816 -18.3757228851318
19.1825981140137 22.6550159454346
20.1161155700684 20.7201519012451
22.5570735931396 -25.9659900665283
-2.49844574928284 0.820794343948364
-3.77288746833801 30.4337635040283
19.7687435150146 24.4181442260742
-3.95608592033386 11.0877132415771
23.6014728546143 18.931037902832
-35.5462913513184 20.0593776702881
20.1247024536133 24.1283836364746
11.8201999664307 27.6574363708496
19.7938346862793 -7.00548315048218
-0.603460371494293 -22.5961532592773
33.0190925598145 36.360294342041
12.6681814193726 -24.9432487487793
20.4819717407227 -8.2312536239624
-0.599072396755219 -20.6507606506348
1.21022295951843 -20.9028949737549
-3.6953547000885 4.42000532150269
19.5961589813232 20.9498291015625
0.596203625202179 -21.0058708190918
-1.09687781333923 36.9979133605957
-2.72260594367981 39.6098518371582
0.532211720943451 -22.6051788330078
22.9545879364014 -25.7156066894531
12.6724424362183 -26.1262874603271
19.2043495178223 -7.12573385238647
34.6372909545898 -12.7313547134399
33.5188903808594 -13.5266895294189
28.9537162780762 -11.4191675186157
35.2645454406738 -14.319281578064
21.433557510376 0.388498544692993
27.9818572998047 -12.5052461624146
22.8628997802734 -27.3654651641846
-2.56779265403748 0.744681477546692
-39.1490936279297 -33.010986328125
20.7295360565186 -13.1700096130371
-20.042854309082 19.3561534881592
35.908332824707 3.63477063179016
21.5178089141846 -13.1391658782959
-3.6014986038208 10.8434076309204
-1.72420179843903 2.28707933425903
4.55786514282227 39.5351524353027
16.73996925354 -8.54905796051025
-9.21341228485107 28.3986473083496
28.4433250427246 -37.6462516784668
-32.7337226867676 23.5710277557373
22.6540336608887 -26.8200263977051
17.6403369903564 -9.62382888793945
-19.5258255004883 21.498556137085
33.9359245300293 37.8609619140625
-14.5313444137573 18.1083927154541
10.9417657852173 -26.7073249816895
22.4994659423828 -25.8835277557373
23.1033344268799 -25.5871028900146
-34.9588775634766 21.248119354248
26.5822448730469 -36.0599822998047
20.9145221710205 -9.0918493270874
19.6704502105713 -14.0175638198853
19.1208190917969 20.9907169342041
15.1718463897705 -11.2228555679321
21.4464797973633 -14.3693609237671
-4.4798378944397 11.6114101409912
4.55768537521362 3.67411994934082
-2.26031875610352 31.9414806365967
-38.094841003418 -30.2895812988281
-4.05060243606567 11.1172475814819
-2.75384283065796 -29.2686958312988
-3.72821378707886 30.4038486480713
22.7081909179688 -25.9950103759766
0.273713916540146 -13.3794860839844
33.7908363342285 -13.8218078613281
24.3998489379883 -25.5018043518066
-17.4098377227783 22.431884765625
11.1277103424072 -27.5603122711182
13.5514640808105 -25.7372035980225
22.5920066833496 -25.9510345458984
-37.9943389892578 -30.3193473815918
-7.79473447799683 18.5771732330322
-15.8326568603516 18.2781848907471
33.199577331543 36.9198226928711
33.0137710571289 36.3587074279785
17.5650386810303 -4.52476119995117
24.0602245330811 17.1405773162842
-2.55520462989807 0.711372315883636
-34.4920997619629 20.5729999542236
-8.50861263275146 18.5473594665527
-37.0506324768066 -21.376615524292
35.9902305603027 -12.8485450744629
5.01152801513672 39.8098793029785
27.2385807037354 -25.2356605529785
23.7845916748047 -37.8325309753418
35.3063697814941 -14.4033184051514
-39.4579658508301 -32.8866577148438
12.2425556182861 -26.2145366668701
26.9065837860107 -27.9465522766113
11.8519525527954 -26.8779602050781
-6.76792907714844 17.9797286987305
-0.552599966526031 31.9437980651855
-0.527242720127106 -20.9003620147705
23.3050117492676 -13.8115491867065
-3.69857239723206 0.0107257468625903
-1.3311243057251 37.1629257202148
-32.9196319580078 20.0575084686279
20.2351951599121 -10.7424201965332
-13.2892599105835 38.2197074890137
-17.8216400146484 21.9628047943115
36.0716857910156 -12.8558301925659
20.3514633178711 -1.36983108520508
-13.2144899368286 37.4930458068848
-39.2081832885742 -32.8032989501953
17.9081211090088 -5.58573627471924
1.28547787666321 -21.9468936920166
20.3316192626953 21.1177673339844
19.8379440307617 -7.25081157684326
7.2018404006958 5.10329437255859
0.487573146820068 -22.6475315093994
-14.2982149124146 38.0084762573242
-34.3560218811035 20.9697971343994
10.2691631317139 38.978832244873
11.7600688934326 27.7858390808105
-4.59219455718994 1.86548006534576
-33.9905586242676 20.3882713317871
33.5155448913574 38.6733932495117
24.1332855224609 -25.960262298584
35.1160697937012 4.3331446647644
-39.4804649353027 -32.8561058044434
34.7173080444336 -12.6224336624146
12.5857019424438 -25.7799186706543
34.7728309631348 -12.1965808868408
20.3822898864746 -8.15084743499756
25.8939399719238 18.5968437194824
-2.21925401687622 1.82219314575195
6.63661766052246 3.67549896240234
19.5155620574951 21.264217376709
8.77762508392334 -27.0288143157959
19.1734848022461 21.0048294067383
33.4092788696289 38.7514457702637
27.9401950836182 -12.5745162963867
11.9527416229248 37.5838088989258
-3.82566070556641 0.454248130321503
-37.3559303283691 18.9928493499756
-39.2698440551758 -32.7226676940918
4.6461935043335 39.7750587463379
-1.29030025005341 2.00468063354492
28.4664821624756 -37.6758918762207
-16.9466953277588 20.3200588226318
19.1691093444824 20.9423084259033
26.330904006958 -35.7330627441406
-1.70362722873688 38.286750793457
20.4321250915527 -8.20669078826904
-4.19444465637207 1.96481645107269
-2.84914135932922 -0.438065111637115
-36.304801940918 20.2695350646973
-19.8209075927734 20.5600852966309
-15.5541334152222 20.0268936157227
12.7092304229736 -27.5022163391113
-0.956972479820251 -20.3512840270996
20.1550483703613 -8.81416320800781
-37.4497413635254 18.9594993591309
19.140510559082 -14.3730525970459
-14.7697601318359 18.469690322876
28.4606590270996 -11.8136320114136
25.5081996917725 17.9252758026123
-34.0286827087402 20.4677505493164
1.54858958721161 -10.8257923126221
22.6558933258057 -27.1813716888428
-3.40937471389771 3.40149664878845
23.7081680297852 18.3545665740967
11.7836265563965 27.7331562042236
-12.2780790328979 34.8453483581543
-37.377254486084 18.9697265625
11.2232818603516 29.5473442077637
0.558891773223877 -14.1326789855957
25.0084362030029 18.0957355499268
19.7142353057861 24.6099853515625
24.070182800293 17.0818710327148
23.2439746856689 -13.7791566848755
22.6810607910156 -27.1484565734863
19.2234039306641 -8.29060077667236
35.2265129089355 -14.3334045410156
28.1723937988281 -11.9532508850098
-19.1063442230225 22.3703861236572
4.68009996414185 39.7933235168457
-0.784193396568298 -22.1258716583252
-1.86014747619629 38.7896423339844
10.4920272827148 29.1583499908447
-37.9696197509766 -30.3671092987061
29.7194938659668 -12.8364505767822
-33.3336181640625 19.6678123474121
-3.7242693901062 -0.0200094003230333
10.5933561325073 37.6127433776855
15.5788764953613 -11.6781635284424
1.03317534923553 -21.1118412017822
22.410493850708 -25.5806655883789
12.3406848907471 38.1488037109375
-39.5159111022949 -32.954216003418
21.4897174835205 -1.52201592922211
21.5900020599365 -28.156717300415
34.9854888916016 4.26817655563354
15.6577234268188 -11.6076173782349
-1.89724171161652 29.3812007904053
35.1818809509277 6.77206373214722
36.0189323425293 -12.8239364624023
22.8380165100098 -26.6569652557373
-2.52327847480774 1.89556491374969
-17.6251888275146 18.3737754821777
-20.2614707946777 19.6201362609863
-1.96989893913269 38.9029083251953
0.982233345508575 -20.6252059936523
21.2161407470703 -1.41609108448029
21.4959125518799 -1.59924852848053
-1.3849333524704 30.6845893859863
6.65768384933472 3.61507201194763
-32.3148460388184 20.2753143310547
18.6465167999268 -7.68219327926636
5.37633943557739 37.1263618469238
23.4855499267578 -26.1290912628174
22.1944789886475 -26.0755634307861
19.03369140625 22.4773769378662
22.5069599151611 -25.9844913482666
18.4524574279785 22.6943950653076
34.824520111084 7.11566543579102
-38.0590858459473 -30.250883102417
-33.7745628356934 20.3282299041748
17.7147808074951 24.4250736236572
21.7689037322998 -24.834545135498
-2.85959339141846 38.1093444824219
25.8472270965576 18.6738376617432
-0.452303230762482 -28.1458396911621
10.5309228897095 -27.757963180542
33.9680480957031 36.7263526916504
24.6132640838623 18.0440998077393
10.5777969360352 27.4918079376221
20.2079658508301 -8.82072257995605
-13.4368457794189 17.7983207702637
4.93984460830688 41.1335067749023
-8.66330528259277 19.2090835571289
-18.2756061553955 22.2600002288818
-6.23925447463989 19.9210586547852
11.1951189041138 29.5034770965576
12.1764516830444 -26.1758632659912
-3.22961235046387 1.96237504482269
31.3818988800049 37.5303077697754
21.9864730834961 -24.5815563201904
19.8625316619873 -15.9669399261475
22.5904178619385 -25.9076175689697
33.1801376342773 36.9234504699707
25.0715465545654 -25.4523277282715
-3.41726112365723 9.76912307739258
19.4069042205811 24.6614170074463
0.762686848640442 -27.9824867248535
21.7734413146973 20.2344837188721
35.3159294128418 4.07237386703491
-39.1814460754395 -33.0117530822754
20.878080368042 -1.25029838085175
33.1574935913086 38.9539833068848
-21.5579395294189 21.5577392578125
-39.561637878418 -32.8884811401367
20.6624565124512 23.7556419372559
24.34836769104 -25.5031681060791
22.7001953125 -27.160888671875
28.6602649688721 -11.6777801513672
25.8558235168457 18.610502243042
29.5232410430908 -12.2967767715454
20.2006397247314 20.8177967071533
22.4815654754639 -27.0453281402588
-0.897700488567352 36.499397277832
21.9307956695557 -25.3641033172607
12.1263990402222 -26.3221740722656
21.9296035766602 19.6602993011475
-37.8044471740723 -30.2372417449951
-3.76131725311279 11.3597574234009
-6.56576204299927 17.1282939910889
0.849546432495117 -28.5609188079834
-34.6146011352539 20.7006969451904
20.0563945770264 20.8652648925781
18.1529922485352 25.0677108764648
10.6246995925903 -27.4506149291992
-37.5687713623047 -24.6654891967773
-16.4079055786133 22.5279521942139
22.4498558044434 -25.8974781036377
0.8659707903862 -28.532751083374
1.87913179397583 -12.3607339859009
20.118932723999 24.0428886413574
25.499137878418 17.9366760253906
0.123601302504539 -12.7179584503174
22.6476535797119 -25.4675235748291
21.9217262268066 -14.8275651931763
-39.5796699523926 -32.8641166687012
11.2810745239258 -28.2816028594971
32.9352035522461 36.3411636352539
33.2249870300293 36.6791915893555
1.03253316879272 -21.669734954834
-16.071268081665 36.0807228088379
25.0489654541016 18.1355209350586
-38.0404014587402 -30.2659435272217
26.6441516876221 -13.1820421218872
34.9378204345703 4.15276956558228
34.8476943969727 -13.0905313491821
-1.90542721748352 -0.0594644360244274
28.6275939941406 -27.2470035552979
0.42240846157074 -13.2496776580811
23.8000659942627 -37.2489166259766
-14.29749584198 18.3552227020264
0.86487865447998 -20.7337074279785
-5.91061353683472 18.4748821258545
20.0232582092285 -1.07180166244507
22.6259841918945 -25.9353408813477
36.461498260498 4.58931064605713
-0.834944188594818 -22.11474609375
26.756950378418 -27.7067775726318
18.1322765350342 23.016263961792
19.4472942352295 -8.59627723693848
-14.940523147583 18.7991771697998
-39.4725341796875 -32.8453216552734
-39.2705879211426 -32.761100769043
33.0747604370117 5.33149528503418
5.40016508102417 39.3184242248535
33.2014923095703 36.9273452758789
12.5646896362305 -25.8925476074219
-14.329083442688 19.2506885528564
5.75270223617554 5.66631126403809
-13.8657054901123 18.5074329376221
34.9373321533203 -13.9132900238037
1.12894380092621 -29.0793647766113
29.526388168335 -12.3362865447998
20.3128852844238 -11.1517963409424
-32.9585304260254 20.133415222168
21.974681854248 -25.4139537811279
19.7825527191162 -7.00940799713135
19.7057037353516 24.2224731445312
28.6990242004395 -11.7487878799438
20.0360927581787 -7.15474891662598
22.3616371154785 -15.0272216796875
-0.838009476661682 36.4568023681641
22.1006107330322 -25.2184963226318
-32.5016784667969 20.5088348388672
35.9423675537109 3.66749095916748
-12.0682888031006 34.75
-0.530802190303802 31.9313945770264
-1.5131539106369 36.5871467590332
-37.0319900512695 -23.483097076416
13.3886280059814 -25.382474899292
5.24798822402954 3.92652463912964
2.0116548538208 -13.1957769393921
23.6003532409668 -26.3139228820801
1.19845235347748 -20.8206672668457
28.5317764282227 -27.2207927703857
6.84459495544434 39.1492958068848
12.6936740875244 -25.0511074066162
22.2545433044434 -27.1498718261719
11.7990064620972 -27.087007522583
-0.259989857673645 -22.409460067749
27.0873126983643 -28.1139430999756
-0.58332484960556 39.8715019226074
34.3974876403809 -12.4937696456909
20.189022064209 20.8087787628174
-0.470905721187592 35.7257423400879
-39.2644844055176 -32.788890838623
25.7594890594482 -25.7108421325684
-36.982048034668 20.8701705932617
34.9007301330566 -12.3266305923462
0.916760921478271 -21.175817489624
19.2605953216553 22.6891975402832
24.9829921722412 18.1102542877197
-14.9188289642334 18.8076248168945
19.334451675415 -8.52245426177979
22.8988513946533 -25.475040435791
17.541711807251 -7.88959121704102
0.731195151805878 -28.1975708007812
21.3328819274902 -1.28008151054382
-1.85787618160248 -0.0840911716222763
34.6147956848145 -13.0887613296509
20.1538848876953 20.7922630310059
-17.7850284576416 22.0107917785645
23.718355178833 -13.4204893112183
27.2313690185547 -25.2720012664795
9.52011871337891 38.9467163085938
-16.4180850982666 18.7215213775635
17.0607776641846 25.6498260498047
20.6085739135742 -10.9016981124878
-1.39211273193359 30.7800388336182
25.7441215515137 -25.7270355224609
-3.81337141990662 0.41996818780899
18.3942108154297 -8.10324192047119
-7.31043004989624 17.4946117401123
34.7949180603027 5.41438722610474
20.0742740631104 -8.20770263671875
36.5148162841797 4.63223123550415
0.0567393079400063 37.3399696350098
18.1620922088623 23.0576114654541
21.4201011657715 -14.3619594573975
-3.25848603248596 0.308947801589966
-2.79149913787842 30.5321998596191
20.2069606781006 -0.223229169845581
21.3567352294922 -1.3048015832901
20.9634666442871 0.608544945716858
35.3023338317871 6.14395999908447
-3.61963868141174 2.12381911277771
-38.0286865234375 21.2419147491455
-20.0483798980713 19.3058948516846
-38.0608787536621 21.264331817627
-33.1623611450195 22.8070240020752
12.1804714202881 -27.2140445709229
11.2804756164551 29.4505348205566
-16.4688396453857 18.6887245178223
1.18719851970673 -13.0315456390381
19.6793689727783 -13.9879474639893
-1.76695370674133 36.7053565979004
11.5113229751587 39.5259475708008
22.7356338500977 -26.2125949859619
28.8471565246582 -11.4539070129395
19.686939239502 22.989538192749
11.4722347259521 28.4158535003662
28.2658157348633 -26.3078098297119
25.8540649414062 -39.784538269043
21.9431915283203 -14.7421436309814
0.0777828395366669 -12.7202806472778
25.0805816650391 -36.6785774230957
20.2156543731689 -8.81486701965332
-4.64643287658691 11.4548044204712
-20.4261341094971 18.3783645629883
25.5102939605713 17.8574733734131
20.4610900878906 -7.20717620849609
33.4800643920898 37.2090950012207
-1.95631515979767 -0.162344291806221
-7.81325197219849 27.1851406097412
-34.2773551940918 20.9890079498291
22.1528568267822 -25.5260639190674
-1.81430947780609 38.7971496582031
1.29605758190155 -20.3350028991699
34.7396125793457 -12.1941184997559
-7.16363096237183 17.9159507751465
18.4879703521729 21.3738403320312
9.76861476898193 29.4035835266113
0.1547961384058 -13.9298496246338
7.20511198043823 5.90711259841919
-2.59369230270386 0.673386514186859
-1.08446300029755 -11.2679214477539
17.9824962615967 -8.34831142425537
17.1168785095215 -12.7089443206787
13.043137550354 -26.472620010376
-2.62229561805725 2.28074741363525
-2.04551339149475 -0.827112436294556
17.8578128814697 -5.16225576400757
-39.2419967651367 -32.7768974304199
-0.485859811306 -20.8452758789062
-20.9751434326172 19.7053813934326
6.24390125274658 4.12714815139771
-3.67015767097473 0.0157123915851116
-19.9164562225342 21.3801784515381
18.1925029754639 -7.79699611663818
-39.2225494384766 -32.8145561218262
7.29509592056274 4.06971502304077
-6.46438646316528 17.9353580474854
32.8949699401855 36.4400253295898
12.9831457138062 37.1399459838867
23.551965713501 -26.2735538482666
35.1042709350586 5.68230485916138
-1.49628496170044 38.9493522644043
36.5010147094727 4.6080174446106
4.7043981552124 39.7460021972656
-39.4701499938965 -32.9432411193848
24.9538097381592 -36.6749801635742
24.457878112793 17.99169921875
15.5903720855713 -11.6174449920654
10.5870819091797 28.0027675628662
-2.75521898269653 38.6032981872559
6.43428230285645 3.9989447593689
-1.44392681121826 36.6571731567383
27.3421993255615 -10.2880725860596
33.2676811218262 38.0606079101562
-38.0753860473633 -30.2325763702393
20.2853374481201 21.1567630767822
22.6718292236328 -25.959566116333
24.84543800354 -23.7334671020508
19.7419033050537 1.17576313018799
11.7916402816772 29.3996257781982
-4.14257621765137 11.5251159667969
1.22357141971588 -21.1464729309082
28.3345813751221 -26.9154186248779
33.0414581298828 36.3335113525391
19.9917736053467 -25.4884834289551
22.4992866516113 -25.7919406890869
23.7079219818115 -26.399543762207
17.5882797241211 -9.15571308135986
34.3199996948242 7.42460155487061
23.0220737457275 -25.7340850830078
-0.683095157146454 -20.5837116241455
-36.9207916259766 -23.9550743103027
15.6500358581543 -11.7139930725098
-0.617008447647095 -22.5788860321045
36.5506744384766 4.54314565658569
1.22305715084076 -13.0771818161011
10.2859897613525 -27.9155578613281
-3.7909049987793 0.38213512301445
-4.90354347229004 11.6928176879883
24.7781009674072 18.8462600708008
34.8423233032227 -13.0362033843994
-33.3543281555176 19.7124862670898
28.4591960906982 -27.406270980835
26.1586875915527 -36.2147598266602
-35.9342994689941 22.0151176452637
0.431347697973251 -13.3098363876343
-39.4656066894531 -32.8796272277832
-17.2062244415283 22.7937774658203
1.27832210063934 -21.9847583770752
-34.2204170227051 21.3114376068115
0.089707612991333 -12.691219329834
-17.2800903320312 18.2824802398682
5.69347476959229 5.21423053741455
12.0425815582275 -26.7347965240479
35.3734016418457 3.96066403388977
-6.45174884796143 17.0898666381836
-4.75257253646851 11.2550888061523
20.0228481292725 -6.61926460266113
-35.8434181213379 -19.8756427764893
20.1655311584473 23.8184604644775
15.561222076416 -11.6873455047607
-36.7406806945801 20.4247741699219
34.6328811645508 4.48025465011597
26.9243812561035 -25.7649116516113
1.20300817489624 -20.9851531982422
35.2932662963867 -14.2979755401611
-35.4967765808105 17.2599182128906
36.431324005127 4.63924694061279
-3.71299624443054 30.7157382965088
26.8223114013672 -28.3011951446533
33.6861381530762 38.5252723693848
24.4032592773438 -35.9253273010254
24.3304748535156 -35.921329498291
-16.2420330047607 18.5221576690674
28.532356262207 -27.3939933776855
26.0710620880127 -25.0041351318359
-31.7710876464844 19.9290523529053
-1.121218085289 1.91201591491699
-20.5020942687988 18.9217967987061
-1.92865967750549 -0.858875215053558
1.92953729629517 -12.2917919158936
-17.2979984283447 21.972240447998
24.8584766387939 -36.6029663085938
20.1673164367676 -8.80918312072754
35.3806037902832 6.11226177215576
22.534236907959 -25.9201774597168
33.9051513671875 37.733455657959
22.0546169281006 -27.1542873382568
20.1718063354492 -8.82983589172363
33.5274543762207 -11.8211040496826
21.1426448822021 -1.33547747135162
33.2881469726562 -12.8263216018677
19.4279174804688 24.701114654541
-3.20132493972778 1.99162089824677
28.0798511505127 -37.2660751342773
-2.64622139930725 2.27812099456787
12.190131187439 -26.2691764831543
0.506524443626404 -20.8675594329834
25.8913192749023 -39.1309127807617
34.0933876037598 7.19933557510376
19.6623878479004 22.7405643463135
-17.3165187835693 20.5063934326172
11.3909273147583 -28.318775177002
24.4133949279785 -24.8203296661377
20.8314723968506 -0.992372393608093
-15.1238346099854 19.0682563781738
-0.860293567180634 0.983945369720459
-32.9014358520508 20.0368709564209
21.3791599273682 23.649133682251
-18.7959690093994 22.1713733673096
28.6616287231445 -11.7735729217529
-20.6041374206543 19.5540084838867
-32.9174118041992 22.5872268676758
-37.783203125 -30.2185192108154
23.7488975524902 -13.4077205657959
-14.3549327850342 19.1901206970215
5.34740352630615 39.3070983886719
-17.3415775299072 18.23313331604
10.652063369751 27.8412055969238
-2.24727749824524 39.6943626403809
21.4507389068604 -14.4115133285522
9.76948547363281 28.4781932830811
20.9479808807373 -9.08423519134521
-17.1461887359619 23.8951950073242
-0.598993122577667 -27.9573421478271
23.1457843780518 -25.5662727355957
4.87433004379272 40.4380378723145
22.1348896026611 -25.689905166626
22.0337543487549 -25.1545867919922
36.5000381469727 4.65524435043335
25.5636692047119 17.8740348815918
-0.627463757991791 -20.7398548126221
22.8702392578125 -25.445837020874
-1.26488840579987 -12.7734069824219
0.464609533548355 -13.3052349090576
17.6209926605225 -7.63187170028687
10.6135215759277 27.4958076477051
-1.75022423267365 29.7261962890625
12.6567087173462 -24.9504051208496
12.6242036819458 -25.010721206665
-36.3238372802734 20.2233409881592
26.0891571044922 -36.3240623474121
31.813102722168 -12.1272821426392
19.6133460998535 22.9417819976807
21.110782623291 -0.97657573223114
7.15583324432373 5.92124795913696
22.6063785552979 -25.1950836181641
10.5387096405029 37.642448425293
25.0619621276855 18.0676040649414
0.119394026696682 37.4214286804199
12.0413293838501 -26.7066516876221
10.655345916748 27.7305297851562
12.1741600036621 -25.9664535522461
-0.630015313625336 -27.8926124572754
-35.2723197937012 19.0580577850342
25.6505641937256 -39.1000213623047
9.8604907989502 38.9326591491699
21.3724308013916 23.609489440918
28.0299034118652 -37.1883125305176
-2.7491307258606 2.26455974578857
-1.27770483493805 37.2365455627441
25.8864879608154 -39.5077972412109
0.763016402721405 -13.0053396224976
29.4897842407227 -12.3962326049805
1.6218147277832 -23.0527954101562
2.02039074897766 -13.4303112030029
1.74081492424011 -27.1321811676025
};


==> figures/visualizations/gmm40/dds_samples.tex <==
\addplot [semithick, dds, opacity=0.7, mark=*, mark size=3, mark options={solid}, only marks]
table {%
5.40463781356812 3.28744769096375
33.7051124572754 -12.7938938140869
5.74208831787109 39.2644577026367
-35.2908058166504 21.0322494506836
10.3298673629761 -27.447790145874
35.8423881530762 5.97722768783569
6.58458614349365 38.9312400817871
37.0914916992188 -12.0505952835083
14.3957872390747 26.9679641723633
35.6920471191406 -11.0142278671265
-16.2012767791748 36.3545455932617
-38.9971656799316 -22.8371715545654
27.6811962127686 -37.6415786743164
24.4981517791748 17.8045825958252
35.6593971252441 6.25125646591187
-34.6952896118164 37.1852493286133
11.3045768737793 29.0867538452148
-17.583532333374 20.8082828521729
37.156867980957 -13.0979022979736
17.3262233734131 -4.07808446884155
14.1457452774048 -12.1179504394531
6.77998304367065 39.6491279602051
-40.5501556396484 -33.1952438354492
-14.9573345184326 34.6175155639648
35.826301574707 5.6636266708374
11.9141225814819 36.985237121582
-37.777515411377 -31.0455799102783
18.6244621276855 23.3897457122803
29.8247928619385 -11.9958925247192
-32.5817031860352 36.961742401123
-3.52796912193298 31.0146408081055
-13.5186185836792 35.699592590332
25.0654621124268 -24.6154861450195
-18.8574180603027 20.2314701080322
25.8324279785156 18.4826145172119
-17.2872009277344 22.8148155212402
13.645676612854 36.5813865661621
-2.6248562335968 -25.9103393554688
-3.6151716709137 13.0836448669434
0.659764468669891 -11.6496629714966
35.1446151733398 4.30180263519287
21.2004070281982 -6.93222141265869
24.384822845459 20.0394878387451
-4.91989755630493 12.336597442627
27.4683322906494 -27.1971321105957
13.3945474624634 -27.2974681854248
34.0382881164551 36.1543235778809
-22.0025157928467 18.0426788330078
-39.279857635498 -25.560079574585
-31.7827453613281 38.7847213745117
36.5528335571289 6.21882772445679
19.938850402832 -8.58746528625488
2.42990493774414 -11.5798940658569
20.6451320648193 -1.5231237411499
-40.008415222168 -32.9495239257812
-15.9450492858887 18.2090511322021
24.13254737854 20.4025955200195
19.352165222168 20.9068279266357
-4.61935758590698 10.6544961929321
-4.06587171554565 11.6682987213135
36.237922668457 5.1015796661377
-32.4930229187012 40.8568305969238
-0.747559070587158 -21.5966053009033
-39.7168731689453 -23.1377925872803
-14.0365056991577 35.0244789123535
-16.8144130706787 17.0989532470703
25.4843101501465 18.8744945526123
24.3157691955566 -37.6633796691895
25.778003692627 -26.218074798584
29.4250183105469 -28.153003692627
-40.3771324157715 -31.6838645935059
-37.5499000549316 -31.0368537902832
33.1174354553223 38.5666885375977
-7.23303937911987 17.3373336791992
-3.35163831710815 -0.00882461667060852
32.2114906311035 37.4692535400391
16.5944995880127 -11.0863380432129
33.7702178955078 6.21573400497437
-8.66600608825684 26.7637462615967
35.9595985412598 4.90316390991211
-32.5046081542969 37.1204795837402
-37.2859916687012 -20.116247177124
25.9547595977783 -37.5098419189453
6.8304591178894 37.7914237976074
-36.5262565612793 -31.770378112793
26.5042343139648 -25.2375450134277
-35.2483863830566 20.8206939697266
5.35025072097778 38.3517456054688
-0.145345330238342 36.1690483093262
-3.23924612998962 11.0504121780396
-6.03686904907227 17.8465919494629
12.6174459457397 -23.2134437561035
12.0535879135132 35.510913848877
7.91932821273804 38.8827095031738
-14.7762537002563 35.206729888916
7.89401531219482 4.87881946563721
-0.191692963242531 -30.1359462738037
-6.12892293930054 10.4188709259033
-32.6012001037598 38.0272827148438
-6.88248634338379 19.9270343780518
13.4428749084473 26.2018623352051
14.5834856033325 -12.6783380508423
23.5887203216553 -25.4023876190186
-2.42128396034241 38.6115379333496
-3.97408437728882 30.3621597290039
-0.350492119789124 36.3799133300781
-39.2821464538574 18.8027801513672
-39.1755218505859 -22.900260925293
20.2101402282715 25.8969573974609
-3.03001284599304 31.1717987060547
-5.73477029800415 11.2682733535767
-37.8681488037109 -30.6907444000244
34.2288208007812 -11.1808414459229
-39.3782196044922 -20.3228893280029
-31.8911933898926 37.6802024841309
28.4842414855957 -28.0877418518066
32.6468887329102 36.4795608520508
-37.5600166320801 -22.54323387146
-8.91933155059814 27.4290580749512
-33.761100769043 41.5105781555176
0.501001238822937 -20.1546993255615
34.4647941589355 8.45343685150146
-22.6714611053467 19.5948848724365
24.7759532928467 17.3206729888916
31.4953746795654 -9.69908428192139
-4.76883268356323 29.7146129608154
-40.2690277099609 -21.3106212615967
-34.1518516540527 24.9686107635498
-8.09635353088379 28.2656593322754
35.9693260192871 -14.9570112228394
-4.05051040649414 11.9899063110352
36.0927505493164 -12.0209331512451
-15.2325973510742 36.9421501159668
0.925739288330078 -30.3194942474365
33.3270263671875 6.14545297622681
27.1681690216064 -36.7538681030273
-39.9763221740723 -22.1499900817871
27.6292629241943 -35.9449729919434
27.0601081848145 -38.2219123840332
21.094108581543 -0.145606592297554
20.2514724731445 -0.761435925960541
30.6167469024658 35.203125
19.9671688079834 1.24448752403259
32.1482276916504 37.0520668029785
32.7973403930664 36.6716423034668
-16.1945362091064 37.1923065185547
-34.7585258483887 20.0715732574463
-1.38046097755432 -30.7102928161621
28.796049118042 -11.4364585876465
5.64595985412598 5.15736675262451
13.3495254516602 -12.770357131958
-7.8377537727356 17.6289710998535
-34.2086563110352 21.5423774719238
25.9676361083984 -38.8394088745117
-15.3917379379272 37.5561256408691
28.2352085113525 -37.8748474121094
1.28510892391205 -23.2554359436035
-3.55582141876221 1.63825345039368
-4.8366436958313 10.132360458374
37.2086639404297 -13.5147819519043
34.5082015991211 36.3093757629395
20.1690540313721 24.0878849029541
7.43353223800659 3.80294823646545
-0.0840030461549759 37.5728530883789
-22.7975788116455 20.5451030731201
-0.40740704536438 1.61490154266357
35.7839660644531 4.39316844940186
35.4653205871582 -11.9854621887207
29.3746719360352 -13.2095499038696
28.7250213623047 -26.54176902771
-34.9045333862305 20.4699687957764
15.6943559646606 -13.9184379577637
20.9365730285645 -7.67918872833252
2.22230243682861 -13.1852235794067
26.8779048919678 18.1767711639404
35.5488357543945 -11.9122714996338
-34.931568145752 -32.1565208435059
-36.3137168884277 22.3560371398926
33.6112060546875 36.5217514038086
6.56459045410156 1.81317555904388
-11.5876874923706 24.1546859741211
34.1523361206055 -13.3417768478394
27.799409866333 -26.7901611328125
-7.08860921859741 19.1039619445801
-37.9292640686035 -20.8053321838379
-22.2947120666504 19.9061489105225
35.3750610351562 35.0612373352051
-29.7969493865967 39.236255645752
-3.94582295417786 29.6684322357178
0.31244957447052 -11.438648223877
0.851561546325684 -28.4951572418213
-16.3056449890137 17.101583480835
23.0421142578125 19.5958938598633
-38.840160369873 19.346471786499
2.04661750793457 -13.0959520339966
32.2802734375 35.5976638793945
11.5610523223877 28.604133605957
-8.05036163330078 18.3657913208008
26.5946750640869 -29.8858203887939
-33.3332901000977 38.1629791259766
32.7555198669434 35.9260787963867
-1.09702515602112 -12.2047548294067
-10.1235952377319 28.0237903594971
32.5752182006836 34.9045524597168
-7.6006236076355 20.2432346343994
-8.53090000152588 27.795877456665
28.7024955749512 -25.5144920349121
-31.6401119232178 38.9166069030762
-30.9342918395996 38.9629783630371
5.54975032806396 40.0263786315918
-14.8889856338501 35.8034133911133
34.9277305603027 5.66833209991455
36.5172729492188 -13.9785127639771
12.5492658615112 -27.5668697357178
-31.4975910186768 38.5205039978027
1.2996940612793 -12.3562116622925
-5.60434675216675 11.4248523712158
37.1665992736816 4.87029790878296
-4.59287452697754 12.0039529800415
5.25860786437988 4.2902307510376
12.4175815582275 38.1253776550293
-35.2555274963379 22.5850658416748
19.3419589996338 23.7514247894287
19.1338386535645 -8.03099250793457
4.96677589416504 3.51587295532227
32.5064964294434 33.9392395019531
-8.66209030151367 27.9838924407959
28.4856281280518 -12.264518737793
11.0681829452515 -27.0143661499023
22.6931648254395 1.27408444881439
13.679368019104 -24.9546222686768
-0.394902855157852 -19.6794261932373
3.35764145851135 -21.0276508331299
5.454345703125 6.60355758666992
-39.9083366394043 -33.8211898803711
6.14092540740967 39.572940826416
10.6683988571167 35.4779663085938
-32.1226539611816 36.8944282531738
35.7173233032227 4.35652732849121
26.3857746124268 -13.1220731735229
0.886425971984863 -11.8042335510254
26.5727920532227 -25.7108688354492
6.77259683609009 4.61796188354492
19.2979202270508 -5.34339427947998
35.9720802307129 -11.4218168258667
25.3506278991699 18.5961647033691
-0.0958049595355988 -28.7001266479492
20.579044342041 20.7333450317383
9.91594219207764 26.9664840698242
-34.9046783447266 20.9520320892334
-6.22389125823975 30.7441749572754
36.789665222168 4.54010152816772
-14.0677852630615 35.6989135742188
34.0615272521973 37.0205993652344
33.4797477722168 34.9012489318848
22.8405094146729 0.527230799198151
21.5060787200928 22.4594707489014
-1.95169126987457 28.6694927215576
35.3697090148926 -12.765588760376
35.284107208252 6.21547412872314
37.904857635498 5.19148302078247
-33.9603233337402 21.4732437133789
33.690788269043 5.67277383804321
-1.12456381320953 39.5285987854004
35.2369537353516 -13.2289142608643
32.133430480957 36.4832496643066
35.8762092590332 4.30528831481934
37.6271553039551 6.06845712661743
25.8049850463867 20.3605499267578
13.7037734985352 37.0733947753906
-0.0714086443185806 37.1758232116699
1.66118240356445 -12.9311294555664
7.31996393203735 4.28687334060669
-38.6764488220215 -22.2627449035645
-37.8940162658691 -23.3733787536621
-21.268669128418 19.4064064025879
31.5051498413086 36.7350044250488
19.8526496887207 25.2621059417725
23.5930728912354 -14.1076965332031
-0.509983599185944 -21.6020736694336
28.4110584259033 -11.3778839111328
22.2057647705078 -12.7877082824707
12.2299957275391 29.745677947998
7.65501403808594 3.29642486572266
7.64277601242065 2.46152853965759
-2.14773058891296 0.757577538490295
-34.8173751831055 21.6383609771729
-36.9828834533691 -32.7883071899414
-3.69530582427979 13.2884206771851
18.3133964538574 -5.9968376159668
27.8516578674316 -14.3981962203979
-39.3686752319336 -30.2013931274414
15.7876091003418 -12.347113609314
21.5867786407471 -24.1540374755859
24.7428913116455 -24.1481113433838
4.87902450561523 38.4621887207031
-5.53491687774658 10.643424987793
-42.2212295532227 -24.1208305358887
34.3869132995605 -13.5392713546753
4.22484254837036 37.959156036377
27.736421585083 -37.8631553649902
27.9695434570312 -12.466607093811
26.7727832794189 -38.7878074645996
24.9935398101807 -35.7806396484375
10.9244327545166 38.2056732177734
-16.5862731933594 21.3140392303467
2.07074761390686 -11.9877452850342
-39.0573463439941 19.0678768157959
-37.5225524902344 -33.0303382873535
-32.2766761779785 39.8967781066895
24.3233604431152 17.5015316009521
-31.9620418548584 39.0972137451172
-3.41171932220459 2.65842318534851
-8.05060577392578 26.8710327148438
-17.670295715332 22.7047309875488
-34.2681350708008 19.6367301940918
-7.19964647293091 19.8502998352051
-5.11774158477783 3.24627947807312
0.610692262649536 -27.6225395202637
-4.21878576278687 0.678787708282471
-38.7137565612793 -32.7150115966797
24.1931457519531 18.6415309906006
18.3569984436035 -4.39345979690552
1.3082834482193 -12.5490303039551
-33.8896789550781 39.9305000305176
32.1598510742188 35.6625633239746
37.5650596618652 6.32293224334717
24.9925861358643 17.2858066558838
-1.21818482875824 38.1096992492676
6.94725465774536 37.6176986694336
-13.5112199783325 35.7765655517578
25.9303417205811 19.5844688415527
17.2892074584961 22.7922210693359
-39.1987915039062 -32.6342544555664
29.489782333374 -27.5857200622559
-38.287971496582 -22.6168251037598
-16.541467666626 21.7529735565186
-13.9010972976685 32.6534233093262
-18.0113220214844 21.6455020904541
-14.2454881668091 37.2802963256836
-40.0554885864258 -20.5192756652832
-32.9185333251953 38.733585357666
18.1432800292969 21.7064647674561
0.409025996923447 -13.3782558441162
25.4604415893555 -38.4304237365723
21.211727142334 -24.4975490570068
12.5636262893677 37.3948822021484
-33.1234664916992 22.0928249359131
-15.8352088928223 17.0003890991211
-32.9266548156738 38.4846572875977
-4.93403339385986 19.767786026001
-3.06366395950317 1.93334031105042
11.2896270751953 29.359037399292
34.9269866943359 37.4935569763184
32.717601776123 36.090404510498
33.1193428039551 -11.3296556472778
0.75093686580658 -27.7527370452881
18.2351398468018 24.4333477020264
-38.3352279663086 -22.4880027770996
28.295581817627 -26.2561130523682
25.9157981872559 -11.4607305526733
10.7487621307373 39.6643486022949
-0.834179818630219 -28.9986209869385
-1.23898267745972 -28.6999168395996
-3.44380950927734 -2.0247962474823
32.8421440124512 35.1417121887207
-39.3253288269043 -32.5732345581055
-20.5337963104248 18.8267803192139
20.7327060699463 -1.77950489521027
24.8337688446045 19.1042098999023
0.125198751688004 -27.7877197265625
6.12408971786499 39.1287231445312
36.3197135925293 -13.2485208511353
1.10389292240143 -14.3621683120728
-33.1690902709961 22.3745460510254
5.4596471786499 3.50372362136841
-38.1115341186523 20.8739738464355
28.8059501647949 -12.3070974349976
-37.8488159179688 -21.458179473877
-38.0754203796387 18.8135185241699
33.507453918457 35.9290313720703
-40.5447006225586 -33.7610015869141
-13.3580274581909 35.5273284912109
6.5300464630127 4.73650789260864
-39.5743827819824 -21.9502983093262
28.9914379119873 -9.52370166778564
9.89842414855957 -26.957555770874
34.4598083496094 -12.4163236618042
-14.5503578186035 17.2723236083984
36.3370513916016 -11.726619720459
-37.9927940368652 20.4683036804199
-31.9928665161133 38.2476692199707
-15.1294775009155 19.0147876739502
-7.82490634918213 26.7364063262939
-39.5952110290527 -21.757152557373
13.5839042663574 -12.0623064041138
-1.76555120944977 0.304253369569778
26.4045524597168 18.9188499450684
-15.9854927062988 35.259204864502
0.959974348545074 -27.6161193847656
25.8974761962891 -39.7890625
37.276611328125 5.62398862838745
12.6882810592651 -26.5760269165039
6.47382879257202 5.73168659210205
18.8466548919678 -9.24256801605225
-2.53604412078857 40.090015411377
-33.4566116333008 37.4393577575684
-38.3396682739258 19.7131042480469
-16.1323471069336 16.4094944000244
-6.56106519699097 18.7450828552246
34.1476631164551 4.22947359085083
-4.1809344291687 11.2875022888184
27.4368648529053 -26.5535144805908
33.0044937133789 35.3611297607422
26.4305057525635 18.2880935668945
35.0544471740723 -11.1658153533936
35.8812637329102 4.71125793457031
18.6083374023438 -13.9436483383179
-22.1108684539795 20.3054866790771
-1.0706262588501 37.5570335388184
34.172046661377 36.3873138427734
35.1435050964355 34.5557479858398
6.76454639434814 6.02480459213257
35.398624420166 -13.5120124816895
-16.7337379455566 33.8005905151367
23.8918762207031 -34.8860855102539
21.084997177124 23.7458438873291
12.6333084106445 -24.0718269348145
23.8674926757812 18.3762531280518
-3.59542036056519 10.5817184448242
-2.80997228622437 38.9228439331055
12.4873065948486 28.4422016143799
35.4186630249023 -11.4486265182495
30.0614929199219 -11.6015968322754
34.1525230407715 5.09991073608398
-1.74046540260315 40.1658363342285
0.940733790397644 -12.5982961654663
24.2366142272949 -15.6636304855347
35.2180976867676 5.8803243637085
-35.0440063476562 21.8485450744629
12.6896114349365 37.8365783691406
20.5588150024414 22.1861820220947
-39.4831428527832 -18.2243461608887
-16.2020530700684 34.863697052002
-18.513090133667 17.3140125274658
-20.4200000762939 23.5712909698486
33.9505157470703 5.75874185562134
-23.1234664916992 22.2905921936035
25.1721305847168 -36.3700981140137
26.0174331665039 -37.3168067932129
-37.9761161804199 -31.8405075073242
-9.36756134033203 30.0136070251465
-15.2266263961792 20.0279083251953
29.5286712646484 -12.9185037612915
-31.3759536743164 38.1198463439941
-14.822226524353 35.0015525817871
26.988676071167 19.4403858184814
34.2336120605469 33.9093627929688
-4.63243961334229 12.3266134262085
-6.20968532562256 11.0061349868774
10.4366359710693 29.0172634124756
27.606616973877 -26.4061050415039
35.6841011047363 6.57258319854736
7.79431009292603 5.13070821762085
1.17804408073425 -30.3646678924561
32.3077278137207 36.1427268981934
0.561741650104523 39.3344039916992
-33.6901473999023 38.2193145751953
35.1053848266602 -13.1871013641357
1.28181552886963 -21.7275524139404
19.9942588806152 -8.67037677764893
-14.0967035293579 36.4761924743652
-40.4212760925293 -22.284366607666
9.14473724365234 27.4182281494141
26.5900478363037 -37.1848907470703
34.5709228515625 36.0815124511719
6.28260612487793 39.2520446777344
36.8344917297363 -11.8865661621094
36.5035934448242 -14.7181606292725
-1.957479596138 0.617157936096191
-3.80870485305786 29.1851425170898
19.2489070892334 22.8885803222656
19.5241737365723 -14.1296920776367
7.65594434738159 3.95459270477295
2.47295308113098 -19.4777450561523
-37.3503761291504 -32.2450523376465
0.50008761882782 -28.8309307098389
35.0332870483398 33.550594329834
-39.7645988464355 -30.9748382568359
6.91873788833618 2.58870434761047
-4.84878444671631 11.4243068695068
-16.8616943359375 37.0919990539551
-6.47376155853271 18.5674247741699
-1.9300479888916 13.0556764602661
-34.1675300598145 36.9165229797363
-38.0030975341797 18.4248237609863
-4.21519470214844 0.297365427017212
19.2852878570557 -7.29280185699463
-32.3857841491699 21.7884101867676
30.1835422515869 35.4909400939941
23.4132652282715 18.1956806182861
18.2019996643066 22.1432800292969
24.7677574157715 19.1120834350586
-2.2006573677063 1.97697377204895
34.3801345825195 37.7463111877441
-16.8450241088867 17.265645980835
-7.01984024047852 26.0077037811279
20.7891464233398 -0.797482848167419
-2.27887415885925 -28.1054878234863
2.03795504570007 -12.5546112060547
33.6073303222656 36.7368431091309
-33.6989936828613 40.6908645629883
-34.4540863037109 20.7480010986328
-4.11410331726074 11.1256799697876
-16.9910831451416 20.6913356781006
18.9847602844238 -12.6852369308472
-31.0709781646729 39.8476905822754
-35.0959625244141 20.8319873809814
26.7671184539795 -39.8383331298828
32.8636856079102 35.6529731750488
-14.0652275085449 34.9148101806641
25.8333721160889 18.2628402709961
20.6584663391113 0.727928936481476
-39.0713844299316 -22.7249546051025
4.93729209899902 37.9279479980469
34.0879783630371 37.2427406311035
-4.86172103881836 12.3574104309082
35.815803527832 5.69693946838379
19.6723289489746 -7.75064611434937
32.5914192199707 36.5618438720703
26.3040351867676 17.6022605895996
27.847412109375 -27.1966228485107
34.8115882873535 35.9094543457031
34.8778381347656 7.15029287338257
-2.41895747184753 38.0638275146484
13.6385765075684 27.9342803955078
21.3403987884521 0.934356272220612
23.2708148956299 -3.04954648017883
-4.88980007171631 9.68060874938965
11.0163307189941 27.2841815948486
-13.9210071563721 35.8304595947266
-14.5917320251465 16.3579788208008
-3.52989387512207 30.2997264862061
18.4625606536865 21.8897743225098
-14.2827234268188 35.7561187744141
25.2829971313477 -40.2593650817871
4.10142135620117 36.6629638671875
22.7457084655762 -22.5244655609131
-0.191555887460709 -13.3457269668579
-17.8012809753418 22.0483360290527
-0.906927347183228 -28.2402896881104
18.2938613891602 -15.4147968292236
24.3743877410889 18.5181617736816
4.07646036148071 2.77055335044861
-1.03247106075287 38.7814254760742
7.64770841598511 38.1246528625488
20.6169776916504 0.786369502544403
-0.623920559883118 -21.8012046813965
0.792053937911987 -28.4584312438965
23.0699443817139 -25.7212009429932
32.8729133605957 37.3880195617676
-1.98921751976013 2.56527853012085
-2.7030394077301 0.628223657608032
-2.21817207336426 1.43832397460938
0.530475676059723 -11.4534635543823
29.7128849029541 -11.8333683013916
-39.5379028320312 -21.5895156860352
-3.67283058166504 30.2006435394287
-3.72063851356506 28.3789825439453
0.755172431468964 -28.651819229126
12.0658655166626 34.777904510498
-32.4946403503418 22.0283603668213
23.3940658569336 -25.7442684173584
-36.380184173584 -32.1657447814941
35.2939605712891 -13.1257925033569
1.48192870616913 -13.597056388855
-40.1991806030273 -23.2756023406982
-37.1476707458496 19.2837791442871
-4.53445816040039 17.7663650512695
-37.6380157470703 -23.9267978668213
13.7515687942505 -25.1209716796875
6.5018892288208 4.34829998016357
36.3386535644531 5.60015201568604
20.7345447540283 -8.5824089050293
-31.1438808441162 37.1359024047852
7.7760705947876 4.41445922851562
-0.224455133080482 37.9046096801758
-0.872336268424988 39.0366630554199
6.27648162841797 5.99834251403809
-1.24881660938263 -29.9596004486084
11.167576789856 30.0025253295898
18.3693981170654 -5.75292348861694
-18.924955368042 21.9448833465576
-7.92072200775146 16.6391792297363
0.172491043806076 38.5808906555176
-4.60988235473633 32.8534278869629
35.7161293029785 -12.2297325134277
-31.4692916870117 36.6549835205078
6.75940465927124 4.49537754058838
29.7810916900635 -27.7166748046875
-10.9121761322021 28.2706298828125
-31.9252624511719 36.5245895385742
-40.0691947937012 -22.9942779541016
28.0657234191895 -27.6480846405029
-39.2121238708496 -20.6759471893311
25.2132472991943 -36.6734886169434
-2.87414574623108 -28.0605068206787
17.4771194458008 22.0568027496338
16.823694229126 -5.47056341171265
36.7234382629395 5.77093505859375
31.7979011535645 35.108081817627
-2.77574682235718 28.9859981536865
0.650815725326538 -12.1350145339966
18.7586135864258 24.80442237854
-0.322228014469147 38.5001068115234
24.0523147583008 19.1549625396729
-34.993335723877 37.1967315673828
15.0561571121216 -10.4963798522949
6.84445142745972 3.16456341743469
-1.56191539764404 1.23457562923431
20.3091411590576 23.843090057373
-16.280725479126 35.9904747009277
0.804445385932922 -29.4793224334717
-38.8173561096191 -31.022066116333
-0.297482073307037 -22.1331462860107
0.338683992624283 -14.6830768585205
7.08380126953125 3.4382655620575
7.38524389266968 37.5299682617188
21.1026039123535 -1.10965061187744
-33.5189781188965 38.5488471984863
-32.6539535522461 38.6729393005371
-2.0617516040802 -26.6126480102539
-5.71780490875244 17.2562522888184
-40.439022064209 -20.5568904876709
-2.81200003623962 1.09518551826477
-7.59725999832153 17.3992252349854
36.5499000549316 -13.1574077606201
25.625431060791 -37.3202896118164
-2.14211893081665 38.4901847839355
-14.2380094528198 36.1202621459961
34.6610488891602 4.42507648468018
-34.0053634643555 37.2475509643555
-33.8085289001465 40.0388069152832
34.6914100646973 37.2189559936523
-38.7470626831055 17.5412750244141
1.91565644741058 -28.8204860687256
-4.14367485046387 29.041130065918
12.0711002349854 -27.0886344909668
-35.1326484680176 22.6016082763672
25.0749988555908 18.8778991699219
34.0382537841797 6.08484077453613
-7.43741798400879 18.2878723144531
-13.6334342956543 36.4264717102051
20.1845455169678 21.911735534668
12.9168815612793 37.0282096862793
24.4874000549316 19.4733409881592
24.2129898071289 17.5347862243652
-5.59193229675293 12.7166452407837
26.0741481781006 -36.2718086242676
-20.3523063659668 19.4801635742188
21.6206645965576 -25.715124130249
-0.281354069709778 36.4094772338867
5.70004796981812 39.2284278869629
-1.41595840454102 0.771568238735199
-39.8728904724121 20.7405624389648
1.54191291332245 -12.2524538040161
22.4620933532715 20.072172164917
22.8140869140625 19.1292114257812
-39.1064338684082 17.6863670349121
0.692724406719208 -22.0052223205566
3.2040536403656 -12.3186292648315
33.9128379821777 35.9610328674316
-31.4019908905029 37.5637016296387
-1.13947808742523 37.7680740356445
-32.1628341674805 37.5643997192383
35.0404853820801 35.2743377685547
-5.46207237243652 18.5382766723633
-38.988109588623 -31.3436870574951
11.0841064453125 30.2681922912598
22.5548629760742 2.47235727310181
28.7011547088623 -25.7515277862549
23.194881439209 -13.5410814285278
34.5185699462891 5.71185636520386
24.8464050292969 -35.2880363464355
19.6921501159668 -9.40650749206543
-37.9249725341797 -31.435977935791
-17.0293369293213 22.6363677978516
34.3808555603027 36.1139221191406
11.8014965057373 37.2512283325195
4.93974494934082 4.87475633621216
28.9875164031982 -11.1415338516235
-15.5656862258911 35.8785247802734
17.3407459259033 -6.05658435821533
-1.84704113006592 -1.58735466003418
30.230993270874 -11.5076370239258
33.8733024597168 4.76091337203979
-39.8339500427246 20.2514572143555
26.5651435852051 -37.6236381530762
20.6767349243164 -7.16106510162354
4.24134254455566 39.6945838928223
-4.77953147888184 11.5008726119995
12.5799198150635 29.4586620330811
-33.762321472168 20.9615364074707
-0.47841888666153 -20.8537101745605
-3.22372651100159 2.3682107925415
11.5797472000122 30.137975692749
33.8427963256836 35.5252952575684
-39.3647956848145 -32.7760124206543
-3.35375642776489 1.06631112098694
-37.5078926086426 -31.673656463623
-30.8313694000244 39.4253921508789
-3.96851539611816 2.31730985641479
-12.8579797744751 36.1254997253418
18.0735816955566 -7.01855278015137
5.97873497009277 38.9186630249023
17.6458187103271 -4.2670578956604
27.4141006469727 18.8348598480225
35.5658531188965 -12.0484104156494
37.0460319519043 6.7560977935791
-21.4990844726562 19.6113910675049
-16.5387954711914 20.7749462127686
0.538583695888519 39.1178550720215
10.7467060089111 29.1186141967773
-15.5411548614502 36.0604133605957
31.1894836425781 35.7711563110352
23.6771869659424 -15.7142524719238
20.0633506774902 25.9651317596436
-39.451229095459 -22.9791965484619
20.7572994232178 19.2983779907227
32.7650146484375 36.7316780090332
-31.3934574127197 39.8822822570801
33.3039703369141 34.9190826416016
-38.1055603027344 -21.7316665649414
-5.52340364456177 11.1763315200806
-37.514575958252 -22.5526466369629
25.6035327911377 -26.8522071838379
-3.48399782180786 30.7365436553955
-5.1571569442749 18.2193603515625
-37.7570877075195 18.860990524292
0.337525546550751 -13.1720685958862
2.02660894393921 -13.5747489929199
-0.256079494953156 -28.6042728424072
12.3958349227905 37.0715255737305
-3.42384004592896 28.5414600372314
-2.44260573387146 38.7344779968262
34.1072120666504 36.6963539123535
20.3099918365479 -7.04965972900391
-37.9244155883789 -22.820650100708
25.627233505249 -23.6096973419189
0.411696135997772 -22.6309795379639
26.3671855926514 -26.3589973449707
2.87024736404419 -11.2056150436401
35.6787643432617 5.80242156982422
35.6230049133301 -14.360668182373
28.3194179534912 -29.0872344970703
35.2815742492676 5.3217339515686
18.7283172607422 21.6300392150879
20.1665649414062 -13.759726524353
7.3775315284729 3.87101531028748
6.59966659545898 1.71047592163086
-7.11768674850464 19.216739654541
12.2359504699707 -26.9847526550293
-3.14545321464539 -0.472603499889374
22.4755077362061 -25.6098861694336
-7.31826400756836 19.4515724182129
18.6654624938965 21.6094036102295
34.9054985046387 -14.0236825942993
31.5293140411377 35.1358604431152
0.041880302131176 -28.4623165130615
35.8909301757812 5.08459997177124
21.480001449585 20.5825443267822
-39.4729995727539 -21.3555603027344
-5.15106153488159 12.4949541091919
36.0225296020508 -15.0575103759766
-33.9835586547852 22.2352123260498
-6.41769170761108 11.4806966781616
-38.6478233337402 17.8935375213623
-15.7932205200195 36.1614532470703
-6.29179668426514 12.4406890869141
1.98395395278931 -10.6922464370728
8.3574686050415 4.50645208358765
20.3770790100098 -13.3962564468384
5.50959205627441 3.6883065700531
-38.6839828491211 -21.0592479705811
35.8878402709961 -12.6525754928589
-22.0595703125 18.9609622955322
26.7593860626221 -38.1016273498535
-10.1453008651733 27.8158683776855
-13.6716833114624 36.2978286743164
33.3595123291016 32.9807815551758
-38.9863624572754 18.7977313995361
-37.2164649963379 -21.8940315246582
6.07903861999512 37.7349395751953
1.34135138988495 -11.9464702606201
-16.2423973083496 33.5463981628418
17.4962024688721 -4.29128837585449
-39.3755416870117 -20.5536155700684
-4.44694662094116 30.9998245239258
-2.758873462677 1.67203545570374
19.1518859863281 21.2025718688965
32.9556198120117 36.3550415039062
22.005989074707 1.2886061668396
34.0084915161133 36.0310440063477
-7.51735496520996 17.0685577392578
1.28304612636566 -21.5425090789795
-31.9085903167725 39.0875816345215
-1.76859772205353 36.8785591125488
-0.576692759990692 37.3517303466797
-40.9092712402344 -31.458194732666
-2.49798822402954 37.4264221191406
-37.9188690185547 -32.3202056884766
14.6273593902588 -11.5805435180664
-39.3866310119629 19.842981338501
19.5071983337402 22.9349040985107
-37.9229888916016 -32.1530990600586
-34.1904945373535 23.6432323455811
-38.8581809997559 -21.9389743804932
-33.2120552062988 38.8141250610352
-37.2750396728516 -31.7401943206787
24.110860824585 17.7260227203369
36.7140846252441 -11.4764413833618
-14.5695943832397 34.40234375
21.9845371246338 -0.356134921312332
10.5729131698608 38.4251403808594
18.5158271789551 -5.34642028808594
2.75546526908875 -12.0644178390503
-0.50999790430069 -28.0734729766846
-16.6570892333984 21.1125717163086
12.945198059082 28.6103515625
-21.7119674682617 19.7717723846436
35.4910202026367 -14.9934453964233
29.5382099151611 -11.4632902145386
-4.00097417831421 0.473994076251984
-8.01201152801514 16.4337310791016
19.6181087493896 24.8483085632324
-8.56226062774658 28.5893783569336
25.171407699585 19.6432723999023
-6.19637632369995 11.7003335952759
37.2078056335449 6.46450519561768
0.770093202590942 -21.34641456604
19.6165733337402 22.4914836883545
25.5497150421143 -37.2272529602051
6.34471273422241 5.28097438812256
5.09369468688965 2.49040079116821
-14.5011224746704 18.2550983428955
15.5284042358398 -13.1238079071045
0.311109721660614 -28.2438335418701
34.4278221130371 36.1757469177246
16.1706523895264 -11.2234058380127
34.5680198669434 7.59131479263306
-14.1466817855835 35.9562492370605
24.5376110076904 18.8075046539307
5.7834038734436 4.59018325805664
-3.15479898452759 12.6217231750488
36.7489128112793 5.36569547653198
20.0075244903564 -7.97072839736938
-39.8294639587402 -21.93190574646
-0.635914921760559 38.2296905517578
33.053394317627 36.8887062072754
-3.00558853149414 1.49197018146515
-13.8694725036621 34.3809280395508
-38.6551933288574 -34.410831451416
36.5089225769043 4.43129682540894
-3.80607914924622 28.6644153594971
-4.64598989486694 12.3562459945679
-16.4328231811523 19.4765949249268
26.8771057128906 -36.7572555541992
-31.3693885803223 38.6236038208008
10.7591238021851 36.544921875
36.9249839782715 -11.6214714050293
-22.5834083557129 21.52707862854
-1.52857339382172 -27.5630931854248
6.65134143829346 6.29708814620972
6.42519235610962 2.81680107116699
-15.7389535903931 18.7028503417969
12.9813556671143 28.1549968719482
18.7110271453857 22.7442398071289
35.3202972412109 -12.3723306655884
28.5317096710205 -26.9091320037842
19.3912487030029 23.3471145629883
-4.89055395126343 0.599463701248169
-2.15156030654907 1.71107983589172
10.9972257614136 28.9091510772705
27.4456977844238 -39.5191650390625
0.498654454946518 -30.7092933654785
0.409479469060898 -27.6072330474854
-37.9352569580078 22.4456882476807
26.0888214111328 17.7526149749756
-3.15339398384094 4.22261571884155
8.96373176574707 39.4227409362793
34.0490455627441 -12.8993673324585
18.4253215789795 -4.64028310775757
-31.2364463806152 39.8764457702637
-14.5281047821045 17.9954109191895
-37.5813598632812 20.7833862304688
-7.8086404800415 29.8455638885498
-2.53337907791138 30.7204456329346
-39.5144882202148 -21.4094753265381
-1.66517996788025 39.1499366760254
11.6976757049561 27.6330738067627
0.746279776096344 -21.4638843536377
25.9065570831299 -36.3924522399902
24.1828269958496 17.9443511962891
-21.2969017028809 17.2164669036865
8.76348400115967 4.61114883422852
-16.8577098846436 17.8543758392334
36.1124000549316 -14.3910341262817
19.6412258148193 24.7260513305664
-33.0134963989258 38.8080406188965
33.0108833312988 35.3057403564453
17.7769718170166 -4.22418546676636
-22.6354389190674 19.0810737609863
24.1543445587158 -24.1763877868652
23.0868263244629 1.21296203136444
32.5217170715332 34.9831390380859
20.3820209503174 25.322566986084
-39.1256523132324 -22.5024795532227
-35.4039344787598 20.7601127624512
32.2598762512207 36.3047142028809
21.1451683044434 0.304419696331024
0.245677649974823 -29.8291530609131
0.398599445819855 -28.6301307678223
35.3136520385742 -12.4975957870483
2.18517637252808 -11.442834854126
19.2270126342773 -12.5684490203857
-36.7335319519043 20.6813430786133
27.2353191375732 -28.9189052581787
-6.42301177978516 12.2496728897095
16.6973876953125 22.3363399505615
-15.2056856155396 35.3925819396973
34.6550178527832 8.16536712646484
20.6247234344482 -7.79211664199829
-21.5395011901855 18.7097244262695
34.4832611083984 -13.3409881591797
-14.9684066772461 17.3115348815918
11.7823047637939 27.4535121917725
-5.94319677352905 13.0876665115356
34.9784240722656 37.3341522216797
0.281677961349487 38.7606010437012
-0.0675078332424164 -20.5376987457275
0.758062660694122 -11.6925067901611
-40.2202262878418 19.7693634033203
2.0508599281311 -12.4951572418213
-38.4848785400391 19.9842700958252
6.20554256439209 4.30818271636963
0.631349265575409 -29.0622882843018
-0.886402904987335 37.8651885986328
-37.9323501586914 19.7782344818115
25.2437725067139 17.3241081237793
-30.7656002044678 38.7038993835449
-4.5398530960083 29.6975688934326
-38.9196586608887 -21.0750007629395
-34.9231834411621 21.3869762420654
-39.215446472168 -21.2188835144043
-34.7612037658691 38.1774024963379
-14.523627281189 18.5977191925049
27.0476932525635 -37.8171730041504
33.2513122558594 36.663444519043
35.5931129455566 5.67390298843384
-38.4083137512207 -21.4312038421631
-36.9811363220215 -34.3454322814941
-31.1772747039795 38.9443206787109
-33.3371849060059 38.6825141906738
13.1137104034424 -27.907829284668
11.5864429473877 27.5715312957764
-39.2350540161133 21.2912464141846
-34.9421081542969 20.1636867523193
-3.53253149986267 2.72897052764893
12.3299074172974 38.486442565918
-38.3571281433105 -32.8599624633789
36.5575866699219 -13.0813007354736
33.8012771606445 6.17823171615601
-32.8163871765137 39.2982444763184
-39.7005805969238 19.1848125457764
5.76485395431519 4.15924787521362
0.584728240966797 -13.4190540313721
-0.886253893375397 -29.1523246765137
-21.7371959686279 18.0602493286133
36.9771995544434 6.14578866958618
33.3123321533203 37.2045707702637
33.8933868408203 -14.2573709487915
0.886430263519287 -13.5092334747314
19.9885139465332 23.1796226501465
32.4998054504395 35.1992835998535
28.211706161499 -28.8071327209473
-38.155143737793 19.4770584106445
20.8948783874512 -0.0384176187217236
27.1787967681885 -37.8470268249512
10.9300127029419 29.4760360717773
27.3547019958496 -25.0222969055176
5.81124782562256 5.94938373565674
-41.3548851013184 -21.9178619384766
33.0306167602539 36.3264999389648
9.91719818115234 28.774133682251
19.0388851165771 -7.73414611816406
35.5835914611816 34.608097076416
6.92085027694702 3.72609734535217
-12.6067419052124 34.5454254150391
16.9852924346924 -4.74310111999512
-14.8703584671021 17.3659839630127
};


==> figures/visualizations/gmm40/fab_samples.tex <==
\addplot [semithick, fab, opacity=0.7, mark=*, mark size=3, mark options={solid}, only marks]
table {%
-35.0898475646973 20.2985343933105
-37.2030258178711 -21.9764060974121
-35.7748146057129 -21.8364562988281
1.37226164340973 -13.3703451156616
5.44458913803101 5.1154842376709
26.5015926361084 -37.5061836242676
30.3890075683594 -13.3027667999268
30.0325508117676 -12.0945253372192
7.01852703094482 35.0983772277832
-4.41084384918213 29.3525829315186
-20.1281623840332 19.6096687316895
-38.3459320068359 19.0952186584473
10.093542098999 39.6276321411133
20.3817768096924 21.733850479126
13.5039548873901 -24.1962242126465
21.43918800354 -26.0006904602051
12.9017734527588 36.092098236084
-12.706371307373 38.3831596374512
23.5118370056152 -27.2825565338135
9.956467628479 25.4719314575195
-5.62282180786133 29.5326881408691
-2.83636474609375 30.7957878112793
17.6028575897217 21.3940448760986
6.80275869369507 6.29228353500366
18.5548839569092 -0.304248750209808
22.1389503479004 -25.5792369842529
-6.28280115127563 12.3636522293091
-4.24882411956787 2.32223439216614
-35.5451889038086 21.8442153930664
27.7445812225342 -13.096794128418
-2.44367861747742 36.7589950561523
-5.06814479827881 12.4697065353394
-1.22902309894562 37.4825057983398
-19.1050300598145 21.2972793579102
18.6454696655273 21.9386405944824
6.88602447509766 6.98320150375366
-8.42288684844971 19.7681522369385
-35.6176071166992 22.5850410461426
10.9544534683228 -27.6211204528809
19.8248291015625 -15.6736574172974
23.8119277954102 18.1422786712646
-39.2346076965332 -20.7780895233154
13.6725912094116 -13.8794136047363
-36.7173690795898 18.1070861816406
-3.77239799499512 31.3419094085693
-37.0277519226074 -32.2249717712402
20.6633739471436 -16.460823059082
15.2906227111816 -11.4375782012939
25.1115055084229 -25.6923847198486
12.2342319488525 37.3381729125977
24.8154926300049 18.2986431121826
-17.0805320739746 18.7642993927002
-39.9131126403809 18.6176013946533
26.5188999176025 -27.0607566833496
28.2497177124023 -11.478946685791
17.2846775054932 -13.735876083374
24.7715187072754 -17.3375053405762
-11.7567691802979 34.7915267944336
33.355640411377 -15.7249336242676
9.7808141708374 34.6460571289062
-4.52334880828857 11.0613222122192
-1.01428067684174 2.91012382507324
-39.6121788024902 -20.7959766387939
10.2560939788818 28.3581256866455
-17.2497596740723 21.8954238891602
-4.7359619140625 13.9332294464111
-40.3647270202637 19.2361431121826
-39.0614776611328 -29.819580078125
-11.7869358062744 27.2497215270996
25.1317749023438 21.5617504119873
-9.26074886322021 26.5040283203125
-2.87718057632446 10.0423517227173
1.01538264751434 -27.6933155059814
-39.7514419555664 -30.0176887512207
13.4217395782471 -22.1434574127197
-22.729362487793 21.8828315734863
-0.242701411247253 -10.2374134063721
-5.18424987792969 -0.550457954406738
24.4790153503418 -24.6982879638672
26.9192085266113 -26.5464706420898
-17.3485927581787 21.1693458557129
4.54391193389893 33.2666625976562
6.75506401062012 3.78962850570679
4.82615947723389 38.132381439209
10.512246131897 29.5260734558105
-31.0383968353271 41.6317939758301
21.7540664672852 -15.9456024169922
0.716275215148926 -20.6038436889648
-18.2388324737549 25.9379100799561
29.6305923461914 -9.57329654693604
-34.910831451416 21.211856842041
25.9245090484619 -36.4241752624512
31.7610931396484 -27.7241134643555
21.780933380127 -26.588794708252
25.3245410919189 0.0429284572601318
16.91721534729 -1.90483021736145
17.4792366027832 -11.1930551528931
-15.846040725708 34.7303848266602
-3.57503271102905 29.5047626495361
-0.803297758102417 35.1516799926758
22.7828788757324 -26.020580291748
-19.3175964355469 24.5529518127441
-34.7561988830566 -30.4447574615479
17.0199451446533 23.0711078643799
13.0221309661865 29.7491779327393
19.6123390197754 -26.505687713623
28.4026279449463 -26.7771072387695
32.7591552734375 36.4344520568848
-38.4295043945312 -22.6626281738281
25.8450412750244 -37.1650695800781
-33.7024078369141 19.4598255157471
-14.5322923660278 18.9971828460693
-5.85246276855469 30.6285457611084
-40.0475082397461 -31.5224571228027
21.549654006958 23.949779510498
19.4690074920654 -13.0237045288086
-2.31170606613159 13.1199293136597
-37.7766571044922 19.3783950805664
-20.1252212524414 20.6773509979248
-39.699161529541 -20.9278831481934
-32.8915672302246 39.919677734375
-21.9054870605469 19.8594741821289
18.7997055053711 23.7185153961182
8.56498908996582 1.81131529808044
20.3248596191406 -1.64020538330078
34.7299766540527 5.48148345947266
11.7461395263672 38.625545501709
24.7828330993652 18.8644580841064
25.5971069335938 15.8195314407349
-1.21139097213745 0.386908292770386
-6.94334554672241 17.8017864227295
21.9496879577637 0.62836217880249
-27.4115734100342 44.2849235534668
20.0862674713135 22.1544628143311
-34.8769226074219 22.2790412902832
11.1932201385498 -26.2716770172119
17.3321933746338 -5.86602115631104
32.9084320068359 36.2487907409668
22.1830024719238 -24.6377964019775
-2.82454442977905 3.0355179309845
23.2027492523193 -14.2115268707275
35.5509300231934 -15.0862617492676
27.6123352050781 -11.1357107162476
-8.53686428070068 18.8698539733887
-36.5198211669922 -20.9044628143311
-37.7858276367188 -23.4025478363037
0.0358453989028931 -11.294900894165
18.3058052062988 21.4479427337646
25.8196792602539 17.5360774993896
-38.1069030761719 -29.6135139465332
-4.91994762420654 4.87802839279175
-7.04256629943848 17.4580268859863
-10.0920391082764 28.0335235595703
26.1456127166748 -26.7883338928223
19.2316017150879 -5.52181816101074
35.6051712036133 -13.610613822937
-3.74017548561096 15.4217576980591
20.8350391387939 22.4273223876953
6.04193162918091 6.78528070449829
-4.19849109649658 12.7759628295898
-35.7885475158691 -31.5838451385498
2.14943647384644 -22.0871410369873
36.746223449707 -14.4825000762939
-5.50484943389893 9.482497215271
31.426872253418 33.2297058105469
18.0600700378418 22.6499843597412
-5.02605104446411 12.8973398208618
-41.1645278930664 -27.1245498657227
-23.8117008209229 20.550745010376
-3.62816405296326 40.7009468078613
27.1936912536621 20.5667858123779
19.2394428253174 -12.1517953872681
-19.0896759033203 20.6523323059082
-38.0657234191895 -17.5723972320557
3.85685205459595 -13.1097373962402
-34.814208984375 21.2209396362305
-38.3463325500488 18.9844264984131
-37.9925727844238 -32.5678977966309
-12.304970741272 35.635440826416
-3.91777801513672 16.2903900146484
-6.85171031951904 25.9837589263916
-39.8226432800293 -19.6445331573486
20.7208671569824 -12.5903615951538
26.300708770752 -25.7600898742676
5.9096622467041 38.9683113098145
-39.4687309265137 -20.4679546356201
1.28550601005554 -19.3521919250488
-38.9882850646973 17.2709197998047
-15.9495162963867 36.0430793762207
21.5305786132812 -24.2433395385742
-9.76530265808105 30.1799259185791
1.11696982383728 -13.2004547119141
17.0136547088623 -7.86128425598145
-21.1792392730713 18.4541244506836
-14.4949045181274 38.4829139709473
-21.8493404388428 21.9184017181396
-4.54169654846191 -0.937384307384491
-10.5070514678955 28.6326370239258
25.2422485351562 -16.3585929870605
-18.13987159729 20.8110694885254
-1.27691888809204 37.4177551269531
35.2884101867676 4.11274576187134
-38.5181884765625 -29.4674987792969
21.7529125213623 1.53649210929871
-1.02965295314789 39.7957420349121
27.1701030731201 -35.708423614502
23.7225589752197 -24.6528511047363
-17.1768283843994 20.8732128143311
27.5023155212402 -25.0896472930908
-6.11390018463135 18.8893165588379
33.1653861999512 6.51922130584717
19.3684883117676 -4.31380558013916
21.870735168457 -24.7356777191162
19.3966617584229 -7.88684797286987
-37.4031677246094 19.4650497436523
-5.92309284210205 26.5790100097656
25.1954765319824 -38.1546096801758
1.2352032661438 1.73591661453247
-37.9251098632812 -34.0024337768555
-5.51725006103516 -18.7780227661133
16.9182643890381 -5.43928289413452
-22.0598545074463 19.3193244934082
19.8604011535645 -26.3268966674805
-16.8545608520508 32.484001159668
-34.0761070251465 21.8834571838379
12.3113565444946 39.2142753601074
-6.60404968261719 16.0947036743164
7.23150444030762 3.05493521690369
19.0918598175049 -6.98841524124146
31.3734245300293 7.22843074798584
10.4435844421387 3.29672384262085
6.56568193435669 5.7429027557373
18.5566825866699 -5.86632347106934
23.7971801757812 16.0734634399414
-39.7336883544922 -21.9029159545898
25.148307800293 -23.9342212677002
23.592113494873 -14.3111143112183
-8.79831695556641 19.2634716033936
24.6610736846924 19.5919380187988
15.1192464828491 -6.04004764556885
-31.4295654296875 -34.0023345947266
-38.2601089477539 -30.6409473419189
9.7399206161499 37.5926055908203
23.5900936126709 16.1709690093994
-3.52200603485107 29.6764011383057
17.9745349884033 -3.97264957427979
-37.8283462524414 -31.6351585388184
-0.238045454025269 -9.34281158447266
-0.514032363891602 39.5398216247559
29.314359664917 31.2671661376953
-39.649040222168 20.4982299804688
28.4479789733887 -27.8174915313721
9.33712387084961 29.5159721374512
31.4098567962646 33.6433296203613
-38.2955665588379 21.5860538482666
25.7162132263184 -25.5526351928711
2.12958002090454 -13.0311431884766
13.2162399291992 28.3426094055176
-5.34749317169189 31.8853015899658
-9.30086421966553 18.3892612457275
11.9833183288574 -12.8797960281372
-9.6811990737915 30.0238494873047
-4.33995056152344 30.3770408630371
5.18121862411499 4.56684446334839
-16.2115917205811 35.6672172546387
-40.3892021179199 -32.2744369506836
-2.2555558681488 13.2960338592529
-35.267017364502 20.6876316070557
34.0595626831055 6.67778778076172
-18.0887413024902 20.7713832855225
25.2070865631104 -25.1681518554688
-38.0103530883789 -30.9459857940674
-12.5118637084961 33.528694152832
20.5013847351074 22.9345798492432
27.9194793701172 -27.5725345611572
10.0006122589111 35.2946510314941
-5.31840562820435 12.2052631378174
-1.77227306365967 30.0027904510498
20.0066814422607 23.4735641479492
15.5159883499146 -13.1149320602417
-18.0084781646729 21.2374057769775
-20.2410583496094 18.6962013244629
14.8061037063599 -11.9232187271118
17.4259243011475 22.8779735565186
26.9814968109131 -37.8778877258301
-8.70629501342773 17.9995174407959
10.9568300247192 -15.7433128356934
-7.86899900436401 19.3200244903564
-40.6951217651367 -19.5290927886963
-14.6380186080933 19.6328468322754
10.456618309021 26.3940467834473
11.3602609634399 38.8106346130371
29.0948429107666 -11.5718936920166
-19.4886322021484 24.1273326873779
20.6115818023682 -11.7816963195801
2.74913263320923 -18.9755821228027
18.7605228424072 22.8905849456787
-27.8011455535889 -18.4767646789551
24.8369636535645 -25.8299102783203
-3.24308657646179 2.93484139442444
-14.677116394043 34.0906448364258
24.5600414276123 16.9335899353027
23.9962291717529 -26.641019821167
0.141388177871704 -13.959056854248
35.0000152587891 37.1951713562012
-37.2267074584961 21.8668460845947
-35.4384536743164 18.9652938842773
-16.2875499725342 17.4852352142334
-34.8589324951172 18.3649368286133
2.22922277450562 -12.1562633514404
-8.46255874633789 17.4747581481934
15.8622169494629 -11.4385318756104
7.12072134017944 3.87949562072754
1.77476322650909 -15.0752506256104
1.06057906150818 -28.6063976287842
24.8529109954834 -26.7378768920898
-38.0910263061523 21.3299121856689
-6.08713722229004 39.5959358215332
22.1668701171875 -26.0175228118896
-1.26469552516937 -27.0852298736572
12.4552011489868 -24.09596824646
-0.477220684289932 -21.1621017456055
28.274242401123 -11.5264205932617
12.8295297622681 38.1823577880859
34.6352043151855 4.67892551422119
7.61263465881348 2.75233769416809
-0.223866581916809 37.122859954834
16.3003349304199 -10.2033948898315
-41.7111129760742 17.8115043640137
27.4396190643311 -35.6820526123047
32.9801979064941 36.3031158447266
11.3246231079102 27.6472511291504
18.4587993621826 -8.51615619659424
26.4401512145996 -24.2765426635742
20.2748241424561 21.4829273223877
-1.12465393543243 36.6530876159668
17.725284576416 24.4758796691895
-36.8300933837891 -20.7670516967773
-21.0051956176758 22.7499332427979
25.036304473877 -23.8272800445557
34.5896377563477 -14.4830303192139
-0.607581257820129 -15.5117692947388
-36.6581687927246 22.3158531188965
-18.5038280487061 22.5299091339111
13.545693397522 -12.5959234237671
34.295051574707 31.2399311065674
-2.43075323104858 4.29721069335938
-34.5056533813477 -35.0519981384277
24.4425086975098 -27.5023727416992
6.44533348083496 0.270059108734131
-3.41613507270813 1.43924140930176
-32.3292045593262 39.4439582824707
21.0515747070312 23.7729682922363
18.2211494445801 24.9379863739014
5.12135744094849 36.9362335205078
17.5659065246582 -9.70370769500732
20.3273010253906 22.3787612915039
-7.18056344985962 19.5581340789795
20.6959323883057 -13.3225688934326
-37.1068420410156 21.1185169219971
-1.55486178398132 30.5816802978516
11.1809816360474 -24.8030910491943
12.9017705917358 -29.142749786377
23.7352600097656 23.3723678588867
-33.6223258972168 20.7079563140869
34.9123878479004 5.22896909713745
-37.4582824707031 18.0817108154297
22.7776660919189 -27.1995544433594
24.3569660186768 -25.2037410736084
8.71672248840332 5.71031093597412
-2.27712774276733 28.1264991760254
-6.69072103500366 25.333324432373
1.9472074508667 -21.154899597168
25.3333015441895 -36.8636131286621
8.71468067169189 -25.5786571502686
35.5040473937988 36.8001861572266
21.1240978240967 -6.99075078964233
-22.7308883666992 19.7119235992432
21.5256175994873 22.971399307251
23.3289203643799 -16.177490234375
-33.5476226806641 5.0801420211792
17.4038543701172 -4.22697496414185
-21.2525253295898 18.8104515075684
0.47482430934906 -20.1882133483887
-40.1476783752441 21.9396724700928
11.59046459198 -24.2236576080322
-33.4385719299316 37.4467163085938
1.18679845333099 -19.8845863342285
9.07395553588867 29.8078670501709
-3.94994616508484 30.5625591278076
22.6301116943359 -0.102064281702042
-34.9150390625 40.1749534606934
15.2097425460815 -11.4075584411621
-37.14111328125 19.0848255157471
16.7714538574219 -10.9425449371338
12.0219573974609 -27.5730648040771
22.8643836975098 1.42068421840668
19.0104026794434 -8.21299457550049
-0.785074710845947 -12.1738796234131
23.3228034973145 -1.15950572490692
-39.1376190185547 19.6981525421143
22.191822052002 -22.7410755157471
11.8161640167236 26.0825023651123
16.6092185974121 -9.51722240447998
3.7694365978241 3.50995016098022
18.7947235107422 24.3307437896729
5.33810710906982 5.97572040557861
-6.59825229644775 8.96770000457764
19.7205486297607 23.5150890350342
27.8349418640137 -7.89736413955688
-34.3371543884277 36.3368835449219
-1.94442224502563 35.655330657959
19.248815536499 23.0677509307861
0.400460720062256 37.2897605895996
-3.70805191993713 32.3141021728516
-9.75211906433105 19.0192222595215
-10.4933853149414 35.5491142272949
26.1225891113281 -37.1814994812012
-34.9808235168457 20.1485023498535
25.3767166137695 -38.8945465087891
16.9796657562256 -12.8481750488281
-8.20772743225098 26.7628593444824
33.2989654541016 35.2003364562988
36.0316505432129 -12.8962993621826
27.6664009094238 -26.081033706665
-34.773868560791 -22.5747184753418
28.9976139068604 -11.0578117370605
19.3754558563232 21.4488391876221
21.643253326416 -14.3673219680786
-5.44953298568726 10.0324039459229
20.5115623474121 -13.8072786331177
2.38164973258972 -14.1547451019287
30.0390090942383 -12.5138053894043
-39.3496055603027 -32.8253479003906
-35.3926162719727 34.3617286682129
20.1889724731445 -1.18701815605164
22.483907699585 -26.5566444396973
26.5410804748535 -27.1771430969238
-41.6634559631348 -33.537914276123
-33.660717010498 22.1304054260254
-2.72269630432129 38.5823364257812
-4.18428564071655 9.12741279602051
15.0399513244629 -27.5867118835449
12.3514862060547 30.3931980133057
13.9598798751831 -10.8792591094971
-33.9566345214844 19.9568958282471
-18.884334564209 21.792293548584
-34.613353729248 22.3543376922607
19.9937076568604 23.7096576690674
8.28383255004883 38.7539138793945
-3.00095891952515 1.02531230449677
22.6852169036865 17.4049510955811
19.2532405853271 -15.0352830886841
12.498083114624 27.8634376525879
6.68049097061157 3.9413754940033
-7.18060970306396 27.4874095916748
15.4261407852173 -13.1180629730225
-1.03914153575897 0.306253790855408
-15.5169353485107 35.8184700012207
3.26265573501587 -15.3509187698364
19.9484767913818 22.7735652923584
22.6185874938965 -34.4733772277832
-16.3179950714111 18.2293281555176
-37.4591178894043 19.9707126617432
5.69363307952881 3.62540698051453
-5.0908031463623 29.404239654541
21.8242092132568 -0.0727344751358032
16.3503189086914 39.1030769348145
-34.687328338623 -31.4212512969971
7.35972690582275 27.2467842102051
23.9634189605713 -25.2073421478271
-2.86765003204346 39.2465667724609
-33.0638580322266 18.5518684387207
11.2975988388062 -24.332239151001
-14.6244297027588 33.1707649230957
30.595890045166 35.8057518005371
-38.2618522644043 -30.9665908813477
29.2390880584717 -15.4728527069092
25.2270832061768 22.4036731719971
-4.23860120773315 28.8573036193848
-19.6039447784424 21.6773147583008
11.6048393249512 -25.7419300079346
20.1300258636475 -12.8229026794434
28.2834815979004 -27.659158706665
-18.2200374603271 21.001651763916
-15.7756624221802 18.4591121673584
23.3303909301758 19.887056350708
-18.1413326263428 18.8623199462891
-3.49731469154358 39.030818939209
11.4884967803955 28.498628616333
-33.3395652770996 36.5507583618164
-6.11271715164185 13.6808891296387
35.949951171875 8.13283729553223
35.5541000366211 -13.6884517669678
15.1644124984741 -6.56532859802246
-35.4886779785156 -21.3567810058594
29.6810817718506 34.0825538635254
25.8776226043701 18.3932685852051
26.3154850006104 16.1749076843262
23.4373207092285 18.8532009124756
19.8098068237305 24.937292098999
22.8290977478027 17.5717945098877
11.931173324585 29.7511291503906
16.3535633087158 -13.0601167678833
-12.1832485198975 34.8563842773438
9.15400505065918 29.6078491210938
31.9920597076416 6.44904947280884
-7.64158630371094 19.2554836273193
-38.222957611084 -30.2481899261475
-14.0056467056274 18.2704563140869
-1.76214361190796 -27.6863899230957
6.07687330245972 34.9497718811035
-14.8319253921509 36.1945610046387
35.6343116760254 -13.7887401580811
11.6050043106079 2.47019815444946
26.7899208068848 -35.716869354248
0.955231070518494 -23.5154113769531
21.2187080383301 -6.55867433547974
9.94898128509521 29.2691841125488
-36.7425765991211 -29.6847648620605
7.68832015991211 39.9635200500488
19.5128479003906 23.5322914123535
34.4808349609375 -13.0727386474609
25.1013431549072 -26.1272125244141
23.1012725830078 20.0839500427246
30.398624420166 31.2506122589111
-5.05665683746338 16.3449172973633
-34.9230995178223 37.4543914794922
-13.7356414794922 35.3492965698242
-36.4383583068848 23.8240985870361
19.296293258667 -4.52146053314209
22.6109943389893 -34.6460037231445
-0.206270396709442 -27.1268138885498
18.4722938537598 23.068531036377
-8.60653209686279 30.4413261413574
24.2196140289307 -24.8933277130127
-2.42222166061401 30.702693939209
36.9046669006348 8.41462421417236
29.0930500030518 -28.4717617034912
-37.0268440246582 22.9731330871582
-41.5991401672363 -18.5645637512207
-8.1692476272583 26.4461193084717
-39.6385345458984 -24.6606311798096
27.5923538208008 -29.4619407653809
17.4739360809326 24.4727535247803
17.5300121307373 24.8302974700928
-0.349011301994324 -26.5551567077637
29.6597366333008 32.0160026550293
-3.23568844795227 13.3095092773438
-39.2446899414062 -32.5449409484863
26.1168842315674 -26.7111988067627
-4.83486557006836 29.1499729156494
20.4535522460938 24.1625785827637
7.60187768936157 4.99548530578613
36.9793853759766 -11.5137596130371
-5.84098625183105 32.518440246582
-12.7716674804688 33.8432083129883
34.0798072814941 6.31816959381104
28.5252017974854 -12.8898487091064
-36.4281044006348 35.9547462463379
-5.31348562240601 29.0690994262695
-9.71152591705322 26.614013671875
-7.50701475143433 19.0372467041016
-28.9764595031738 39.6513671875
34.3079109191895 -13.1639766693115
22.3942527770996 -23.7412395477295
17.1558494567871 1.69285869598389
31.9465522766113 38.489933013916
-30.9128971099854 37.0668830871582
-1.54354643821716 -13.8694276809692
-15.3422813415527 35.0373153686523
-3.51031374931335 28.8650150299072
29.9896049499512 -12.1292171478271
34.409049987793 35.4400863647461
12.7397222518921 -23.4704399108887
-39.3611526489258 -20.1657810211182
6.16719245910645 40.5510482788086
-40.3666534423828 -30.4682579040527
-19.4810886383057 37.8184661865234
27.5070114135742 -26.8221855163574
-35.1718482971191 21.3372478485107
31.854923248291 -11.6979074478149
-39.9783134460449 -22.5684032440186
-40.0977592468262 21.1246509552002
33.6950492858887 7.79309940338135
21.0200500488281 -14.7405185699463
-2.40458035469055 12.6287488937378
17.4311790466309 23.3934993743896
20.1576633453369 -13.5399560928345
23.9407024383545 -23.9840393066406
1.6555187702179 -14.3579158782959
-32.8073234558105 34.5986595153809
25.4734039306641 20.7148780822754
-32.9778137207031 37.0750274658203
6.82333517074585 3.53675365447998
34.8471870422363 -12.1885461807251
19.8710193634033 -9.07561302185059
23.1964378356934 -24.1927833557129
23.8677501678467 -13.545578956604
-43.8428230285645 -41.5317535400391
20.8337860107422 23.1981639862061
38.097770690918 -13.1150074005127
-39.6437530517578 -23.5198459625244
-37.9899978637695 20.1837749481201
-18.1044692993164 21.2823429107666
13.963264465332 -26.3691825866699
-39.4915809631348 -22.8189563751221
6.30739498138428 39.7774085998535
-10.0009593963623 27.8357067108154
-14.985725402832 18.216287612915
0.0232268571853638 0.279640376567841
-7.66469192504883 28.8933010101318
20.4408149719238 -2.00950241088867
1.40508103370667 -14.5251140594482
-3.21811008453369 1.30732440948486
14.124924659729 -11.8366136550903
-16.3325290679932 17.8897438049316
23.8300704956055 17.4418659210205
8.32525157928467 28.7969226837158
27.0993614196777 -28.6679515838623
23.9497489929199 20.9535846710205
21.9452514648438 1.04598701000214
21.2170524597168 -6.01803874969482
-3.50896096229553 32.5008010864258
-42.1501502990723 26.2537403106689
27.7997055053711 -13.1291780471802
34.0113830566406 35.2847633361816
-30.7182273864746 37.9446334838867
19.7868995666504 -8.07969760894775
-12.6300954818726 36.1557540893555
7.05978631973267 5.71540403366089
-36.1765899658203 -20.4827079772949
-34.9245719909668 36.3016624450684
-38.8203086853027 20.6297988891602
18.7578392028809 21.9812793731689
18.4734287261963 -9.43311786651611
-8.73776340484619 30.0916328430176
9.59390068054199 29.2680282592773
-3.22521781921387 2.76833271980286
-1.17008495330811 40.5337982177734
-36.6528396606445 36.3509750366211
20.4912662506104 22.1934013366699
-35.7438201904297 21.9746742248535
13.4646091461182 27.9958629608154
18.2196464538574 23.8405990600586
8.94381046295166 3.84326338768005
5.72085523605347 37.187671661377
19.4018898010254 22.9900245666504
28.6166458129883 -10.4758024215698
-38.508602142334 -21.1517295837402
0.77616286277771 2.81685090065002
23.1229858398438 18.6797294616699
11.7991724014282 -25.9827899932861
-36.3491668701172 20.668140411377
-33.5205497741699 37.075122833252
-15.2281398773193 35.1319541931152
37.3256149291992 -13.924952507019
-40.8137359619141 -34.7457275390625
33.4684448242188 8.01090717315674
12.5338582992554 30.096607208252
-39.895092010498 -32.4608459472656
-20.8184642791748 20.6458015441895
-21.8675765991211 19.2823371887207
29.6065444946289 -28.7249565124512
24.9902858734131 -35.7929000854492
2.51948118209839 -13.8059883117676
-0.515872240066528 -31.1160316467285
20.340389251709 -13.7514839172363
-37.1601486206055 19.4796562194824
11.6967697143555 36.6704292297363
-34.3847007751465 36.1782417297363
15.1333255767822 -13.1284523010254
30.1436595916748 -11.5556697845459
-35.7985725402832 -31.5945110321045
-16.9635047912598 22.7670860290527
25.3302154541016 -38.0704154968262
-17.7658958435059 37.5439109802246
-22.8792419433594 21.9846000671387
19.7576999664307 -3.36775755882263
-34.2803115844727 39.6578903198242
-11.2151727676392 29.8527584075928
2.98894047737122 -12.6760654449463
5.57094860076904 35.9390144348145
-34.5315818786621 22.8766288757324
9.33317470550537 37.4704093933105
-1.2931489944458 36.5273666381836
17.0216522216797 -11.253490447998
22.1132965087891 -24.5265522003174
5.65480756759644 5.63157558441162
29.6862545013428 -13.0033082962036
13.2465953826904 -26.2737941741943
-1.93552541732788 37.0935325622559
15.8434963226318 25.0284118652344
37.2350120544434 -9.09967994689941
13.3236379623413 -25.5129280090332
-8.2763614654541 18.0855083465576
26.856029510498 -9.72878646850586
-4.6418137550354 11.9248132705688
9.68009376525879 28.711633682251
-2.80139374732971 28.2452507019043
-40.5135116577148 20.0043525695801
19.4218215942383 20.3518180847168
17.5856628417969 -5.80360698699951
33.095458984375 -11.460090637207
14.4506845474243 -11.3176851272583
21.8328437805176 -13.547176361084
-5.11054039001465 1.22438263893127
6.71800994873047 -0.284117698669434
17.0437107086182 1.84252679347992
-40.2379875183105 -33.1286163330078
27.9078731536865 -28.9089679718018
23.4890480041504 19.3483238220215
27.6562690734863 -24.8785514831543
-1.20658683776855 -30.0772132873535
-3.14583158493042 25.8995819091797
27.6061153411865 -12.7032070159912
-20.9059638977051 19.005672454834
21.9706630706787 24.1316432952881
10.3237161636353 3.87797355651855
4.64940643310547 39.5317115783691
-22.7981185913086 21.4808311462402
13.3763904571533 28.6411952972412
25.5937747955322 -25.3122749328613
13.3842391967773 37.4103050231934
24.0165100097656 18.0217704772949
13.2748193740845 -26.9083786010742
-21.958703994751 19.4388389587402
18.7365436553955 25.0106430053711
33.621639251709 -11.9376668930054
13.7287883758545 -26.6516246795654
10.0423564910889 6.06443166732788
-3.74495601654053 38.9657821655273
-6.47039318084717 19.9727573394775
-1.44067823886871 1.01684069633484
12.5849361419678 35.7787322998047
26.6102142333984 -25.167200088501
0.503177165985107 -12.4174470901489
-9.47152042388916 -11.8513031005859
18.4494094848633 21.2171459197998
1.92661571502686 -27.7866382598877
24.2271728515625 -9.06528854370117
20.0681953430176 20.9040718078613
23.7424564361572 16.0000877380371
24.3773822784424 15.2793684005737
27.6622085571289 -28.6727199554443
10.9279747009277 28.4448680877686
19.8809642791748 22.8692359924316
16.8390369415283 23.7289066314697
17.5965595245361 -9.72821712493896
17.61061668396 20.6173648834229
36.179630279541 6.24059343338013
-4.11847734451294 13.5518970489502
18.4826240539551 -8.31285858154297
33.2419052124023 -8.59851741790771
18.5944766998291 -8.43477821350098
-16.6539897918701 17.2865295410156
-4.94628524780273 12.3128385543823
23.1462631225586 -14.6124153137207
-3.30407571792603 -13.1362609863281
26.1594905853271 -25.4501476287842
-1.50971150398254 -30.4830017089844
-19.8397274017334 18.9428768157959
10.3475713729858 29.8455219268799
22.9271793365479 -25.9128532409668
36.1530838012695 -13.5787353515625
12.0071620941162 37.3745307922363
1.55161499977112 -20.2760238647461
28.3937110900879 -28.1847190856934
19.92893409729 5.77164745330811
-11.1489925384521 27.8064842224121
1.36749839782715 -11.3656091690063
-0.949063897132874 37.61865234375
18.9966239929199 -6.91579437255859
10.2564964294434 28.6277465820312
24.9712905883789 -38.0599784851074
15.1677856445312 -23.4949645996094
11.1563405990601 28.5096645355225
-0.404125213623047 -20.6276321411133
33.7104759216309 -11.2831974029541
12.7640256881714 28.9453411102295
-7.17374134063721 11.0663499832153
26.6627063751221 -26.0747489929199
-14.8264589309692 34.3327865600586
19.5334606170654 20.4760303497314
23.4315357208252 18.1933650970459
-35.3678588867188 33.176872253418
28.5138931274414 -11.8082056045532
-16.873161315918 36.0055503845215
-17.7950534820557 22.1885585784912
1.39349591732025 -29.3560066223145
16.4782695770264 4.03895092010498
11.5423994064331 35.7644424438477
19.5313968658447 -6.86012554168701
31.1448650360107 34.4853096008301
27.6715793609619 -13.3580408096313
-30.3014869689941 38.1065101623535
-38.8439750671387 -22.9102973937988
33.1022987365723 36.053653717041
18.4287071228027 -5.7346887588501
4.70377111434937 40.1251754760742
-3.14129590988159 12.4240560531616
14.5375814437866 -13.5531711578369
-17.3224544525146 18.7892608642578
18.2323665618896 -5.26261043548584
15.3671951293945 -10.7867393493652
-15.5488128662109 18.7762546539307
-0.220913946628571 -29.8462333679199
-40.2133827209473 19.6691055297852
0.541632175445557 -22.2896137237549
28.4802188873291 -25.2418231964111
22.1089916229248 23.4225788116455
-39.7132873535156 -31.0493087768555
21.2375259399414 -0.830853044986725
-15.4626483917236 36.0765190124512
-30.9641380310059 38.5315208435059
26.2060680389404 -37.1025085449219
17.8274040222168 -3.731285572052
10.795262336731 31.0187149047852
29.8160552978516 34.4160575866699
38.8994369506836 -12.6378955841064
6.52841138839722 37.9260520935059
3.29691648483276 -12.5418481826782
-5.38810205459595 27.9618759155273
20.7693405151367 -16.6827545166016
-0.392724752426147 -21.9367923736572
-12.5038299560547 34.928653717041
-3.82507658004761 1.60468721389771
-2.91507053375244 29.876501083374
-34.5470924377441 20.7636699676514
-17.7673892974854 18.8000297546387
7.3187780380249 4.93001937866211
24.0559024810791 20.2895221710205
10.0241222381592 28.4723777770996
14.0104360580444 -27.2707901000977
-7.56099510192871 11.4548254013062
11.7361183166504 41.7949485778809
12.4369325637817 27.1381053924561
-25.6138248443604 44.0337181091309
16.145881652832 -11.9644956588745
25.2889366149902 -23.2570724487305
-34.5781135559082 -19.0871734619141
18.7063484191895 -6.17604207992554
23.0781173706055 -15.2063894271851
-40.469051361084 -22.4275989532471
-8.22327041625977 17.7628631591797
18.8680381774902 -4.59470510482788
25.2803955078125 -25.461576461792
27.2140617370605 -9.67249202728271
-39.3842277526855 18.348014831543
23.1072330474854 -27.5368690490723
20.194465637207 26.2724609375
18.0755062103271 23.9359741210938
-2.76532554626465 30.3537082672119
6.81401300430298 39.7404441833496
25.6681842803955 16.1851711273193
-37.5360908508301 -30.6603202819824
-11.4922227859497 30.3845405578613
-20.8530044555664 18.9582405090332
-17.6285934448242 20.8563652038574
-30.1076965332031 39.0904350280762
20.3583240509033 -7.83913612365723
28.6348686218262 -12.9024219512939
-31.2371368408203 36.1250534057617
-12.3158388137817 36.0621299743652
6.81229257583618 36.597599029541
-14.7445182800293 18.7167797088623
1.13019013404846 -11.4293098449707
7.73057746887207 38.662841796875
15.9767780303955 -10.6257076263428
14.2542104721069 -27.6169509887695
-31.0504093170166 38.4998626708984
11.4425973892212 -25.2395000457764
-9.93091869354248 28.9800891876221
-12.7122440338135 33.6055183410645
37.1983642578125 5.62701225280762
26.3916664123535 -37.6108589172363
0.419224083423615 -28.1203746795654
18.407356262207 -3.20979309082031
23.8571624755859 -14.8244867324829
-38.0302124023438 -32.0396270751953
17.1569557189941 21.2182636260986
34.4151344299316 7.13757991790771
21.4466400146484 -27.6774291992188
23.6666049957275 -16.6673221588135
30.2235851287842 -10.2319822311401
-33.3550071716309 39.2281913757324
19.1051406860352 -13.0343065261841
5.26069688796997 36.6665725708008
34.0454216003418 -14.3815383911133
11.4332666397095 24.7781066894531
-6.63947820663452 29.9561996459961
-12.1189126968384 28.4911556243896
-13.8351497650146 33.591724395752
1.40340983867645 -15.748987197876
28.0190925598145 -14.969220161438
26.1777305603027 -39.0496788024902
3.07273483276367 -13.0836811065674
-31.9705581665039 36.4358558654785
-35.0438995361328 22.6526355743408
-39.7661323547363 21.6664276123047
-32.1543807983398 37.8466644287109
19.533597946167 -14.3929662704468
13.0779371261597 28.1979923248291
-4.11076164245605 30.5455474853516
19.1277046203613 -11.8409585952759
15.7587327957153 -6.53783559799194
-1.69090723991394 0.131355047225952
-8.33433628082275 18.2921485900879
4.32141876220703 2.71595931053162
24.3200988769531 16.4744281768799
-34.0602188110352 21.7406730651855
-16.3380546569824 16.6256885528564
34.5773086547852 -13.4452753067017
-34.0153770446777 22.1653099060059
-18.8138275146484 20.7055759429932
7.08610820770264 40.0714454650879
1.21888959407806 -14.1541156768799
19.5953254699707 -4.09271430969238
-37.5431251525879 20.0143661499023
-34.0575065612793 37.1564559936523
-8.02287673950195 28.2260799407959
-30.2109336853027 37.7374610900879
0.443624287843704 -23.1257648468018
34.3729782104492 35.3891258239746
-17.6458358764648 16.8684101104736
25.116828918457 19.8139343261719
20.5631713867188 -2.47714710235596
-17.8143463134766 20.5620098114014
23.3670902252197 -25.1534786224365
9.83850574493408 27.848726272583
35.8520317077637 -13.6925849914551
16.3077030181885 -6.80004644393921
19.2886333465576 24.4898242950439
11.6765737533569 -29.5868186950684
28.0825634002686 -29.3969593048096
-40.5949211120605 -21.6232147216797
12.4157075881958 29.9973793029785
28.8431453704834 -13.9885540008545
5.50224733352661 38.2171478271484
23.9423561096191 -14.4050645828247
-32.0871429443359 37.3173637390137
-5.43910455703735 12.8040990829468
26.7677135467529 -32.4981231689453
6.51655912399292 1.49378430843353
-4.04483461380005 -1.49313127994537
3.48274517059326 5.90180730819702
25.2206649780273 -22.5288047790527
18.8959903717041 22.0218963623047
-3.3586254119873 27.7909717559814
19.9879837036133 -6.31976222991943
2.63659286499023 -11.6929130554199
16.5958786010742 22.2299308776855
15.6202259063721 21.622184753418
12.4312047958374 26.1061248779297
19.4762725830078 -5.43595504760742
9.50268363952637 37.3964576721191
0.714859127998352 -20.3597068786621
-33.8686904907227 36.7485847473145
-13.0677175521851 34.5794105529785
-17.88743019104 22.5823383331299
29.4951210021973 -13.7256736755371
27.2834167480469 -28.0566902160645
15.1286449432373 -25.529821395874
14.6343269348145 -12.66872215271
16.2860641479492 -10.9098749160767
-21.6803340911865 19.9952812194824
16.3338108062744 -5.98116970062256
0.198978185653687 -11.5260801315308
-37.8884353637695 -23.566951751709
22.9302234649658 -15.3819971084595
28.8221626281738 -14.1372966766357
1.63746809959412 -11.0124206542969
18.6140937805176 -8.43986892700195
27.9176025390625 -39.0247802734375
25.3292236328125 19.9082775115967
35.2809982299805 7.22769546508789
23.8713054656982 -28.1108894348145
32.8104667663574 33.8790512084961
12.0733165740967 28.3195381164551
-8.5664119720459 17.2302093505859
-4.72102832794189 30.2113571166992
20.2283096313477 22.1084098815918
-19.2899761199951 21.0218143463135
-37.2314262390137 -30.9895572662354
34.0854797363281 -13.2301864624023
19.8307189941406 23.2623043060303
4.91923809051514 40.5077362060547
26.4652309417725 -13.5735692977905
-34.8728866577148 22.6741981506348
-33.8985939025879 35.7863540649414
-34.30224609375 21.6858329772949
30.6773796081543 -11.1333141326904
-12.1270580291748 33.2485313415527
-20.7207336425781 21.2478675842285
-11.399320602417 27.2491683959961
23.9539566040039 19.6425914764404
-5.90757942199707 16.5681247711182
11.3286752700806 30.8573055267334
34.305850982666 36.5668792724609
-16.8982982635498 17.6831359863281
};

==> figures/visualizations/gmm40/gmmvi_samples.tex <==
\addplot [semithick, gmmvi, opacity=0.7, mark=*, mark size=3, mark options={solid}, only marks]
table {%
22.085563659668 -8.89354705810547
11.5344333648682 -28.7058563232422
-6.80036354064941 20.0720443725586
19.8311347961426 23.0908145904541
17.1082096099854 -7.01155233383179
-38.0323257446289 19.6396179199219
-16.6095542907715 20.6775665283203
6.68388748168945 38.4648208618164
23.2967834472656 -25.3108921051025
12.3647346496582 27.4461231231689
12.5202913284302 29.068151473999
-34.1262702941895 36.8135108947754
35.8240432739258 4.65394878387451
-38.2797470092773 -23.0614204406738
25.57763671875 -26.5428867340088
-8.35847949981689 27.1362228393555
-39.0181045532227 -32.6841316223145
-14.2463006973267 19.2091979980469
28.6821365356445 -13.5990104675293
-8.61923217773438 27.1226768493652
16.5133571624756 -8.67819786071777
34.2472496032715 39.030704498291
-8.3317289352417 27.8282260894775
-38.4416656494141 -32.4590873718262
-4.91748428344727 28.2379817962646
37.3619956970215 -13.1227264404297
-2.98437833786011 -29.7441539764404
12.5504198074341 -24.7861385345459
-10.0741119384766 28.3258094787598
-12.7719326019287 35.2362937927246
18.703275680542 22.4660167694092
18.8175506591797 24.2782344818115
25.9074745178223 -24.7646389007568
3.75137853622437 39.2048149108887
-0.87950325012207 28.6647243499756
19.8590488433838 23.2145977020264
20.4545288085938 -25.5626831054688
15.0433044433594 -12.0703763961792
-39.2802200317383 20.3464603424072
23.3722076416016 -0.698822915554047
22.2016925811768 -25.6849346160889
24.6492042541504 19.8158168792725
28.7406444549561 -11.8704919815063
31.937816619873 36.4628486633301
-14.6972684860229 35.5007591247559
-34.2212905883789 21.4731578826904
33.2405204772949 34.6775321960449
12.7343883514404 37.9068145751953
-39.4254493713379 20.5941963195801
25.5800914764404 -27.407527923584
-37.9058036804199 20.6539459228516
25.1394538879395 -25.2532978057861
20.4538555145264 -15.7895946502686
-37.5361480712891 -31.7721138000488
-1.72214937210083 38.5107345581055
12.9055204391479 -26.5959033966064
21.9223690032959 -24.413595199585
-3.68495321273804 29.8795032501221
-7.50048208236694 20.0998668670654
24.1907215118408 -25.7985916137695
16.8963031768799 -13.4543113708496
24.6333065032959 18.5892448425293
-14.9027910232544 16.8569869995117
17.6054782867432 -5.40769052505493
-38.1321907043457 -33.2911834716797
21.1522922515869 1.08345329761505
-2.17962598800659 36.8856544494629
34.920654296875 37.1556739807129
16.4271926879883 -9.94443893432617
22.4647235870361 -1.05272674560547
-38.7438163757324 -31.2754821777344
-14.3669471740723 17.8734283447266
-1.22895097732544 36.6646690368652
18.5140800476074 22.2272529602051
-14.3443241119385 35.982364654541
-19.0161876678467 20.1124954223633
21.6133995056152 -24.2965698242188
-4.48600959777832 0.589483737945557
0.238893449306488 -29.1961269378662
10.2177867889404 -25.2899589538574
1.9885641336441 -23.3771381378174
15.4088268280029 -12.3213291168213
-37.5786933898926 -21.1392841339111
-3.46591782569885 10.4542102813721
33.2970085144043 35.5430068969727
6.60455656051636 2.63885450363159
15.5762691497803 -11.5156507492065
18.1797962188721 -4.6998028755188
20.5707473754883 -8.16166114807129
1.97589886188507 -13.2432727813721
0.548412442207336 -28.2557621002197
20.2537078857422 23.5179424285889
35.0897789001465 -12.0901794433594
27.4311008453369 16.7564754486084
20.635627746582 -15.0866117477417
11.2487201690674 37.0811080932617
15.9016361236572 -5.30248546600342
17.7967529296875 21.6972732543945
-6.47626686096191 12.0228443145752
6.01527547836304 3.30681610107422
19.5196514129639 21.2323455810547
-8.00271701812744 17.8037624359131
-31.8902187347412 39.8598823547363
21.0530986785889 -12.8320417404175
17.8298110961914 -4.69690990447998
-15.2216796875 18.0553722381592
-35.0426406860352 21.1645927429199
0.499164998531342 -11.3220720291138
16.0572681427002 -14.1351385116577
-33.2486953735352 36.8682174682617
-38.4477005004883 20.5879802703857
11.437388420105 36.3461112976074
-5.7188401222229 19.0516052246094
5.5110182762146 36.3999824523926
-39.5202713012695 22.095329284668
21.3397331237793 22.5060081481934
24.8733234405518 -36.7813186645508
-19.1338195800781 21.5372505187988
-14.9154720306396 16.763427734375
-15.0009956359863 37.8817558288574
27.2155017852783 -36.9499664306641
-2.16706609725952 29.6645126342773
26.2492160797119 -24.6702861785889
23.954381942749 16.0860900878906
36.9460678100586 7.794508934021
-6.61121320724487 11.3846292495728
-2.51932168006897 37.8631401062012
19.9887638092041 -13.8077735900879
-20.2854518890381 19.6467132568359
5.78985214233398 4.45518159866333
12.2802772521973 27.7675113677979
-2.74257802963257 38.1238288879395
-14.0237874984741 35.4697189331055
1.22817373275757 -28.650333404541
-6.5112738609314 31.226318359375
-17.3952827453613 21.4509353637695
-33.059139251709 38.0534286499023
36.9460868835449 6.34836292266846
19.8391437530518 24.4836711883545
24.0626049041748 -36.9356956481934
30.3212852478027 -12.0459222793579
-8.40930652618408 28.5807857513428
-18.2247638702393 22.0579147338867
24.8009757995605 -26.165641784668
21.4584732055664 -15.5313386917114
22.7107582092285 -0.246922671794891
33.49609375 36.0483665466309
19.8283710479736 -6.693528175354
-16.8735599517822 22.1884746551514
36.0920753479004 -11.8268995285034
26.2821044921875 -26.6802806854248
-0.98149436712265 -28.6191482543945
-1.84686458110809 -0.853274703025818
17.7208137512207 -5.66689205169678
-12.9021282196045 34.9383277893066
26.7001457214355 -37.2712326049805
32.9297370910645 35.3021621704102
33.1829605102539 37.5049705505371
-13.4325428009033 35.228084564209
21.0552558898926 1.80036628246307
19.0073146820068 -4.36412334442139
0.965880155563354 -21.9724006652832
32.5618858337402 37.7707443237305
-22.9780540466309 19.5625038146973
4.50306844711304 38.5252838134766
19.7607555389404 22.4268417358398
29.6302928924561 -11.289252281189
12.4942712783813 -26.0491199493408
25.5398368835449 -27.1915378570557
20.5414581298828 -2.0940682888031
34.2941551208496 -12.4775381088257
-3.70499539375305 30.6987724304199
-2.20316362380981 1.74438977241516
0.599750161170959 -13.9833507537842
17.9193687438965 21.3432540893555
35.169620513916 -14.511926651001
17.9524974822998 -12.232738494873
12.3884134292603 38.6753540039062
6.09423542022705 6.34716892242432
-17.2691917419434 22.9320106506348
-5.52024698257446 30.9937744140625
-9.66526031494141 27.6690902709961
25.9445495605469 -39.4359436035156
16.4940929412842 -4.50404119491577
20.9239044189453 -0.745266437530518
10.8895635604858 -26.3894863128662
25.1665573120117 -37.3128852844238
0.0792631879448891 -28.5779552459717
-1.36014866828918 1.82757031917572
-3.52226734161377 -0.364367842674255
21.3943538665771 -14.4894933700562
-0.236092925071716 -22.2795295715332
1.01778447628021 -21.178337097168
15.8841199874878 -10.7361326217651
-18.1031589508057 21.0617866516113
1.60440039634705 -29.223783493042
7.17479848861694 4.41788911819458
-38.3494300842285 -32.5799827575684
-14.2009582519531 35.1869201660156
-35.4479713439941 20.2096500396729
18.3990783691406 -12.5203380584717
21.860595703125 -14.2911396026611
19.6324024200439 -7.84855604171753
0.328528881072998 37.6634483337402
32.9606132507324 34.8892822265625
18.2589550018311 -5.49035024642944
-5.72418880462646 17.2688312530518
11.5370712280273 28.9801959991455
22.5086326599121 -1.46245348453522
18.7738018035889 22.6173229217529
-2.29189682006836 37.7279624938965
-13.5970706939697 18.8171138763428
18.4545154571533 23.6435737609863
19.8679580688477 -15.0773000717163
-13.9288768768311 35.7465705871582
-33.8258361816406 21.5198059082031
-38.6821098327637 -31.2702159881592
28.9446182250977 -10.967809677124
22.7445793151855 -24.0324897766113
-8.66472244262695 28.3156547546387
-38.9124603271484 -20.9425868988037
12.1128730773926 26.4000816345215
-2.44220185279846 -0.360001683235168
-0.753510177135468 -28.2127418518066
15.6457014083862 -14.7164831161499
33.7763290405273 36.9955368041992
34.6789398193359 6.04151248931885
2.32701754570007 -20.7578544616699
22.4601364135742 -25.4094085693359
17.7545375823975 23.0221195220947
11.206690788269 29.3353614807129
12.8743915557861 -27.4268207550049
-4.09315586090088 28.5714454650879
10.9150276184082 27.2460594177246
-7.05097484588623 17.4182529449463
17.9099159240723 -4.79372215270996
0.0705780982971191 -12.3232097625732
-2.0857880115509 0.599402785301208
-34.1972351074219 20.7535018920898
5.87617635726929 40.8600997924805
-0.84306126832962 37.2920112609863
-37.2626953125 20.2296581268311
12.3974456787109 -26.3222122192383
28.2145729064941 -12.8264265060425
35.8679504394531 4.15086269378662
22.5145473480225 -25.2287406921387
-1.24850058555603 37.1772270202637
-0.61610746383667 37.1471328735352
-34.6359901428223 37.6633682250977
-34.9885025024414 21.6622085571289
-0.376245141029358 -12.5653610229492
-36.8817100524902 -31.1999282836914
-19.5973892211914 21.6029777526855
0.351269602775574 37.3659591674805
12.2976350784302 28.2523078918457
19.9460983276367 23.783712387085
-15.2462501525879 19.0511035919189
-4.08186149597168 11.8581218719482
-39.0721282958984 19.4049053192139
-5.67998313903809 12.1020698547363
19.6398448944092 -8.90198802947998
21.2642669677734 0.869394779205322
-0.00480671506375074 -28.1172695159912
18.5918483734131 -6.46193170547485
5.40594291687012 36.8221397399902
12.4018259048462 29.0079879760742
27.2057209014893 -36.1899681091309
-1.75687026977539 38.226448059082
23.4758529663086 -15.1786117553711
22.4966468811035 -25.6867351531982
21.5111389160156 22.6829452514648
-9.30481910705566 25.5611000061035
10.326322555542 28.7370090484619
25.6739177703857 -26.402853012085
19.3401870727539 24.2213764190674
25.0571365356445 18.9446849822998
11.3136806488037 -27.3373012542725
-5.79295921325684 18.3865871429443
22.679594039917 1.01662027835846
29.3430004119873 -11.3113460540771
-0.482930839061737 -29.3374710083008
1.48512721061707 -21.9250087738037
10.6642351150513 37.4526596069336
21.7144336700439 -16.019495010376
-9.91117477416992 27.9135036468506
26.8326854705811 -38.1075325012207
-1.39006304740906 37.8499755859375
23.1376171112061 -25.2102069854736
33.3542175292969 37.6101760864258
-0.331176280975342 -22.5038909912109
38.333324432373 6.7429051399231
25.5208187103271 -25.4768047332764
19.4229698181152 21.8610877990723
-4.42475891113281 1.32585895061493
32.2744140625 35.0723915100098
23.0597743988037 0.075136810541153
21.1178855895996 -1.77801525592804
-39.2315826416016 -21.4192676544189
21.3821678161621 -24.5004196166992
-15.1146116256714 18.0985469818115
7.50244998931885 39.0031585693359
25.957540512085 -25.7402477264404
-21.1549053192139 20.2293853759766
11.110279083252 28.9039402008057
-2.90473413467407 29.0344371795654
25.8905601501465 -36.4671478271484
-32.706371307373 38.0568580627441
18.9117851257324 21.2547607421875
26.7278099060059 -27.0264358520508
33.7969245910645 6.25209188461304
11.3661165237427 27.8010845184326
-2.73651647567749 30.1242008209229
15.156023979187 -12.5717182159424
6.63617658615112 36.8762626647949
-15.1188955307007 35.6729049682617
-32.6869277954102 37.8340950012207
2.64176535606384 -13.5977172851562
35.3990859985352 6.84292840957642
-36.0313911437988 21.0078525543213
25.3745784759521 19.1815090179443
-6.09797859191895 11.2918100357056
-3.21108627319336 30.2900066375732
35.8969879150391 -12.3731679916382
19.2894840240479 -8.07829284667969
11.9610357284546 28.7576580047607
-7.01196193695068 19.2883319854736
-9.80844783782959 27.7419757843018
11.8789167404175 37.8615570068359
1.83417928218842 -28.3589057922363
-2.61208486557007 37.2106094360352
-1.89444613456726 -28.1206569671631
28.4447288513184 -29.9852600097656
0.240830272436142 -20.6164112091064
34.1049461364746 34.8623313903809
13.6341714859009 -25.0281925201416
-37.220386505127 -33.2457847595215
19.42893409729 -4.19586849212646
-2.54818725585938 0.290304183959961
-34.4240989685059 36.3588829040527
28.4187335968018 -12.1545848846436
11.0702056884766 29.6319332122803
36.3419342041016 7.12661409378052
23.7095241546631 18.3063163757324
28.3702735900879 -12.5978584289551
-19.2966423034668 20.9288349151611
-0.536910176277161 -27.9111194610596
21.2973594665527 -15.0470294952393
-4.40266370773315 11.1798610687256
12.0919809341431 35.75830078125
7.27769088745117 37.324104309082
-15.3065624237061 17.4455013275146
19.1043853759766 -12.9252958297729
-1.63249135017395 26.9618911743164
-6.12227916717529 12.4810581207275
23.1754131317139 -27.2927093505859
-20.5627861022949 19.5664253234863
-17.709436416626 23.0857677459717
16.0914611816406 -12.4098300933838
0.00290831667371094 -28.6047115325928
8.37211990356445 39.8257598876953
-1.09411799907684 2.91749477386475
33.131046295166 36.9631767272949
0.794488608837128 -13.9228839874268
0.849543154239655 -30.0418567657471
-0.42633455991745 38.7226524353027
-18.4913539886475 20.7048759460449
7.19150066375732 3.37637376785278
-39.7212829589844 -33.2942924499512
-35.4403953552246 22.427267074585
24.6153907775879 -25.6508159637451
20.6970672607422 -15.8578262329102
25.427360534668 -16.8718605041504
0.0966434478759766 35.8087196350098
11.1214818954468 28.9805450439453
15.7013626098633 -11.8450603485107
20.8280639648438 21.7072525024414
28.1802253723145 -26.8661651611328
33.5942420959473 35.5221214294434
-0.758064985275269 37.1829109191895
19.0609245300293 -6.74263572692871
22.3260746002197 -24.4986972808838
-16.3376312255859 18.8261585235596
-0.513567566871643 -12.6035146713257
28.3693103790283 -9.56199836730957
-38.4140930175781 -22.4530487060547
-17.106819152832 22.796350479126
-37.5788497924805 18.9770069122314
12.2036056518555 -26.3157653808594
-4.42028522491455 11.1168203353882
-7.03706741333008 28.4716777801514
20.5111560821533 -24.6298637390137
22.7968463897705 18.2691650390625
34.563175201416 -13.5894241333008
23.0224609375 -25.6702575683594
-16.5607013702393 18.717212677002
28.4817905426025 -12.7329607009888
12.9950313568115 -12.4369354248047
-7.48116874694824 28.6011333465576
-3.42171907424927 7.58687782287598
15.2390422821045 -8.97775077819824
-9.70709800720215 25.8693561553955
-3.57116794586182 0.902844905853271
13.3759126663208 -27.4538726806641
21.0022735595703 -2.77176332473755
0.531995952129364 -21.8271789550781
-38.2082939147949 -22.3093147277832
-39.3147621154785 -20.7852420806885
4.49455261230469 38.7995529174805
-3.35292553901672 30.3388404846191
-8.75115013122559 18.864221572876
19.0186347961426 -5.73554706573486
20.5566654205322 -1.07557916641235
17.2279834747314 -11.2662086486816
0.63383150100708 1.19319653511047
24.1059398651123 -25.649055480957
21.930757522583 -15.3809413909912
24.184907913208 -24.8172779083252
34.8563575744629 -12.2655467987061
-1.63666880130768 36.7947311401367
-1.25916159152985 0.707646250724792
-21.7382793426514 20.3532562255859
-37.4847106933594 18.6152477264404
-0.525182247161865 -22.7587432861328
11.6714153289795 -26.4845218658447
1.29914093017578 -21.5892181396484
-0.849665224552155 39.5961380004883
-4.11863660812378 11.6627912521362
-38.9337844848633 -22.0403995513916
-5.56687259674072 11.2135925292969
-3.75028133392334 8.26549053192139
37.0720024108887 -12.1860322952271
34.399242401123 -12.6563291549683
7.75481224060059 4.73661231994629
27.0318717956543 -12.9276342391968
-21.6988391876221 22.8972511291504
29.4162750244141 -11.686806678772
-2.98165369033813 1.37184548377991
-3.25191640853882 0.84375387430191
35.7404289245605 -12.9955997467041
25.0421104431152 -25.9214019775391
33.1343421936035 35.132495880127
-3.3873450756073 31.1851806640625
16.8055572509766 -11.4491930007935
-1.73158264160156 37.1668701171875
-18.3600273132324 21.9259128570557
2.07302308082581 -13.1420240402222
25.8411464691162 -27.0773658752441
-2.78960800170898 30.39821434021
-4.46151161193848 31.0471572875977
19.470142364502 22.5456352233887
1.66836428642273 -11.2420787811279
12.1832580566406 28.3343772888184
29.7871036529541 -13.0433320999146
-2.89998197555542 1.87119495868683
24.4945545196533 20.2002582550049
-37.6024017333984 -20.4234199523926
23.8903884887695 -26.6185302734375
-10.013876914978 26.8178234100342
-32.7792739868164 39.9430885314941
-38.0494079589844 20.2378463745117
26.467845916748 -28.3831634521484
-10.1375665664673 28.428674697876
-1.8664984703064 39.9150199890137
-13.0766611099243 36.7087478637695
7.5108585357666 3.30121493339539
-5.56481409072876 13.2686100006104
-2.18527579307556 1.01956081390381
-8.23668479919434 16.9481792449951
-41.1590156555176 -23.1932983398438
-31.5865039825439 38.6888236999512
22.6335639953613 -16.1288681030273
18.8423156738281 24.5562877655029
20.3206729888916 -6.43290615081787
11.224705696106 -28.2761287689209
28.5515460968018 -12.750433921814
34.2973709106445 -12.9697484970093
20.4556159973145 -9.20120525360107
-38.5804634094238 -32.450325012207
22.2207336425781 -16.3412628173828
34.7105941772461 5.11944770812988
2.89269471168518 -12.7371788024902
6.84624242782593 4.93710803985596
-18.152515411377 21.9949836730957
14.7598247528076 -12.2420711517334
22.81667137146 -13.0893526077271
22.6115188598633 -25.4690742492676
5.6041088104248 39.4851913452148
22.9890727996826 -1.06177377700806
0.133580327033997 -22.9086532592773
-17.4915885925293 20.2032775878906
11.897141456604 27.945837020874
5.98335123062134 39.4576034545898
18.8096523284912 23.8886756896973
10.9779920578003 38.4985198974609
-16.7785739898682 36.8891525268555
23.5375061035156 0.410417944192886
-1.73781490325928 30.3709030151367
2.06029272079468 -19.6840953826904
-15.8587656021118 16.4487190246582
25.8413543701172 -24.8685493469238
26.5827980041504 -38.8446159362793
7.18345737457275 40.8527069091797
-32.7337036132812 39.1463470458984
34.9129867553711 -13.7452297210693
26.8555068969727 -37.3183898925781
-4.83942699432373 2.96434688568115
-34.5971755981445 20.0172176361084
27.2191600799561 -27.4151229858398
-5.69386863708496 10.3040008544922
11.9136829376221 -25.721658706665
12.5717916488647 28.7836589813232
-19.4443035125732 21.9425849914551
-10.4353761672974 26.5451030731201
18.170238494873 20.768985748291
-36.1050071716309 21.393871307373
-18.2336578369141 21.6818561553955
-38.2634010314941 -31.9224948883057
-38.524829864502 -31.457088470459
24.0118236541748 -16.0976371765137
6.63515281677246 4.03625869750977
-15.2477474212646 38.1422691345215
-20.5776309967041 19.9645023345947
-33.6938591003418 20.8656063079834
-35.7927894592285 19.0694046020508
19.3078117370605 -5.78591918945312
15.0854215621948 -11.6574735641479
-38.4849433898926 -31.3226566314697
24.9201354980469 -37.0410537719727
1.87852668762207 -12.6678771972656
26.1682415008545 -28.3826961517334
11.7274875640869 29.7278480529785
27.1632251739502 -10.197114944458
13.2492580413818 35.8017044067383
-38.4674797058105 -20.9041957855225
18.202543258667 23.9538612365723
13.3594951629639 -11.9620971679688
18.5793151855469 -8.54085540771484
-6.17067050933838 11.9480485916138
21.8352241516113 -14.4534645080566
-38.901538848877 -21.7370853424072
-8.55771732330322 18.9489517211914
8.02013874053955 3.22912096977234
21.4090614318848 -24.8576583862305
33.8517646789551 35.4412612915039
-14.2113122940063 36.7427787780762
-36.3272323608398 22.085391998291
5.66744899749756 2.81903910636902
20.1925716400146 -1.72801673412323
0.551484704017639 -21.2228412628174
18.4062747955322 -13.8305225372314
35.9131774902344 7.0400505065918
35.6769409179688 -12.9321842193604
-36.6883087158203 18.4277114868164
-3.15231609344482 37.2009582519531
-31.0607299804688 36.8864784240723
13.4105186462402 35.9659767150879
11.6248512268066 36.3117599487305
-2.59564781188965 30.3163814544678
20.2370548248291 -12.4889030456543
34.4469413757324 -12.4874038696289
3.44483160972595 -13.2948608398438
-18.9218120574951 21.179313659668
16.6518096923828 -5.62921524047852
-3.78187251091003 30.6965065002441
21.6923561096191 -26.4589767456055
-2.2779438495636 -28.8908405303955
27.7259464263916 -26.3934383392334
10.5397825241089 40.2050247192383
32.7736892700195 36.1150054931641
11.7971868515015 -24.5711765289307
36.3111305236816 -13.9950828552246
37.126277923584 -13.1177349090576
6.49422550201416 3.21701002120972
-37.5370979309082 20.0698432922363
-39.3301734924316 -33.8899803161621
-21.9900856018066 19.7539615631104
11.6883039474487 37.3982200622559
-38.306037902832 20.298770904541
18.5240592956543 23.575159072876
22.3994293212891 -25.4214477539062
23.5530261993408 -15.4135961532593
18.3863296508789 -9.15808486938477
21.3534889221191 0.566593050956726
-38.099681854248 -31.4148120880127
28.3352146148682 -25.5920886993408
0.104570031166077 36.4737091064453
12.3828353881836 28.2603054046631
-16.8627700805664 18.0734672546387
-36.5959091186523 -32.666446685791
6.68087959289551 38.5510749816895
14.3588743209839 -12.5259056091309
-22.8201560974121 18.3994121551514
-32.727294921875 36.057918548584
5.40578317642212 39.1447830200195
-20.9647598266602 18.3391189575195
-2.66875982284546 30.2333850860596
19.4802856445312 21.4653339385986
11.8755159378052 27.2617607116699
32.7761192321777 36.1707458496094
17.8737010955811 -9.47316360473633
36.5510368347168 -11.46741771698
21.3867874145508 -25.9772033691406
35.5183067321777 6.00743579864502
-19.217472076416 20.8196487426758
15.1734771728516 -12.3053283691406
0.392568469047546 -20.318510055542
-16.5335350036621 16.6971187591553
5.62158012390137 40.1476173400879
-34.401252746582 21.6922416687012
25.2147178649902 -37.5467300415039
-5.77009725570679 11.6226196289062
-2.75886797904968 0.694827318191528
25.2098922729492 -27.6477127075195
-7.94035148620605 17.1555023193359
20.6490840911865 21.7905826568604
-18.3476257324219 22.2053356170654
0.279663264751434 -12.3272256851196
24.958984375 -22.9150123596191
1.32388854026794 -27.1932373046875
19.1822891235352 -8.0634241104126
-0.294721871614456 -29.9641513824463
-32.4478530883789 39.8619689941406
5.09735679626465 4.89598941802979
-2.73069715499878 39.4425582885742
-38.4564247131348 -32.3041152954102
-5.14819622039795 17.282205581665
-36.0957069396973 20.3291397094727
-15.9119701385498 36.0233001708984
20.8578948974609 24.8898296356201
23.8240203857422 -25.858528137207
-38.8637504577637 -20.4712104797363
20.5162696838379 -13.7374076843262
-19.2852363586426 21.4968318939209
-38.6639709472656 18.5590438842773
21.1444225311279 0.570321202278137
-33.5482521057129 37.3608703613281
-17.0273475646973 20.5074005126953
36.6674003601074 5.1371488571167
18.7001323699951 -14.0548038482666
-6.03510665893555 17.0262775421143
-3.79267287254333 28.9307861328125
-39.7496871948242 -22.3490104675293
0.527875304222107 -29.51100730896
18.5020313262939 -12.8988447189331
-7.72898769378662 20.1525440216064
11.5548000335693 27.7043151855469
-4.73340797424316 30.4946365356445
20.8181934356689 20.5012836456299
10.2667751312256 28.9003963470459
-39.8254737854004 19.9685382843018
6.66706037521362 4.79937028884888
0.825374484062195 -27.6993465423584
-39.5637512207031 -32.842658996582
34.6856346130371 7.07346820831299
-37.5525550842285 -21.4495620727539
-34.7907981872559 21.6599521636963
20.5629272460938 23.3130512237549
0.41374683380127 37.8249130249023
20.6890716552734 -7.8690071105957
-6.27894878387451 18.9991397857666
-38.79931640625 -31.8928642272949
6.2560338973999 3.22400116920471
-2.97957372665405 28.7173252105713
-3.75513696670532 29.0853576660156
25.3631458282471 -26.0224361419678
-5.59319353103638 11.8204669952393
18.4911136627197 21.0160827636719
-14.8106622695923 34.649528503418
-2.81022071838379 38.3153686523438
27.6335792541504 -27.6659870147705
-2.53297305107117 -0.583075642585754
32.9585876464844 36.9250221252441
-38.5644302368164 -22.7470283508301
13.437162399292 -26.9308643341064
12.0125694274902 28.2760143280029
23.3121929168701 -26.1361560821533
-8.31341075897217 19.5007972717285
-34.2921600341797 22.1520442962646
5.41424131393433 39.5901145935059
-38.7294807434082 20.3122501373291
6.20787525177002 39.1407814025879
19.5765647888184 -8.04382038116455
-20.2943363189697 21.2870254516602
14.1363153457642 -26.2253913879395
-6.830970287323 11.9090003967285
11.1229934692383 37.5998039245605
-34.650016784668 21.513313293457
22.8801116943359 -26.2405471801758
-3.4670033454895 11.5088710784912
32.8626556396484 37.9999237060547
13.1900262832642 -26.8693695068359
2.29625582695007 -22.0636825561523
-39.2376823425293 20.8437538146973
24.8730030059814 17.5159931182861
4.64883279800415 36.1073226928711
5.8743782043457 38.7179985046387
20.1370372772217 -15.0729913711548
23.2122573852539 -23.7359027862549
-37.712287902832 -32.4089736938477
-39.2602691650391 -22.3482818603516
-40.0140342712402 -31.24853515625
4.60084629058838 39.3148155212402
4.22624683380127 37.824893951416
32.1568298339844 37.1620254516602
-17.9485511779785 17.3592109680176
-32.4407730102539 38.425708770752
-3.1921398639679 1.0022087097168
21.940990447998 -2.05130171775818
-41.2161483764648 -22.469841003418
35.762767791748 -13.8851337432861
-4.66763210296631 31.6727390289307
-3.58383178710938 2.90184783935547
-2.92208051681519 30.2033882141113
21.1940536499023 0.550013661384583
-21.1242504119873 19.2933044433594
11.4012289047241 28.7130355834961
-38.5524024963379 -32.1188087463379
-33.4741630554199 37.7674522399902
-16.4302730560303 21.3020782470703
19.0822486877441 22.0430088043213
-12.3773498535156 29.0825424194336
-8.32909107208252 27.9894485473633
-23.6079254150391 19.0978889465332
-6.91330146789551 18.2170124053955
16.4159164428711 -12.0555877685547
29.6301574707031 -25.3612937927246
34.6484603881836 -12.3418121337891
27.4490032196045 -38.1274070739746
-18.5379619598389 21.3573837280273
1.25499892234802 -22.8281784057617
26.1384716033936 17.2661552429199
23.1391105651855 -25.9805755615234
13.7365636825562 -25.3945045471191
19.7673587799072 -14.5325736999512
-6.08162593841553 19.41233253479
19.4906616210938 -5.09058475494385
-1.8198618888855 37.7038192749023
2.40756797790527 -12.0279817581177
32.1689071655273 37.0222930908203
-33.7167892456055 38.7558212280273
-15.5553636550903 17.3988628387451
11.381049156189 36.2656326293945
-10.9413909912109 27.3145332336426
-0.0963940098881721 -28.0762958526611
33.153392791748 35.6015243530273
17.3944644927979 -12.2305250167847
11.5799341201782 35.3177680969238
-22.6793518066406 20.6204776763916
-14.5362968444824 35.6552886962891
35.6434669494629 6.80803108215332
27.0619640350342 -37.7433090209961
-19.4919776916504 20.7911243438721
-37.0082855224609 18.6715793609619
34.0766105651855 36.794075012207
0.550203382968903 -13.2568254470825
27.8667945861816 -27.0253009796143
21.9904441833496 -0.430710166692734
-30.9902038574219 37.2015991210938
8.34641456604004 6.20705890655518
-37.390308380127 -30.4892024993896
-38.0136528015137 -31.8830051422119
-13.5911931991577 17.7301788330078
-12.5937051773071 35.7774963378906
35.3405876159668 -12.8980474472046
-33.2896842956543 39.0383567810059
35.5193328857422 5.88568544387817
0.720468103885651 -29.1663150787354
-16.3133888244629 18.655481338501
6.20021724700928 3.62328600883484
21.4003810882568 -2.99129271507263
-35.2308883666992 21.0465507507324
14.5931940078735 -12.5378408432007
18.0797004699707 21.8984413146973
20.238452911377 -6.44057369232178
-18.7627944946289 20.9589252471924
19.3946018218994 -7.40510654449463
22.6298561096191 -25.5419406890869
-2.49119663238525 28.3755989074707
14.8457565307617 -11.9272241592407
-39.8043937683105 -22.349573135376
21.7957649230957 24.9985237121582
15.9180402755737 -11.6810913085938
13.0179738998413 36.1925964355469
17.1333904266357 -5.81504440307617
11.291145324707 -24.6566410064697
15.6808013916016 -11.9486627578735
-10.3103227615356 28.9525527954102
28.6598262786865 -13.0648603439331
35.8172340393066 6.45469617843628
15.0032920837402 -12.7124252319336
24.1628761291504 18.9855155944824
-38.8847579956055 18.7385921478271
12.3066110610962 -25.4395580291748
11.9593086242676 37.9051704406738
-0.0638778209686279 38.4396781921387
16.9787101745605 -5.19808864593506
23.9296894073486 -24.8363208770752
12.5721473693848 -25.3819351196289
18.2018032073975 -6.2507438659668
5.82138252258301 3.91453289985657
-1.72476029396057 38.6689949035645
19.80446434021 22.3508815765381
-33.6588821411133 36.3694877624512
-22.5345897674561 18.6636829376221
21.2833843231201 23.7393093109131
34.8012237548828 37.2571449279785
16.3184547424316 -5.12305736541748
-6.59301614761353 9.82795143127441
22.2240200042725 -14.0225353240967
6.43249416351318 5.05197286605835
26.3063507080078 -26.7696189880371
24.451192855835 18.0598011016846
11.0715866088867 28.9179935455322
-2.93914365768433 31.473690032959
-15.6720304489136 19.5003147125244
21.5670776367188 -25.9458923339844
23.794942855835 -26.9378280639648
15.5877656936646 -11.1342630386353
20.393705368042 -13.5319833755493
20.7492370605469 -1.51716446876526
-17.5381546020508 21.9378967285156
-0.649878740310669 -28.8046836853027
-17.9836235046387 19.7232513427734
8.09818744659424 38.7675361633301
6.67160606384277 3.01117134094238
-39.7720108032227 -22.0796451568604
-18.1981773376465 21.5243091583252
-37.8564224243164 -30.3867053985596
22.4175872802734 -1.36380469799042
31.800443649292 35.5280532836914
11.4230709075928 27.0416698455811
-38.6061897277832 -23.1692810058594
34.2527389526367 37.0408973693848
6.39059543609619 39.3417663574219
33.3171844482422 35.3901519775391
-39.6787796020508 -22.2669639587402
22.3972434997559 -15.3220129013062
0.493778795003891 -27.9747142791748
21.501350402832 0.280219167470932
-35.1818618774414 21.976634979248
-6.06888628005981 17.5325546264648
-19.9936580657959 20.7154884338379
11.0686407089233 38.759822845459
-5.53023147583008 12.1615896224976
35.1756401062012 36.3426208496094
12.6726226806641 -25.3432579040527
36.1994819641113 5.3385534286499
10.5788106918335 37.5952072143555
-35.7169799804688 21.4706535339355
20.8483867645264 -12.5767974853516
-2.70410585403442 10.6581974029541
24.1701946258545 -24.9606590270996
24.7902736663818 -38.1768836975098
-16.202299118042 18.8459587097168
-34.9345817565918 20.1778450012207
10.7529487609863 29.5938911437988
28.5015182495117 -14.3638181686401
-14.4442949295044 17.4909934997559
22.974781036377 -25.2422046661377
-1.14280164241791 -28.9084587097168
22.9960632324219 -25.7846622467041
6.20519781112671 37.1751251220703
-3.27402019500732 1.49085485935211
24.0908908843994 -26.5948925018311
6.13454103469849 40.4526443481445
-22.286735534668 20.1567249298096
25.4571857452393 17.4967861175537
20.1218013763428 -12.6769237518311
-1.01549196243286 -27.9395408630371
26.2062091827393 -36.3856010437012
16.3158798217773 -5.11746740341187
35.9018440246582 6.90819597244263
22.7130126953125 -13.8640432357788
26.6266784667969 -34.263599395752
-0.0293683409690857 -22.7799587249756
7.88195753097534 37.3541450500488
0.894894003868103 -11.1772775650024
17.7285690307617 -5.42898893356323
16.5745582580566 -12.4247560501099
12.0852651596069 28.1167259216309
15.0936851501465 -12.1556606292725
19.4424915313721 24.6899909973145
-5.31417798995972 10.5206279754639
-1.94622802734375 0.944482147693634
-38.7752342224121 -31.7979984283447
22.0413818359375 2.19542932510376
22.5914115905762 -25.8208465576172
6.45223951339722 41.8805122375488
19.0976829528809 -13.130558013916
9.85436916351318 28.8517894744873
0.0605463683605194 -29.2226257324219
-0.616012811660767 -20.8068962097168
12.2538614273071 -26.8175563812256
24.7105102539062 -25.372953414917
-39.2194786071777 20.0391120910645
22.6053447723389 -14.1705932617188
28.5561103820801 -12.4456424713135
-14.2225313186646 34.3928604125977
-7.10547208786011 17.658561706543
-0.100330948829651 36.0817832946777
-2.45436501502991 1.20011603832245
19.1372585296631 -11.1412744522095
35.5071220397949 5.03789091110229
16.9439010620117 -6.17492198944092
29.9809093475342 -11.598105430603
1.17407333850861 -12.1194581985474
-5.95443248748779 17.516134262085
-10.039023399353 27.6348915100098
21.4518604278564 -24.1023712158203
6.50006484985352 39.0120429992676
28.5372829437256 -11.9232177734375
20.390266418457 -12.0203399658203
26.3269424438477 -24.9390678405762
19.1813297271729 -5.77590036392212
21.4379291534424 0.04250368475914
24.3486938476562 19.5052719116211
10.9602766036987 37.6027069091797
1.36987125873566 -21.742582321167
19.1952247619629 23.361572265625
-14.5717439651489 36.4828224182129
-3.14618802070618 -30.8532066345215
-12.5555086135864 37.5193634033203
27.3116836547852 -12.9232587814331
18.4703750610352 -4.96162080764771
-1.54403066635132 39.8803024291992
10.7522478103638 36.0013961791992
-17.4186954498291 21.7140769958496
26.1428451538086 -34.6367835998535
0.96499490737915 -12.9237365722656
22.2555389404297 -24.9913444519043
11.4723806381226 27.4564437866211
-0.420944213867188 1.53106641769409
-8.61705875396729 25.7228050231934
19.6218204498291 -13.5815687179565
0.782624244689941 -28.3450546264648
0.744714260101318 -20.7106418609619
-18.7351493835449 24.3846130371094
-17.8515625 21.800329208374
-6.28335189819336 16.7983570098877
-38.4486846923828 19.2831649780273
12.8493185043335 -27.6924457550049
19.0672645568848 -8.3289794921875
35.7776145935059 7.69891166687012
22.0763854980469 -0.441218793392181
-37.365852355957 -32.7566719055176
22.3154850006104 23.8656234741211
-21.2311382293701 19.9513244628906
23.7988567352295 -24.1050224304199
19.4616966247559 23.5650596618652
-38.868896484375 -22.6705684661865
15.8813714981079 -11.8283538818359
0.661926209926605 -29.8986415863037
23.0925273895264 -2.87815999984741
-21.9885139465332 20.8943290710449
-20.0784244537354 21.6543579101562
32.1876678466797 35.0653915405273
11.1045274734497 36.6924667358398
24.7274341583252 18.4144554138184
11.2434577941895 38.5112266540527
17.1365451812744 -6.90943622589111
35.1607933044434 5.14574289321899
23.2001876831055 -25.0315456390381
22.5081062316895 -16.1836013793945
11.4135751724243 -26.2069931030273
-16.3488006591797 22.2264976501465
16.1356353759766 -12.2093601226807
5.49622058868408 4.14756727218628
21.8021011352539 -13.9822130203247
-33.0917358398438 38.8676109313965
-8.92596626281738 28.5943775177002
32.3541030883789 34.913932800293
25.0772380828857 -25.2107391357422
-21.6052932739258 20.7274570465088
28.9699440002441 -10.9662752151489
25.0097694396973 19.0907764434814
-40.2317848205566 -23.2734222412109
-38.4136199951172 20.5273723602295
35.4495315551758 6.17470598220825
-38.565128326416 19.3210849761963
2.42969846725464 -13.1726741790771
27.5993347167969 -27.8957138061523
2.62043762207031 -12.6250705718994
19.7842864990234 -6.93115615844727
22.3387813568115 -1.4732164144516
36.0014190673828 -11.6079025268555
23.9748077392578 -25.8063087463379
-32.7811508178711 37.7457046508789
2.36025333404541 -12.6995887756348
12.9622583389282 -24.2765064239502
9.90899181365967 -27.2002754211426
-17.1414031982422 19.4698925018311
11.3023548126221 37.959228515625
-1.93978476524353 39.7674522399902
-19.069299697876 21.2615413665771
0.508520066738129 -11.2776470184326
-15.8933372497559 17.9828968048096
1.93239545822144 -13.0686883926392
2.14222240447998 -11.9559030532837
-37.3401679992676 -31.1193428039551
-31.7936210632324 37.3552322387695
};


==> figures/visualizations/gmm40/gt_samples.tex <==
\addplot [semithick, red, opacity=0.5, mark=*, mark size=3, mark options={solid}, only marks]
table {%
17.4416313171387 -5.40016555786133
0.40688493847847 -27.4275493621826
1.52752804756165 -11.9982976913452
7.02853298187256 2.73487901687622
17.8423309326172 22.3049736022949
24.6525287628174 -23.8590641021729
-23.3187198638916 17.8477516174316
-37.4694976806641 19.4755725860596
-13.4167890548706 34.8238334655762
35.4178619384766 -11.0546283721924
-38.5880012512207 -22.3803024291992
26.5014362335205 -36.0532569885254
-0.274681091308594 -19.963659286499
-9.84927558898926 28.4097061157227
-32.7083473205566 38.6875762939453
-39.1037368774414 21.0624389648438
-38.5078277587891 -31.3569355010986
34.6926460266113 4.99514722824097
5.88764619827271 38.6732215881348
-13.1164073944092 35.9514808654785
26.658899307251 -39.2044448852539
22.5992012023926 0.20674592256546
-13.9639091491699 35.9945182800293
-5.48520183563232 31.0881404876709
18.2174034118652 -6.05398035049438
-3.7510814666748 1.03371870517731
18.9547920227051 23.8145999908447
18.1736335754395 -5.92514181137085
15.3769407272339 -13.3931045532227
-6.60268688201904 30.0559101104736
-9.48730945587158 29.181770324707
12.79234790802 -25.7050628662109
22.2104797363281 -1.9405837059021
-13.7620220184326 18.8172092437744
25.4920463562012 -37.7857131958008
-0.591497898101807 -11.7324676513672
21.7200393676758 20.836576461792
35.0873641967773 6.40311717987061
20.1387023925781 19.4154586791992
-2.54940295219421 -0.559081435203552
29.7484912872314 -13.3304262161255
-36.1567039489746 -31.4735565185547
21.5058288574219 -1.66556918621063
-21.8659496307373 17.7253284454346
-1.17106008529663 -11.4146785736084
15.7761869430542 -5.54564380645752
-36.3322677612305 21.1097373962402
15.4426155090332 -10.9641618728638
18.5994052886963 -7.35100936889648
25.1637916564941 -35.9730339050293
20.0492286682129 22.610912322998
-39.125560760498 -21.8003482818604
-16.9700660705566 21.8165473937988
-20.9477920532227 18.9212589263916
10.9610261917114 28.2753028869629
-8.15726566314697 17.453821182251
-3.13075566291809 30.2323246002197
16.4219264984131 -10.7142581939697
37.0201606750488 5.55447292327881
-15.6708841323853 36.0030097961426
-6.30459547042847 13.3104276657104
29.5448722839355 -12.0740737915039
-0.368779450654984 -29.5710411071777
-33.033260345459 37.1547775268555
-2.91473913192749 0.407055377960205
0.717839360237122 -21.3670597076416
-17.0664310455322 18.7015323638916
-2.22963809967041 1.18611526489258
19.0241584777832 -12.3298091888428
28.5055541992188 -12.5747737884521
6.31667852401733 39.4780006408691
1.08388710021973 -12.7239227294922
19.8681526184082 -15.7542476654053
19.813756942749 -5.00542736053467
34.4755325317383 6.87308645248413
12.0895919799805 -25.9865818023682
-37.9191703796387 -21.0740833282471
18.6249198913574 -7.92518043518066
27.8087310791016 -12.8954124450684
-2.78741335868835 37.6681213378906
1.67521667480469 -11.4310121536255
34.0896530151367 5.02061700820923
19.3979625701904 -7.95353317260742
32.3068084716797 35.4272193908691
29.7120685577393 -12.4067335128784
7.89822483062744 3.70939135551453
5.82412624359131 38.1366729736328
32.8788757324219 35.7726440429688
-9.55975723266602 26.6891345977783
10.8720684051514 28.7147808074951
20.6971225738525 -0.434423416852951
33.7156028747559 4.14398765563965
-14.2964735031128 37.3585815429688
19.0480098724365 -8.61236763000488
-16.3694705963135 18.4319038391113
-14.9401054382324 35.0891418457031
28.715841293335 -12.7056159973145
21.2659492492676 -24.098424911499
-7.48646068572998 15.6560344696045
33.8025894165039 4.74652576446533
-32.8915672302246 36.6254081726074
-33.5985450744629 36.706226348877
13.2760591506958 -25.2881717681885
-0.0688240528106689 38.0998916625977
21.4104766845703 -26.5283012390137
-38.2527160644531 19.1247291564941
19.9794902801514 26.0628929138184
24.2172832489014 17.2378940582275
24.8533935546875 18.6758670806885
-2.72607803344727 37.6403160095215
19.889123916626 -13.5618896484375
22.0390815734863 0.261900305747986
32.234001159668 36.6748352050781
33.3030548095703 35.3340835571289
-2.01802968978882 37.8640098571777
-17.4615688323975 18.1250476837158
37.1044921875 -11.7732992172241
36.9305648803711 -12.6723680496216
20.1447334289551 20.318489074707
22.2422733306885 -26.5148067474365
19.6188659667969 -9.47342395782471
19.4995536804199 24.870584487915
21.7917461395264 0.712274432182312
20.805965423584 22.3356018066406
-1.87547397613525 37.5528182983398
27.7260417938232 -28.229700088501
-16.3926486968994 21.4066123962402
-38.4747924804688 -31.6842174530029
-9.12650680541992 27.9534149169922
24.4435520172119 18.7288589477539
12.4154691696167 36.448616027832
-3.82082653045654 0.934516727924347
-2.19589042663574 37.2744979858398
-21.0618190765381 19.5632743835449
37.1904029846191 6.94338941574097
0.55105596780777 -20.3451995849609
-14.3605842590332 35.9147109985352
-18.7154197692871 22.073766708374
-0.348703622817993 -11.7292861938477
-0.538062989711761 38.0500869750977
-0.475903213024139 -29.1189479827881
-15.8465051651001 35.5646781921387
34.3927803039551 -12.6546545028687
-3.29785990715027 29.5119323730469
-33.9817848205566 24.1366310119629
25.3582801818848 -37.5186157226562
-15.2122755050659 35.2102394104004
-7.41253519058228 17.3177490234375
-4.21176624298096 2.57666802406311
19.2362747192383 -15.7695064544678
18.8754024505615 22.9882926940918
-17.8945426940918 21.5528373718262
-19.4066944122314 21.1275367736816
20.1952304840088 -8.63556671142578
-6.28445911407471 10.4517498016357
-4.11738872528076 30.4842739105225
21.0304851531982 0.0508639216423035
-4.98285388946533 11.7562532424927
17.5454425811768 -11.1085557937622
26.8305988311768 -36.7691307067871
13.0901384353638 -11.7847871780396
28.3511161804199 -13.3995218276978
19.9132041931152 -12.692964553833
-16.5793724060059 35.9087409973145
-4.81155157089233 32.1504173278809
-38.2891006469727 21.0644416809082
25.9385147094727 19.4026870727539
11.1182804107666 36.7051696777344
-9.31435680389404 19.222713470459
-16.9816589355469 21.506368637085
32.3625144958496 37.0724067687988
-3.9358983039856 29.2596817016602
-38.0863304138184 -32.3541946411133
-16.8069248199463 21.528148651123
19.6253280639648 -9.37731647491455
20.0656318664551 22.634220123291
6.73980236053467 39.9456939697266
28.2649707794189 -10.7264013290405
26.4645481109619 -25.7729415893555
-8.05515289306641 18.3441905975342
20.0934619903564 -11.5021190643311
11.8549537658691 30.3990306854248
37.4462432861328 7.32467699050903
-35.5009574890137 21.2445755004883
22.3239727020264 -14.6095409393311
28.0507354736328 -12.9825401306152
-1.53400838375092 1.06045532226562
17.7622489929199 -4.46932029724121
4.67282199859619 37.6234588623047
22.6327342987061 -25.0519466400146
0.638744115829468 -12.5203151702881
-17.3175601959229 22.7604389190674
-21.3770160675049 19.8157634735107
21.2078037261963 -13.6851778030396
-0.724025130271912 -27.4533309936523
-2.13858222961426 0.730188846588135
-35.9936866760254 20.4683094024658
10.4337062835693 35.6321220397949
33.2208099365234 36.892635345459
-10.031909942627 27.9040145874023
22.8342151641846 17.6129856109619
0.35923844575882 -22.4287796020508
-7.81874561309814 17.2376079559326
12.598388671875 -26.9113788604736
18.8295726776123 21.5339603424072
12.1392669677734 -25.6186542510986
-14.660457611084 35.0367622375488
7.10675191879272 5.2803201675415
-19.9951877593994 19.4985504150391
5.45591115951538 3.36930584907532
0.66625040769577 -21.0613441467285
27.3065280914307 -29.3166942596436
17.7500915527344 21.9405822753906
-6.52418231964111 12.5973253250122
11.8480844497681 37.988166809082
-37.2008895874023 23.3780689239502
12.6182947158813 -25.9831352233887
-37.714054107666 -33.0574226379395
4.62388324737549 39.4050178527832
11.8670120239258 28.635232925415
-4.08646249771118 28.9247589111328
-39.0636215209961 -32.081127166748
-38.7515716552734 -31.7945041656494
18.2340278625488 -7.95453691482544
5.51035785675049 38.3288154602051
-1.70381903648376 38.1449432373047
-5.78678703308105 11.5416793823242
-3.14561986923218 1.24228870868683
33.8509292602539 35.2806434631348
-1.44876265525818 0.909848690032959
13.3486576080322 -26.5944957733154
14.8194942474365 -13.0374031066895
21.6609287261963 -11.8495492935181
-19.9812259674072 21.1606197357178
17.1753177642822 -6.94043636322021
21.7170104980469 -14.4727096557617
-21.3213939666748 20.1352634429932
21.0471382141113 24.1356658935547
23.7970714569092 -35.6477394104004
10.0445098876953 36.3880081176758
25.2164974212646 -24.5524291992188
-21.9785346984863 20.5720748901367
11.437029838562 29.2524566650391
22.7844696044922 -25.3298969268799
25.6209926605225 20.8344879150391
11.1047649383545 29.5535354614258
15.39208984375 -12.2425813674927
-37.985294342041 18.5833625793457
19.7510433197021 25.0964546203613
-7.14903259277344 29.3720512390137
11.4380168914795 35.4212837219238
16.1161060333252 -2.43584275245667
-2.58782744407654 0.164186418056488
34.3623046875 36.7933464050293
-14.5852870941162 16.7127151489258
-38.2257614135742 -22.4282894134521
12.1177453994751 -26.8896064758301
12.6006879806519 -26.2930583953857
34.1697540283203 37.3296356201172
0.662239789962769 -20.7228736877441
-16.247049331665 36.4385070800781
12.5902004241943 38.0501594543457
18.9471988677979 -8.27872753143311
-38.033260345459 19.6857662200928
34.3685989379883 7.63441276550293
35.7850875854492 7.82106876373291
19.2603397369385 21.3517932891846
36.1814117431641 -13.316554069519
20.8648662567139 21.4804744720459
-0.90089339017868 -27.072509765625
24.7764072418213 18.8142852783203
28.1315574645996 -12.4036235809326
20.5181789398193 21.7116870880127
35.3552856445312 5.70722246170044
20.4375495910645 -7.74258279800415
-12.3218002319336 36.6629867553711
35.1572151184082 -11.5199794769287
-7.31092023849487 18.6541595458984
-0.101944327354431 -22.3630504608154
-8.15069770812988 28.3628787994385
-38.7035980224609 18.2059803009033
-33.3212814331055 20.7486839294434
-9.28677272796631 17.9802951812744
-2.79848027229309 1.39493274688721
25.1907348632812 -36.5745506286621
2.60429692268372 -13.2858972549438
-38.6360816955566 -34.4923667907715
17.0879898071289 -12.0461883544922
11.5940551757812 30.0905876159668
-2.29816365242004 0.870231628417969
0.355280131101608 -29.8705158233643
34.5413818359375 36.2769584655762
34.2686576843262 37.2246398925781
5.36375617980957 37.8037872314453
1.50668323040009 -13.6582412719727
7.06724405288696 6.00739192962646
19.8875045776367 -12.4003877639771
-0.354531705379486 38.2413368225098
26.8758907318115 -26.5577983856201
6.10996723175049 37.6964912414551
22.4209270477295 -12.9644031524658
26.6648616790771 -24.6686134338379
19.8496150970459 -8.5434684753418
13.1239891052246 36.8101539611816
33.8067016601562 34.8104591369629
0.847117722034454 -20.7973442077637
2.16949462890625 -27.413215637207
26.4445819854736 19.9306564331055
19.3388633728027 21.2427921295166
14.4626922607422 -11.1755104064941
36.3593864440918 -13.7305688858032
0.0289326906204224 39.317985534668
-38.6731605529785 18.7331314086914
33.2946929931641 37.2976417541504
-14.5007381439209 36.3063926696777
24.9513244628906 18.2039012908936
0.941949784755707 -22.1275119781494
-15.8554124832153 19.5147304534912
-17.5328426361084 18.5089683532715
7.54308032989502 3.77730274200439
18.9195442199707 -8.14808464050293
25.3212051391602 -27.4196758270264
-0.658459305763245 1.71599876880646
27.8199043273926 -37.3008499145508
32.3372802734375 35.4301605224609
27.4057483673096 -25.9116344451904
-6.59575748443604 12.0459403991699
-3.11741352081299 29.9552536010742
36.239330291748 -13.4809122085571
12.5783557891846 37.7785034179688
10.3111429214478 29.0098133087158
33.8547210693359 6.4049277305603
-5.83285093307495 12.7776851654053
22.8391971588135 -25.5498542785645
-34.3385696411133 21.5812873840332
19.6812591552734 -9.84437942504883
18.3316612243652 -6.3069109916687
-9.65281009674072 28.3294868469238
2.31424570083618 -11.8549022674561
-37.6246910095215 -22.4327869415283
24.2691555023193 -14.6700706481934
-37.3924751281738 -33.5457878112793
24.7194194793701 -36.7101097106934
-3.71864175796509 11.6972055435181
-38.8278617858887 21.1284656524658
35.2118492126465 -12.8511829376221
14.1659231185913 -12.45982837677
20.1896667480469 20.8044700622559
-5.70342445373535 0.939868092536926
-21.70627784729 18.9368267059326
-3.49160170555115 29.266227722168
-0.976908564567566 37.2301788330078
19.1057300567627 23.4819107055664
-39.6249580383301 20.0185031890869
6.00025129318237 39.1892585754395
24.5144271850586 18.0189895629883
-3.88302516937256 11.9516458511353
11.8343114852905 -25.8046760559082
20.9260768890381 22.4640369415283
-37.8012771606445 21.1973991394043
-38.3576965332031 -32.6782341003418
8.58219337463379 4.34279584884644
20.4605255126953 21.3242835998535
1.24218654632568 -20.8372440338135
5.09860467910767 39.7389984130859
-38.6099662780762 19.1352653503418
-39.9647674560547 -30.7592506408691
27.6765403747559 -13.2463808059692
18.8977012634277 -13.063286781311
24.0395259857178 -26.1765747070312
0.0769136771559715 -29.2203330993652
27.7809944152832 -25.5697402954102
5.68177223205566 4.53243494033813
-2.15954494476318 1.60667908191681
22.6879940032959 -14.4665231704712
0.44143682718277 -13.1311235427856
-1.38150751590729 1.7106659412384
-6.53424739837646 13.077582359314
7.84093189239502 39.9642715454102
-2.9480996131897 29.893346786499
-38.3772468566895 -22.0695247650146
-3.21294355392456 30.1098022460938
-1.97882759571075 37.5008697509766
22.3490695953369 -13.6124572753906
-37.8201751708984 20.2234573364258
-40.0578002929688 -22.0903720855713
2.72436475753784 -28.2547721862793
31.3906421661377 36.1278457641602
28.5544624328613 -26.7712841033936
10.5924301147461 -25.7608528137207
-4.6307897567749 28.8557624816895
21.6772480010986 22.1767482757568
-1.76676917076111 38.6677436828613
19.5006694793701 23.9616031646729
22.2240409851074 -26.1511840820312
29.0091075897217 -14.5590772628784
24.8538131713867 -24.685375213623
-32.259651184082 39.0861053466797
17.7136421203613 24.1810684204102
13.4115772247314 -24.0306663513184
-32.6838264465332 38.2109222412109
-0.687233865261078 -29.0140399932861
16.338493347168 -11.2368516921997
36.0018119812012 -12.6755952835083
24.2852478027344 -36.1868362426758
6.85758066177368 4.60727739334106
-23.088134765625 19.1851043701172
35.2966156005859 -13.7601337432861
19.4071769714355 22.7276802062988
12.7618026733398 28.8874111175537
11.9932889938354 -26.415096282959
11.8334350585938 -26.6896572113037
7.30002403259277 37.9899253845215
-4.39973735809326 12.5074710845947
-17.3206195831299 23.2137279510498
-39.6911125183105 -21.6692562103271
18.8394737243652 -4.32965421676636
20.5623950958252 -14.1897611618042
10.8433637619019 29.2230548858643
22.3066139221191 -1.24102354049683
-2.49325561523438 29.7953090667725
32.5310897827148 35.5170669555664
-20.0639114379883 20.7466259002686
4.60727214813232 38.1452789306641
26.2776851654053 17.7178611755371
11.9185485839844 27.1213684082031
17.6778697967529 -5.97343397140503
18.6907215118408 -8.95591259002686
20.9411430358887 -13.2733516693115
10.7714185714722 38.3166007995605
-1.80680322647095 37.7135543823242
-15.0605125427246 36.3684158325195
21.0596961975098 -14.3797798156738
-13.9346904754639 35.1319618225098
0.902304530143738 -23.4590835571289
16.9419384002686 -5.20933437347412
-21.6194610595703 19.8553524017334
1.55132055282593 -10.971960067749
26.5454425811768 -38.3821830749512
24.0446128845215 18.470531463623
-0.590031981468201 38.4912147521973
-35.1341514587402 20.2102394104004
-31.4590873718262 39.8035697937012
23.0451889038086 -15.4305868148804
-3.79495143890381 30.4758701324463
23.4915046691895 -24.7810325622559
16.6045818328857 -4.57496881484985
0.148599535226822 -28.9209766387939
-5.71299314498901 19.6500415802002
-2.2845242023468 1.98357629776001
37.3405075073242 5.57405996322632
-16.6903781890869 16.9814548492432
34.3559265136719 36.4476585388184
23.43967628479 -27.5170402526855
20.829719543457 -13.1163530349731
22.4460735321045 18.1588726043701
18.5000915527344 -6.88822269439697
12.7528686523438 29.7350826263428
23.5409088134766 -13.2740297317505
18.911750793457 -14.8790674209595
19.6516742706299 -13.9972724914551
-15.1662950515747 35.6022758483887
-31.6786727905273 39.7568321228027
-2.05104732513428 37.517692565918
-32.9170036315918 38.9878463745117
-4.5841064453125 29.5460338592529
36.0188674926758 -12.5855112075806
0.334421217441559 -21.2035293579102
-38.5100212097168 -21.8341789245605
28.9254474639893 -12.3004903793335
-37.6920776367188 19.5011730194092
-4.31120252609253 11.9152727127075
37.6475944519043 7.14614820480347
6.6740927696228 39.0491600036621
20.9362487792969 -1.21010935306549
36.8205642700195 5.13460779190063
5.6452898979187 38.4020652770996
-38.6601943969727 -32.2166023254395
-38.696647644043 -21.718074798584
17.9008083343506 20.6502342224121
-3.00767493247986 2.00253438949585
-4.01365375518799 29.5025768280029
-1.65734398365021 37.0307655334473
-40.0244903564453 -21.6756725311279
10.1525945663452 37.8584442138672
-32.0705604553223 38.0155220031738
20.2728595733643 -0.81609445810318
28.824577331543 -12.0976762771606
-34.1393394470215 21.2330570220947
11.3312101364136 38.9146881103516
15.1830339431763 -11.7021207809448
-8.17281913757324 17.566915512085
6.77132272720337 5.00628709793091
33.338752746582 37.3623504638672
6.6757287979126 4.21865224838257
19.6070785522461 0.286183416843414
-39.6582450866699 21.3459529876709
7.5771017074585 4.00451564788818
-34.7371864318848 22.2232837677002
-0.171056866645813 -13.6272993087769
36.2233772277832 6.35810470581055
-38.0926246643066 -23.5484466552734
-6.76210880279541 15.6782159805298
18.1388835906982 21.5761241912842
5.24511909484863 39.946662902832
1.28113114833832 -12.4173908233643
-37.357250213623 -21.5588645935059
20.6652393341064 24.1801776885986
11.0962686538696 35.2891044616699
-32.2011604309082 38.5556182861328
17.8699188232422 -9.28466320037842
18.4677543640137 21.1608791351318
-21.8434944152832 20.0239086151123
-6.67984247207642 19.3380241394043
34.781307220459 -14.4029407501221
-34.1507987976074 20.9644031524658
21.4541206359863 -25.1840553283691
10.9474697113037 37.3879547119141
14.3430843353271 -11.5337772369385
-15.5263137817383 36.0813674926758
36.040470123291 6.10364151000977
-9.0088586807251 29.0088348388672
19.4028663635254 24.7406883239746
-39.8026466369629 20.2291412353516
21.9777240753174 -26.1034736633301
22.0295143127441 0.938367128372192
24.0666236877441 -26.5269947052002
35.389533996582 5.68974733352661
26.8352432250977 -38.0970420837402
27.1573390960693 -24.2180805206299
27.1147747039795 -27.0044002532959
24.5824165344238 -26.2844581604004
28.9718151092529 -26.115385055542
-4.46253776550293 28.8810691833496
-38.5538101196289 18.0383682250977
-38.8512191772461 -21.2980251312256
21.7811584472656 -26.9067935943604
16.5791549682617 -5.50177001953125
32.8452758789062 36.0437507629395
20.9681053161621 0.0813904106616974
19.7205276489258 24.0381641387939
-38.9541168212891 -21.6985626220703
-5.38731908798218 10.5476522445679
-33.5418167114258 38.1347236633301
0.73320072889328 -28.1633815765381
12.3987045288086 -26.9216537475586
17.542631149292 -11.9735069274902
13.0848655700684 -26.1259613037109
36.4127388000488 6.96114826202393
11.8152551651001 38.0062561035156
23.5912132263184 -35.6176071166992
21.4972286224365 -25.0874671936035
-19.2077007293701 23.1310844421387
-38.8258895874023 -31.9222965240479
-18.7131938934326 20.7175350189209
-7.1544361114502 18.2845420837402
34.599609375 5.17091274261475
5.00303888320923 38.8602294921875
-17.226634979248 18.9836559295654
-16.1102409362793 19.5839252471924
35.1703720092773 -12.8139209747314
20.2619476318359 24.6563110351562
22.9294338226318 -15.3716888427734
16.688289642334 -13.8462524414062
21.973237991333 -25.6454086303711
20.9872531890869 -1.0986008644104
20.1918334960938 -13.2663173675537
-16.1343955993652 17.7101955413818
20.4004764556885 -26.5316143035889
22.0069789886475 0.162198722362518
-34.4016075134277 37.9577255249023
30.2712268829346 -27.3316249847412
26.3254241943359 -26.3359699249268
13.0351676940918 29.7412109375
21.9757232666016 -2.52100133895874
15.9940118789673 -14.4478626251221
-2.09932017326355 37.3493156433105
8.4131326675415 3.21424102783203
12.3830451965332 38.1314277648926
34.8145141601562 6.90742874145508
8.1466007232666 4.04409837722778
26.1707992553711 -27.5453948974609
12.1992979049683 -26.5162811279297
11.2058591842651 29.4568710327148
27.1020565032959 -36.1795692443848
30.6375389099121 34.0414505004883
-17.8985805511475 22.679931640625
-36.6622314453125 -32.3392715454102
37.2578544616699 8.15376663208008
17.2907676696777 -5.17515707015991
19.8452415466309 23.7683067321777
11.3145198822021 -26.885721206665
11.4291105270386 -26.7084274291992
-38.2077369689941 -30.4399719238281
34.0922737121582 -14.6165781021118
-15.2790508270264 18.8835220336914
22.8121776580811 -25.9799747467041
20.811372756958 -13.5667428970337
-20.7974224090576 20.2311153411865
19.7366046905518 -9.57624435424805
22.4103183746338 -25.2435894012451
35.3446998596191 8.32227516174316
24.8131370544434 -36.9741554260254
10.7935237884521 29.9077377319336
19.3598365783691 20.6549415588379
0.255202531814575 -29.308198928833
26.6712036132812 -25.6466484069824
-22.2645835876465 22.8308277130127
-7.05539417266846 10.6261281967163
22.3080596923828 -25.1637344360352
26.8030128479004 -27.2531623840332
25.3358211517334 19.5301513671875
20.3777980804443 -14.083251953125
-17.9023876190186 21.8976001739502
-4.05592727661133 30.7748565673828
33.8282318115234 -13.9680671691895
20.4101066589355 -9.03609943389893
24.537691116333 -16.5416526794434
24.8135318756104 17.6518440246582
5.86911344528198 40.0128364562988
33.5435943603516 33.9070091247559
12.5608577728271 29.0389537811279
-0.598617792129517 -30.0046577453613
-19.3079414367676 20.5882129669189
-36.8984413146973 -21.7614212036133
-4.9486927986145 9.81362056732178
5.97498416900635 39.0010604858398
12.0042676925659 38.255054473877
-5.63853168487549 18.6732196807861
-3.09726977348328 30.64137840271
23.6427879333496 -24.7662963867188
34.1695747375488 -11.1727628707886
2.56182098388672 -22.2187557220459
26.5241832733154 -37.7751808166504
28.101224899292 -13.305365562439
11.3224992752075 38.6800994873047
-9.98404502868652 28.7839241027832
35.7229690551758 -11.6783332824707
-6.18054056167603 17.3865280151367
18.3642673492432 21.6505546569824
-41.0859031677246 20.3583126068115
-16.3325519561768 17.9989986419678
-15.3466186523438 17.1191902160645
6.94118547439575 5.16203832626343
6.44891929626465 3.47531604766846
17.1351795196533 -11.6940565109253
23.9226608276367 -26.4560375213623
-15.8968963623047 20.3261241912842
-17.0942211151123 21.1165866851807
11.9103622436523 -27.5063076019287
16.3977832794189 -10.6178026199341
-34.6433868408203 21.5473823547363
-36.9337577819824 -23.5270404815674
-9.76964664459229 28.374942779541
25.8787078857422 17.4470634460449
20.5250282287598 24.0783653259277
18.9472789764404 -11.6532068252563
-0.387426376342773 -28.6018524169922
23.7654304504395 -26.2903118133545
20.5805263519287 -0.324506014585495
33.5711517333984 5.79982757568359
-39.2039642333984 -21.2414035797119
-39.8541641235352 -22.9884262084961
-5.33392524719238 11.0334520339966
-18.3254318237305 22.057653427124
5.91521072387695 37.0775413513184
7.11790037155151 37.5539627075195
19.0445995330811 23.1823196411133
11.4760999679565 -23.8470993041992
-4.91430282592773 29.1988906860352
11.0930786132812 -26.5410575866699
-38.4276924133301 20.1499080657959
-4.65405464172363 11.1198358535767
26.2954025268555 17.7012424468994
-15.8612470626831 18.002067565918
20.2883434295654 23.5887145996094
36.9564781188965 -13.5865306854248
-23.0218410491943 20.8076286315918
17.075777053833 -5.553391456604
-38.5396308898926 -30.6057815551758
19.4942302703857 -7.11318635940552
19.4525375366211 -14.3680753707886
5.26335096359253 39.0787353515625
6.34642744064331 3.57538080215454
24.1841602325439 -25.948429107666
-37.8887367248535 -21.368968963623
-39.444221496582 -32.0108413696289
-14.0543813705444 36.4290504455566
5.79419565200806 4.23469638824463
-34.6760215759277 37.8196296691895
7.1212363243103 5.64621877670288
37.4340667724609 6.46373224258423
-4.4233512878418 12.3934545516968
-22.894458770752 19.1967697143555
-2.95461130142212 0.614311337471008
24.3092842102051 -13.9859619140625
10.9139890670776 28.647159576416
-18.9109802246094 20.8251247406006
-17.2628612518311 23.6117153167725
-17.1659088134766 21.6031532287598
-21.8277168273926 19.5962829589844
27.6065521240234 -27.7908458709717
-1.95334339141846 1.30535364151001
19.7169704437256 -12.892954826355
-21.2993316650391 18.9924831390381
20.1486949920654 -8.44713592529297
5.62900590896606 4.60357141494751
0.135349810123444 -19.5231075286865
26.0776634216309 18.5602207183838
-14.7255926132202 34.9252700805664
-0.382656097412109 39.2006301879883
-5.0355281829834 12.1688613891602
-36.5231170654297 -20.3001861572266
35.156322479248 -13.1462287902832
15.6807775497437 -13.2048568725586
23.5643367767334 -25.4290885925293
25.3991889953613 -35.743766784668
20.3568725585938 24.7932453155518
-4.34280586242676 0.255799174308777
19.7185211181641 -11.8999853134155
17.8228740692139 -6.08810615539551
11.6325759887695 37.3871955871582
19.8575229644775 -13.5733509063721
-15.3496341705322 36.2002792358398
11.7399473190308 -26.7822647094727
27.6002140045166 -37.9360847473145
-33.7920379638672 18.8714294433594
25.2092552185059 -24.9660129547119
17.9353637695312 -13.490665435791
-15.6225509643555 34.549430847168
-35.7040061950684 20.7546863555908
24.2491550445557 19.1095008850098
20.690845489502 0.494317293167114
-3.32899308204651 29.153736114502
-6.51904630661011 17.0379524230957
-37.954906463623 -33.3598861694336
1.18949663639069 -12.6021499633789
12.4310302734375 -25.8565673828125
20.1335792541504 -13.4342947006226
-6.4936580657959 12.2775344848633
-8.71467113494873 27.7250499725342
26.2694797515869 17.6696758270264
20.4048748016357 -13.60671043396
7.16769886016846 39.4981651306152
-15.6630716323853 18.5771141052246
36.6382522583008 -12.2356519699097
-0.862668454647064 38.6324615478516
12.0181188583374 -23.8401260375977
15.0636892318726 -12.2785053253174
19.173095703125 23.6996917724609
2.13736915588379 -22.1568069458008
19.6917934417725 21.7328281402588
28.1048793792725 -27.0755157470703
-5.19209671020508 11.080620765686
-39.9021873474121 21.7478065490723
-39.1666259765625 18.7044696807861
16.0352611541748 -11.781792640686
25.8156547546387 20.7181053161621
11.0167083740234 29.1893558502197
31.9771938323975 37.8789482116699
-18.7232913970947 21.6967163085938
33.7360000610352 5.52052354812622
4.78761672973633 5.65512466430664
18.1483974456787 -6.05249500274658
-15.7664804458618 18.2588596343994
5.90154504776001 38.4470672607422
2.33928251266479 -22.3809909820557
-9.21863460540771 26.5661334991455
34.6374664306641 37.0940818786621
22.8329296112061 -14.6727981567383
18.308837890625 -3.55853128433228
11.0532255172729 37.1559944152832
20.0489311218262 -13.0125427246094
33.0748405456543 36.5574989318848
-17.2868881225586 19.381856918335
19.761568069458 22.1146697998047
35.7727165222168 -13.5999603271484
-4.76241016387939 29.9956359863281
13.5893650054932 37.1813125610352
20.5551128387451 24.8811492919922
-4.06071662902832 12.0999822616577
17.5819244384766 23.0868053436279
16.0222702026367 -12.0722236633301
17.604341506958 -5.45916366577148
24.7976932525635 18.1085433959961
24.1668434143066 -24.9207515716553
19.2971973419189 24.7373924255371
23.0658493041992 -25.5189266204834
33.61865234375 36.7058944702148
34.1552429199219 36.4317321777344
-3.43968486785889 10.730504989624
11.5697822570801 38.1371383666992
-0.358612418174744 -21.7944889068604
21.80908203125 0.0617250800132751
21.501802444458 0.3774453997612
16.9486885070801 -5.36302614212036
-2.83221077919006 32.3618392944336
11.9451141357422 -25.6870956420898
11.0861253738403 29.1911106109619
-17.108850479126 20.9777946472168
-9.65590286254883 27.0292739868164
-17.0025653839111 17.3712711334229
11.7305202484131 38.0552711486816
20.9849758148193 -13.587474822998
-15.2475423812866 37.1847381591797
15.1844434738159 -11.2393217086792
35.8831520080566 5.24127101898193
-33.6352882385254 38.6411361694336
11.7397766113281 -28.0741291046143
6.49943494796753 2.81970715522766
35.765811920166 -14.3682174682617
20.8848667144775 -14.2158555984497
-14.1654720306396 36.6413688659668
-18.7055435180664 21.0906867980957
17.1504516601562 -5.70021820068359
-15.6973457336426 18.4477443695068
-38.6939888000488 20.7744750976562
-38.8987770080566 -32.7235679626465
22.0899677276611 -15.6347818374634
34.2817153930664 -13.2635593414307
7.60440683364868 2.62035942077637
1.91892027854919 -21.4572677612305
27.292106628418 -35.3942985534668
-0.11670908331871 -28.4863300323486
10.6379766464233 29.4362564086914
-37.7971687316895 -33.0045051574707
29.2656002044678 -11.3829011917114
9.04708766937256 27.6775226593018
24.8805999755859 18.15403175354
25.0677585601807 -26.5743236541748
-36.6181449890137 -30.6640701293945
22.7701969146729 -23.0181636810303
25.5212898254395 -26.3773612976074
20.1723556518555 23.8758544921875
13.162914276123 -27.2824325561523
1.29571580886841 -22.9915008544922
36.670223236084 6.60422515869141
7.83052396774292 5.33616924285889
29.5270023345947 -11.4744720458984
8.47206783294678 5.25799226760864
15.2209577560425 -11.5379648208618
27.0120639801025 -30.8699150085449
21.1107749938965 -26.2560615539551
25.560583114624 18.7693538665771
0.673336982727051 36.3767509460449
-37.2328491210938 -31.0561504364014
-39.6515083312988 -32.0478401184082
1.59983491897583 -21.9559993743896
7.25666618347168 4.02016735076904
26.1362190246582 -27.1658267974854
25.7774772644043 -26.1877841949463
-4.65259456634521 30.1761379241943
-32.5770225524902 38.7881355285645
-0.300345897674561 -20.1355438232422
-15.2113065719604 35.4814224243164
26.3226661682129 -37.6099891662598
5.51714468002319 41.1511688232422
-3.27793788909912 11.4239206314087
35.4186477661133 5.49962282180786
13.1673517227173 38.3489036560059
-0.638092219829559 36.107837677002
34.6446762084961 8.10297584533691
-17.6249771118164 16.6236610412598
-15.1046180725098 16.8413181304932
25.584810256958 -36.9794654846191
32.2170028686523 36.6539154052734
26.5015697479248 -27.1460380554199
20.8244094848633 -1.31572318077087
17.395975112915 -6.38840675354004
-23.2525367736816 20.2657051086426
-39.0192184448242 20.603422164917
13.5291166305542 -27.8494663238525
14.9452066421509 -11.1809759140015
-7.3464150428772 18.34619140625
0.305238544940948 -21.9995498657227
35.6168327331543 -13.4465026855469
35.076831817627 -14.4349555969238
-34.352596282959 20.3618450164795
4.79017496109009 3.62681293487549
-0.863532304763794 37.2665939331055
20.3489894866943 0.980387449264526
10.9888944625854 39.0901374816895
1.81769025325775 -11.4761447906494
34.5630722045898 5.65443801879883
-21.4429531097412 21.8937301635742
-13.8474950790405 34.8475036621094
-7.77054882049561 10.8155879974365
-0.0670872926712036 -13.8194561004639
19.0497779846191 24.3578472137451
-33.8944473266602 22.2644386291504
22.8908748626709 -17.0352897644043
22.3887538909912 -12.996675491333
18.588020324707 20.4076042175293
35.7535820007324 -12.9419212341309
25.0878105163574 19.7757873535156
-14.4112768173218 35.1185874938965
-0.138682007789612 -30.0777282714844
1.6523323059082 -11.7185029983521
10.8354740142822 37.4173583984375
-6.59971618652344 11.4754524230957
-18.8103466033936 19.7892589569092
12.3109979629517 -23.4076862335205
23.8686904907227 -14.4278297424316
-15.3046798706055 18.9929027557373
-31.3694801330566 36.7115478515625
-23.0820178985596 20.8095932006836
5.11081981658936 2.92043423652649
-7.58932542800903 17.1799163818359
26.9305324554443 -37.3635215759277
9.80728912353516 39.0038948059082
18.8001842498779 -12.1600923538208
-4.00961780548096 29.4242763519287
-18.6631183624268 21.6455364227295
-9.09537887573242 28.4922904968262
14.6366968154907 -12.1694002151489
-7.31922006607056 17.0718898773193
23.5783615112305 18.4083957672119
18.306468963623 24.6459541320801
1.74930334091187 -27.87819480896
21.7852268218994 -25.8483543395996
22.6007881164551 -38.0444221496582
18.8040351867676 -6.79974889755249
-38.6741485595703 -31.4828281402588
18.897518157959 -8.90655422210693
33.6765594482422 35.6451416015625
24.6963520050049 -24.5367622375488
-38.7438049316406 -33.0514488220215
-14.8255767822266 36.6375961303711
-32.6511764526367 39.1292495727539
21.3954906463623 -15.63853931427
35.1492919921875 36.3946800231934
4.36931419372559 38.4841690063477
-2.35889053344727 36.1791343688965
-21.4447650909424 19.7076358795166
13.7132635116577 -26.3520030975342
-0.246402829885483 -29.783712387085
10.3818941116333 27.9655704498291
-4.59385538101196 29.6150302886963
27.8922443389893 -27.5062637329102
-4.56665325164795 0.893021106719971
-33.7061996459961 39.7494468688965
6.96794271469116 2.75874638557434
29.4353275299072 -11.246657371521
12.3178005218506 -25.7898693084717
29.7480010986328 -13.5320310592651
32.4930267333984 36.799503326416
2.49840617179871 -22.5965785980225
5.92998504638672 40.27001953125
-39.6235008239746 -22.4611968994141
14.8321208953857 -25.5753974914551
25.6213474273682 -36.7321166992188
19.350622177124 -12.4502601623535
-9.70569801330566 28.2331485748291
-4.76692628860474 12.6052179336548
-4.85777473449707 11.322135925293
-0.856096625328064 38.6122817993164
6.79908227920532 4.35855960845947
10.5803508758545 37.4483337402344
-5.42178535461426 11.708438873291
-22.6170387268066 20.0419483184814
9.85978507995605 28.8127746582031
34.5956802368164 -11.2054862976074
12.1641836166382 27.2695446014404
22.5752964019775 -24.9203834533691
-32.0534820556641 37.4814414978027
25.10693359375 19.618595123291
-0.434235781431198 -29.3549709320068
-9.9063024520874 27.1096878051758
-18.18776512146 19.7401828765869
15.0559711456299 -11.2729606628418
-4.16897964477539 31.1915283203125
16.2626399993896 -6.18920278549194
25.014347076416 -37.0973320007324
-17.3985652923584 20.7236843109131
-40.0892448425293 -22.0542335510254
-34.1349067687988 21.0225296020508
-0.0481623411178589 38.6937026977539
-0.621774196624756 -14.5189113616943
10.7997894287109 27.9375877380371
-14.8212261199951 35.2953872680664
20.6462211608887 0.178753912448883
6.30902147293091 3.39378213882446
27.4670734405518 -12.2958221435547
-32.9234008789062 37.6796493530273
0.736957192420959 -29.0069465637207
22.3929328918457 -14.9127902984619
23.6072959899902 -25.3234958648682
-9.88541984558105 26.5867958068848
21.8782749176025 -24.1059112548828
0.132764935493469 -14.3174819946289
23.5925216674805 -26.3083992004395
-14.2960758209229 35.0392189025879
6.26101064682007 38.7844161987305
-8.26847553253174 27.2110996246338
-37.6733512878418 -32.699390411377
-34.0477523803711 23.2809276580811
10.2983140945435 29.4181423187256
19.8186702728271 22.8015384674072
18.186071395874 -5.4840235710144
5.16236209869385 39.8998870849609
24.6815433502197 16.673698425293
-14.8195600509644 35.2713088989258
-10.519871711731 28.1697444915771
-38.2684669494629 22.2197723388672
-33.9797401428223 19.6654243469238
27.194860458374 -28.0853061676025
34.9093971252441 -14.1487607955933
-3.75495767593384 12.8446989059448
-35.3205718994141 21.2211494445801
22.8950443267822 17.8681297302246
-6.90027523040771 11.0700693130493
-15.5422468185425 17.9760913848877
2.53963613510132 -30.8142127990723
23.288257598877 -15.5577039718628
22.6731090545654 -26.1436290740967
13.4386873245239 37.7014312744141
-40.4903945922852 16.5892772674561
-8.49634170532227 28.0396690368652
21.3384132385254 -6.91153335571289
-33.3168106079102 19.3658313751221
34.4165992736816 -12.2876996994019
24.5235633850098 -24.0776824951172
19.9129390716553 22.0090065002441
11.3385391235352 38.1609497070312
-36.1300086975098 18.6151752471924
-7.99402523040771 20.0944023132324
26.6269950866699 -26.2695999145508
5.24496650695801 38.9269523620605
-38.7910461425781 -23.1546154022217
-18.2747383117676 23.4999179840088
19.1026515960693 1.08628165721893
0.8499396443367 -22.8688316345215
17.769100189209 -5.04371929168701
0.669321060180664 39.2398452758789
34.8685836791992 6.08064746856689
28.3923435211182 -11.9039850234985
19.8422336578369 -4.32498216629028
12.1280946731567 36.7111587524414
16.2920112609863 -12.1902704238892
22.4458446502686 -15.6860437393188
28.4747905731201 -13.1270236968994
-23.7869815826416 20.0552597045898
-13.2155418395996 34.9475746154785
18.1082515716553 -7.0681529045105
19.4100437164307 24.0193214416504
-0.63042140007019 -12.3289356231689
36.1707229614258 5.66828966140747
-2.60657858848572 -0.178720474243164
-1.31087815761566 1.84567058086395
-39.0183601379395 18.6249122619629
29.0730514526367 -29.2967681884766
-9.31714630126953 27.6102046966553
-39.2274284362793 -21.992546081543
21.2775897979736 0.145015209913254
29.5525093078613 -13.6517915725708
-4.73161172866821 30.2478542327881
22.4328880310059 -0.762822806835175
2.1118643283844 -13.707537651062
-21.7809009552002 19.8800449371338
10.0749263763428 39.5461158752441
-14.0239706039429 34.6639022827148
18.8366432189941 22.7561798095703
5.04431676864624 39.7310523986816
35.5584373474121 -14.0831890106201
27.8331699371338 -25.8798408508301
33.2376708984375 35.8764343261719
1.57623386383057 -20.1179237365723
-15.4921522140503 35.7464714050293
-36.0370483398438 21.022668838501
18.0819606781006 21.5801811218262
1.0547821521759 -21.4772052764893
-33.4927062988281 38.7307357788086
10.90221118927 29.5577087402344
21.5483570098877 0.244258463382721
25.0338401794434 16.6919364929199
7.02785682678223 37.2157936096191
34.5203437805176 5.98952198028564
23.8435192108154 -26.7199287414551
19.5208473205566 24.0856609344482
18.2196025848389 -3.23571705818176
5.3467116355896 38.5482406616211
-33.4111213684082 20.1574687957764
18.5524253845215 -13.2975397109985
-4.20354413986206 30.7185249328613
7.90651702880859 2.15985822677612
-20.0138874053955 18.7408828735352
0.264088541269302 -28.5232601165771
-31.3695831298828 38.2696266174316
35.6226272583008 -11.8519725799561
23.1555671691895 -25.5961303710938
20.4931983947754 24.8746242523193
22.4777069091797 -1.49546313285828
22.1933345794678 -26.1297378540039
27.3711929321289 -27.610143661499
26.0011425018311 -26.0884819030762
-38.3329124450684 19.8643264770508
-21.680549621582 20.8338451385498
19.2869300842285 21.0719871520996
-36.8134117126465 18.6959743499756
35.5343170166016 7.53125762939453
29.0717868804932 -12.1211090087891
19.1857471466064 23.964656829834
19.4376735687256 24.2264652252197
28.3500061035156 -12.9113130569458
8.26650714874268 39.250057220459
-2.44615793228149 2.38186740875244
-3.77221012115479 30.8617115020752
34.7973175048828 4.86732196807861
35.2357406616211 -10.9348297119141
12.8300981521606 -24.3675689697266
12.5965909957886 -26.7595996856689
19.962438583374 23.1942176818848
6.96383428573608 2.67872476577759
25.1447200775146 -35.5903167724609
-18.4391193389893 19.642204284668
-32.2520523071289 38.6417465209961
-35.3108444213867 20.8274478912354
-8.65216827392578 17.5849761962891
-6.78714418411255 11.0511627197266
19.6632232666016 20.5954036712646
36.8385200500488 -13.0040664672852
-15.4423723220825 36.7778358459473
20.8964462280273 -25.4342880249023
22.6858959197998 -15.1770973205566
28.4902381896973 -11.6926546096802
-38.2301940917969 19.0749816894531
26.1610221862793 -35.8345184326172
6.68308639526367 4.37112331390381
0.158496469259262 -23.4284782409668
-22.2974090576172 21.2894630432129
33.5764083862305 4.43122100830078
28.6391677856445 -27.5175399780273
27.2261028289795 -27.0974216461182
24.8234004974365 -25.2238082885742
-14.2102270126343 35.6773719787598
24.5200328826904 -26.9666423797607
26.5368213653564 -26.7842597961426
12.5609922409058 27.8715133666992
-15.5047960281372 35.733772277832
-4.65696811676025 28.9497394561768
0.0259658098220825 -13.949315071106
34.6708335876465 3.90180969238281
-4.32521772384644 11.1494302749634
21.5400009155273 -26.4714641571045
-35.1437950134277 21.458381652832
-20.6360168457031 20.1614379882812
-38.5051612854004 20.6160049438477
34.9126510620117 -13.8202486038208
-34.2460823059082 37.6361770629883
-15.7190027236938 21.4817981719971
-13.9647150039673 32.4111862182617
-19.2308235168457 21.7330112457275
19.765567779541 -5.19640779495239
20.1088943481445 23.7538375854492
7.24126100540161 5.15505599975586
19.2643127441406 23.2392292022705
34.2192878723145 37.1144523620605
-4.36884546279907 11.6441488265991
20.4799289703369 -7.53299617767334
24.9163188934326 -14.1244792938232
20.3195304870605 -14.3925228118896
-14.6299142837524 35.7174949645996
-8.84939670562744 17.6901245117188
5.22731876373291 38.0339508056641
-35.3760757446289 22.2140445709229
-3.45046591758728 2.64632654190063
-9.18490695953369 27.9201812744141
-15.8494577407837 17.3455982208252
-37.9869346618652 -22.4325580596924
19.0728721618652 1.81834769248962
-39.439582824707 -22.259162902832
17.2589225769043 -6.9368371963501
28.9548282623291 -12.6814813613892
16.304557800293 -11.6850547790527
12.7855844497681 37.5535202026367
27.517879486084 -12.2617359161377
20.0165176391602 22.9950923919678
20.9012813568115 -14.3790636062622
17.3839836120605 -6.42757129669189
-0.966454803943634 -29.1661262512207
-35.7076034545898 20.4050521850586
-38.1751136779785 -22.074577331543
-38.5940437316895 -22.0994682312012
21.3260231018066 -6.01644611358643
25.2760429382324 -35.5989570617676
18.2794513702393 23.5419960021973
33.3688125610352 35.7938346862793
-36.9383277893066 -31.5540676116943
24.7119522094727 -35.8666343688965
5.41612482070923 38.2300720214844
18.0923881530762 23.3351192474365
19.9602699279785 -13.6578598022461
-22.5687084197998 19.2832546234131
29.2809162139893 -11.9140148162842
13.1778545379639 29.4030208587646
-38.7632446289062 -21.1385555267334
-38.3138389587402 20.9442501068115
12.726490020752 -25.3516254425049
1.71423375606537 -20.9270000457764
-6.55204391479492 17.8553123474121
-10.1929683685303 29.0903282165527
5.86164379119873 3.76550889015198
-1.54227375984192 31.229154586792
21.5612831115723 -14.1548871994019
7.0527720451355 5.55315923690796
-10.8800554275513 29.295768737793
13.0050172805786 -25.6692237854004
0.737440466880798 -20.828052520752
17.690113067627 22.7807292938232
-7.86427307128906 17.7086391448975
-17.902271270752 20.6324901580811
19.206823348999 -7.76945304870605
0.281190514564514 -12.0389556884766
19.5197067260742 -13.8658561706543
29.4289169311523 -28.1228294372559
6.57815885543823 3.87981390953064
-33.5626907348633 21.0616302490234
-8.61462879180908 16.9100933074951
25.4935150146484 20.0683841705322
34.6686935424805 -11.6934280395508
-3.12372756004333 30.1965179443359
-2.49553346633911 36.4637794494629
6.49420642852783 39.3657913208008
22.6077575683594 -13.773754119873
19.7218933105469 -8.79190826416016
-15.0540456771851 35.3836898803711
-4.32968902587891 12.082631111145
24.6260070800781 -26.8897552490234
19.7540016174316 -5.58465766906738
34.7253303527832 34.4408798217773
21.6364402770996 -25.5900821685791
27.6077346801758 -11.3059434890747
20.5131855010986 -14.1593837738037
19.1649379730225 21.8897304534912
-37.4871635437012 -32.5644493103027
0.684351086616516 -12.400369644165
-20.9938564300537 22.2519283294678
16.4287891387939 -12.6304769515991
-39.3072776794434 -23.1441345214844
15.1146326065063 -11.7576389312744
22.576208114624 0.694057106971741
11.2272605895996 -26.5747680664062
18.8303318023682 -13.5744457244873
21.6489009857178 -26.500581741333
20.7594890594482 -8.2756872177124
-10.3436346054077 27.7878284454346
20.6588554382324 -8.54382228851318
15.305643081665 -11.5909729003906
19.0148315429688 23.1194801330566
-17.5263729095459 19.2852878570557
10.7141141891479 37.6980285644531
19.3280544281006 -6.49561786651611
-2.35081648826599 0.0933352708816528
-2.62764739990234 28.7247638702393
-38.8946876525879 -22.236478805542
7.31608963012695 5.32646894454956
-2.95895457267761 0.359986901283264
-2.1765296459198 1.13001465797424
18.1265716552734 -5.68607616424561
-2.75601601600647 2.21288204193115
-7.59542465209961 29.4260120391846
33.5304946899414 35.9033851623535
26.9492111206055 -28.5560741424561
35.7377662658691 7.03520679473877
-5.78120708465576 17.6817035675049
-8.43236923217773 27.7148723602295
6.44084215164185 3.44573664665222
-6.82878112792969 19.1193256378174
13.1301736831665 -26.3162403106689
-2.72939276695251 0.300749242305756
-37.8963508605957 20.2307281494141
18.1197395324707 -6.50128889083862
34.7064819335938 6.83473968505859
-1.55179464817047 38.2597427368164
-7.09201049804688 18.0301914215088
19.6692085266113 22.5899906158447
-11.8667736053467 36.0031661987305
-39.8415336608887 19.1421852111816
-13.6613788604736 35.4394454956055
22.0025482177734 -23.1150970458984
21.0643119812012 -11.673641204834
17.457405090332 -6.99778270721436
16.5499401092529 -11.2229862213135
-15.0225086212158 17.5469627380371
22.8836822509766 -15.8883037567139
31.9706020355225 35.5749206542969
23.8101634979248 -15.2454919815063
12.5003862380981 38.0822601318359
-3.69493651390076 11.7818202972412
15.4545669555664 -13.7477426528931
22.2977981567383 -14.3912534713745
-12.8535165786743 34.1791381835938
-8.19353675842285 27.4577655792236
1.03981173038483 -22.0599689483643
23.4123554229736 -24.544563293457
18.1531963348389 21.3056659698486
-30.9890060424805 37.6500625610352
12.6330871582031 -25.8075942993164
-35.9731826782227 22.7007446289062
26.0113372802734 -37.0500755310059
21.9084358215332 -0.818355560302734
-22.729679107666 20.9544277191162
-35.5266647338867 20.8126220703125
-14.5567922592163 37.2168502807617
17.6553726196289 22.9189739227295
-16.6433563232422 20.8154926300049
19.3643321990967 -8.89235305786133
22.6673698425293 -13.6849794387817
28.5416393280029 -26.3578853607178
-14.4375352859497 35.7097816467285
14.0734977722168 -26.8519248962402
-1.60311114788055 2.33738541603088
-32.2508277893066 37.1521377563477
-15.2476844787598 17.9164237976074
18.5854148864746 -6.63619756698608
33.9949798583984 37.251091003418
10.4141550064087 26.9898910522461
-39.1732902526855 -33.5172424316406
27.8923301696777 -27.2579135894775
24.6626434326172 18.3752975463867
20.5241451263428 -8.56516361236572
20.7697639465332 24.1315422058105
-32.1114921569824 38.2963676452637
21.2286853790283 -7.75102090835571
24.7068710327148 18.3142395019531
2.40810966491699 -20.5041790008545
-36.0149574279785 -22.4138603210449
18.87327003479 0.0633269548416138
-39.1197319030762 19.7249355316162
-31.4394626617432 39.4812812805176
-22.04856300354 19.1007308959961
-14.9933710098267 36.3589897155762
-3.77835702896118 29.9026546478271
19.1034049987793 22.8264236450195
19.2299633026123 -12.6289224624634
-2.51458024978638 29.9764099121094
-3.9579918384552 30.7687149047852
33.8510513305664 -14.6460990905762
-40.2941474914551 -32.149486541748
18.0074672698975 -6.52253437042236
6.08818054199219 37.5497055053711
21.4936847686768 -13.3144903182983
-2.41368436813354 1.76062631607056
24.1836929321289 17.9220638275146
22.5651588439941 -24.5494232177734
2.64237642288208 -12.6906747817993
-0.00869172811508179 -21.4415321350098
27.9418983459473 -13.1147174835205
-4.02916860580444 28.8811092376709
-38.1315994262695 -32.9406623840332
-39.7297439575195 20.1264095306396
-18.7171077728271 19.5418891906738
18.8948993682861 22.3148422241211
-37.4704322814941 17.8840656280518
-18.3135433197021 19.272518157959
-3.27426671981812 29.782356262207
0.611808300018311 -27.4707374572754
10.5193243026733 28.4134502410889
12.9113454818726 37.5570106506348
1.60333001613617 -12.6196317672729
17.9697132110596 -6.414626121521
34.9104423522949 -14.2880973815918
26.2365703582764 -24.6624698638916
11.1901063919067 37.3116569519043
-36.6633682250977 -32.6618804931641
33.0936164855957 35.117130279541
0.500472784042358 -22.710355758667
28.6589183807373 -28.50022315979
17.7549705505371 -5.597487449646
-39.6046409606934 -32.7931060791016
30.156213760376 -11.0615425109863
21.0515289306641 20.3574924468994
20.0724487304688 23.459644317627
-6.16450452804565 11.9371185302734
16.2745933532715 -4.69379663467407
6.128249168396 4.78538227081299
35.3564872741699 -13.1814622879028
17.3686237335205 -11.3324871063232
-16.1534099578857 36.3925094604492
27.97971534729 -23.1865386962891
-6.3667573928833 18.2400798797607
6.02043628692627 38.2584991455078
-2.96556925773621 30.9004611968994
29.1156940460205 -13.0560684204102
20.1682739257812 20.1182918548584
21.6970901489258 -7.32469844818115
16.3257961273193 -11.275616645813
4.67438507080078 39.6987266540527
20.6566143035889 -7.46373987197876
10.3528985977173 29.3827533721924
25.3381614685059 -36.1050682067871
-35.6382026672363 22.5699195861816
21.6525058746338 0.683424353599548
-4.06531953811646 30.3487014770508
24.5251770019531 19.1141872406006
-1.52436816692352 0.141926348209381
19.6749668121338 -14.9396171569824
26.39186668396 -28.1626319885254
-5.35819721221924 11.2708568572998
-0.173611640930176 -11.6076745986938
18.0254287719727 -5.02355003356934
38.0320014953613 6.44345045089722
-33.3191604614258 39.774097442627
24.6887989044189 18.0872421264648
19.4345436096191 23.7395477294922
17.1564846038818 -11.4299716949463
16.6904144287109 -4.56715202331543
18.4972648620605 -5.59022426605225
28.2448234558105 -12.5601072311401
-38.9854431152344 -33.3422813415527
19.3858642578125 -12.6785221099854
-35.0359878540039 20.2157096862793
25.3115768432617 18.316198348999
0.358360111713409 -13.053858757019
-37.2537307739258 -31.4021110534668
-14.8987064361572 19.6448745727539
21.6887798309326 -25.3264484405518
-38.5713043212891 -23.3001804351807
-38.6267852783203 18.8739700317383
11.4982995986938 26.9571857452393
11.1241550445557 37.8153915405273
-15.4757871627808 16.3880844116211
-31.8622970581055 39.7524108886719
30.1272525787354 -12.1911029815674
5.34904384613037 39.0558815002441
20.4743232727051 -1.95415484905243
27.7298431396484 -11.5139503479004
-39.0173759460449 -24.270866394043
24.177942276001 -23.801477432251
5.71635246276855 38.6054191589355
10.8415517807007 -26.062427520752
29.3465328216553 -13.8605604171753
19.9705905914307 24.6774005889893
18.2143859863281 -6.74286460876465
29.6995525360107 -12.1976222991943
17.7907333374023 -11.253662109375
9.99224853515625 27.7456550598145
12.3474006652832 37.0884552001953
17.8948936462402 22.9855690002441
-0.0850875377655029 -14.0618371963501
-15.7523975372314 18.2335376739502
-3.86764645576477 1.63027596473694
37.3584976196289 -13.5550241470337
34.491527557373 -13.5210294723511
18.2486763000488 -6.61040639877319
-40.6000671386719 -22.5960502624512
-8.96903133392334 28.593599319458
-38.4475479125977 19.4401454925537
-4.33192491531372 12.1007862091064
20.6830234527588 21.8969802856445
0.705078959465027 -14.6387243270874
-38.5151405334473 20.9584159851074
-6.14212799072266 10.8592481613159
-34.4706535339355 22.1495304107666
-5.66733837127686 10.3221797943115
-14.2556076049805 35.6119537353516
-1.49128258228302 36.8264236450195
20.2089004516602 21.7443714141846
-16.1526184082031 35.6980133056641
28.5557403564453 -12.3027601242065
19.9376888275146 23.7764492034912
-36.9095115661621 21.7577419281006
21.1328773498535 22.4563808441162
5.19954061508179 39.557991027832
-11.2095184326172 27.7878837585449
26.1037521362305 -29.0172290802002
-0.326337337493896 37.4834861755371
21.3255424499512 -27.3037014007568
12.4671936035156 35.7003631591797
-31.4736576080322 38.5441818237305
-37.8234214782715 19.4787769317627
-4.18889379501343 30.2265949249268
11.7950086593628 27.5997581481934
18.8494491577148 -8.06839847564697
-21.2208023071289 19.8068542480469
21.4016990661621 -14.4180307388306
-22.4874725341797 21.2700977325439
-9.09526920318604 16.7085399627686
13.5067472457886 -12.3902072906494
-37.2057838439941 18.8349437713623
11.8155488967896 -25.519380569458
33.7624359130859 37.090446472168
17.1742572784424 -5.88045883178711
-1.32492673397064 -21.168285369873
9.96174240112305 36.9637565612793
19.411340713501 -14.4290590286255
-33.4098281860352 37.903377532959
-3.72473430633545 29.9393253326416
27.604528427124 -14.3895416259766
4.96794509887695 38.8472099304199
23.0633125305176 -15.3850040435791
-38.2354393005371 -34.2713279724121
0.263824790716171 -22.7738971710205
-21.5447521209717 20.6118602752686
-37.7375411987305 -21.8899116516113
6.3315634727478 39.7305374145508
-5.00806188583374 12.5870714187622
-0.138384580612183 39.0512733459473
-16.9385814666748 22.4508056640625
-20.227575302124 20.9170436859131
17.0910205841064 -8.47833061218262
-5.41152381896973 16.4511032104492
-3.94858264923096 13.7262582778931
-4.20622873306274 1.60947847366333
-2.5496346950531 0.0660258531570435
20.154447555542 23.4927921295166
-38.5840797424316 -22.8145713806152
-16.8340930938721 21.3565425872803
35.544548034668 5.28296279907227
23.6850261688232 -15.1015567779541
8.44779586791992 3.96247959136963
35.7481231689453 5.25248432159424
-17.0982971191406 17.6051979064941
22.437385559082 -14.3738479614258
-38.4264831542969 -23.6096324920654
21.7793827056885 -1.29954767227173
15.0674467086792 -12.7715167999268
-34.2070236206055 22.8333377838135
0.617521643638611 -21.9016857147217
-38.2623748779297 19.2252960205078
27.2692317962646 -27.4356803894043
-32.4700698852539 39.6869125366211
24.392822265625 -26.8470287322998
23.5338497161865 -25.4215755462646
-2.79694962501526 29.5487213134766
-39.051139831543 -21.789436340332
35.1161079406738 -16.5022144317627
18.5745735168457 23.967586517334
0.723392248153687 -22.261962890625
-39.5103797912598 17.2332630157471
22.8329086303711 -14.2803287506104
7.51050424575806 2.58864307403564
-0.0960440635681152 38.3386268615723
35.2590103149414 6.31185913085938
-15.3724851608276 19.2443351745605
2.42309284210205 -19.8111782073975
25.4396057128906 19.3776817321777
21.9004955291748 -14.3709774017334
0.260004222393036 -20.6443576812744
26.5871696472168 -26.8048706054688
-38.0896339416504 -31.3905906677246
-39.7950592041016 -22.0002708435059
-6.35041046142578 12.6724891662598
20.3136024475098 -14.6452436447144
-9.56934547424316 27.7877922058105
-41.4995269775391 -21.5178680419922
9.79735946655273 27.5424747467041
34.8249244689941 5.40764331817627
-16.2729549407959 17.966625213623
0.171764403581619 -21.1734409332275
-1.76570105552673 -12.3178186416626
-18.3205471038818 20.8665390014648
17.9944229125977 -5.3397421836853
-6.02861022949219 12.9476537704468
-36.4464454650879 -32.5445747375488
12.2376317977905 38.2388687133789
-39.7007026672363 -31.1749076843262
-38.3491363525391 19.3132820129395
22.2917308807373 -14.981915473938
0.423974990844727 -19.3061065673828
18.8830585479736 -6.50533390045166
-11.9951944351196 34.6684150695801
36.5426750183105 5.64804267883301
-34.4240913391113 20.6424655914307
23.8036937713623 -14.189790725708
20.5637741088867 -25.5044956207275
12.1722526550293 29.617244720459
12.625524520874 26.3186416625977
-33.2603797912598 21.2022037506104
-23.1167144775391 20.644458770752
-22.6200180053711 20.9553451538086
19.0978946685791 21.4595241546631
-32.7713584899902 38.530086517334
20.2167320251465 -8.18320846557617
20.598482131958 -14.660228729248
-37.269287109375 -21.5345516204834
-2.69224119186401 28.6932582855225
19.064977645874 21.2565498352051
35.160457611084 6.84432220458984
-12.8741331100464 34.8888397216797
11.2383518218994 27.4175930023193
-35.749755859375 20.6588802337646
-34.0405158996582 37.5541496276855
-7.04103660583496 27.9853191375732
-1.2079291343689 1.67965722084045
17.7878742218018 -11.8773565292358
8.17470932006836 4.74312686920166
23.2671184539795 -12.8229236602783
-13.9702968597412 35.6273536682129
21.3211669921875 0.0562910437583923
-3.15136003494263 29.0139083862305
-4.29044485092163 12.0970439910889
-18.2965869903564 21.4790458679199
-20.7178134918213 21.0307598114014
12.5000600814819 -26.0022087097168
-3.97759342193604 0.65451180934906
-37.1902389526367 -29.9105339050293
-0.614866852760315 38.3413276672363
26.0455856323242 -36.2112731933594
-3.81504106521606 -0.615482568740845
-10.0101051330566 27.5527687072754
20.0875282287598 23.5842227935791
12.9075689315796 36.2364616394043
35.0717086791992 6.44754028320312
7.83382511138916 41.0423698425293
-14.0692329406738 35.1920700073242
-38.5198631286621 -23.9899730682373
18.0787601470947 22.4103488922119
10.4377584457397 37.155574798584
-2.75504422187805 1.27761220932007
-21.4998245239258 20.954891204834
-14.8485774993896 17.0104084014893
25.3873615264893 -37.8283042907715
22.1549663543701 -12.5712976455688
-16.0806217193604 33.6327362060547
22.9049263000488 -25.8107490539551
14.9239597320557 -14.2961406707764
19.5485782623291 -13.8513774871826
-33.6657905578613 37.6032791137695
0.135243818163872 -28.8491382598877
19.6488246917725 -6.52411508560181
-38.690731048584 -32.8197479248047
-2.38994121551514 0.0863444805145264
20.7346706390381 0.796860575675964
5.72821140289307 3.96970248222351
19.2614822387695 -10.8233318328857
20.2123203277588 -8.49328136444092
6.59272003173828 39.0204620361328
-3.52548360824585 1.15720641613007
-38.4744720458984 19.043701171875
19.2467842102051 22.3924446105957
-39.0958404541016 -22.7775402069092
28.3949642181396 -13.1157808303833
-14.1654281616211 33.8789482116699
34.4970436096191 5.94020986557007
-7.58522510528564 28.8640575408936
6.08163070678711 4.36036491394043
-3.1760356426239 2.16594457626343
-1.20787084102631 36.6093788146973
17.236743927002 -6.49982500076294
22.4632911682129 -14.1179008483887
-2.19876217842102 0.412787020206451
20.1460990905762 -14.1539039611816
-33.4914474487305 21.7220115661621
30.1826152801514 -13.1030349731445
-12.6542234420776 35.0839309692383
-37.4800796508789 -31.6466007232666
23.4444141387939 -14.6830635070801
0.339959263801575 -12.4741592407227
-10.9408130645752 28.8144073486328
-38.7105865478516 17.324254989624
10.2698793411255 30.5095653533936
34.3160591125488 5.8030309677124
-3.4989070892334 12.5055494308472
25.6208400726318 17.734790802002
21.5344200134277 -25.6712398529053
23.557373046875 18.0886402130127
-2.17640161514282 0.98490297794342
-37.1894645690918 -31.6859188079834
28.0466194152832 -26.5309410095215
-3.97788572311401 11.405725479126
33.5311737060547 36.5021324157715
22.1337223052979 -23.7900390625
24.7118473052979 -25.4927291870117
11.8050966262817 36.9175682067871
-39.0960922241211 -21.4887619018555
11.8567457199097 -26.970890045166
22.9057273864746 -0.261574923992157
18.4921989440918 24.8280754089355
-39.9586067199707 -21.1205101013184
26.5476760864258 -38.493709564209
6.82188749313354 6.95121765136719
-18.1568470001221 21.0603008270264
11.0230379104614 29.3361072540283
-3.80932903289795 29.3326950073242
-14.4740133285522 35.1114501953125
1.07269537448883 -24.1068267822266
-38.6416625976562 -22.3574333190918
-32.5214233398438 35.5301818847656
27.0643787384033 -26.8437366485596
23.3878650665283 18.2713832855225
23.2209815979004 -15.2220859527588
28.4308910369873 -13.4017105102539
17.6195049285889 -4.48567533493042
19.3242626190186 -8.89220428466797
17.5432624816895 -7.18412685394287
-39.9760665893555 -22.816047668457
37.0230522155762 -13.2363958358765
27.0279693603516 -25.5296401977539
24.4796295166016 17.7276306152344
-1.48912525177002 37.6984748840332
-7.21918296813965 16.9375305175781
28.4883499145508 -13.196496963501
22.1109218597412 -0.399479269981384
12.7264223098755 37.8364219665527
1.70789849758148 -13.6209278106689
24.7557964324951 -36.9093589782715
-4.45495796203613 30.9391994476318
14.7248992919922 -25.4820556640625
0.13456703722477 -28.5657901763916
-39.2119407653809 -21.222074508667
20.7353916168213 -15.3161611557007
-0.230206489562988 38.3701133728027
14.0293388366699 -26.1912498474121
7.94122791290283 3.46418237686157
-15.0262117385864 17.5004634857178
33.362434387207 36.5549774169922
34.320140838623 37.3051719665527
26.6905574798584 18.3737335205078
-8.01933479309082 18.9707126617432
34.7725601196289 34.8824272155762
22.353666305542 -25.721227645874
25.9253787994385 -26.7665309906006
15.757532119751 -12.5629034042358
22.4292316436768 -23.4472045898438
-0.042065441608429 -21.1996269226074
36.5985298156738 -14.5242900848389
-4.31544828414917 11.1593008041382
22.7356510162354 -14.5056037902832
19.4701061248779 -8.97716331481934
-15.8397169113159 21.2360534667969
20.7813186645508 -8.52373695373535
-39.0318756103516 -24.0373668670654
-3.65237355232239 0.224089324474335
11.7429609298706 38.5801277160645
20.4296741485596 -12.9437484741211
26.129955291748 -26.0951366424561
27.8871402740479 -26.6022777557373
7.23020935058594 38.7937431335449
-38.8519058227539 -21.0172500610352
24.8313484191895 -37.9127082824707
-14.5112466812134 35.2664031982422
2.54121851921082 -28.427791595459
-3.52689433097839 30.8974208831787
30.8883533477783 35.735538482666
28.7732791900635 -11.7411260604858
-1.38346529006958 1.29447460174561
13.090238571167 37.2421607971191
5.09027290344238 37.2509613037109
33.9190139770508 35.4765625
-38.5222206115723 -30.322509765625
-7.78637266159058 18.7822952270508
22.018102645874 -0.150407806038857
-18.9616012573242 22.9960403442383
29.1911678314209 -12.821343421936
-17.5788803100586 20.91237449646
32.6751823425293 35.4054374694824
18.7282810211182 -6.97226810455322
-1.55796372890472 37.7184448242188
34.6787643432617 35.8463439941406
-12.954686164856 35.1960487365723
5.20793056488037 2.67795372009277
-37.6996650695801 20.9781703948975
13.2749156951904 28.9822120666504
23.2235927581787 -15.0580587387085
20.1288566589355 22.3717842102051
-37.2801055908203 -33.771728515625
-23.8804378509521 20.8914337158203
12.7148637771606 28.878438949585
-3.3818199634552 1.92330086231232
-39.9685287475586 20.3641872406006
36.8404655456543 5.29710102081299
11.5920829772949 -26.204137802124
11.5041646957397 37.8182678222656
21.3706855773926 -14.2110319137573
-39.7940864562988 -21.7021942138672
-39.2519111633301 19.2412891387939
27.9791679382324 -12.6632204055786
11.1852359771729 -28.6144733428955
27.8207931518555 -28.4138927459717
-20.8771286010742 20.142204284668
4.92226314544678 39.2083740234375
19.9692401885986 25.5137481689453
12.368803024292 -25.2165222167969
-5.05930995941162 12.5101184844971
-35.1295127868652 38.2890014648438
-16.1169013977051 18.764123916626
18.9092578887939 -12.151834487915
12.0722093582153 -26.6736106872559
13.319465637207 37.9676322937012
34.7495269775391 -13.2278060913086
-6.23122215270996 10.3791179656982
23.918664932251 18.8613147735596
-16.0097579956055 21.6589527130127
19.670482635498 -2.77069187164307
-32.8522109985352 38.7365188598633
-7.77409410476685 16.7118988037109
17.1928043365479 -5.83386611938477
-15.0419387817383 36.3242301940918
22.9364337921143 -16.4488105773926
-39.3835296630859 -21.7989711761475
36.1740760803223 -15.4961853027344
25.2741928100586 -24.3423881530762
-37.5956077575684 -31.1835880279541
-15.278076171875 17.1571216583252
20.7887439727783 -0.419251948595047
0.326367378234863 39.1586952209473
20.6619167327881 25.5207214355469
35.6806221008301 6.33224153518677
-18.2049541473389 20.7904624938965
22.3225040435791 -14.8827266693115
15.7880926132202 -12.4401264190674
0.197520226240158 -20.585262298584
-0.143794104456902 -28.6682739257812
32.5714645385742 37.4419631958008
32.5782432556152 36.4515151977539
18.1132278442383 -5.91510391235352
-0.616680026054382 -21.6251792907715
-15.2686376571655 35.1133308410645
26.3413696289062 -26.8528175354004
19.6683521270752 -13.9805059432983
33.1870231628418 35.0239677429199
23.602611541748 -25.3444709777832
24.1629219055176 19.0182571411133
27.6365623474121 -27.1394939422607
-40.774772644043 -23.5862197875977
12.2087078094482 37.5040283203125
-4.61584043502808 12.3460931777954
14.0350475311279 -11.3278341293335
0.838772058486938 -21.7975311279297
-37.7741317749023 -33.1586380004883
-34.481330871582 20.1074657440186
28.2830448150635 -27.2302207946777
19.46022605896 20.6806812286377
-33.9158172607422 37.8013038635254
-0.758175849914551 -20.5461711883545
20.913143157959 24.7114181518555
-37.3901824951172 20.6203212738037
6.11786842346191 38.638111114502
-14.6181449890137 36.2976722717285
24.4486694335938 17.5429267883301
-40.2903137207031 -23.3118877410889
0.151555091142654 -29.7611141204834
32.4403076171875 36.6574325561523
17.9932250976562 23.4266777038574
19.6704807281494 0.192966938018799
-15.6488018035889 35.6277313232422
24.7995300292969 16.7693920135498
-15.5136766433716 19.52028465271
-22.0101451873779 19.5826091766357
-22.3519878387451 20.3365287780762
-14.2455720901489 18.5770969390869
-37.8025054931641 -32.9262619018555
-2.89724040031433 28.6768074035645
22.5078811645508 0.222105324268341
-34.3105087280273 20.5872402191162
18.7661437988281 -7.42846250534058
-2.30446004867554 38.844310760498
0.94070690870285 -20.2150211334229
-39.2763595581055 -22.0160675048828
19.4360847473145 -14.9203948974609
-2.67378616333008 29.8741130828857
-40.00146484375 -23.5982570648193
-15.0943536758423 34.887264251709
20.049259185791 -13.168306350708
-18.8958072662354 22.0622749328613
20.3807468414307 -16.0068130493164
12.9704484939575 -27.1844501495361
10.6345081329346 -25.8679866790771
-14.8226251602173 36.4394836425781
-38.9495620727539 -23.3979721069336
18.9148616790771 -8.10581970214844
26.168981552124 -37.4357299804688
-7.95114374160767 27.8343963623047
24.8896045684814 -14.5482702255249
-20.7996253967285 18.183500289917
0.277850717306137 -29.2800807952881
1.8111664056778 -21.075626373291
-6.39511060714722 11.3796453475952
8.78613471984863 3.38420701026917
22.5698585510254 -16.1123199462891
6.24990653991699 38.9954032897949
10.6631364822388 -25.9175910949707
33.2906799316406 6.82254076004028
23.8000774383545 -24.5303211212158
18.1011867523193 23.2570476531982
18.9074440002441 -3.06311416625977
-3.30464935302734 0.977638483047485
-7.74064159393311 19.722843170166
19.7098407745361 -8.54088973999023
-7.48064231872559 18.9390602111816
10.6200685501099 38.2984313964844
-34.0923919677734 19.9641227722168
0.444032430648804 -13.3531732559204
18.5783023834229 -10.1924610137939
-7.15001773834229 18.025899887085
25.3602256774902 -26.5927906036377
-20.8653316497803 18.7721347808838
23.5496387481689 -14.8863382339478
-6.98687267303467 10.7053499221802
30.2155723571777 -12.9241285324097
12.449501991272 36.4238357543945
-34.2390899658203 21.9217224121094
18.2265720367432 -5.0699405670166
-34.9400482177734 20.302225112915
7.93434572219849 5.40009212493896
22.2275104522705 -26.4835834503174
-1.03579652309418 0.840045571327209
26.9451313018799 -27.4701461791992
-2.28674840927124 1.17387163639069
22.720458984375 -26.2566528320312
12.2302942276001 -25.2885360717773
-1.18498146533966 1.46283721923828
5.46853160858154 4.47604370117188
12.7674827575684 27.7871608734131
24.0698909759521 -26.8414459228516
22.8450775146484 0.291127324104309
0.990663409233093 -20.0695610046387
21.8958358764648 -25.1029109954834
11.6786127090454 36.2318496704102
12.8538951873779 37.0038375854492
34.4324493408203 36.7517242431641
11.0478277206421 29.1092338562012
32.6627655029297 37.3232841491699
28.1565418243408 -25.9061813354492
23.2473087310791 -15.543140411377
-3.50454139709473 27.7357482910156
-15.8828010559082 17.5329666137695
31.6259460449219 36.3024520874023
-3.78214740753174 11.8710079193115
26.0258560180664 18.5193004608154
0.465637773275375 -22.6735897064209
27.9281635284424 -26.9077758789062
-6.64481496810913 17.1776790618896
-3.90362358093262 1.82979345321655
17.686164855957 21.5494251251221
-18.5291938781738 20.9062576293945
25.7730236053467 -37.2476615905762
23.6056079864502 -28.6433887481689
27.2857151031494 -28.0998554229736
-6.02029228210449 17.6806945800781
-38.8052215576172 -31.413688659668
35.7533912658691 -12.686598777771
-39.8925170898438 -23.1149368286133
-32.1249313354492 37.8569869995117
-33.6111526489258 21.5662231445312
-4.01228761672974 29.7130527496338
10.9308443069458 38.1666374206543
7.3608193397522 38.8943061828613
-39.6792869567871 19.3600540161133
-0.371935248374939 -11.1329536437988
19.9824619293213 -8.21834278106689
-3.57357287406921 -0.107963085174561
-16.5420513153076 21.3097343444824
-4.07381200790405 30.0918235778809
20.0383205413818 23.5086364746094
23.9175319671631 -36.2181015014648
6.81593799591064 2.92565774917603
-0.521637499332428 -28.3439540863037
16.1991844177246 -10.4106540679932
2.16260457038879 -21.6844043731689
32.8058700561523 35.3329238891602
-34.940258026123 21.2093238830566
23.5277423858643 -23.8140525817871
21.5446128845215 -1.15551209449768
11.6195373535156 30.501335144043
33.2244567871094 36.2130355834961
-0.128409147262573 -12.9810886383057
20.229585647583 22.866870880127
-38.2715682983398 -32.5287055969238
21.6390380859375 -14.1576023101807
7.00098371505737 40.4926261901855
22.6013336181641 0.43294358253479
1.766676902771 -20.9832801818848
-5.30145692825317 27.9123973846436
-0.414720416069031 35.7116203308105
-15.9209241867065 20.647159576416
12.2173919677734 -26.7539329528809
21.210578918457 -13.5952234268188
6.16835117340088 39.6542892456055
-35.8065490722656 20.5762424468994
26.1905956268311 -37.4790687561035
0.382306337356567 -14.0941429138184
2.1888906955719 -12.8700971603394
-32.0342674255371 37.8320083618164
29.3688545227051 -11.2455654144287
25.7390842437744 -38.7042236328125
-39.7082138061523 19.8106365203857
23.743824005127 -14.3295383453369
-1.42308628559113 -27.7868480682373
23.0922660827637 -26.0631484985352
-20.2444076538086 21.5720691680908
5.5955491065979 37.2657470703125
-9.45242118835449 18.0394706726074
20.2977638244629 -12.227222442627
5.2722864151001 5.06988048553467
-1.004350066185 -22.3954219818115
-38.0773849487305 -32.5101776123047
-6.68037033081055 18.4964370727539
13.5542945861816 28.6655158996582
-16.311107635498 16.4841232299805
-4.75185060501099 29.4489593505859
-2.03747463226318 2.12284517288208
37.9156265258789 5.78621292114258
-13.3999099731445 35.2002220153809
-38.975772857666 -22.8411808013916
-0.387591242790222 -20.0335845947266
8.77973461151123 5.31589603424072
12.1536998748779 30.1387157440186
6.12187957763672 39.3044586181641
};


==> figures/visualizations/gmm40/ldvi_samples.tex <==
\addplot [semithick, ldvi, opacity=0.7, mark=*, mark size=3, mark options={solid}, only marks]
table {%
36.0850372314453 -12.3575572967529
-2.87458252906799 37.7732124328613
12.9215507507324 36.6542663574219
-31.2122287750244 39.3140716552734
22.505895614624 -26.5369682312012
-10.2940864562988 29.4578189849854
26.0647773742676 -38.0473937988281
-3.81425499916077 1.58806598186493
36.5086402893066 -10.8411426544189
-22.0914859771729 21.527681350708
-35.2835807800293 20.6337356567383
-39.2092933654785 19.8201122283936
-37.3493003845215 -19.787712097168
-39.9033050537109 -21.8440990447998
-34.0951614379883 38.8757972717285
-38.6204986572266 19.6085815429688
1.656853556633 -27.0916881561279
24.3925399780273 -25.4203109741211
34.3744888305664 36.3700485229492
0.0386395789682865 -21.68310546875
8.41549491882324 2.537193775177
26.0743236541748 -24.2125644683838
-15.6600704193115 34.3001174926758
33.7934951782227 36.1196136474609
34.8829689025879 6.90192651748657
-39.4666442871094 -23.1479434967041
32.4728889465332 36.0933685302734
-15.8565921783447 19.3554439544678
4.46490812301636 4.3477897644043
-32.9000930786133 36.4158592224121
32.5131492614746 38.5852317810059
36.236328125 4.31753587722778
-40.4584617614746 -21.9564456939697
-2.89493346214294 38.0871124267578
12.4636001586914 37.631664276123
28.2364253997803 -36.8822441101074
-38.69873046875 20.5898952484131
6.42367458343506 3.70949578285217
-37.420970916748 -32.9485359191895
-40.3364105224609 -23.2522125244141
-33.2875175476074 20.3271636962891
24.8065586090088 -38.9888877868652
-4.34119606018066 29.9815921783447
-38.139835357666 19.1683921813965
34.8118324279785 5.71935558319092
26.4002017974854 -36.1922035217285
-0.694420456886292 -20.7603187561035
19.503231048584 0.935460209846497
33.9228858947754 37.2379112243652
27.3131561279297 -38.7000694274902
-39.8780937194824 -30.6469631195068
-39.3895988464355 -24.7007102966309
11.1807193756104 37.5503005981445
-36.9679946899414 -32.4553642272949
-3.93340015411377 13.3596668243408
11.480354309082 -24.5368251800537
2.1880886554718 -13.7371644973755
24.193883895874 -36.7368507385254
-37.2986640930176 -31.3588581085205
31.7793731689453 36.3002662658691
-40.5676956176758 -23.2764549255371
35.1834945678711 35.1824073791504
32.714656829834 35.8863067626953
33.6712799072266 37.4764289855957
36.8009147644043 6.90791654586792
1.2589236497879 -12.4869003295898
12.7254762649536 39.0521430969238
-37.2390022277832 -31.6214790344238
-36.6784896850586 22.425313949585
-39.1817054748535 21.381742477417
11.6270799636841 40.1197090148926
0.53007972240448 -22.0524444580078
29.2235164642334 -12.0132741928101
18.4172496795654 -12.8556804656982
26.9492645263672 -37.3338012695312
-5.10423421859741 11.7614879608154
24.6615467071533 -38.5222244262695
-35.099723815918 39.3863334655762
24.1993427276611 -24.5675430297852
36.7429313659668 -12.6568756103516
6.70353317260742 39.4956359863281
31.9274005889893 36.9179000854492
25.0145454406738 -28.2065505981445
3.2981550693512 -12.8485155105591
-39.0248146057129 -21.8608589172363
29.468843460083 -11.7548294067383
-39.4593315124512 -22.6504592895508
25.2703475952148 -37.1397361755371
-13.9142761230469 35.6004867553711
-29.7002868652344 37.7946929931641
-18.7198543548584 22.6572875976562
-13.7817192077637 34.7726783752441
32.188606262207 36.4716377258301
-2.65100479125977 1.33685672283173
-40.1648445129395 -21.980110168457
32.3400039672852 36.4285736083984
34.7428131103516 5.55397510528564
-39.6314468383789 -22.260311126709
-34.1554679870605 38.7358818054199
-1.06560134887695 2.92393088340759
25.6936225891113 -37.4143943786621
-0.301144629716873 -28.3538589477539
32.5042915344238 36.5666885375977
-32.4293441772461 20.1982593536377
35.185230255127 37.3218803405762
20.9880619049072 -7.58107423782349
6.52713584899902 39.565788269043
-34.1025352478027 39.6448554992676
-1.25315451622009 -22.5619049072266
-8.23605632781982 16.7973918914795
11.9432697296143 29.8529357910156
31.9493465423584 34.917797088623
-37.6682586669922 -22.9736557006836
-14.4254884719849 34.8651924133301
31.7137832641602 35.3176536560059
-0.11497001349926 -27.9874286651611
-33.3819046020508 39.4935493469238
24.7809791564941 -24.3439083099365
12.0416851043701 37.0746421813965
-37.1779327392578 -31.9761238098145
31.8717269897461 36.8359565734863
12.676381111145 36.6188278198242
33.0375099182129 37.0303039550781
-38.8029441833496 -20.9207611083984
24.8720283508301 -36.4517974853516
-38.4692764282227 -22.0334377288818
35.2067756652832 6.23703384399414
21.7844524383545 -16.2532062530518
-10.1321067810059 29.2174282073975
32.7673835754395 35.2099380493164
6.51142549514771 4.08749151229858
-39.3952980041504 -23.7556476593018
-38.5420112609863 -32.6454963684082
5.653480052948 3.43937563896179
20.692195892334 -14.4611530303955
-32.9598045349121 21.1729106903076
-1.9160168170929 37.372257232666
10.0184011459351 31.1545219421387
-39.920711517334 -31.5102653503418
28.1048755645752 -13.7282943725586
26.0505199432373 -37.6303901672363
25.1785221099854 -38.2270011901855
26.5961990356445 -36.428596496582
-18.9521713256836 23.3111629486084
17.6386661529541 -5.89907026290894
-33.9456176757812 39.2541694641113
-34.2731475830078 38.0104370117188
2.10671043395996 -19.8458080291748
-0.815190970897675 -21.5119476318359
34.7448959350586 33.7740211486816
11.0567092895508 36.607006072998
2.87234020233154 -14.1630020141602
25.6007289886475 -36.7135276794434
-32.3751907348633 38.1341934204102
-38.3007202148438 -31.7143325805664
33.2863922119141 35.6904602050781
25.4931087493896 -37.8842239379883
32.5584907531738 37.109733581543
-38.2372436523438 -21.8198223114014
9.30308532714844 27.4005661010742
-32.2375259399414 38.664379119873
35.6084442138672 35.5364837646484
25.2351093292236 -36.4297904968262
-36.1512832641602 -31.5146446228027
-0.933183491230011 1.09124648571014
1.13670110702515 -23.4299278259277
-1.27164006233215 -21.9086990356445
24.4926471710205 17.4751739501953
19.7652549743652 -11.7482900619507
-41.4234809875488 19.1598682403564
30.913293838501 35.6854286193848
-32.4787826538086 39.2207679748535
-30.8367233276367 38.6368675231934
18.3188362121582 21.1747245788574
-37.8445053100586 -22.1625728607178
25.320198059082 -25.0083885192871
-38.7742767333984 -32.3905754089355
-36.0773582458496 -31.1148376464844
-7.24744606018066 10.9017658233643
-39.2590751647949 21.5598964691162
-34.7973480224609 21.4116897583008
30.2130069732666 -12.7436590194702
-37.5816879272461 -32.593864440918
33.9767913818359 37.7373733520508
25.0882205963135 -36.7245140075684
-39.8798599243164 -33.4539985656738
-39.942684173584 -22.4673957824707
16.1518630981445 -13.6816701889038
11.2186117172241 28.6984767913818
-39.2398986816406 -20.4341869354248
11.5238637924194 36.2173805236816
-37.1500205993652 -32.3374328613281
-35.9516181945801 38.449779510498
37.085693359375 -10.5672664642334
23.6468200683594 -26.2132225036621
27.226245880127 -36.3712692260742
26.1710052490234 -35.2733192443848
-38.6741676330566 -32.623779296875
34.2184448242188 -12.5198183059692
24.314302444458 -38.757396697998
19.9717807769775 0.0350906886160374
-1.24859535694122 -22.8537425994873
-40.3140983581543 -32.2428283691406
23.4160442352295 -14.0091466903687
-40.0904731750488 -21.8791046142578
32.9980010986328 35.311939239502
-39.1485824584961 -21.1346569061279
31.7108001708984 35.7761993408203
20.0013904571533 22.7305507659912
-3.32213664054871 9.43692207336426
37.3468170166016 5.1076135635376
-40.5003700256348 19.6402359008789
11.6702146530151 37.1189270019531
-39.4052238464355 18.3970050811768
27.5501823425293 -13.152982711792
35.504322052002 5.55165386199951
30.4125442504883 -12.3799247741699
-34.1888084411621 37.448299407959
-3.00677633285522 0.789910912513733
-38.7754974365234 -32.346321105957
32.3952674865723 36.7597351074219
1.71252918243408 -22.6357955932617
-36.9339942932129 -31.7389640808105
25.8422660827637 -36.3941688537598
-29.5631580352783 38.1646423339844
-41.3515472412109 -23.140531539917
24.3888874053955 -37.5473899841309
-34.5273361206055 20.8130512237549
-35.942024230957 -32.2814903259277
26.0653285980225 -37.4921531677246
32.6004180908203 37.053295135498
26.6515083312988 -35.8292617797852
35.5624694824219 7.13008499145508
0.771360099315643 -22.0178146362305
26.7648792266846 -38.0270919799805
21.4130802154541 -0.211598217487335
-32.8372001647949 40.0034980773926
15.264461517334 -11.9991283416748
-39.6665458679199 -34.0549011230469
36.0888900756836 -14.2764444351196
-15.157299041748 36.4550018310547
0.120539419353008 -29.720235824585
-18.8388290405273 21.0972461700439
5.49525499343872 39.096118927002
-37.6927528381348 -30.9392833709717
4.72389888763428 37.9911689758301
-37.3984870910645 -31.6193141937256
27.2076435089111 -25.2943286895752
24.4892311096191 -37.4733276367188
-36.7276268005371 -31.7538394927979
36.0798072814941 -12.5619497299194
26.0477428436279 -36.3884735107422
37.6347694396973 -11.9517908096313
-34.3416633605957 21.2572250366211
33.1853256225586 38.0282897949219
34.1858863830566 -12.7388257980347
33.9255638122559 35.1758728027344
-34.007755279541 22.9970436096191
-39.7210464477539 -21.1113567352295
-38.9223976135254 -21.0802459716797
-7.43750095367432 18.7101860046387
26.3709526062012 -37.9863624572754
-39.803882598877 -32.4591255187988
11.4791526794434 37.8492279052734
-33.080265045166 36.7238006591797
20.6614246368408 -8.56493091583252
9.66021156311035 28.8877372741699
-38.9052429199219 -20.2406883239746
31.8256034851074 36.0047912597656
-39.5373001098633 18.000244140625
-40.1607894897461 -21.5190258026123
-4.68644332885742 12.0124406814575
-38.4117088317871 20.2653141021729
35.9844703674316 5.6530179977417
7.01885414123535 38.0866050720215
5.90549850463867 6.14976072311401
7.87814903259277 4.28214502334595
0.210426956415176 36.3807601928711
27.7800235748291 -37.9545478820801
30.1974334716797 -12.5521488189697
-37.3737754821777 -30.3569965362549
33.4869842529297 34.2751235961914
-39.129566192627 -32.5356369018555
-35.1640243530273 21.984073638916
-40.0920906066895 -31.3702392578125
-16.8770523071289 22.0687942504883
25.6561489105225 -36.4989852905273
21.3728866577148 -1.83458662033081
11.7606735229492 38.1321792602539
-32.8998031616211 37.8880386352539
-7.01436805725098 18.4647407531738
25.4742984771729 18.7291259765625
-39.9678535461426 -31.1952629089355
32.7003135681152 35.6312675476074
-34.6697616577148 37.4504127502441
-4.70385456085205 28.7405261993408
18.234712600708 23.9999351501465
0.647887170314789 -30.0172901153564
-0.905862092971802 -27.5238456726074
10.8058605194092 28.4057712554932
28.9566841125488 -12.4197597503662
-39.7913436889648 -21.0091438293457
26.9889507293701 -13.4225406646729
-37.8433456420898 -23.6792945861816
-34.2204666137695 21.5498905181885
36.2188377380371 6.80507850646973
0.338419228792191 36.9462928771973
-33.1544647216797 35.1810874938965
33.9679107666016 2.6708824634552
35.0113182067871 -12.1997318267822
31.4015102386475 36.6573295593262
31.7231674194336 37.0147171020508
35.1324882507324 -11.071982383728
-13.9538192749023 34.7969932556152
-32.4302864074707 38.3912239074707
21.3422603607178 -15.8423223495483
32.782356262207 36.1717643737793
-39.7843055725098 -21.5553646087646
35.0123252868652 4.66785144805908
22.2939929962158 -14.4260606765747
32.2568092346191 35.5736427307129
22.8706474304199 -25.7597904205322
1.47433865070343 -22.5317649841309
-3.40768575668335 29.5726585388184
-37.2709045410156 -21.8896903991699
-39.3863487243652 -30.6221046447754
-39.2052803039551 20.495885848999
-36.6386070251465 -23.1054439544678
18.8572978973389 23.2064914703369
-32.0434532165527 38.7839317321777
12.4401206970215 38.3902206420898
22.4821624755859 -26.2445850372314
-38.9828147888184 19.2477188110352
-2.39018225669861 28.8917350769043
26.6448001861572 -38.7655296325684
-37.7745361328125 -22.4544525146484
-35.7467460632324 20.9880046844482
23.875036239624 -38.2704200744629
29.3635215759277 -27.2639541625977
26.5995864868164 -37.1640472412109
-39.7538185119629 -21.8638477325439
-32.1642379760742 37.5410003662109
-37.2166633605957 -31.5287780761719
-39.2168960571289 -32.8068618774414
0.575997471809387 -29.8159141540527
-40.4140853881836 18.8271560668945
6.66437864303589 5.40058422088623
-38.9895973205566 17.2864036560059
-17.1102275848389 20.2009410858154
11.1684856414795 35.893669128418
-39.0507011413574 -24.228796005249
31.1039848327637 -11.5271558761597
26.3061771392822 -36.5268402099609
26.0255546569824 -36.812442779541
33.1192665100098 36.7259368896484
4.90696430206299 40.4710578918457
34.5720596313477 35.9751205444336
-40.7312774658203 -22.7134819030762
33.8622894287109 35.5941581726074
-37.6395111083984 -30.6037998199463
33.0844535827637 35.8074722290039
-39.3747596740723 -21.7696304321289
36.3002471923828 -12.5394487380981
-18.8795890808105 21.3155269622803
-39.4873733520508 19.9833240509033
11.4193773269653 38.8892631530762
-34.277530670166 36.3392906188965
27.1126899719238 -11.436861038208
19.1291313171387 0.391778171062469
32.9746589660645 34.6074638366699
-38.7229270935059 20.5479679107666
32.8452911376953 34.3284759521484
34.4223899841309 37.9266662597656
-0.0650992691516876 -10.9655179977417
-38.901180267334 -31.5445766448975
-2.85734701156616 1.67920875549316
-14.4108695983887 18.093189239502
-37.7718086242676 -21.2287845611572
-33.6380805969238 24.2361793518066
7.32539987564087 4.37683248519897
6.79935455322266 4.68600368499756
34.1221084594727 37.9093208312988
-40.5230255126953 -22.7118148803711
-22.5346755981445 21.9343662261963
-38.6624183654785 -21.1900844573975
-15.1137113571167 16.2646331787109
-39.4937973022461 -20.3858547210693
-37.3967247009277 -32.6486511230469
11.2119674682617 35.5607490539551
-4.20652341842651 10.0636434555054
35.2197074890137 -12.7850847244263
-0.374682813882828 -13.6187677383423
35.5954360961914 -13.7427568435669
25.6695613861084 -27.448112487793
-34.9171752929688 22.1664752960205
-33.6380271911621 22.3639545440674
23.4771537780762 -0.923904955387115
-37.5732841491699 -31.8665332794189
7.15310716629028 38.7207679748535
-39.1854286193848 -30.7357540130615
1.04011142253876 -30.5484218597412
10.8487815856934 29.3184280395508
-38.8735198974609 -32.0663375854492
-39.3239479064941 -21.257926940918
-38.6474761962891 18.5819149017334
-1.14215636253357 -22.0068378448486
25.8362579345703 -37.2253799438477
33.9142646789551 36.3685417175293
0.592105209827423 -27.4682903289795
18.3791580200195 -0.1877531260252
22.7525463104248 -26.4306964874268
32.9709396362305 37.9144821166992
-37.6920700073242 -21.2070846557617
-37.8965530395508 -31.8808326721191
35.9606246948242 6.46202850341797
-34.6892356872559 21.5983028411865
-17.0515232086182 21.2242050170898
-1.3011668920517 -28.7739372253418
-40.4613990783691 -23.4595928192139
-39.0870780944824 17.5462284088135
37.0543403625488 6.27979230880737
35.4582328796387 35.6414413452148
-32.1699447631836 39.3899421691895
12.8726644515991 40.9283714294434
24.6670894622803 18.3866119384766
-37.8131103515625 -30.6485652923584
24.0149116516113 -26.4981899261475
18.9887390136719 21.4271240234375
-14.5436067581177 18.1248474121094
35.420093536377 4.99412155151367
22.4957675933838 0.825825214385986
13.4519596099854 38.6263771057129
-0.701957106590271 -28.8000793457031
26.1942005157471 -36.9520683288574
35.0511436462402 34.5422515869141
34.1281394958496 6.9248161315918
12.1236371994019 26.8441486358643
25.2912673950195 -37.3484954833984
5.06171226501465 38.6801643371582
6.62603330612183 38.6435623168945
27.1052474975586 -11.9200038909912
27.418140411377 -26.5374698638916
20.836254119873 -23.5862693786621
30.0352516174316 -14.3121366500854
-36.1232223510742 -32.6193771362305
16.0938205718994 -11.4417905807495
21.6638278961182 -26.3966636657715
-32.54833984375 39.4322776794434
-38.5180816650391 -31.1674537658691
-40.5984992980957 -21.1558284759521
6.52445602416992 38.2089614868164
-38.3350944519043 -32.0127449035645
-36.2532615661621 -31.5391254425049
10.8362894058228 27.439359664917
26.8308715820312 -37.3601531982422
12.4559602737427 37.0034980773926
-33.925350189209 37.6007347106934
31.2935199737549 35.1214370727539
9.48355579376221 37.4729118347168
-38.2812385559082 -33.6462783813477
-33.9861640930176 38.6817016601562
24.0470943450928 -25.574535369873
-38.6401824951172 -22.8228874206543
-34.5775985717773 22.8656272888184
29.8391571044922 -12.3990850448608
-37.6733589172363 -31.9091968536377
-38.3495483398438 -32.4366912841797
-34.621036529541 36.9536170959473
-39.0118370056152 -32.2030067443848
26.9555320739746 -37.2994041442871
27.0707092285156 -37.6889228820801
-39.2374153137207 -22.5536708831787
11.4425554275513 36.6707077026367
-0.526602327823639 -28.8060874938965
21.9913806915283 -26.6949596405029
13.7326698303223 38.2602272033691
-1.80524146556854 38.026050567627
-36.6267280578613 -34.1469116210938
25.5038719177246 19.3289813995361
-32.2941246032715 36.4214286804199
-11.5336389541626 26.3919734954834
34.7123069763184 34.7371253967285
34.8750343322754 6.17435789108276
-38.3464851379395 -21.8017292022705
6.53966331481934 40.5118217468262
24.3371505737305 -37.9432182312012
-1.44726312160492 0.189252570271492
-36.9119186401367 -31.1576404571533
36.0211791992188 5.39154529571533
26.5936717987061 -37.833438873291
-35.7279205322266 21.6834335327148
-32.0866584777832 38.3902282714844
26.2809352874756 -35.7087860107422
36.7149696350098 -14.2542905807495
-34.3310508728027 38.0057220458984
-31.5429553985596 37.8202362060547
-38.838020324707 -31.6695995330811
-38.4839935302734 -22.960636138916
34.6250152587891 -13.5464181900024
33.1370239257812 35.2592163085938
0.198513120412827 -27.1913394927979
-37.5603828430176 -29.7909851074219
-38.3640632629395 19.9004058837891
-2.27367663383484 38.583381652832
35.635124206543 -12.7870635986328
26.2358055114746 -37.2474594116211
6.9995551109314 38.7708282470703
-36.8975677490234 19.2842483520508
26.5473937988281 -35.9674110412598
-39.9759750366211 -22.7535514831543
-36.3861122131348 -32.2646598815918
-14.1468486785889 35.2371673583984
34.6468734741211 36.232982635498
25.8532485961914 -36.7637634277344
-35.4980888366699 19.5740165710449
21.4545516967773 -1.94506704807281
-37.7547454833984 -32.4234161376953
23.0829257965088 -26.3470249176025
-36.6023330688477 18.7902336120605
23.2595882415771 -25.4990253448486
-31.5616912841797 37.0369758605957
-37.3439292907715 -31.9026508331299
-38.4916954040527 -31.168514251709
24.0605792999268 -35.3221321105957
-39.5287246704102 -23.2325000762939
0.222330197691917 -20.7399406433105
-31.2578201293945 38.8820419311523
25.8910484313965 -34.8624229431152
-33.4157104492188 38.0624351501465
-6.69664335250854 18.2025756835938
25.6534538269043 -36.819263458252
26.5506153106689 -37.2242126464844
36.3791656494141 5.27920961380005
6.64095544815063 5.45775127410889
34.1032524108887 34.7899475097656
-38.3826942443848 -32.0359687805176
-35.3888130187988 -31.3698329925537
-39.4578590393066 -20.2026252746582
-32.2218017578125 39.4769096374512
37.2311935424805 4.62259197235107
1.22480702400208 -11.3470964431763
-37.7606048583984 -30.4495506286621
22.4356575012207 -15.1626710891724
31.982234954834 37.8788566589355
17.4326229095459 -5.43412590026855
-2.83773970603943 -0.140653133392334
-39.1760063171387 -30.060583114624
25.7294731140137 18.02197265625
35.7761764526367 6.96326494216919
-0.989906251430511 -28.943395614624
34.0610656738281 37.4104614257812
24.6298713684082 -38.8221817016602
25.8246402740479 -36.9527397155762
25.2315502166748 -37.8597564697266
-34.4199562072754 37.7819557189941
-39.3324775695801 -23.9359760284424
-36.8271446228027 -32.4220771789551
-32.7767677307129 38.5273857116699
-16.4322376251221 18.1574535369873
26.5870666503906 -35.0223236083984
36.0493469238281 -11.1180305480957
-34.8455352783203 23.2002468109131
-4.13183975219727 29.4562473297119
34.0936088562012 35.7545852661133
-34.7076568603516 21.6974334716797
-32.0239410400391 40.5068740844727
-40.0448379516602 -23.1093769073486
-33.9195976257324 37.3015251159668
6.22794437408447 38.0080642700195
-40.5364189147949 -22.2396831512451
22.1789531707764 0.156253501772881
-35.6179237365723 21.7138900756836
-14.8456544876099 34.7162246704102
-40.9004898071289 18.4169273376465
-36.792594909668 18.9204044342041
19.8246154785156 -2.09123659133911
-0.843014240264893 39.0024185180664
-37.3305854797363 -23.1449565887451
-38.6633071899414 19.507719039917
-38.1250648498535 -31.5900974273682
35.8213653564453 -10.7940692901611
-2.70250129699707 31.211109161377
-38.2991371154785 -31.2849540710449
-36.4284172058105 -31.2190570831299
-32.2118110656738 39.6587944030762
35.7257766723633 6.06637573242188
36.0667724609375 5.26570844650269
6.82352209091187 3.39330244064331
-39.9515724182129 20.6175556182861
-37.6530113220215 19.8200397491455
33.1782493591309 36.1750564575195
34.0740737915039 38.1010627746582
-16.1734981536865 18.5389308929443
36.8205795288086 5.92798042297363
-32.2731857299805 39.5205459594727
25.4469814300537 -37.0757598876953
36.8845634460449 5.73860502243042
-39.898551940918 -23.3358039855957
27.0597515106201 -36.7758445739746
-2.19258284568787 38.0657691955566
-38.3047561645508 -32.0987014770508
-31.9354381561279 37.1162300109863
-0.354386538267136 -28.5933418273926
-40.2395172119141 -23.4764823913574
-34.3347091674805 22.6622562408447
26.2793292999268 -36.4201736450195
-40.1915245056152 -24.8779640197754
22.4327011108398 -14.9558086395264
33.2078895568848 35.6224060058594
26.2395515441895 -39.2911415100098
26.3220520019531 -35.5211067199707
-37.2031097412109 -30.9213714599609
36.3451080322266 6.14820194244385
1.84328806400299 -20.860279083252
-38.8959045410156 -33.9863014221191
0.757427632808685 -29.370698928833
27.8859825134277 -37.9379119873047
24.4590320587158 -13.3477373123169
-39.1655349731445 -31.7205028533936
32.3391761779785 35.083812713623
-7.73801183700562 18.7062835693359
-1.14378309249878 37.7204551696777
-18.0429725646973 21.1172847747803
36.266185760498 6.47396802902222
0.614197075366974 -20.2683773040771
10.9893159866333 38.7295455932617
-40.4925422668457 -33.468017578125
-14.45751953125 35.4731483459473
-33.3098297119141 38.3506507873535
-32.9130935668945 38.224235534668
24.2607688903809 -36.2775535583496
32.941219329834 38.2922821044922
35.8148612976074 7.20971202850342
26.9771194458008 -24.4389915466309
6.30018663406372 37.7932929992676
33.0732307434082 37.5158615112305
12.2413711547852 -26.4547443389893
-38.9571723937988 18.7639350891113
-31.7826271057129 38.7947044372559
33.8504753112793 35.8193206787109
35.6109275817871 -13.7471618652344
-40.384952545166 -24.560432434082
-39.4240074157715 -32.1749382019043
-38.6179695129395 -21.5893802642822
0.330552726984024 -29.7484855651855
27.7619934082031 -37.5623893737793
34.4225654602051 -12.8371248245239
-1.18727707862854 -28.6051959991455
7.64916706085205 4.44078826904297
-38.1900825500488 -21.9681873321533
0.825831413269043 -13.1255531311035
-38.2795677185059 -32.4691467285156
25.5160179138184 -34.2588729858398
-37.2437705993652 -31.893575668335
-17.9478378295898 21.4494609832764
2.67035150527954 -21.5589981079102
27.4891796112061 -12.5592203140259
-38.6362609863281 -30.6649684906006
27.2354125976562 -38.6263999938965
-39.3972969055176 19.5316829681396
0.281303972005844 -27.8680744171143
-39.2239685058594 -32.7623748779297
7.92518949508667 4.69046401977539
-34.7606086730957 38.0763397216797
-39.3539276123047 -21.2208118438721
24.2944889068604 -36.3718643188477
-34.8355941772461 20.9744777679443
-18.9132499694824 20.7453155517578
-1.25450563430786 39.4758224487305
-3.33061408996582 38.8149681091309
20.3907299041748 23.8216209411621
37.1179428100586 -12.1755046844482
-37.8879661560059 -32.4487571716309
-12.4730291366577 35.226749420166
33.7660980224609 37.4546279907227
26.56005859375 -36.232723236084
-33.3069229125977 36.9493827819824
34.1752548217773 5.98230695724487
-15.1914653778076 18.5291366577148
11.0951328277588 39.0721740722656
-36.3523216247559 20.3847503662109
11.6902694702148 29.5212574005127
37.0352439880371 -14.0160236358643
27.5766048431396 -38.8412933349609
35.950065612793 4.75657939910889
-31.7261867523193 37.3673553466797
-32.6553993225098 38.2489395141602
32.274356842041 37.0003051757812
34.2437133789062 35.5369453430176
-34.1947135925293 23.19606590271
-31.8520736694336 36.9211349487305
34.7562866210938 35.9871139526367
-37.3842468261719 -31.6255207061768
-38.3372383117676 -21.5995140075684
15.3873605728149 -13.2141046524048
-0.124550066888332 -28.0566291809082
-0.130790084600449 0.109537787735462
34.7327308654785 -11.6927661895752
-40.6311492919922 -31.8513622283936
-31.6810722351074 37.9465484619141
-1.73250138759613 -28.2089653015137
17.4530162811279 -13.6310520172119
-37.8423385620117 -31.2955226898193
34.9247779846191 6.77675867080688
-34.1081848144531 21.4756507873535
-33.2982177734375 20.4518604278564
-39.862003326416 20.7519073486328
13.4417905807495 -28.071647644043
33.6756935119629 35.4098205566406
31.2474746704102 33.6500511169434
35.9847259521484 -13.9300994873047
35.7485008239746 -13.8183336257935
11.4066791534424 38.538688659668
27.5852661132812 -11.3108825683594
33.8223304748535 -11.7546405792236
-40.5385284423828 -29.4913520812988
20.962776184082 -0.537841141223907
33.7818031311035 34.7115821838379
25.1019897460938 -36.2693023681641
-33.2189903259277 39.065113067627
12.0099420547485 39.2065925598145
35.2754898071289 -14.0653047561646
0.681269228458405 -21.7133483886719
-38.1488609313965 -31.1960334777832
12.8820247650146 38.1182098388672
20.1299686431885 -13.7508115768433
27.7427501678467 -37.7757759094238
34.9996681213379 35.3461875915527
27.4864311218262 -13.2073764801025
32.9803810119629 36.3886871337891
-0.598915636539459 38.9416847229004
18.3967838287354 -8.5067310333252
32.8136863708496 35.9449195861816
27.2164669036865 -36.1744003295898
-38.6405982971191 20.5815563201904
32.382640838623 38.7638549804688
35.2001762390137 7.45471906661987
-37.9100494384766 21.7344150543213
24.610200881958 -38.4804573059082
-31.2509384155273 38.9902687072754
26.2503223419189 -37.750072479248
0.270647317171097 -12.0385265350342
-32.0082626342773 38.7563400268555
34.5087585449219 6.03354978561401
12.6216249465942 36.5454063415527
6.76841926574707 39.3622131347656
-39.4032936096191 -23.8405647277832
27.0035858154297 -36.2545509338379
6.67860746383667 39.75537109375
31.5908355712891 35.9902534484863
-32.808837890625 38.1012191772461
37.1627235412598 -13.6754703521729
-39.5742874145508 16.5904979705811
-35.9705848693848 18.4914703369141
-38.7849197387695 -33.2822341918945
-14.3875255584717 38.2278060913086
36.6174583435059 4.77901601791382
-39.9605140686035 -21.7705307006836
35.4319953918457 5.37941122055054
15.8100967407227 -10.7622556686401
-38.6319351196289 20.6527900695801
21.8512172698975 -25.595645904541
0.182695254683495 -29.3798694610596
10.390585899353 28.3036479949951
-37.6078338623047 -31.5266532897949
-33.3160400390625 39.1406669616699
-38.4669914245605 -21.9106845855713
-39.4211807250977 -33.2282409667969
26.6269092559814 -36.7384948730469
11.583740234375 28.8818759918213
5.71560764312744 36.9369964599609
-39.7691078186035 -23.4748191833496
21.5068950653076 0.46102574467659
35.7920455932617 -14.2238512039185
-3.94111108779907 -0.119840152561665
22.1325054168701 -15.1035089492798
24.169620513916 -14.153112411499
29.0773639678955 -27.7855949401855
9.05287647247314 38.3357925415039
6.49414539337158 3.43804717063904
-38.0564384460449 -30.9667472839355
-22.1507301330566 19.2434978485107
7.82916116714478 39.3365745544434
34.9864120483398 6.72580099105835
33.334415435791 35.3736419677734
5.72791481018066 40.008975982666
-40.0082015991211 -19.9168186187744
35.8229217529297 6.46358633041382
-39.6613235473633 -34.4519195556641
-8.23422241210938 28.2147979736328
33.6452865600586 35.9022216796875
33.9474868774414 36.3035011291504
33.8750991821289 36.3825340270996
26.7685298919678 -36.0970001220703
37.4069786071777 -10.4475889205933
26.2437343597412 -35.3732032775879
26.2701110839844 -25.54248046875
36.0494575500488 5.28740262985229
36.1260223388672 5.05601024627686
34.6497497558594 6.7612943649292
-39.4994125366211 -31.6022987365723
-38.1328468322754 19.8788642883301
-31.9298706054688 38.6094131469727
25.0106315612793 18.9002590179443
25.203462600708 -25.0065059661865
-36.1365852355957 -30.9362716674805
-36.4814643859863 -32.5650596618652
-8.54632377624512 15.8577175140381
36.6198768615723 -13.5307159423828
-38.8829917907715 -32.7899742126465
25.7612266540527 -35.6115112304688
30.060417175293 -11.2322940826416
36.4885559082031 6.55558490753174
-12.9755802154541 35.5308876037598
-38.9216537475586 -23.0659275054932
-19.3023300170898 19.7181587219238
25.4477825164795 -35.7787780761719
-39.0431518554688 20.0474128723145
35.5955924987793 4.86476850509644
-38.823169708252 -32.7533836364746
-38.8720893859863 -33.0417938232422
-20.697286605835 20.855224609375
-37.9840965270996 -31.6307640075684
-0.253666162490845 -27.853307723999
33.8620719909668 35.458137512207
-1.18844783306122 -30.2366962432861
29.7756690979004 -13.1230401992798
31.763053894043 36.3474617004395
-1.48279213905334 37.41796875
34.587833404541 6.10848903656006
-38.5597610473633 -21.5817108154297
34.1748542785645 5.15072202682495
-30.3011932373047 37.0033721923828
26.0092926025391 -36.8526878356934
-40.0913619995117 -23.1625499725342
36.0038414001465 -11.5360689163208
27.244535446167 -37.2363128662109
-40.7653656005859 -22.4983062744141
-14.0656852722168 34.6724586486816
13.9803400039673 -26.5063076019287
34.6104049682617 -12.0279865264893
-17.0674476623535 22.5005779266357
-38.3333129882812 -32.9004058837891
-40.2353858947754 -23.1749458312988
27.4528980255127 -37.170768737793
33.7885246276855 36.570987701416
-33.1168327331543 38.8959579467773
-32.2739906311035 38.0660858154297
34.3484535217285 35.8858222961426
-39.5823173522949 -31.0626792907715
26.7684478759766 -36.5243148803711
19.5688934326172 21.617467880249
-34.4478607177734 22.0570316314697
-15.3091249465942 36.0518188476562
19.6230316162109 -8.8629789352417
26.7205009460449 -23.3936424255371
32.3770599365234 39.2147789001465
-37.7740592956543 -31.6218948364258
23.4419059753418 17.0948009490967
21.9527492523193 -25.5898494720459
34.2153739929199 5.75712585449219
-30.4057674407959 38.3477745056152
29.8014163970947 -14.5363206863403
31.4795246124268 35.0762176513672
7.41063451766968 38.0415687561035
0.0130492001771927 -21.1680068969727
1.64865815639496 -12.8273315429688
-38.6681632995605 -31.915563583374
-38.2655792236328 -32.331657409668
33.7302551269531 36.2213287353516
-38.3709030151367 -22.7231559753418
-0.615975618362427 -26.5038452148438
34.4709014892578 35.2363815307617
26.9955539703369 -37.6647644042969
-38.5077857971191 20.3733158111572
-38.8234443664551 19.3388290405273
-39.7816734313965 -22.3516273498535
-35.2687873840332 20.4111022949219
35.6415138244629 35.4467124938965
27.2356777191162 -36.7600631713867
21.5725841522217 -26.3668117523193
25.4418754577637 -36.3950462341309
32.6752853393555 35.2940711975098
-4.03402805328369 31.5108184814453
-32.7887115478516 36.2092514038086
-39.426944732666 -30.9778823852539
34.1437149047852 35.173511505127
24.8045806884766 -35.9929618835449
19.7896957397461 -8.27822875976562
25.180908203125 -38.2510604858398
31.1150989532471 34.7955093383789
-1.60612177848816 1.13977515697479
-40.421802520752 -30.5343780517578
35.8626403808594 34.6441383361816
6.90208005905151 40.3795776367188
-0.0281584970653057 -21.4171371459961
25.5474052429199 -37.6773262023926
26.1738986968994 -36.8134689331055
34.0108070373535 36.6839332580566
26.0446548461914 -40.4117317199707
1.92879438400269 -22.937198638916
0.686660587787628 -28.0293674468994
-37.0231513977051 -33.0316925048828
-5.73676204681396 11.4909315109253
-37.9662437438965 18.9754829406738
26.2055149078369 -37.7587509155273
5.30916118621826 40.4878158569336
37.079216003418 -11.9207563400269
-32.1460723876953 36.9613876342773
-40.2782020568848 -20.2601737976074
2.93706393241882 -11.1770401000977
-39.000301361084 -32.563835144043
4.74860334396362 37.8529586791992
-38.2737083435059 18.8153038024902
32.4378776550293 36.6308135986328
12.8901071548462 28.1548099517822
-33.3952331542969 39.3305816650391
24.9341335296631 -25.9455871582031
9.21288776397705 37.4395523071289
-0.851588189601898 2.91985487937927
-38.6547927856445 18.308313369751
33.3469390869141 37.5759391784668
34.2235641479492 35.4331359863281
-1.71979868412018 27.2999134063721
18.6960029602051 -13.5730247497559
-36.0718231201172 21.5945453643799
-34.6412620544434 23.666841506958
20.6105995178223 -13.49476146698
-38.3074111938477 18.5157222747803
27.5143928527832 -36.5177879333496
-33.8964195251465 22.3640384674072
-33.0556869506836 39.855842590332
33.2117233276367 36.2625312805176
34.7827186584473 36.0113792419434
34.7810478210449 35.8199005126953
13.111138343811 26.6802444458008
25.7672290802002 -37.4237670898438
29.3589611053467 -26.6802959442139
-37.9147911071777 20.4700031280518
33.8325843811035 35.9200172424316
35.2039947509766 7.19390678405762
-36.3455810546875 -31.8600425720215
31.5243053436279 36.8344383239746
1.87563252449036 -27.3512439727783
33.8422203063965 36.6416130065918
25.256217956543 -36.8712425231934
-14.3100500106812 35.965633392334
24.5864028930664 -36.9823265075684
1.29886794090271 -24.2599792480469
-37.947452545166 -20.7703094482422
29.0723896026611 -37.3081817626953
34.7781791687012 37.0243911743164
-37.0446166992188 -32.4671401977539
-39.1035766601562 -30.9759120941162
27.2188262939453 -34.8588790893555
-36.9768753051758 -33.6928367614746
-38.5083999633789 -21.0808525085449
32.6852607727051 37.0923309326172
-37.3170623779297 -30.7721557617188
-3.38456654548645 1.48078107833862
-40.1400299072266 19.4873237609863
32.3259811401367 35.9457511901855
-34.8644218444824 21.9338512420654
31.4756965637207 37.4629707336426
27.8569946289062 -36.267276763916
25.2427616119385 -36.8367195129395
25.2687473297119 -35.8823852539062
27.6941318511963 -11.7167072296143
-38.345832824707 -29.67919921875
-34.3032569885254 37.1415405273438
-38.8604125976562 -32.3179512023926
32.0996627807617 34.6202545166016
27.9875354766846 -26.7516937255859
-33.8191223144531 37.4480476379395
33.7674827575684 4.67228174209595
5.12991189956665 37.548713684082
-39.781192779541 -22.6463947296143
-38.2413940429688 -32.6733016967773
5.694007396698 38.9596405029297
28.1942157745361 -13.6721897125244
-34.4727592468262 22.8413581848145
22.5550727844238 -13.8223342895508
-33.3176155090332 37.1579704284668
34.6020698547363 -11.3797922134399
-5.95891666412354 11.030858039856
27.0304851531982 -37.8793830871582
10.9240112304688 38.8792457580566
-0.767066121101379 -21.0124607086182
36.7379722595215 4.92467451095581
35.8698196411133 6.16882181167603
-3.52670454978943 29.1705589294434
-34.6178398132324 40.143424987793
24.5919628143311 -26.6599426269531
32.6308784484863 33.7243385314941
31.5507259368896 36.6786460876465
-33.926456451416 38.6167526245117
35.0313911437988 38.7462768554688
-9.13497829437256 28.8087043762207
-31.0839900970459 39.4068832397461
24.3516883850098 -36.9302062988281
};

==> figures/visualizations/gmm40/mcd_samples.tex <==
\addplot [semithick, mcd, opacity=0.7, mark=*, mark size=3, mark options={solid}, only marks]
table {%
10.669563293457 -25.5463047027588
33.1358604431152 35.3659439086914
-21.3505420684814 20.7217559814453
27.0990562438965 -36.1786499023438
-37.0961990356445 19.8731002807617
25.7139663696289 -34.2931671142578
-1.10044932365417 -27.8666648864746
25.5971431732178 -37.0435256958008
34.5354385375977 36.9096527099609
34.0789070129395 36.1234512329102
-39.4056243896484 -21.3806819915771
36.6516761779785 -12.6046657562256
-0.91810804605484 -26.8798313140869
-38.6190452575684 -32.8938789367676
33.566349029541 36.5668869018555
31.9366321563721 36.3267097473145
-34.3513298034668 37.2023887634277
-20.9646701812744 20.0264415740967
-38.6777114868164 -29.6180191040039
26.8254776000977 -38.1414756774902
-39.2881774902344 -32.2817344665527
27.2916564941406 -36.7037811279297
34.7604484558105 -11.7991123199463
-15.5876779556274 35.5999794006348
34.8603973388672 4.52835083007812
-37.3973922729492 -31.6914119720459
35.4065322875977 -12.8844985961914
-38.5038833618164 -32.1268348693848
6.71617317199707 5.32661628723145
32.8337326049805 37.1289520263672
18.8093719482422 23.2153377532959
32.7510414123535 36.1526794433594
-32.0871887207031 37.1993827819824
-2.57723546028137 29.266622543335
-38.3282623291016 -31.56911277771
-6.95989608764648 18.9873046875
25.1548900604248 -36.6198463439941
-39.2862129211426 18.7661800384521
-0.0200121402740479 38.2806091308594
31.3286304473877 35.1197395324707
0.910319328308105 -21.0466423034668
-33.139705657959 39.1962928771973
-38.3180923461914 -22.2640323638916
-37.8044242858887 -31.8424510955811
22.1099662780762 -15.1797943115234
35.1930465698242 35.2770156860352
36.1391906738281 -13.7653179168701
1.27264511585236 -28.3771286010742
-37.4643287658691 -31.6998310089111
-15.4683046340942 36.4679718017578
35.6318550109863 8.2602596282959
26.2919769287109 -37.9271469116211
-33.3254661560059 37.6635856628418
-7.42753839492798 18.993127822876
-38.425365447998 -31.093620300293
-0.391936928033829 -26.2632789611816
-38.2976455688477 -33.3085670471191
0.389182686805725 -21.4363975524902
-39.8429832458496 -32.9345626831055
-0.625522375106812 38.4789085388184
-0.933266878128052 -26.4841918945312
-34.6039924621582 36.925422668457
35.40283203125 7.38572454452515
-39.7019500732422 17.8059558868408
-0.78305721282959 -28.2289390563965
34.679084777832 38.2129211425781
25.915319442749 -35.6322975158691
12.9959516525269 -25.6611766815186
25.8231048583984 -36.4941902160645
25.7746925354004 -37.5461654663086
-38.5195198059082 -33.1499824523926
34.7723655700684 35.7792739868164
-39.5150299072266 -32.3485527038574
-37.852165222168 -35.007495880127
-38.4306373596191 -32.0216407775879
-34.492015838623 21.1554298400879
-8.39978504180908 27.7908306121826
-34.0742797851562 39.4681777954102
-37.1527633666992 -21.0515232086182
-32.7574691772461 36.8453788757324
34.818058013916 6.52166366577148
32.3531799316406 35.3934516906738
28.9654064178467 -13.7422819137573
-34.5961875915527 37.5324020385742
36.2013053894043 5.20589685440063
4.12778806686401 38.6398773193359
32.6053771972656 36.2171249389648
25.329288482666 -38.1453018188477
-7.94641923904419 27.2611446380615
34.0676231384277 -11.9990673065186
-34.0077972412109 37.0910720825195
-38.8653793334961 -30.8826332092285
35.1173896789551 -13.1081390380859
33.1993980407715 37.2692108154297
-4.84548282623291 2.31943106651306
33.9356307983398 36.1566200256348
-38.18017578125 22.4581108093262
-38.802677154541 -31.411247253418
28.8503971099854 -28.1757926940918
-36.2661476135254 20.7859706878662
29.0185375213623 -12.3753395080566
16.8088703155518 -6.46027183532715
36.3904991149902 7.94476413726807
6.89426183700562 38.8743438720703
26.593225479126 -37.7251510620117
27.447473526001 -12.6708269119263
35.7148933410645 -13.1442842483521
35.4342155456543 5.79959535598755
15.2051372528076 -11.8315391540527
28.4974613189697 -11.6942367553711
-2.35316181182861 38.0655708312988
30.5212478637695 36.1917114257812
-37.5032997131348 -20.7891292572021
35.3822212219238 6.7819299697876
34.8883781433105 -12.0890769958496
-39.049976348877 -21.6264896392822
10.0666694641113 36.3032608032227
-35.1255645751953 -31.8497753143311
-14.1630954742432 35.4425430297852
33.6037712097168 34.2932205200195
22.2211971282959 21.3198947906494
-39.1924247741699 -30.9486064910889
-39.5752067565918 -24.0761604309082
-9.04433917999268 17.6540622711182
-37.2447814941406 -32.2995185852051
-39.581901550293 -20.253490447998
-5.19837713241577 10.8366708755493
32.3230895996094 36.0441246032715
-39.1034049987793 20.24631690979
-38.7728157043457 -31.5453186035156
37.9046211242676 5.48398017883301
0.65319412946701 -29.4255046844482
-4.83001089096069 12.5556240081787
-38.3859558105469 -32.8269882202148
-34.1991729736328 37.4590301513672
32.1641960144043 35.5827674865723
26.3553695678711 -36.1371459960938
36.8584976196289 -13.5220956802368
21.1484661102295 -9.16287136077881
19.1592559814453 24.3627033233643
32.8032035827637 34.9908142089844
-31.2008438110352 40.8107070922852
-39.6705436706543 -32.3818054199219
35.8383598327637 -11.4082069396973
2.88322353363037 -13.175332069397
-37.99462890625 -24.3289108276367
35.4810791015625 -10.8718557357788
24.3894786834717 -36.26318359375
-17.9783916473389 20.576545715332
19.8378925323486 24.0790405273438
-33.232105255127 37.0626449584961
36.1797409057617 6.94203090667725
7.33667850494385 6.41638326644897
-39.2179985046387 -22.5340366363525
-0.576031446456909 39.4328193664551
12.5225095748901 28.0540676116943
-39.7115898132324 19.9607009887695
5.57692861557007 40.4040832519531
-30.6990203857422 37.9521141052246
-33.7239837646484 22.523998260498
33.6787490844727 34.7718276977539
-36.202392578125 20.6131801605225
-37.5022239685059 -32.109561920166
16.4776172637939 -13.2209024429321
-39.1827125549316 -20.0971927642822
36.3566474914551 5.53781127929688
26.2667827606201 -29.638370513916
-37.4406852722168 19.7893085479736
25.9700546264648 -37.3037719726562
-33.2666549682617 38.8831520080566
32.2734413146973 35.2038383483887
-4.60164165496826 1.30488061904907
-38.1774215698242 20.7827224731445
33.2838935852051 35.4794540405273
-39.8829574584961 -24.5280590057373
32.0867042541504 36.0553321838379
1.62513136863708 -20.8784790039062
-5.67967319488525 10.1204624176025
-34.3102912902832 21.9333095550537
23.3516883850098 -23.8889904022217
-36.3741569519043 21.8886661529541
-39.7741928100586 -23.3945350646973
-33.9650917053223 38.5672149658203
-32.459228515625 36.5414161682129
2.20175719261169 -28.4244499206543
19.3785839080811 24.8309993743896
-38.8754463195801 -33.101676940918
-2.0681471824646 29.4569473266602
33.5661811828613 35.4919700622559
-33.5373268127441 39.8415756225586
-38.0901679992676 17.6368103027344
6.11561346054077 38.7871475219727
-32.4962997436523 38.5330352783203
-0.903789043426514 -28.0412254333496
-0.168606758117676 -28.5134429931641
36.2919006347656 -12.8806552886963
26.7865600585938 -37.6757774353027
-35.7173233032227 22.7850933074951
-37.5975875854492 -22.6191349029541
25.7222442626953 -36.2340469360352
25.0587024688721 -13.4524993896484
26.2773914337158 -34.3381538391113
24.8078861236572 -14.3965253829956
23.864631652832 -37.5378265380859
-5.69430160522461 12.3351554870605
-38.3935737609863 -32.1911735534668
-37.9723472595215 -31.6392002105713
-38.6481819152832 -32.410717010498
34.3255882263184 -11.9445848464966
-30.9130840301514 37.4466819763184
11.8760004043579 36.3086624145508
-31.7400360107422 37.7703552246094
15.1844444274902 -12.4294586181641
-39.9176483154297 -32.5773277282715
-18.9528522491455 20.8796119689941
31.3376979827881 36.1914482116699
8.32143020629883 4.16121006011963
-33.5735702514648 38.1707229614258
37.3527069091797 -12.3538408279419
33.9037933349609 36.6865081787109
33.7599792480469 36.6437149047852
34.3571853637695 35.2967376708984
-35.1845207214355 20.9018154144287
32.295093536377 35.9818458557129
24.2992782592773 -37.5768203735352
26.6527690887451 -35.7209777832031
-8.46189403533936 27.6930541992188
-37.2902793884277 -23.2494010925293
-35.8098945617676 22.0972003936768
-37.6596298217773 -22.1486988067627
33.0577926635742 37.4370079040527
-34.0230979919434 22.2263717651367
-39.2486877441406 -30.7950553894043
19.6602096557617 24.9514255523682
24.7507419586182 -37.1278762817383
34.5076560974121 -12.8005399703979
-38.1507835388184 20.5978298187256
0.240394115447998 -27.6548328399658
-40.0561256408691 -23.0213088989258
-40.4845199584961 -29.9488925933838
-1.70277035236359 38.5667381286621
26.6723651885986 -37.1374740600586
-32.7435569763184 39.6266822814941
10.327787399292 38.5463409423828
-40.5128288269043 -24.5208873748779
-3.7774019241333 10.6866931915283
35.549991607666 -12.4775791168213
-7.21394443511963 18.5191993713379
-36.2280082702637 -20.4810943603516
16.70871925354 22.707555770874
-38.9838523864746 -32.2678070068359
33.6445541381836 36.2005043029785
37.6676559448242 5.70387983322144
-0.642225623130798 40.0580673217773
32.7634925842285 37.136116027832
-4.0294942855835 31.2955493927002
24.3300361633301 18.8070297241211
8.70305919647217 38.2530212402344
3.75263166427612 38.2437171936035
-30.8400478363037 36.9528465270996
21.1450901031494 -1.29819083213806
35.6371383666992 5.23790693283081
34.5415725708008 6.57409048080444
-37.3011779785156 -32.4591751098633
-3.26834797859192 29.3564224243164
33.3263359069824 36.1263771057129
-0.290869772434235 -28.7141819000244
25.2561340332031 -36.0447959899902
-2.43896746635437 37.384105682373
35.1276054382324 4.67960977554321
6.77494716644287 3.84459614753723
36.8238220214844 6.40824413299561
-29.9807891845703 37.528190612793
-38.6985130310059 -21.4421157836914
-38.0798950195312 -30.5244235992432
13.2049856185913 36.1794929504395
34.6685676574707 8.48017311096191
-37.5304489135742 -32.2857360839844
33.3514137268066 35.5132293701172
33.5697975158691 33.1623344421387
-37.7370872497559 -30.2523136138916
-39.1454429626465 -33.1993598937988
35.7832298278809 -11.7348880767822
-39.9094047546387 -22.2851161956787
14.3218441009521 -25.9453296661377
25.5809383392334 -36.5920333862305
36.4941673278809 7.07159090042114
24.4085731506348 -37.2521018981934
-38.4468040466309 -33.7338180541992
-40.1535110473633 -22.5260791778564
26.782054901123 -37.8736839294434
-0.757175087928772 37.0697402954102
-38.3106956481934 19.6434478759766
26.2861385345459 -10.039701461792
-33.4461669921875 20.9390411376953
-2.31793403625488 -29.9435329437256
-21.8405647277832 20.5867080688477
-38.5947151184082 -33.9686470031738
0.0887601375579834 -28.7451400756836
-18.7089500427246 19.2508869171143
22.0988311767578 20.6448516845703
32.3545188903809 36.211669921875
20.6618881225586 -13.5510921478271
-2.60758376121521 29.6735076904297
-21.1186962127686 20.8626117706299
-37.0890045166016 -33.743782043457
33.8963050842285 -13.5501575469971
14.0805492401123 -12.0618495941162
-33.4561500549316 39.2631378173828
-6.33129596710205 9.72402763366699
27.0519828796387 -37.6211013793945
21.6058464050293 -27.5471382141113
-33.5177154541016 37.297176361084
32.0803337097168 37.9565773010254
-33.5269546508789 38.4030151367188
-17.0178642272949 21.8215274810791
-15.0953722000122 37.3389282226562
-1.34815108776093 -27.9773368835449
-13.0605268478394 38.1981391906738
24.9220714569092 -36.8791084289551
-23.4147872924805 20.650426864624
36.6554641723633 -12.0678396224976
-33.007942199707 39.422794342041
-38.3268165588379 -20.5505237579346
-7.74302244186401 19.6059265136719
-35.1960639953613 23.4739322662354
-38.3168907165527 18.8283767700195
-39.867244720459 -23.0010223388672
6.89765310287476 5.44409942626953
27.7220935821533 -37.6656532287598
14.1517677307129 35.5790748596191
13.8855991363525 38.6234092712402
35.381664276123 5.49366855621338
-35.5284881591797 21.6410236358643
-32.3038368225098 36.9222602844238
35.3857078552246 5.87388849258423
-0.999059081077576 -30.9016933441162
-15.2540082931519 17.5503883361816
-37.7063369750977 -30.1961116790771
-38.5058364868164 -21.3648490905762
-39.8272438049316 -22.6907215118408
-40.8742065429688 20.2563362121582
26.0498027801514 -38.024730682373
30.8344898223877 -11.0766162872314
-38.2075500488281 19.5832633972168
-35.3401527404785 20.6590557098389
35.4123497009277 4.46238708496094
-34.3544731140137 21.7728958129883
-38.5650634765625 -30.8970508575439
33.193489074707 37.2725982666016
26.8513278961182 -37.9477653503418
34.4485816955566 36.6531219482422
-7.47170209884644 18.6625995635986
7.74909591674805 1.71897637844086
32.3688812255859 35.6252479553223
26.4750118255615 -36.7050514221191
-39.0879859924316 18.009407043457
-1.17163908481598 37.2625465393066
-37.916202545166 -20.8840446472168
25.4550018310547 -36.803653717041
-39.6938285827637 20.961483001709
33.2181243896484 37.3563652038574
27.1974639892578 -38.2299308776855
27.046365737915 -36.755687713623
1.26825344562531 -21.4088382720947
-32.573314666748 38.5070877075195
0.110052883625031 38.5546913146973
9.27587127685547 28.7005519866943
35.0878677368164 -14.3653182983398
26.506139755249 -11.464035987854
20.018102645874 21.8385276794434
32.4095039367676 35.9797782897949
0.268941283226013 38.6269416809082
-39.4609718322754 19.8642673492432
36.4810905456543 8.01311683654785
36.8601036071777 -11.3849258422852
22.8233623504639 -13.6200284957886
-39.8126678466797 -20.931058883667
-38.7888107299805 -32.4385528564453
26.8708801269531 -37.3408164978027
34.4635810852051 -11.7876110076904
-39.2614364624023 -31.1775894165039
-4.16512870788574 12.4533720016479
35.7293357849121 5.46476459503174
0.875213742256165 -27.5195159912109
34.9972152709961 -13.9536437988281
2.74401044845581 -29.8043994903564
-30.6768035888672 39.7418365478516
0.0899913609027863 -20.4139022827148
-32.4594345092773 39.3940963745117
36.1100006103516 -12.6443672180176
-8.84692001342773 25.2791404724121
-37.444522857666 -21.5590553283691
27.0513744354248 -24.7040309906006
-1.59223771095276 -0.115996301174164
7.73629808425903 36.8145141601562
32.894359588623 36.6020851135254
-40.5453910827637 18.7143783569336
-36.0660743713379 39.2431182861328
26.3411331176758 -39.4425315856934
-31.7594966888428 35.7718811035156
25.8841705322266 -36.2597579956055
0.213221788406372 -12.7351503372192
24.0410461425781 -39.4942855834961
26.2429180145264 -36.7951469421387
-32.1053314208984 37.6973075866699
21.8906326293945 0.235830843448639
26.980712890625 -40.3445816040039
31.0094375610352 37.8741798400879
34.2680435180664 -14.0468053817749
-39.2103691101074 -32.4093208312988
-31.9391059875488 37.4805641174316
33.7970848083496 36.2507057189941
31.8076725006104 35.9332466125488
-34.6968688964844 23.8306140899658
26.5839424133301 -36.0656509399414
-21.0928287506104 22.1044235229492
-2.16320872306824 39.3140907287598
26.9569301605225 -37.2482223510742
34.6095008850098 -13.8762578964233
23.8521099090576 -36.2318916320801
-37.2036437988281 19.7286758422852
-19.2910499572754 20.0891513824463
25.7995853424072 -37.8176879882812
-1.30841469764709 -10.3308153152466
14.8421173095703 -11.9833059310913
35.6742630004883 -14.4765138626099
36.6666641235352 -12.5588626861572
33.6090049743652 7.69373846054077
-39.2816619873047 -32.0551109313965
24.3258399963379 -38.5626983642578
-38.5244560241699 -32.1548347473145
-34.795467376709 37.4955863952637
-39.8019409179688 -21.5592727661133
-34.707893371582 21.0247173309326
26.8090534210205 -39.1586723327637
-36.3576240539551 21.2892475128174
24.1362171173096 -24.9722156524658
26.9581298828125 -37.8750534057617
-35.8555221557617 -31.2394046783447
1.48419034481049 -12.8857841491699
-37.8292503356934 -32.3276557922363
36.7061309814453 -11.6881265640259
32.5915832519531 36.7181816101074
18.9201641082764 -9.63051319122314
12.5835218429565 39.7827072143555
36.0630302429199 -14.292929649353
18.6194610595703 -1.51552772521973
19.3241004943848 23.9375476837158
-35.9763641357422 -31.7672557830811
-1.36810445785522 -26.7942714691162
-38.3230438232422 -23.3018741607666
-38.3293724060059 -21.758508682251
26.5478591918945 -37.3300285339355
16.7201251983643 20.3381633758545
24.4664039611816 18.4193553924561
-0.823457896709442 -28.752498626709
-32.8946838378906 36.852294921875
-3.15102624893188 13.1601848602295
-33.4452018737793 37.4597854614258
-38.7462539672852 16.9708805084229
-32.9665756225586 39.0591735839844
-34.6814460754395 20.5041828155518
12.7496433258057 -24.8427848815918
-35.7360954284668 20.8283710479736
6.66444063186646 39.0900344848633
-9.60294723510742 19.1869964599609
36.7936210632324 6.41793918609619
-3.69003319740295 29.1303825378418
-31.6894779205322 38.2446937561035
35.2058715820312 7.91730976104736
5.59444141387939 36.0220947265625
-20.5284786224365 21.9253215789795
-37.3887825012207 -32.3526840209961
-23.106164932251 20.6693267822266
-33.03564453125 22.6010608673096
12.2240495681763 35.5559730529785
31.3389987945557 35.5532341003418
33.9870185852051 -12.8390941619873
-37.8027954101562 -31.2688846588135
12.3273372650146 28.9834480285645
25.5890426635742 -26.8878364562988
-37.8793907165527 -30.6930999755859
10.9830369949341 37.4246673583984
7.30126667022705 4.33367919921875
-37.5778579711914 -30.2255535125732
-38.1060447692871 -35.3327217102051
32.1130981445312 35.1941184997559
-17.926685333252 21.4924564361572
-16.293888092041 18.4058570861816
25.0975761413574 -37.9224395751953
-39.3734474182129 -33.3500480651855
-38.7229309082031 18.7530403137207
33.6643753051758 35.3229522705078
-39.579174041748 -32.7931022644043
34.6775131225586 5.52769994735718
26.1977672576904 -37.6983947753906
-38.3313331604004 -33.5340766906738
32.8311233520508 34.1506233215332
-16.6966304779053 20.1693019866943
-31.9009685516357 39.0179557800293
-41.3403625488281 -23.9038257598877
-33.7965354919434 19.4776611328125
25.250093460083 -37.2949028015137
-40.0297775268555 -33.1574935913086
-32.8750991821289 23.1260452270508
-37.4489364624023 -30.5738315582275
0.344255805015564 -29.0553703308105
34.0388984680176 4.49520397186279
25.801607131958 -37.5979232788086
30.6449794769287 33.8096313476562
35.5295333862305 6.93109703063965
-21.4543342590332 21.8431015014648
-41.2057685852051 -32.363883972168
23.4349880218506 -27.8343372344971
27.2269382476807 -28.3422813415527
33.2113952636719 35.3176918029785
26.9023265838623 -37.0567626953125
-38.3954010009766 -31.6665000915527
24.5294609069824 17.1567058563232
35.7663650512695 -12.4859247207642
-37.7697372436523 -33.5688438415527
-39.7703399658203 -22.9509468078613
-41.5038757324219 -22.7854404449463
26.1132068634033 -37.6593437194824
25.8269424438477 -38.6830291748047
35.2959327697754 35.9778289794922
23.1044311523438 17.1906108856201
21.8013782501221 23.0743751525879
-38.4818878173828 19.9404335021973
26.2955093383789 -38.2513580322266
-36.7474327087402 17.6295146942139
-38.3364944458008 -22.2649250030518
-32.6540336608887 36.661678314209
24.8976154327393 -25.3985500335693
24.1758365631104 -37.4846305847168
-37.4044532775879 23.6589794158936
-35.2201690673828 38.3999366760254
10.686351776123 29.4229831695557
-30.4516487121582 35.9081268310547
25.4674186706543 -37.1466636657715
0.894228339195251 -26.3298034667969
-3.01581764221191 -0.0736010372638702
27.2682762145996 -35.8254051208496
-38.853214263916 -31.5725116729736
-37.9140167236328 -30.7063217163086
36.6338119506836 -11.4767456054688
26.0014152526855 -39.3578224182129
-34.3584747314453 37.6667137145996
37.1517753601074 6.50255489349365
-37.6342544555664 -19.9496612548828
-37.3029479980469 -31.2160186767578
7.32923126220703 2.90697598457336
33.6193084716797 33.9578590393066
-38.6201248168945 -33.8440628051758
-33.9192314147949 37.8851127624512
20.1619415283203 0.66406774520874
34.6862716674805 -10.5340585708618
-31.0716400146484 37.6395683288574
31.6262626647949 35.4508590698242
25.1706619262695 -36.3798942565918
-39.7646713256836 21.5160751342773
-4.42867231369019 11.2756376266479
-39.0697021484375 -23.6964092254639
-37.1912879943848 -22.2624320983887
5.47599172592163 38.1859436035156
24.9678745269775 -25.2135448455811
34.9397583007812 -10.9272794723511
35.2841644287109 34.7374305725098
-32.1735305786133 39.955249786377
-8.12691497802734 19.6009464263916
-2.81859254837036 37.3030395507812
25.8860492706299 -38.4280204772949
-0.531087279319763 37.4797172546387
-20.3032455444336 20.4183559417725
-37.7401733398438 -31.6250267028809
29.2310123443604 -11.7369241714478
-35.0958557128906 21.9881420135498
-30.086841583252 37.5465812683105
6.46510648727417 5.06538105010986
-38.9585762023926 -22.8416633605957
35.0289039611816 -13.3762483596802
35.4982719421387 4.64440727233887
34.2946510314941 5.95812892913818
-31.3538818359375 39.8441886901855
25.0770492553711 -36.685718536377
24.0454196929932 -25.7833118438721
-32.9564781188965 39.8522872924805
-34.5610313415527 20.6134510040283
-39.5249481201172 -30.2020359039307
32.8400764465332 36.303409576416
-39.4678649902344 -32.3995208740234
26.0993556976318 -37.0992012023926
-34.2630882263184 39.6169929504395
37.7173080444336 -13.7080049514771
34.1788940429688 36.222583770752
34.4506568908691 4.06948137283325
-11.5033769607544 28.2236099243164
10.5183277130127 36.7384414672852
-33.3408813476562 38.2818832397461
-32.8715744018555 39.9855804443359
-14.6154594421387 36.1081275939941
37.8425025939941 -14.5784730911255
27.4089546203613 -37.1366577148438
-31.9350757598877 35.5119476318359
26.1979694366455 -37.6428680419922
-32.4797439575195 39.804386138916
10.0502300262451 27.6229000091553
24.1930122375488 -35.9485931396484
1.75131630897522 -20.470344543457
23.7523651123047 -35.2748222351074
9.47577476501465 35.890926361084
-37.8067970275879 20.6991672515869
24.3925609588623 16.1367053985596
5.86003923416138 38.4340629577637
-38.9306030273438 -33.4543724060059
-37.8868370056152 -33.4327049255371
1.19564867019653 -28.8417701721191
25.6859493255615 -36.2364692687988
-38.8798599243164 -31.2237968444824
-30.8093204498291 38.1328735351562
27.4785652160645 -27.3846321105957
-38.5880317687988 -21.9890327453613
-32.5460548400879 38.4560356140137
1.4922970533371 -12.4140367507935
25.8852138519287 -36.5807342529297
-2.31218409538269 1.17903423309326
-38.5663414001465 -31.9940986633301
5.19713401794434 40.2756538391113
20.7780075073242 -26.0359287261963
35.0046691894531 -14.6181869506836
24.6899719238281 -37.1419792175293
-36.8515472412109 -32.6696662902832
-38.0428314208984 -21.7602996826172
5.78752708435059 38.2960357666016
36.6649703979492 -14.0488805770874
36.0248260498047 6.80549049377441
34.1035614013672 4.68765878677368
-17.1924228668213 23.7021770477295
-39.6825637817383 -22.5635471343994
-38.285457611084 -32.7012901306152
26.6595096588135 -36.9630661010742
32.7173385620117 38.2988052368164
36.0727081298828 -11.1266794204712
34.3330268859863 35.0833396911621
-40.1736755371094 -31.9542102813721
20.352352142334 -14.5768375396729
36.0229949951172 35.532096862793
-33.4054489135742 37.2074012756348
-14.9307422637939 35.5146751403809
-34.1630401611328 38.3612289428711
-0.761115431785583 1.61145758628845
-39.0921974182129 -30.6378154754639
-31.0701751708984 38.6506423950195
30.30637550354 -10.5767498016357
20.0681381225586 -12.2568063735962
-33.693675994873 37.5993995666504
23.7397155761719 -38.4103126525879
26.5191307067871 -36.8437652587891
33.1314811706543 36.5177116394043
-38.3387718200684 -19.9965171813965
32.4995384216309 37.0222129821777
26.2652015686035 -38.0766220092773
25.6201725006104 -38.9213447570801
11.4785757064819 36.3946495056152
13.7123212814331 -26.645263671875
33.0796928405762 36.0231781005859
15.4704132080078 -4.78661108016968
-14.1614875793457 34.488166809082
-0.696761190891266 37.7022933959961
12.5035781860352 38.3840141296387
12.4639053344727 28.9717025756836
-37.0428848266602 -32.6623497009277
33.1325035095215 35.8616104125977
29.8355579376221 36.9753189086914
-3.05227971076965 36.9594268798828
33.4582748413086 34.8884162902832
27.0094032287598 -34.1577033996582
34.5711059570312 5.56976270675659
26.8656005859375 -36.4216690063477
2.66098356246948 -10.9313278198242
33.7055931091309 37.1056022644043
12.6074409484863 37.0744819641113
-38.4846343994141 -32.0999221801758
33.3999938964844 -12.4986896514893
23.1214160919189 -16.7907447814941
-8.75986671447754 28.1966075897217
27.6207313537598 -37.2181167602539
4.26870489120483 37.5877227783203
12.0988426208496 28.6730327606201
-35.0831184387207 37.8858489990234
-1.79912269115448 37.4612159729004
5.54455518722534 39.2765769958496
26.4973487854004 -38.7272453308105
-37.7607841491699 20.3157844543457
-34.0577507019043 38.2775688171387
-1.00984573364258 36.4866218566895
36.4264755249023 -13.8467845916748
-33.7747268676758 37.6546897888184
26.5310039520264 -37.4760589599609
2.06759977340698 -23.2595291137695
-39.6317901611328 -23.7307834625244
33.3720970153809 35.463005065918
-37.9505271911621 20.2510089874268
25.2153453826904 -36.7030715942383
-40.3590888977051 -32.0693206787109
25.7896919250488 -36.4636344909668
26.2839870452881 -35.5684432983398
-36.8314971923828 20.5275630950928
-2.20373725891113 0.552311658859253
-38.5988845825195 20.9531650543213
32.1857795715332 36.0839958190918
-39.9251289367676 -30.494421005249
-36.73828125 -34.144157409668
-7.65441656112671 17.4951477050781
-14.311671257019 17.3011741638184
0.740479826927185 -20.6774387359619
-19.1489143371582 19.3913230895996
-21.6262912750244 18.3951721191406
35.1734504699707 -12.6445274353027
-37.4184494018555 20.2454452514648
-38.0209121704102 17.7403030395508
-31.73020362854 38.4769706726074
31.9019050598145 34.3491821289062
-38.081111907959 -30.8775272369385
-32.9297523498535 38.7219161987305
26.1189937591553 -37.6552505493164
-33.3384056091309 36.9102096557617
-38.5381851196289 -31.875904083252
-40.0116767883301 -30.7371463775635
17.997838973999 24.5593338012695
-40.1057929992676 -33.1004905700684
33.444652557373 35.3727416992188
-31.8171863555908 37.5923805236816
32.4445571899414 33.9836044311523
23.6839370727539 -38.4720344543457
-38.1768493652344 21.0976543426514
-4.6789288520813 29.6032619476318
18.9643592834473 24.5820159912109
26.129976272583 -39.1626510620117
-38.7321166992188 -21.9164657592773
25.9862442016602 -38.5975914001465
27.4105339050293 -37.7449340820312
-37.0760650634766 -24.0860748291016
24.4343414306641 -39.2496032714844
32.3605194091797 37.1185913085938
4.28132152557373 3.97036457061768
-36.6567230224609 -31.0521221160889
-36.7325744628906 22.2095165252686
-33.7664756774902 39.1827850341797
36.4942359924316 6.91875457763672
-2.47678136825562 2.64417552947998
10.7550954818726 38.0054016113281
1.51147496700287 -22.5513439178467
-32.521484375 37.2725296020508
-37.4015655517578 18.7330493927002
-36.9230880737305 -34.932487487793
25.1128711700439 -36.4074363708496
25.9962711334229 -36.9113693237305
-3.88275718688965 2.94412732124329
24.5284099578857 -37.8705940246582
-32.0451469421387 38.3468360900879
25.704273223877 -37.5081558227539
-38.6186943054199 -22.681116104126
-37.7291564941406 -31.2775096893311
6.77249670028687 37.7096366882324
35.1039772033691 5.40995740890503
36.0644073486328 -12.1001663208008
33.671989440918 5.68762350082397
19.0588512420654 24.5165100097656
-34.4784278869629 20.0240707397461
-7.658522605896 18.3103981018066
-37.9222145080566 -22.6636409759521
-3.15180230140686 -1.08881258964539
25.3157978057861 -36.9061508178711
-31.9614276885986 36.4562606811523
35.660327911377 -12.3653869628906
-38.0397148132324 -22.6524486541748
6.65320348739624 4.52103614807129
1.38391637802124 -24.4265308380127
-2.79148077964783 10.2318096160889
-38.8395500183105 -21.2437419891357
-39.3161697387695 -32.4344215393066
5.43593406677246 38.1981048583984
12.2113933563232 37.9032440185547
-39.1646118164062 21.0116157531738
-33.4594192504883 20.6626319885254
34.5710220336914 -13.4003734588623
25.3812084197998 -36.5150451660156
33.2908020019531 37.1266593933105
-35.7214546203613 -29.3267917633057
-39.6395301818848 -22.4654445648193
-38.199577331543 20.1051559448242
34.9267654418945 6.21242570877075
10.714035987854 36.7750663757324
0.979942679405212 -21.0390033721924
-37.595287322998 -32.047004699707
-16.9087181091309 18.8509960174561
-36.8155784606934 -30.5711307525635
23.5692329406738 -23.3034477233887
-39.6463203430176 18.6881656646729
11.9893035888672 38.4807434082031
33.7859573364258 36.3201293945312
34.0924072265625 -11.2238397598267
11.792028427124 38.8398246765137
-35.8131408691406 -33.0407295227051
19.1869163513184 -7.57291841506958
-38.7342948913574 20.6747055053711
-31.0682640075684 38.0861053466797
-33.6638832092285 19.7510986328125
-37.288459777832 21.3362293243408
5.88059949874878 39.670768737793
23.6293258666992 17.5215129852295
33.7404022216797 -14.4666614532471
-38.5970230102539 -32.0942192077637
-31.7418746948242 39.2761459350586
33.1312141418457 36.2203178405762
32.9465026855469 36.4715118408203
25.9468460083008 -35.1892395019531
-40.6574096679688 -22.7378616333008
-38.8095436096191 -32.5813179016113
36.456901550293 -13.7915849685669
23.3287086486816 -27.7027931213379
6.10047006607056 37.8053283691406
-39.2342758178711 18.729434967041
32.8584938049316 35.7779922485352
-9.61724853515625 16.0737762451172
-40.377555847168 -24.8080577850342
-17.2849941253662 21.6996746063232
-30.8406791687012 38.7281494140625
12.2461738586426 -26.8100910186768
33.6254844665527 5.0554370880127
27.0695667266846 -36.8017730712891
27.2485580444336 -37.4685287475586
37.3183403015137 4.64675998687744
-32.5623779296875 37.4504928588867
-33.8629188537598 38.0936431884766
-32.5483055114746 37.2930755615234
35.5354118347168 -13.6373472213745
7.44722080230713 5.11006355285645
35.8666801452637 -12.4047203063965
-37.4798965454102 -32.6445083618164
-1.64787638187408 35.975471496582
-0.389740407466888 -27.5993137359619
-33.6188659667969 19.6135139465332
-35.5703887939453 22.1766395568848
-39.7620010375977 -30.7451152801514
-6.26796245574951 18.1194038391113
34.1179580688477 35.5596237182617
-38.3847694396973 -30.9876766204834
35.6647071838379 -12.9008226394653
12.4363784790039 37.1372909545898
34.0094108581543 36.0824775695801
-33.7118110656738 38.4252815246582
7.36658954620361 37.7610969543457
-34.8894081115723 23.3285236358643
27.0905742645264 -38.2475128173828
34.2121658325195 6.91797065734863
-38.3723754882812 -32.5827102661133
34.2989044189453 4.88205480575562
-2.50100612640381 2.13421583175659
17.4254627227783 -8.84140968322754
-39.5390243530273 -21.7130641937256
-33.1080665588379 35.0993804931641
32.8956756591797 36.5878753662109
-38.5866050720215 -32.3280906677246
11.5600366592407 -26.530065536499
-9.4915075302124 27.5760192871094
-31.9262733459473 36.9606437683105
-34.8103370666504 22.3456420898438
-33.851203918457 37.5107803344727
25.39821434021 -38.5096702575684
0.327260434627533 -12.5109844207764
35.0973815917969 -12.2934303283691
-38.6355590820312 -30.3629112243652
34.6364593505859 -13.7125625610352
23.7674331665039 -37.9174118041992
-35.9197006225586 -32.3880271911621
-38.6986961364746 -30.4156761169434
33.5237884521484 38.8862152099609
-31.5107707977295 38.2873764038086
34.703987121582 35.9777145385742
27.2200756072998 -36.5373954772949
27.2136459350586 -38.8103065490723
33.3092803955078 36.367359161377
-34.1607208251953 37.6843719482422
35.264720916748 8.00501823425293
-36.7084655761719 -32.9274673461914
-7.72577571868896 27.4454879760742
32.4250221252441 35.5880088806152
-38.2119369506836 -32.404857635498
25.5598964691162 -38.3190536499023
-39.5063743591309 -29.906587600708
1.02308249473572 -10.6135263442993
-39.052059173584 -22.2766761779785
33.3977432250977 35.1820640563965
32.7020301818848 36.7899131774902
23.2168045043945 -38.5273132324219
25.865873336792 -36.031852722168
-34.6321411132812 20.9698848724365
10.6705570220947 37.5348510742188
-39.326732635498 -21.2639236450195
25.632963180542 -35.7395973205566
35.9389839172363 36.6965370178223
26.8740310668945 -37.3889236450195
-38.6109085083008 -30.930534362793
33.2682151794434 37.0228691101074
5.79333114624023 36.1955223083496
-38.1641120910645 19.9246597290039
33.7538833618164 33.5684776306152
27.9808044433594 -12.4525995254517
-39.7013244628906 -30.8254547119141
-37.9855804443359 -23.857141494751
-14.171329498291 17.1856555938721
33.0487861633301 35.7251052856445
29.2826175689697 -11.7407398223877
-35.9677886962891 21.9817447662354
-32.0440521240234 39.9641227722168
33.2666282653809 36.3988990783691
-40.140625 -21.0096893310547
1.20028281211853 -21.628625869751
-39.2882690429688 -31.9326725006104
11.6060991287231 39.459228515625
-38.8591156005859 -32.5833854675293
-34.8904037475586 19.9505443572998
33.6487731933594 -14.0054712295532
25.6219825744629 -38.8197631835938
31.7821712493896 37.3648071289062
-32.8206634521484 40.6883277893066
4.78421115875244 39.8150825500488
26.2473430633545 18.2258758544922
33.4455947875977 36.3573036193848
-3.60173606872559 41.5815544128418
-38.8567695617676 -30.0327644348145
-33.6683082580566 38.1249389648438
12.7898197174072 -26.0582046508789
-38.3854026794434 19.0255489349365
25.5804748535156 18.4468612670898
35.1701774597168 37.3706550598145
33.4494514465332 6.51945686340332
-35.277416229248 38.0618782043457
36.2114143371582 4.65719509124756
34.5352096557617 -11.9417495727539
-14.640585899353 35.2690811157227
35.929615020752 -12.5685911178589
-36.3835639953613 21.4115619659424
-39.8176116943359 -21.8097286224365
28.25901222229 -13.3362550735474
1.02576446533203 -10.9765844345093
-33.8709144592285 21.4895839691162
-39.3531188964844 -31.4889850616455
-36.2552261352539 20.3167324066162
28.3325901031494 -37.5848617553711
25.751859664917 -36.7336196899414
-38.5574417114258 -29.6778907775879
-38.5168113708496 -31.6269207000732
35.3773612976074 36.0593109130859
25.6368656158447 -37.7205924987793
5.13560009002686 39.883861541748
32.8631210327148 35.4431076049805
25.1884841918945 16.7069187164307
-7.97427034378052 16.5945167541504
-35.762035369873 20.6019496917725
-34.0189895629883 39.3963470458984
-36.4079666137695 -34.2746658325195
26.8615131378174 -37.3669166564941
-39.1251754760742 -22.372486114502
-37.4072418212891 -34.9861640930176
34.8591117858887 -12.9473247528076
19.8815250396729 0.706623435020447
31.8430976867676 34.3768882751465
23.7895984649658 -24.4784679412842
35.9166221618652 7.21703863143921
-32.0934181213379 37.8643417358398
36.4010314941406 -14.5934753417969
-39.3586311340332 -30.9411735534668
35.5983276367188 5.27834844589233
11.8194007873535 37.6779670715332
-0.292341291904449 -30.6215915679932
-39.4139366149902 -22.0119781494141
33.2839508056641 36.4737396240234
-38.6547546386719 -32.9336051940918
-38.0940971374512 19.7524070739746
-33.322811126709 38.4207916259766
36.5032081604004 5.67078733444214
-39.118236541748 -32.4978103637695
24.2223167419434 -34.327507019043
-35.3918304443359 20.3398895263672
-15.3297872543335 34.933177947998
-37.1681442260742 -32.7328796386719
27.7873229980469 -37.0991363525391
34.0558967590332 35.8869819641113
35.3105888366699 -13.9735651016235
-39.7319602966309 -31.8902225494385
26.488431930542 -37.2131309509277
26.4344482421875 -36.744083404541
-16.5273761749268 35.9331665039062
12.5279264450073 37.2205429077148
-18.0697269439697 24.1643867492676
-39.2890243530273 -20.4488372802734
};


==> figures/visualizations/gmm40/mfvi_samples.tex <==
\addplot [semithick, mfvi, opacity=0.7, mark=*, mark size=3, mark options={solid}, only marks]
table {%
18.0340366363525 -3.89385986328125
19.0040149688721 -10.8098402023315
18.4992580413818 -13.7370357513428
19.9698257446289 -0.72566556930542
19.9556617736816 -4.70160865783691
19.1240978240967 -16.167688369751
18.8296909332275 -7.68719911575317
18.3907375335693 -7.60511112213135
18.1370601654053 -9.01530170440674
18.8893184661865 -9.88476848602295
21.6626663208008 -5.49776172637939
14.9740266799927 -8.31573677062988
18.4146881103516 -2.94627237319946
21.0004844665527 -7.37367725372314
17.881031036377 -9.79098415374756
17.8553524017334 -11.0971374511719
18.1070823669434 -5.49458312988281
20.2403469085693 -9.94921684265137
17.0399322509766 -7.17947912216187
18.3658542633057 -9.5630989074707
17.4768753051758 -13.5887842178345
20.1425552368164 -18.4453105926514
20.2467060089111 -14.0105304718018
19.0273704528809 -0.786180973052979
18.650505065918 -8.52199363708496
19.6946926116943 -14.8835296630859
21.3689384460449 -14.7254962921143
19.4188022613525 -16.8554000854492
20.4020595550537 -9.42478561401367
19.0359001159668 -9.94060611724854
19.7154235839844 -8.51165866851807
17.2547302246094 -12.5653228759766
19.0841579437256 -7.01956939697266
20.1325283050537 -7.66766977310181
19.9899845123291 -12.5318727493286
19.0643634796143 -5.47168445587158
21.0008964538574 -8.12185001373291
18.4872074127197 -4.2548246383667
17.9211463928223 -6.61021995544434
20.5135803222656 -8.27755737304688
17.2797470092773 -4.18135023117065
18.3798732757568 -8.8965015411377
18.0893878936768 -7.71607303619385
20.6833457946777 -7.45718955993652
20.0068378448486 -13.9237403869629
21.5339221954346 -5.80118179321289
21.9202098846436 -10.7540874481201
16.4473304748535 -5.78844118118286
18.8821697235107 -12.5728893280029
19.9123783111572 -13.322380065918
16.8369808197021 -6.27108669281006
18.903247833252 -12.8554496765137
17.5732135772705 -5.62513542175293
19.4058208465576 -11.3506050109863
19.912633895874 -11.5522241592407
18.0558376312256 -7.94495391845703
18.500244140625 -8.31154441833496
16.6417770385742 -10.5221357345581
16.3616046905518 -4.78473854064941
20.0593490600586 -14.5623865127563
20.1372489929199 -9.60765171051025
19.7323150634766 -5.74732065200806
17.7448234558105 -2.29694271087646
20.5264949798584 -6.45985794067383
15.7839012145996 -9.28822422027588
18.0453701019287 -5.18905162811279
19.3703689575195 -8.33355236053467
20.047872543335 -12.6726655960083
17.1090965270996 -0.661721229553223
21.4230728149414 -8.54167747497559
19.6654605865479 -1.69514799118042
18.9223766326904 -8.21602439880371
20.6628494262695 -12.35853099823
21.100564956665 -8.78186511993408
18.2357196807861 -9.5941686630249
17.4016437530518 -7.0191650390625
20.7683181762695 -2.73475933074951
19.8343372344971 -9.17722129821777
19.8924789428711 -7.0147385597229
20.626314163208 -9.91688919067383
16.3352870941162 -6.8690242767334
21.0115852355957 -11.7184648513794
15.7400770187378 -10.0809450149536
19.8923301696777 -13.8102197647095
18.7397804260254 -8.44461917877197
20.4015007019043 -8.70754337310791
17.9453392028809 -7.24492263793945
17.7707595825195 -16.1303329467773
19.5113334655762 -7.50109958648682
20.9990577697754 -6.07524681091309
19.9249725341797 -12.3819093704224
18.7379913330078 -11.1653137207031
17.991512298584 -10.7178812026978
19.3876209259033 -5.51638221740723
19.5289363861084 -3.75672006607056
18.9131374359131 -2.93059110641479
19.9021244049072 -7.4205322265625
19.6198043823242 -6.48578071594238
18.4986801147461 -7.85611295700073
16.1894702911377 -8.47562694549561
15.8526229858398 -12.3979110717773
18.6215629577637 -12.4939117431641
16.3648700714111 -9.50700187683105
17.817907333374 -9.54532909393311
15.0522193908691 -8.11729049682617
19.3357677459717 -10.0740003585815
18.6052379608154 -9.45988941192627
19.0853214263916 -16.2920169830322
18.0065364837646 -7.48229360580444
19.050537109375 -7.98266363143921
20.707368850708 -10.1299285888672
21.0352993011475 -6.73050308227539
20.0859622955322 -8.45485687255859
18.1936359405518 -9.14860439300537
22.0426254272461 -5.92452526092529
19.0895137786865 -4.56056833267212
18.8181896209717 -12.2158899307251
17.6456508636475 -8.02229595184326
18.7010154724121 -12.3765230178833
17.1614742279053 -3.81632375717163
18.0633926391602 -8.26334381103516
20.4312114715576 -15.0885028839111
18.4049987792969 -8.0218505859375
20.1025772094727 -10.9036111831665
21.1062316894531 -13.4910163879395
19.1109428405762 -9.94617462158203
19.1581649780273 -9.91438961029053
19.2879467010498 -13.733715057373
20.3727149963379 -11.8825483322144
20.6320152282715 -10.8634967803955
17.4923553466797 -8.07483863830566
19.293643951416 -11.0097017288208
21.7422256469727 -6.04603385925293
19.1036472320557 -5.8092303276062
17.1964321136475 -7.34290885925293
16.3445148468018 -7.23838710784912
18.5272731781006 -6.57775688171387
17.9295711517334 -7.40086603164673
18.8259963989258 -11.0902919769287
17.2448844909668 -7.77361392974854
17.9916515350342 -8.56005191802979
19.4420776367188 -7.18480157852173
19.2573204040527 -11.7509355545044
19.6466274261475 -3.20125007629395
21.5855541229248 -8.74223327636719
22.7345943450928 -4.62901306152344
18.7484836578369 -7.61506414413452
18.9387435913086 -7.97135162353516
19.58083152771 -6.38606262207031
19.733419418335 -6.83849811553955
20.7417297363281 -2.78568887710571
18.0941677093506 -5.50713920593262
20.3264751434326 -6.14466238021851
19.1702651977539 -7.65022373199463
19.7389068603516 -7.50220012664795
20.9784832000732 -8.77297782897949
18.4792366027832 -13.8938827514648
17.4988117218018 -7.65509557723999
17.6889057159424 -10.9579057693481
18.6121978759766 -12.3639183044434
16.6130828857422 -3.10610342025757
20.7708721160889 -10.9789142608643
18.1517772674561 -15.4245128631592
18.9816036224365 -10.0291757583618
20.5581874847412 -8.14469623565674
19.0251846313477 -9.10272216796875
20.6125297546387 -9.47274971008301
20.283618927002 -6.76789093017578
21.2936954498291 -8.77699947357178
17.7962512969971 -6.59919834136963
19.4408512115479 -9.65508079528809
19.6169471740723 -9.89852046966553
18.9559764862061 -11.5886669158936
20.211820602417 -15.4507102966309
20.93625831604 -6.13275718688965
17.6875419616699 -13.3050899505615
18.4780292510986 -7.38410329818726
17.297327041626 -12.5150680541992
17.7901706695557 -14.1121883392334
16.6215953826904 -10.5560531616211
19.292989730835 -8.91256046295166
18.0433197021484 -15.5068454742432
15.6611356735229 -10.8902320861816
19.9123401641846 -9.28632259368896
17.0804462432861 -10.388617515564
17.411226272583 -6.1292085647583
20.034236907959 -6.39250659942627
18.6794242858887 -11.7374458312988
17.2291851043701 -10.75257396698
18.6593017578125 -7.36094808578491
19.0706195831299 -12.2354679107666
20.7089996337891 -9.21170234680176
16.9662456512451 -4.68786239624023
18.679012298584 -8.63560581207275
19.6269207000732 -12.0424060821533
18.5385723114014 -10.2098436355591
16.7040977478027 -12.3544960021973
18.7241535186768 -2.14785528182983
18.0751457214355 -12.2603530883789
16.1538829803467 -9.85892486572266
20.9468383789062 -8.27866554260254
18.4587345123291 -11.413257598877
18.4595832824707 -8.55181980133057
19.8531036376953 -11.650203704834
18.0509643554688 -9.08597564697266
22.5009231567383 -11.2220878601074
20.0227432250977 -9.90626525878906
18.5031394958496 -9.5204553604126
19.0831890106201 -8.28885269165039
16.4291591644287 -12.6661128997803
18.4116458892822 -10.717267036438
22.8809967041016 -11.0206432342529
19.3331508636475 -8.73294830322266
19.0516891479492 -5.69491529464722
19.136646270752 -7.30002403259277
18.0575199127197 -3.4779748916626
16.9517822265625 -10.1839618682861
16.2837104797363 -9.24405479431152
19.5068912506104 -10.1212329864502
21.6841449737549 -1.27556180953979
20.3333549499512 -5.28622341156006
20.0576705932617 -7.46044063568115
19.285530090332 -11.1766796112061
18.3854560852051 -11.8148002624512
15.5991401672363 -6.9805850982666
18.6600189208984 -8.55855369567871
16.1038780212402 -8.08579540252686
15.6886291503906 -8.69691944122314
18.888786315918 -13.3285341262817
19.9505233764648 -11.4694671630859
19.6721801757812 -9.91911029815674
19.1047039031982 -6.67478275299072
18.8551006317139 -10.5345258712769
21.2528171539307 -10.322774887085
19.5009174346924 -11.8049488067627
18.8264236450195 -11.7745513916016
19.4019565582275 -9.24871730804443
16.5477924346924 -7.49421215057373
18.0447959899902 -9.0549430847168
19.6266002655029 -7.2006368637085
16.0836544036865 -8.55960464477539
19.4877471923828 -7.26854372024536
18.6655178070068 -7.55856084823608
18.2690467834473 -10.1396894454956
18.4502010345459 -10.4773302078247
18.9609375 -2.61781024932861
21.1033821105957 -10.4582672119141
21.8196659088135 -10.141263961792
19.9048309326172 -8.91707897186279
16.1198558807373 -13.958890914917
18.7984924316406 -11.8728799819946
19.2393665313721 -9.71400260925293
19.1145725250244 -12.813777923584
20.7073078155518 -12.2191925048828
19.3786239624023 -7.94867849349976
16.8420524597168 -7.30110120773315
16.4589729309082 -4.05300998687744
20.4422950744629 -13.6895408630371
19.7319297790527 -12.715576171875
20.5091590881348 -4.55101251602173
19.8835639953613 -8.85561847686768
16.8187351226807 -4.55144071578979
18.5961093902588 -7.76895523071289
18.2055530548096 -11.2331123352051
17.5303287506104 -5.60879898071289
21.4413928985596 -9.87797832489014
19.3552169799805 -12.0209407806396
20.0528144836426 -13.280481338501
14.8002920150757 -5.739182472229
15.2340059280396 -10.6235103607178
19.3783264160156 -16.0832176208496
18.7898120880127 -5.92350053787231
19.3452987670898 -15.0750465393066
20.0539035797119 -8.69629096984863
19.8263530731201 -13.8342838287354
22.4861431121826 -8.27414989471436
19.576192855835 -7.71357488632202
17.273998260498 -9.1640043258667
18.8111248016357 -6.37521648406982
19.7159290313721 -11.6907978057861
20.6729068756104 -4.37352514266968
16.4382667541504 -13.7262840270996
19.0719604492188 -11.4416198730469
21.8216915130615 -5.24868011474609
17.0568599700928 -7.97086906433105
17.643575668335 -14.343168258667
20.8362693786621 -9.44277667999268
18.4951095581055 -10.3930587768555
18.6899909973145 -6.50568771362305
21.4664745330811 -5.69062805175781
20.4032096862793 -15.1705913543701
18.4066848754883 -14.8270311355591
19.7482242584229 -9.08505249023438
18.3989238739014 -7.30148935317993
18.0441303253174 -7.12762546539307
17.1529941558838 -3.00336360931396
17.9396896362305 -10.360857963562
19.5074253082275 -13.3815689086914
16.1555137634277 -7.8955192565918
17.801944732666 -5.66348266601562
18.4212875366211 -7.66245651245117
15.9722919464111 -14.3183326721191
17.5855598449707 -4.59252548217773
17.138219833374 -6.51755523681641
21.9812088012695 -12.6692991256714
20.9007091522217 -7.74453496932983
20.0339031219482 -12.3685569763184
19.732931137085 -0.071070671081543
20.6019744873047 -13.3219375610352
17.9149646759033 -11.767035484314
18.7010726928711 -11.5781116485596
17.2436351776123 -15.296760559082
20.7729816436768 -6.88116264343262
16.4075012207031 -5.04764652252197
18.9188117980957 -10.0407199859619
17.0574226379395 -10.8955755233765
19.2425804138184 -5.04885292053223
16.6997108459473 -4.20161056518555
20.6160373687744 -10.5757961273193
19.2116298675537 -12.8937530517578
20.5637474060059 -15.6939525604248
17.8030834197998 -10.2750329971313
20.6644172668457 -10.2159824371338
16.9022445678711 -11.0198593139648
19.7501068115234 -12.9605541229248
21.23512840271 -1.44383144378662
18.8437118530273 -11.3026161193848
18.7618179321289 -12.4706163406372
19.1329345703125 -6.02574920654297
21.4083290100098 -8.1321907043457
21.2859878540039 -7.6965012550354
16.4063720703125 -7.52495908737183
18.8053970336914 -9.84297561645508
19.5276679992676 -10.6830835342407
17.465295791626 -5.37761878967285
18.2981243133545 -5.00276803970337
19.1400012969971 -11.4118766784668
20.7241859436035 -12.9372577667236
19.1955699920654 -6.52905559539795
17.2061367034912 -7.9064884185791
20.3708534240723 -5.77673816680908
16.6585941314697 -5.79610443115234
16.2648754119873 -12.9929885864258
16.8317642211914 -3.46737861633301
18.3650379180908 -10.0060806274414
18.7079677581787 -3.47531747817993
19.6997108459473 -11.6406412124634
19.0095520019531 -8.71796321868896
21.721097946167 -11.196252822876
17.0811862945557 -10.5345859527588
20.7450275421143 -21.3607368469238
19.3072814941406 -8.84372615814209
19.8882808685303 -3.66216135025024
20.7876815795898 -16.9140167236328
19.1382141113281 -9.04027080535889
20.1345386505127 -9.82526969909668
19.1592102050781 -12.3651733398438
19.9718456268311 -8.22847652435303
21.9776668548584 -5.42363929748535
18.8579635620117 -7.38701248168945
17.8140048980713 -10.8567905426025
19.462007522583 -6.17585277557373
17.6727313995361 -8.50459671020508
18.4803199768066 -8.86215591430664
19.6560230255127 -9.40269947052002
19.9531326293945 -1.93970203399658
20.2088088989258 -4.10218477249146
18.3867034912109 -6.57587051391602
20.2801532745361 -7.494544506073
20.9205455780029 -6.43532943725586
14.0360069274902 -15.0359525680542
19.3906688690186 -7.86032819747925
20.8642158508301 -12.8767290115356
17.7606468200684 -9.8568229675293
21.0665588378906 -6.87754535675049
17.7763500213623 -12.155481338501
19.1970977783203 -10.5776195526123
20.1459808349609 -12.036247253418
17.6519966125488 -10.9951257705688
19.6855697631836 -9.37270164489746
19.5437717437744 -10.2711381912231
18.2084655761719 -4.0691294670105
22.2997703552246 -12.0685043334961
20.0831165313721 -10.3655500411987
17.4715347290039 -8.55814552307129
16.0939788818359 -7.99685049057007
18.9797801971436 -9.89171314239502
20.2936420440674 -1.2884669303894
20.9493179321289 -5.70364999771118
19.6713905334473 -10.0371980667114
18.6188716888428 -8.67727375030518
17.3935642242432 -7.34349632263184
18.0586204528809 -14.4398880004883
17.1806373596191 -6.49364757537842
19.381254196167 -4.0371208190918
18.4422092437744 -11.4596929550171
19.905725479126 -8.24281787872314
16.4966793060303 -7.99398899078369
19.7320766448975 -4.82586097717285
17.3810482025146 -6.77041292190552
20.4059581756592 -2.5880970954895
17.4107551574707 -6.94388008117676
17.4664192199707 -9.99857139587402
20.602294921875 -6.62969970703125
18.8241863250732 -9.50911331176758
20.6453800201416 -9.18288230895996
18.9269752502441 -8.62041473388672
18.4438133239746 -13.7261390686035
18.8636951446533 -4.49343013763428
20.8643131256104 -7.10934591293335
18.851469039917 -5.75398445129395
17.9878692626953 -4.04218721389771
17.975227355957 -8.34318447113037
18.5042915344238 -4.39249467849731
22.5440521240234 -9.6689453125
17.2436752319336 -6.87143611907959
19.9236297607422 -8.36165714263916
18.9904937744141 -8.17687892913818
17.0715503692627 -6.81946611404419
19.7815780639648 -9.11855506896973
18.7230567932129 -6.7562952041626
20.8502922058105 -4.22440624237061
17.5654716491699 -3.19824409484863
19.4552211761475 -13.1815986633301
19.0628452301025 -3.74294090270996
17.3253498077393 -15.4901275634766
18.6457500457764 -9.37907600402832
18.6916732788086 -13.5761241912842
19.0792179107666 -7.69568490982056
19.0650634765625 -14.190601348877
20.4246940612793 -6.59328842163086
19.8516273498535 -11.4228363037109
15.5155420303345 -12.4970798492432
20.1827411651611 -5.931809425354
16.7755432128906 -7.73163747787476
18.1005611419678 -8.49172401428223
21.7652816772461 -7.76231336593628
17.4258842468262 -11.2414178848267
15.8341484069824 -7.7075023651123
18.1674919128418 -13.3554801940918
19.9427490234375 -4.72646903991699
18.6345062255859 -7.93967819213867
16.252384185791 -3.73833084106445
16.1361713409424 -8.39178371429443
19.0039348602295 -9.54063987731934
16.781494140625 -9.1226806640625
19.5792598724365 -11.369330406189
20.330904006958 -11.4665746688843
19.4135360717773 -9.86338043212891
18.9095020294189 -9.0740852355957
18.3025245666504 -5.48761463165283
16.0866889953613 -4.44664716720581
20.8662185668945 -6.5143575668335
20.369800567627 -8.61427211761475
21.024169921875 -11.9158353805542
18.3740139007568 -11.9527854919434
18.1675872802734 -8.61727333068848
17.9040565490723 -17.1223182678223
19.3841552734375 -9.28628349304199
20.299165725708 -10.3710536956787
17.5887432098389 -8.03402137756348
18.8178539276123 -4.41440773010254
21.5360698699951 -9.0700798034668
16.8720035552979 -14.8755865097046
17.9921188354492 -9.2681188583374
19.005090713501 -12.3200712203979
19.4536952972412 -4.42919874191284
15.687084197998 -12.3534641265869
18.0192947387695 -3.72448539733887
19.1700668334961 -9.37061214447021
17.7226943969727 -12.0767822265625
18.1924877166748 -11.1487073898315
20.0483779907227 -5.68253707885742
17.5271587371826 -9.40968608856201
17.535327911377 -8.23542976379395
20.3551807403564 -5.8895435333252
15.9993677139282 -2.63864135742188
18.5563507080078 -4.66838502883911
21.493335723877 -10.4074478149414
22.5661563873291 -9.82149505615234
18.3198261260986 -6.08477592468262
17.9994850158691 -7.82648181915283
20.3648777008057 -7.47887086868286
20.5192909240723 -7.16105842590332
17.3930549621582 -7.4846658706665
15.69140625 -2.50244617462158
16.4252300262451 -8.0748348236084
17.7320175170898 -6.3976469039917
18.3624362945557 -5.89917993545532
17.7476959228516 -11.7785930633545
21.3902835845947 -14.4957466125488
19.2477626800537 -8.0139274597168
17.0087223052979 -8.72621440887451
19.3266448974609 -7.83146810531616
16.6133251190186 -6.43090629577637
17.4152488708496 -10.4044227600098
15.1343145370483 -7.89992713928223
18.7864894866943 -1.89823722839355
19.6178760528564 -9.25776958465576
20.2744750976562 -11.0934677124023
19.1309146881104 -7.77958250045776
21.8948459625244 -8.51675796508789
19.7265892028809 -10.7592468261719
17.6196022033691 -12.9170331954956
19.3565521240234 -9.23924350738525
17.831428527832 -5.69915390014648
20.2795791625977 -12.3985986709595
16.8244895935059 -7.19459533691406
19.0353546142578 -9.52710151672363
17.3839645385742 -13.9908170700073
17.6871547698975 -7.29882192611694
20.299991607666 -9.48885822296143
18.3291282653809 -8.11207675933838
15.7886390686035 -10.5401363372803
18.9594974517822 -8.92251014709473
17.8592433929443 -12.8212146759033
17.3785305023193 -13.1820602416992
19.8003330230713 -9.61477565765381
20.9805164337158 -2.39218330383301
18.3203563690186 -8.36274147033691
17.7515869140625 -13.3161315917969
20.6590232849121 -9.96424961090088
17.9697399139404 -4.73429584503174
15.9288997650146 -10.0457334518433
21.2637958526611 -13.7371520996094
17.9818572998047 -4.34251165390015
16.8379211425781 -5.59605264663696
20.7570209503174 -9.43264484405518
20.4558753967285 -9.5645637512207
20.4664134979248 -5.54533195495605
18.9458141326904 -3.90643501281738
17.8131446838379 -8.7077169418335
17.5407981872559 -4.59194087982178
18.7000637054443 -9.45442676544189
18.6187496185303 -14.9000272750854
18.8824100494385 -7.4036750793457
19.4353408813477 -5.30726957321167
16.1562767028809 -10.1894407272339
17.347240447998 -6.45073127746582
18.9047355651855 -13.2359170913696
17.1480369567871 -6.93651056289673
22.5539779663086 -13.7563018798828
18.3119144439697 -7.36728763580322
17.209774017334 -5.38600826263428
20.5676536560059 -9.20527076721191
18.4352054595947 -6.11623477935791
21.581937789917 -12.2559518814087
18.3678207397461 -3.96725654602051
20.0869693756104 -8.97849178314209
18.4907932281494 -8.82750225067139
16.049108505249 -9.42682552337646
16.326732635498 -11.0490732192993
18.0272655487061 -10.3985223770142
17.7812175750732 -14.0687131881714
17.4031028747559 -10.0137729644775
18.8010635375977 -10.9238758087158
21.4267654418945 -6.65647029876709
18.4752216339111 -13.2676181793213
19.4676818847656 -7.0454683303833
18.3883171081543 -2.44372272491455
19.1763534545898 -12.1514797210693
21.4214153289795 -4.74815797805786
19.2049007415771 -7.54229497909546
19.7701721191406 -7.86046648025513
16.3288249969482 -9.9940013885498
18.0061569213867 -12.5508632659912
20.516056060791 -10.8653907775879
19.0619144439697 -11.4624176025391
20.641809463501 -2.26286172866821
20.9438381195068 -6.1688084602356
17.6284008026123 -16.9741439819336
16.2691097259521 -4.36061382293701
19.4580402374268 -3.38784408569336
18.2197227478027 -5.56709718704224
20.7830219268799 -15.9860382080078
19.0985221862793 -13.7275953292847
15.7176809310913 -10.7628393173218
18.7579364776611 -11.0883417129517
17.4883232116699 -4.57828569412231
16.9190711975098 -5.94501972198486
15.966588973999 -6.08327674865723
16.4617519378662 -8.88134002685547
17.0785579681396 -11.4025192260742
19.2062320709229 -11.4720907211304
20.7316989898682 -13.8299350738525
16.5796775817871 -7.0348596572876
21.5723075866699 -11.3458375930786
21.6544284820557 -4.54008674621582
17.3611106872559 -9.19881343841553
19.4963607788086 -8.05461883544922
19.6258659362793 -6.45642471313477
17.3531799316406 -9.28373718261719
18.4514102935791 -5.74170970916748
18.9954032897949 -2.74497556686401
19.3539218902588 -5.45962190628052
20.6413764953613 -8.17087745666504
18.4955921173096 -7.2814040184021
16.9124145507812 -12.6370134353638
19.6010322570801 -13.4001617431641
20.4137840270996 -10.0351552963257
16.6786804199219 -7.53176927566528
20.3044452667236 -5.41483640670776
17.3843326568604 -7.8643159866333
16.8723526000977 -5.85054016113281
19.7287693023682 -4.07130193710327
18.8954105377197 -4.99053287506104
23.6109638214111 -7.98936319351196
18.9280300140381 -9.78514003753662
24.4962730407715 -8.31124591827393
15.422191619873 -5.87760353088379
20.1153221130371 -2.35951709747314
19.4334735870361 -8.48489952087402
20.9650459289551 -7.14084529876709
21.604736328125 -3.82926940917969
20.7074165344238 0.880450248718262
16.4781017303467 -8.24639511108398
21.2241802215576 -10.920524597168
20.2801036834717 -10.0250720977783
18.5527839660645 -3.46350765228271
15.5546703338623 -4.11843585968018
20.7765960693359 -6.33407688140869
19.0385627746582 -6.06601428985596
19.575569152832 -6.21194839477539
18.3347511291504 -8.99586200714111
18.6265621185303 -11.6905574798584
18.8153400421143 -9.32655811309814
22.9046936035156 -12.1268968582153
16.9091758728027 -13.6629209518433
16.6019420623779 -7.52863121032715
18.3910102844238 -11.5431604385376
17.8939304351807 -10.1612548828125
17.8935089111328 -2.01692199707031
16.4285469055176 -5.64352512359619
21.5274600982666 -12.172492980957
17.6682872772217 -10.6267471313477
19.2911205291748 -6.68903827667236
19.9685688018799 -8.42063999176025
18.9078712463379 -11.9515295028687
18.4756832122803 -8.72490119934082
18.5371379852295 -9.80549049377441
19.99635887146 -7.5330286026001
20.2568702697754 -9.4517068862915
19.9735660552979 -5.76949787139893
19.653865814209 -11.0220365524292
20.0211315155029 -8.21287059783936
17.0281677246094 -11.2032299041748
19.5709552764893 -10.6290531158447
17.878023147583 -3.77292060852051
21.5667343139648 -11.5306797027588
19.4199600219727 -6.09490966796875
18.52467918396 -10.1273403167725
17.5473098754883 -4.96126461029053
20.3525352478027 -4.2716760635376
18.4246482849121 -10.8632097244263
18.512731552124 -8.23349475860596
19.6411991119385 -12.0642919540405
18.3871250152588 -4.36872720718384
18.629789352417 -11.2384338378906
18.2370834350586 -9.81337833404541
19.7483062744141 -0.963895320892334
23.3712539672852 -7.05444288253784
18.1761722564697 -16.6659297943115
21.5117835998535 -7.29669380187988
18.3461952209473 -13.6317882537842
17.4917392730713 -8.72249889373779
19.1853332519531 -11.9615020751953
19.614953994751 -14.294490814209
15.9400043487549 -4.74525451660156
20.1480236053467 -7.41332387924194
17.0263500213623 -5.58470058441162
18.2917766571045 -4.43486261367798
17.4106960296631 -8.06837177276611
16.4678554534912 -8.24535655975342
17.8188591003418 -5.42008972167969
18.4154357910156 -6.9410343170166
16.8659114837646 -9.00000953674316
19.7779998779297 -7.51461029052734
20.6402339935303 -3.87838506698608
19.522481918335 -8.97218608856201
18.6772975921631 -13.157075881958
19.4307632446289 -8.08718872070312
17.3969535827637 -10.7444839477539
20.6248531341553 -11.4909439086914
17.1844787597656 -7.76436424255371
19.7664432525635 -1.64048099517822
21.0230388641357 -12.9756784439087
18.7406940460205 -15.9233455657959
15.8175859451294 -8.98707866668701
21.3626708984375 -7.01128530502319
19.6924095153809 -10.9317531585693
18.6189098358154 -5.18464946746826
17.9394798278809 -3.43084049224854
18.7872734069824 -9.05331707000732
19.9184532165527 -7.00304317474365
19.6482105255127 -7.02598190307617
18.8171329498291 -10.4372034072876
17.8569564819336 -11.5006856918335
21.0260810852051 -10.8816471099854
18.4914207458496 -2.20088148117065
18.1726989746094 -14.2931118011475
17.5615882873535 -8.72826671600342
18.9701862335205 -6.24258852005005
17.8225746154785 -7.1964282989502
20.0062141418457 -9.48693084716797
21.1865100860596 -6.31736946105957
18.9046077728271 -9.07306671142578
21.3147754669189 -10.5283527374268
17.8767433166504 -10.5509004592896
20.250862121582 -8.90476608276367
15.4372482299805 -7.2205982208252
19.5915012359619 -7.21922779083252
20.7444152832031 -4.62686443328857
19.7914810180664 -7.07927703857422
20.0047912597656 -5.82778930664062
19.8223762512207 -8.61170482635498
18.9516639709473 -7.54403114318848
19.1214618682861 -7.25669193267822
19.5919647216797 -2.7883415222168
17.7361431121826 -8.01049041748047
18.3238925933838 -11.2610292434692
20.8571147918701 -8.7088041305542
18.0731525421143 -3.08716440200806
20.0297832489014 -6.53061485290527
19.7129955291748 -10.2837238311768
21.705005645752 -5.46071434020996
16.5947952270508 -16.1389770507812
18.9836006164551 -9.48622226715088
19.0729064941406 -14.3135242462158
19.2644805908203 -8.88505172729492
19.8937244415283 -9.24057483673096
18.2221069335938 -10.911563873291
17.560754776001 -11.0093307495117
16.6144065856934 -8.86348628997803
17.6104621887207 -14.9679412841797
19.0039157867432 -16.045524597168
15.909686088562 -8.09965229034424
19.7446784973145 -13.8198261260986
17.249584197998 -10.255392074585
22.9629192352295 -10.6629209518433
17.7707977294922 -15.0058460235596
18.2217960357666 -9.39574432373047
18.9070491790771 -11.4583616256714
17.7292766571045 -10.7669878005981
18.5573616027832 -12.9806728363037
20.4082870483398 -6.85597515106201
19.5809917449951 -9.41250228881836
18.180290222168 -9.88441371917725
18.9115238189697 -10.5723543167114
15.8879318237305 -6.91210746765137
17.4090194702148 -6.22511577606201
19.9374313354492 -9.47538757324219
16.3554763793945 -15.9607410430908
22.0807933807373 -10.8961563110352
20.8902072906494 -11.1562776565552
16.6121406555176 -12.1172542572021
15.1213483810425 -7.86383867263794
18.0904521942139 -9.98142623901367
19.6348915100098 -10.955662727356
18.4238758087158 -12.5368061065674
19.4938449859619 -7.23473310470581
17.9387168884277 -6.88054656982422
18.7676849365234 -6.61523342132568
17.7027645111084 -11.6334857940674
16.781665802002 -12.1072406768799
20.2989807128906 -12.1818151473999
19.1015434265137 -5.9730224609375
21.8749370574951 -6.18337631225586
18.4824180603027 -10.122950553894
23.2242565155029 -9.13412380218506
18.351203918457 -8.0132474899292
18.912899017334 -2.15211868286133
19.4057502746582 -8.98323440551758
17.2782878875732 -6.83456182479858
17.6762180328369 -8.2733736038208
19.8423919677734 -5.89618825912476
19.3878784179688 -9.12879848480225
17.7556552886963 -11.9478883743286
20.9485168457031 -7.19460916519165
21.275333404541 -10.8630990982056
18.2571353912354 -8.49036693572998
15.7998819351196 -9.66347503662109
20.8157653808594 -6.22993040084839
18.7366886138916 -11.4977951049805
19.771505355835 -11.5409088134766
16.5297908782959 -12.4011259078979
18.2141361236572 -11.4174947738647
18.071195602417 -4.03358268737793
17.5487899780273 -5.38067054748535
19.2200756072998 -4.21626281738281
18.9959487915039 -2.8196063041687
19.6443862915039 -7.16225385665894
19.6271533966064 -7.50279998779297
16.4910411834717 -4.74041080474854
17.2805461883545 -6.54853057861328
16.7568645477295 -4.85948753356934
17.1279544830322 -14.7523860931396
16.2115287780762 -5.25921821594238
17.7919120788574 -10.7249822616577
17.8446254730225 -2.22133541107178
20.4008235931396 -8.38631820678711
17.284200668335 -5.42821264266968
19.2616958618164 -12.2044916152954
21.8264541625977 -7.48696756362915
18.8131561279297 -7.51511812210083
18.1616916656494 -5.65053844451904
18.0207767486572 -9.3453426361084
20.1775360107422 -10.7313184738159
17.8320140838623 -8.93113136291504
21.3176231384277 -10.1119375228882
17.9893646240234 -3.44248390197754
16.9777488708496 -5.65576171875
16.07861328125 -7.61284828186035
21.9129009246826 -3.08783721923828
18.8155574798584 -4.96560001373291
18.4558048248291 -4.44132518768311
17.8211669921875 -6.52870559692383
18.785852432251 -10.7578430175781
15.2586135864258 -7.19475841522217
22.6931056976318 -8.35401058197021
17.5954647064209 -8.08962059020996
17.7868919372559 -11.4512424468994
21.0223197937012 -5.08294773101807
19.2715263366699 -11.996973991394
19.2039585113525 -8.16062450408936
17.180290222168 -5.67183637619019
17.4164886474609 -8.19597625732422
20.3957118988037 -10.7156410217285
18.1022186279297 -7.30653285980225
18.818775177002 -10.7075910568237
19.053295135498 -14.7635898590088
16.334342956543 -11.5401668548584
19.0938358306885 -11.0207576751709
17.5117645263672 -6.32705688476562
17.0927028656006 -5.96650981903076
18.0421009063721 -4.51166248321533
18.6093692779541 -8.09049224853516
19.0549964904785 -11.3519954681396
21.8795890808105 -8.38852977752686
15.5317325592041 -7.31385564804077
17.2335777282715 -10.9797592163086
15.2402095794678 -2.59055519104004
18.3872413635254 -18.5015296936035
21.1015357971191 -10.158411026001
16.836576461792 -14.0939807891846
18.0575160980225 -9.8891773223877
19.5140228271484 -0.173049926757812
17.3691825866699 -9.71265411376953
18.1942443847656 -8.14446544647217
18.5906257629395 -6.40492534637451
18.4642105102539 -4.22529268264771
16.0285472869873 -13.51735496521
17.4834785461426 -6.97843408584595
20.603609085083 -5.11487483978271
18.2210330963135 -9.49188423156738
19.1197261810303 -8.38607883453369
20.4063491821289 -14.6637535095215
18.0143909454346 -11.8235187530518
19.8547801971436 -6.09842538833618
16.0703659057617 -9.52679443359375
21.9789791107178 -9.09784889221191
19.9151554107666 -10.3994474411011
19.3754825592041 -9.38022899627686
19.2579727172852 -7.29052305221558
19.177734375 -7.84850215911865
18.4990901947021 -9.16698741912842
18.5455684661865 -11.7278928756714
20.0116901397705 -8.16928005218506
18.0461540222168 -10.1831302642822
19.824779510498 -10.4091491699219
18.267110824585 -9.12536239624023
14.7840957641602 -9.67742347717285
20.001148223877 -14.7790498733521
18.7589645385742 -7.40989971160889
21.8970031738281 -5.83354187011719
18.220344543457 -11.2848510742188
21.0800132751465 -4.57764291763306
16.9013805389404 -12.7423791885376
19.6950244903564 -8.44592475891113
20.5758876800537 -10.0714883804321
18.4321002960205 -7.10688447952271
18.2054996490479 -13.4820947647095
18.6229343414307 -8.47765636444092
19.6442718505859 -11.4804201126099
19.4020843505859 -9.82413005828857
18.151611328125 -8.46566677093506
19.3484058380127 -15.486499786377
19.103084564209 -11.2117919921875
21.0549755096436 -8.55007171630859
20.6737308502197 -12.0650177001953
18.0340538024902 -12.8204126358032
17.7453079223633 -6.20419502258301
20.8181762695312 -9.36752128601074
17.9014739990234 -16.2805557250977
19.76735496521 -10.6284055709839
16.6847400665283 -7.38142538070679
18.3327503204346 -17.3424949645996
18.3642730712891 -9.3764533996582
19.7241859436035 -7.05777168273926
17.6004028320312 -11.1015777587891
16.8858985900879 -7.02697420120239
20.5014152526855 -7.58475255966187
20.6520919799805 -6.01063823699951
17.5811157226562 -2.7566876411438
20.2892971038818 -12.0306396484375
16.2978820800781 -7.97268009185791
19.8195209503174 -7.28418588638306
19.0603656768799 -17.7407341003418
18.6452541351318 -8.996413230896
21.2209854125977 -14.4726638793945
18.5327606201172 -6.13238334655762
21.8570365905762 -7.94336414337158
17.6727256774902 -3.53242254257202
21.0924835205078 -6.46489524841309
19.9327564239502 -7.59548854827881
19.6336574554443 -3.3160252571106
19.561450958252 -6.17460155487061
18.7278079986572 -4.91192150115967
19.6360893249512 -13.0805072784424
16.9326705932617 -4.25070381164551
17.7550106048584 -3.73291301727295
16.8989410400391 -7.00768327713013
20.8058681488037 -12.290225982666
16.9367160797119 -10.99547290802
17.8273906707764 -8.6289529800415
17.7994384765625 -9.05690479278564
17.4648571014404 -12.3859996795654
17.3150653839111 -16.1415920257568
20.281120300293 -8.5056848526001
19.5213356018066 -7.12919950485229
17.5490989685059 -5.54473114013672
20.5964908599854 -9.98812675476074
16.3937091827393 -14.8896512985229
19.5299339294434 -12.0990257263184
16.518217086792 -14.7833824157715
19.3073596954346 -5.10340213775635
18.407377243042 -6.73842763900757
19.5744533538818 -7.70548391342163
18.9738311767578 -5.99936485290527
16.5307350158691 -9.18462753295898
16.8556499481201 -7.80026388168335
19.510440826416 -13.9986896514893
21.1076393127441 -3.31895446777344
20.6886081695557 -9.44257545471191
19.2393474578857 -14.6976871490479
18.7409648895264 -12.8251457214355
18.0176029205322 -10.7703914642334
18.2980041503906 -3.8820629119873
18.7709217071533 -6.1845006942749
20.4317970275879 -12.5246124267578
19.8588676452637 -3.99516010284424
20.4003028869629 -9.15499973297119
16.6684646606445 -14.8910350799561
19.8934364318848 -10.7235670089722
17.8999404907227 -9.8337230682373
21.2492561340332 -5.39308929443359
18.737886428833 -7.92187643051147
19.9076023101807 -15.7400932312012
17.6688289642334 -7.13514137268066
17.6502990722656 -11.8143339157104
18.3470115661621 -5.79884719848633
22.6072540283203 -2.82567071914673
17.4066505432129 -14.6878070831299
17.3519840240479 -7.41356182098389
17.2081508636475 -9.58645629882812
18.9016284942627 -13.3804912567139
18.7410221099854 -8.99157524108887
20.4674396514893 -8.86264228820801
19.6056461334229 -9.50702857971191
20.1424369812012 -10.2464275360107
21.4769515991211 -8.95613098144531
17.6051788330078 0.877640724182129
17.9617767333984 -9.52642631530762
19.2632350921631 -3.20699310302734
18.8094539642334 -6.2371244430542
20.0938892364502 -3.2121696472168
17.5565605163574 -7.06687116622925
18.4556427001953 -11.8760919570923
19.1474876403809 -8.60565090179443
20.7864780426025 -12.9532260894775
18.0018711090088 -5.52216053009033
15.2310266494751 -5.8346152305603
16.9288787841797 -6.10056161880493
18.9823379516602 -6.61178159713745
15.3467082977295 -3.37897539138794
18.4731941223145 -9.67388248443604
17.3923797607422 -6.74784421920776
17.6918258666992 -4.05346727371216
18.8436050415039 -5.72094058990479
18.0886688232422 -9.33548450469971
18.4425106048584 -11.5901498794556
16.2442321777344 -14.5724945068359
18.93434715271 -9.76797676086426
17.3396606445312 -9.27657985687256
23.2763328552246 -7.57596683502197
20.6612567901611 -6.53472900390625
15.3298664093018 -5.73932409286499
20.0093116760254 -7.28294324874878
16.5196628570557 -7.08129262924194
20.5038967132568 -1.66795969009399
17.7939529418945 -8.21238422393799
};


==> figures/visualizations/gmm40/pis_samples.tex <==
\addplot [semithick, pis, opacity=0.7, mark=*, mark size=3, mark options={solid}, only marks]
table {%
-3.33321166038513 -0.753214359283447
-2.06448674201965 0.603443264961243
-1.7477525472641 1.38335919380188
-2.20405387878418 0.75313401222229
-3.92750859260559 0.33832910656929
-3.25607562065125 2.36103630065918
-3.87237358093262 2.80768656730652
-3.58105182647705 1.94210636615753
-4.90826654434204 2.47184634208679
-3.21768021583557 -0.0942877158522606
-2.67286968231201 1.19012105464935
-3.27345156669617 0.245988190174103
-1.03185951709747 2.14080333709717
-3.08186221122742 2.94008374214172
-4.32495069503784 1.65178155899048
-3.03918266296387 1.16808426380157
-3.77327275276184 1.83369183540344
-2.46915483474731 0.745506048202515
-2.06423664093018 -1.11610913276672
-4.21559953689575 1.99740266799927
-3.43965435028076 0.304575979709625
-2.87985348701477 1.7991818189621
-3.90998482704163 0.610598385334015
-2.36119771003723 -0.670643270015717
-2.80308890342712 0.333267211914062
-2.65340614318848 1.02763175964355
-2.63472867012024 1.71406686306
-3.64038848876953 0.350729405879974
-3.93750524520874 3.48020482063293
-3.09742975234985 4.27921581268311
-2.14876103401184 1.69317328929901
-2.62254166603088 0.654772460460663
-2.95895552635193 2.07563519477844
7.55366182327271 4.70527076721191
-3.03648161888123 0.898173928260803
-3.87340044975281 -0.665806949138641
-2.66049790382385 0.140748009085655
-3.21104121208191 -0.0250496305525303
-2.59690856933594 0.140331447124481
-4.28815412521362 -0.394190788269043
-3.52069926261902 1.09780621528625
-2.50199437141418 0.400674760341644
-3.45173048973083 0.453738033771515
-2.7476212978363 2.25571346282959
-1.44455480575562 0.694451808929443
-1.31908273696899 1.52199470996857
-3.72046089172363 -0.565612852573395
-3.36508059501648 0.962269008159637
-3.03100347518921 2.08574676513672
-0.274435758590698 0.51974231004715
-3.13132166862488 0.825800955295563
-1.72998464107513 1.16271150112152
-1.68598294258118 2.24186372756958
-4.93202209472656 3.55164980888367
-2.062251329422 0.897336006164551
-2.84826946258545 2.05144834518433
-1.55996954441071 0.363806217908859
-0.731070637702942 -0.0679998397827148
-2.3971586227417 1.76154482364655
-3.12083387374878 1.5634663105011
-3.01637601852417 2.05021858215332
-3.34545421600342 1.24539053440094
-4.08206224441528 1.9866281747818
-0.994202554225922 -0.931201040744781
-3.08462691307068 0.681102573871613
-3.57603788375854 1.30027878284454
-3.51846146583557 0.548588395118713
-0.995164692401886 1.35123360157013
-3.71198773384094 -0.688007473945618
-2.81664824485779 0.0732262507081032
-3.03579521179199 1.04791688919067
-3.29309701919556 -1.57046687602997
-3.50721716880798 0.915277183055878
-1.68881392478943 1.79715192317963
-2.07443928718567 0.358196765184402
-2.83696603775024 1.09407377243042
-2.66803216934204 0.883816123008728
-2.15796661376953 2.23978304862976
-3.03049254417419 1.13900697231293
-4.11100578308105 3.350581407547
-4.19866561889648 1.20501828193665
-2.42264914512634 2.29820346832275
-3.25430202484131 2.23043656349182
-4.81060647964478 -0.542062640190125
-0.863909184932709 1.25868272781372
-1.34035122394562 2.17939400672913
-4.15015506744385 -0.651675760746002
-3.3196849822998 3.35256004333496
-1.38746190071106 1.23902893066406
-2.86511325836182 -0.131889924407005
-2.58180332183838 3.73721575737
-2.96293973922729 1.04068303108215
-2.61558103561401 1.74131107330322
-0.847855687141418 1.20119035243988
-1.69813811779022 2.7682900428772
-3.21783685684204 3.52490639686584
-2.56154608726501 3.0075352191925
-1.24918937683105 0.555229842662811
-2.93798351287842 2.07230639457703
-3.24475765228271 1.9644718170166
-0.732895255088806 0.29626789689064
-2.2982337474823 1.52604675292969
-4.16630029678345 2.60014867782593
-1.77678656578064 1.27001917362213
-2.06779456138611 0.495537519454956
-2.34217572212219 2.76454925537109
-2.93935799598694 -0.424735397100449
-2.04253911972046 2.05611562728882
-2.65718245506287 -0.685599207878113
-2.25333666801453 1.0475105047226
-2.4027681350708 2.02584290504456
-1.90206205844879 1.53972554206848
-2.60766363143921 -1.13397121429443
-1.23515498638153 -0.512699007987976
-2.21304726600647 1.48374247550964
-1.90283727645874 0.617866814136505
8.02728366851807 5.2495265007019
-0.354196101427078 -0.229740530252457
-2.56832265853882 0.877350330352783
-1.71523761749268 2.06545424461365
-4.10224962234497 -0.109896212816238
-1.26806926727295 2.94092845916748
-2.21177172660828 1.06038701534271
5.77583694458008 2.65510630607605
-1.72632133960724 2.02242493629456
-1.70858263969421 0.692294657230377
-3.98903799057007 1.42684423923492
-4.96628761291504 -1.17153537273407
-1.77739584445953 0.70029628276825
-2.9300971031189 1.51242852210999
-2.74444055557251 0.9314244389534
-2.8448793888092 1.77354991436005
-1.18971741199493 1.87656486034393
-1.61893546581268 -0.382606387138367
-1.89476478099823 1.43261969089508
-4.14945602416992 0.290349245071411
-2.95195770263672 1.78770291805267
-3.92817354202271 1.30153405666351
-3.34415078163147 2.58145713806152
-2.62362313270569 1.66987025737762
-3.70093894004822 -1.41295063495636
-3.81884956359863 1.61435437202454
-2.86347126960754 -1.29497528076172
-1.47078239917755 1.26771140098572
-1.96358478069305 2.03201484680176
-3.6528697013855 1.45311188697815
-4.43464517593384 0.355918943881989
-2.95952010154724 3.18628692626953
-2.16215300559998 1.75013637542725
-2.90431785583496 0.807224750518799
-3.66840934753418 0.930291950702667
-2.94015002250671 -1.33841717243195
-2.029616355896 1.0152245759964
-4.05941724777222 1.83713185787201
-4.43030834197998 1.2980090379715
-3.97367572784424 0.839999496936798
-2.49080276489258 2.35364365577698
-3.29081153869629 2.06488585472107
-2.04697489738464 1.87470757961273
-4.55979537963867 1.60443091392517
-3.97972393035889 2.13576912879944
-3.42762684822083 -0.457576900720596
-4.04169797897339 0.268102288246155
-1.22763562202454 2.61136555671692
-2.51625156402588 2.10908079147339
-3.27030944824219 0.247114643454552
-2.98497986793518 1.40362083911896
-1.54489839076996 0.826136708259583
-2.52555871009827 1.38095080852509
-4.08556461334229 2.37458229064941
-2.72833061218262 1.40477466583252
-3.37318420410156 2.10552453994751
-4.42343425750732 0.174212664365768
-2.45492434501648 0.987873315811157
-1.73770928382874 1.51307332515717
-3.04264497756958 1.79401683807373
-1.81387066841125 2.46513366699219
-1.98876011371613 0.135923638939857
-1.67282629013062 0.378544420003891
-5.81337738037109 3.21996545791626
-2.92967414855957 0.444972634315491
-3.67915034294128 2.65082764625549
-2.70571708679199 3.32650709152222
-2.63221740722656 -0.909862995147705
-3.05367588996887 1.07439720630646
-3.1676037311554 1.78023314476013
-2.60830450057983 0.0791343823075294
-3.01659059524536 1.88375794887543
-3.78779172897339 1.87698984146118
-4.13883066177368 0.72539222240448
-0.670656085014343 2.1215488910675
-2.40711402893066 1.59156262874603
-1.90707898139954 0.775954008102417
-2.47611117362976 0.0863326340913773
6.11072969436646 0.318405836820602
-2.03656196594238 1.36161839962006
-3.91760110855103 0.389534115791321
5.6899790763855 3.8548891544342
-2.0801956653595 1.45665013790131
-1.59357511997223 1.19721603393555
-3.78849053382874 2.13306617736816
-2.92195582389832 1.16980600357056
-4.15133571624756 1.2760648727417
-1.51723265647888 -1.09368228912354
-2.81911635398865 1.59184801578522
-0.779349207878113 2.36675405502319
-3.61910510063171 1.74704313278198
-4.57952785491943 1.46379554271698
-4.97718143463135 0.481353908777237
-2.65103673934937 1.02679765224457
-2.88117456436157 2.39854025840759
-3.65078234672546 1.69296443462372
-4.9433650970459 0.996228098869324
-0.539165377616882 0.526243984699249
-3.13236713409424 0.721741616725922
-2.17618799209595 1.59972393512726
-3.43244814872742 0.273361951112747
-1.80022096633911 1.42487156391144
-4.7239818572998 -0.805424451828003
-2.86600661277771 1.71843302249908
-1.58907508850098 -0.0820573419332504
-3.96264052391052 0.710224509239197
-3.33474159240723 1.93434476852417
-2.32945775985718 0.86467444896698
-3.77920722961426 1.69446444511414
-1.58599162101746 1.19396650791168
-2.40682792663574 0.0573180951178074
-2.98614978790283 1.48747336864471
-3.66576647758484 0.854663610458374
-2.42118167877197 3.4677517414093
-2.9052402973175 1.57809019088745
-2.51018762588501 1.20278000831604
-1.73159658908844 0.714101374149323
-1.99228870868683 -0.395890742540359
-2.00182199478149 2.34738802909851
-4.46053457260132 0.915088534355164
-3.01398086547852 -0.557209610939026
-3.60129332542419 1.55476653575897
-0.99374121427536 1.11584460735321
-2.98126792907715 2.17422986030579
-1.71166598796844 0.796633660793304
-2.5201370716095 0.525349497795105
-3.02294540405273 1.38944947719574
-3.0243604183197 0.823187172412872
-1.28823912143707 1.20660948753357
-1.34359467029572 2.24812197685242
-4.86777877807617 -0.0312782488763332
-3.70733380317688 1.71394062042236
-2.95887041091919 2.27286672592163
-3.76422071456909 0.967285513877869
-3.37832093238831 0.990444660186768
-2.90359139442444 3.40389895439148
-3.72618746757507 0.209974780678749
-2.19163751602173 -0.476306796073914
-2.72519111633301 0.559818923473358
-4.88916397094727 0.0343019254505634
-1.44894421100616 0.671063661575317
-1.81134212017059 2.41261124610901
-3.62467217445374 -0.709851145744324
-2.9674015045166 1.28236627578735
-2.39995837211609 0.215869709849358
-3.15231394767761 3.75021004676819
-2.96541285514832 0.20263484120369
-2.69133639335632 0.463698863983154
-1.94006657600403 1.93544399738312
-2.66895031929016 2.13543581962585
-2.64695024490356 -0.227716878056526
-1.92637825012207 2.53631114959717
-4.06961488723755 1.28622698783875
-3.04065823554993 2.39984321594238
-1.25456774234772 2.45524621009827
-4.07497072219849 1.95546841621399
-1.48673927783966 0.906140685081482
-1.49484491348267 0.157046034932137
-2.93409037590027 -0.160288631916046
-2.92197585105896 0.653968393802643
-4.33907890319824 -0.911317765712738
-3.56369280815125 1.84370958805084
-1.98382461071014 1.04479110240936
-2.92361283302307 0.792670249938965
-3.49138188362122 -0.335394442081451
-3.06556510925293 2.33285403251648
-1.44867742061615 0.195219859480858
-2.98722648620605 -0.0763848572969437
-3.60094809532166 4.77139806747437
-1.40493106842041 -1.5286191701889
-3.98755025863647 2.2229015827179
-3.04761433601379 0.488028228282928
-3.35991597175598 -0.0940956398844719
-2.1764714717865 0.00632690172642469
-2.65164685249329 -0.415218263864517
-1.69899725914001 0.519334137439728
-1.43875920772552 0.450753033161163
-1.85051476955414 0.818025708198547
-1.38447141647339 2.73151183128357
-1.85440182685852 0.747893929481506
-3.7399890422821 2.07184815406799
-1.92799985408783 -0.276657938957214
-2.31588268280029 1.65318727493286
-3.00501942634583 -0.0444907136261463
-1.6345362663269 0.677444815635681
-3.99103116989136 1.22358322143555
-0.831847310066223 2.11104440689087
-4.34914302825928 -1.86880612373352
-3.99164247512817 1.97933423519135
-3.13096594810486 3.07806205749512
-3.43519854545593 0.0540388748049736
-3.13084101676941 1.88598537445068
-3.33956742286682 2.89407777786255
-3.37854623794556 0.623337686061859
-3.4140522480011 1.53002512454987
-2.11117744445801 0.577496826648712
-3.44180178642273 2.08473134040833
-1.29073214530945 1.87277138233185
-1.89614057540894 1.51431572437286
-1.60919964313507 0.144204929471016
-3.69335436820984 -0.596815764904022
-3.52889752388 2.28546571731567
-2.76890325546265 1.18240189552307
-3.4595468044281 1.92650473117828
-1.76027011871338 1.15252470970154
-3.0159010887146 2.50873899459839
-3.52710032463074 2.18719172477722
-5.0576605796814 4.00910139083862
-3.78838634490967 3.43139815330505
-2.49348998069763 2.24921941757202
-3.36568808555603 0.434869050979614
-0.900548934936523 1.74368143081665
-3.84932208061218 -0.18521611392498
-1.55953466892242 0.920331239700317
-3.33736181259155 -0.252969682216644
-1.64114737510681 0.914178431034088
-3.17627239227295 2.57939434051514
-3.07368350028992 1.28166520595551
-0.331363022327423 0.824356436729431
-2.90587377548218 0.601565480232239
-2.93584418296814 0.757481098175049
-1.79536199569702 1.05242121219635
-2.63895010948181 -0.0494170673191547
-5.49377012252808 0.984588146209717
-2.60636878013611 1.66264092922211
-3.79998087882996 2.80057072639465
-1.68437683582306 0.682577729225159
-4.60782623291016 0.345956832170486
-3.19890999794006 2.15078520774841
-2.02666711807251 0.204253897070885
-1.51468443870544 0.179382666945457
-1.9613242149353 0.513652801513672
-2.72874021530151 1.5383415222168
-0.72256475687027 1.42154800891876
-3.76378703117371 2.52755284309387
-1.6039879322052 0.241232857108116
-3.45110034942627 0.48840993642807
-1.83995974063873 2.48701405525208
-1.24255573749542 2.22014379501343
-2.30141139030457 3.31660008430481
-3.60970282554626 3.10992193222046
-1.01660513877869 1.41771376132965
-1.89526045322418 1.1940770149231
-3.25928330421448 -1.41468048095703
-3.12309718132019 1.62076580524445
-2.0892128944397 2.60607028007507
-3.28963303565979 3.10476279258728
-3.89097452163696 2.0659453868866
-3.29056024551392 0.922946453094482
-2.30643558502197 0.462917983531952
-2.52639698982239 1.4099406003952
-2.45254015922546 2.39091372489929
-1.52526414394379 -0.831293344497681
-2.56981754302979 1.01416742801666
-4.13105249404907 0.523674309253693
-2.01130890846252 3.60862445831299
-3.12648916244507 1.48522472381592
-1.80358338356018 2.0589804649353
-3.51737213134766 1.14701449871063
-3.27415561676025 0.222300082445145
-1.92716419696808 -0.0555409342050552
-2.02259111404419 0.759780704975128
-1.75084257125854 1.18173348903656
-4.39218044281006 1.84102296829224
-2.90836381912231 1.57047295570374
-2.39212274551392 1.38858675956726
-1.61661601066589 2.22968673706055
-2.66097187995911 1.28776037693024
-3.67075157165527 1.18496906757355
-1.29391014575958 0.610938131809235
-2.74245119094849 1.98283541202545
-4.54346561431885 0.783056616783142
-3.15182757377625 0.504817962646484
-3.12297463417053 -0.468920767307281
-2.38706207275391 2.33028244972229
-2.63864421844482 1.57957208156586
-3.6184995174408 1.44615232944489
-2.65628671646118 1.0120952129364
-2.02938199043274 1.90193724632263
-1.90369081497192 1.04814803600311
-3.8531014919281 1.41879653930664
-2.94868731498718 2.81346082687378
-1.73344123363495 -0.23735585808754
-2.06353831291199 0.978321731090546
-2.82133960723877 0.799607932567596
-4.18796110153198 1.56646859645844
-1.83456981182098 0.707203984260559
-2.11345648765564 1.14079916477203
-2.21184062957764 1.12055850028992
-2.29058289527893 2.51357626914978
-3.09339308738708 3.65900731086731
-3.59779739379883 1.29385709762573
-3.63375163078308 0.686959028244019
-3.579509973526 -0.388216614723206
-3.45696496963501 3.38448190689087
-2.28446245193481 0.735841393470764
-3.67115879058838 1.5259667634964
-2.61580324172974 0.586176037788391
-4.28156089782715 0.883512377738953
-2.53458261489868 2.10462379455566
-2.21904683113098 -1.36265313625336
-0.576282382011414 0.540547430515289
-1.55701947212219 1.56794583797455
-2.17510271072388 0.886181116104126
6.6849799156189 5.08847427368164
8.21084880828857 3.06416702270508
-3.69991016387939 1.27348375320435
-2.71237277984619 0.435801714658737
-2.82549738883972 -0.839798510074615
-3.5705509185791 0.840404570102692
-1.75155758857727 1.24744689464569
-2.47953510284424 0.646558165550232
-2.68722701072693 0.0494939237833023
-1.0985244512558 0.543860375881195
-2.50284886360168 0.887289106845856
-2.9043025970459 -0.00843830965459347
-3.28123354911804 1.97184944152832
-4.89753866195679 0.886496067047119
-2.5206184387207 -0.728822827339172
-3.65277552604675 2.20417904853821
-4.66942596435547 0.96258807182312
-2.13379526138306 0.289559572935104
-1.75181698799133 0.845646440982819
-3.66556406021118 2.21825051307678
-1.94795382022858 0.561647236347198
-1.53203475475311 0.154461741447449
-2.64563941955566 2.256756067276
-3.12370300292969 1.99022924900055
-1.50835907459259 0.998306453227997
-0.994441568851471 0.610466599464417
6.95576000213623 4.24215221405029
-3.59026384353638 1.0437479019165
-2.13089156150818 1.45923161506653
-3.03251242637634 1.53466284275055
-1.72261679172516 0.645617663860321
-2.2873592376709 1.22545564174652
-2.55045866966248 1.30878674983978
-1.9201648235321 1.65458142757416
-2.80457782745361 1.68615627288818
-0.928412735462189 1.5725269317627
-2.80265641212463 0.265765517950058
-2.67429685592651 1.91631627082825
-2.1367609500885 1.53019797801971
-2.31733536720276 3.12395739555359
-1.95065331459045 0.575402438640594
-3.10992860794067 2.18164825439453
-2.77058029174805 0.723643481731415
-2.41952300071716 0.561177730560303
5.91172885894775 3.61723446846008
-2.41268372535706 1.0683114528656
0.877509295940399 1.49878692626953
-4.28146982192993 1.1295599937439
-2.60622358322144 0.240051731467247
-2.33450317382812 0.880358457565308
-3.23188996315002 1.50464928150177
-3.19252562522888 2.49719905853271
-2.82435727119446 0.231885328888893
-2.7929093837738 -0.511784315109253
-1.96129775047302 1.61436295509338
-2.01590180397034 2.77233791351318
-4.25468444824219 0.91478443145752
-3.0798978805542 -0.2702357172966
-4.12945365905762 -1.31781435012817
-3.21463942527771 1.80387055873871
-3.53633284568787 0.957708179950714
-2.39279723167419 0.746330797672272
-3.34719777107239 1.8888144493103
-2.016526222229 1.25919008255005
-1.56630611419678 0.563932716846466
-3.32970094680786 1.14509284496307
-2.83330678939819 0.961445808410645
-1.57538306713104 0.98150235414505
-3.56931495666504 0.269478738307953
-4.08957290649414 0.736624181270599
-2.69887161254883 1.36839532852173
-4.36279058456421 1.48365533351898
-3.70189571380615 2.24625992774963
-1.98437523841858 3.76689720153809
-2.60439467430115 -1.35061609745026
-1.60165357589722 0.79801744222641
-2.44666504859924 0.613550007343292
-3.0230119228363 2.80561780929565
-2.53598833084106 2.5385947227478
-0.981503367424011 0.720361590385437
-2.38088822364807 0.482634127140045
-0.780612587928772 2.42467093467712
-1.99916017055511 0.793435096740723
-4.1353645324707 2.11626768112183
-2.80106520652771 2.26501750946045
-1.80971395969391 1.57865643501282
-3.83976936340332 1.74668598175049
-3.01916694641113 0.0722749978303909
-4.72404384613037 -0.674591064453125
-2.65096640586853 -0.217084154486656
-2.11231923103333 -0.093942828476429
-2.6717517375946 -0.399949073791504
-2.38350510597229 1.26868867874146
-1.7310791015625 2.08563637733459
-3.23758339881897 0.160634413361549
-3.25513386726379 2.38373041152954
-3.10163116455078 0.741085052490234
-3.53725290298462 1.80921268463135
-3.34732365608215 -0.840562164783478
-2.17581701278687 2.62750363349915
-2.70649981498718 1.54108166694641
-2.55875658988953 1.14571344852448
-4.35297250747681 0.218466207385063
-2.15225648880005 1.64195883274078
-3.49283027648926 -0.680060684680939
-2.28262734413147 0.843162059783936
-2.06559658050537 0.616185307502747
-1.39709484577179 0.951388835906982
-2.53029251098633 0.910961985588074
-2.36196804046631 1.80334317684174
-2.34874963760376 0.70258766412735
-0.754917919635773 1.12899768352509
-1.58134865760803 1.96729290485382
6.17575645446777 2.89569878578186
-2.78969192504883 0.659351050853729
-1.20868587493896 3.47269892692566
-1.08834838867188 1.87522900104523
-2.89984893798828 0.774007737636566
-1.63684892654419 -0.779062569141388
-2.93804383277893 0.93137913942337
-3.28464388847351 1.37056636810303
-2.25433111190796 1.3170759677887
-2.13938355445862 0.893712937831879
-3.98909759521484 0.941313683986664
-4.52332973480225 1.27310597896576
-3.00342583656311 1.73109984397888
-1.45378029346466 0.512707650661469
-3.34665012359619 0.00106011889874935
-0.935956180095673 2.4309823513031
-4.955153465271 0.435031563043594
-3.17834901809692 3.36536312103271
-2.91573071479797 1.70374441146851
5.33488512039185 1.93068408966064
5.09824419021606 4.91025018692017
-2.01032447814941 3.89142870903015
-3.66686916351318 2.30562710762024
-2.39659905433655 1.20669674873352
-3.17910885810852 -0.795056998729706
-2.1340434551239 1.1204069852829
-2.28318428993225 0.723362386226654
-1.36205589771271 0.541701912879944
-2.20802688598633 2.88581824302673
-1.52500259876251 3.02950215339661
-2.93614602088928 2.26288175582886
-4.56195402145386 2.16387987136841
-4.16205406188965 1.5991438627243
-2.27393388748169 1.53552341461182
-5.84668302536011 0.816058158874512
-1.95077085494995 1.98384320735931
-3.75345706939697 1.97971642017365
-4.01456928253174 1.76803255081177
-3.44453406333923 1.98573076725006
-2.76785349845886 -0.783954441547394
-2.02102446556091 1.52479982376099
-1.9385027885437 1.33904051780701
-3.01364374160767 1.93602812290192
-3.67700743675232 0.7208491563797
-2.94301509857178 1.99943768978119
-3.95560812950134 0.784113883972168
-3.36393237113953 1.04337441921234
-2.05677795410156 1.71772050857544
-1.55729353427887 0.458767950534821
-3.6425621509552 0.0618591234087944
-2.93842387199402 1.04147386550903
-2.07728409767151 2.60213375091553
-4.35563230514526 0.327867805957794
-4.35898351669312 1.03321707248688
-1.13731729984283 -0.642192900180817
-1.27350378036499 0.540619969367981
-1.58430552482605 1.74054396152496
-3.22755861282349 1.84830403327942
-4.01172637939453 -0.659656524658203
-2.67178392410278 1.20909547805786
-2.00778388977051 2.34270644187927
-1.58599150180817 -0.469518423080444
-3.71815347671509 -0.69188529253006
-2.08377361297607 2.4062488079071
-3.44690370559692 2.57510018348694
-4.92636251449585 0.998187303543091
-1.79683315753937 2.18260717391968
-2.04214143753052 2.99263572692871
-1.18724155426025 0.297548115253448
-0.679576873779297 2.29998898506165
-4.35338973999023 1.68819034099579
-1.04291903972626 -0.0656134113669395
-3.2093198299408 0.827346444129944
-3.97839713096619 -0.314615070819855
-4.47292041778564 -0.15629668533802
-1.63781046867371 -1.01293957233429
-2.5651433467865 1.7134040594101
-3.72278118133545 2.06821203231812
-3.51686644554138 0.755352318286896
-3.02822661399841 0.668314218521118
-3.20333695411682 -0.227061733603477
-1.64758765697479 1.24083137512207
-2.34380722045898 0.442862242460251
-0.258722871541977 -0.0221082977950573
-2.24217867851257 2.18130683898926
-3.3055272102356 0.201585158705711
-3.87608432769775 1.42281651496887
-2.7016613483429 2.49602580070496
-4.20923948287964 0.795269429683685
-3.53583431243896 0.994483470916748
-0.681205749511719 2.3343493938446
-1.50516724586487 -0.00862040091305971
-2.96913290023804 -0.579020380973816
-3.00037312507629 2.01702308654785
-2.48770833015442 1.69486880302429
-1.37428772449493 1.2509697675705
-2.63775205612183 1.98825287818909
-2.82236218452454 2.29645872116089
-2.74031782150269 1.06901967525482
-2.4895350933075 1.01518833637238
-2.79373717308044 0.237344682216644
-2.85001945495605 0.587344110012054
-0.687326788902283 0.942607343196869
-3.19616675376892 1.71731972694397
-1.85080444812775 1.86476719379425
-3.73952031135559 2.26325631141663
-2.91818904876709 1.83849847316742
-3.05775284767151 0.312025547027588
-2.3125114440918 0.930894136428833
-2.04486346244812 1.17077147960663
-3.81359267234802 1.79307949542999
-3.12678241729736 0.648547887802124
-2.2715859413147 0.632560908794403
-1.71736907958984 1.90684866905212
-3.04800510406494 1.3631706237793
-2.92142105102539 0.849053859710693
-2.83172297477722 0.691650688648224
-1.87408208847046 1.22402405738831
-3.18525385856628 1.3599773645401
-3.31929802894592 -0.223013132810593
-0.968730986118317 1.34162330627441
-2.47728133201599 0.885276198387146
-4.32734298706055 1.97960782051086
-3.46689915657043 1.67813408374786
-2.94360160827637 1.82152605056763
-2.81928563117981 0.489501953125
-1.92055332660675 0.685686469078064
-3.15189814567566 1.35359466075897
-3.19947981834412 0.233879014849663
-2.03756022453308 0.806741654872894
-3.8620069026947 1.35127580165863
-3.10189270973206 2.50812911987305
-2.23415637016296 2.86094832420349
-3.41128039360046 1.27981662750244
-2.78147983551025 0.783353328704834
-3.61217308044434 2.0993914604187
-1.67719173431396 0.566392123699188
-0.955453515052795 0.871007680892944
-2.76933217048645 -0.691103875637054
5.33489561080933 3.56528520584106
-3.37576508522034 1.90068852901459
-1.89427065849304 1.56302571296692
-4.9090142250061 0.389949381351471
-0.314571112394333 2.21654915809631
-1.77844095230103 1.82958042621613
-3.0348174571991 0.808858871459961
-2.27710795402527 -0.40116947889328
-4.64137935638428 -0.762592017650604
-1.14650452136993 0.0319917537271976
-2.75452661514282 1.08021414279938
-2.19128561019897 -0.833461225032806
-1.04432570934296 1.65034067630768
-1.78854012489319 0.451994895935059
-2.66727542877197 2.75941491127014
-3.16626214981079 1.69867742061615
-3.26803493499756 0.990765511989594
-1.44648969173431 -0.691851079463959
-3.17068243026733 1.38289487361908
-2.20398306846619 2.19302010536194
-2.07873153686523 1.18305766582489
-1.90923833847046 0.735714614391327
-1.99949359893799 1.95263838768005
-3.71386027336121 0.438885390758514
-2.17423987388611 1.56491637229919
7.28044462203979 2.56947994232178
-3.42478585243225 0.48586031794548
-4.28590869903564 0.152946025133133
-2.34947776794434 0.416360795497894
-3.454922914505 1.0617870092392
-2.19929218292236 -0.849985003471375
-2.61060357093811 1.88342046737671
-3.75635457038879 2.40278792381287
-2.76398420333862 0.376413732767105
-3.35935997962952 2.42954039573669
-1.52925980091095 2.00327062606812
-1.62111341953278 1.26104068756104
-1.80874145030975 0.571117639541626
-3.06874108314514 1.55899965763092
-2.88214063644409 1.48527455329895
-3.04472947120667 -0.438308566808701
-4.0900821685791 1.17146277427673
-1.34028220176697 1.26284468173981
-2.22576856613159 -0.667559862136841
-2.21807909011841 2.32045555114746
-3.39352583885193 0.936087012290955
-1.9746675491333 1.19063758850098
-3.38118577003479 1.86108601093292
-3.47509670257568 0.612271964550018
-1.48215091228485 0.291402131319046
-4.13144636154175 1.0381041765213
-1.78286743164062 0.510813653469086
-1.97377717494965 -0.233169674873352
-3.8966224193573 2.86892914772034
-2.5156409740448 -0.742035448551178
-2.79993486404419 1.05356645584106
-1.39146995544434 1.44524991512299
-2.89239931106567 -0.320042073726654
-1.76179277896881 1.95376992225647
-2.06691336631775 2.76560759544373
-2.35342121124268 2.17107748985291
-2.39227724075317 1.0115282535553
-3.42200493812561 1.2847695350647
-3.84704732894897 0.828550517559052
-3.82822155952454 0.48262757062912
-1.77760303020477 1.53597617149353
-2.34749126434326 1.82714331150055
-3.20481014251709 0.524060428142548
-1.92836272716522 3.629075050354
-2.06111097335815 2.01667809486389
-3.07051539421082 0.0178514793515205
-3.85585260391235 0.209012910723686
-2.18338227272034 1.45850467681885
-1.63977813720703 2.31392097473145
-1.58696937561035 0.704985618591309
-3.3447597026825 1.21567022800446
-2.45670008659363 1.59255194664001
-4.00618839263916 1.85601663589478
-3.20385265350342 -0.0087221646681428
-4.79589557647705 1.50467646121979
-4.38137865066528 2.08676338195801
-3.67904210090637 0.7722128033638
-1.1639518737793 1.72957372665405
-3.04289531707764 0.315837144851685
-3.60101938247681 0.657778024673462
-3.02599716186523 0.281906306743622
-3.89775538444519 1.52333152294159
-1.94636702537537 1.55060362815857
-2.73062777519226 0.922018885612488
-2.87452816963196 2.438800573349
-3.65499472618103 -0.173970639705658
-2.09700345993042 1.00828647613525
-4.25123977661133 1.1837158203125
-3.70373177528381 3.41570949554443
-2.19368672370911 0.0694267973303795
-2.98200750350952 0.46983876824379
-2.92840766906738 2.07926368713379
-3.8649001121521 1.99429440498352
-1.98872339725494 1.36386585235596
-2.69012665748596 1.42328488826752
-1.63601839542389 -0.405051052570343
-3.90870690345764 -0.689943730831146
-1.61171138286591 -0.24571904540062
-1.96562480926514 1.63915681838989
-1.67536580562592 0.981217980384827
-3.94077634811401 -0.339639902114868
-0.840150952339172 2.17148399353027
5.77519512176514 3.79200959205627
-3.25548315048218 2.24712467193604
-1.78454434871674 1.28548669815063
-1.9680198431015 2.28936362266541
-1.64518344402313 1.99327993392944
-2.11563444137573 0.0659819394350052
-3.64011359214783 0.877220153808594
-0.584468305110931 0.989483892917633
-3.92078876495361 0.2623610496521
-4.0186595916748 2.59715485572815
-2.71955561637878 0.586328148841858
-2.50299096107483 0.726570129394531
-3.41286849975586 0.833327412605286
-3.11053514480591 -0.0754006281495094
-3.63701963424683 1.99264812469482
-2.96275520324707 1.03667962551117
-1.60106682777405 2.01531863212585
-2.16482996940613 0.931539595127106
-4.04894208908081 0.627436697483063
-1.71901094913483 1.65800142288208
-1.53152716159821 0.93169903755188
-3.48732662200928 0.990796804428101
-2.33124089241028 0.830117046833038
-2.54826974868774 1.71229684352875
-3.62601089477539 1.05842745304108
-1.89396214485168 0.403686106204987
-3.17177414894104 1.79676616191864
-1.84934341907501 0.48029899597168
-2.9945273399353 1.67107617855072
-3.19535875320435 1.55201780796051
-1.80534076690674 1.48515284061432
-2.6258270740509 1.06468820571899
-2.55265092849731 0.921403110027313
-3.48919224739075 2.600750207901
-3.31626534461975 2.20074582099915
-2.7720890045166 0.456053167581558
-1.64665770530701 3.83614110946655
-2.09232902526855 1.80648398399353
-2.62684178352356 0.144022539258003
-1.82785427570343 0.522357225418091
-1.05708682537079 3.0347888469696
-1.03019094467163 0.736619412899017
-3.74324679374695 0.0692643895745277
-2.68184113502502 1.81679606437683
-1.70013272762299 2.49642276763916
-2.76824593544006 1.84965300559998
-3.767409324646 -0.403575360774994
-1.82954287528992 1.43979823589325
-2.04197859764099 1.03333985805511
-3.16108751296997 1.02151298522949
-2.8707389831543 0.371658265590668
-2.13234877586365 2.14525747299194
-4.61763000488281 1.07791030406952
-2.04913282394409 1.04823851585388
-3.26931929588318 0.308270782232285
-4.64157009124756 1.07663893699646
-6.17486429214478 0.725484311580658
-4.23771381378174 0.68218857049942
-3.89512896537781 0.295083433389664
-3.48999524116516 1.59255433082581
-3.19561147689819 0.841004550457001
-2.75074410438538 1.58912527561188
-3.51726746559143 0.691177248954773
-2.40183019638062 1.29937422275543
-1.61667358875275 -0.661966145038605
-2.88346934318542 0.0564443506300449
-2.37834239006042 0.826940059661865
-0.704846560955048 1.58096396923065
-2.95934963226318 0.355913877487183
-2.2414984703064 -0.495200395584106
-2.48971462249756 0.909578621387482
-2.47973608970642 2.92156839370728
-3.84755396842957 2.03508806228638
-2.70437932014465 1.35344636440277
-3.65828943252563 -0.850356101989746
-2.25508093833923 2.03695821762085
-1.14995789527893 1.84494817256927
-2.34341764450073 2.37009000778198
-2.38801217079163 0.146477118134499
-2.0285427570343 1.53525149822235
-2.12531590461731 0.445958346128464
-5.02766990661621 1.42074191570282
-2.72632884979248 1.67082166671753
-3.66615033149719 1.69839358329773
-4.26025247573853 -0.753433704376221
-2.21854734420776 -0.30527999997139
-1.97073137760162 1.33745646476746
-3.5198757648468 2.51185917854309
-2.5063111782074 0.571630537509918
-2.99178981781006 1.18943583965302
-2.96464610099792 0.269198775291443
-3.55762910842896 0.305582463741302
-2.06690549850464 0.31028887629509
-1.23363614082336 2.41072368621826
-2.64626121520996 0.787632405757904
-2.52481889724731 2.31324076652527
-3.67289066314697 1.37568628787994
-4.31754684448242 1.95396780967712
-3.77553296089172 -0.111080504953861
-3.7314715385437 0.265834957361221
-1.77341270446777 0.1087297052145
-2.59387230873108 -1.20089447498322
-1.40350353717804 -0.657536387443542
-3.48095059394836 1.14827275276184
-2.67775106430054 0.52611917257309
-2.34331798553467 0.515384495258331
-4.37100410461426 0.796756029129028
-0.287699341773987 0.963760793209076
-1.85913193225861 2.39792370796204
-3.13090372085571 1.40811419487
-4.6155424118042 0.724718987941742
-3.88695549964905 -0.555320203304291
-2.5671603679657 0.613021373748779
-2.47281336784363 1.25859928131104
-2.69790363311768 0.176115319132805
-1.11870288848877 0.173422917723656
-2.48398566246033 1.77022325992584
-1.92767679691315 2.48393821716309
-1.82485091686249 0.570990741252899
-2.6301486492157 -0.153325766324997
-3.42682266235352 2.49621224403381
-3.2537522315979 0.164898306131363
-2.9844605922699 0.755780577659607
-1.16399013996124 0.341980993747711
-2.76310300827026 0.398301601409912
-0.357347220182419 0.292330980300903
-3.5090708732605 0.780891060829163
-1.79680502414703 1.38459086418152
-1.79988849163055 0.301300078630447
-0.680683016777039 1.40083968639374
-4.10475778579712 0.909754514694214
-2.09298324584961 0.500157952308655
-1.71641027927399 0.935353457927704
-4.04891490936279 0.826938092708588
-1.98269104957581 1.95902001857758
-2.11952948570251 3.72910165786743
-4.58355093002319 1.98802161216736
-1.88208532333374 2.72115540504456
-3.10963487625122 -0.929750442504883
-3.25167679786682 -0.0117375114932656
-1.92238509654999 1.39135527610779
-2.11608386039734 0.50845330953598
-3.75819730758667 1.29248642921448
-1.73675775527954 0.362679988145828
-1.69616842269897 2.04067850112915
-3.16098999977112 2.22378206253052
0.863075256347656 2.20989012718201
-3.34396028518677 1.27919149398804
-2.04392147064209 1.33793473243713
-1.29610443115234 0.506762564182281
-3.40088415145874 2.03562140464783
-2.55984449386597 1.56841254234314
-2.20268130302429 0.20820751786232
-1.16984283924103 1.45334529876709
-1.17097342014313 1.72603940963745
-2.82445621490479 1.9888277053833
-3.81678915023804 3.14698672294617
-0.615290284156799 0.427834808826447
-2.74995136260986 1.0314234495163
-1.86220991611481 2.34915161132812
-4.59443378448486 1.67666566371918
-3.93080687522888 0.661796391010284
7.90697336196899 3.44850921630859
-2.82522797584534 1.73545503616333
-3.39382314682007 -0.738923907279968
-0.0947448238730431 0.797820568084717
-1.88260471820831 1.93023383617401
-1.86585450172424 1.50481772422791
-3.66421604156494 -0.0696074143052101
-3.49764847755432 1.87122762203217
-3.47505283355713 1.29235279560089
-1.80241763591766 -1.02322459220886
-2.06630611419678 0.512154817581177
-2.5532808303833 -0.317552268505096
-1.09144151210785 1.7534419298172
-4.23463487625122 0.88065493106842
-1.83522510528564 1.58781123161316
-1.59366154670715 3.52537965774536
-2.72950792312622 2.15872192382812
-3.56531929969788 1.51716315746307
-4.64375734329224 2.36681008338928
-1.99438118934631 1.25965106487274
-2.62634372711182 2.07641196250916
-3.01733827590942 0.0894166603684425
-3.539626121521 0.651989579200745
-2.494544506073 2.08186197280884
-3.21410298347473 1.03663992881775
-2.47566556930542 1.3006603717804
-3.50844836235046 0.6888747215271
-2.40166878700256 0.285911440849304
-3.35529708862305 0.520148634910583
-3.62737584114075 1.94365441799164
-2.08824920654297 2.22187638282776
-4.6111888885498 2.69005990028381
-1.90060317516327 2.53204584121704
-2.58191132545471 1.62606048583984
-2.18409609794617 0.601292610168457
-3.64110112190247 0.229121267795563
-2.49055814743042 2.04056882858276
-2.8081521987915 1.1328067779541
-3.12071657180786 2.2816014289856
-1.15981066226959 3.17258334159851
8.27747631072998 5.29047298431396
-2.86503624916077 0.8400838971138
-3.42646837234497 3.28825235366821
5.80407619476318 3.90601277351379
-0.996340990066528 0.986511290073395
-3.50226044654846 1.73440039157867
-2.61351442337036 0.922734439373016
-0.938341975212097 -1.13275861740112
-4.97146797180176 1.48900032043457
-3.52606987953186 0.221445947885513
-3.43077611923218 0.711254000663757
-2.11803770065308 1.08560645580292
-1.00701594352722 -0.172624483704567
-2.77523398399353 -0.396396368741989
-2.54238057136536 0.213683724403381
-3.95575881004333 2.01780772209167
-3.25539469718933 0.405079305171967
-2.53426098823547 2.12093091011047
-3.05471444129944 2.50009489059448
};


==> figures/visualizations/gmm40/smc_samples.tex <==
\addplot [semithick, smc, opacity=0.7, mark=*, mark size=3, mark options={solid}, only marks]
table {%
-4.95809173583984 30.9081935882568
34.5495643615723 33.6470756530762
-1.0714704990387 -27.7382755279541
5.89994239807129 -15.8454999923706
3.17859697341919 -12.0481834411621
35.6553688049316 5.62990808486938
-37.4864768981934 19.0332717895508
24.7519378662109 -12.6968584060669
-22.7191982269287 18.6034832000732
0.693470418453217 -29.0639457702637
-22.7841033935547 22.1544303894043
-36.0292015075684 -29.5557708740234
-34.3483924865723 37.4191474914551
15.6571311950684 -12.0103340148926
16.8686046600342 -5.14137077331543
-6.82231140136719 19.1783485412598
-15.4982233047485 35.7237510681152
-16.1959037780762 37.1520462036133
-36.1613273620605 -31.0927677154541
2.69781231880188 -20.6849403381348
-22.4331951141357 20.7969646453857
-17.8129177093506 16.0538463592529
33.8438262939453 5.19662237167358
28.1051006317139 34.619987487793
-0.609399318695068 -22.5144672393799
-15.3534774780273 35.7924118041992
6.01892471313477 37.5664138793945
16.0650901794434 -23.1974239349365
24.8578414916992 16.5647964477539
-0.546662509441376 -11.1188888549805
36.0662727355957 6.04157400131226
-18.8230648040771 20.2536697387695
35.6141357421875 7.29275512695312
-34.6779403686523 -32.6598930358887
-32.6452980041504 35.8618316650391
19.727180480957 -12.6765556335449
10.2041673660278 27.7455253601074
-9.77865886688232 25.5130844116211
8.43597412109375 30.6740646362305
-38.2106590270996 -30.7943286895752
12.353196144104 27.1644840240479
17.1154022216797 21.5435256958008
20.6669101715088 23.0764865875244
-40.1566963195801 18.7412719726562
-15.578085899353 36.1828498840332
-35.6273002624512 -24.5276222229004
-41.8494186401367 -31.3762722015381
-33.8719635009766 38.638973236084
-20.6671524047852 20.2407188415527
14.6602754592896 -11.1410665512085
-0.319931268692017 -22.9721813201904
7.28345489501953 4.00565385818481
0.375816881656647 -21.2524833679199
33.6318778991699 36.237865447998
-37.933666229248 -21.7533168792725
14.5738010406494 -14.2897367477417
-16.8704032897949 25.445219039917
3.56881356239319 -21.9008255004883
-5.23774385452271 18.2315731048584
-22.3636856079102 19.2823543548584
-30.3141002655029 39.9038047790527
24.9495906829834 -15.4963293075562
-2.76983785629272 1.60705924034119
-2.36397194862366 2.51146030426025
22.6814136505127 0.0190400257706642
-23.4661388397217 18.364501953125
0.123301096260548 -11.7987766265869
-33.8385963439941 37.7788314819336
19.6689643859863 -8.37254905700684
-15.5737152099609 36.9878196716309
37.2627143859863 6.05249643325806
11.2857818603516 26.0886859893799
-10.2849340438843 27.8257789611816
24.7908630371094 -15.3609533309937
37.7567520141602 -12.5192127227783
0.357919812202454 -30.9948272705078
0.497469335794449 -29.7096977233887
24.0103549957275 -13.3211536407471
26.3207244873047 -39.2009162902832
-7.67375373840332 24.489595413208
-39.7778129577637 -20.3388977050781
-38.3820343017578 -34.106876373291
38.4764671325684 3.14504981040955
-33.7046699523926 19.848352432251
27.4973583221436 -26.39333152771
36.5847702026367 4.79759979248047
25.0847148895264 19.0530166625977
6.21822834014893 -12.6429862976074
-38.9051361083984 -19.6758728027344
-2.84343814849854 0.0359865725040436
21.9059143066406 24.9482936859131
19.9605464935303 -11.640115737915
-35.005989074707 37.6784515380859
19.424503326416 21.970796585083
20.9259815216064 -26.0850429534912
26.0549831390381 -37.209056854248
-2.32199859619141 0.873575806617737
-37.590404510498 35.8185997009277
-36.4809188842773 37.4446449279785
35.955883026123 5.87667512893677
10.618706703186 -11.5315160751343
-16.112377166748 35.0879936218262
-32.285099029541 40.5171089172363
20.4496784210205 -28.6763610839844
10.4123344421387 36.1469078063965
10.5727529525757 4.7578558921814
-17.5447673797607 18.4942264556885
-0.428639948368073 -22.5288925170898
-41.2217254638672 -20.5627498626709
8.52873516082764 4.08769655227661
-0.429632812738419 -26.4592609405518
-36.8078804016113 -21.5024795532227
10.3274221420288 2.34401488304138
7.8547248840332 2.22157979011536
14.1641960144043 39.1058464050293
-39.4495277404785 -21.6676769256592
37.1662216186523 -13.9665746688843
0.676356494426727 -24.6862754821777
14.0410184860229 -30.55592918396
-31.7336750030518 38.6649627685547
6.25088691711426 1.84009802341461
35.253662109375 36.5741729736328
33.4848251342773 35.293586730957
22.141975402832 -21.8968734741211
-0.699417531490326 -0.363596260547638
-39.4350242614746 -30.2084808349609
-3.74570059776306 38.920597076416
-36.4259643554688 -31.4396991729736
3.36049795150757 2.96895408630371
-0.94830846786499 -30.12575340271
20.9363212585449 -9.72661113739014
2.52823710441589 2.77420973777771
-3.14359188079834 29.351001739502
21.5426788330078 0.258681833744049
28.0178279876709 -26.5553321838379
-19.7401866912842 20.0244026184082
20.6994438171387 -13.4147481918335
-37.750431060791 -25.1476192474365
-7.28938674926758 19.580924987793
20.138111114502 -8.86440086364746
32.1414947509766 37.135929107666
27.2615051269531 -28.5842990875244
-37.7873382568359 -20.9795932769775
-18.096586227417 34.8470611572266
5.693274974823 -22.8268718719482
20.8236675262451 -13.2737464904785
37.114013671875 6.33136558532715
31.0685195922852 36.4303970336914
25.9129295349121 -26.4668579101562
32.9169616699219 -13.8129062652588
5.89719581604004 2.60219550132751
14.4334735870361 -12.155234336853
33.8988265991211 37.367561340332
-8.50814723968506 15.1055841445923
6.95564031600952 5.66250848770142
-22.96044921875 20.3433513641357
8.58357620239258 -26.2732353210449
33.2403526306152 33.5970420837402
-10.9051265716553 28.8765678405762
-21.287389755249 22.1720237731934
18.655797958374 25.076566696167
-1.37419939041138 3.32769393920898
-2.41624426841736 -2.82609677314758
-38.1001853942871 -29.4945220947266
9.71070289611816 2.51142835617065
29.3679103851318 -28.9590606689453
19.7662353515625 19.8299942016602
-31.4693279266357 38.4697723388672
13.5024223327637 -24.5419960021973
-0.363825559616089 -29.9128513336182
34.4602355957031 -9.88007831573486
27.3401908874512 16.6747131347656
34.4195747375488 -12.836745262146
2.54895496368408 -10.8859367370605
18.8991527557373 23.9274463653564
-0.351848959922791 -13.1589279174805
0.815249443054199 -19.6624031066895
-1.14274072647095 -22.0245246887207
-20.9302082061768 18.8500595092773
25.0387840270996 -21.5501918792725
1.45988309383392 -20.6637840270996
35.8563575744629 5.84569931030273
21.3687171936035 -18.9263286590576
-3.42637705802917 5.37700653076172
24.4329128265381 -37.0013236999512
20.2291145324707 21.5622005462646
-38.2363777160645 -23.4645023345947
-35.413158416748 -33.3688697814941
9.04523468017578 5.10028028488159
0.310260474681854 -20.654317855835
-37.8510475158691 -22.3148345947266
-4.51692533493042 2.74016547203064
12.8901586532593 -12.6953754425049
-39.6844635009766 17.4859924316406
-37.929386138916 -31.6434001922607
-2.07438683509827 -1.72722625732422
34.383903503418 33.6422653198242
-32.3978614807129 37.4042930603027
-40.4724197387695 -22.1528987884521
-38.0784530639648 -32.7372665405273
-33.0983352661133 37.0443534851074
-37.2324829101562 20.8241863250732
-14.6686506271362 18.5194702148438
23.2132701873779 -1.06344366073608
-36.9425811767578 19.7877140045166
32.9747695922852 6.44902563095093
-19.1692886352539 22.3985366821289
-33.3117599487305 37.5816459655762
-0.40982574224472 -22.1304950714111
-33.9078140258789 39.3828659057617
19.9973659515381 -16.0284309387207
36.449089050293 5.79404306411743
-2.19229364395142 37.6609878540039
-33.0393447875977 38.028995513916
24.9892311096191 17.1871242523193
25.3333511352539 16.8519401550293
-0.327717542648315 -29.8424835205078
19.6629257202148 -25.3324661254883
-36.2985572814941 -33.2534599304199
-39.3198013305664 -28.6811790466309
32.8182334899902 6.24499130249023
33.1615753173828 35.972354888916
-36.5473899841309 -31.8705081939697
0.581502795219421 -29.9526119232178
13.6460990905762 -30.4425315856934
17.9882831573486 21.1123886108398
-0.403215408325195 -22.4640769958496
13.6086711883545 -12.1154336929321
-3.78747701644897 12.448073387146
11.7365379333496 27.7867794036865
-15.2070646286011 17.9950389862061
-35.9840049743652 37.4122123718262
-38.3347969055176 -23.0865612030029
32.8538513183594 33.3044242858887
23.7594432830811 -25.1587944030762
27.9416198730469 -12.5743265151978
18.3978385925293 26.3176956176758
-7.2094783782959 20.4386386871338
-40.9394226074219 -23.5264091491699
18.3908443450928 -3.87533855438232
20.6003646850586 25.5894660949707
-1.46388053894043 3.41055178642273
23.4912128448486 19.5023937225342
-3.54445886611938 39.4391632080078
-21.4502296447754 20.4011764526367
-38.8637275695801 -21.3009071350098
-0.287130653858185 -13.8953485488892
-34.2476806640625 38.9762878417969
5.83414888381958 4.04084348678589
11.8299684524536 26.0098361968994
0.569294452667236 -34.1134986877441
21.9149551391602 -13.9718885421753
-33.5470504760742 39.5804443359375
-40.7323226928711 -19.9184551239014
-13.1678771972656 33.1400032043457
36.9792518615723 7.9639835357666
-38.159610748291 -31.4118194580078
31.5027103424072 -12.2828407287598
11.1987066268921 34.093204498291
14.1925897598267 -13.5732307434082
-17.7735214233398 22.3707065582275
-6.83120346069336 29.3197956085205
-0.37344890832901 -26.9356250762939
3.46679353713989 -13.3365840911865
21.5141334533691 1.79795658588409
-24.113597869873 18.1070919036865
-21.3887672424316 20.1556453704834
24.9216423034668 17.0266437530518
13.3647680282593 27.1853370666504
24.6009063720703 -1.81640863418579
23.7970657348633 18.129919052124
-6.17779159545898 38.865047454834
0.772373259067535 36.8164596557617
-38.1805572509766 24.1832084655762
10.3269901275635 -23.8944396972656
35.0399436950684 7.06489419937134
-32.5672073364258 39.0053253173828
-6.0258731842041 19.6863422393799
-20.725471496582 21.3334522247314
29.8654537200928 33.4395599365234
5.4806957244873 41.5781402587891
30.0778465270996 35.3141593933105
9.58754253387451 34.9884643554688
11.7551565170288 -25.3881168365479
-0.504493594169617 -2.38970589637756
1.94591403007507 -13.6422023773193
24.7999153137207 -9.03774929046631
-6.77044057846069 28.8178691864014
22.0930786132812 -26.6674251556396
5.85981369018555 39.9512138366699
-4.18941783905029 10.4325265884399
-6.10515308380127 28.4497737884521
-38.335277557373 -32.787353515625
10.3195476531982 27.7371234893799
22.1228542327881 1.82404518127441
-0.625339865684509 -11.226450920105
16.1469745635986 -10.7631807327271
-4.79803276062012 30.9313106536865
-15.0139865875244 33.4234733581543
-34.953426361084 20.5024719238281
21.2057876586914 0.317017942667007
-3.32329082489014 -0.317118763923645
-3.33471632003784 11.9723224639893
35.4607887268066 -13.976634979248
24.9201889038086 -24.1646919250488
3.44426703453064 4.29401016235352
2.82153058052063 -15.3894443511963
-18.5380458831787 19.544412612915
-35.9687881469727 -32.1010551452637
-5.14151287078857 27.9927616119385
-39.6403961181641 -25.0644149780273
-16.1281356811523 22.6642665863037
-12.6570882797241 34.5861053466797
32.989372253418 35.0521697998047
-0.911129713058472 -22.4103565216064
37.1964530944824 -10.1588945388794
11.8772859573364 37.1982307434082
33.4107933044434 33.6883926391602
19.1496429443359 21.6583919525146
21.5542774200439 -24.6071605682373
-6.27811527252197 21.0381565093994
24.3758430480957 -25.629222869873
-20.5924644470215 20.0843353271484
20.5747203826904 24.3321514129639
14.1947708129883 -25.5070056915283
-17.3420143127441 37.2013969421387
7.84767866134644 39.851676940918
-34.9219055175781 -30.6442165374756
-0.717226088047028 -29.729061126709
-0.920596361160278 -27.152458190918
-37.0317077636719 -33.5607414245605
-39.2097702026367 -31.1705360412598
-18.4672603607178 20.6336154937744
21.4056911468506 -24.6587677001953
28.8744144439697 -28.2144203186035
31.5682373046875 32.7588310241699
-21.4787483215332 20.1065692901611
25.6064586639404 17.07594871521
25.5430297851562 21.1272659301758
25.9726696014404 -26.2941093444824
-2.03413319587708 -14.3839445114136
26.8967151641846 17.9673194885254
-7.33832883834839 11.9995861053467
-0.566062271595001 -21.5196628570557
-15.1959495544434 36.2604331970215
25.4295482635498 -27.0824546813965
1.99631237983704 -11.2814884185791
8.78454494476318 38.9076538085938
24.687572479248 -39.7028884887695
-34.9953842163086 -22.9656848907471
-38.0062255859375 -22.3935680389404
-21.7434959411621 23.4050445556641
35.324535369873 3.63233518600464
15.9666929244995 -12.3817958831787
-30.7793960571289 40.0330848693848
-4.23145723342896 0.593103885650635
9.91362857818604 37.5037002563477
1.63140320777893 -23.7258033752441
-15.6710433959961 20.0076847076416
9.8147439956665 -26.0549850463867
32.4248237609863 35.7067375183105
34.4297180175781 -11.9030628204346
20.7880306243896 -24.4024505615234
-39.4629554748535 -25.5002346038818
-3.48877739906311 28.1920909881592
-39.1018562316895 -31.1889247894287
26.5001087188721 -9.22426605224609
-2.81417751312256 15.0910501480103
25.3875751495361 25.0351753234863
-36.5393447875977 -21.3204307556152
-14.4278392791748 34.1923789978027
37.1099433898926 7.29031276702881
21.9890365600586 -0.100344695150852
19.4865589141846 -0.688444137573242
7.34938335418701 2.55714321136475
-21.1876487731934 19.6029567718506
25.566780090332 16.0539684295654
11.3289527893066 -24.7669010162354
-14.8284730911255 35.2213287353516
32.0083961486816 34.8436889648438
-10.0852355957031 28.0880737304688
20.5646152496338 24.7019634246826
19.3724231719971 23.0666637420654
-0.719280600547791 -28.8703517913818
33.9079170227051 35.8539848327637
-5.49277305603027 30.3418827056885
1.35402834415436 -15.5775661468506
20.3280410766602 23.6929626464844
27.6818332672119 -14.7984418869019
9.58437919616699 4.99456787109375
-12.3075180053711 38.3064842224121
-35.5475692749023 21.3046989440918
-24.9346981048584 21.8636646270752
34.1851997375488 3.06168484687805
-1.58983755111694 -20.3140163421631
-42.2136726379395 -24.4469890594482
11.9683885574341 28.2535495758057
-1.73556709289551 13.1437854766846
7.85397529602051 4.05250120162964
-4.4011058807373 13.2565355300903
32.6884918212891 38.225944519043
-14.5409460067749 16.6149921417236
19.9925308227539 -8.90243816375732
20.9988441467285 -11.0299291610718
-7.06211090087891 10.1435375213623
-35.1957397460938 18.5031147003174
12.3023452758789 -27.5216102600098
26.4457225799561 -26.1114540100098
-38.9198188781738 -33.0951690673828
-7.31487989425659 20.5797805786133
20.9442157745361 22.9242134094238
36.8573951721191 -15.1407413482666
38.6727104187012 4.67111730575562
24.2110958099365 16.8735809326172
-5.56910848617554 19.8820285797119
9.06425189971924 -24.982572555542
36.6525039672852 37.4811782836914
14.4045753479004 -10.6826877593994
0.26006281375885 38.3339958190918
-36.1163864135742 -30.6027050018311
18.4535255432129 26.5008010864258
-0.550468146800995 -15.6261463165283
-0.447540730237961 -28.6112804412842
-16.6712379455566 34.6818695068359
13.2988986968994 -27.7142276763916
33.1066932678223 36.3535194396973
-23.7923908233643 19.5296630859375
-38.0134658813477 20.3429985046387
18.1754703521729 -15.5702886581421
-33.6344833374023 37.702564239502
13.3907833099365 -25.9110164642334
-2.83385705947876 -0.749497830867767
8.04671764373779 4.81701612472534
32.7984580993652 37.0940589904785
-36.2653007507324 21.2429714202881
-41.1185111999512 -25.0405464172363
29.19895362854 -11.2568817138672
19.435998916626 -6.89874172210693
15.5056476593018 -25.3719329833984
18.5504417419434 -8.57005882263184
13.1438817977905 26.7642879486084
29.9382915496826 -26.8171367645264
28.6860694885254 -33.6469230651855
6.63374423980713 4.91589212417603
-35.9975738525391 -32.4086380004883
14.0857362747192 37.9935073852539
-1.19036209583282 38.4343299865723
11.7496728897095 -26.7024040222168
-42.3712272644043 -18.6084289550781
-15.446325302124 21.8053550720215
-10.7084054946899 33.8129806518555
19.8790054321289 22.6121234893799
13.268611907959 26.7163639068604
24.882266998291 -24.7301387786865
-30.8856143951416 36.8728103637695
-1.78218472003937 -22.2366714477539
16.2756080627441 -4.46299457550049
-16.4203834533691 32.0108413696289
-36.7641983032227 26.1226577758789
2.07376265525818 -20.6644916534424
-40.6964416503906 -24.0046520233154
-6.22378921508789 26.6743087768555
-38.7544097900391 -22.691478729248
-1.54264008998871 -30.766996383667
25.1208267211914 20.2944221496582
-14.9976415634155 17.1993675231934
17.2282104492188 -12.7327489852905
30.416919708252 35.3787002563477
-2.39452481269836 1.045689702034
15.3380012512207 -10.3019905090332
25.2357769012451 -15.4835634231567
35.7597198486328 34.1212730407715
-0.342891156673431 -20.7744312286377
-1.32751381397247 1.86530113220215
-4.64906787872314 -14.8302030563354
-32.9084663391113 36.7673263549805
10.441427230835 37.0783157348633
-2.78739452362061 30.5222759246826
26.0525302886963 19.5251941680908
0.63370156288147 -10.3468036651611
13.5581226348877 -28.5944805145264
-39.9785118103027 -21.3068752288818
25.0574817657471 -36.3300552368164
35.8591690063477 37.4183349609375
20.3141479492188 0.606326818466187
24.1414546966553 17.3981380462646
17.8731517791748 -5.33814668655396
24.6202926635742 -38.202766418457
15.0146713256836 -12.4600381851196
24.3701667785645 14.8138380050659
-2.51173233985901 -0.190923720598221
25.1342258453369 -37.86083984375
-30.7061958312988 39.6114845275879
0.614845216274261 -29.5363540649414
12.3698854446411 36.9994812011719
23.303243637085 -25.4700946807861
19.4723720550537 -26.8798484802246
12.1883506774902 28.009090423584
1.32473981380463 -21.5664443969727
21.2132720947266 -1.63131523132324
-34.771427154541 39.8659324645996
0.864673376083374 -27.8839321136475
-40.1761779785156 18.807544708252
-2.10069417953491 -21.3549671173096
-9.49627113342285 19.6974506378174
0.629856824874878 -24.5193157196045
27.747220993042 -38.4587478637695
33.5263252258301 35.6982421875
6.20453691482544 6.23764657974243
32.2331390380859 35.9622840881348
17.3456764221191 -8.8875093460083
35.2430686950684 5.24021482467651
6.39682579040527 39.8187789916992
-32.050609588623 40.3979835510254
21.7836856842041 -0.757118582725525
-15.8194036483765 20.7903747558594
22.1595230102539 -24.3217506408691
-37.8512802124023 -33.1482315063477
-38.8456573486328 -22.527250289917
8.45193481445312 4.78368043899536
33.8149871826172 37.6077842712402
19.0518951416016 -4.58746719360352
-3.68077969551086 0.995910108089447
16.1071262359619 -14.7153444290161
-33.323600769043 37.8214073181152
18.6782093048096 25.0229663848877
-1.49700033664703 37.2591094970703
17.5829048156738 21.4236717224121
8.15388488769531 3.95822238922119
15.1281929016113 28.7547950744629
0.335215151309967 -21.4811916351318
-39.6488494873047 -22.2651252746582
9.90139675140381 -25.8425140380859
-10.1813220977783 27.5647964477539
1.2011958360672 -30.1916465759277
35.3185234069824 6.84833574295044
-1.17506146430969 -3.18236470222473
-18.2429504394531 38.7870941162109
5.63184261322021 38.5605163574219
-34.1948928833008 -29.1364994049072
37.2756271362305 9.03571224212646
-33.0747756958008 40.4447402954102
-1.10644888877869 37.6474876403809
-34.8265190124512 20.8276081085205
-22.3633651733398 21.3269176483154
-32.3534927368164 38.3596725463867
13.4344568252563 -25.0744361877441
19.4148635864258 -14.3932056427002
39.5029792785645 -11.2447891235352
-38.5305976867676 -22.5904064178467
-37.8765678405762 -30.7936573028564
25.0068492889404 -36.4781150817871
-15.4648199081421 21.5300807952881
36.3047828674316 5.77181434631348
-35.6501159667969 18.8263359069824
-2.37401604652405 -30.1002941131592
-30.4516105651855 38.7779312133789
-38.8925132751465 18.7196140289307
17.0550632476807 23.540584564209
20.6913471221924 -25.3298759460449
0.436613798141479 -21.6255931854248
3.23243856430054 -22.9415683746338
14.7863855361938 -14.614616394043
35.1919822692871 35.0415878295898
-17.0697326660156 35.016284942627
16.9601650238037 -7.84499931335449
-40.2689094543457 -32.940315246582
28.278450012207 -37.3881759643555
-38.6547889709473 -32.6102676391602
25.1999645233154 -36.6861686706543
15.119607925415 -24.9258918762207
21.1060466766357 -16.0380020141602
31.5624675750732 34.9191017150879
34.314868927002 7.33391189575195
1.47123110294342 -10.5633583068848
36.6976776123047 9.47411918640137
-37.5868606567383 -21.4951362609863
25.3384056091309 -35.3838996887207
-1.16007542610168 -12.6049346923828
30.6205348968506 -15.2683248519897
-31.3362140655518 38.075569152832
28.3468761444092 -36.658748626709
-38.4965171813965 -31.922534942627
-9.69415187835693 28.3518314361572
18.8624496459961 20.4748134613037
25.8891620635986 18.942195892334
-40.9138488769531 -21.0359935760498
2.14464592933655 -29.1804122924805
-1.88614189624786 -0.25743243098259
17.7168426513672 -10.1883554458618
-39.4683418273926 -34.8771324157715
-31.9594249725342 39.3874282836914
25.6307487487793 -25.274829864502
-0.11377365142107 -21.0285968780518
-5.05648994445801 31.8296871185303
22.6488361358643 -17.18701171875
-40.2483177185059 -31.6947345733643
17.9437160491943 22.1033878326416
35.0098495483398 38.1953315734863
-31.0375080108643 37.1828765869141
-39.0872840881348 -25.0564346313477
25.6427745819092 18.9158935546875
24.5910053253174 -13.968825340271
-3.87281823158264 12.438383102417
-39.4280624389648 -21.440559387207
-33.8162460327148 37.0810928344727
-38.7997131347656 -33.3780174255371
-9.74503707885742 17.6827869415283
1.57707595825195 -32.1848754882812
-2.33409643173218 -29.0691184997559
25.2727127075195 15.3154191970825
19.4835109710693 22.2945880889893
21.4374656677246 0.107378989458084
-14.8619070053101 18.6421451568604
7.87946081161499 3.91758584976196
-38.5402374267578 -31.2911853790283
-38.4070854187012 -30.3592662811279
33.6028823852539 35.2026481628418
11.631329536438 -24.7156314849854
37.6021194458008 4.60463809967041
7.18291902542114 5.12384939193726
32.3711700439453 35.7976722717285
-28.7561321258545 38.5062561035156
17.2388401031494 -6.52975511550903
-40.9878730773926 -23.5619964599609
16.4106845855713 24.6212215423584
23.9597797393799 -37.6841125488281
20.624662399292 23.6221485137939
-3.76613569259644 37.33056640625
22.6695861816406 -14.7371768951416
38.6731224060059 4.2423095703125
21.4215965270996 -24.4322853088379
-37.5393180847168 -33.1168441772461
21.9286670684814 -0.607268631458282
21.3835945129395 1.73934018611908
25.4836311340332 18.7319221496582
-0.375864088535309 -14.0237150192261
35.0427780151367 5.16428995132446
12.1508960723877 38.835865020752
-39.3631935119629 -20.5338973999023
-9.52461528778076 25.2372016906738
-16.9552173614502 34.16845703125
22.48655128479 -1.55357241630554
2.84135866165161 -22.8703994750977
17.0964641571045 21.9305038452148
25.429931640625 15.4777278900146
25.1770343780518 18.983959197998
-2.34949707984924 37.0581359863281
-5.0420937538147 14.7904977798462
1.61616230010986 -13.7658910751343
-37.1260185241699 -29.8020191192627
8.60950660705566 1.6087304353714
22.4448337554932 -28.1460285186768
-40.2545318603516 -23.1459903717041
24.795238494873 17.7099590301514
-5.23821067810059 12.9197902679443
9.42160987854004 26.9120922088623
1.12192416191101 -24.1961364746094
12.7153949737549 -24.7175922393799
31.7715072631836 38.0368156433105
-3.5412061214447 32.3645286560059
-5.61828279495239 16.80784034729
35.5045928955078 -14.2463006973267
-0.924631178379059 0.626498520374298
-39.4945259094238 -31.9673271179199
-2.40777492523193 38.1811752319336
0.0212831757962704 -13.1140260696411
-0.530594527721405 -13.839147567749
-2.67219734191895 -29.3619441986084
20.4603710174561 -15.6301174163818
34.0782470703125 -12.8703966140747
9.47084045410156 26.3690586090088
-41.0898513793945 -22.680643081665
-2.45507669448853 -28.1788864135742
-4.4018988609314 30.4037132263184
36.7702522277832 5.56544971466064
37.2253799438477 -12.7871017456055
-40.4931221008301 -32.5248680114746
17.2572917938232 -12.8034057617188
11.9973201751709 29.8318405151367
-19.5895156860352 21.9395713806152
0.698664784431458 37.8571014404297
-2.15007257461548 30.7938899993896
-39.6636238098145 -22.5777320861816
34.8102569580078 -12.1906728744507
18.9918899536133 23.5032253265381
-1.06353724002838 -13.8558502197266
35.9791030883789 37.1304244995117
-37.9432563781738 -25.3144779205322
-5.04462766647339 -0.447423934936523
0.81991320848465 -21.169506072998
35.9767646789551 35.2961959838867
12.5404214859009 -27.3703308105469
-5.70456314086914 9.13944435119629
24.2981052398682 20.2044258117676
-34.1017723083496 19.2250022888184
1.66977250576019 -27.6408271789551
-37.9658737182617 -30.712329864502
37.0040397644043 7.76823616027832
2.7241735458374 -21.4307861328125
-22.7346496582031 19.9472560882568
11.0327568054199 4.58210611343384
-33.6902008056641 38.5568008422852
-17.5746994018555 14.8432369232178
-16.4311199188232 33.0546035766602
9.56435871124268 28.0456085205078
21.4228706359863 22.3094615936279
28.7905235290527 -37.1206588745117
-0.110099792480469 -28.966947555542
21.1846370697021 -26.4616832733154
-29.5997924804688 37.0958518981934
-35.5291900634766 -34.7782287597656
9.85168266296387 26.8515243530273
26.7863159179688 -36.0796012878418
36.0841789245605 35.7939071655273
-39.9353179931641 -31.8502826690674
-34.3529777526855 38.2863883972168
32.2649383544922 36.1605453491211
-0.854612529277802 -30.6415424346924
1.06635677814484 30.6747932434082
9.60094165802002 26.0717487335205
-3.4584846496582 -0.219744712114334
0.795247077941895 -13.8128509521484
-12.564697265625 38.3189468383789
-5.38527059555054 31.0102443695068
-33.8933944702148 20.87721824646
22.3324680328369 -1.90159261226654
-38.2320899963379 -20.802677154541
20.8187484741211 19.769006729126
8.39072608947754 27.1325531005859
24.296817779541 13.5429906845093
11.5045385360718 40.1939735412598
-34.1697387695312 35.7438163757324
10.8217353820801 -26.0430183410645
-18.46462059021 23.1185111999512
-40.0686721801758 -24.0917453765869
13.8351898193359 -12.0944919586182
7.82199668884277 5.17013168334961
34.6208190917969 -13.0093088150024
-1.1931836605072 -32.4247550964355
11.2832117080688 -26.3252067565918
17.1123218536377 -8.57488441467285
-1.84231507778168 2.09617686271667
23.9703407287598 -26.1755924224854
23.312068939209 -13.955958366394
15.7685251235962 -9.66527271270752
1.53559160232544 -14.4596061706543
-38.9300804138184 -32.0342140197754
-15.155876159668 18.5960369110107
18.0250606536865 -0.224444672465324
2.29592299461365 -12.1870994567871
0.204743593931198 -22.942813873291
33.1812973022461 36.5956535339355
-6.49507427215576 9.28391551971436
-0.926625609397888 -22.4974498748779
-20.7681522369385 19.2886524200439
24.3540706634521 18.4041881561279
-37.6312713623047 -21.8241939544678
12.7900638580322 -25.1229724884033
-20.2649345397949 19.1711349487305
34.3995819091797 -16.0403213500977
34.7310829162598 4.9391713142395
37.3954162597656 6.99560737609863
32.2625312805176 37.3607788085938
-38.3051872253418 -23.7837467193604
-35.5317268371582 21.7329597473145
13.9323101043701 -13.5957899093628
31.5392646789551 34.3869323730469
-1.14641797542572 -22.6880893707275
-4.47318983078003 31.7093334197998
19.0586910247803 18.9339389801025
4.44328641891479 -11.0313129425049
-39.2404861450195 -20.5365695953369
-15.7622623443604 35.6967964172363
-39.5905303955078 -23.2606983184814
38.1929054260254 3.52749228477478
-0.916640102863312 -21.1655044555664
-0.18427711725235 37.9230918884277
-37.2142753601074 -32.0832672119141
13.8326120376587 -13.1132907867432
-39.3475303649902 -24.1966419219971
-6.26136445999146 12.5540599822998
-19.0956535339355 23.198766708374
25.2658519744873 -31.521312713623
14.0707569122314 -26.9939842224121
23.7546463012695 -25.4404449462891
33.4927024841309 35.1004066467285
16.212890625 -12.5046062469482
-37.6033020019531 -30.151554107666
-2.43306183815002 -20.0245590209961
31.239315032959 34.4735069274902
25.5498237609863 -36.618522644043
22.2374362945557 2.61485266685486
34.0127906799316 38.0344314575195
-20.7175598144531 19.9946308135986
-34.440845489502 36.392879486084
11.8134908676147 -27.3073749542236
18.384407043457 22.4909706115723
-19.0696544647217 22.4347763061523
-39.4116020202637 -23.3961009979248
20.7788200378418 -0.35069665312767
33.4871139526367 36.4156761169434
-32.0190887451172 37.8947830200195
6.02267742156982 40.0633125305176
25.4777202606201 15.9790115356445
-36.1660690307617 38.1053085327148
-38.9324798583984 -21.79319190979
-0.557605624198914 0.114191435277462
-40.5766296386719 -18.0591583251953
-6.42019319534302 16.6444683074951
-3.31525754928589 3.0546019077301
-36.8319816589355 -32.7013320922852
21.8255615234375 -1.85959029197693
-3.34734988212585 -0.431355386972427
0.60137403011322 -30.1803531646729
24.475866317749 -34.6470947265625
1.78639352321625 -15.1774120330811
26.1693897247314 -35.9199523925781
18.8043117523193 -3.67173194885254
24.2620067596436 -1.50819945335388
32.7527008056641 9.02397632598877
10.6935129165649 25.9048080444336
8.963210105896 35.9877395629883
28.607364654541 -38.8957328796387
25.1494598388672 18.3823833465576
34.8654632568359 8.90071773529053
28.0120811462402 -13.7849721908569
-4.78271007537842 10.8385066986084
20.7911891937256 22.6637363433838
-39.782829284668 -24.5893173217773
34.3582992553711 8.08061122894287
7.43294477462769 6.63952922821045
-39.5549240112305 20.758846282959
-6.26437616348267 30.4531478881836
16.0421657562256 -3.95822691917419
0.469360679388046 -10.373438835144
-1.33111751079559 -25.9366226196289
0.216501548886299 -31.05517578125
12.9530038833618 -9.13128566741943
24.6934051513672 -36.390453338623
34.0600814819336 36.3956336975098
15.0554332733154 -24.7147006988525
-39.5473480224609 -24.4579925537109
6.99322080612183 38.0214233398438
35.2256698608398 33.7119674682617
30.7025356292725 -38.277702331543
36.4514770507812 5.53654479980469
-39.6018104553223 21.0093078613281
14.6852645874023 -13.0448484420776
8.33600902557373 3.64636397361755
34.8380279541016 39.7095146179199
-1.54899024963379 -27.9090270996094
-0.145276382565498 -12.5609655380249
-2.8299126625061 -28.9636554718018
-21.58180809021 21.5142230987549
-1.11778485774994 -31.3193550109863
33.4141006469727 37.6433906555176
-20.9541625976562 21.9468231201172
2.70305895805359 -13.3891716003418
27.3202228546143 -32.0340003967285
21.5482959747314 -1.70371150970459
20.6808395385742 -17.4214401245117
21.9003086090088 1.17001509666443
-17.1002941131592 35.8021583557129
-3.12975454330444 4.91698360443115
-16.4451351165771 23.2494201660156
24.2876758575439 -16.6808090209961
37.6641387939453 -11.8331022262573
-15.4711027145386 18.2646102905273
-13.3150806427002 35.1300086975098
-12.6568565368652 29.7455463409424
10.5050792694092 29.8183307647705
-24.0778121948242 18.8748569488525
-9.13767719268799 28.7071361541748
20.639087677002 -7.79354000091553
33.6486129760742 37.7309074401855
25.189603805542 -40.6112098693848
2.45328092575073 -28.8183784484863
-3.20950245857239 31.4938793182373
0.721960544586182 -11.7901029586792
30.6768398284912 -12.8625383377075
-37.3465766906738 18.0083122253418
-2.2230486869812 -0.553400993347168
1.4015291929245 -14.6339998245239
7.89321088790894 5.83102607727051
13.0005254745483 41.2600402832031
-32.1909980773926 38.276725769043
-13.9145154953003 36.4048919677734
28.1285419464111 -39.2454071044922
3.72669649124146 -13.6850328445435
20.7673187255859 0.781393706798553
28.445592880249 -37.2427520751953
-22.7950115203857 20.1501083374023
-1.55320382118225 39.5778923034668
2.57330751419067 37.2858200073242
23.7133941650391 18.9190158843994
-13.7306842803955 33.1737251281738
10.8179664611816 27.9689121246338
27.951961517334 -13.4368696212769
-39.1971435546875 -30.741003036499
-33.9728088378906 21.0887794494629
4.00861120223999 -11.5032329559326
-35.4943695068359 22.1406955718994
-38.2332763671875 -21.098258972168
25.4629955291748 -38.2559127807617
32.5383186340332 31.4225692749023
-34.2802772521973 38.2514343261719
19.1824054718018 -0.00849665142595768
-4.04150295257568 28.8197479248047
37.0048599243164 -14.0361289978027
-15.3432884216309 35.8754653930664
21.7326545715332 -13.7080974578857
17.1746253967285 -4.09880065917969
15.4720582962036 -10.2246799468994
-1.24847805500031 -1.35103440284729
35.0280265808105 -14.2310419082642
35.3933296203613 37.1597328186035
-15.8466300964355 20.0025177001953
-19.8907012939453 22.9749851226807
33.0789947509766 36.01416015625
20.4384956359863 -8.19148254394531
36.9522399902344 7.29777145385742
-35.9122428894043 19.807107925415
21.5230770111084 1.50930309295654
0.595401585102081 -23.6656055450439
33.6635475158691 34.5144386291504
12.2908821105957 32.6531677246094
33.9999198913574 4.04632711410522
17.9533519744873 19.7057304382324
0.945940136909485 -20.7221584320068
32.0401763916016 37.0943565368652
-32.1638298034668 39.7303428649902
35.2280654907227 -9.35470581054688
31.3672904968262 39.4548034667969
-9.20948886871338 17.892333984375
36.7418060302734 38.137134552002
-36.1443939208984 -33.3549423217773
19.9350929260254 -8.32634544372559
-17.5892868041992 20.265193939209
-22.6551742553711 16.5856075286865
35.5567855834961 5.35547637939453
3.98347043991089 36.7961196899414
-9.49885654449463 20.2629489898682
4.079993724823 3.63824391365051
5.51237916946411 2.33855986595154
-2.19735884666443 3.05577373504639
2.12801027297974 -23.2549133300781
28.9795742034912 -10.5931329727173
34.0640182495117 35.1735610961914
-18.4889850616455 21.1719741821289
31.4460620880127 36.3522644042969
21.5601234436035 -24.8484210968018
6.96876525878906 37.8785820007324
1.06922936439514 -8.65236663818359
-31.0474414825439 40.7103233337402
19.325267791748 -1.64313149452209
1.68890118598938 -22.0921592712402
12.9635534286499 -28.1434707641602
-42.4270401000977 18.4325866699219
32.7305068969727 36.9344825744629
19.3744621276855 -14.6725034713745
-16.6141548156738 18.2087478637695
-39.1955070495605 -21.9235038757324
20.3758792877197 -4.24285364151001
21.0796928405762 -0.0533832348883152
20.3083209991455 0.227421179413795
-39.4539909362793 19.5276031494141
36.1505508422852 4.31561374664307
12.730770111084 -26.5627994537354
-23.7900505065918 20.2778606414795
-41.2826347351074 -30.5698585510254
-35.007266998291 36.7153968811035
-36.5121459960938 21.4286365509033
34.9748382568359 3.90698790550232
-37.6124229431152 -31.6597137451172
-5.08054876327515 30.5571212768555
1.87111711502075 -29.0849800109863
-1.26338744163513 -28.0472888946533
17.7729797363281 -1.23094475269318
-23.220516204834 19.5426063537598
-8.40427780151367 29.519624710083
1.52382671833038 -18.3659400939941
24.1149749755859 0.126780971884727
7.53577518463135 2.68846082687378
-32.0970268249512 37.3023338317871
17.6009712219238 -8.67412567138672
28.2556667327881 -16.2476634979248
-37.7711982727051 -18.1899642944336
19.1418304443359 -12.5985527038574
-24.4678897857666 24.7061729431152
-7.47996520996094 29.1833076477051
-4.63111066818237 0.135423541069031
35.9927215576172 5.11109113693237
0.410094916820526 -30.3575401306152
-15.341926574707 39.2896690368652
1.50325512886047 -11.2695064544678
-0.79167503118515 -8.18538093566895
-2.65097761154175 -24.2696437835693
-37.6257286071777 19.0760593414307
-27.9084453582764 37.8094024658203
};

==> results/tables/elbo_eubo_table.tex <==
\begin{table}
% \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
\label{table:vi_results}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cccccccc}
\begin{tabular}{l|cccccccccc}
\toprule
  \textbf{ELBO}   & IGMM ($D=2$) & IGMM ($D=50$)& IGMM ($D=200$)  & GMM ($D=2$) & GMM ($D=50$)& GMM ($D=200$)  & STMM ($D=2$) & STMM ($D=50$)& STMM ($D=200$) & NICE \\ 
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $-3.01 \scriptstyle \pm 0.004$ % IGMM 2
& $-3.699 \scriptstyle \pm 0.001$ % IGMM 50
& $-3.73 \scriptstyle \pm 0.003$ % IGMM 200
& $-0.694 \scriptstyle \pm 0.008$ % GMM 2
& $-48.454 \scriptstyle \pm 0.067$ % GMM 50
& $-279.006 \scriptstyle \pm 0.382$ % GMM 200
& $0.000 \scriptstyle{\pm 0.000}$ % STMM 2
& $-6.364 \scriptstyle \pm 0.006$ % STMM 50
& $-17.386 \scriptstyle \pm 0.016$ % STMM 200
& $-14.22 \scriptstyle \pm 0.009$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $-0.002 \scriptstyle \pm 0.002$ % IGMM 2
& $-3.602 \scriptstyle \pm 0.229$ % IGMM 50
& $-3.689 \scriptstyle \pm 0.0$ % IGMM 200
& $-0.002 \scriptstyle \pm 0.007$ % GMM 2
& $-0.052 \scriptstyle \pm 0.03$ % GMM 50
& $-2.708 \scriptstyle \pm 0.0$ % GMM 200
& $0.000 \scriptstyle{\pm 0.000}$ % STMM 2
& $-4.62 \scriptstyle \pm 0.163$ % STMM 50
& $0.000 \scriptstyle{\pm 0.000}$ % STMM 200
& N/A % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NFVI
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $-9.09 \scriptstyle \pm 0.033$ % IGMM 2
& $-2462.479 \scriptstyle \pm 10.506$ % IGMM 50
& $-15780.962 \scriptstyle \pm 42.909$ % IGMM 200
& $-0.117 \scriptstyle \pm 0.019$ % GMM 2
& $-7.899 \scriptstyle \pm 0.692$ % GMM 50
& $-40.409 \scriptstyle \pm 2.114$ % GMM 200
& $-0.022 \scriptstyle \pm 0.032$ % STMM 2
& $-4.799 \scriptstyle \pm 1.58$ % STMM 50
& $-52.85 \scriptstyle \pm 3.418$ % STMM 200
& $-163.719 \scriptstyle \pm 1.859$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $-3.046 \scriptstyle \pm 0.439$ % IGMM 2
& $-1241.237 \scriptstyle \pm 147.377$ % IGMM 50
& $-8690.66 \scriptstyle \pm 474.741$ % IGMM 200
& $-0.037 \scriptstyle \pm 0.046$ % GMM 2
& $-8.077 \scriptstyle \pm 1.081$ % GMM 50
& $-55.963 \scriptstyle \pm 5.771$ % GMM 200
& $-0.017 \scriptstyle \pm 0.072$ % STMM 2
& $-9.26 \scriptstyle \pm 3.687$ % STMM 50
& $-75.945 \scriptstyle \pm 6.189$ % STMM 200
& $-68.748 \scriptstyle \pm 8.73$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $-3.527 \scriptstyle \pm 0.063$ % IGMM 2
& $-777.939 \scriptstyle \pm 16.578$ % IGMM 50
& $-4614.218 \scriptstyle \pm 97.283$ % IGMM 200
& $-0.005 \scriptstyle \pm 0.003$ % GMM 2
& $-2.39 \scriptstyle \pm 0.518$ % GMM 50
& $-27.369 \scriptstyle \pm 1.16$ % GMM 200
& $0.012 \scriptstyle \pm 0.011$ % STMM 2
& $-0.388 \scriptstyle \pm 0.623$ % STMM 50
& $-21.877 \scriptstyle \pm 1.572$ % STMM 200
& $-9.21 \scriptstyle \pm 0.414$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SNF
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $-6.463 \scriptstyle \pm 1.113$ % IGMM 2
& $-1296.493 \scriptstyle \pm 621.829$ % IGMM 50
& $-724.248 \scriptstyle \pm 500.415$ % IGMM 200
& $-0.036 \scriptstyle \pm 0.025$ % GMM 2
& $-5.241 \scriptstyle \pm 2.033$ % GMM 50
& $-103.082 \scriptstyle \pm 26.15$ % GMM 200
& $-0.181 \scriptstyle \pm 0.1$ % STMM 2
& $-35.09 \scriptstyle \pm 3.522$ % STMM 50
& $-40.207 \scriptstyle \pm 3.347$ % STMM 200
& $-5.425 \scriptstyle \pm 0.158$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $-0.731 \scriptstyle \pm 0.021$ % IGMM 2
& $-16.1 \scriptstyle \pm 0.203$ % IGMM 50
& $-65.212 \scriptstyle \pm 0.324$ % IGMM 200
& $-0.097 \scriptstyle \pm 0.008$ % GMM 2
& $-44.219 \scriptstyle \pm 0.391$ % GMM 50
& $-227.681 \scriptstyle \pm 2.07$ % GMM 200
& $0.000 \scriptstyle{\pm 0.000}$ % STMM 2
& $-48.428 \scriptstyle \pm 0.408$ % STMM 50
& $-288.589 \scriptstyle \pm 0.684$ % STMM 200
& $-133.24 \scriptstyle \pm 0.874$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $-2.678 \scriptstyle \pm 0.166$ % IGMM 2
& $-888.236 \scriptstyle \pm 8.752$ % IGMM 50
& $-4250.623 \scriptstyle \pm 212.37$ % IGMM 200
& $-0.615 \scriptstyle \pm 0.017$ % GMM 2
& $-315.35 \scriptstyle \pm 13.627$ % GMM 50
& $-14009.77 \scriptstyle \pm 269.53$ % GMM 200
& $-1.538 \scriptstyle \pm 0.017$ % STMM 2
& $-91.37 \scriptstyle \pm 0.095$ % STMM 50
& $-407.958 \scriptstyle \pm 0.27$ % STMM 200
& $-1054.014 \scriptstyle \pm 24.39$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $-3.84 \scriptstyle \pm 0.236$ % IGMM 2
& $-43.818 \scriptstyle \pm 0.325$ % IGMM 50
& $-302.141 \scriptstyle \pm 3.012$ % IGMM 200
& $-0.065 \scriptstyle \pm 0.004$ % GMM 2
& $-23.77 \scriptstyle \pm 0.718$ % GMM 50
& $-231.006 \scriptstyle \pm 7.9$ % GMM 200
& $-1.228 \scriptstyle \pm 0.022$ % STMM 2
& $-75.584 \scriptstyle \pm 0.316$ % STMM 50
& $-341.382 \scriptstyle \pm 1.146$ % STMM 200
& $-255.933 \scriptstyle \pm 29.543$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $-3.821 \scriptstyle \pm 0.341$ % IGMM 2
& $-25.264 \scriptstyle \pm 0.252$ % IGMM 50
& $-108.881 \scriptstyle \pm 4.515$ % IGMM 200
& $-0.073 \scriptstyle \pm 0.005$ % GMM 2
& $-4.058 \scriptstyle \pm 0.028$ % GMM 50
& $-1565.573 \scriptstyle \pm 27.132$ % GMM 200
& $-0.105 \scriptstyle \pm 0.01$ % STMM 2
& $-7.745 \scriptstyle \pm 0.062$ % STMM 50
& $-26.751 \scriptstyle \pm 0.203$ % STMM 200
& $-30.6 \scriptstyle \pm 0.186$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%
%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
% \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
\label{table:vi_results}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cccccccc}
\begin{tabular}{l|cccccccccc}
\toprule
  \textbf{EUBO}   & IGMM ($D=2$) & IGMM ($D=50$)& IGMM ($D=200$)  & GMM ($D=2$) & GMM ($D=50$)& GMM ($D=200$)  & STMM ($D=2$) & STMM ($D=50$)& STMM ($D=200$) & NICE \\ 
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $168.026 \scriptstyle \pm 1.489$ % IGMM 2
& $23047.8 \scriptstyle \pm 60.134$ % IGMM 50
& $97607.177 \scriptstyle \pm 14.443$ % IGMM 200
& $0.68 \scriptstyle \pm 0.002$ % GMM 2
& $935.358 \scriptstyle \pm 16.032$ % GMM 50
& $4726.95 \scriptstyle \pm 8.408$ % GMM 200
& $0.000 \scriptstyle{\pm 0.000}$ % STMM 2
& $914.951 \scriptstyle \pm 0.465$ % STMM 50
& $3595.229 \scriptstyle \pm 0.736$ % STMM 200
& $543.178 \scriptstyle \pm 0.669$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $0.004 \scriptstyle \pm 0.003$ % IGMM 2
& $2515.443 \scriptstyle \pm 1123.587$ % IGMM 50
& $6324.869 \scriptstyle \pm 5971.896$ % IGMM 200
& $0.003 \scriptstyle \pm 0.007$ % GMM 2
& $8.569 \scriptstyle \pm 5.037$ % GMM 50
& $0.000 \scriptstyle{\pm 0.000}$ % GMM 200
& $0.002 \scriptstyle \pm 0.001$ % STMM 2
& $184.637 \scriptstyle \pm 55.118$ % STMM 50
& $0.000 \scriptstyle{\pm 0.000}$ % STMM 200
& N/A % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NFVI
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $1.663 \scriptstyle \pm 0.137$ % IGMM 2
& $109.287 \scriptstyle \pm 1.088$ % IGMM 50
& $468.091 \scriptstyle \pm 5.11$ % IGMM 200
& $0.249 \scriptstyle \pm 0.248$ % GMM 2
& $10.204 \scriptstyle \pm 0.763$ % GMM 50
& $27.392 \scriptstyle \pm 1.298$ % GMM 200
& $0.108 \scriptstyle \pm 0.072$ % STMM 2
& $7.907 \scriptstyle \pm 2.032$ % STMM 50
& $51.973 \scriptstyle \pm 3.038$ % STMM 200
& $133.069 \scriptstyle \pm 0.698$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $2.744 \scriptstyle \pm 1.373$ % IGMM 2
& $135.317 \scriptstyle \pm 27.147$ % IGMM 50
& $513.179 \scriptstyle \pm 17.674$ % IGMM 200
& $0.284 \scriptstyle \pm 0.05$ % GMM 2
& $29.834 \scriptstyle \pm 14.835$ % GMM 50
& $234.341 \scriptstyle \pm 103.942$ % GMM 200
& $83.865 \scriptstyle \pm 39.692$ % STMM 2
& $413.699 \scriptstyle \pm 63.8$ % STMM 50
& $1084.139 \scriptstyle \pm 84.99$ % STMM 200
& $199.117 \scriptstyle \pm 3.399$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $2.05 \scriptstyle \pm 0.029$ % IGMM 2
& $215.942 \scriptstyle \pm 1.484$ % IGMM 50
& $917.075 \scriptstyle \pm 9.723$ % IGMM 200
& $0.134 \scriptstyle \pm 0.007$ % GMM 2
& $22.199 \scriptstyle \pm 0.462$ % GMM 50
& $1369.65 \scriptstyle \pm 1230.756$ % GMM 200
& $170.812 \scriptstyle \pm 68.532$ % STMM 2
& $1051.354 \scriptstyle \pm 301.885$ % STMM 50
& $2565.726 \scriptstyle \pm 270.621$ % STMM 200
& $104.176 \scriptstyle \pm 9.294$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SNF
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $1.072 \scriptstyle \pm 0.071$ % IGMM 2
& $\infty$ % IGMM 50
& $\infty$ % IGMM 200
& $0.23 \scriptstyle \pm 0.415$ % GMM 2
& $302.636 \scriptstyle \pm 305.794$ % GMM 50
& $258.651 \scriptstyle \pm 45.895$ % GMM 200
& $0.114 \scriptstyle \pm 0.026$ % STMM 2
& $30.875 \scriptstyle \pm 1.719$ % STMM 50
& $\infty$ % STMM 200
& $\infty$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $9.714 \scriptstyle \pm 0.211$ % IGMM 2
& $419.838 \scriptstyle \pm 3.276$ % IGMM 50
& $1720.661 \scriptstyle \pm 12.254$ % IGMM 200
& $4.968 \scriptstyle \pm 0.046$ % GMM 2
& $408.45 \scriptstyle \pm 7.693$ % GMM 50
& $3162.189 \scriptstyle \pm 183.531$ % GMM 200
& $4.859 \scriptstyle \pm 0.029$ % STMM 2
& $177.535 \scriptstyle \pm 0.478$ % STMM 50
& $641.838 \scriptstyle \pm 0.55$ % STMM 200
& $1128.436 \scriptstyle \pm 13.726$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $2.136 \scriptstyle \pm 0.062$ % IGMM 2
& $108.822 \scriptstyle \pm 3.076$ % IGMM 50
& $973.636 \scriptstyle \pm 85.268$ % IGMM 200
& $0.531 \scriptstyle \pm 0.011$ % GMM 2
& $293.853 \scriptstyle \pm 6.102$ % GMM 50
& $\infty$ % GMM 200
& $0.894 \scriptstyle \pm 0.016$ % STMM 2
& $60.519 \scriptstyle \pm 0.17$ % STMM 50
& $254.58 \scriptstyle \pm 0.664$ % STMM 200
& $741.752 \scriptstyle \pm 20.284$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $26.539 \scriptstyle \pm 9.463$ % IGMM 2
& $2785.126 \scriptstyle \pm 88.016$ % IGMM 50
& $551.403 \scriptstyle \pm 18.087$ % IGMM 200
& $0.074 \scriptstyle \pm 0.005$ % GMM 2
& $36.438 \scriptstyle \pm 1.198$ % GMM 50
& $\infty$ % GMM 200
& $0.806 \scriptstyle \pm 0.01$ % STMM 2
& $51.955 \scriptstyle \pm 0.321$ % STMM 50
& $223.143 \scriptstyle \pm 1.069$ % STMM 200
& $0.000 \scriptstyle{\pm 0.000}$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $53.192 \scriptstyle \pm 14.543$ % IGMM 2
& $8252.215 \scriptstyle \pm 1024.625$ % IGMM 50
& $37456.045 \scriptstyle \pm 9975.166$ % IGMM 200
& $0.081 \scriptstyle \pm 0.007$ % GMM 2
& $296.747 \scriptstyle \pm 35.059$ % GMM 50
& $1071.204 \scriptstyle \pm 62.892$ % GMM 200
& $0.784 \scriptstyle \pm 0.097$ % STMM 2
& $450.376 \scriptstyle \pm 20.523$ % STMM 50
& $2127.893 \scriptstyle \pm 228.31$ % STMM 200
& $270.394 \scriptstyle \pm 14.047$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> results/tables/emc_table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{minipage}{\textwidth}
\begin{table*}[t!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\toprule
   & \multicolumn{6}{c}{\textbf{MoG}} & \multicolumn{6}{c}{\textbf{MoS}}   \\ 
   & \multicolumn{3}{c}{\textbf{ELBO} $\uparrow$} & \multicolumn{3}{c}{\textbf{EUBO} $\downarrow$}   
   & \multicolumn{3}{c}{\textbf{ELBO} $\uparrow$} & \multicolumn{3}{c}{\textbf{EUBO} $\downarrow$}
   \\ 
\textbf{Method}   
& $d=2$ & $d=50$  & $d=200$ & $d=2$ & $d=50$  & $d=200$
& $d=2$ & $d=50$  & $d=200$ & $d=2$ & $d=50$  & $d=200$
\\ 
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
 % & \multicolumn{6}{c}{\textbf{MoG}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $-3.010 \scriptstyle \pm 0.004$ % ELBO d=2
& $-3.699 \scriptstyle \pm 0.001$ % ELBO d=50
& $-3.730 \scriptstyle \pm 0.003$ % ELBO d=200
& $168.0 \scriptstyle \pm 1.489$ % EUBO d=2
& $23047.8 \scriptstyle \pm 60.13$ % EUBO d=50
& $97607.177 \scriptstyle \pm 14.44$ % EUBO d=200
& $-0.689 \scriptstyle \pm 0.007$ % ELBO d=2
& $-6.364 \scriptstyle \pm 0.006$ % ELBO d=50
& $-17.38 \scriptstyle \pm 0.016$ % ELBO d=200
& $0.949 \scriptstyle \pm 0.005$ % EUBO d=2
& $914.9 \scriptstyle \pm 0.465$ % EUBO d=50
& $3595. \scriptstyle \pm 0.736$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $\mathbf{-0.002 \scriptstyle \pm 0.002}$ % ELBO d=2
& $\mathbf{-0.425 \scriptstyle \pm 0.092}$ % ELBO d=50
& $\mathbf{-0.698 \scriptstyle \pm 0.089}$ % ELBO d=200
& $\mathbf{0.004 \scriptstyle \pm 0.003}$ % EUBO d=2
& $698.2 \scriptstyle \pm 571.8$ % EUBO d=50
& $1734 \scriptstyle \pm 1220$ % EUBO d=200
& $\mathbf{-0.001 \scriptstyle \pm 0.000}$ % ELBO d=2
& $-4.200 \scriptstyle \pm 0.197$ % ELBO d=50
& $\mathbf{-17.12 \scriptstyle \pm 0.449}$ % ELBO d=200
& $\mathbf{0.001 \scriptstyle \pm 0.000}$ % EUBO d=2
& $119.9 \scriptstyle \pm 37.83$ % EUBO d=50
& $771.6 \scriptstyle \pm 340.5$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NFVI
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=200
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=200
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $-9.090 \scriptstyle \pm 0.033$ % ELBO d=2
& $-2462 \scriptstyle \pm 10.50$ % ELBO d=50
& $-15780.962 \scriptstyle \pm 42.90$ % ELBO d=200
& $1.663 \scriptstyle \pm 0.137$ % EUBO d=2
& $109.2 \scriptstyle \pm 1.088$ % EUBO d=50
& $\mathbf{468.0 \scriptstyle \pm 5.110}$ % EUBO d=200
& $-0.022 \scriptstyle \pm 0.032$ % ELBO d=2
& $-4.799 \scriptstyle \pm 1.580$ % ELBO d=50
& $-52.85 \scriptstyle \pm 3.418$ % ELBO d=200
& $0.108 \scriptstyle \pm 0.072$ % EUBO d=2
& $\mathbf{7.907 \scriptstyle \pm 2.032}$ % EUBO d=50
& $\mathbf{51.97 \scriptstyle \pm 3.038}$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $-3.046 \scriptstyle \pm 0.439$ % ELBO d=2
& $-1241 \scriptstyle \pm 147.3$ % ELBO d=50
& $-8690 \scriptstyle \pm 474.7$ % ELBO d=200
& $2.744 \scriptstyle \pm 1.373$ % EUBO d=2
& $135.3 \scriptstyle \pm 27.14$ % EUBO d=50
& $513.1 \scriptstyle \pm 17.67$ % EUBO d=200
& $-0.017 \scriptstyle \pm 0.072$ % ELBO d=2
& $-9.260 \scriptstyle \pm 3.687$ % ELBO d=50
& $-75.94 \scriptstyle \pm 6.189$ % ELBO d=200
& $83.86 \scriptstyle \pm 39.69$ % EUBO d=2
& $413.6 \scriptstyle \pm 63.80$ % EUBO d=50
& $1084. \scriptstyle \pm 84.99$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $-3.527 \scriptstyle \pm 0.063$ % ELBO d=2
& $-777.9 \scriptstyle \pm 16.57$ % ELBO d=50
& $-4614 \scriptstyle \pm 97.28$ % ELBO d=200
& $2.050 \scriptstyle \pm 0.029$ % EUBO d=2
& $215.9 \scriptstyle \pm 1.484$ % EUBO d=50
& $917.0 \scriptstyle \pm 9.723$ % EUBO d=200
& $-0.012 \scriptstyle \pm 0.011$ % ELBO d=2
& $\mathbf{-0.388 \scriptstyle \pm 0.623}$ % ELBO d=50
& $-21.87 \scriptstyle \pm 1.572$ % ELBO d=200
& $170.8 \scriptstyle \pm 68.53$ % EUBO d=2
& $1051. \scriptstyle \pm 301.8$ % EUBO d=50
& $2565. \scriptstyle \pm 270.6$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SNF
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $-6.463 \scriptstyle \pm 1.113$ % ELBO d=2
& $-1296. \scriptstyle \pm 621.8$ % ELBO d=50
& $-724.2 \scriptstyle \pm 500.4$ % ELBO d=200
& $1.072 \scriptstyle \pm 0.071$ % EUBO d=2
& N/A % EUBO d=50
& N/A % EUBO d=200
& $-0.181 \scriptstyle \pm 0.100$ % ELBO d=2
& $-35.09 \scriptstyle \pm 3.522$ % ELBO d=50
& $-40.20 \scriptstyle \pm 3.347$ % ELBO d=200
& $0.114 \scriptstyle \pm 0.026$ % EUBO d=2
& $30.87 \scriptstyle \pm 1.719$ % EUBO d=50
& N/A % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $9.714 \scriptstyle \pm 0.211$ % ELBO d=2
& $419.8 \scriptstyle \pm 3.276$ % ELBO d=50
& $1720 \scriptstyle \pm 12.25$ % ELBO d=200
& $9.714 \scriptstyle \pm 0.211$ % EUBO d=2
& $419.8 \scriptstyle \pm 3.276$ % EUBO d=50
& $1720 \scriptstyle \pm 12.25$ % EUBO d=200
& $-0.245 \scriptstyle \pm 0.012$ % ELBO d=2
& $-48.42 \scriptstyle \pm 0.408$ % ELBO d=50
& $-288.5 \scriptstyle \pm 0.684$ % ELBO d=200
& $4.859 \scriptstyle \pm 0.029$ % EUBO d=2
& $177.5 \scriptstyle \pm 0.478$ % EUBO d=50
& $641.8 \scriptstyle \pm 0.550$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $-2.678 \scriptstyle \pm 0.166$ % ELBO d=2
& $-888.2 \scriptstyle \pm 8.752$ % ELBO d=50
& $-4250. \scriptstyle \pm 212.3$ % ELBO d=200
& $2.136 \scriptstyle \pm 0.062$ % EUBO d=2
& $\mathbf{108.8 \scriptstyle \pm 3.076}$ % EUBO d=50
& $973.6 \scriptstyle \pm 85.26$ % EUBO d=200
& $-1.538 \scriptstyle \pm 0.017$ % ELBO d=2
& $-91.37 \scriptstyle \pm 0.095$ % ELBO d=50
& $-407.9 \scriptstyle \pm 0.270$ % ELBO d=200
& $0.894 \scriptstyle \pm 0.016$ % EUBO d=2
& $60.51 \scriptstyle \pm 0.170$ % EUBO d=50
& $254.5 \scriptstyle \pm 0.664$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $-3.840 \scriptstyle \pm 0.236$ % ELBO d=2
& $-43.81 \scriptstyle \pm 0.325$ % ELBO d=50
& $-302.1 \scriptstyle \pm 3.012$ % ELBO d=200
& $26.53 \scriptstyle \pm 9.463$ % EUBO d=2
& $2785. \scriptstyle \pm 88.01$ % EUBO d=50
& $551.4 \scriptstyle \pm 18.08$ % EUBO d=200
& $-1.228 \scriptstyle \pm 0.022$ % ELBO d=2
& $-75.584 \scriptstyle \pm 0.316$ % ELBO d=50
& $-341.382 \scriptstyle \pm 1.146$ % ELBO d=200
& $0.806 \scriptstyle \pm 0.01$ % EUBO d=2
& $51.955 \scriptstyle \pm 0.321$ % EUBO d=50
& $223.143 \scriptstyle \pm 1.069$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $-3.821 \scriptstyle \pm 0.341$ % ELBO d=2
& $-25.26 \scriptstyle \pm 0.252$ % ELBO d=50
& $-108.8 \scriptstyle \pm 4.515$ % ELBO d=200
& $53.19 \scriptstyle \pm 14.54$ % EUBO d=2
& $8252. \scriptstyle \pm 1024.$ % EUBO d=50
& $37456.045 \scriptstyle \pm 9975.$ % EUBO d=200
& $-0.105 \scriptstyle \pm 0.01$ % ELBO d=2
& $-7.745 \scriptstyle \pm 0.062$ % ELBO d=50
& $-26.751 \scriptstyle \pm 0.203$ % ELBO d=200
& $0.784 \scriptstyle \pm 0.097$ % EUBO d=2
& $450.376 \scriptstyle \pm 20.523$ % EUBO d=50
& $2127.893 \scriptstyle \pm 228.31$ % EUBO d=200
\\
% 
% \multicolumn{10}{c}{\underline{ELBO}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \midrule
%  & \multicolumn{6}{c}{\textbf{MoS}} \\
% \midrule
% MFVI

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% GMMVI

% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % NFVI
% % & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=2
% % & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=50
% % & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=200
% % & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=2
% % & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=50
% % & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=200
% % \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SMC

% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AFT

% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CRAFT

% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % SNF
% % & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 2
% % & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 50
% % & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 200
% % & $0.000 \scriptstyle{\pm 0.000}$ % GMM 2
% % & $0.000 \scriptstyle{\pm 0.000}$ % GMM 50
% % & $0.000 \scriptstyle{\pm 0.000}$ % GMM 200
% % & $0.000 \scriptstyle{\pm 0.000}$ % STMM 2
% % & $0.000 \scriptstyle{\pm 0.000}$ % STMM 50
% % & $0.000 \scriptstyle{\pm 0.000}$ % STMM 200
% % & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% % \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FAB

% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DDS

% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MCD

% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LDVI

% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CMCD

% \\
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\caption{Mean and standard deviation of ELBO and EUBO values for MoG and MoS for varying dimensions $d$. various target densities. Best results are highlighted in bold. N/A indicates that reasonable results could not be obtained due to numerical problems. }
\label{tab:dim}
\end{table*}

% \end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> results/tables/ess_table.tex <==
\begin{minipage}[b]{\textwidth}
\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{l|ccc|ccc}
\toprule
   & \multicolumn{3}{c|}{$\textbf{ESS}_{r} \ \uparrow$} & \multicolumn{3}{c}{$\textbf{ESS}_{f} \ \uparrow$}  \vspace{0.2cm} \\ 
\textbf{Method}   & $d=2$ & $d=50$  & $d=200$ & $d=2$ & $d=50$  & $d=200$   \\ 
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
 & \multicolumn{6}{c}{\textbf{MoG}} \\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $0.081 \scriptstyle \pm 0.014$ % ELBO d=2
& $0.977 \scriptstyle \pm 0.003$ % ELBO d=50
& $0.921 \scriptstyle \pm 0.002$ % ELBO d=200
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=2
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=50
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $\mathbf{0.994 \scriptstyle \pm 0.015}$ % ELBO d=2
& $\mathbf{0.999 \scriptstyle \pm 0.001}$ % ELBO d=50
& $\mathbf{0.986 \scriptstyle \pm 0.011}$ % ELBO d=200
& $\mathbf{0.993 \scriptstyle \pm 0.016}$ % EUBO d=2
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=50
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $0.240 \scriptstyle \pm 0.019$ % ELBO d=2
& $0.003 \scriptstyle \pm 0.001$ % ELBO d=50
& $0.000 \scriptstyle \pm 0.000$ % ELBO d=200
& $0.003 \scriptstyle \pm 0.001$ % EUBO d=2
& $0.000 \scriptstyle \pm 0.000$% EUBO d=50
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $0.055 \scriptstyle \pm 0.002$ % ELBO d=2
& $0.000 \scriptstyle \pm 0.000$ % ELBO d=50
& $0.000 \scriptstyle \pm 0.000$ % ELBO d=200
& $0.037 \scriptstyle \pm 0.085$ % EUBO d=2
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=50
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $0.039 \scriptstyle \pm 0.002$ % ELBO d=2
& $0.002 \scriptstyle \pm 0.000$ % ELBO d=50
& $0.000 \scriptstyle \pm 0.000$ % ELBO d=200
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=2
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=50
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $0.266 \scriptstyle \pm 0.183$ % ELBO d=2
& $0.002 \scriptstyle \pm 0.001$ % ELBO d=50
& $0.000 \scriptstyle \pm 0.000$ % ELBO d=200
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=2
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=50
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\midrule
 & \multicolumn{6}{c}{\textbf{MoS}} \\
\midrule

MFVI
& $0.367 \scriptstyle \pm 0.004$ % ELBO d=2
& $\mathbf{0.030 \scriptstyle \pm 0.006}$ % ELBO d=50
& $\mathbf{0.006 \scriptstyle \pm 0.001}$ % ELBO d=200
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=2
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=50
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $\mathbf{0.998 \scriptstyle \pm 0.000}$ % ELBO d=2
& $0.025 \scriptstyle \pm 0.004$ % ELBO d=50
& $0.004 \scriptstyle \pm 0.001$ % ELBO d=200
& $\mathbf{0.998 \scriptstyle \pm 0.000}$ % EUBO d=2
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=50
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $0.656 \scriptstyle \pm 0.005$ % ELBO d=2
& $0.001 \scriptstyle \pm 0.000$ % ELBO d=50
& $0.000 \scriptstyle \pm 0.000$ % ELBO d=200
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=2
& $0.000 \scriptstyle \pm 0.000$% EUBO d=50
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $0.293 \scriptstyle \pm 0.007$ % ELBO d=2
& $0.000 \scriptstyle \pm 0.000$ % ELBO d=50
& $0.000 \scriptstyle \pm 0.000$ % ELBO d=200
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=2
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=50
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $0.301 \scriptstyle \pm 0.011$ % ELBO d=2
& $0.000 \scriptstyle \pm 0.000$ % ELBO d=50
& $0.000 \scriptstyle \pm 0.000$ % ELBO d=200
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=2
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=50
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $0.809 \scriptstyle \pm 0.014$ % ELBO d=2
& $0.016 \scriptstyle \pm 0.002$ % ELBO d=50
& $0.003 \scriptstyle \pm 0.000$ % ELBO d=200
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=2
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=50
& $0.000 \scriptstyle \pm 0.000$ % EUBO d=200
\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\captionof{table}{Forward and reverse ESS values MoG and MoS target with varying dimensions $d$. Best results are highlighted with bold font.}
\label{tab:ess}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{minipage}[b]{\textwidth}
\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{l|ccc|ccc}
\toprule
   & \multicolumn{3}{c|}{$\mathbf{\Delta  \log Z}_r \ \downarrow$} & \multicolumn{3}{c}{$\mathbf{\Delta \log Z}_f \ \downarrow$}  \vspace{0.2cm} \\ 
\textbf{Method}   & $d=2$ & $d=50$  & $d=200$ & $d=2$ & $d=50$  & $d=200$   \\ 
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
 & \multicolumn{6}{c}{\textbf{MoG}} \\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $0.096 \scriptstyle \pm 0.061$ % ELBO d=2
& $3.632 \scriptstyle \pm 0.072$ % ELBO d=50
& $3.675 \scriptstyle \pm 0.011$ % ELBO d=200
& $2.21 \scriptstyle \pm 0.455$ % EUBO d=2
& $0.418 \scriptstyle \pm 0.347$ % EUBO d=50
& $0.367 \scriptstyle \pm 0.273$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $\mathbf{0.000 \scriptstyle \pm 0.001}$ % ELBO d=2
& $\mathbf{0.425 \scriptstyle \pm 0.093}$ % ELBO d=50
& $\mathbf{0.652 \scriptstyle \pm 0.082}$ % ELBO d=200
& $\mathbf{0.001 \scriptstyle \pm 0.001}$ % EUBO d=2
& $\mathbf{0.016 \scriptstyle \pm 0.014}$ % EUBO d=50
& $\mathbf{0.022 \scriptstyle \pm 0.016}$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NFVI
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=200
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=200
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $0.064 \scriptstyle \pm 0.032$ % ELBO d=2
& $2109.057 \scriptstyle \pm 11.352$ % ELBO d=50
& $14802.012 \scriptstyle \pm 50.301$ % ELBO d=200
& $1.571 \scriptstyle \pm 0.158$ % EUBO d=2
& $105.897 \scriptstyle \pm 1.268$ % EUBO d=50
& $457.918 \scriptstyle \pm 6.013$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $0.232 \scriptstyle \pm 0.293$ % ELBO d=2
& $1063.314 \scriptstyle \pm 158.795$ % ELBO d=50
& $8224.093 \scriptstyle \pm 483.804$ % ELBO d=200
& $2.645 \scriptstyle \pm 1.319$ % EUBO d=2
& $120.626 \scriptstyle \pm 7.451$ % EUBO d=50
& $492.677 \scriptstyle \pm 21.403$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $0.012 \scriptstyle \pm 0.004$ % ELBO d=2
& $549.203 \scriptstyle \pm 16.553$ % ELBO d=50
& $4026.878 \scriptstyle \pm 102.274$ % ELBO d=200
& $2.217 \scriptstyle \pm 0.264$ % EUBO d=2
& $181.773 \scriptstyle \pm 1.757$ % EUBO d=50
& $814.24 \scriptstyle \pm 9.416$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SNF
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $0.011 \scriptstyle \pm 0.002$ % ELBO d=2
& $3.102 \scriptstyle \pm 0.466$ % ELBO d=50
& $3.468 \scriptstyle \pm 0.181$ % ELBO d=200
& $1.587 \scriptstyle \pm 0.181$ % EUBO d=2
& N/A % EUBO d=50
& N/A % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $0.016 \scriptstyle \pm 0.004$ % ELBO d=2
& $1.928 \scriptstyle \pm 0.292$ % ELBO d=50
& $28.412 \scriptstyle \pm 1.214$ % ELBO d=200
& $6.521 \scriptstyle \pm 0.261$ % EUBO d=2
& $402.851 \scriptstyle \pm 2.534$ % EUBO d=50
& $1688.725 \scriptstyle \pm 12.231$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $0.029 \scriptstyle \pm 0.009$ % ELBO d=2
& $139.57 \scriptstyle \pm 5.504$ % ELBO d=50
& $1610.726 \scriptstyle \pm 81.323$ % ELBO d=200
& $0.514 \scriptstyle \pm 0.528$ % EUBO d=2
& $65.67 \scriptstyle \pm 3.608$ % EUBO d=50
& $552.493 \scriptstyle \pm 45.185$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $0.103 \scriptstyle \pm 0.044$ % ELBO d=2
& $17.106 \scriptstyle \pm 0.777$ % ELBO d=50
& $205.913 \scriptstyle \pm 5.436$ % ELBO d=200
& $1.725 \scriptstyle \pm 0.359$ % EUBO d=2
& $24.109 \scriptstyle \pm 0.931$ % EUBO d=50
& $308.66 \scriptstyle \pm 8.568$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $0.091 \scriptstyle \pm 0.088$ % ELBO d=2
& $6.851 \scriptstyle \pm 0.57$ % ELBO d=50
& $55.669 \scriptstyle \pm 2.517$ % ELBO d=200
& $2.388 \scriptstyle \pm 0.097$ % EUBO d=2
& $9.204 \scriptstyle \pm 1.661$ % EUBO d=50
& $69.276 \scriptstyle \pm 4.694$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\midrule
 & \multicolumn{6}{c}{\textbf{MoS}} \\
\midrule

MFVI
& $0.008 \scriptstyle \pm 0.003$ % ELBO d=2
& $3.391 \scriptstyle \pm 0.262$ % ELBO d=50
& $8.651 \scriptstyle \pm 0.591$ % ELBO d=200
& $0.05 \scriptstyle \pm 0.011$ % EUBO d=2
& $0.031 \scriptstyle \pm 0.011$ % EUBO d=50
& $20.657 \scriptstyle \pm 0.058$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $\mathbf{0.000 \scriptstyle \pm 0.000}$ % ELBO d=2
& $\mathbf{1.140 \scriptstyle \pm 0.205}$ % ELBO d=50
& $\mathbf{8.407 \scriptstyle \pm 0.507}$ % ELBO d=200
& $\mathbf{0.001 \scriptstyle \pm 0.000}$ % EUBO d=2
& $\mathbf{0.316 \scriptstyle \pm 0.129}$ % EUBO d=50
& $\mathbf{10.941 \scriptstyle \pm 2.158}$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NFVI
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=200
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=200
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $0.027 \scriptstyle \pm 0.016$ % ELBO d=2
& $4.065 \scriptstyle \pm 1.592$ % ELBO d=50
& $50.184 \scriptstyle \pm 3.455$ % ELBO d=200
& $0.091 \scriptstyle \pm 0.073$ % EUBO d=2
& $7.203 \scriptstyle \pm 2.062$ % EUBO d=50
& $49.4 \scriptstyle \pm 3.081$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $0.054 \scriptstyle \pm 0.057$ % ELBO d=2
& $8.514 \scriptstyle \pm 3.727$ % ELBO d=50
& $73.425 \scriptstyle \pm 6.25$ % ELBO d=200
& $82.771 \scriptstyle \pm 39.32$ % EUBO d=2
& $410.205 \scriptstyle \pm 63.627$ % EUBO d=50
& $1073.529 \scriptstyle \pm 84.944$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $0.004 \scriptstyle \pm 0.002$ % ELBO d=2
& $0.632 \scriptstyle \pm 0.15$ % ELBO d=50
& $18.867 \scriptstyle \pm 1.585$ % ELBO d=200
& $158.179 \scriptstyle \pm 67.568$ % EUBO d=2
& $1079.617 \scriptstyle \pm 361.956$ % EUBO d=50
& $2557.977 \scriptstyle \pm 278.777$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SNF
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $0.004 \scriptstyle \pm 0.001$ % ELBO d=2
& $2.968 \scriptstyle \pm 0.369$ % ELBO d=50
& $10.228 \scriptstyle \pm 0.421$ % ELBO d=200
& $1.586 \scriptstyle \pm 2.845$ % EUBO d=2
& $152.025 \scriptstyle \pm 32.336$ % EUBO d=50
& N/A % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $0.005 \scriptstyle \pm 0.002$ % ELBO d=2
& $14.506 \scriptstyle \pm 0.743$ % ELBO d=50
& $188.676 \scriptstyle \pm 3.091$ % ELBO d=200
& $2.988 \scriptstyle \pm 1.101$ % EUBO d=2
& $138.224 \scriptstyle \pm 2.312$ % EUBO d=50
& $540.066 \scriptstyle \pm 3.639$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $0.008 \scriptstyle \pm 0.002$ % ELBO d=2
& $46.134 \scriptstyle \pm 2.772$ % ELBO d=50
& $308.787 \scriptstyle \pm 3.666$ % ELBO d=200
& $0.066 \scriptstyle \pm 0.009$ % EUBO d=2
& $38.923 \scriptstyle \pm 1.004$ % EUBO d=50
& $206.156 \scriptstyle \pm 3.396$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $0.009 \scriptstyle \pm 0.003$ % ELBO d=2
& $32.8 \scriptstyle \pm 1.241$ % ELBO d=50
& $244.412 \scriptstyle \pm 2.419$ % ELBO d=200
& $0.048 \scriptstyle \pm 0.039$ % EUBO d=2
& $29.47 \scriptstyle \pm 1.381$ % EUBO d=50
& $169.545 \scriptstyle \pm 2.822$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $0.004 \scriptstyle \pm 0.001$ % ELBO d=2
& $3.032 \scriptstyle \pm 0.29$ % ELBO d=50
& $10.408 \scriptstyle \pm 0.692$ % ELBO d=200
& $0.03 \scriptstyle \pm 0.061$ % EUBO d=2
& $1.162 \scriptstyle \pm 0.366$ % EUBO d=50
& $18.321 \scriptstyle \pm 2.048$ % EUBO d=200
\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\captionof{table}{Forward and reverse estimation of $\log Z$ on MoG and MoS target with varying dimensions $d$. Best results are highlighted with bold font.}
\label{tab:fwd_rev_lnz}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> results/tables/fevals_table.tex <==
\begin{table}
% \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
\label{table:vi_results}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cccccccc}
\begin{tabular}{l|rrrrrrrr}
\toprule
  \textbf{NFE}   & Funnel (10) & Credit (25)& Seeds (26) & Cancer (31) &  Brownian (32) & Ionosphere (35) & Sonar (61)  & LGCP (1600) \\ 
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
NFVI
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SNF
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
PIS
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> results/tables/fwd_rev_kl_table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t!]
% \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cc|cc|cc|cc|cc}
\toprule
& \multicolumn{2}{c}{\textbf{Funnel}} 
& \multicolumn{2}{c}{\textbf{MoG} $(d=50)$}  
& \multicolumn{2}{c}{\textbf{MoS} $(d=50)$} 
& \multicolumn{2}{c}{$14 \times 14$ \textbf{Digits}}  
& \multicolumn{2}{c}{$28 \times 28$ \textbf{Fashion}} 
\vspace{0.2cm}
\\ 
& {\textbf{ELBO} $\uparrow$}
& {\textbf{EUBO} $\downarrow$}
& {\textbf{ELBO} $\uparrow$}
& {\textbf{EUBO} $\downarrow$}
& {\textbf{ELBO} $\uparrow$}
& {\textbf{EUBO} $\downarrow$}
& {\textbf{ELBO} $\uparrow$}
& {\textbf{EUBO} $\downarrow$}
& {\textbf{ELBO} $\uparrow$}
& {\textbf{EUBO} $\downarrow$}
\\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $-1.834 \scriptstyle \pm 0.009$
& $105.694 \scriptstyle \pm 0.002$
& $-3.69 \scriptstyle \pm 0.0$
& $164.114 \scriptstyle \pm 0.0$
& $-5.957 \scriptstyle \pm 0.007$
& $72.663 \scriptstyle \pm 0.005$
& $-14.004 \scriptstyle \pm 0.005$
& $210.713 \scriptstyle \pm 0.024$
& $-58.082 \scriptstyle \pm 0.009$
& $938.632 \scriptstyle \pm 0.055$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $-0.013 \scriptstyle \pm 0.001$
& $-33.987 \scriptstyle \pm 3.513$
& $-1.715 \scriptstyle \pm 0.119$
& $-6351.06 \scriptstyle \pm 1097.981$
& $-3.89 \scriptstyle \pm 0.122$
& $-279.166 \scriptstyle \pm 62.92$
& $-7.166 \scriptstyle \pm 0.16$
& $-253.283 \scriptstyle \pm 7.02$
& $-18.137 \scriptstyle \pm 3.85$
& $-1877.877 \scriptstyle \pm 18.454$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $-0.242 \scriptstyle \pm 0.047$
& $4.69 \scriptstyle \pm 0.0$
& $-877.034 \scriptstyle \pm 10.231$
& $161.921 \scriptstyle \pm 0.0$
& $-4.634 \scriptstyle \pm 1.088$
& $81.325 \scriptstyle \pm 0.0$
& $-185.057 \scriptstyle \pm 0.257$
& $376.093 \scriptstyle \pm 0.0$
& $-12187.873 \scriptstyle \pm 134.695$
& $1532.904 \scriptstyle \pm 0.0$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $-0.293 \scriptstyle \pm 0.088$
& $431.329 \scriptstyle \pm 143.186$
& $-927.16 \scriptstyle \pm 103.812$
& $117.63 \scriptstyle \pm 22.161$
& $-4.923 \scriptstyle \pm 1.546$
& $207.625 \scriptstyle \pm 24.148$
& $-64.442 \scriptstyle \pm 4.464$
& $214.486 \scriptstyle \pm 4.87$
& $-11828.529 \scriptstyle \pm 1608.069$
& $1448.335 \scriptstyle \pm 11.085$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $-0.027 \scriptstyle \pm 0.06$
& $263.474 \scriptstyle \pm 7.864$
& $-451.399 \scriptstyle \pm 7.561$
& $103.674 \scriptstyle \pm 0.069$
& $-0.295 \scriptstyle \pm 0.256$
& $212.21 \scriptstyle \pm 6.16$
& $-11.154 \scriptstyle \pm 0.307$
& $89.518 \scriptstyle \pm 1.904$
& $-520.475 \scriptstyle \pm 5.531$
& $1578.114 \scriptstyle \pm 2.36$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $-0.014 \scriptstyle \pm 0.003$
& $0.012 \scriptstyle \pm 0.002$
& $-299.916 \scriptstyle \pm 253.455$
& $93.56 \scriptstyle \pm 5.086$
& $75.735 \scriptstyle \pm 175.894$
& $18.088 \scriptstyle \pm 2.503$
& $-11.396 \scriptstyle \pm 0.153$
& $12.084 \scriptstyle \pm 0.171$
& $80236732403.708 \scriptstyle \pm 138974097184.917$
& $394.346 \scriptstyle \pm 263.681$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $-0.611 \scriptstyle \pm 0.005$
& N/A
& $-185.021 \scriptstyle \pm 0.743$
& $43.67 \scriptstyle \pm 0.457$
& $-69.358 \scriptstyle \pm 0.633$
& $47.834 \scriptstyle \pm 0.82$
& $-1457.646 \scriptstyle \pm 13.804$
& $293.191 \scriptstyle \pm 0.208$
& $-21196.583 \scriptstyle \pm 472.858$
& $1276.456 \scriptstyle \pm 1.033$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& N/A
& N/A
& $-29.034 \scriptstyle \pm 0.591$
& $51.137 \scriptstyle \pm 0.177$
& $-28.471 \scriptstyle \pm 1.018$
& $20.887 \scriptstyle \pm 1.042$
& $-875.104 \scriptstyle \pm 43.597$
& $323.158 \scriptstyle \pm 0.142$
& $-16227.975 \scriptstyle \pm 738.056$
& $1185.331 \scriptstyle \pm 6.66$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
PIS
& $-3.198 \scriptstyle \pm 0.042$
& $104.975 \scriptstyle \pm 0.002$
& $-16.881 \scriptstyle \pm 0.026$
& $3626.12 \scriptstyle \pm 1.36$
& $-29.261 \scriptstyle \pm 1.743$
& $88.192 \scriptstyle \pm 0.005$
& $-172.988 \scriptstyle \pm 0.63$
& $2748.938 \scriptstyle \pm 19.194$
& $-2988.21 \scriptstyle \pm 14.137$
& $11179.374 \scriptstyle \pm 11.724$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DIS
& $-1.021 \scriptstyle \pm 0.436$
& $40.892 \scriptstyle \pm 38.482$
& $-181.348 \scriptstyle \pm 15.47$
& $546.335 \scriptstyle \pm 30.861$
& $-36.704 \scriptstyle \pm 0.629$
& $193.27 \scriptstyle \pm 3.293$
& $-840.122 \scriptstyle \pm 18.66$
& $1745.719 \scriptstyle \pm 205.745$
& $-15337.229 \scriptstyle \pm 154.075$
& $20347.781 \scriptstyle \pm 318.729$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $-0.597 \scriptstyle \pm 0.142$
& $148.841 \scriptstyle \pm 7.347$
& $-13.284 \scriptstyle \pm 0.46$
& $291.867 \scriptstyle \pm 0.047$
& $-31.681 \scriptstyle \pm 0.363$
& $86.014 \scriptstyle \pm 0.001$
& $-156.145 \scriptstyle \pm 6.063$
& $881.476 \scriptstyle \pm 22.832$
& $-2617.761 \scriptstyle \pm 46.789$
& $3925.231 \scriptstyle \pm 106.877$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GBS
& $-2.6 \scriptstyle \pm 0.078$
& $110.167 \scriptstyle \pm 0.0$
& $-35.771 \scriptstyle \pm 1.105$
& $67.819 \scriptstyle \pm 2.157$
& $-99.369 \scriptstyle \pm 0.158$
& $73.545 \scriptstyle \pm 0.107$
& $-154.186 \scriptstyle \pm 1.387$
& $106.777 \scriptstyle \pm 0.113$
& $-2198.997 \scriptstyle \pm 36.564$
& $705.996 \scriptstyle \pm 11.665$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
    \caption{ELBO values for various target densities. Best results are highlighted using bold font. N/A indicates that reasonable results could not be obtained due to numerical problems. OOM refers to out-of-memory problems. \red{Mention target samples.}
    }
    \vspace{-0.2cm}
\label{table:elbos}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> results/tables/fwd_rev_lnZ_table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t!]
% \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cc|cc|cc|cc|cc}
\toprule
& \multicolumn{2}{c}{\textbf{Funnel}} 
& \multicolumn{2}{c}{\textbf{MoG} $(d=50)$}  
& \multicolumn{2}{c}{\textbf{MoS} $(d=50)$} 
& \multicolumn{2}{c}{$14 \times 14$ \textbf{Digits}}  
& \multicolumn{2}{c}{$28 \times 28$ \textbf{Fashion}} 
\vspace{0.2cm}
\\ 
& {$\mathbf{\Delta \log Z}_{r} \downarrow$}
& {$\mathbf{\Delta \log Z}_{f} \downarrow$}
& {$\mathbf{\Delta \log Z}_{r} \downarrow$}
& {$\mathbf{\Delta \log Z}_{f} \downarrow$}
& {$\mathbf{\Delta \log Z}_{r} \downarrow$}
& {$\mathbf{\Delta \log Z}_{f} \downarrow$}
& {$\mathbf{\Delta \log Z}_{r} \downarrow$}
& {$\mathbf{\Delta \log Z}_{f} \downarrow$}
& {$\mathbf{\Delta \log Z}_{r} \downarrow$}
& {$\mathbf{\Delta \log Z}_{f} \downarrow$}
\\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $0.612 \scriptstyle \pm 0.101$
& $0.036 \scriptstyle \pm 0.001$
& $3.658 \scriptstyle \pm 0.04$
& $0.185 \scriptstyle \pm 0.002$
& $3.009 \scriptstyle \pm 0.291$
& $0.048 \scriptstyle \pm 0.002$
& $7.388 \scriptstyle \pm 0.107$
& $5.866 \scriptstyle \pm 0.016$
& $34.389 \scriptstyle \pm 0.757$
& $108.379 \scriptstyle \pm 0.438$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $0.001 \scriptstyle \pm 0.0$
& $0.024 \scriptstyle \pm 0.002$
& $1.715 \scriptstyle \pm 0.119$
& $322.798 \scriptstyle \pm 76.335$
& $1.282 \scriptstyle \pm 0.221$
& $543.329 \scriptstyle \pm 135.095$
& $3.087 \scriptstyle \pm 0.348$
& $267.044 \scriptstyle \pm 4.072$
& $8.717 \scriptstyle \pm 2.266$
& $1392.604 \scriptstyle \pm 136.253$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $0.187 \scriptstyle \pm 0.054$
& $2.676 \scriptstyle \pm 0.0$
& $690.721 \scriptstyle \pm 11.215$
& $161.796 \scriptstyle \pm 0.0$
& $3.88 \scriptstyle \pm 1.105$
& $80.992 \scriptstyle \pm 0.0$
& $80.184 \scriptstyle \pm 0.162$
& $375.676 \scriptstyle \pm 0.0$
& $11742.014 \scriptstyle \pm 139.276$
& $1530.824 \scriptstyle \pm 0.0$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $0.181 \scriptstyle \pm 0.106$
& $414.619 \scriptstyle \pm 141.542$
& $765.624 \scriptstyle \pm 108.027$
& $110.955 \scriptstyle \pm 18.372$
& $4.081 \scriptstyle \pm 1.579$
& $205.297 \scriptstyle \pm 23.918$
& $16.726 \scriptstyle \pm 2.511$
& $163.871 \scriptstyle \pm 6.557$
& $11653.343 \scriptstyle \pm 1628.565$
& $1071.777 \scriptstyle \pm 9.475$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $0.091 \scriptstyle \pm 0.018$
& $255.046 \scriptstyle \pm 7.478$
& $337.094 \scriptstyle \pm 9.296$
& $100.987 \scriptstyle \pm 0.065$
& $0.822 \scriptstyle \pm 0.087$
& $210.245 \scriptstyle \pm 6.098$
& $1.458 \scriptstyle \pm 0.406$
& $63.792 \scriptstyle \pm 3.329$
& $445.101 \scriptstyle \pm 8.273$
& $1156.718 \scriptstyle \pm 7.81$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $0.001 \scriptstyle \pm 0.0$
& $0.019 \scriptstyle \pm 0.003$
& $2.952 \scriptstyle \pm 0.247$
& $126.363 \scriptstyle \pm 1.789$
& $3.358 \scriptstyle \pm 1.062$
& $84.592 \scriptstyle \pm 22.649$
& $0.847 \scriptstyle \pm 0.076$
& $63.91 \scriptstyle \pm 1.565$
& $350.544 \scriptstyle \pm 599.01$
& $3721.72 \scriptstyle \pm 4646.803$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $0.207 \scriptstyle \pm 0.039$
& N/A
& $31.319 \scriptstyle \pm 1.793$
& $21.148 \scriptstyle \pm 1.478$
& $28.607 \scriptstyle \pm 1.275$
& $24.757 \scriptstyle \pm 0.841$
& $884.61 \scriptstyle \pm 9.674$
& $258.84 \scriptstyle \pm 3.047$
& $15122.09 \scriptstyle \pm 996.768$
& $1125.475 \scriptstyle \pm 5.198$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& N/A
& N/A
& $8.159 \scriptstyle \pm 0.775$
& $15.477 \scriptstyle \pm 0.815$
& $4.36 \scriptstyle \pm 0.741$
& $5.472 \scriptstyle \pm 0.938$
& $537.763 \scriptstyle \pm 25.076$
& $265.674 \scriptstyle \pm 1.181$
& $12237.989 \scriptstyle \pm 381.833$
& $1087.592 \scriptstyle \pm 4.844$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
PIS
& $0.918 \scriptstyle \pm 0.598$
& $0.436 \scriptstyle \pm 0.002$
& $7.122 \scriptstyle \pm 0.63$
& $3113.492 \scriptstyle \pm 1.978$
& $12.248 \scriptstyle \pm 0.326$
& $54.09 \scriptstyle \pm 0.151$
& $104.002 \scriptstyle \pm 0.847$
& $2149.224 \scriptstyle \pm 19.391$
& $1884.013 \scriptstyle \pm 10.207$
& $8785.873 \scriptstyle \pm 9.88$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DIS
& $0.113 \scriptstyle \pm 0.083$
& $25.544 \scriptstyle \pm 8.267$
& $87.709 \scriptstyle \pm 8.942$
& $369.352 \scriptstyle \pm 16.293$
& $10.448 \scriptstyle \pm 0.607$
& $87.897 \scriptstyle \pm 5.255$
& $569.837 \scriptstyle \pm 35.408$
& $1354.472 \scriptstyle \pm 181.145$
& $8807.43 \scriptstyle \pm 337.642$
& $17566.52 \scriptstyle \pm 256.653$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $0.19 \scriptstyle \pm 0.077$
& $0.321 \scriptstyle \pm 0.052$
& $1.739 \scriptstyle \pm 0.442$
& $207.545 \scriptstyle \pm 1.163$
& $7.952 \scriptstyle \pm 0.299$
& $53.411 \scriptstyle \pm 0.024$
& $82.46 \scriptstyle \pm 5.48$
& $659.497 \scriptstyle \pm 9.786$
& $1579.602 \scriptstyle \pm 41.652$
& $2910.345 \scriptstyle \pm 71.256$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GBS
& $0.553 \scriptstyle \pm 0.273$
& $0.127 \scriptstyle \pm 0.008$
& $8.103 \scriptstyle \pm 1.696$
& $9.321 \scriptstyle \pm 0.776$
& $53.767 \scriptstyle \pm 0.732$
& $47.441 \scriptstyle \pm 0.098$
& $75.16 \scriptstyle \pm 2.321$
& $62.733 \scriptstyle \pm 1.168$
& $1495.194 \scriptstyle \pm 42.031$
& $527.58 \scriptstyle \pm 9.426$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
    \caption{ELBO values for various target densities. Best results are highlighted using bold font. N/A indicates that reasonable results could not be obtained due to numerical problems. OOM refers to out-of-memory problems. \red{Mention target samples.}
    }
    \vspace{-0.2cm}
\label{table:elbos}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> results/tables/gmm40_dim_results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}{\textwidth}
\begin{minipage}[h]{0.36\textwidth}
\centering
 \resizebox{\textwidth}{!}{%
\includegraphics[]{results/entropy/IGMM.pdf}
}
\captionof{figure}{EMC for different dimensions}
\end{minipage}
\hfill
\begin{minipage}[h]{0.59\textwidth}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccc|ccc}
\toprule
   & \multicolumn{3}{c|}{\textbf{ELBO} $\uparrow$} & \multicolumn{3}{c}{\textbf{EUBO} $\downarrow$}   \\ 
\textbf{Method}   & $d=2$ & $d=50$  & $d=200$ & $d=2$ & $d=50$  & $d=200$   \\ 
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $-3.01 \scriptstyle \pm 0.004$ % ELBO d=2
& $-3.699 \scriptstyle \pm 0.001$ % ELBO d=50
& $-3.73 \scriptstyle \pm 0.003$ % ELBO d=200
& $168.026 \scriptstyle \pm 1.489$ % EUBO d=2
& $23047.8 \scriptstyle \pm 60.134$ % EUBO d=50
& $97607.177 \scriptstyle \pm 14.443$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $\mathbf{-0.002 \scriptstyle \pm 0.002}$ % ELBO d=2
& $\mathbf{-0.425 \scriptstyle \pm 0.092}$ % ELBO d=50
& $\mathbf{-0.698 \scriptstyle \pm 0.089}$ % ELBO d=200
& $\mathbf{0.004 \scriptstyle \pm 0.003}$ % EUBO d=2
& $698.25 \scriptstyle \pm 571.8$ % EUBO d=50
& $1734.625 \scriptstyle \pm 1220.704$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NFVI
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=200
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=200
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $-9.09 \scriptstyle \pm 0.033$ % ELBO d=2
& $-2462.479 \scriptstyle \pm 10.506$ % ELBO d=50
& $-15780.962 \scriptstyle \pm 42.909$ % ELBO d=200
& $1.663 \scriptstyle \pm 0.137$ % EUBO d=2
& $109.287 \scriptstyle \pm 1.088$ % EUBO d=50
& $\mathbf{468.091 \scriptstyle \pm 5.11}$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $-3.046 \scriptstyle \pm 0.439$ % ELBO d=2
& $-1241.237 \scriptstyle \pm 147.377$ % ELBO d=50
& $-8690.66 \scriptstyle \pm 474.741$ % ELBO d=200
& $2.744 \scriptstyle \pm 1.373$ % EUBO d=2
& $135.317 \scriptstyle \pm 27.147$ % EUBO d=50
& $513.179 \scriptstyle \pm 17.674$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $-3.527 \scriptstyle \pm 0.063$ % ELBO d=2
& $-777.939 \scriptstyle \pm 16.578$ % ELBO d=50
& $-4614.218 \scriptstyle \pm 97.283$ % ELBO d=200
& $2.05 \scriptstyle \pm 0.029$ % EUBO d=2
& $215.942 \scriptstyle \pm 1.484$ % EUBO d=50
& $917.075 \scriptstyle \pm 9.723$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SNF
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $-6.463 \scriptstyle \pm 1.113$ % ELBO d=2
& $-1296.493 \scriptstyle \pm 621.829$ % ELBO d=50
& $-724.248 \scriptstyle \pm 500.415$ % ELBO d=200
& $1.072 \scriptstyle \pm 0.071$ % EUBO d=2
& $\infty$ % EUBO d=50
& $\infty$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $9.714 \scriptstyle \pm 0.211$ % ELBO d=2
& $419.838 \scriptstyle \pm 3.276$ % ELBO d=50
& $1720.661 \scriptstyle \pm 12.254$ % ELBO d=200
& $9.714 \scriptstyle \pm 0.211$ % EUBO d=2
& $419.838 \scriptstyle \pm 3.276$ % EUBO d=50
& $1720.661 \scriptstyle \pm 12.254$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $-2.678 \scriptstyle \pm 0.166$ % ELBO d=2
& $-888.236 \scriptstyle \pm 8.752$ % ELBO d=50
& $-4250.623 \scriptstyle \pm 212.37$ % ELBO d=200
& $2.136 \scriptstyle \pm 0.062$ % EUBO d=2
& $\mathbf{108.822 \scriptstyle \pm 3.076}$ % EUBO d=50
& $973.636 \scriptstyle \pm 85.268$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $-3.84 \scriptstyle \pm 0.236$ % ELBO d=2
& $-43.818 \scriptstyle \pm 0.325$ % ELBO d=50
& $-302.141 \scriptstyle \pm 3.012$ % ELBO d=200
& $26.539 \scriptstyle \pm 9.463$ % EUBO d=2
& $2785.126 \scriptstyle \pm 88.016$ % EUBO d=50
& $551.403 \scriptstyle \pm 18.087$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $-3.821 \scriptstyle \pm 0.341$ % ELBO d=2
& $-25.264 \scriptstyle \pm 0.252$ % ELBO d=50
& $-108.881 \scriptstyle \pm 4.515$ % ELBO d=200
& $53.192 \scriptstyle \pm 14.543$ % EUBO d=2
& $8252.215 \scriptstyle \pm 1024.625$ % EUBO d=50
& $37456.045 \scriptstyle \pm 9975.166$ % EUBO d=200
\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\captionof{table}{A table beside a figure}
\end{minipage}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \begin{table*}
% % \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
% \label{table:vi_results}
% \begin{center}
% \begin{small}
% \begin{sc}
% \resizebox{\textwidth}{!}{%
% % \begin{tabular}{l|cccccccc}
% \begin{tabular}{l|ccc|ccc}
% \toprule
%    & \multicolumn{3}{c|}{\textbf{ELBO}} & \multicolumn{3}{c}{\textbf{EUBO}}   \\ 
% \textbf{Method}   & $d=2$ & $d=50$  & $d=200$ & $d=2$ & $d=50$  & $d=200$   \\ 
% \midrule
% % \multicolumn{10}{c}{\underline{ELBO}} \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MFVI
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=200
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=200
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% GMMVI
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=200
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=200
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NFVI
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=200
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=200
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SMC
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=200
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=200
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AFT
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=200
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=200
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CRAFT
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=200
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=200
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % SNF
% % & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 2
% % & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 50
% % & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 200
% % & $0.000 \scriptstyle{\pm 0.000}$ % GMM 2
% % & $0.000 \scriptstyle{\pm 0.000}$ % GMM 50
% % & $0.000 \scriptstyle{\pm 0.000}$ % GMM 200
% % & $0.000 \scriptstyle{\pm 0.000}$ % STMM 2
% % & $0.000 \scriptstyle{\pm 0.000}$ % STMM 50
% % & $0.000 \scriptstyle{\pm 0.000}$ % STMM 200
% % & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% % \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FAB
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=200
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=200
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DDS
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=200
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=200
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MCD
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=200
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=200
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LDVI
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=200
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=200
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CMCD
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=200
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=200
% \\
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \bottomrule
% \end{tabular}
% }
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> results/tables/ln_z_table.tex <==
\begin{table}[t!]
% \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{.4\textwidth}{!}{%
% \begin{tabular}{l|cccccccc}
\begin{tabular}{l|cc}
\toprule
  $\mathbf{\Delta \log Z}_{r} \, \downarrow$   & \textbf{Funnel} & \textbf{ManyWell} \\ % GMM (50)& STMM (50) & BMM (50) &   NICE (144) & -  &- \\ 
    % & $\mathbf{\Delta \log Z} \, \downarrow$ & $\mathbf{\Delta \log Z} \, \downarrow$
    %  \\
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $0.693 \scriptstyle \pm 0.095$ % Funnel
% & $0.09 \scriptstyle \pm 0.001$
% & $178.326 \scriptstyle \pm 0.228$
& $2.634 \scriptstyle \pm 0.044$ % ManyWell
% & $26.38 \scriptstyle \pm 1.339$ % GMM
% & $3.397 \scriptstyle \pm 0.245$ % STMM
% & $7.177 \scriptstyle \pm 0.503$ % BMM
% & $7.220 \scriptstyle \pm 0.354$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $\mathbf{0.002 \scriptstyle \pm 0.001}$% Funnel
% & $0.000 \scriptstyle{\pm 0.000}$
% & $0.000 \scriptstyle{\pm 0.000}$
& $1.055 \scriptstyle \pm 0.018$ % ManyWell
% & $0.055 \scriptstyle \pm 0.027$ % GMM
% & $1.471 \scriptstyle \pm 0.211$ % STMM
% & $0.415 \scriptstyle \pm 0.069$ % BMM
% & N/A % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NFVI
% & $0.000 \scriptstyle{\pm 0.000}$ % Funnel
% & $0.000 \scriptstyle{\pm 0.000}$ % ManyWell
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$ % -
% & $0.000 \scriptstyle{\pm 0.000}$ % -
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $0.220 \scriptstyle \pm 0.080$ % Funnel
% & $0.026 \scriptstyle \pm 0.007$
% & $152.839 \scriptstyle \pm 5.083$
& $0.576 \scriptstyle \pm 0.357$ % ManyWell
% & $1.797 \scriptstyle \pm 0.900$ % GMM
% & $2.923 \scriptstyle \pm 1.542$ % STMM
% & $489.6 \scriptstyle \pm 753.2$ % BMM
% & $70.15 \scriptstyle \pm 9.340$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $0.184 \scriptstyle \pm 0.087$ % Funnel
% & $0.021 \scriptstyle \pm 0.005$
% & $145.451 \scriptstyle \pm 5.596$
& $0.749 \scriptstyle \pm 0.717$ % ManyWell
% & $1.060 \scriptstyle \pm 0.647$  % GMM
% & $3.227 \scriptstyle \pm 1.425$  % STMM
% & $131.1 \scriptstyle \pm 14.91$  % BMM
% & $16.46 \scriptstyle \pm 4.432$  % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $0.101 \scriptstyle \pm 0.014$ % Funnel
% & $0.012 \scriptstyle \pm 0.001$
% & $133.53 \scriptstyle \pm 0.988$
& $0.253 \scriptstyle \pm 0.081$ % ManyWell
% & $0.574 \scriptstyle \pm 0.108$ % GMM
% & $0.701 \scriptstyle \pm 0.159$ % STMM
% & $85.073 \scriptstyle \pm 4.526$ % BMM
% & $\mathbf{1.003 \scriptstyle \pm 0.207}$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SNF
& $0.138 \scriptstyle \pm 0.022$ % Funnel
% & $0.018 \scriptstyle \pm 0.002$
% & $143.121 \scriptstyle \pm 1.407$
& $\mathbf{0.142 \scriptstyle \pm 0.054}$ % ManyWell
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $1.39 \scriptstyle \pm 0.419$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$ % -
% & $0.000 \scriptstyle{\pm 0.000}$ % -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
% & $0.000 \scriptstyle{\pm 0.000}$ % ManyWell
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM
& $0.337 \scriptstyle \pm 0.0$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$ % -
% & $0.000 \scriptstyle{\pm 0.000}$ % -
\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $0.145 \scriptstyle \pm 0.000$ % Funnel
% & $0.000 \scriptstyle{\pm 0.000}$ % ManyWell
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM
& $1.911 \scriptstyle \pm 0.000$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$ % -
% & $0.000 \scriptstyle{\pm 0.000}$ % -
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PIS
% & $0.148 \scriptstyle \pm 0.030$ % Funnel
% & $0.000 \scriptstyle{\pm 0.000}$
% & $0.000 \scriptstyle{\pm 0.000}$
% & $33.21 \scriptstyle \pm 16.46$ % ManyWell
% & $2.984 \scriptstyle \pm 0.230$ % GMM
% & $2.820 \scriptstyle \pm 0.156$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $0.231 \scriptstyle \pm 0.016$ % Funnel
% & $0.062 \scriptstyle \pm 0.001$
% & $170.088 \scriptstyle \pm 0.434$
& $2.340 \scriptstyle \pm 0.264$ % ManyWell
% & $19.87 \scriptstyle \pm 10.49$ % GMM
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $0.145 \scriptstyle \pm 0.035$ % Funnel
% & $0.000 \scriptstyle{\pm 0.000}$
% & $0.000 \scriptstyle{\pm 0.000}$
& $0.768 \scriptstyle \pm 0.168$ % ManyWell
% & $3.113 \scriptstyle \pm 1.030$ % GMM
% & $1.568 \scriptstyle \pm 0.638$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $152.7 \scriptstyle \pm 47.02$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $0.057 \scriptstyle \pm 0.008$ % Funnel
% & $0.007 \scriptstyle \pm 0.001$
% & $120.015 \scriptstyle \pm 0.941$
& $0.196 \scriptstyle \pm 0.095$ % ManyWell
% & $28.78 \scriptstyle \pm 35.51$ % GMM
% & $9.354 \scriptstyle \pm 2.604$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $568.5 \scriptstyle \pm 260.6$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
    \caption{Results for the reverse estimation error of $\log Z$.
    }
\label{tab:lnz}
\vspace{-0.3cm}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> results/tables/ln_z_table_old.tex <==
\begin{table}[t!]
% \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
\label{table:lnz_results}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{.47\textwidth}{!}{%
% \begin{tabular}{l|cccccccc}
\begin{tabular}{l|cccc}
\toprule
     & \textbf{Funnel} & \textbf{ManyWell} \\ % GMM (50)& STMM (50) & BMM (50) &   NICE (144) & -  &- \\ 
& $\mathbf{\Delta \log Z} \, \downarrow$ & MMD & W2 & $\mathbf{\Delta \log Z} \, \downarrow$
     
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $0.693 \scriptstyle \pm 0.095$ % Funnel
& $2.634 \scriptstyle \pm 0.044$ % ManyWell
% & $26.38 \scriptstyle \pm 1.339$ % GMM
% & $3.397 \scriptstyle \pm 0.245$ % STMM
% & $7.177 \scriptstyle \pm 0.503$ % BMM
% & $7.220 \scriptstyle \pm 0.354$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $\mathbf{0.002 \scriptstyle \pm 0.001}$% Funnel
& $1.055 \scriptstyle \pm 0.018$ % ManyWell
% & $0.055 \scriptstyle \pm 0.027$ % GMM
% & $1.471 \scriptstyle \pm 0.211$ % STMM
% & $0.415 \scriptstyle \pm 0.069$ % BMM
% & N/A % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NFVI
% & $0.000 \scriptstyle{\pm 0.000}$ % Funnel
% & $0.000 \scriptstyle{\pm 0.000}$ % ManyWell
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$ % -
% & $0.000 \scriptstyle{\pm 0.000}$ % -
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $0.220 \scriptstyle \pm 0.080$ % Funnel
& $0.576 \scriptstyle \pm 0.357$ % ManyWell
% & $1.797 \scriptstyle \pm 0.900$ % GMM
% & $2.923 \scriptstyle \pm 1.542$ % STMM
% & $489.6 \scriptstyle \pm 753.2$ % BMM
% & $70.15 \scriptstyle \pm 9.340$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $0.184 \scriptstyle \pm 0.087$ % Funnel
& $0.749 \scriptstyle \pm 0.717$ % ManyWell
% & $1.060 \scriptstyle \pm 0.647$  % GMM
% & $3.227 \scriptstyle \pm 1.425$  % STMM
% & $131.1 \scriptstyle \pm 14.91$  % BMM
% & $16.46 \scriptstyle \pm 4.432$  % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $0.101 \scriptstyle \pm 0.014$ % Funnel
& $0.253 \scriptstyle \pm 0.081$ % ManyWell
% & $0.574 \scriptstyle \pm 0.108$ % GMM
% & $0.701 \scriptstyle \pm 0.159$ % STMM
% & $85.073 \scriptstyle \pm 4.526$ % BMM
% & $\mathbf{1.003 \scriptstyle \pm 0.207}$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SNF
& $0.138 \scriptstyle \pm 0.022$ % Funnel
& $\mathbf{0.142 \scriptstyle \pm 0.054}$ % ManyWell
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $1.39 \scriptstyle \pm 0.419$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$ % -
% & $0.000 \scriptstyle{\pm 0.000}$ % -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FAB
% & $0.000 \scriptstyle{\pm 0.000}$ % Funnel
% & $0.000 \scriptstyle{\pm 0.000}$ % ManyWell
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$ % -
% & $0.000 \scriptstyle{\pm 0.000}$ % -
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DDS
% & $0.000 \scriptstyle{\pm 0.000}$ % Funnel
% & $0.000 \scriptstyle{\pm 0.000}$ % ManyWell
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$ % -
% & $0.000 \scriptstyle{\pm 0.000}$ % -
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
PIS
& $0.148 \scriptstyle \pm 0.030$ % Funnel
& $33.21 \scriptstyle \pm 16.46$ % ManyWell
% & $2.984 \scriptstyle \pm 0.230$ % GMM
% & $2.820 \scriptstyle \pm 0.156$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $0.231 \scriptstyle \pm 0.016$ % Funnel
& $2.340 \scriptstyle \pm 0.264$ % ManyWell
% & $19.87 \scriptstyle \pm 10.49$ % GMM
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $0.145 \scriptstyle \pm 0.035$ % Funnel
& $0.768 \scriptstyle \pm 0.168$ % ManyWell
% & $3.113 \scriptstyle \pm 1.030$ % GMM
% & $1.568 \scriptstyle \pm 0.638$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $152.7 \scriptstyle \pm 47.02$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $0.057 \scriptstyle \pm 0.008$ % Funnel
& $0.196 \scriptstyle \pm 0.095$ % ManyWell
% & $28.78 \scriptstyle \pm 35.51$ % GMM
% & $9.354 \scriptstyle \pm 2.604$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $568.5 \scriptstyle \pm 260.6$ % NICE
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & $0.000 \scriptstyle{\pm 0.000}$  % -
% & -
% & -
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
    \caption{\red{Add MoG and STMM for same $d$? Remove NICE since it is already there. Add reverse estimation here.}
    }
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> results/tables/mmd_table.tex <==
\begin{table*}
% \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
\label{table:vi_results}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cccccccc}
\begin{tabular}{l|rrrrrrrr}
\toprule
  $\text{MMD}^2$  & Funnel (10) & Reacher (10) & Credit (25)& Cancer (31) & GMM (50)& STMM (50) & BMM (50) &  NICE (144) \\ 
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.316 \scriptstyle \pm 0.0$ % Reacher
& $0.296 \scriptstyle \pm 0.0$ % Credit
& $0.201 \scriptstyle \pm 0.001$ % Cancer
& $0.021 \scriptstyle \pm 0.0$ % GMM
& $0.037 \scriptstyle \pm 0.0$ % STMM
& $0.061 \scriptstyle \pm 0.0$ % BMM
& $0.116 \scriptstyle \pm 0.0$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.19 \scriptstyle \pm 0.154$ % Reacher
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.52 \scriptstyle \pm 0.023$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % GMM
& $0.031 \scriptstyle \pm 0.014$ % STMM
& $0.005 \scriptstyle \pm 0.002$ % BMM
& $0.000 \scriptstyle{\pm 0.000}$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NFVI
% & $0.000 \scriptstyle{\pm 0.000}$ % Funnel
% & $0.000 \scriptstyle{\pm 0.000}$ % Reacher
% & $0.000 \scriptstyle{\pm 0.000}$ % Credit
% & $0.000 \scriptstyle{\pm 0.000}$ % Cancer
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.64 \scriptstyle \pm 0.164$ % Reacher
& $1.108 \scriptstyle \pm 0.012$ % Credit
& $0.548 \scriptstyle \pm 0.003$ % Cancer
& $0.075 \scriptstyle \pm 0.041$ % GMM
& $0.197 \scriptstyle \pm 0.072$ % STMMe
& $0.392 \scriptstyle \pm 0.06$ % BMM
& $0.017 \scriptstyle \pm 0.011$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.589 \scriptstyle \pm 0.011$ % Reacher
& $0.838 \scriptstyle \pm 0.174$ % Credit
& $0.398 \scriptstyle \pm 0.064$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % GMM
& $0.146 \scriptstyle \pm 0.08$ % STMMre
& $0.357 \scriptstyle \pm 0.022$ % BMM
& $0.017 \scriptstyle \pm 0.013$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.629 \scriptstyle \pm 0.037$ % Reacher
& $0.702 \scriptstyle \pm 0.145$ % Credit
& $0.083 \scriptstyle \pm 0.009$ % Cancer
& $0.022 \scriptstyle \pm 0.002$ % GMM
& $0.059 \scriptstyle \pm 0.01$ % STMM
& $0.331 \scriptstyle \pm 0.015$ % BMM
& $0.005 \scriptstyle \pm 0.001$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SNF
% & $0.000 \scriptstyle{\pm 0.000}$ % Funnel
% & $0.000 \scriptstyle{\pm 0.000}$ % Reacher
% & $0.000 \scriptstyle{\pm 0.000}$ % Credit
% & $0.000 \scriptstyle{\pm 0.000}$ % Cancer
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FAB
% & $0.000 \scriptstyle{\pm 0.000}$ % Funnel
% & $0.000 \scriptstyle{\pm 0.000}$ % Reacher
% & $0.000 \scriptstyle{\pm 0.000}$ % Credit
% & $0.000 \scriptstyle{\pm 0.000}$ % Cancer
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DDS
% & $0.000 \scriptstyle{\pm 0.000}$ % Funnel
% & $0.000 \scriptstyle{\pm 0.000}$ % Reacher
% & $0.000 \scriptstyle{\pm 0.000}$ % Credit
% & $0.000 \scriptstyle{\pm 0.000}$ % Cancer
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
PIS
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.159 \scriptstyle \pm 0.001$ % Reacher
& $0.195 \scriptstyle \pm 0.001$ % Credit
& $0.439 \scriptstyle \pm 0.005$ % Cancer
& $0.137 \scriptstyle \pm 0.0$ % GMM
& $0.133 \scriptstyle \pm 0.0$ % STMM
& $0.000 \scriptstyle{\pm 0.000}$ % BMM
& $0.000 \scriptstyle{\pm 0.000}$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Reacher
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % GMM
& $0.007 \scriptstyle \pm 0.002$ % STMM
& $0.000 \scriptstyle{\pm 0.000}$ % BMM
& $0.000 \scriptstyle{\pm 0.000}$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Reacher
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.004 \scriptstyle \pm 0.0$ % GMM
& $0.012 \scriptstyle \pm 0.002$ % STMM
& $0.000 \scriptstyle{\pm 0.000}$ % BMM
& $0.009 \scriptstyle \pm 0.005$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Reacher
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.02 \scriptstyle \pm 0.006$ % GMM
& $0.007 \scriptstyle \pm 0.002$ % STMM
& $0.000 \scriptstyle{\pm 0.000}$ % BMM
& $0.039 \scriptstyle \pm 0.013$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\caption{Maybe we don't put these figures here but just put the plots in here, showing that these metrics are not really reliable.}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> results/tables/mog_mos_kl.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{minipage}{\textwidth}
\begin{table*}[t!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\toprule
   & \multicolumn{6}{c}{\textbf{MoG}} & \multicolumn{6}{c}{\textbf{MoS}}   \\ 
   & \multicolumn{3}{c}{\textbf{ELBO} $\uparrow$} & \multicolumn{3}{c}{\textbf{EUBO} $\downarrow$}   
   & \multicolumn{3}{c}{\textbf{ELBO} $\uparrow$} & \multicolumn{3}{c}{\textbf{EUBO} $\downarrow$}
   \\ 
\textbf{Method}   
& $d=2$ & $d=50$  & $d=200$ & $d=2$ & $d=50$  & $d=200$
& $d=2$ & $d=50$  & $d=200$ & $d=2$ & $d=50$  & $d=200$
\\ 
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
 % & \multicolumn{6}{c}{\textbf{MoG}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $-3.011 \scriptstyle \pm 0.002$
& $-3.69 \scriptstyle \pm 0.0$
& $-3.695 \scriptstyle \pm 0.001$
& $3.089 \scriptstyle \pm 0.0$
& $164.114 \scriptstyle \pm 0.0$
& $666.954 \scriptstyle \pm 0.0$
& $-1.038 \scriptstyle \pm 0.007$
& $-5.957 \scriptstyle \pm 0.007$
& $-16.969 \scriptstyle \pm 0.011$
& $1.218 \scriptstyle \pm 0.001$
& $72.663 \scriptstyle \pm 0.005$
& $324.202 \scriptstyle \pm 0.044$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $-0.045 \scriptstyle \pm 0.011$
& $-1.715 \scriptstyle \pm 0.119$
& $-1.709 \scriptstyle \pm 0.058$
& $3.619 \scriptstyle \pm 1.308$
& $240.459 \scriptstyle \pm 51.135$
& $645.405 \scriptstyle \pm 6.309$
& $-0.001 \scriptstyle \pm 0.0$
& $-3.89 \scriptstyle \pm 0.122$
& $-15.649 \scriptstyle \pm 0.173$
& $0.002 \scriptstyle \pm 0.001$
& $57.746 \scriptstyle \pm 1.928$
& $268.513 \scriptstyle \pm 17.652$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $-2.095 \scriptstyle \pm 0.009$
& $-877.034 \scriptstyle \pm 10.231$
& $-6816.697 \scriptstyle \pm 44.195$
& $2.734 \scriptstyle \pm 0.0$
& $161.921 \scriptstyle \pm 0.0$
& $662.404 \scriptstyle \pm 0.0$
& $-0.01 \scriptstyle \pm 0.016$
& $-4.634 \scriptstyle \pm 1.088$
& $-52.535 \scriptstyle \pm 7.564$
& $1.272 \scriptstyle \pm 0.0$
& $81.325 \scriptstyle \pm 0.0$
& $340.984 \scriptstyle \pm 0.0$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $-1.778 \scriptstyle \pm 0.09$
& $-927.16 \scriptstyle \pm 103.812$
& $-6053.823 \scriptstyle \pm 260.996$
& $1.248 \scriptstyle \pm 0.045$
& $117.63 \scriptstyle \pm 22.161$
& $439.434 \scriptstyle \pm 16.788$
& $-0.041 \scriptstyle \pm 0.031$
& $-4.923 \scriptstyle \pm 1.546$
& $-50.328 \scriptstyle \pm 6.627$
& $0.67 \scriptstyle \pm 0.1$
& $207.625 \scriptstyle \pm 24.148$
& $12801.561 \scriptstyle \pm 2892.674$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $-0.666 \scriptstyle \pm 0.026$
& $-451.399 \scriptstyle \pm 7.561$
& $-2836.471 \scriptstyle \pm 57.695$
& $0.976 \scriptstyle \pm 0.007$
& $103.674 \scriptstyle \pm 0.069$
& $425.5 \scriptstyle \pm 0.707$
& $-0.002 \scriptstyle \pm 0.002$
& $-0.339 \scriptstyle \pm 0.18$
& $-22.687 \scriptstyle \pm 0.358$
& $0.346 \scriptstyle \pm 0.013$
& $212.21 \scriptstyle \pm 6.16$
& $12553.883 \scriptstyle \pm 645.758$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $-19.932 \scriptstyle \pm 12.805$
& $-299.916 \scriptstyle \pm 253.455$
& $-63.212 \scriptstyle \pm 56.191$
& $0.865 \scriptstyle \pm 0.113$
& $93.56 \scriptstyle \pm 5.086$
& $386.884 \scriptstyle \pm 12.161$
& $-0.257 \scriptstyle \pm 0.075$
& $75.735 \scriptstyle \pm 175.894$
& $-98.558 \scriptstyle \pm 7.688$
& $0.162 \scriptstyle \pm 0.055$
& $18.088 \scriptstyle \pm 2.503$
& $227.514 \scriptstyle \pm 0.32$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $-0.651 \scriptstyle \pm 0.014$
& $-185.021 \scriptstyle \pm 0.743$
& $-4017.832 \scriptstyle \pm 20.356$
& $0.652 \scriptstyle \pm 0.008$
& $43.67 \scriptstyle \pm 0.457$
& $358.687 \scriptstyle \pm 2.112$
& $-1.215 \scriptstyle \pm 0.005$
& $-69.358 \scriptstyle \pm 0.633$
& $-308.728 \scriptstyle \pm 0.45$
& $0.734 \scriptstyle \pm 0.002$
& $47.834 \scriptstyle \pm 0.82$
& $208.626 \scriptstyle \pm 0.525$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $-0.986 \scriptstyle \pm 0.136$
& $-29.034 \scriptstyle \pm 0.591$
& $-956.576 \scriptstyle \pm 6.27$
& $1.072 \scriptstyle \pm 0.242$
& $51.137 \scriptstyle \pm 0.177$
& $375.527 \scriptstyle \pm 3.11$
& $-0.311 \scriptstyle \pm 0.034$
& $-28.471 \scriptstyle \pm 1.018$
& $-173.716 \scriptstyle \pm 2.629$
& $0.198 \scriptstyle \pm 0.008$
& $20.887 \scriptstyle \pm 1.042$
& $132.711 \scriptstyle \pm 1.817$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
PIS
& $-0.585 \scriptstyle \pm 0.016$
& $-16.881 \scriptstyle \pm 0.026$
& $-65.7 \scriptstyle \pm 0.201$
& $7.344 \scriptstyle \pm 0.004$
& $3626.12 \scriptstyle \pm 1.36$
& $16979.347 \scriptstyle \pm 4.47$
& $-0.387 \scriptstyle \pm 0.009$
& $-29.261 \scriptstyle \pm 1.743$
& $-306.678 \scriptstyle \pm 0.548$
& $1.868 \scriptstyle \pm 0.0$
& $88.192 \scriptstyle \pm 0.005$
& $363.435 \scriptstyle \pm 0.03$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DIS
& $-1.85 \scriptstyle \pm 0.359$
& $-181.348 \scriptstyle \pm 15.47$
& $-14142.693 \scriptstyle \pm 17807.605$
& $6.653 \scriptstyle \pm 0.357$
& $546.335 \scriptstyle \pm 30.861$
& $15792.004 \scriptstyle \pm 18966.782$
& $-0.157 \scriptstyle \pm 0.023$
& $-36.704 \scriptstyle \pm 0.629$
& $-819.959 \scriptstyle \pm 6.264$
& $4.778 \scriptstyle \pm 0.038$
& $193.27 \scriptstyle \pm 3.293$
& $658.575 \scriptstyle \pm 7.82$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $-0.527 \scriptstyle \pm 0.022$
& $-13.284 \scriptstyle \pm 0.46$
& $-60.642 \scriptstyle \pm 2.333$
& $4.176 \scriptstyle \pm 0.0$
& $291.867 \scriptstyle \pm 0.047$
& $1224.926 \scriptstyle \pm 2.485$
& $-0.11 \scriptstyle \pm 0.007$
& $-31.681 \scriptstyle \pm 0.363$
& $-244.188 \scriptstyle \pm 3.504$
& $1.783 \scriptstyle \pm 0.0$
& $86.014 \scriptstyle \pm 0.001$
& $351.204 \scriptstyle \pm 0.005$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GBS
& $-0.473 \scriptstyle \pm 0.061$
& $-35.771 \scriptstyle \pm 1.105$
& $-161.259 \scriptstyle \pm 20.704$
& $0.485 \scriptstyle \pm 0.047$
& $67.819 \scriptstyle \pm 2.157$
& $204.498 \scriptstyle \pm 48.539$
& $-0.064 \scriptstyle \pm 0.004$
& $-99.369 \scriptstyle \pm 0.158$
& $-258.263 \scriptstyle \pm 2.639$
& $0.064 \scriptstyle \pm 0.004$
& $73.545 \scriptstyle \pm 0.107$
& $147.412 \scriptstyle \pm 1.504$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\caption{Mean and standard deviation of ELBO and EUBO values for MoG and MoS for varying dimensions $d$. various target densities. Best results are highlighted in bold. N/A indicates that reasonable results could not be obtained due to numerical problems. }
\label{tab:dim}
\end{table*}

% \end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> results/tables/mog_mos_logZ.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{minipage}{\textwidth}
\begin{table*}[t!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\toprule
   & \multicolumn{6}{c}{\textbf{MoG}} & \multicolumn{6}{c}{\textbf{MoS}}   \\ 
   & \multicolumn{3}{c}{$\mathbf{\Delta \log Z}_{r} \downarrow$} & \multicolumn{3}{c}{$\mathbf{\Delta \log Z}_{f} \downarrow$}   
   & \multicolumn{3}{c}{$\mathbf{\Delta \log Z}_{r} \downarrow$} & \multicolumn{3}{c}{$\mathbf{\Delta \log Z}_{f} \downarrow$}
   \\ 
\textbf{Method}   
& $d=2$ & $d=50$  & $d=200$ & $d=2$ & $d=50$  & $d=200$
& $d=2$ & $d=50$  & $d=200$ & $d=2$ & $d=50$  & $d=200$
\\ 
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
 % & \multicolumn{6}{c}{\textbf{MoG}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $0.084 \scriptstyle \pm 0.066$
& $3.658 \scriptstyle \pm 0.04$
& $3.676 \scriptstyle \pm 0.013$
& $0.15 \scriptstyle \pm 0.002$
& $0.185 \scriptstyle \pm 0.002$
& $0.176 \scriptstyle \pm 0.005$
& $0.018 \scriptstyle \pm 0.003$
& $3.009 \scriptstyle \pm 0.291$
& $8.048 \scriptstyle \pm 0.758$
& $0.114 \scriptstyle \pm 0.0$
& $0.048 \scriptstyle \pm 0.002$
& $5.982 \scriptstyle \pm 0.019$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $0.044 \scriptstyle \pm 0.011$
& $1.715 \scriptstyle \pm 0.119$
& $1.709 \scriptstyle \pm 0.058$
& $0.003 \scriptstyle \pm 0.002$
& $0.048 \scriptstyle \pm 0.007$
& $0.028 \scriptstyle \pm 0.027$
& $0.0 \scriptstyle \pm 0.0$
& $1.282 \scriptstyle \pm 0.221$
& $7.126 \scriptstyle \pm 0.377$
& $0.0 \scriptstyle \pm 0.0$
& $0.084 \scriptstyle \pm 0.055$
& $5.708 \scriptstyle \pm 0.478$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $0.069 \scriptstyle \pm 0.01$
& $690.721 \scriptstyle \pm 11.215$
& $6326.621 \scriptstyle \pm 51.428$
& $2.728 \scriptstyle \pm 0.0$
& $161.796 \scriptstyle \pm 0.0$
& $661.945 \scriptstyle \pm 0.0$
& $0.016 \scriptstyle \pm 0.009$
& $3.88 \scriptstyle \pm 1.105$
& $49.846 \scriptstyle \pm 7.638$
& $1.262 \scriptstyle \pm 0.0$
& $80.992 \scriptstyle \pm 0.0$
& $338.745 \scriptstyle \pm 0.0$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $0.023 \scriptstyle \pm 0.015$
& $765.624 \scriptstyle \pm 108.027$
& $5567.272 \scriptstyle \pm 277.527$
& $1.157 \scriptstyle \pm 0.038$
& $110.955 \scriptstyle \pm 18.372$
& $420.932 \scriptstyle \pm 12.987$
& $0.024 \scriptstyle \pm 0.014$
& $4.081 \scriptstyle \pm 1.579$
& $47.121 \scriptstyle \pm 6.693$
& $0.639 \scriptstyle \pm 0.095$
& $205.297 \scriptstyle \pm 23.918$
& $12765.117 \scriptstyle \pm 2877.898$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $0.008 \scriptstyle \pm 0.001$
& $337.094 \scriptstyle \pm 9.296$
& $2504.363 \scriptstyle \pm 64.97$
& $0.901 \scriptstyle \pm 0.007$
& $100.987 \scriptstyle \pm 0.065$
& $415.277 \scriptstyle \pm 0.455$
& $0.004 \scriptstyle \pm 0.001$
& $0.822 \scriptstyle \pm 0.087$
& $19.738 \scriptstyle \pm 0.342$
& $0.333 \scriptstyle \pm 0.013$
& $210.245 \scriptstyle \pm 6.098$
& $12516.502 \scriptstyle \pm 631.899$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $0.007 \scriptstyle \pm 0.003$
& $2.952 \scriptstyle \pm 0.247$
& $3.331 \scriptstyle \pm 0.229$
& $1.193 \scriptstyle \pm 0.125$
& $126.363 \scriptstyle \pm 1.789$
& $545.226 \scriptstyle \pm 5.62$
& $0.005 \scriptstyle \pm 0.001$
& $3.358 \scriptstyle \pm 1.062$
& $43.419 \scriptstyle \pm 4.69$
& $0.268 \scriptstyle \pm 0.093$
& $84.592 \scriptstyle \pm 22.649$
& $13514.417 \scriptstyle \pm 101.955$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $0.01 \scriptstyle \pm 0.002$
& $31.319 \scriptstyle \pm 1.793$
& $2354.02 \scriptstyle \pm 60.855$
& $0.009 \scriptstyle \pm 0.005$
& $21.148 \scriptstyle \pm 1.478$
& $305.656 \scriptstyle \pm 2.662$
& $0.01 \scriptstyle \pm 0.002$
& $28.607 \scriptstyle \pm 1.275$
& $210.536 \scriptstyle \pm 1.393$
& $0.068 \scriptstyle \pm 0.01$
& $24.757 \scriptstyle \pm 0.841$
& $147.321 \scriptstyle \pm 1.272$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $0.038 \scriptstyle \pm 0.015$
& $8.159 \scriptstyle \pm 0.775$
& $647.953 \scriptstyle \pm 7.212$
& $0.031 \scriptstyle \pm 0.008$
& $15.477 \scriptstyle \pm 0.815$
& $282.699 \scriptstyle \pm 4.105$
& $0.004 \scriptstyle \pm 0.001$
& $4.36 \scriptstyle \pm 0.741$
& $103.224 \scriptstyle \pm 2.118$
& $0.017 \scriptstyle \pm 0.003$
& $5.472 \scriptstyle \pm 0.938$
& $83.029 \scriptstyle \pm 0.819$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $0.026 \scriptstyle \pm 0.011$
& $51.218 \scriptstyle \pm 2.809$
& $306.127 \scriptstyle \pm 24.673$
& $0.03 \scriptstyle \pm 0.008$
& $79.227 \scriptstyle \pm 3.758$
& $440.341 \scriptstyle \pm 4.252$
& $0.004 \scriptstyle \pm 0.001$
& $10.533 \scriptstyle \pm 0.404$
& $167.654 \scriptstyle \pm 1.564$
& $0.005 \scriptstyle \pm 0.002$
& $12.835 \scriptstyle \pm 0.275$
& $148.676 \scriptstyle \pm 2.851$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
PIS
& $0.267 \scriptstyle \pm 0.006$
& $7.122 \scriptstyle \pm 0.63$
& $40.699 \scriptstyle \pm 0.543$
& $0.094 \scriptstyle \pm 0.038$
& $3113.492 \scriptstyle \pm 1.978$
& $16071.743 \scriptstyle \pm 3.046$
& $0.275 \scriptstyle \pm 0.016$
& $12.248 \scriptstyle \pm 0.326$
& $209.981 \scriptstyle \pm 2.573$
& $0.342 \scriptstyle \pm 0.001$
& $54.09 \scriptstyle \pm 0.151$
& $304.178 \scriptstyle \pm 0.329$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DIS
& $0.058 \scriptstyle \pm 0.03$
& $87.709 \scriptstyle \pm 8.942$
& $11646.394 \scriptstyle \pm 15938.051$
& $1.39 \scriptstyle \pm 0.458$
& $369.352 \scriptstyle \pm 16.293$
& $14376.906 \scriptstyle \pm 17877.127$
& $0.049 \scriptstyle \pm 0.005$
& $10.448 \scriptstyle \pm 0.607$
& $658.634 \scriptstyle \pm 4.952$
& $3.212 \scriptstyle \pm 0.028$
& $87.897 \scriptstyle \pm 5.255$
& $433.741 \scriptstyle \pm 10.78$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $0.012 \scriptstyle \pm 0.005$
& $1.739 \scriptstyle \pm 0.442$
& $27.506 \scriptstyle \pm 2.584$
& $1.698 \scriptstyle \pm 0.029$
& $207.545 \scriptstyle \pm 1.163$
& $1052.805 \scriptstyle \pm 1.732$
& $0.005 \scriptstyle \pm 0.001$
& $7.952 \scriptstyle \pm 0.299$
& $155.502 \scriptstyle \pm 3.594$
& $0.315 \scriptstyle \pm 0.0$
& $53.411 \scriptstyle \pm 0.024$
& $291.566 \scriptstyle \pm 0.102$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GBS
& $0.007 \scriptstyle \pm 0.001$
& $8.103 \scriptstyle \pm 1.696$
& $87.971 \scriptstyle \pm 14.656$
& $0.008 \scriptstyle \pm 0.001$
& $9.321 \scriptstyle \pm 0.776$
& $72.634 \scriptstyle \pm 12.301$
& $0.002 \scriptstyle \pm 0.0$
& $53.767 \scriptstyle \pm 0.732$
& $157.791 \scriptstyle \pm 2.947$
& $0.01 \scriptstyle \pm 0.002$
& $47.441 \scriptstyle \pm 0.098$
& $101.874 \scriptstyle \pm 2.214$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\caption{Mean and standard deviation of ELBO and EUBO values for MoG and MoS for varying dimensions $d$. various target densities. Best results are highlighted in bold. N/A indicates that reasonable results could not be obtained due to numerical problems. }
\label{tab:dim}
\end{table*}

% \end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> results/tables/mog_nice_table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{minipage}[b]{0.5\textwidth}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccccccc}
\toprule
& $\mathbf{\Delta \log Z}_{\model} \downarrow$ & \textbf{ELBO} $\uparrow$ & \textbf{EUBO} $\downarrow$& \textbf{EMC}  $\uparrow$& \textbf{MMD} $\downarrow$& $\textbf{WD}\, \downarrow$ \\ 
\midrule
%  & \multicolumn{6}{c}{\textbf{MoG}} \\
% \midrule
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MFVI
% & $0.096 \scriptstyle \pm 0.061$ % log Z
% & $-3.01 \scriptstyle \pm 0.004$ % ELBO
% & $168.026 \scriptstyle \pm 1.489$ % EUBO
% & $0.382 \scriptstyle \pm 0.003$ % EMC
% & $0.082 \scriptstyle \pm 0.001$ % MMD
% & $413.194 \scriptstyle \pm 9.042$ % Wasserstein
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% GMMVI
% & $\mathbf{0.0 \scriptstyle \pm 0.0}$ % log Z
% & $\mathbf{-0.002 \scriptstyle \pm 0.002}$ % ELBO
% & $\mathbf{0.004 \scriptstyle \pm 0.003}$ % EUBO
% & $\mathbf{0.997 \scriptstyle \pm 0.0}$ % EMC
% & $\mathbf{0.0 \scriptstyle \pm 0.0}$ % MMD
% & $\mathbf{5.728 \scriptstyle \pm 0.72}$ % Wasserstein
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % NFVI
% % & $0.0 \scriptstyle \pm 0.0$ % log Z
% % & $0.0 \scriptstyle \pm 0.0$ % ELBO
% % & $0.0 \scriptstyle \pm 0.0$ % EUBO
% % & $0.0 \scriptstyle \pm 0.0$ % EMC
% % & $0.0 \scriptstyle \pm 0.0$ % MMD
% % & $0.0 \scriptstyle \pm 0.0$ % Wasserstein
% % \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SMC
% & $0.064 \scriptstyle \pm 0.032$ % log Z
% & $-9.09 \scriptstyle \pm 0.033$ % ELBO
% & $1.663 \scriptstyle \pm 0.137$ % EUBO
% & $0.963 \scriptstyle \pm 0.004$ % EMC
% & $0.005 \scriptstyle \pm 0.001$ % MMD
% & $90.995 \scriptstyle \pm 11.649$ % Wasserstein
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AFT
% & $0.232 \scriptstyle \pm 0.293$ % log Z
% & $-3.046 \scriptstyle \pm 0.439$ % ELBO
% & $2.744 \scriptstyle \pm 1.373$ % EUBO
% & $0.849 \scriptstyle \pm 0.082$ % EMC
% & $0.008 \scriptstyle \pm 0.01$ % MMD
% & $131.354 \scriptstyle \pm 58.859$ % Wasserstein
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CRAFT
% & $0.012 \scriptstyle \pm 0.004$ % log Z
% & $-3.527 \scriptstyle \pm 0.063$ % ELBO
% & $2.05 \scriptstyle \pm 0.029$ % EUBO
% & $0.986 \scriptstyle \pm 0.002$ % EMC
% & $\mathbf{0.0 \scriptstyle \pm 0.0}$ % MMD
% & $16.879 \scriptstyle \pm 1.225$ % Wasserstein
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % SNF
% % & $0.0 \scriptstyle \pm 0.0$ % log Z
% % & $0.0 \scriptstyle \pm 0.0$ % ELBO
% % & $0.0 \scriptstyle \pm 0.0$ % EUBO
% % & $0.0 \scriptstyle \pm 0.0$ % EMC
% % & $0.0 \scriptstyle \pm 0.0$ % MMD
% % & $0.0 \scriptstyle \pm 0.0$ % Wasserstein
% % \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FAB
% & $0.011 \scriptstyle \pm 0.002$ % log Z
% & $-6.463 \scriptstyle \pm 1.113$ % ELBO
% & $1.072 \scriptstyle \pm 0.071$ % EUBO
% & $\mathbf{0.99 \scriptstyle \pm 0.002}$ % EMC
% & $\mathbf{0.0 \scriptstyle \pm 0.0}$ % MMD
% & $13.806 \scriptstyle \pm 3.765$ % Wasserstein
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DDS
% & $0.016 \scriptstyle \pm 0.004$ % log Z
% & $-0.731 \scriptstyle \pm 0.021$ % ELBO
% & $9.714 \scriptstyle \pm 0.211$ % EUBO
% & $0.978 \scriptstyle \pm 0.002$ % EMC
% & $\mathbf{0.002 \scriptstyle \pm 0.0}$ % MMD
% & $48.52 \scriptstyle \pm 6.74$ % Wasserstein
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MCD
% & $0.029 \scriptstyle \pm 0.009$ % log Z
% & $-2.678 \scriptstyle \pm 0.166$ % ELBO
% & $2.136 \scriptstyle \pm 0.062$ % EUBO
% & $0.799 \scriptstyle \pm 0.002$ % EMC
% & $0.031 \scriptstyle \pm 0.0$ % MMD
% & $341.736 \scriptstyle \pm 6.102$ % Wasserstein
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LDVI
% & $0.103 \scriptstyle \pm 0.044$ % log Z
% & $-3.84 \scriptstyle \pm 0.236$ % ELBO
% & $26.539 \scriptstyle \pm 9.463$ % EUBO
% & $0.893 \scriptstyle \pm 0.014$ % EMC
% & $0.014 \scriptstyle \pm 0.001$ % MMD
% & $189.372 \scriptstyle \pm 13.956$ % Wasserstein
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CMCD
% & $0.091 \scriptstyle \pm 0.088$ % log Z
% & $-3.821 \scriptstyle \pm 0.341$ % ELBO
% & $53.192 \scriptstyle \pm 14.543$ % EUBO
% & $0.139 \scriptstyle \pm 0.138$ % EMC
% & $0.1 \scriptstyle \pm 0.002$ % MMD
% & $642.48 \scriptstyle \pm 86.812$ % Wasserstein
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \midrule
%  & \multicolumn{6}{c}{\textbf{NICE}} \\
% \midrule

MFVI
& $7.126 \scriptstyle \pm 0.44$ % log Z
& $-14.22 \scriptstyle \pm 0.009$ % ELBO
& $543.178 \scriptstyle \pm 0.669$ % EUBO
& $0.0 \scriptstyle \pm 0.0$ % EMC
& $0.109 \scriptstyle \pm 0.0$ % MMD
& $253.098 \scriptstyle \pm 0.124$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $3.82 \scriptstyle \pm 0.245$ % log Z
& $-8.187 \scriptstyle \pm 0.152$ % ELBO
& $126.564 \scriptstyle \pm 11.214$ % EUBO
& $0.193 \scriptstyle \pm 0.027$ % EMC
& $0.142 \scriptstyle \pm 0.012$ % MMD
& $215.645 \scriptstyle \pm 3.612$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NFVI
% & $0.0 \scriptstyle \pm 0.0$ % log Z
% & $0.0 \scriptstyle \pm 0.0$ % ELBO
% & $0.0 \scriptstyle \pm 0.0$ % EUBO
% & $0.0 \scriptstyle \pm 0.0$ % EMC
% & $0.0 \scriptstyle \pm 0.0$ % MMD
% & $0.0 \scriptstyle \pm 0.0$ % Wasserstein
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $82.824 \scriptstyle \pm 2.518$ % log Z
& $-163.719 \scriptstyle \pm 1.859$ % ELBO
& $133.069 \scriptstyle \pm 0.698$ % EUBO
& $0.905 \scriptstyle \pm 0.075$ % EMC
& $0.013 \scriptstyle \pm 0.009$ % MMD
& $145.63 \scriptstyle \pm 8.278$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $31.137 \scriptstyle \pm 8.967$ % log Z
& $-68.748 \scriptstyle \pm 8.73$ % ELBO
& $199.117 \scriptstyle \pm 3.399$ % EUBO
& $0.772 \scriptstyle \pm 0.131$ % EMC
& $0.045 \scriptstyle \pm 0.032$ % MMD
& $201.695 \scriptstyle \pm 25.397$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $1.125 \scriptstyle \pm 0.196$ % log Z
& $-9.21 \scriptstyle \pm 0.414$ % ELBO
& $\mathbf{104.176 \scriptstyle \pm 9.294}$ % EUBO
& $0.828 \scriptstyle \pm 0.11$ % EMC
& $\mathbf{0.007 \scriptstyle \pm 0.002}$ % MMD
& $\mathbf{133.749 \scriptstyle \pm 4.144}$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SNF
% & $0.0 \scriptstyle \pm 0.0$ % log Z
% & $0.0 \scriptstyle \pm 0.0$ % ELBO
% & $0.0 \scriptstyle \pm 0.0$ % EUBO
% & $0.0 \scriptstyle \pm 0.0$ % EMC
% & $0.0 \scriptstyle \pm 0.0$ % MMD
% & $0.0 \scriptstyle \pm 0.0$ % Wasserstein
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $\mathbf{0.715 \scriptstyle \pm 0.122}$ % log Z
& $\mathbf{-5.425 \scriptstyle \pm 0.158}$ % ELBO
& N/A % EUBO
& $0.876 \scriptstyle \pm 0.008$ % EMC
& $0.038 \scriptstyle \pm 0.006$ % MMD
& $142.666 \scriptstyle \pm 2.717$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $67.036 \scriptstyle \pm 3.045$ % log Z
& $-133.24 \scriptstyle \pm 0.874$ % ELBO
& $1128.436 \scriptstyle \pm 13.726$ % EUBO
& $0.872 \scriptstyle \pm 0.003$ % EMC
& $0.033 \scriptstyle \pm 0.0$ % MMD
& $185.319 \scriptstyle \pm 0.992$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $459.611 \scriptstyle \pm 21.631$ % log Z
& $-1054.014 \scriptstyle \pm 24.39$ % ELBO
& $741.752 \scriptstyle \pm 20.284$ % EUBO
& $\mathbf{0.923 \scriptstyle \pm 0.003}$ % EMC
& $0.036 \scriptstyle \pm 0.001$ % MMD
& $186.404 \scriptstyle \pm 1.356$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LDVI
% & $nan \scriptstyle \pm nan$ % log Z
% & $-635.519 \scriptstyle \pm 213.559$ % ELBO
% & $nan \scriptstyle \pm nan$ % EUBO
% & $nan \scriptstyle \pm nan$ % EMC
% & $nan \scriptstyle \pm nan$ % MMD
% & $nan \scriptstyle \pm nan$ % Wasserstein
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $10.64 \scriptstyle \pm 0.597$ % log Z
& $-30.6 \scriptstyle \pm 0.186$ % ELBO
& $270.394 \scriptstyle \pm 14.047$ % EUBO
& $0.099 \scriptstyle \pm 0.005$ % EMC
& $0.087 \scriptstyle \pm 0.001$ % MMD
& $219.448 \scriptstyle \pm 0.648$ % Wasserstein
\\

\bottomrule
\end{tabular}
}
\captionof{table}{\red{We were not able to obtain reasonable results for PIS and SNF LDVI.}A table beside a figure}
\label{tab:nice}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> results/tables/mog_results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}{\textwidth}
\begin{minipage}[b]{0.4\textwidth}
\centering
 \resizebox{\textwidth}{!}{%
\begin{tabular}{cccc}
\includegraphics[width=0.32\textwidth]{figures/visualizations/gmm40/pdfs/mfvi.pdf} &   
\includegraphics[width=0.32\textwidth]{figures/visualizations/gmm40/pdfs/gmmvi.pdf} &   
\includegraphics[width=0.32\textwidth]{figures/visualizations/gmm40/pdfs/gmm40.pdf} &    
\\
\includegraphics[width=0.32\textwidth]{figures/visualizations/gmm40/pdfs/fab.pdf} &   
\includegraphics[width=0.32\textwidth]{figures/visualizations/gmm40/pdfs/dds.pdf} &   
\includegraphics[width=0.32\textwidth]{figures/visualizations/gmm40/pdfs/pis.pdf} &   
\\
\end{tabular}
}
\captionof{figure}{A table beside a figure}
\end{minipage}
\hfill
\begin{minipage}[b]{0.6\textwidth}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccccccc}
\toprule
& $\Delta \log Z \downarrow$ & ELBO $\uparrow$ & EUBO $\downarrow$& EMC  $\uparrow$& MMD $\downarrow$& $\mathcal{W}_2\, \downarrow$ \\ 
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $0.096 \scriptstyle \pm 0.061$ % log Z
& $-3.01 \scriptstyle \pm 0.004$ % ELBO
& $168.026 \scriptstyle \pm 1.489$ % EUBO
& $0.382 \scriptstyle \pm 0.003$ % EMC
& $0.082 \scriptstyle \pm 0.001$ % MMD
& $413.194 \scriptstyle \pm 9.042$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $\mathbf{0.0 \scriptstyle \pm 0.0}$ % log Z
& $\mathbf{-0.002 \scriptstyle \pm 0.002}$ % ELBO
& $\mathbf{0.004 \scriptstyle \pm 0.003}$ % EUBO
& $\mathbf{0.997 \scriptstyle \pm 0.0}$ % EMC
& $\mathbf{0.0 \scriptstyle \pm 0.0}$ % MMD
& $\mathbf{5.728 \scriptstyle \pm 0.72}$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NFVI
% & $0.0 \scriptstyle \pm 0.0$ % log Z
% & $0.0 \scriptstyle \pm 0.0$ % ELBO
% & $0.0 \scriptstyle \pm 0.0$ % EUBO
% & $0.0 \scriptstyle \pm 0.0$ % EMC
% & $0.0 \scriptstyle \pm 0.0$ % MMD
% & $0.0 \scriptstyle \pm 0.0$ % Wasserstein
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $0.064 \scriptstyle \pm 0.032$ % log Z
& $-9.09 \scriptstyle \pm 0.033$ % ELBO
& $1.663 \scriptstyle \pm 0.137$ % EUBO
& $0.963 \scriptstyle \pm 0.004$ % EMC
& $0.005 \scriptstyle \pm 0.001$ % MMD
& $90.995 \scriptstyle \pm 11.649$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $0.232 \scriptstyle \pm 0.293$ % log Z
& $-3.046 \scriptstyle \pm 0.439$ % ELBO
& $2.744 \scriptstyle \pm 1.373$ % EUBO
& $0.849 \scriptstyle \pm 0.082$ % EMC
& $0.008 \scriptstyle \pm 0.01$ % MMD
& $131.354 \scriptstyle \pm 58.859$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $0.012 \scriptstyle \pm 0.004$ % log Z
& $-3.527 \scriptstyle \pm 0.063$ % ELBO
& $2.05 \scriptstyle \pm 0.029$ % EUBO
& $0.986 \scriptstyle \pm 0.002$ % EMC
& $\mathbf{0.0 \scriptstyle \pm 0.0}$ % MMD
& $16.879 \scriptstyle \pm 1.225$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SNF
% & $0.0 \scriptstyle \pm 0.0$ % log Z
% & $0.0 \scriptstyle \pm 0.0$ % ELBO
% & $0.0 \scriptstyle \pm 0.0$ % EUBO
% & $0.0 \scriptstyle \pm 0.0$ % EMC
% & $0.0 \scriptstyle \pm 0.0$ % MMD
% & $0.0 \scriptstyle \pm 0.0$ % Wasserstein
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $0.011 \scriptstyle \pm 0.002$ % log Z
& $-6.463 \scriptstyle \pm 1.113$ % ELBO
& $1.072 \scriptstyle \pm 0.071$ % EUBO
& $\mathbf{0.99 \scriptstyle \pm 0.002}$ % EMC
& $\mathbf{0.0 \scriptstyle \pm 0.0}$ % MMD
& $13.806 \scriptstyle \pm 3.765$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $0.016 \scriptstyle \pm 0.004$ % log Z
& $-0.731 \scriptstyle \pm 0.021$ % ELBO
& $9.714 \scriptstyle \pm 0.211$ % EUBO
& $0.978 \scriptstyle \pm 0.002$ % EMC
& $\mathbf{0.002 \scriptstyle \pm 0.0}$ % MMD
& $48.52 \scriptstyle \pm 6.74$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $0.029 \scriptstyle \pm 0.009$ % log Z
& $-2.678 \scriptstyle \pm 0.166$ % ELBO
& $2.136 \scriptstyle \pm 0.062$ % EUBO
& $0.799 \scriptstyle \pm 0.002$ % EMC
& $0.031 \scriptstyle \pm 0.0$ % MMD
& $341.736 \scriptstyle \pm 6.102$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $0.103 \scriptstyle \pm 0.044$ % log Z
& $-3.84 \scriptstyle \pm 0.236$ % ELBO
& $26.539 \scriptstyle \pm 9.463$ % EUBO
& $0.893 \scriptstyle \pm 0.014$ % EMC
& $0.014 \scriptstyle \pm 0.001$ % MMD
& $189.372 \scriptstyle \pm 13.956$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $0.091 \scriptstyle \pm 0.088$ % log Z
& $-3.821 \scriptstyle \pm 0.341$ % ELBO
& $53.192 \scriptstyle \pm 14.543$ % EUBO
& $0.139 \scriptstyle \pm 0.138$ % EMC
& $0.1 \scriptstyle \pm 0.002$ % MMD
& $642.48 \scriptstyle \pm 86.812$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\captionof{table}{A table beside a figure}
\end{minipage}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> results/tables/nice_emc_table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t!]
% \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cc}
\toprule
& $14 \times 14$ \textbf{Digits}
& $28 \times 28$ \textbf{Fashion}
% \vspace{0.2cm}
\\ 
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $0.0 \scriptstyle \pm 0.0$
& $0.0 \scriptstyle \pm 0.0$
\\
GMMVI
& $0.164 \scriptstyle \pm 0.081$
& $0.217 \scriptstyle \pm 0.167$
\\
SMC
& $0.873 \scriptstyle \pm 0.0$
& $0.0 \scriptstyle \pm 0.0$
\\
AFT
& $0.727 \scriptstyle \pm 0.0$
& $0.011 \scriptstyle \pm 0.0$
\\
CRAFT
& $0.772 \scriptstyle \pm 0.07$
& $0.016 \scriptstyle \pm 0.027$
\\
FAB
& $0.915 \scriptstyle \pm 0.007$
& $0.349 \scriptstyle \pm 0.137$
\\
MCD
& $0.851 \scriptstyle \pm 0.01$
& $0.619 \scriptstyle \pm 0.001$
\\
LDVI
& $0.951 \scriptstyle \pm 0.002$
& $0.608 \scriptstyle \pm 0.005$
\\
PIS
& $0.816 \scriptstyle \pm 0.011$
& $0.62 \scriptstyle \pm 0.004$
\\
DIS
& $0.818 \scriptstyle \pm 0.009$
& $0.612 \scriptstyle \pm 0.008$
\\
DDS
& $0.816 \scriptstyle \pm 0.012$
& $0.621 \scriptstyle \pm 0.008$
\\
GBS
& $0.796 \scriptstyle \pm 0.005$
& $0.621 \scriptstyle \pm 0.006$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
    \caption{ELBO values for various target densities. Best results are highlighted using bold font. N/A indicates that reasonable results could not be obtained due to numerical problems. OOM refers to out-of-memory problems. \red{Mention target samples.}
    }
    \vspace{-0.2cm}
\label{table:elbos}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> results/tables/nice_results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}{\textwidth}
\begin{minipage}[b]{0.39\textwidth}
\centering
 \resizebox{\textwidth}{!}{%
\begin{tabular}{cccc}
\includegraphics[width=0.2\textwidth]{figures/visualizations/nice/nice_mfvi.pdf} &   
\includegraphics[width=0.2\textwidth]{figures/visualizations/nice/nice_gmmvi.pdf} &   
\includegraphics[width=0.2\textwidth]{figures/illustrations/nice.pdf} &   
\\
% \tiny MFVI &   
% \tiny MFVI &   
% \tiny MFVI &   
% \\
\includegraphics[width=0.2\textwidth]{figures/visualizations/nice/nice_smc.pdf} &   
\includegraphics[width=0.2\textwidth]{figures/visualizations/nice/nice_aft.pdf} &   
\includegraphics[width=0.2\textwidth]{figures/visualizations/nice/nice_craft.pdf} &  
\\
% \tiny MFVI &   
% \tiny MFVI &   
% \tiny MFVI & 
% \\
\end{tabular}
}
\captionof{figure}{A table beside a figure}
\end{minipage}
\hfill
\begin{minipage}[b]{0.59\textwidth}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccccccc}
\toprule
& $\Delta \log Z \downarrow$ & ELBO $\uparrow$ & EUBO $\downarrow$& EMC  $\uparrow$& MMD $\downarrow$& $\mathcal{W}_2\, \downarrow$  \\ 
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $7.126 \scriptstyle \pm 0.44$ % log Z
& $-14.22 \scriptstyle \pm 0.009$ % ELBO
& $543.178 \scriptstyle \pm 0.669$ % EUBO
& $0.0 \scriptstyle \pm 0.0$ % EMC
& $0.109 \scriptstyle \pm 0.0$ % MMD
& $253.098 \scriptstyle \pm 0.124$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $3.82 \scriptstyle \pm 0.245$ % log Z
& $-8.187 \scriptstyle \pm 0.152$ % ELBO
& $126.564 \scriptstyle \pm 11.214$ % EUBO
& $0.193 \scriptstyle \pm 0.027$ % EMC
& $0.142 \scriptstyle \pm 0.012$ % MMD
& $215.645 \scriptstyle \pm 3.612$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NFVI
% & $0.0 \scriptstyle \pm 0.0$ % log Z
% & $0.0 \scriptstyle \pm 0.0$ % ELBO
% & $0.0 \scriptstyle \pm 0.0$ % EUBO
% & $0.0 \scriptstyle \pm 0.0$ % EMC
% & $0.0 \scriptstyle \pm 0.0$ % MMD
% & $0.0 \scriptstyle \pm 0.0$ % Wasserstein
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $82.824 \scriptstyle \pm 2.518$ % log Z
& $-163.719 \scriptstyle \pm 1.859$ % ELBO
& $133.069 \scriptstyle \pm 0.698$ % EUBO
& $0.905 \scriptstyle \pm 0.075$ % EMC
& $0.013 \scriptstyle \pm 0.009$ % MMD
& $145.63 \scriptstyle \pm 8.278$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $31.137 \scriptstyle \pm 8.967$ % log Z
& $-68.748 \scriptstyle \pm 8.73$ % ELBO
& $199.117 \scriptstyle \pm 3.399$ % EUBO
& $0.772 \scriptstyle \pm 0.131$ % EMC
& $0.045 \scriptstyle \pm 0.032$ % MMD
& $201.695 \scriptstyle \pm 25.397$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $1.125 \scriptstyle \pm 0.196$ % log Z
& $-9.21 \scriptstyle \pm 0.414$ % ELBO
& $\mathbf{104.176 \scriptstyle \pm 9.294}$ % EUBO
& $0.828 \scriptstyle \pm 0.11$ % EMC
& $\mathbf{0.007 \scriptstyle \pm 0.002}$ % MMD
& $\mathbf{133.749 \scriptstyle \pm 4.144}$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SNF
% & $0.0 \scriptstyle \pm 0.0$ % log Z
% & $0.0 \scriptstyle \pm 0.0$ % ELBO
% & $0.0 \scriptstyle \pm 0.0$ % EUBO
% & $0.0 \scriptstyle \pm 0.0$ % EMC
% & $0.0 \scriptstyle \pm 0.0$ % MMD
% & $0.0 \scriptstyle \pm 0.0$ % Wasserstein
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $\mathbf{0.715 \scriptstyle \pm 0.122}$ % log Z
& $\mathbf{-5.425 \scriptstyle \pm 0.158}$ % ELBO
& $INF$ % EUBO
& $0.876 \scriptstyle \pm 0.008$ % EMC
& $0.038 \scriptstyle \pm 0.006$ % MMD
& $142.666 \scriptstyle \pm 2.717$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $67.036 \scriptstyle \pm 3.045$ % log Z
& $-133.24 \scriptstyle \pm 0.874$ % ELBO
& $1128.436 \scriptstyle \pm 13.726$ % EUBO
& $0.872 \scriptstyle \pm 0.003$ % EMC
& $0.033 \scriptstyle \pm 0.0$ % MMD
& $185.319 \scriptstyle \pm 0.992$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $459.611 \scriptstyle \pm 21.631$ % log Z
& $-1054.014 \scriptstyle \pm 24.39$ % ELBO
& $741.752 \scriptstyle \pm 20.284$ % EUBO
& $\mathbf{0.923 \scriptstyle \pm 0.003}$ % EMC
& $0.036 \scriptstyle \pm 0.001$ % MMD
& $186.404 \scriptstyle \pm 1.356$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $nan \scriptstyle \pm nan$ % log Z
& $-635.519 \scriptstyle \pm 213.559$ % ELBO
& $nan \scriptstyle \pm nan$ % EUBO
& $nan \scriptstyle \pm nan$ % EMC
& $nan \scriptstyle \pm nan$ % MMD
& $nan \scriptstyle \pm nan$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $10.64 \scriptstyle \pm 0.597$ % log Z
& $-30.6 \scriptstyle \pm 0.186$ % ELBO
& $270.394 \scriptstyle \pm 14.047$ % EUBO
& $0.099 \scriptstyle \pm 0.005$ % EMC
& $0.087 \scriptstyle \pm 0.001$ % MMD
& $219.448 \scriptstyle \pm 0.648$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\captionof{table}{A table beside a figure}
\end{minipage}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> results/tables/nice_table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}
% \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
\label{table:vi_results}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cccccccc}
\begin{tabular}{l|ccccccc}
\toprule
    & $\Delta \log Z$ & ELBO & EUBO & EMC  & MMD & $\mathcal{W}_2$ \\ 
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $0.0 \scriptstyle \pm 0.0$ % log Z
& $0.0 \scriptstyle \pm 0.0$ % ELBO
& $0.0 \scriptstyle \pm 0.0$ % EUBO
& $0.0 \scriptstyle \pm 0.0$ % EMC
& $0.0 \scriptstyle \pm 0.0$ % MMD
& $0.0 \scriptstyle \pm 0.0$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $0.0 \scriptstyle \pm 0.0$ % log Z
& $0.0 \scriptstyle \pm 0.0$ % ELBO
& $0.0 \scriptstyle \pm 0.0$ % EUBO
& $0.0 \scriptstyle \pm 0.0$ % EMC
& $0.0 \scriptstyle \pm 0.0$ % MMD
& $0.0 \scriptstyle \pm 0.0$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NFVI
% & $0.0 \scriptstyle \pm 0.0$ % log Z
% & $0.0 \scriptstyle \pm 0.0$ % ELBO
% & $0.0 \scriptstyle \pm 0.0$ % EUBO
% & $0.0 \scriptstyle \pm 0.0$ % EMC
% & $0.0 \scriptstyle \pm 0.0$ % MMD
% & $0.0 \scriptstyle \pm 0.0$ % Wasserstein
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $0.0 \scriptstyle \pm 0.0$ % log Z
& $0.0 \scriptstyle \pm 0.0$ % ELBO
& $0.0 \scriptstyle \pm 0.0$ % EUBO
& $0.0 \scriptstyle \pm 0.0$ % EMC
& $0.0 \scriptstyle \pm 0.0$ % MMD
& $0.0 \scriptstyle \pm 0.0$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $0.0 \scriptstyle \pm 0.0$ % log Z
& $0.0 \scriptstyle \pm 0.0$ % ELBO
& $0.0 \scriptstyle \pm 0.0$ % EUBO
& $0.0 \scriptstyle \pm 0.0$ % EMC
& $0.0 \scriptstyle \pm 0.0$ % MMD
& $0.0 \scriptstyle \pm 0.0$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $0.0 \scriptstyle \pm 0.0$ % log Z
& $0.0 \scriptstyle \pm 0.0$ % ELBO
& $0.0 \scriptstyle \pm 0.0$ % EUBO
& $0.0 \scriptstyle \pm 0.0$ % EMC
& $0.0 \scriptstyle \pm 0.0$ % MMD
& $0.0 \scriptstyle \pm 0.0$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SNF
% & $0.0 \scriptstyle \pm 0.0$ % log Z
% & $0.0 \scriptstyle \pm 0.0$ % ELBO
% & $0.0 \scriptstyle \pm 0.0$ % EUBO
% & $0.0 \scriptstyle \pm 0.0$ % EMC
% & $0.0 \scriptstyle \pm 0.0$ % MMD
% & $0.0 \scriptstyle \pm 0.0$ % Wasserstein
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $0.0 \scriptstyle \pm 0.0$ % log Z
& $0.0 \scriptstyle \pm 0.0$ % ELBO
& $0.0 \scriptstyle \pm 0.0$ % EUBO
& $0.0 \scriptstyle \pm 0.0$ % EMC
& $0.0 \scriptstyle \pm 0.0$ % MMD
& $0.0 \scriptstyle \pm 0.0$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $0.0 \scriptstyle \pm 0.0$ % log Z
& $0.0 \scriptstyle \pm 0.0$ % ELBO
& $0.0 \scriptstyle \pm 0.0$ % EUBO
& $0.0 \scriptstyle \pm 0.0$ % EMC
& $0.0 \scriptstyle \pm 0.0$ % MMD
& $0.0 \scriptstyle \pm 0.0$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $0.0 \scriptstyle \pm 0.0$ % log Z
& $0.0 \scriptstyle \pm 0.0$ % ELBO
& $0.0 \scriptstyle \pm 0.0$ % EUBO
& $0.0 \scriptstyle \pm 0.0$ % EMC
& $0.0 \scriptstyle \pm 0.0$ % MMD
& $0.0 \scriptstyle \pm 0.0$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $0.0 \scriptstyle \pm 0.0$ % log Z
& $0.0 \scriptstyle \pm 0.0$ % ELBO
& $0.0 \scriptstyle \pm 0.0$ % EUBO
& $0.0 \scriptstyle \pm 0.0$ % EMC
& $0.0 \scriptstyle \pm 0.0$ % MMD
& $0.0 \scriptstyle \pm 0.0$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $0.0 \scriptstyle \pm 0.0$ % log Z
& $0.0 \scriptstyle \pm 0.0$ % ELBO
& $0.0 \scriptstyle \pm 0.0$ % EUBO
& $0.0 \scriptstyle \pm 0.0$ % EMC
& $0.0 \scriptstyle \pm 0.0$ % MMD
& $0.0 \scriptstyle \pm 0.0$ % Wasserstein
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> results/tables/nice_table_V2.tex <==

\begin{table}[h]
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cccccc|cccccc}
\toprule
& \multicolumn{6}{c}{$14 \times 14$ \textbf{Digits}}
& \multicolumn{6}{c}{$28 \times 28$ \textbf{Fashion}}
\vspace{0.2cm}
\\
& {$\mathbf{\Delta \log Z}_{r} \downarrow$}
& {$\mathbf{\Delta \log Z}_{f} \downarrow$}
& {\textbf{ELBO} $\uparrow$}
& {\textbf{EUBO} $\downarrow$}
& {\textbf{ESS}$_r$ $\uparrow$}
& {\textbf{ESS}$_f$ $\uparrow$}
& {$\mathbf{\Delta \log Z}_{r} \downarrow$}
& {$\mathbf{\Delta \log Z}_{f} \downarrow$}
& {\textbf{ELBO} $\uparrow$}
& {\textbf{EUBO} $\downarrow$}
& {\textbf{ESS}$_r$ $\uparrow$}
& {\textbf{ESS}$_f$ $\uparrow$}
\\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
\\
GMMVI
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
\\
SMC
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
\\
AFT
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
\\
CRAFT
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
\\
FAB
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
\\
MCD
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
\\
LDVI
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
\\
CMCD
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
\\
PIS
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
\\
DIS
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
\\
DDS
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
\\
GFN
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
& $0.000\scriptstyle \pm 0.0$ % log Z
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\captionof{table}{Various performance criteria for different methods on the NICE target. We were not able to obtain reasonable results for SNF and PIS. N/A is caused by numerical problems.}
\label{tab:nice}
\end{table}

==> results/tables/stmm40_dim_results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}{\textwidth}
\begin{minipage}[h]{0.36\textwidth}
\centering
 \resizebox{\textwidth}{!}{%
\includegraphics[]{results/entropy/STMM.pdf}
}
\captionof{figure}{EMC for different dimensions}
\end{minipage}
\hfill
\begin{minipage}[h]{0.59\textwidth}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccc|ccc}
\toprule
   & \multicolumn{3}{c|}{\textbf{ELBO} $\uparrow$} & \multicolumn{3}{c}{\textbf{EUBO} $\downarrow$}   \\ 
\textbf{Method}   & $d=2$ & $d=50$  & $d=200$ & $d=2$ & $d=50$  & $d=200$   \\ 
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $\mathbf{0.000 \scriptstyle{\pm 0.000}}$ % ELBO d=2
& $-6.364 \scriptstyle \pm 0.006$ % ELBO d=50
& $-17.386 \scriptstyle \pm 0.016$ % ELBO d=200
& $\mathbf{0.000 \scriptstyle{\pm 0.000}}$ % EUBO d=2
& $914.951 \scriptstyle \pm 0.465$ % EUBO d=50
& $3595.229 \scriptstyle \pm 0.736$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $\mathbf{-0.001 \scriptstyle \pm 0.0}$ % ELBO d=2
& $-4.2 \scriptstyle \pm 0.197$ % ELBO d=50
& $\mathbf{-17.129 \scriptstyle \pm 0.449}$ % ELBO d=200
& $\mathbf{0.001 \scriptstyle \pm 0.0}$ % EUBO d=2
& $119.945 \scriptstyle \pm 37.837$ % EUBO d=50
& $771.698 \scriptstyle \pm 340.564$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NFVI
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % ELBO d=200
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=2
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=50
% & $0.000 \scriptstyle{\pm 0.000}$ % EUBO d=200
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $-0.022 \scriptstyle \pm 0.032$ % ELBO d=2
& $-4.799 \scriptstyle \pm 1.58$ % ELBO d=50
& $-52.85 \scriptstyle \pm 3.418$ % ELBO d=200
& $0.108 \scriptstyle \pm 0.072$ % EUBO d=2
& $\mathbf{7.907 \scriptstyle \pm 2.032}$ % EUBO d=50
& $\mathbf{51.973 \scriptstyle \pm 3.038}$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $-0.017 \scriptstyle \pm 0.072$ % ELBO d=2
& $-9.26 \scriptstyle \pm 3.687$ % ELBO d=50
& $-75.945 \scriptstyle \pm 6.189$ % ELBO d=200
& $83.865 \scriptstyle \pm 39.692$ % EUBO d=2
& $413.699 \scriptstyle \pm 63.8$ % EUBO d=50
& $1084.139 \scriptstyle \pm 84.99$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $0.012 \scriptstyle \pm 0.011$ % ELBO d=2
& $\mathbf{-0.388 \scriptstyle \pm 0.623}$ % ELBO d=50
& $-21.877 \scriptstyle \pm 1.572$ % ELBO d=200
& $170.812 \scriptstyle \pm 68.532$ % EUBO d=2
& $1051.354 \scriptstyle \pm 301.885$ % EUBO d=50
& $2565.726 \scriptstyle \pm 270.621$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SNF
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % IGMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 2
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 50
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM 200
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $-0.181 \scriptstyle \pm 0.1$ % ELBO d=2
& $-35.09 \scriptstyle \pm 3.522$ % ELBO d=50
& $-40.207 \scriptstyle \pm 3.347$ % ELBO d=200
& $0.114 \scriptstyle \pm 0.026$ % EUBO d=2
& $30.875 \scriptstyle \pm 1.719$ % EUBO d=50
& $\infty$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $\mathbf{0.000 \scriptstyle{\pm 0.000}}$ % ELBO d=2
& $-48.428 \scriptstyle \pm 0.408$ % ELBO d=50
& $-288.589 \scriptstyle \pm 0.684$ % ELBO d=200
& $4.859 \scriptstyle \pm 0.029$ % EUBO d=2
& $177.535 \scriptstyle \pm 0.478$ % EUBO d=50
& $641.838 \scriptstyle \pm 0.55$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $-1.538 \scriptstyle \pm 0.017$ % ELBO d=2
& $-91.37 \scriptstyle \pm 0.095$ % ELBO d=50
& $-407.958 \scriptstyle \pm 0.27$ % ELBO d=200
& $0.894 \scriptstyle \pm 0.016$ % EUBO d=2
& $60.519 \scriptstyle \pm 0.17$ % EUBO d=50
& $254.58 \scriptstyle \pm 0.664$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $-1.228 \scriptstyle \pm 0.022$ % ELBO d=2
& $-75.584 \scriptstyle \pm 0.316$ % ELBO d=50
& $-341.382 \scriptstyle \pm 1.146$ % ELBO d=200
& $0.806 \scriptstyle \pm 0.01$ % EUBO d=2
& $51.955 \scriptstyle \pm 0.321$ % EUBO d=50
& $223.143 \scriptstyle \pm 1.069$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $-0.105 \scriptstyle \pm 0.01$ % ELBO d=2
& $-7.745 \scriptstyle \pm 0.062$ % ELBO d=50
& $-26.751 \scriptstyle \pm 0.203$ % ELBO d=200
& $0.784 \scriptstyle \pm 0.097$ % EUBO d=2
& $450.376 \scriptstyle \pm 20.523$ % EUBO d=50
& $2127.893 \scriptstyle \pm 228.31$ % EUBO d=200
\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\captionof{table}{A table beside a figure}
\end{minipage}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> results/tables/wallclock_table.tex <==
\begin{table}
% \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
\label{table:vi_results}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cccccccc}
\begin{tabular}{l|rrrrrrrr}
\toprule
  \textbf{Wall Clock}   & Funnel (10) & Credit (25)& Seeds (26) & Cancer (31) &  Brownian (32) & Ionosphere (35) & Sonar (61)  & LGCP (1600) \\ 
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $16s$ % Funnel
& $17s$ % Credit
& $24s$ % Seeds
& $29.504 \scriptstyle \pm 0.817$ % Cancer
& $18.441 \scriptstyle \pm 6.493$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $1h14m12s$ % Credit
& $53m54s$ % Seeds
& $605.211 \scriptstyle \pm 198.351$ % Cancer
& $6949.556 \scriptstyle \pm 803.798$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
NFVI
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $1s$ % Funnel
& $2s$ % Credit
& $2s$ % Seeds
& $1.774 \scriptstyle \pm 0.055$ % Cancer
& $14.505 \scriptstyle \pm 0.149$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $7s$ % Funnel
& $19s$ % Credit
& $27s$ % Seeds
& $18.759 \scriptstyle \pm 0.163$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $19s$ % Funnel
& $2m17s$ % Credit
& $123.509 \scriptstyle \pm 41.739$ % Seeds
& $321.668 \scriptstyle \pm 27.269$ % Cancer
& $145.856 \scriptstyle \pm 50.596$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SNF
& $4m9s$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $862.612 \scriptstyle \pm 521.58$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $2198.54 \scriptstyle \pm 1175.255$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
PIS
& $29m26s$ % Funnel
& $2h15m25s$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $6459.434 \scriptstyle \pm 753.174$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $23m32s$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $4767.729 \scriptstyle \pm 1240.253$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $1h18m50s$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> results/tables/wasserstein_mmd_table.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[t!]
% % \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
% \begin{center}
% \begin{small}
% \begin{sc}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cc|cc|cc|cc|cc}
% \toprule
% & \multicolumn{2}{c}{\textbf{Seeds}} 
% & \multicolumn{2}{c}{\textbf{Brownian}}  
% & \multicolumn{2}{c}{\textbf{Ionosphere}} 
% & \multicolumn{2}{c}{\textbf{Sonar}}  
% & \multicolumn{2}{c}{\textbf{LGCP}} 
% \vspace{0.2cm}
% \\ 
% & {\textbf{ELBO} $\uparrow$}
% & {\textbf{ESS}$_r$ $\uparrow$}
% & {\textbf{ELBO} $\uparrow$}
% & {\textbf{ESS}$_r$ $\uparrow$}
% & {\textbf{ELBO} $\uparrow$}
% & {\textbf{ESS}$_r$ $\uparrow$}
% & {\textbf{ELBO} $\uparrow$}
% & {\textbf{ESS}$_r$ $\uparrow$}
% & {\textbf{ELBO} $\uparrow$}
% & {\textbf{ESS}$_r$ $\uparrow$}
% \\
% \midrule
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MFVI
% & $-76.74 \scriptstyle \pm 0.006$ % log Z
% & $0.031 \scriptstyle \pm 0.004$ % log Z
% & $-3.856 \scriptstyle \pm 0.014$ % log Z
% & $0.019 \scriptstyle \pm 0.003$ % log Z
% & $-123.417 \scriptstyle \pm 0.035$ % log Z
% & $0.006 \scriptstyle \pm 0.001$ % log Z
% & $-137.7 \scriptstyle \pm 0.027$ % log Z
% & $0.003 \scriptstyle \pm 0.000$ % log Z
% & $383.146 \scriptstyle \pm 0.07$ % log Z
% & $0.001 \scriptstyle \pm 0.000$ % log Z
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MCD
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LDVI
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SMC
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & N/A % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & N/A % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & N/A % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & N/A % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & N/A % log Z
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AFT
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & N/A % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & N/A % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & N/A % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & N/A % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & N/A % log Z
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CRAFT
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & N/A % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & N/A % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & N/A % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & N/A % log Z
% & $0.000\scriptstyle \pm 0.000$ % log Z
% & N/A % log Z
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \bottomrule
% \end{tabular}
% }
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.15in
%     \caption{ELBO values for various target densities. Best results are highlighted using bold font. N/A indicates that reasonable results could not be obtained due to numerical problems. OOM refers to out-of-memory problems.
%     }
%     \vspace{-0.2cm}
% \label{table:elbos}
% \end{table*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t!]
% \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cc|cc|cc|cc|cc}
\toprule
& \multicolumn{2}{c}{\textbf{Funnel}} 
& \multicolumn{2}{c}{\textbf{MoG} $(d=50)$}  
& \multicolumn{2}{c}{\textbf{MoS} $(d=50)$} 
& \multicolumn{2}{c}{$14 \times 14$ \textbf{Digits}}  
& \multicolumn{2}{c}{$28 \times 28$ \textbf{Fashion}} 
\vspace{0.2cm}
\\ 
& {$W_{2}$ $\downarrow$}
& {$\text{MMD}$ $\downarrow$}
& {$W_{2}$ $\downarrow$}
& {$\text{MMD}$ $\downarrow$}
& {$W_{2}$ $\downarrow$}
& {$\text{MMD}$ $\downarrow$}
& {$W_{2}$ $\downarrow$}
& {$\text{MMD}$ $\downarrow$}
& {$W_{2}$ $\downarrow$}
& {$\text{MMD}$ $\downarrow$}
\\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \rowcolor{lightgray}
% $\x_i \sim \pi$
% & $121.027 \scriptstyle \pm 7.368$ % Funnel W2
% & $0.032 \scriptstyle \pm 0.002$ % Funnel MMD
% & $2687.0017 \scriptstyle \pm 323.009$ % MoG W2
% & $0.032 \scriptstyle \pm 0.002$ % MoG MMD
% & $716.99191 \scriptstyle \pm 597.279$ % MoS W2
% & $0.033 \scriptstyle \pm 0.002$ % MoS MMD
% & $109.98888 \scriptstyle \pm 0.348$ % Digits W2
% & $0.033 \scriptstyle \pm 0.001$ % Digits MMD
% & $260.30606 \scriptstyle \pm 2.923$ % Fashion W2
% & $0.031 \scriptstyle \pm 0.002$ % Fashion MMD
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $178.264 \scriptstyle \pm 0.271$ % Funnel W2
& $0.303 \scriptstyle \pm 0.002$ % Funnel MMD
& $39360.196 \scriptstyle \pm 12.49$ % MoG W2
& $0.209 \scriptstyle \pm 0.000$ % MoG MMD
& $2462.26 \scriptstyle \pm 1.009$ % MoS W2
& $0.215 \scriptstyle \pm 0.000$ % MoS MMD
& $254.179 \scriptstyle \pm 0.025$ % Digits W2
& $0.351 \scriptstyle \pm 0.000$ % Digits MMD
& $1327.517 \scriptstyle \pm 0.845$ % Fashion W2
& $0.285 \scriptstyle \pm 0.000$ % Fashion MMD
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $\mathbf{105.620 \scriptstyle \pm 3.472}$ % Funnel W2
& $\mathbf{0.031 \scriptstyle \pm 0.000}$ % Funnel MMD
& $32004.968 \scriptstyle \pm 1069.873$ % MoG W2
& $0.203 \scriptstyle \pm 0.013$ % MoG MMD
& $1255.216 \scriptstyle \pm 296.925$ % MoS W2
& $0.135 \scriptstyle \pm 0.017$ % MoS MMD
& $207.163 \scriptstyle \pm 14.6$ % Digits W2
& $0.373 \scriptstyle \pm 0.042$ % Digits MMD
& $1343.495 \scriptstyle \pm 136.929$ % Fashion W2
& $0.462 \scriptstyle \pm 0.033$ % Fashion MMD
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $149.353 \scriptstyle \pm 2.973$ % Funnel W2
& $0.162 \scriptstyle \pm 0.015$ % Funnel MMD
& $46351.236 \scriptstyle \pm 4.795$ % MoG W2
& $0.631 \scriptstyle \pm 0.000$ % MoG MMD
& $3297.64 \scriptstyle \pm 1372.65$ % MoS W2
& $0.431 \scriptstyle \pm 0.161$ % MoS MMD
& $159.255 \scriptstyle \pm 1.877$ % Digits W2
& $1.168 \scriptstyle \pm 0.008$ % Digits MMD
& $6696.287 \scriptstyle \pm 250.478$ % Fashion W2
& $1.556 \scriptstyle \pm 0.008$ % Fashion MMD
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $145.138 \scriptstyle \pm 6.061$ % Funnel W2
& $0.159 \scriptstyle \pm 0.010$ % Funnel MMD
& $44914.194 \scriptstyle \pm 1154.412$ % MoG W2
& $0.622 \scriptstyle \pm 0.009$ % MoG MMD
& $2648.41 \scriptstyle \pm 301.357$% MoS W2
& $0.395 \scriptstyle \pm 0.082$ % MoS MMD
& $172.685 \scriptstyle \pm 3.661$ % Digits W2
& $1.180 \scriptstyle \pm 0.004$ % Digits MMD
& $6413.147 \scriptstyle \pm 548.66$ % Fashion W2
& $1.538 \scriptstyle \pm 0.010$ % Fashion MMD
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $134.335 \scriptstyle \pm 0.663$ % Funnel W2
& $0.115 \scriptstyle \pm 0.003$ % Funnel MMD
& $43412.038 \scriptstyle \pm 420.996$ % MoG W2
& $0.604 \scriptstyle \pm 0.002$ % MoG MMD
& $1893.926 \scriptstyle \pm 117.324$ % MoS W2
& $0.257 \scriptstyle \pm 0.024$ % MoS MMD
& $151.791 \scriptstyle \pm 11.023$ % Digits W2
& $0.139 \scriptstyle \pm 0.032$ % Digits MMD
& $1413.303 \scriptstyle \pm 11.202$ % Fashion W2
& $0.562 \scriptstyle \pm 0.002$ % Fashion MMD
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $153.894 \scriptstyle \pm 3.916$ % Funnel W2
& $0.032 \scriptstyle \pm 0.000$% Funnel MMD
& $9567.319 \scriptstyle \pm 626.172$ % MoG W2
& $0.073 \scriptstyle \pm 0.005$ % MoG MMD
& $1204.16 \scriptstyle \pm 147.75$ % MoS W2
& $0.093 \scriptstyle \pm 0.014$ % MoS MMD
& $\mathbf{126.863 \scriptstyle \pm 0.581}$ % Digits W2
& $\mathbf{0.129 \scriptstyle \pm 0.003}$ % Digits MMD
& $1186.967 \scriptstyle \pm 263.487$ % Fashion W2
& $0.347 \scriptstyle \pm 0.007$ % Fashion MMD
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $163.317 \scriptstyle \pm 0.101$ % Funnel W2
& $0.228 \scriptstyle \pm 0.001$ % Funnel MMD
& $5026.147 \scriptstyle \pm 40.035$% MoG W2
& $0.043 \scriptstyle \pm 0.000$ % MoG MMD
& $6418.981 \scriptstyle \pm 22.15$ % MoS W2
& $0.256 \scriptstyle \pm 0.000$ % MoS MMD
& $220.71 \scriptstyle \pm 5.547$ % Digits W2
& $0.252 \scriptstyle \pm 0.007$ % Digits MMD
& $1898.472 \scriptstyle \pm 3.783$ % Fashion W2
& $0.327 \scriptstyle \pm 0.002$% Fashion MMD
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& N/A % Funnel W2
& N/A % Funnel MMD
& $5038.42 \scriptstyle \pm 73.777$ % MoG W2
& $0.043 \scriptstyle \pm 0.000$% MoG MMD
& $2919.688 \scriptstyle \pm 103.417$ % MoS W2
& $0.182 \scriptstyle \pm 0.003$ % MoS MMD
& $154.167 \scriptstyle \pm 0.816$ % Digits W2
& $0.133 \scriptstyle \pm 0.000$ % Digits MMD
& $3432.724 \scriptstyle \pm 406.222$ % Fashion W2
& $0.284 \scriptstyle \pm 0.016$ % Fashion MMD
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CMCD
% & $133.342 \scriptstyle \pm 0.995$ % Funnel W2
% & $0.109 \scriptstyle \pm 0.002$ % Funnel MMD
% & $5056.567 \scriptstyle \pm 238.224$ % MoG W2
% & $0.044 \scriptstyle \pm 0.000$ % MoG MMD
% & $\mathbf{626.963 \scriptstyle \pm 21.861}$ % MoS W2
% & $\mathbf{0.061 \scriptstyle \pm 0.003}$ % MoS MMD
% & $167.552 \scriptstyle \pm 1.825$ % Digits W2
% & $0.191 \scriptstyle \pm 0.004$ % Digits MMD
% & $\mathbf{1118.719 \scriptstyle \pm 1.929}$ % Fashion W2
% & $0.363 \scriptstyle \pm 0.001$ % Fashion MMD
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
PIS
& N/A % Funnel W2
& N/A % Funnel MMD
& $10495.164 \scriptstyle \pm 83.207$ % MoG W2
& $0.083 \scriptstyle \pm 0.000$ % MoG MMD
& $2113.172 \scriptstyle \pm 31.172$ % MoS W2
& $0.218 \scriptstyle \pm 0.007$ % MoS MMD
& $186.007 \scriptstyle \pm 0.466$ % Digits W2
& $0.193 \scriptstyle \pm 0.001$ % Digits MMD
& $1484.598 \scriptstyle \pm 5.125$ % Fashion W2
& $\mathbf{0.240 \scriptstyle \pm 0.000}$ % Fashion MMD
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DIS
& $118.947 \scriptstyle \pm 12.81$ % Funnel W2
& $0.159 \scriptstyle \pm 0.036$ % Funnel MMD
& $\mathbf{3044.733 \scriptstyle \pm 464.785}$ % MoG W2
& $\mathbf{0.034 \scriptstyle \pm 0.003}$ % MoG MMD
& $2200.59 \scriptstyle \pm 18.737$ % MoS W2
& $0.155 \scriptstyle \pm 0.001$ % MoS MMD
& $220.392 \scriptstyle \pm 11.69$ % Digits W2
& $0.194 \scriptstyle \pm 0.011$ % Digits MMD
& $3927.754 \scriptstyle \pm 858.922$ % Fashion W2
& $0.282 \scriptstyle \pm 0.019$ % Fashion MMD
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $142.890 \scriptstyle \pm 9.552$ % Funnel W2
& $0.172 \scriptstyle \pm 0.031$ % Funnel MMD
& $5551.107 \scriptstyle \pm 116.403$ % MoG W2
& $0.046 \scriptstyle \pm 0.001$ % MoG MMD
& $2154.884 \scriptstyle \pm 3.861$ % MoS W2
& $0.131 \scriptstyle \pm 0.001$ % MoS MMD
& $188.789 \scriptstyle \pm 2.297$ % Digits W2
& $0.173 \scriptstyle \pm 0.003$ % Digits MMD
& $1811.685 \scriptstyle \pm 24.479$ % Fashion W2
& $0.208 \scriptstyle \pm 0.006$ % Fashion MMD
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GBS
& $178.075 \scriptstyle \pm 0.103$ % Funnel W2
& $0.305 \scriptstyle \pm 0.002$ % Funnel MMD
& $5080.413 \scriptstyle \pm 125.882$ % MoG W2
& $0.043 \scriptstyle \pm 0.001$ % MoG MMD
& $5722.074 \scriptstyle \pm 22.712$ % MoS W2
& $0.232 \scriptstyle \pm 0.000$ % MoS MMD
& $186.436 \scriptstyle \pm 1.834$ % Digits W2
& $0.176 \scriptstyle \pm 0.005$ % Digits MMD
& $1137.399 \scriptstyle \pm 1.819$ % Fashion W2
& $0.246 \scriptstyle \pm 0.003$ % Fashion MMD
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
    \caption{ELBO values for various target densities. Best results are highlighted using bold font. N/A indicates that reasonable results could not be obtained due to numerical problems. OOM refers to out-of-memory problems. \red{Mention target samples.}
    }
    \vspace{-0.2cm}
\label{table:elbos}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[t!]
% % \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
% \begin{center}
% \begin{small}
% \begin{sc}
% % \resizebox{\textwidth}{!}{%
% \begin{tabular}{l}
% \toprule
% \textbf{MFVI} \\
% Learning rate \\ 
% Initial Variance \\
% Iterations \\
% \midrule
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textbf{GMMVI} \\
% Number of initial components \\ 
% Initial Variance \\ 
% Iterations \\
% \midrule
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textbf{GMMVI} \\
% Number of initial components \\ 
% Initial Variance \\ 
% Iterations \\
% \midrule
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \bottomrule
% \end{tabular}
% % }
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.15in
%     \caption{ELBO values for various target densities. Best results are highlighted using bold font. N/A indicates that reasonable results could not be obtained due to numerical problems. OOM refers to out-of-memory problems.
%     }
%     \vspace{-0.2cm}
% \label{table:elbos}
% \end{table*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> results/tables/wasserstein_table.tex <==
\begin{table*}
% \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
\label{table:vi_results}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cccccccc}
\begin{tabular}{l|rrrrrrrr}
\toprule
  $\mathcal{W}_2$   & Funnel (10) & Reacher (10) & Credit (25)& Cancer (31) & GMM (50)& STMM (50) & BMM (50) &  NICE (144) \\ 
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $179.868 \scriptstyle \pm 0.090$ % Funnel
& $1.632 \scriptstyle \pm 0.003$ % Reacher
& $1.2 \scriptstyle \pm 0.0$ % Credit
& $638.483 \scriptstyle \pm 0.601$ % Cancer
& $3198.009 \scriptstyle \pm 1.804$ % GMM
& $2384.929 \scriptstyle \pm 2.932$ % STMM
& $2041.722 \scriptstyle \pm 8.265$ % BMM
& $253.93 \scriptstyle \pm 0.089$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $104.522 \scriptstyle \pm 4.386$ % Funnel
& $0.991 \scriptstyle \pm 0.705$ % Reacher
& $0.021 \scriptstyle \pm 0.001$ % Credit
& $1489.245 \scriptstyle \pm 3.565$ % Cancer
& $2163.398 \scriptstyle \pm 32.639$ % GMM
& $1683.716 \scriptstyle \pm 233.162$ % STMM
& $590.244 \scriptstyle \pm 129.594$ % BMM
& $0.000 \scriptstyle{\pm 0.000}$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NFVI
% & $0.000 \scriptstyle{\pm 0.000}$ % Funnel
% & $0.000 \scriptstyle{\pm 0.000}$ % Reacher
% & $0.000 \scriptstyle{\pm 0.000}$ % Credit
% & $0.000 \scriptstyle{\pm 0.000}$ % Cancer
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $152.839 \scriptstyle \pm 5.083$ % Funnel
& $6.355 \scriptstyle \pm 1.973$ % Reacher
& $13.125 \scriptstyle \pm 0.365$ % Credit
& $1402.045 \scriptstyle \pm 10.298$ % Cancer
& $3851.638 \scriptstyle \pm 370.385$ % GMM
& $2912.389 \scriptstyle \pm 349.041$ % STMMe
& $3437.179 \scriptstyle \pm 551.073$ % BMM
& $139.54 \scriptstyle \pm 14.157$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $145.451 \scriptstyle \pm 5.596$ % Funnel
& $2.853 \scriptstyle \pm 0.034$ % Reacher
& $11.466 \scriptstyle \pm 2.777$ % Credit
& $1005.632 \scriptstyle \pm 136.713$ % Cancer
& $4055.084 \scriptstyle \pm 371.625$ % GMM
& $2645.473 \scriptstyle \pm 434.89$ % STMMre
& $3092.356 \scriptstyle \pm 185.203$ % BMM
& $142.0 \scriptstyle \pm 17.315$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $133.530 \scriptstyle \pm 0.988$ % Funnel
& $3.178 \scriptstyle \pm 0.494$ % Reacher
& $7.682 \scriptstyle \pm 1.652$ % Credit
& $544.798 \scriptstyle \pm 13.556$ % Cancer
& $3235.171 \scriptstyle \pm 42.657$ % GMM
& $2025.494 \scriptstyle \pm 80.104$ % STMM
& $2952.233 \scriptstyle \pm 48.744$ % BMM
& $127.855 \scriptstyle \pm 1.913$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SNF
% & $0.000 \scriptstyle{\pm 0.000}$ % Funnel
% & $0.000 \scriptstyle{\pm 0.000}$ % Reacher
% & $0.000 \scriptstyle{\pm 0.000}$ % Credit
% & $0.000 \scriptstyle{\pm 0.000}$ % Cancer
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FAB
% & $0.000 \scriptstyle{\pm 0.000}$ % Funnel
% & $0.000 \scriptstyle{\pm 0.000}$ % Reacher
% & $0.000 \scriptstyle{\pm 0.000}$ % Credit
% & $0.000 \scriptstyle{\pm 0.000}$ % Cancer
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DDS
% & $0.000 \scriptstyle{\pm 0.000}$ % Funnel
% & $0.000 \scriptstyle{\pm 0.000}$ % Reacher
% & $0.000 \scriptstyle{\pm 0.000}$ % Credit
% & $0.000 \scriptstyle{\pm 0.000}$ % Cancer
% & $0.000 \scriptstyle{\pm 0.000}$ % GMM
% & $0.000 \scriptstyle{\pm 0.000}$ % STMM
% & $0.000 \scriptstyle{\pm 0.000}$ % BMM
% & $0.000 \scriptstyle{\pm 0.000}$ % NICE
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
PIS
& $118.225 \scriptstyle \pm 1.493$ % Funnel
& $30.01 \scriptstyle \pm 0.505$ % Reacher
& $11.386 \scriptstyle \pm 1.508$ % Credit
& $1209.722 \scriptstyle \pm 14.566$ % Cancer
& $3266.044 \scriptstyle \pm 1.642$ % GMM
& $1836.202 \scriptstyle \pm 1.932$ % STMM
& $0.000 \scriptstyle{\pm 0.000}$ % BMM
& $0.000 \scriptstyle{\pm 0.000}$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $170.088 \scriptstyle \pm 0.434$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Reacher
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $2116.131 \scriptstyle \pm 596.076$ % Cancer
& $3307.304 \scriptstyle \pm 191.785$ % GMM
& $1772.169 \scriptstyle \pm 261.068$ % STMM
& $0.000 \scriptstyle{\pm 0.000}$ % BMM
& $0.000 \scriptstyle{\pm 0.000}$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Reacher
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $2761.161 \scriptstyle \pm 59.148$ % GMM
& $1691.826 \scriptstyle \pm 122.879$ % STMM
& $0.000 \scriptstyle{\pm 0.000}$ % BMM
& $144.77 \scriptstyle \pm 15.574$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $120.015 \scriptstyle \pm 0.941$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Reacher
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $3481.447 \scriptstyle \pm 864.24$ % GMM
& $1522.749 \scriptstyle \pm 92.067$ % STMM
& $0.000 \scriptstyle{\pm 0.000}$ % BMM
& $182.736 \scriptstyle \pm 20.349$ % NICE
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> results/utils/commands.tex <==


\newcommand{\elbo}[1]{[
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={function evaluations},
xmajorgrids,
xmin=#1, xmax=1,
xmode=log,
xtick style={color=black},
y grid style={darkgray176},
ylabel={ELBO},
ymajorgrids,
ymin=2, ymax=3,
% ymode=log,
ytick style={color=black}
]}

==> results/utils/table_template.tex <==
\begin{table}
% \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
\label{table:vi_results}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cccccccc}
\begin{tabular}{l|rrrrrrrr}
\toprule
  \textbf{ELBO}   & Funnel (10) & Credit (25)& Seeds (26) & Cancer (31) &  Brownian (32) & Ionosphere (35) & Sonar (61)  & LGCP (1600) \\ 
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MFVI
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
GMMVI
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
NFVI
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SMC
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
AFT
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CRAFT
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SNF
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
FAB
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
PIS
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
MCD
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
LDVI
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& $0.000 \scriptstyle{\pm 0.000}$ % Funnel
& $0.000 \scriptstyle{\pm 0.000}$ % Credit
& $0.000 \scriptstyle{\pm 0.000}$ % Seeds
& $0.000 \scriptstyle{\pm 0.000}$ % Cancer
& $0.000 \scriptstyle{\pm 0.000}$ % Brownian
& $0.000 \scriptstyle{\pm 0.000}$ % Ionosphere
& $0.000 \scriptstyle{\pm 0.000}$ % Sonar
& $0.000 \scriptstyle{\pm 0.000}$ % LGCP
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/discussion.tex <==
\section{Discussion} \label{sec:discussion}
\begin{enumerate}
    \item Flow transport methods work well but are hard to scale due to memory constraints
\end{enumerate}

==> sections/experiments/elbo_vis.tex <==
\subsection{ELBO}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccccc}
  \multicolumn{4}{c}{\includegraphics[width=0.8\textwidth]{figures/visualizations/legend.pdf}} \\
  \includegraphics[width=0.24\textwidth]{results/funnel/elbo_fevals.pdf} &   
  \includegraphics[width=0.24\textwidth]{results/credit/elbo_fevals.pdf} &   
  \includegraphics[width=0.24\textwidth]{results/seeds/elbo_fevals.pdf} &   
  \includegraphics[width=0.24\textwidth]{results/cancer/elbo_fevals.pdf} &   
  \\
   Funnel &   
   Credit &   
  Seeds &   
  Cancer &   
  \\
  \includegraphics[width=0.24\textwidth]{results/brownian/elbo_fevals.pdf} &   
  \includegraphics[width=0.24\textwidth]{results/ionosphere/elbo_fevals.pdf} &   
  \includegraphics[width=0.24\textwidth]{results/sonar/elbo_fevals.pdf} &   
  \includegraphics[width=0.24\textwidth]{results/lgcp/elbo_fevals.pdf} &  
  \\
     Brownian &   
   Ionosphere &   
  Sonar &   
  LGCP &   
  \\
\end{tabular}
\caption{caption}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/experiments/funnel.tex <==
% \subsection{funnel}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure*}
% \setlength{\tabcolsep}{1pt}
% \begin{tabular}{ccccccc}
%   \multicolumn{6}{c}{\includegraphics[width=0.8\textwidth]{figures/visualizations/legend.pdf}} \\
%   \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/mfvi.pdf} &   
%   \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/gmmvi.pdf} &   
%   \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/funnel.pdf} &   
%   \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/smc.pdf} &   
%   \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/aft.pdf} &   
%   \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/craft.pdf} &  
%   \\
%   \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/fab.pdf} &   
%   \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/dds.pdf} &   
%   \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/pis.pdf} &   
%   \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/mcd.pdf} &   
%   \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/ldvi.pdf} &   
%   \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/cmcd.pdf} &  
%   \\
% \end{tabular}
% \caption{caption}
% \end{figure*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/experiments/gmm40.tex <==
\subsection{GMM40}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccccccc}
  \multicolumn{6}{c}{\includegraphics[width=0.8\textwidth]{figures/visualizations/legend.pdf}} \\
  \includegraphics[width=0.16\textwidth]{figures/visualizations/gmm40/pdfs/mfvi.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/gmm40/pdfs/gmmvi.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/gmm40/pdfs/gmm40.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/gmm40/pdfs/smc.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/gmm40/pdfs/aft.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/gmm40/pdfs/craft.pdf} &  
  \\
  \includegraphics[width=0.16\textwidth]{figures/visualizations/gmm40/pdfs/fab.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/gmm40/pdfs/dds.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/gmm40/pdfs/pis.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/gmm40/pdfs/mcd.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/gmm40/pdfs/ldvi.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/gmm40/pdfs/cmcd.pdf} &  
  \\
    \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/mfvi.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/gmmvi.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/funnel.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/smc.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/aft.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/craft.pdf} &  
  \\
  \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/fab.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/dds.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/pis.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/mcd.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/ldvi.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/cmcd.pdf} &  
  \\
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_mfvi.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_gmmvi.pdf} &   
  \includegraphics[width=0.16\textwidth]{example-image} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_smc.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_aft.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_craft.pdf} &  
  \\
  MFVI &
  GMMVI &
  NFVI &
  SMC &
  AFT &
  CRAFT &
  \\
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_fab.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_dds.pdf} &   
  \includegraphics[width=0.16\textwidth]{example-image} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_mcd.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_ldvi.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_cmcd.pdf} &  
  \\
  FAB &
  DDS &
  PIS &
  MCD &
  LDVI &
  CMCD &
  \\
\end{tabular}
\caption{caption}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/experiments/lnz_vis.tex <==
\subsection{Log Normalizer}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccc}
  \multicolumn{3}{c}{\includegraphics[width=0.8\textwidth]{figures/visualizations/legend.pdf}} \\
  \includegraphics[width=0.32\textwidth]{results/funnel/lnz_fevals.pdf} &   
  \includegraphics[width=0.32\textwidth]{results/many_well/lnz_fevals.pdf} &   
  \\
  % % Funnel &   
  % % ManyWell &   
  % % GMM &   
  % % \\
  % \includegraphics[width=0.32\textwidth]{results/stmm50D/lnz_fevals.pdf} &   
  % \includegraphics[width=0.32\textwidth]{results/nice/lnz_fevals.pdf} &   
  % \\
  % STMM &   
  % BMM &   
  % NICE &   
  % \\
\end{tabular}
\caption{caption}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/experiments/nice.tex <==
\subsection{nice}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccccccc}
  \multicolumn{6}{c}{} \\
  % \includegraphics[width=0.8\textwidth]{figures/visualizations/legend.pdf}} \\
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_mfvi.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_gmmvi.pdf} &   
  \includegraphics[width=0.16\textwidth]{example-image} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_smc.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_aft.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_craft.pdf} &  
  \\
  MFVI &
  GMMVI &
  NFVI &
  SMC &
  AFT &
  CRAFT &
  
  \\
  
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_fab.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_dds.pdf} &   
  \includegraphics[width=0.16\textwidth]{example-image} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_mcd.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_ldvi.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/nice/nice_cmcd.pdf} &  
  \\
  FAB &
  DDS &
  PIS &
  MCD &
  LDVI &
  CMCD &
  
  \\
  
\end{tabular}
\caption{caption}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/experiments/robot.tex <==
\subsection{robot}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccccccc}
  \multicolumn{6}{c}{\includegraphics[width=0.8\textwidth]{figures/visualizations/legend.pdf}} \\
  \includegraphics[width=0.16\textwidth]{figures/visualizations/robot/pdfs/mfvi_robot.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/robot/pdfs/gmmvi_robot.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/funnel.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/robot/pdfs/smc_robot.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/robot/pdfs/aft_robot.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/robot/pdfs/craft_robot.pdf} &  
  \\
  \includegraphics[width=0.16\textwidth]{figures/visualizations/robot/pdfs/fab_robot.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/robot/pdfs/dds_robot.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/pis.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/mcd.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/ldvi.pdf} &   
  \includegraphics[width=0.16\textwidth]{figures/visualizations/funnel/pdfs/cmcd.pdf} &  
  \\
\end{tabular}
\caption{caption}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/related_work_cp.tex <==
\section{Related Work} \label{sec:relwork}
% \begin{itemize}
%     \item VI was introduced to treat integration as optimization....
%     \item To make VI scalable, use stochastic optimization, Monte Carlo estimation and a gradient estimator (Reparameterization Trick or Reinforce)
%     \item Early stages: MFVI
%     \item Then Normalizing Flows
%     \item While first seen as separate methods for tackling the same problems, there now exist many approaches that combine these two...
% \end{itemize}

A  variety of Monte Carlo (MC) techniques have been developed to tackle the sampling problem and estimation of $Z$. In particular Annealed Importance Sampling (AIS) \citep{neal2001annealed} and its Sequential Monte Carlo (SMC) extensions \citep{del2006sequential} are often regarded as a gold standard baseline to compute $Z$. These approaches typically construct a proposal distribution with a sequence of Markov chain Monte Carlo (MCMC) transitions that typically target annealed versions of the posterior $\pi$.

Variational inference (VI) is a popular alternative to Markov Chain Monte Carlo (MCMC) and SMC where one considers a flexible family of easy-to-sample distributions $q^{\theta}$ whose parameters $\theta$ are optimized by minimizing a discrepancy, typically the reverse Kullback--Leibler (KL) divergence, i.e.,
\begin{equation*}
    \KL(\model(\x)\|\pi(\x)) = \underbrace{\int_{\rd} \model(\x) \log \frac{\gamma(\x)}{\model(\x)} \dx}_{\text{ELBO}} + \log Z 
\end{equation*}
It is well known that minimizing the reverse KL is equivalent to maximizing the evidence lower bound (ELBO) and that $\text{ELBO} \leq \log Z$ with equality if and only if $\model = \target$.
Typical choices for $q^{\theta}$ include mean-field approximation \citep{Wainwright:2008} or normalizing flows \citep{papamakarios2019normalizing}. To construct more flexible variational distributions \citep{Agakov2004} modeled $q^{\theta}(\x)$ as the marginal of an auxiliary extended distribution; i.e. $q^{\theta}(\x)=\int q^{\theta}(\x,\uu)\mathrm{d}\uu$. As this marginal is typically intractable, $\theta$ is then learned by minimizing a discrepancy measure between $q^{\theta}(\x,\uu)$ and an extended target $p^{\theta}(\x,\uu)=\pi(\x)p^\theta(\uu|\x)$ where $p^\theta(\uu|\x)$ is an auxiliary conditional distribution.

Over recent years, Monte Carlo techniques have been fruitfully combined with variational techniques. For example, AIS can be thought of as a procedure where $q^{\theta}(\x,\uu)$ is the joint distribution of a Markov chain defined by a sequence of MCMC kernels whose final state is $\x$ while $p^{\theta}(\x,\uu)$ is the corresponding AIS extended target \citep{neal2001annealed}. The parameters $\theta$ of these kernels can then be optimized by minimizing $\KL(q^{\theta}||p^{\theta})$ using stochastic gradient descent \citep{wunoe2020stochastic, Geffner:2021,Thin:2021, ZhangAIS2021,doucet2022annealed,geffner2022langevin}.


In what follows we will discuss an auxiliary variables approach where the variables are samples from a Markov chain e.g. $\uu=(\x_{t_1},  \hdots \x_{t_{K-1}})$ and $\x_{t_{K}} = \x$, this approach encompasses the majority of the variational methods that we explore in this work.

\subsection{VI on Path Space}

As previously remarked a powerful tool for characterizing a flexible yet tractable variational distribution is to generate a sequence of random variables such as:
\begin{align}
  \model(\x_{t_1},  \hdots \x_{t_{K}}) = p_0(\x_0) \prod_k F_{k+1 | k} (\x_{t_{k+1}}  | \x_{t_{k}} )
\end{align}
where $F_{k+1 | k} (\x_{t_{k+1}}  | \x_{t_{k}} )$ can be characterized tractably (i.e $F_{k+1 | k} (\x_{t_{k+1}}  | \x_{t_{k}} ) = \mathcal{N}(x_{t_{k+1}} \vert \x_{t_{k}} \!+\! f_{\theta}(\x_{t_k}, t_k)\delta_k, \sigma^2 \delta_k)$). This induces a very flexible marginal distribution for $\x_{t_K}$ however we have no closed form for the marginal density and thus we must work with the augmented KL on the joints:
\begin{align}
 \KL(\model (\x_{t_K})&\vert\vert \pi(\x_{t_K})) \label{eq:path_kl} \\
 &\leq \KL (\model(\x_{t_1},  \hdots \x_{t_{K}})\vert\vert p^{\theta}(\x_{t_1},  \hdots \x_{t_{K}}) )  \nonumber
\end{align}
where we must define backward $p^{\theta}$ process that starts at the target distribution $\pi$ and goes toward $p_0$ or can be trained to reach $p_0$:
\begin{align}
  p^\theta(\x_{t_1},  \hdots \x_{t_{K}}) \propto  \gamma(\x_{T_K}) \prod_k B_{k-1 | k} (\x_{t_{k-1}}  | \x_{t_{k}} )
\end{align}
where as before we can use a Gaussian transition $B_{k-1 | k} (\x_{t_{k-1}}  | \x_{t_{k}} ) = \mathcal{N}(x_{t_{k-1}} \vert \x_{t_{k}} \!+\! g_{\theta}(\x_{t_k}, t_k)\delta_k, \sigma^2 \delta_k)$. A particular common choice for the forward and backwards process in the Gaussian transition setting is $f_\theta = \frac{\sigma^2}{2} (\beta_t^\theta \nabla \ln \pi +  (1-\beta_t^\theta )\nabla \ln p_0)$ and $g_\theta(x,t) =f_\theta(x, T-t)$ which recovers the variational objective for tuning AIS \citep{geffner2022langevin,neal2001annealed,doucet2022annealed}. Note in the small $\delta_k$ limit these processes converge to forward and backwards time SDEs respectively \citep{vargas2023transport, richter2023improved} inducing the path distributions $\mathbb{Q}^{p_0,f}$ and $ \mathbb{P}^{\pi,g}$ respectively which can be thought of as continuous time analogous of $\model$ and $p^\theta$.


Then as illustrated in \citep{richter2023improved,vargas2023transport} depending on how we parametrise $f_\theta$ and $g_\theta$ minimizing $\KL(\mathbb{Q}^{p_0,f}\vert\vert \mathbb{P}^{\pi,g})$ can recover a wide arrange of variational methods we explore in this work such as AFT \citep{arbel2021annealed}, AIS \citep{neal2001annealed}, UHA\citep{Geffner:2021}, MCD \citep{doucet2022annealed}, LDVI\citep{geffner2022langevin}, DDS\citep{vargas2023denoising}, DIS\citep{berner2022optimal} , PIS \citep{zhang2021path}, CMCD \citep{vargas2023transport}. For a deeper exploration on these connections and a more formal introduction, we point the reader to \citep{richter2023improved,vargas2023transport}.

\subsubsection{IS on Path Space}

Once a proposal $q^\theta$ has been learned via minimizing Equation \ref{eq:path_kl} we can carry out importance sampling using the path distributions to estimate $Z$:
\begin{align}
    Z = \mathbb{E}_{\x_{t_0:t_{k}} \sim \model } \Bigg[ \underbrace{\frac{\gamma(\x_{T_K}) \prod_k B_{k-1 | k} (\x_{t_{k-1}} | \x_{t_{k}} )}{ p_0(\x_0) \prod_k F_{k+1 | k} (\x_{t_{k+1}}  | \x_{t_{k}} )}}_{w(\x_{t_0:t_{K}})}\Bigg],
\end{align}
notice that most variational methods we consider optimize a divergence such as Equation \ref{eq:path_kl} which minimizes the variance of the IS weights $w(\x_{t_0:t_{K}})$.



==> supplementary_material/ablations/loss_fn.tex <==
\subsection{Ablation Study: Loss-Function} \label{abl:loss_fn}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Experimental Setup.} \cite{richter2023improved} proposed to use VarGrad \cite{richter2020vargrad} as an alternative to maximizing the ELBO. They showed that VarGrad helps with mode collapse. Here, we compare ELBO and Vargrad on the MoG target for DDS and CMCD for a varying number of dimensions. The results are shown in Table \ref{abl_loss}.

\textbf{Discussion.} We generally observe higher EMC values using VarGrad. However, they come with the cost of significantly higher looseness in the ELBO.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h!]
% \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
\begin{center}
\begin{small}
\begin{sc} {
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|ccc|ccc}
\toprule
   &   & \multicolumn{3}{c|}{\textbf{ELBO} $\uparrow$} & \multicolumn{3}{c}{\textbf{EMC} $\uparrow$}   \\ 
 \textbf{Method} & \textbf{Loss}  & $d=2$ & $d=50$  & $d=200$ & $d=2$ & $d=50$  & $d=200$   \\ 
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DDS
& ELBO
& $\mathbf{-0.612 \scriptstyle \pm 0.019}$ % ELBO d=2
& $\mathbf{-15.598 \scriptstyle \pm 0.106}$ % ELBO d=50
& $\mathbf{-63.101 \scriptstyle \pm 0.253}$ % ELBO d=200
& $\mathbf{0.984 \scriptstyle \pm 0.001}$ % EUBO d=2
& $\mathbf{0.992 \scriptstyle \pm 0.001}$ % EUBO d=50
& $\mathbf{0.983 \scriptstyle \pm 0.002}$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& VarGrad
& $-3.73 \scriptstyle \pm 0.287$ % ELBO d=2
& $-43.533 \scriptstyle \pm 3.134$ % ELBO d=50
& $-210.878 \scriptstyle \pm 14.927$ % ELBO d=200
& $0.954 \scriptstyle \pm 0.008$ % EUBO d=2
& $0.985 \scriptstyle \pm 0.004$ % EUBO d=50
& $\mathbf{0.979 \scriptstyle \pm 0.008}$ % EUBO d=200
\\
\midrule
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
CMCD
& ELBO
& $\mathbf{-3.295 \scriptstyle \pm 0.162}$ % ELBO d=2
& $\mathbf{-13.176 \scriptstyle \pm 0.135}$ % ELBO d=50
& $\mathbf{-56.499 \scriptstyle \pm 3.139}$ % ELBO d=200
& $\mathbf{0.719 \scriptstyle \pm 0.025}$ % EUBO d=2
& $0.0 \scriptstyle \pm 0.0$ % EUBO d=50
& $0.0 \scriptstyle \pm 0.0$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& VarGrad
& $-4.882 \scriptstyle \pm 0.304$ % ELBO d=2
& $-11199.27 \scriptstyle \pm 5658.388$ % ELBO d=50
& $-88696.432 \scriptstyle \pm 42.207$ % ELBO d=200
& $0.36 \scriptstyle \pm 0.07$ % EUBO d=2
& $\mathbf{0.249 \scriptstyle \pm 0.43}$ % EUBO d=50
& $\mathbf{0.989 \scriptstyle \pm 0.001}$ % EUBO d=200
\\
\bottomrule
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
}}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\caption{ELBO and EMC values for different loss functions, that is, ELBO and VarGrad \cite{richter2020vargrad} on the MoG target.}
\label{abl_loss}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> supplementary_material/ablations/network.tex <==
\subsection{Ablation Study: Network Architecture} \label{abl:network}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Experimental Setup.} We compare the network architecture proposed by 
\cite{geffner2022langevin} and \cite{zhang2021path} with different number of hidden layer for MCD \cite{doucet2022annealed} on the MoG target. The main difference between these architectures is that \cite{zhang2021path} use a sinusoidal position embedding for the time while \cite{geffner2022langevin} uses random features for embedding the time. Results are shown in Table \ref{abl_network} 

\textbf{Discussion.} 
% The results comparing \cite{geffner2022langevin} Score Network with \cite{zhang2021path} PIS Network are presented in Table \ref{abl_network} regarding \red{Todo}. 
Surprisingly increasing the number of layer of the networks tends to lead to worse performance in high dimensions. Moreover, the results are mixed as to which time embedding is preferable.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h!]
% \caption{\textbf{VI Results.} $ \log Z$ values for a different number of steps $K$.}
\begin{center}
\begin{small}
\begin{sc} {
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|ccc|ccc}
\toprule
  \textbf{Network} & & \multicolumn{3}{c|}{\textbf{ELBO} $\uparrow$} & \multicolumn{3}{c}{\textbf{EMC} $\uparrow$}   \\ 
\textbf{Architecture} & \textbf{Layers}  & $d=2$ & $d=50$  & $d=200$ & $d=2$ & $d=50$  & $d=200$   \\ 
\midrule
% \multicolumn{10}{c}{\underline{ELBO}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\cite{geffner2022langevin}
& 2
& $-2.384 \scriptstyle \pm 0.059$ % ELBO d=2
& $-878.12 \scriptstyle \pm 8.598$ % ELBO d=50
& $\mathbf{-3610.809 \scriptstyle \pm 278.257}$ % ELBO d=200
& $0.798 \scriptstyle \pm 0.003$ % EUBO d=2
& $0.994 \scriptstyle \pm 0.001$ % EUBO d=50
& $0.988 \scriptstyle \pm 0.0$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& 4
& $-1.875 \scriptstyle \pm 0.057$ % ELBO d=2
& $\mathbf{-823.108 \scriptstyle \pm 21.124}$ % ELBO d=50
& $-4269.703 \scriptstyle \pm 383.171$ % ELBO d=200
& $0.8 \scriptstyle \pm 0.002$ % EUBO d=2
& $0.994 \scriptstyle \pm 0.001$ % EUBO d=50
& $0.988 \scriptstyle \pm 0.001$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& 6
& $\mathbf{-1.856 \scriptstyle \pm 0.145}$ % ELBO d=2
& $-832.888 \scriptstyle \pm 12.31$ % ELBO d=50
& $-5655.213 \scriptstyle \pm 502.352$ % ELBO d=200
& $0.8 \scriptstyle \pm 0.002$ % EUBO d=2
& $0.994 \scriptstyle \pm 0.0$ % EUBO d=50
& $0.989 \scriptstyle \pm 0.0$ % EUBO d=200
\\
\midrule
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\cite{zhang2021path}
& 2
& $-1.545 \scriptstyle \pm 0.039$ % ELBO d=2
& $\mathbf{-1161.208 \scriptstyle \pm 101.582}$ % ELBO d=50
& $\mathbf{-37063.991 \scriptstyle \pm 90.883}$ % ELBO d=200
& $0.801 \scriptstyle \pm 0.001$ % EUBO d=2
& $0.994 \scriptstyle \pm 0.001$ % EUBO d=50
& $0.988 \scriptstyle \pm 0.001$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& 4
& $-1.219 \scriptstyle \pm 0.061$ % ELBO d=2
& $-1281.489 \scriptstyle \pm 104.318$ % ELBO d=50
& $-38194.788 \scriptstyle \pm 166.082$ % ELBO d=200
& $0.801 \scriptstyle \pm 0.002$ % EUBO d=2
& $0.994 \scriptstyle \pm 0.0$ % EUBO d=50
& $0.989 \scriptstyle \pm 0.001$ % EUBO d=200
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& 6
& $\mathbf{-1.139 \scriptstyle \pm 0.023}$ % ELBO d=2
& $-1200.573 \scriptstyle \pm 179.776$ % ELBO d=50
& $-40336.673 \scriptstyle \pm 153.416$ % ELBO d=200
& $0.801 \scriptstyle \pm 0.002$ % EUBO d=2
& $0.994 \scriptstyle \pm 0.0$ % EUBO d=50
& $0.988 \scriptstyle \pm 0.001$ % EUBO d=200
\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
}}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\caption{ELBO and EMC values for network architectures proposed by \cite{geffner2022langevin} and \cite{zhang2021path} with different number of hidden layer for MCD \cite{doucet2022annealed} on the MoG target. The main difference between these architectures is that \cite{zhang2021path} use a sinusoidal position embedding for the time while \cite{geffner2022langevin} use random features.}
\label{abl_network}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> supplementary_material/hparam_table_old.tex <==
\newpage

\begin{table}[hbtp]
\centering


\resizebox{\textwidth}{!}{  

\begin{tabular}{l|c|ccccccccc}
	\toprule 
         \textbf{Methods} / Parameters   & Grid 
         & Funnel & GMM  & STMM  & BMM  & ManyWell  & Reacher & Nice & - & ADLP \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{MFVI}  & \\
        Initial Scale   & \{0.1, 1, 10\} & 1 & 10 & 10 & 0.1 & 0.1 & 0.1 & 10 & - & -\\
        Learning Rate   & $\{ 10^{-2},10^{-3},10^{-4},10^{-5} \}$ & $10^{-2}$ & $10^{-3}$ & $10^{-3}$ & $10^{-2}$ & $10^{-4}$ & $10^{-3}$  & $10^{-3}$ & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{GMMVI}  & \\
        Initial Scale  & \{0.1, 1, 10\} & 0.1 & 10 & 10 & 10 & 10 & 0.1 & -  & - & -\\
        % Prior Scale & \{0.1, 1, 10\} & 0.1 & - & - & - & - & - & -  & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{NFVI}  & \\
        Initial Scale   & \{0.1, 1, 10\} & - & - & - & - & - & - & - & - & -\\
        Learning Rate   & $\{10^{-3},10^{-4},10^{-5} \}$ & - & - & - & - & - & - & - & - & -\\
        % Flow Type & \{\} & - & - & - & - & - & - & - & - & -\\
        Num. Flows & \{\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{SMC}  & \\
        Initial Scale   & \{0.1, 1, 10\} & 1 & 10 & 10 & 1 & 1 & 0.1 & 1 & - & -\\
        HMC stepsize ($\beta \leq 0.5$) & \{0.001, 0.01, 0.05, 0.1, 0.2\}  &  0.001 & 0.2 & 0.2 & 0.1 & 0.2 & 0.01 & 0.1 & - & - \\
        HMC stepsize ($\beta > 0.5$) & \{0.001, 0.01, 0.05, 0.1, 0.2\}  & 0.1 & 0.2 & 0.2 & 0.05 & 0.001 & 0.1 & 0.1 & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{AFT}  & \\
        Initial Scale   & \{0.1, 1, 10\} & 1 & 10 & 10 & 1 & 1 & 0.1 & 1 & - & -\\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-4}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & - & -\\
        % Flow Type & \{\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{CRAFT/SNF}  & \\
        Initial Scale   & \{0.1, 1, 10\} & 1 & 10 & 10 & 0.1 & 1 & - & 1 & - & -\\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & $10^{-4}$ & $10^{-4}$ & $10^{-4}$ & $10^{-4}$ & $10^{-3}$ & $10^{-3}$ & - & -\\
        % Flow Type & \{\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{FAB}  & \\
        Initial Scale   & \{0.1, 1, 10\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % \textbf{SNF}  & \\
        % Initial Scale   & \{0.1, 1, 10\} & 1 & - & - & - & - & - & - & - & -\\
        % Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & - & - & - & - & - & - & - & -\\
        % Flow Type & \{\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{DDS}  & \\
        Initial Scale   & \{0.1, 1, 10\} & - & - & - & - & - & - & - & - & -\\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & - & - & - & - & - & - & - & - & -\\        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{PIS}  & \\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-4}$ & $10^{-3}$ & $10^{-5}$ & $10^{-3}$  & - & -\\        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % \midrule
        % \textbf{ULA}  & \\
        % Initial Scale   & \{0.1, 1, 10\} & 1 & 0.1 & - & - & - & - & - & - & -\\
        % Learning Rate & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & $10^{-3}$ & - & - & - & - & - & - & -\\
        % $q_0$ trainable & \{\text{True, False}\} & True & True & - & - & - & - & - & - & -\\
        % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{UHA/LDVI}  & \\
        Initial Scale   & \{0.1, 1, 10\} & 1 & 10 & 1 & 0.1 & 0.1 & - & 0.1 & - & -\\
        Learning Rate & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-4}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & - & $10^{-3}$ & - & -\\
        % $q_0$ trainable & \{\text{True, False}\} & True & True & True & True & - & - & True & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{ULA/MCD}  & \\
        Initial Scale   & \{0.1, 1, 10\} & 1 & 0.1 & 1 & 1 & 0.1 & - & 10 & - & -\\
        Learning Rate & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & - &  $10^{-3}$ & - & -\\
        % $q_0$ trainable & \{\text{True, False}\} & True & True & True & True & - & - & True & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{CMCD}  & \\
        Initial Scale   & \{0.1, 1, 10\} & 1 & 1 & 10 & - & 1 & - & 10 & - & -\\
        Learning Rate & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & - & $10^{-3}$ & - & $10^{-3}$ & - & -\\
        % $q_0$ trainable & \{\text{True, False}\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\bottomrule
\end{tabular}
}
 \caption{Hyperparameter Selection for all VI algorithms. The `Grid' column indicates the values over which we performed a grid search. The values in the column which are marked with experiment names indicate which values were chosen for the reported results.}\label{hparams}
\vskip -0.15in
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage

\begin{table}[hbtp]
\centering


\resizebox{\textwidth}{!}{  

\begin{tabular}{l|c|ccccccccc}
	\toprule 
         \textbf{Methods} / Parameters   & Grid 
         & Credit & Cancer  & Brownian  & Sonar  & Seeds  & Ionosphere & LGCP & GMM40 & - \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{MFVI}  & \\
        Initial Scale   & \{0.1, 1, 10\} & 0.1 & 10 & 1 & 0.1 & 1 & 1 & 0.1 & - & -\\
        Learning Rate   & $\{ 10^{-2},10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & $10^{-2}$ & $10^{-3}$ & $10^{-3}$ & $10^{-4}$ & $10^{-4}$ & $10^{-3}$ & $10^{-2}$ & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{GMMVI}  & \\
        Initial Scale  & \{0.1, 1, 10\} & 0.1 & 1 & 0.1 & 1 & 0.1 & 10 & NA & - & -\\
        % Prior Scale & \{0.1, 1, 10\} & 0.1 & - & - & - & - & - & -  & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{NFVI}  & \\
        Initial Scale   & \{0.1, 1, 10\} & - & - & - & - & - & - & - & - & -\\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & - & - & - & - & - & - & - & - & -\\
        % Flow Type & \{\} & - & - & - & - & - & - & - & - & -\\
        Num. Flows & \{4,8,16,32\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{SMC}  & \\
        Initial Scale   & \{0.1, 1, 10\}& 0.1 & 1 & 1 & 1 & 1 & 1 & 1 & - & -\\
        HMC stepsize ($\beta \leq 0.5$) & \{0.001, 0.01, 0.05, 0.1, 0.2\} & 0.1 & 0.05 & 0.001 & 0.05 & 0.2 & 0.2 & 0.01 & 0.2& -\\
        HMC stepsize ($\beta > 0.5$) & \{0.001, 0.01, 0.05, 0.1, 0.2\} & 0.1 & 0.01 & 0.05 & 0.001 & 0.05 & 0.2 & 0.2 & 0.001 & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{AFT}  & \\
        Initial Scale   & \{0.1, 1, 10\} & 0.1 & 0.1 & NA & 1 & 1 & 1 & 1 & - & - \\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & $10^{-3}$ & NA & $10^{-3}$ & $10^{-4}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & -\\
        % Flow Type & \{\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{CRAFT/SNF}  & \\
        Initial Scale   & \{0.1, 1, 10\} & 0.1 & 1 & 
1 & 1 &  0.1 & 0.1 & 1 & - & -\\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-4}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & -\\
        % Flow Type & \{\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{FAB}  & \\
        Initial Scale   & \{0.1, 1, 10\} & - & - & - & - & - & - & - & - & -\\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & - & - & - & - & - & - & - & - & -\\
        % Flow Type & \{\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % \textbf{SNF}  & \\
        % Initial Scale   & \{0.1, 1, 10\} & 1 & - & - & - & - & - & - & - & -\\
        % Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & - & - & - & - & - & - & - & -\\
        % Flow Type & \{\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{DDS}  & \\
        Initial Scale   & \{0.1, 1, 10\} & - & - & - & - & - & - & - & - & -\\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & - & - & - & - & - & - & - & - & -\\        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{PIS}  & \\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-4}$ & $10^{-4}$ & $10^{-4}$ & $10^{-3}$ & $10^{-3}$ & $10^{-4}$ & Prob & $10^{-3}$ & -\\ 
       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % \midrule
        % \textbf{ULA}  & \\
        % Initial Scale   & \{0.1, 1, 10\} & 1 & 0.1 & - & - & - & - & - & - & -\\
        % Learning Rate & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & $10^{-3}$ & - & - & - & - & - & - & -\\
        % $q_0$ trainable & \{\text{True, False}\} & True & True & - & - & - & - & - & - & -\\
        % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{UHA/LDVI}  & \\
        Initial Scale   & \{0.1, 1, 10\} & 0.1 & 0.1 & 1 & 1 & 0.1 & 0.1 & 0.1 & - & -\\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & -\\
        % $q_0$ trainable & \{\text{True, False}\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{ULA/MCD}  & \\
        Initial Scale   & \{0.1, 1, 10\} & 0.1 & 0.1 & 1 & 0.1 & 0.1 & 1 & 1 & - & -\\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-4}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & -\\
        % $q_0$ trainable & \{\text{True, False}\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{CMCD}  & \\
        Initial Scale   & \{0.1, 1, 10\} & P & 0.1 & 0.1 & 0.1 & 0.1 & 1 & 1 & - & -\\
        Learning Rate & $\{ 10^{-3},10^{-4},10^{-5} \}$ & - & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & -\\
        % $q_0$ trainable & \{\text{True, False}\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\bottomrule
\end{tabular}
}
 \caption{Hyperparameter Selection for all VI algorithms. The `Grid' column indicates the values over which we performed a grid search. The values in the column which are marked with experiment names indicate which values were chosen for the reported results.}\label{hparams2}
\vskip -0.15in
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage

\begin{table}[hbtp]
\centering


\resizebox{\textwidth}{!}{  

\begin{tabular}{l|c|ccccccccc}
	\toprule 
         \textbf{Methods} / Parameters   & Grid 
         & GMM40 & GMM  & STMM  & BMM  & NICE  & - & - & - & - \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{MFVI}  & \\
        Learning Rate   & $\{ 10^{-2},10^{-3},10^{-4},10^{-5} \}$ & $10^{-2}$ & $10^{-3}$ & $10^{-3}$  & $10^{-3}$  & $10^{-3}$ & - & - & - & -\\

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{NFVI}  & \\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & - & - & - & - & - & - & - & - & -\\
        % Flow Type & \{\} & - & - & - & - & - & - & - & - & -\\
        Num. Flows & \{4,8,16,32\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{SMC}  & \\
        HMC stepsize ($\beta \leq 0.5$) & \{0.001, 0.01, 0.05, 0.1, 0.2\} & 0.2 & 0.2 & 0.2 & 0.2 & 0.2 & - & - & - & -\\
        HMC stepsize ($\beta > 0.5$) & \{0.001, 0.01, 0.05, 0.1, 0.2\}& 0.001 & 0.2 & 0.2 & 0.001 &  0.1  & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{AFT}  & \\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & $10^{-3}$ & $10^{-4}$ & $10^{-4}$  & $10^{-3}$ & - & - & - & -\\
        % Flow Type & \{\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{CRAFT/SNF}  & \\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & $10^{-3}$ & $10^{-4}$ & $10^{-3}$  & $10^{-3}$ & - & - & - & -\\
        % Flow Type & \{\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{FAB}  & \\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & - & - & - & - & - & - & - & - & -\\
        % Flow Type & \{\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % \textbf{SNF}  & \\
        % Initial Scale   & \{0.1, 1, 10\} & 1 & - & - & - & - & - & - & - & -\\
        % Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & - & - & - & - & - & - & - & -\\
        % Flow Type & \{\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{DDS}  & \\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & - & - & - & - & - & - & - & - & -\\
        \midrule
        \textbf{PIS}  & \\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & $10^{-4}$ & $10^{-3}$ & - & - & - & -\\
       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % \midrule
        % \textbf{ULA}  & \\
        % Initial Scale   & \{0.1, 1, 10\} & 1 & 0.1 & - & - & - & - & - & - & -\\
        % Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & - & - & - & - & - & - & - & - & -\\
        % $q_0$ trainable & \{\text{True, False}\} & True & True & - & - & - & - & - & - & -\\
        % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{UHA/LDVI}  & \\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & P & $10^{-3}$ & - & - & - & -\\
        % $q_0$ trainable & \{\text{True, False}\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{ULA/MCD}  & \\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & P & $10^{-3}$ & - & - & - & -\\
        % $q_0$ trainable & \{\text{True, False}\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \textbf{CMCD}  & \\
        Learning Rate   & $\{ 10^{-3},10^{-4},10^{-5} \}$ & $10^{-3}$ & $10^{-3}$ & $10^{-3}$ & P & $10^{-3}$  & - & - & - & -\\
        % $q_0$ trainable & \{\text{True, False}\} & - & - & - & - & - & - & - & - & -\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\bottomrule
\end{tabular}
}
 \caption{Hyperparameter Selection for all VI algorithms. The `Grid' column indicates the values over which we performed a grid search. The values in the column which are marked with experiment names indicate which values were chosen for the reported results.}\label{hparams2}
\vskip -0.15in
\end{table}
